Tao: A Learning Framework for Adaptive Nearest Neighbor Search using Static Features Only

Approximate nearest neighbor (ANN) search is a fundamental problem in areas such as data management,information retrieval and machine learning. Recently, Li et al. proposed a learned approach named AdaptNN to support adaptive ANN query processing. In the middle of query execution, AdaptNN collects a number of runtime features and predicts termination condition for each individual query, by which better end-to-end latency is attained. Despite its efficiency, using runtime features complicates the learning process and leads to performance degradation. Radically different from AdaptNN, we argue that it is promising to predict termination condition before query exetution. Particularly, we developed Tao, a general learning framework for Terminating ANN queries Adaptively using Only static features. Upon the arrival of a query, Tao first maps the query to a local intrinsic dimension (LID) number, and then predicts the termination condition using LID instead of runtime features. By decoupling prediction procedure from query execution, Tao eliminates the laborious feature selection process involved in AdaptNN. Besides, two design principles are formulated to guide the application of Tao and improve the explainability of the prediction model. We integrate two state-of-the-art indexing approaches, i.e., IMI and HNSW, into Tao, and evaluate the performance over several million to billion-scale datasets. Experimental results show that, in addition to its simplicity and generality , Tao achieves up to 2.69x speedup even compared to its counterpart, at the same high accuracy targets.

==> icde2022-reviews_files/appCore <==
var app=window.app||{};(function(n){"use strict";n.settings={};n.settings.pageSize=50;n.settings.progressIndicatorId="progressIndicator";n.settings.progressIndicatorTimeout=100;n.settings.messagesBlockId="messages";n.settings.messagesShowTime=3e3;n.settings.stackMessages=!0;n.settings.autoSaveDelay=6e4;n.settings.queryProgressDelay=3e3;n.settings.submissionWelcomeInstructionChars=1e4;n.settings.reviewWelcomeInstructionChars=4e3;n.settings.metaReviewWelcomeInstructionChars=4e3})(window.app),function(n){"use strict";RegExp.escape=function(n){return n.replace(/[-[\]{}()*+?.,\\^$|#\s]/g,"\\$&")};String.prototype.format=function(t){var i=this,r=function(n,t){var r=new RegExp(RegExp.escape("{"+n+"}"),"g");i=i.replace(r,t)};return n.isArray(t)||n.isPlainObject(t)?n.each(t,r):n.each(arguments,r),i};String.prototype.htmlEncode=function(){return document.createElement("a").appendChild(document.createTextNode(this)).parentNode.innerHTML};String.prototype.htmlMultiLineEncode=function(){return this.htmlEncode().replace(/\r\n|\r|\n/g,"<br/>")};String.prototype.htmlMultiLine=function(){return this.replace(/\r\n|\r|\n/g,"<br/>")};String.prototype.zeroPadding=function(n){for(var t="",i=0;i<n-this.length;i++)t+="0";return t+this};Date.prototype.format=function(n){var t=this;return n.replace(/(yyyy|mm|dd|hh|nn|ss|fff)/g,function(n){switch(n.toLowerCase()){case"yyyy":return t.getFullYear();case"mm":return(t.getMonth()+1).toString().zeroPadding(2);case"dd":return t.getDate().toString().zeroPadding(2);case"hh":return t.getHours().toString().zeroPadding(2);case"nn":return t.getMinutes().toString().zeroPadding(2);case"ss":return t.getSeconds().toString().zeroPadding(2);case"fff":return t.getMilliseconds().toString().zeroPadding(3)}})};Boolean.prototype.toYesNo=function(){var n=this;return n?"Yes":"No"};Number.prototype.formatSize=function(){function t(n){return n=n.toFixed(1),n.substr(n.length-2)==".0"?n.substr(0,n.length-2):n}var n=this;return(n/1073741824).toFixed(1)>=1?t(n/1073741824)+" Gb":(n/1048576).toFixed(1)>=1?t(n/1048576)+" Mb":(n/1024).toFixed(1)>=1?t(n/1024)+" Kb":n+" byte"+(n>1?"s":"")};Array.prototype.remove=function(n){for(var t=0;t<this.length;t++)this[t]===n&&(this.splice(t,1),t--);return this}}(window.jQuery),function(n,t,i){"use strict";function r(n){var t=n.parent();t.addClass("active")}var u=n('ul.nav > li > a[href^="'+t.pathname+'"]');u.length>0?r(u):n.each(n("ul.nav > li > a[href]"),function(){var u=n(this),f=u.attr("href").split(/\{\d+\}/),i="";if(n.each(f,function(){i+=RegExp.escape(this)+".+"}),i="^"+i.substr(0,i.length-2)+"$",new RegExp(i).test(t.pathname)){r(u);return}});i.highlightMenu=function(t){var i=n('ul.nav > li > a[href*="'+t+'"]');r(i)}}(window.jQuery,window.location,window.app)

==> icde2022-reviews_files/appScripts <==
function ExternalReviewModel(n,t){var i=this;i.id=n.Id;i.title=n.Title;i.abstract=n.Abstract;i.track=n.Track;i.reviewId=n.ReviewId;i.filesUploaded=n.FilesUploaded;i.reviewingEnabled=n.ReviewingEnabled;i.firstName=n.FirstName;i.lastName=n.LastName;i.email=n.Email;i.userId=n.UserId;i.downloadLink=function(){return t.submissionFile.format(i.id)};i.editReviewUrl=function(){return i.reviewId?t.reviewDetails.format(i.reviewId):t.reviewCreate.format(i.id,i.userId)};i.viewReviewUrl=function(){return i.reviewId?t.reviewView.format(i.reviewId):null};i.viewUrl=function(){return t.submissionSummary.format(i.id)}}function ExternalReviewPage(n,t){var i=this;i.$element=$(n);i.conference=window.cmt3.conference.name;i.page=ko.observable(1);i.top=ko.observable(25);i.sort=ko.observable("Id");i.controller="ExternalReviewModels";i.filters=[];i._total=ko.observable(0);i.selected=ko.observable(0);i.externalReviewModels=ko.observableArray();i.listen();i.Pager=ko.pager(i.selected,i.top);i.Pager().CurrentPage.subscribe(function(){i.page(i.Pager().CurrentPage());i.show()});i.pageUrls=t}(function(n,t){"use strict";t&&(t.jsonHandler&&(t.jsonHandler.recognizeDates=!0),n.OData||(n.OData=t))})(window,window&&window.odatajs&&window.odatajs.oData),function(n,t){"use strict";n.cookies={getValue:function(n){return!n||!this.contains(n)?null:unescape(t.cookie.replace(new RegExp("(?:^|.*;\\s*)"+escape(n).replace(/[\-\.\+\*]/g,"\\$&")+"\\s*\\=\\s*((?:[^;](?!;))*[^;]?).*"),"$1"))},setValue:function(n,i,r,u,f,e){if(n&&!/^(?:expires|max\-age|path|domain|secure)$/.test(n)){var o="";if(r)switch(typeof r){case"number":o="; max-age="+r;break;case"string":o="; expires="+r;break;case"object":r.hasOwnProperty("toGMTString")&&(o="; expires="+r.toGMTString())}t.cookie=escape(n)+"="+escape(i)+o+(f?"; domain="+f:"")+(u?"; path="+u:"")+(e?"; secure":"")}},remove:function(n){if(n&&this.hasItem(n)){var i=new Date;i.setDate(i.getDate()-1);t.cookie=escape(n)+"=; expires="+i.toGMTString()+"; path=/"}},contains:function(n){return new RegExp("(?:^|;\\s*)"+escape(n).replace(/[\-\.\+\*]/g,"\\$&")+"\\s*\\=").test(t.cookie)}}}(window.app,window.document),function(n){"use strict";n.enums={userRole:{author:"Author",reviewer:"Reviewer",externalReviewer:"External Reviewer",metaReviewer:"Meta-Reviewer",seniorMetaReviewer:"Senior Meta-Reviewer",trackChair:"Track Chair",reference:"Reference",chair:"Chair",proceedingEditor:"Proceeding Editor",administrator:"Administrator"},userRoleCodeRoleMap:{CH:"Chair",AD:"Administrator",AT:"Author",ER:"External Reviewer",MR:"Meta-Reviewer",SM:"Senior Meta-Reviewer",RV:"Reviewer",TC:"Track Chair",RF:"Reference",PE:"Proceeding Editor",AL:"All",NS:"Not Set"},questionType:{agreement:1,comment:2,options:3,optionsWithValue:4,optionsWithUserInput:5,optionsWithOther:6},optionsType:{radioButtonList:1,checkboxList:2,dropDown:3,listBox:4},formType:{submission:1,review:2,cameraready:3,authorfeedback:4,metareview:5,chairnote:6,reproducibility:7,metareviewernote:8,seniormetareviewernote:9,reviewernote:10,userinformation:11},aggregateType:{average:1,minimum:2,maximum:4,spread:8},objectType:{track:"Track",session:"Session",submission:"Submission"},activityType:{newPaperSubmission:1,editPaperSubmission:2,reviewSubmission:3,reviewDiscussion:4,authorNotification:5,cameraReadySubmission:6,reviewerBidding:7,authorFeedback:8,supplementaryMaterial:9,metaReviewSubmission:10,metaReviewerBidding:11},httpStatusCodes:{success:{ok:200,noContent:204},failure:{badRequest:400,notFound:404,conflict:409}},disputedConflictStatus:{NotDisputed:"Not Disputed",Pending:"Pending",Kept:"Conflict Kept",Deleted:"Conflict Deleted"},hasFlag:function(n,t){return(n&t)==t},reviewersStatPageMode:{metaReviewer:"metaReviewer",chair:"chair"},inviteType:{reviewer:0,metaReviewer:1,seniorMetaReviewer:2},trackUserType:{reviewer:0,metaReviewer:1,seniorMetaReviewer:2},bidOptions:{1:"Not Entered",2:"Not Willing",3:"In A Pinch",4:"Willing",5:"Eager"},assignmentType:{reviewer:0,metaReviewer:1,seniorMetaReviewer:2},externalProfile:{googleScholar:"https://scholar.google.com/citations?user={0}",semanticScholar:"https://www.semanticscholar.org/author/{0}",dblp:"https://dblp.org/pid/{0}"},inviteStatusOptions:["NotResponded","Accepted","Declined"],inviteStatusOptionsSubstitutions:{NotResponded:"Not responded",Accepted:"Accepted",Declined:"Declined"},iThenticateFileStatuses:["NotSent","Sent","Pending","Done","Error"],iThenticateFileStatusSubstitutions:{NotSent:"Not Sent",Sent:"Sent",Pending:"Pending",Done:"Done",Error:"Error"},noteType:{reviewer:0,metaReviewer:1,seniorMetaReviewer:2,chair:3}}}(window.app),function(n,t,i,r,u,f){"use strict";var e={log:function(){if(f){var n=Function.prototype.bind.call(f.log,f);n.apply(f,arguments)}},error:function(){if(f){var n=Function.prototype.bind.call(f.error,f);n.apply(f,arguments)}},checkConsoleForDetailsMessage:function(){return""}};i.defaultError=function(t){var i,r,u;t.response.body?t.response.headers["Content-Type"]&&t.response.headers["Content-Type"].indexOf("text/html")!=-1?(i="{0} ({1}).".format(t.response.statusText,t.response.statusCode)+e.checkConsoleForDetailsMessage(),r=t.response.body,u="html"):(i="{0} ({1}):".format(t.response.statusText,t.response.statusCode),r=n.getODataErrorMessage(t).message+e.checkConsoleForDetailsMessage(),u="text"):(i="",r="Server returned empty response.",u="text");n.addMessage(r,i,"error",u);e.error(t)};n.processXmlHttpRequestError=function(t){var i="{0} ({1}):".format(t.statusText,t.status),r=n.getWebApiErrorMessage(t)+e.checkConsoleForDetailsMessage();n.addMessage(r,i,"error");e.error(t)};r(t).ajaxError(function(t,i,r){if(!i.errorHandled){var f="{0} ({1}):".format(i.statusText,i.status),u="";i.responseJSON!=undefined&&i.responseJSON.Message!=undefined&&(u+=i.responseJSON.Message);u+=e.checkConsoleForDetailsMessage();n.addMessage(u,f,"error");e.log(t,i,r)}});n.getODataErrorMessage=function(n){var i=n.message||n.response.statusText,f="",r,t;return i[i.length-1]!="."&&(i+="."),r=n.response.headers["Content-Type"],r||(r=n.response.headers["content-type"]),u!=undefined&&r&&r.indexOf("json")!=-1&&(t=u.parse(n.response.body).error,t&&(t.code&&(f=t.code),t.message&&(i=t.message),t.innererror&&(i+=" "+t.innererror.message))),{errorCode:f,message:i}};n.getWebApiErrorMessage=function(n){var t=n.responseText||n.response,i;if(u!=undefined){try{i=u.parse(t)}catch(r){return t}i.Message&&(t=i.Message,i.ExceptionMessage&&(t+=" "+i.ExceptionMessage))}return t};n.processException=function(t){var i=t.toString();i[i.length-1]!="."&&(i+=".");i+=e.checkConsoleForDetailsMessage();n.addMessage(i,null,"error");e.error(t.toString());e.log(t.stack)}}(window.app,window.document,window.OData,window.jQuery,window.JSON,window.console),function(n,t){"use strict";ko.validation.init({insertMessages:!1,errorClass:null,errorElementClass:null,errorMessageClass:null,stubProperty:null});ko.validation.localize({required:"Value is required.",min:"Value must be greater than or equal to {0}.",max:"Value must be less than or equal to {0}.",minLength:"Value must contain at least {0} characters.",maxLength:"Value must contain no more than {0} characters.",pattern:"Value is incorrect.",step:"Value must increment by {0}.",email:"Value must be email address.",date:"Value must be a date.",dateISO:"Value must be a date.",number:"Value must be a number.",digit:"Value must be a whole number.",phoneUS:"Value must be a phone number.",equal:"Values must equal.",notEqual:"Values must not equal.",unique:"Value must be unique."});ko.validation.rules.requiredCheckbox={validator:function(n){return n?!0:!1}};ko.validation.registerExtenders();ko.bindingHandlers.allowBindings={init:function(n,t){var i=ko.utils.unwrapObservable(t());return{controlsDescendantBindings:!i}}};ko.virtualElements.allowedBindings.allowBindings=!0;ko.bindingHandlers.formatChildLinks={update:function(n,i){var r=i(),u;if(r!=null){if(t.isArray(r))for(u=0;u<r.length;u++)r[u]=ko.unwrap(r[u]);else r=[ko.unwrap(r)];t(n).find("a").each(function(){var n=t(this);n.data("href")==undefined&&n.data("href",n.attr("href"));n.attr("href",n.data("href").format(r))})}}};ko.bindingHandlers.fadeVisible={init:function(n,i){var r=i();t(n).toggle(ko.unwrap(r))},update:function(n,i){var r=i();ko.unwrap(r)?t(n).fadeIn():t(n).fadeOut()}};ko.bindingHandlers.slideDownVisible={init:function(n,i){var r=i();t(n).toggle(ko.unwrap(r))},update:function(n,i){var r=i();ko.unwrap(r)?t(n).slideDown():t(n).slideUp()}};ko.bindingHandlers.valueWithInit={init:function(n,t,i,r){var u=t(),f=n.value;u(f);ko.bindingHandlers.value.init(n,t,i,r)},update:ko.bindingHandlers.value.update};ko.bindingHandlers.iframeHtml={update:function(n,t){var i=t();i=ko.unwrap(i);n.contentDocument.write(i)}};ko.bindingHandlers.triggerClickOnEnterKey={init:function(n){t(n).keydown(function(i){var r=i.which?i.which:i.keyCode;r===13&&t(n).click()})}};ko.bindingHandlers.tooltip={init:function(n,i){var u=ko.utils.unwrapObservable(i()),r={};ko.utils.extend(r,ko.bindingHandlers.tooltip.options);ko.utils.extend(r,u);t(n).tooltip(r);ko.utils.domNodeDisposal.addDisposeCallback(n,function(){t(n).tooltip("destroy")})},options:{placement:"right",trigger:"hover",html:!0}};ko.applyBindingsAndShow=function(t,i){var r=n.getElementById(i);if(!r)throw new Error("Element with id='{0}' does not exist.".format(i));ko.applyBindings(t,r);r.style.display="block"};ko.observableArray.fn.withPausing=function(){return this.pauseNotifications=!1,this.suspendNotifications=function(){this.pauseNotifications=!0},this.resumeNotifications=function(){this.pauseNotifications=!1},this.notifySubscribers=function(){this.pauseNotifications||ko.subscribable.fn.notifySubscribers.apply(this,arguments)},this};ko.observable.fn.withPausing=function(){return this.pauseNotifications=!1,this.suspendNotifications=function(){this.pauseNotifications=!0},this.resumeNotifications=function(){this.pauseNotifications=!1},this.notifySubscribers=function(){this.pauseNotifications||ko.subscribable.fn.notifySubscribers.apply(this,arguments)},this};ko.setupWizardSteps=function(n,t){function u(n){i.currentStep(n);i.hideSteps();i.steps[i.currentStep()].isVisible(!0);i.afterNextStepInvoked!=null&&i.afterNextStepInvoked()}function f(n){i.currentStep(n);i.hideSteps();i.steps[i.currentStep()].isVisible(!0);i.afterPrevStepInvoked!=null&&i.afterPrevStepInvoked()}var i=n,r;for(i.steps=[],i.backButtonTitles=[],i.fwdButtonTitles=[],i.currentStep=ko.observable(-1),i.mayGoFwd=null,i.mayGoBack=null,i.beforeNextStepInvoked=null,i.afterNextStepInvoked=null,i.beforePrevStepInvoked=null,i.afterPrevStepInvoked=null,r=0;r<t;r++)i.steps[r]={isVisible:ko.observable(!1),skip:ko.observable(!1)};i.startOver=function(){i.hideSteps();i.currentStep(-1);i.nextStep()};i.nextStep=function(){var n=i.nextStepNum();n!=null&&(i.beforeNextStepInvoked==null||i.beforeNextStepInvoked(function(){u(n)}))&&u(n)};i.prevStep=function(){var n=i.prevStepNum();n!=null&&(i.beforePrevStepInvoked==null||i.beforePrevStepInvoked(function(){f(n)}))&&f(n)};i.hideSteps=function(){for(var n=0;n<i.steps.length;n++)i.steps[n].isVisible(!1)};i.prevStepNum=ko.computed(function(){var n=i.currentStep();do n--;while(n>=0&&i.steps[n].skip());return n>=0?n:null});i.nextStepNum=ko.computed(function(){var n=i.currentStep();do n++;while(n<t&&i.steps[n].skip());return n<t?n:null});i.canGoBack=ko.computed(function(){return i.prevStepNum()!=null&&(i.mayGoBack==null||i.mayGoBack())});i.canGoFwd=ko.computed(function(){return i.nextStepNum()!=null&&(i.mayGoFwd==null||i.mayGoFwd())});i.backButtonTitle=ko.computed(function(){var n=i.backButtonTitles[i.currentStep()];return n===undefined||n==null?"Previous":n});i.fwdButtonTitle=ko.computed(function(){var n=i.fwdButtonTitles[i.currentStep()];return n===undefined||n==null?"Next":n})};ko.extenders.validateBeforeSet=function(n,t){n.validationEnabled=!1;var i=ko.pureComputed({read:function(){return this()},write:function(n){var i=this();!this.validationEnabled||t(n)?(this(n),this.notifySubscribers(n)):this.notifySubscribers(i)},owner:n}).extend({notify:"always"});return i(n()),n.validationEnabled=!0,i.enableValidation=function(){n.validationEnabled=!0},i.disableValidation=function(){n.validationEnabled=!1},i};ko.extenders.trackChanges=function(n,t){return t&&(n.isChanged=ko.observable(!1),n.originalValue=n(),n.subscribe(function(t){n.isChanged(t!=n.originalValue)})),n};ko.bindingHandlers.editableInline={init:function(n,i,r,u,f){function a(){h!=e.text()&&(e.changed&&typeof e.changed=="function"&&e.changed.call(f.$data,f.$data,h,e.text()),h=e.text())}var v=ko.utils.unwrapObservable(i()),e={},h;ko.utils.extend(e,ko.bindingHandlers.editableInline.options);ko.utils.extend(e,v);var l=t(n),c=t("<"+e.viewer.tag+" />",e.viewer.attr).addClass("inline-editable"),s=t("<span />"),y=t("<i />").addClass("icon-edit"),o=t("<"+e.editor.tag+" />",e.editor.attr);c.append(s);c.append(y);l.append(c);l.append(o);ko.applyBindingsToNode(s.get(0),{text:e.text});ko.applyBindingsToNode(o.get(0),{value:e.text});h=e.text;c.click(function(){h=e.text();o.width(s.width());s.hide();o.show();o.focus()});o.blur(function(){s.show();o.hide();a()});o.keypress(function(n){n.keyCode===13&&(s.show(),o.hide(),a())})},options:{viewer:{tag:"div",attr:{}},editor:{tag:"input",attr:{type:"text",style:"display: none"}},changed:null}}}(window.document,window.jQuery),function(n){"use strict";function t(){return!0}function i(n,t){var r=n[t]&&n[t].isAutoMapped&&n[t].isAutoMapped(),i;if(r)return!0;if(n.__autoMappedFields__)for(i=0;i<n.__autoMappedFields__.length;i++)if(n.__autoMappedFields__[i]==t)return!0;return!1}ko.subscribable.fn.autoMap=function(){return this.isAutoMapped=t,this};n.autoMap=function(n,r){var f,e,u,o,s;if(n===undefined)return{isAutoMapped:t};n===null&&(n={});f=r===undefined;f&&(r={});e=[];for(u in n)i(n,u)&&(o=u.substr(0,1).toUpperCase()+u.substr(1,u.length),f?r[o]=ko.unwrap(n[u]):(s=r===null?null:r[o]===undefined?ko.unwrap(r[u]):r[o],ko.isObservable(n[u])?(n[u](s),n[u].isModified&&n[u].isModified(!1)):(n[u]=s,e.push(u))));return e.length>0&&(n.__autoMappedFields__=e),f?r:n}}(window.app),function(n){function i(n,t){this.displayName=n;this.operator=t;this.getFilterString=function(n,i){return typeof i=="string"&&(i="'"+i+"'"),n+" "+t+" "+i}}function r(n,t,r){i.call(this,n,t);r=r||"true";this.getFilterString=function(n,i){return typeof i=="string"&&(i="'"+i+"'"),"("+t+"("+n+","+i+") eq "+r+")"}}var t=this;t.operators={equal:new i("equal to","eq"),is:new i("is","eq"),notEqual:new i("not equal to","ne"),isNot:new i("is not","ne"),greaterThan:new i("greater than","gt"),greaterThanOrEqual:new i("greater than or equal","ge"),lessThan:new i("less than","lt"),lessThanOrEqual:new i("less than or equal","le"),contains:new r("contains","contains"),doesNotContain:new r("does not contain","contains","false"),startsWith:new r("starts with","startswith"),doesNotStartWith:new r("does not start with","startswith","false"),endsWith:new r("ends with","endswith"),doesNotEndWith:new r("does not end with","endswith","false")};t.Filter=function(n,t,i){var r=this;r.options=[];r.property=n;r.operators=t;r.operator=ko.observable(i&&i.operator&&r.operators.find(function(n){return n===i.operator}));r.value=ko.observable(i&&i.value);r.getValue=function(){return r.value()||""};this.getFilterString=function(){var n=this.operator(),t;return n?(t=r.getValue(),t?n.getFilterString(r.property,r.getValue()):null):""}};t.NumericFilter=function(n,i){var r=this,u=[t.operators.equal,t.operators.notEqual,t.operators.greaterThan,t.operators.greaterThanOrEqual,t.operators.lessThan,t.operators.lessThanOrEqual];t.Filter.call(r,n,u,i);r.getValue=function(){return parseInt(r.value())||0}};t.StringFilter=function(n,i){var r=[t.operators.contains,t.operators.doesNotContain,t.operators.equal,t.operators.notEqual,t.operators.startsWith,t.operators.doesNotStartWith,t.operators.endsWith,t.operators.doesNotEndWith];t.Filter.call(this,n,r,i)};t.OptionsFilter=function(n,i){var r=this,u=[t.operators.is,t.operators.isNot];t.Filter.call(this,n,u,i);r.options=i&&i.options||[]};n.filtering=this}(window.app),function(n,t,i,r,u){"use strict";function a(n,t,i,r){return{type:n,caption:t,text:i,html:r}}function v(){var n=this;n.visible=ko.observable(!1);n.messages=ko.observableArray([]);n.fadeIn=function(n){n.nodeType===1&&i(n).hide().slideDown()};n.fadeOut=function(n){n.nodeType===1&&i(n).slideUp(function(){i(n).remove()})};n.remove=function(t){n.messages.remove(t)}}function c(n){var t=u.getItem("delayedMessages");return n&&l(null),t?JSON.parse(t)||[]:[]}function l(n){n?u.setItem("delayedMessages",JSON.stringify(n)):u.removeItem("delayedMessages")}function y(n){var t=c(!1);t.push(n);l(t)}var f=new v,h,o,s,e;if(n.addMessage=function(t,i,u,e,o){u=u||"success";e=e||"text";var s=a(u,i,e=="text"?t:null,e=="html"?t:null);if(o){y(s);return}f.messages().length!=0||f.visible()||f.visible(!0);n.settings.stackMessages||f.messages.pop();f.messages.push(s);u!="error"&&r(function(){f.messages.remove(s)},n.settings.messagesShowTime)},n.addErrorMessage=function(t,i,r,u){n.addMessage(t,i,"error",r,u)},h=t.getElementById(n.settings.messagesBlockId),h&&ko.applyBindings(f,h),o=c(!0),o)for(s=0;s<o.length;s++)e=o[s],n.addMessage(e.html||e.text,e.caption,e.type,e.html?"html":"text",!1)}(window.app,window.document,window.jQuery,window.setTimeout,window.sessionStorage),function(n,t){"use strict";n.page={scrollToId:function(n){var i=t.getElementById(n);i!=undefined&&t.body.scrollTop>i.offsetTop&&(t.body.scrollTop=i.offsetTop)},post:function(n,t,i){var r,f,u;i=i||"post";r=document.createElement("form");r.setAttribute("method",i);r.setAttribute("action",n);for(f in t)t.hasOwnProperty(f)&&(u=document.createElement("input"),u.setAttribute("type","hidden"),u.setAttribute("name",f),u.setAttribute("value",t[f]),r.appendChild(u));document.body.appendChild(r);r.submit();document.body.removeChild(r)},saveState:function(n,t){sessionStorage&&sessionStorage.setItem(n,JSON.stringify(t))},loadState:function(n){if(!sessionStorage)return null;try{return JSON.parse(sessionStorage.getItem(n))}catch(t){}return null},appendToState:function(n,t){var r=this,i=r.loadState(n);i||(i={});r.saveState(n,$.extend({},i,t))}}}(window.app,window.document),function(n,t){"use strict";function i(n,t){r.style[n]!=t&&(r.style[n]=t)}var r=t.getElementById(n.settings.progressIndicatorId);n.showProgress=function(){i("display","block");i("aria-busy","true")};n.hideProgress=function(){i("display","none");i("aria-busy","false")}}(window.app,window.document),function(n,t,i){"use strict";n.url={getUrlParts:function(){return t.pathname.split("/")},queryString:{getValue:function(n,i){var f,e,o,s,u,h,r;for(n&&(n=encodeURIComponent(n)),f={},i?(o=i.split("?"),e=o.length>1?o[1]:""):e=t.search,s=e.split(/\?|&/),u=0;u<s.length;u++)if(h=s[u],h!="")if(r=h.split("="),n){if(n==r[0])return decodeURIComponent(r[1])}else r[1]&&(f[decodeURIComponent(r[0])]=decodeURIComponent(r[1]));return n?null:f},setValue:function(n,t,i){t=encodeURIComponent(t);i=encodeURIComponent(i);var r=new RegExp("([?|&])"+t+"=.*?(&|$)","i");return n.match(r)?n.replace(r,"$1"+t+"="+i+"$2"):n.indexOf("?")==-1?n+"?"+t+"="+i:n+"&"+t+"="+i}},hash:{getValue:function(n){if(n)return n.split("#")[1];var i=t.hash.substr(1,t.hash.length-1);return i==""?null:i},setValue:function(n,i){return i?i.split("#")[0]+(n[0]=="#"?"":"#")+(n||""):(t.hash=n||"",t.href)},remove:function(n){return n?n.split("#")[0]:t.hash=""}}};n.url.navigateTo=function(r,u){if(n.showProgress(),u)if(typeof u=="string")r=n.url.hash.setValue(u,r);else for(var f in u)u[f]!=null&&(r=n.url.queryString.setValue(r,f,u[f]));i(function(){t.href=r},1)};n.url.open=function(t,r){if(r)if(typeof r=="string")t=n.url.hash.setValue(r,t);else for(var u in r)r[u]!=null&&(t=n.url.queryString.setValue(t,u,r[u]));i(function(){window.open(t)},1)}}(window.app,window.location,window.setTimeout),function(n){"use strict";n.capitalize=function(n){return n.replace(/^(.)|\s(.)/g,function(n){return n.toUpperCase()})};n.highlight=function(n,t){var i=t.replace(/[\-\[\]{}()*+?.,\\\^$|#\s]/g,"\\$&");return n.replace(new RegExp("(\\b"+i+")","ig"),function(n,t){return"<strong>"+t+"<\/strong>"})};n.formatUndefinableDateTime=function(n){if(n){var t=n.toString();return t.substring(0,t.indexOf(".")).replace("T"," ")}return"never"};n.computeSubjectAreaColumnPairs=function(n){for(var r=[],t=Math.floor(n.length/2),i,u;t<n.length-1;)if(n[t].parentSubjectAreaId===null&&n[t+1].parentSubjectAreaId!==null&&n[t].id===n[t+1].parentSubjectAreaId||n[t].parentSubjectAreaId!==null&&n[t+1].parentSubjectAreaId!==null&&n[t].parentSubjectAreaId===n[t+1].parentSubjectAreaId)t++;else break;for(i=0;i<t+1;i++)u=t+1+i<n.length?[n[i],n[t+1+i]]:[n[i]],r.push(u);return r};n.AggregateColumn=function(n,t,i,r,u,f){var e=this;e.key=n;e.avg=i;e.min=r;e.max=u;e.spread=f;e.id=t};n.QuestionResponseColumn=function(n,t){var i=this;i.text=t;i.id=n};n.Suggestion=function(n){var t=this;t.id=n.Id;t.firstName=n.FirstName;t.lastName=n.LastName;t.email=n.Email;t.rank=n.Rank;t.getText=function(){return t.firstName===""&&t.lastName===""?t.rank:t.rank+" - "+t.firstName+" "+t.lastName+" ("+t.email+")"}};n.Track=function(){var t=this;t.id=n.autoMap();t.name=n.autoMap()};n.SubmissionStatus=function(){var t=this;t.id=n.autoMap();t.name=n.autoMap();t.trackId=n.autoMap()};n.UserTag=function(){var t=this;t.id=n.autoMap();t.tag=n.autoMap()};n.GetEventFilter=function(n){var t=n.target,i=ko.contextFor(t);return i.$root.getFilter()};n.disableLink=function(n){setTimeout(function(){n.attr("disabled","disabled")},1)};n.enableLink=function(n){setTimeout(function(){n.removeAttr("disabled")},0)};n.File=function(){var t=this;t.id=n.autoMap();t.originalName=n.autoMap();t.size=n.autoMap();t.formattedSize=n.autoMap();t.uploadDate=n.autoMap();t.downloadLink=n.autoMap()};n.Question=function(){var t=this;t.order=n.autoMap();t.details=n.autoMap();t.answers=[]};n.QuestionAnswer=function(){var t=this;t.text=n.autoMap();t.value=n.autoMap()};n.Review=function(){var t=this;t.reviewerNumber=n.autoMap();t.reviewerName=n.autoMap();t.isSubmitted=n.autoMap();t.questions=[];t.files=[]};n.MetaReview=function(){var t=this;t.metaReviewerNumber=n.autoMap();t.metaReviewerName=n.autoMap();t.isSubmitted=n.autoMap();t.questions=[];t.files=[]};n.MessageList=function(n){function i(n){var t=""+(n.getMonth()+1),i=""+n.getDate(),e=n.getFullYear(),r=n.getHours(),u=n.getMinutes(),f=n.getSeconds();return t.length<2&&(t="0"+t),i.length<2&&(i="0"+i),r.length<2&&(r="0"+r),u.length<2&&(u="0"+u),f.length<2&&(f="0"+f),[e,t,i].join("-")+" "+[r,u,f].join(":")}var t=this;t.id=n.Id;t.reviewer=n.FirstName+" "+n.LastName;t.replyAuthor=n.ReplyAuthor;t.replyDate=n.ReplyDate;t.date=n.Date;t.topicId=n.TopicId;t.topic=n.Topic;t.message=n.Text.htmlMultiLineEncode();t.text=ko.observable();t.dateFormatted=function(){return i(t.date)};t.replyDateFormatted=function(){return t.replyDate?i(t.replyDate):""}}}(window.app),function(n,t,i){"use strict";i(t).ajaxStart(function(){});i(t).ajaxStop(function(){})}(window.app,window.document,window.jQuery,window.setTimeout,window.clearTimeout),function(n,t,i,r,u){"use strict";function e(){var e=0,t=0;this.request=function(o,s,h){function p(i){e++;i==0?(n.showProgress(),t!=0&&u(t)):t==0&&(t=r(function(){n.showProgress()},n.settings.progressIndicatorTimeout))}function w(t){v();try{s&&typeof s=="function"&&s(t);c.resolve(t.data)}catch(i){n.processException(i)}}function b(t){v();try{c.reject(t);h&&typeof h=="function"&&h(t)}catch(i){n.processException(i)}}function v(){y&&--e==0&&(t!=0&&(u(t),t=0),n.hideProgress())}var y=o.showProgressIndicator==undefined?!0:o.showProgressIndicator,l,c,a;return(o.showProgressIndicator==undefined?!0:o.showProgressIndicator)&&(l=o.progressIndicatorTimeout||n.settings.progressIndicatorTimeout,p(l)),o.recognizeDates=!0,o.headers.Accept="application/json;odata.metadata=full",o.headers.Prefer="return=representation",c=i.Deferred(),a=f.request(o,w,b),i.extend(c.promise(),a)}}var f=t.net.defaultHttpClient,o=t.defaultSuccess;t.net.defaultHttpClient=new e;t.defaultSuccess=function(){}}(window.app,window.OData,window.jQuery,window.setTimeout,window.clearTimeout),function(n){"use strict";function i(n){return n.replace(/([.*+?^=!:${}()|\[\]\/\\])/g,"\\$1")}function o(n){return n==null||n==undefined||typeof n!="string"?n:n.replace(new RegExp(i("'"),"g"),"''")}function s(n){return n==null||n==undefined||typeof n!="string"?n:n.replace(new RegExp(i("''"),"g"),"'")}function h(){return window.cmt3&&window.cmt3.conference?window.cmt3.conference.name:null}function r(n,t,i,r,o){function h(n){var i="?";for(var t in n)n[t]!=null&&(i+=encodeURIComponent((e[t]?"$":"")+t)+"="+encodeURIComponent(n[t])+"&");return i.substring(0,i.length-1)}if(!t)throw new Error("'entitySet' must be specified.");var s={entitySet:"/"+t};return s.conferenceName=n?"/"+n:"",typeof i=="object"&&(o=i,i=null),typeof r=="object"&&(o=r,r=null),s.key=i?f.format(i):"",s.action=r?"/"+r:"",s.queryString=o?h(o):"",u.format(s)}var t=window.cmt3.context.path?window.cmt3.context.path:"",u=(t=="/"?"":t)+"/api/odata{conferenceName}{entitySet}{key}{action}{queryString}",f="({0})",e={orderby:!0,top:!0,skip:!0,filter:!0,expand:!0,format:!0,select:!0,count:!0};n.odata={escapeParam:function(n){return o(n)},unescapeParam:function(n){return s(n)},getUrl:function(n,t,i,u){return r(h(),n,t,i,u)},getGlobalUrl:function(n,t,i,u){return r(null,n,t,i,u)},buildContainsQuery:function(n,t,i){for(var u=i?"not(":"(",r=0;r<t.length;r++)u+=n+" eq "+t[r],r!=t.length-1&&(u+=" or ");return u+")"},processRedirectResponse:function(t){n.url.navigateTo(t.RedirectUrl)},getErrorMessage:function(n){if(!n||!n.response||!n.response.body)return"";var t=$.parseJSON(n.response.body);return!t||!t.error||!t.error.message?"":t.error.message},entitySet:{myConferences:"MyConferences",conferences:"Conferences",conflictReasons:"ConflictReasons",emails:"Emails",emailTemplates:"EmailTemplates",files:"Files",forms:"Forms",optionsTypes:"OptionsTypes",questions:"Questions",questionTypes:"QuestionTypes",questionDisplayLogic:"QuestionDisplayLogic",reviewDrafts:"ReviewDrafts",reviewModels:"ReviewModels",metaReviewDrafts:"MetaReviewDrafts",authorFeedbackDrafts:"AuthorFeedbackDrafts",reviewerViews:"ReviewerViews",metaReviewerViews:"MetaReviewerViews",reviewerSubmissionViews:"ReviewerSubmissionViews",metaReviewerSubmissionViews:"MetaReviewerSubmissionViews",seniorMetaReviewerSubmissionViews:"SeniorMetaReviewerSubmissionViews",metaReviewModels:"MetaReviewModels",trackReviewerViews:"TrackReviewerViews",trackStatuses:"TrackStatuses",reviews:"Reviews",metaReviews:"MetaReviews",reviewVersionViews:"ReviewVersionViews",reviewerNotes:"ReviewerNotes",reviewerNoteViews:"ReviewerNoteViews",metaReviewerNotes:"MetaReviewerNotes",metaReviewerNoteViews:"MetaReviewerNoteViews",seniorMetaReviewerNotes:"SeniorMetaReviewerNotes",seniorMetaReviewerNoteViews:"SeniorMetaReviewerNoteViews",chairNotes:"ChairNotes",chairNoteViews:"ChairNoteViews",reviewDiscussions:"ReviewDiscussions",authorFeedbacks:"AuthorFeedbacks",authorFeedbackViews:"AuthorFeedbackViews",reviewViews:"ReviewViews",metaReviewViews:"MetaReviewViews",discussionMessages:"DiscussionMessages",reviewSnapshotAuthorViews:"ReviewSnapshotAuthorViews",roles:"Roles",subjectAreas:"SubjectAreas",submissions:"Submissions",deletedSubmissions:"DeletedSubmissions",generalSettings:"GeneralSettings",authorFeedbackSettings:"AuthorFeedbackSettings",reviewSettings:"ReviewSettings",conflictSettings:"ConflictSettings",metaReviewSettings:"MetaReviewSettings",seniorMetaReviewSettings:"SeniorMetaReviewSettings",cameraReadySubmissions:"CameraReadySubmissions",cameraReadySubmissionSettings:"CameraReadySubmissionSettings",submissionSettings:"SubmissionSettings",submissionStatuses:"SubmissionStatuses",submissionViews:"SubmissionViews",submissionAuthorViews:"SubmissionAuthorViews",cameraReadySubmissionViews:"CameraReadySubmissionViews",emailMessages:"EmailMessages",tracks:"Tracks",trackSummaries:"TrackSummaries",users:"Users",userModels:"UserModels",trackReviewers:"TrackReviewers",trackMetaReviewers:"TrackMetaReviewers",trackSeniorMetaReviewers:"TrackSeniorMetaReviewers",manageReviewerInvites:"ManageReviewerInvites",manageInviteReviewers:"ManageInviteReviewers",manageInviteMetaReviewers:"ManageInviteMetaReviewers",manageInviteSeniorMetaReviewers:"ManageInviteSeniorMetaReviewers",manageReviewerInvitesForSubmission:"ManageReviewerInvitesForSubmission",biddings:"BiddingModels",reviewers:"ReviewerModels",metaReviewers:"MetaReviewerModels",supplementary:"Supplementary",inplaceRevision:"InplaceRevision",copyrights:"Copyrights",referenceModels:"ReferenceModels",userSettingsModels:"UserSettingsModels",statuses:"PaperStatuses",biddingReviewModels:"BiddingReviewModels",metaBiddingModels:"MetaBiddingModels",metaBiddingReviewModels:"MetaBiddingReviewModels",suggestionViews:"SuggestionViews",suggestionModels:"SuggestionModels",inviteStatusModels:"InviteStatusModels",openAcademicPublishes:"OpenAcademicPublishes",userDisputeConflicts:"UserDisputeConflicts",chairDisputeConflicts:"ChairManageDisputedConflicts",conflictDomains:"ConflictDomains",proceedingEditorModels:"ProceedingEditorModels",tpmsSettings:"TpmsSettings",tpmsSubmissions:"TpmsSubmissions",tpmsMatchingRequests:"TpmsMatchingRequests",tpmsScores:"TpmsScores",userTypeOptions:"UserTypeOptions",userTypes:"UserTypes",seniorMetaReviewerBiddingViews:"SeniorMetaReviewerBiddingViews",seniorMetaReviewerBiddingModels:"SeniorMetaReviewerBiddingModels",presentations:"Presentations",sessions:"Sessions",rooms:"Rooms",individualConflictViews:"IndividualConflictViews",conferenceSessionSettings:"ConferenceSessionSettings",submissionModels:"SubmissionModels",seniorMetaReviewerRatingOptions:"SeniorMetaReviewerRatingOptions",sharedMetaReviewerRecommendationOptions:"SharedMetaReviewerRecommendationOptions",trackMetaReviewerGroups:"TrackMetaReviewerGroups",questionInvisibleByTags:"QuestionInvisibleByTags",iThenticateSettings:"IThenticateSettings",iThenticateResults:"IThenticateResults",iThenticateRetrieveResults:"IThenticateRetrieveResults",iThenticateSubmissions:"IThenticateSubmissions",submissionFilesModel:"SubmissionFilesModel",userInformationModels:"UserInformationModels",authorFeedbackComments:"AuthorFeedbackComments",reviewerSubmissionComparisons:"ReviewerSubmissionComparisons",metaReviewerSubmissionComparisons:"MetaReviewerSubmissionComparisons",conferenceRequests:"ConferenceRequests",accountProcessingRequests:"AccountProcessingRequests"}}}(window.app,window.location),function(n,t,i){"use strict";t.ServerList=function(r){function w(n,t,i){return h==null?!1:i.filterComparator.areEqual(n,h)&&v(t)||i.filterComparator.isSubFilter(n,h)&&c}function v(n){return c||f+n<=u.length}function o(t,i){return n.isFunction(t)?t(i):t}function y(i,r,f,e){var s={},h,c;if(u.length>0&&(s.skip=u.length),f!=Infinity&&e.preLoadpageCount!=null&&e.preLoadpageCount!=Infinity&&(s.count="true",s.top=(f+e.preLoadpageCount)*e.pageSize),e.odataFilter&&(s.filter=o(e.odataFilter,i)),e.odataOrderByFields&&(s.orderby=o(e.odataOrderByFields,r)),e.odataExpandFields&&(s.expand=o(e.odataExpandFields)),e.odataCustomQuery){h=o(e.odataCustomQuery);for(c in h)s[c]=h[c]}return n.isPlainObject(e.entitySet)?t.odata[e.entitySet.isGlobal?"getGlobalUrl":"getUrl"](e.entitySet.entitySet,e.entitySet.key,e.entitySet.action,s):t.odata.getUrl(e.entitySet,s)}var s=this,l=n.extend(!0,{},t.ServerList.defaults,r),u=[],f,h,p,e,c,a;s.getTotalCount=function(){return e};s.clear=function(){u.length=0;f=0;h=null;p=null;e=0;c=!1};s.clear();s.getItems=function(t,r,s){return n.Deferred(function(v){var b,p,d,g,k,nt,tt,it;if(r==null&&(r=Infinity),p=s?n.extend(!0,{},l,s):l,typeof p.showProgressIndicator=="undefined"&&(p.showProgressIndicator=!0),t?a.resetLength(t):t=[],r==0){v.resolve(t);return}if(d=r*p.pageSize,f=0,g=o(p.filter),n.isFunction(p.localFilter)&&w(g,d,p)){if(k=[],p.filterComparator.isEmpty(g))d==Infinity?k.push.apply(k,u):k.push.apply(k,u.slice(0,d)),f=d,e=u.length;else{for(nt=0,b=0;b<u.length;b++)if(tt=p.localFilter(u[b],g),tt&&(k.push(tt),++nt==d))break;for(f=b+1,e=nt,b=f;b<u.length;b++)p.localFilter(u[b],g)&&++e}p.sort&&p.sort(k);t(k);v.resolve(t)}else u.length=0,h=g,it=y(g,null,r,p),i.read({requestUri:it,showProgressIndicator:p.showProgressIndicator},function(n){for(b=0;b<n.value.length;b++){var i=p.itemConstructor(n.value[b]);u.push(i);b<d&&t.push(i)}f=a.getLength(t);e=n["@odata.count"]||u.length;c=u.length==e;v.resolve(t)})}).promise()};s.addItems=function(t,r,s){return n.Deferred(function(h){var p,w,b,k,d,g;if(r==null&&(r=Infinity),w=s?n.extend(!0,{},l,s):l,t||(t=[]),r==0){h.resolve(t);return}if(b=r*w.pageSize,k=o(w.filter),n.isFunction(w.localFilter)&&v(b)){if(w.filterComparator.isEmpty(k))b==Infinity?(t.push.apply(t,u.slice(f)),f=u.length):t.push.apply(t,u.slice(f,f+=b)),e=u.length;else{for(d=0,p=f;p<u.length;p++)if(g=w.localFilter(u[p],k),g&&(t.push(g),++d==b))break;if(f=p+1,e==0)for(e=d,p=f;p<u.length;p++)w.localFilter(u[p],k)&&++e}h.resolve(t)}else i.read(y(k,null,r,w),function(n){for(p=0;p<n.value.length;p++){var i=w.itemConstructor(n.value[p]);u.push(i);p<b&&t.push(i)}f=a.getLength(t);e=n["@odata.count"]||u.length;c=u.length==e;h.resolve(t)})}).promise()};a={getLength:function(t){return n.isFunction(t)?t().length:t.length},resetLength:function(t){n.isFunction(t)?t.removeAll():t.length=0}}};n.extend(t.ServerList,{defaults:{entitySet:null,filter:null,orderBy:null,pageSize:t.settings&&t.settings.pageSize?t.settings.pageSize:Infinity,preLoadpageCount:0,localFilter:function(n,t){return n?n.indexOf(t)>-1?n:null:null},localOrderBy:function(n,t){return n<t?-1:n>t?1:0},itemConstructor:function(n){return n},filterComparator:{isEmpty:function(n){return!n},areEqual:function(n,t){return n==t},isSubFilter:function(n,t){return(n||"").indexOf(t)==0}},odataFilter:null,odataOrderByFields:null,odataExpandFields:null,odataCustomQuery:null}})}(window.jQuery,window.app,window.OData),function(n,t){"use strict";n.ShowMore=function(i){var r=this,u;if(r.options={elementId:"showMore",showNumbers:ko.observable(!0)},r.nextCount=ko.observable(0),r.allCount=ko.observable(0),r.showMoreVisible=ko.observable(!1),r.showAllVisible=ko.observable(!1),r.showMore=function(){i(1)},r.showAll=function(){i(Infinity)},r.updateCount=function(t,i){var u=t-i;r.nextCount(u>n.settings.pageSize?n.settings.pageSize:u);r.allCount(t);r.showMoreVisible(u>n.settings.pageSize);r.showAllVisible(u>0)},r.removeOne=function(){r.allCount(r.allCount()-1)},u=t.getElementById(r.options.elementId),!u)throw new Error("Element with id='{0}' does not exist.".format(r.options.elementId));ko.applyBindings(r,u)}}(window.app,window.document),function(n,t){window.cmt3.errors.length>0&&n.each(window.cmt3.errors,function(n,i){t.addMessage(i,"Application error:","error")});window.cmt3.logger||(window.cmt3.logger={error:function(n){console&&console.error(n)},info:function(n){console&&console.info(n)},warn:function(n){console&&console.warn(n)},log:function(n){console&&console.log(n)}})}(window.jQuery,window.app),function(n,t,i){"use strict";n.FormService=function(){function r(){var t=this;t.id=n.autoMap();t.formType=n.autoMap();t.formTypeName=n.autoMap();t.trackId=n.autoMap();t.name=n.autoMap();t.description=n.autoMap();t.isVisibleToAuthorEnabledToEdit=n.autoMap();t.isVisibleToAuthorDuringFeedbackEnabledToEdit=n.autoMap();t.isVisibleToAuthorAfterNotificationEnabledToEdit=n.autoMap();t.isVisibleToReviewerEnabledToEdit=n.autoMap();t.isVisibleToMetaReviewerEnabledToEdit=n.autoMap();t.isVisibleToOtherReviewerEnabledToEdit=n.autoMap();t.isVisibleToSeniorMetaReviewerEnabledToEdit=n.autoMap()}var u=this;u.loadForm=function(u,f){return i.Deferred(function(i){var e=n.odata.getUrl(n.odata.entitySet.forms,{filter:"FormType eq {0} and TrackId eq {1}".format(n.odata.escapeParam(u),n.odata.escapeParam(f)),orderby:"CreateDate desc",top:"1"}),o={requestUri:e,method:"GET",showProgressIndicator:!1};t.request(o,function(t){if(t.value.length==1){var f=n.autoMap(new r,t.value[0]);i.resolve(f)}else n.addMessage("Form of type '{0}' does not exists.".format(u),null,"error"),i.resolve(null)})}).promise()}}}(window.app,window.OData,window.jQuery),function(n,t,i,r){"use strict";n.QuestionService=function(){function o(t){var i=this,r,u;i.id=n.autoMap();i.title=n.autoMap();i.required=ko.observable().autoMap();i.isLocked=n.autoMap();i.questionType=n.autoMap();i.optionsType=n.autoMap();i.details=n.autoMap();i.additionalInfo=n.autoMap();i.order=n.autoMap();i.heading=n.autoMap();i.commentLength=n.autoMap();i.visibleToAuthorDuringFeedback=n.autoMap();i.visibleToAuthorAfterNotification=n.autoMap();i.visibleToReviewer=n.autoMap();i.visibleToMetaReviewer=n.autoMap();i.visibleToOtherReviewer=n.autoMap();i.hasAdditionalInfo=function(){return i.additionalInfo&&i.additionalInfo.trim().length!==0};i.getAdditionalInfo=function(){return i.additionalInfo||""};i.visibilityInfo=function(){var n=[];return i.visibleToAuthorDuringFeedback&&n.push("visible to authors during feedback"),i.visibleToAuthorAfterNotification&&n.push("visible to authors after notification"),i.visibleToOtherReviewer&&n.push("visible to other reviewers"),i.visibleToReviewer&&n.push("visible to reviewers"),i.visibleToMetaReviewer&&n.push("visible to meta-reviewers"),n.length>0?"("+n.join(", ")+")":null};i.choices=[];i.conditionQuestionChoiceIds=[];i.formType=t;i.validationEnabled=!0;i.answer=ko.observable().extend({required:{onlyIf:function(){return i.validationEnabled&&i.required()}}});i.onOtherFieldFocus=function(){i.answer(f)};i.answer.subscribe(function(){i.answer()!==f&&i.otherAnswer("")});i.otherAnswer=ko.observable().extend({required:{onlyIf:function(){return i.validationEnabled&&i.answer()===f}}});i.previousAnswer=ko.observable();i.selectedChoiceIds=ko.observableArray();i.selectedChoiceIds.subscribe(function(n){i.answer(n.join())});i.setAgreementTypeValidator=function(){i.required()&&(i.answer=i.answer.extend({equal:{params:!0,message:"You must accept agreement to continue."}}))};r=null;u=null;i.subscribeAnswerChanged=function(n){i.unsubscribeAnswerChanged();u=i.answer.subscribe(function(n){i.previousAnswer(n)},this,"beforeChange");r=i.answer.subscribe(function(t){n(i,t,i.previousAnswer())})};i.unsubscribeAnswerChanged=function(){r&&r.dispose();u&&u.dispose()};i.subscribeChoicesChanged=function(n){i.selectedChoiceIds.subscribe(function(t){t.forEach(function(t){(t.status==="added"||t.status==="deleted")&&n(i,t)})},null,"arrayChange")};i.setUpAnswerCharsLeft=function(){i.questionType==n.enums.questionType.comment&&(i.answer=i.answer.extend({maxlength:i.commentLength}));i.answerCharsLeft=ko.computed(function(){if(i.questionType!=n.enums.questionType.comment||i.commentLength==null)return 0;var t=0,r=i.answer();return typeof r=="string"&&(t=r.length),Math.max(i.commentLength-t,0)})}}function e(){var t=this;t.id=n.autoMap();t.order=n.autoMap();t.text=n.autoMap();t.value=n.autoMap();t.requireAnswer=ko.observable(!1);t.answer=ko.observable().autoMap().extend({required:{onlyIf:t.requireAnswer}});t.comment=ko.observable().autoMap()}var u=this,f="-1";u.parseQuestionsDirect=function(t,i){for(var v=[],s,u,c,r,l,a,h=0;h<i.length;h++){for(c=i[h],r=n.autoMap(new o(t),c),r.setUpAnswerCharsLeft(),r.questionType===n.enums.questionType.agreement&&r.setAgreementTypeValidator(),l=c.Choices,u=0;u<l.length;u++)s=n.autoMap(new e,l[u]),s.id=s.id.toString(),r.choices.push(s);for(r.questionType===n.enums.questionType.optionsWithOther&&(s=new e,s.id=f,r.choices.push(s)),a=c.ConditionQuestionChoiceIds,u=0;u<a.length;u++)r.conditionQuestionChoiceIds.push(a[u]);v.push(r)}return v};u.loadQuestionsDirect=function(r,f){return i.Deferred(function(i){var e=n.odata.getUrl(n.odata.entitySet.questions,{orderby:"Order",filter:"FormId eq {0}".format(n.odata.escapeParam(f))});t.read({requestUri:e,showProgressIndicator:!1},function(n){var t=u.parseQuestionsDirect(r,n.value);i.resolve(t)})}).promise()};u.loadQuestions=function(u,f){return i.Deferred(function(i){r.loadForm(u,f).done(function(r){var f=n.odata.getUrl(n.odata.entitySet.questions,{orderby:"Order",filter:"FormId eq {0}".format(n.odata.escapeParam(r.id))});t.read({requestUri:f,showProgressIndicator:!1},function(t){for(var s,f,l,h,a,r,v=[],c=0;c<t.value.length;c++){for(s=t.value[c],f=n.autoMap(new o(u),s),f.setUpAnswerCharsLeft(),f.questionType==n.enums.questionType.agreement&&f.setAgreementTypeValidator(),l=s.Choices,r=0;r<l.length;r++)h=n.autoMap(new e,l[r]),h.id=h.id.toString(),f.choices.push(h);for(a=s.ConditionQuestionChoiceIds,r=0;r<a.length;r++)f.conditionQuestionChoiceIds.push(a[r]);v.push(f)}i.resolve(v)}).fail(i.reject)})}).promise()};u.setAnswersFromJson=function(t,i){for(var c={},s,u,h,e,r,o=0;o<t.length;o++)c[t[o].id]=t[o],t[o].selectedChoiceIds.removeAll(),t[o].answer(null),t[o].answer.isModified(!1);for(s=0;s<i.length;s++)if(e=i[s],r=c[e.QuestionId],r)switch(r.questionType){case n.enums.questionType.agreement:r.answer(!0);break;case n.enums.questionType.comment:r.answer(e.Text);break;case n.enums.questionType.options:case n.enums.questionType.optionsWithValue:for(u=0;u<r.choices.length;u++)if(r.choices[u].id==e.QuestionChoiceId){r.selectedChoiceIds.push(r.choices[u].id.toString());break}r.answer(r.selectedChoiceIds().join());break;case n.enums.questionType.optionsWithOther:if(e.QuestionChoiceId){for(u=0;u<r.choices.length;u++)if(r.choices[u].id==e.QuestionChoiceId){r.selectedChoiceIds.push(r.choices[u].id.toString());break}}else e.Text&&(r.selectedChoiceIds.push(f.toString()),r.otherAnswer(e.Text));r.answer(r.selectedChoiceIds().join());break;case n.enums.questionType.optionsWithUserInput:for(u=0;u<r.choices.length;u++)if(h=r.choices[u],h.id==e.QuestionChoiceId){h.answer(e.Answer);h.comment(e.Comment);break}}};u.getAnswersJson=function(t){for(var r=[],u,i,e,o=0;o<t.length;o++){i=t[o];switch(i.questionType){case n.enums.questionType.agreement:i.answer()&&r.push({QuestionId:i.id});break;case n.enums.questionType.comment:i.answer()&&r.push({QuestionId:i.id,Text:i.answer()});break;case n.enums.questionType.options:case n.enums.questionType.optionsWithValue:switch(i.optionsType){case n.enums.optionsType.radioButtonList:case n.enums.optionsType.dropDown:i.answer()&&r.push({QuestionId:i.id,QuestionChoiceId:i.answer()});break;case n.enums.optionsType.checkboxList:case n.enums.optionsType.listBox:for(u=0;u<i.selectedChoiceIds().length;u++)r.push({QuestionId:i.id,QuestionChoiceId:i.selectedChoiceIds()[u]})}break;case n.enums.questionType.optionsWithOther:i.answer()&&(i.answer()!==f?r.push({QuestionId:i.id,QuestionChoiceId:i.answer()}):r.push({QuestionId:i.id,Text:i.otherAnswer()}));break;case n.enums.questionType.optionsWithUserInput:for(u=0;u<i.choices.length;u++)(e=i.choices[u],e.answer)&&r.push({QuestionId:i.id,QuestionChoiceId:e.id,Answer:e.answer(),Comment:e.comment()})}}return r};u.subscribeAnswerChanged=function(t,i){for(var u,r=0;r<t.length;r++){u=t[r];switch(u.optionsType){case n.enums.optionsType.radioButtonList:case n.enums.optionsType.dropDown:u.subscribeAnswerChanged(i)}}};u.unsubscribeAnswerChanged=function(n){for(var t=0;t<n.length;t++)n[t].unsubscribeAnswerChanged()};u.subscribeChoicesChanged=function(t,i){for(var u,r=0;r<t.length;r++){u=t[r];switch(u.optionsType){case n.enums.optionsType.checkboxList:case n.enums.optionsType.listBox:u.subscribeChoicesChanged(i)}}}}}(window.app,window.OData,window.jQuery,new window.app.FormService),function(n,t){n.CaptchaService=function(){function i(t){var i=this;t||(t="audioCaptchaChallenge");i.type=ko.observable("visual");i.challengeId=ko.observable();i.challenge=ko.observable();i.response=ko.observable("").extend({required:!0});i.azureRegion=ko.observable();i.isLoading=ko.observable(!1);i.isResponseFieldFocused=ko.observable(!1);i.currentModeLabel=ko.pureComputed(function(){return i.type()==="visual"?"Enter the characters you see":"Press 1 to play or repeat the audio. Enter the words you hear in any order."});i.switchModeLabel=ko.pureComputed(function(){return i.type()==="visual"?"Audio":"Picture"});i.switchModeTitle=ko.pureComputed(function(){return i.type()==="visual"?"Switch to the audio challenge":"Switch to the visual challenge"});i.switchMode=function(){i.type(i.type()==="visual"?"audio":"visual");i.getNew()};i.keyDown=function(n,t){return i.type()==="audio"&&t.key==="1"?(i.playAudio(),!1):!0};i.playAudio=function(){if(i.type()==="audio"){var n=document.getElementById(t);n&&(n.currentTime=0,n.play())}};i.getRequestModel=function(){return{TestCaptchaRequest:{ChallengeId:i.challengeId(),InputSolution:i.response()},AzureRegion:i.azureRegion(),ChallengeType:i.type()}};i.getNew=function(t){i.response("");(t||t===undefined)&&i.isResponseFieldFocused(!0);i.isLoading(!0);n.getCaptcha(i.type()).done(function(n){i.challengeId(n.ChallengeId);i.challenge((i.type()==="visual"?"data:image/jpeg;base64, ":"data:audio/mp3;base64, ")+n.ChallengeString);i.azureRegion(n.AzureRegion)}).always(function(){i.isLoading(!1)})}}var n=this;n.createViewModel=function(n){return new i(n)};n.getCaptcha=function(n){return t.get("/api/CaptchaService/GetCaptchaChallenge?challengeType="+n)}}}(window.app,window.jQuery),function(n,t,i){"use strict";n.RoleService=function(){function u(){var t=this;t.role=n.autoMap();t.submissionListUrl=n.autoMap();t.conferenceDefaultUrl=n.autoMap()}var r=this;r.getCurrentRoleDescriptor=function(){return i.Deferred(function(i){var r={requestUri:n.odata.getUrl(n.odata.entitySet.users,null,"GetCurrentRoleDescriptor"),method:"POST",showProgressIndicator:!1};t.request(r,function(t){i.resolve(n.autoMap(new u,t))}).fail(i.reject)}).promise()}}}(window.app,window.OData,window.jQuery);var messages={assignment:{item_title_papers:"This field MUST contains\npositive number\nGREATER THAN OR EQUAL TO\nalready assigned to this paper.",item_title_reviewers:"This field MUST contains\npositive number\nGREATER THAN OR EQUAL TO\nalready assigned to this paper,\nbut must not exceed quota (if applicable).",assign_title:"This field MUST contains\npositive number ONLY.",increase_title:"This field MUST contains\npositive number ONLY."}};(function(n,t,i){"use strict";function r(t,i){this.$element=n("<div>").addClass(t).hide();this.$all=n("<input>").attr({name:"selected",type:"checkbox",checked:i});this.$text=n("<span>");this.$label=n("<label>").addClass("label").append(this.$all).append(this.$text);this.$element.append(n("<div>").addClass("all").append(this.$label));this.$list=n("<ul>").addClass("list");this.$element.append(this.$list);this.item='<li class="item"><label><input type="checkbox" class="flag"/><span class="title"><\/span><\/label><\/li>';this.listen()}t.AbstractFilter=function(t,i,r,u,f){this.$container=n(i);this.$holder=n(t);this.model=r;this.field=u;this.substitutions=f;this.$query=n("<input>").addClass("input").attr("type","text").attr("value",this.watermark());this.$clear=n("<span>").addClass("link-remove").append(n("<a>").text("Clear").attr("href","#"));this.show();this.listen()};t.AbstractFilter.prototype={listen:function(){this.$query.on("keyup",n.proxy(this.keyup,this)).on("focus",n.proxy(this.focus,this)).on("focusout",n.proxy(this.blur,this));this.$clear.on("mousedown",n.proxy(this.clear,this))},show:function(){var t=n("<div>").addClass("query").attr("title",this.help());t.append(this.$query).append(this.$clear);this.$container.append(t)},help:function(){return"Start typing here."},keyup:function(n){switch(n.keyCode){case 13:n.preventDefault();this.search()}},focus:function(){var n=this.$query.val();this.$query.parent().width()<200&&(this.$query.data("original-width",this.$query.parent().width()),this.$query.parent().animate({width:"200px"}),this.$query.parent().css({zIndex:"10"}));n==this.watermark()&&this.$query.val("")},blur:function(){var t=this.$query.val(),n=this.$query.data("original-width");n&&(this.$query.removeData("original-width"),this.$query.parent().animate({width:n}),this.$query.parent().css({zIndex:"1"}));t==""&&this.$query.val(this.watermark());this.valid()?this.$query.removeClass("error"):this.$query.addClass("error")},valid:function(){return!0},watermark:function(){return"All"},clear:function(){this.reset();this.search()},reset:function(){this.$query.val(this.watermark())},search:function(){n(document).trigger("data.filter")},state:function(n){return n&&this.$query.val(n),this.$query.val()},getValue:function(){return null}};t.TextFilter=function(n,i,r,u,f){var e=this;e.doNotLower=!1;t.AbstractFilter.call(this,n,i,r,u,f)};t.TextFilter.prototype=n.extend({},t.AbstractFilter.prototype,{doNotLower:!1,match:function(n){var t=this,i="contains\\({0},'(\\S+)'\\)".format(t.doNotLower?t.field:"tolower\\("+t.field+"\\)"),r=new RegExp(i,"g");return r.test(n)},setValue:function(i){var r=this,f="contains\\({0},'(\\S+)'\\)".format(r.doNotLower?r.field:"tolower\\("+r.field+"\\)"),e=new RegExp(f,"g"),u=e.exec(i);u!=undefined&&u.length==2&&this.$query.val(n.trim(t.odata.unescapeParam(u[1])))},getValue:function(){var r=this,i=r.$query.val();return i!=null&&i.length>=2&&i!=r.watermark()?(i=n.trim(i),r.doNotLower||(i=i.toLowerCase()),("(contains({0},'"+t.odata.escapeParam(i)+"'))").format(r.doNotLower?r.field:"tolower("+r.field+")")):null},watermark:function(){return"filter..."},help:function(){return"Type any text here and then press Enter."}});t.NumericFilter=function(n,i,r,u,f){t.AbstractFilter.call(this,n,i,r,u,f)};t.NumericFilter.prototype=n.extend({},t.AbstractFilter.prototype,{match:function(n){var t=new RegExp(this.field+"\\s+(ge|le|ne|eq|gt|lt)\\s+([0-9]*.[0-9]+|[0-9]+)","g");return t.test(n)},setValue:function(t){var u=new RegExp(this.field+"\\s+(ge|le|ne|eq|gt|lt)\\s+([0-9]*.[0-9]+|[0-9]+)","g"),i=u.exec(t),r;if(i!=undefined&&i.length==3){r="eq";switch(n.trim(i[1])){case"ge":r=">= ";break;case"le":r="<= ";break;case"ne":r="<> ";break;case"gt":r="> ";break;case"lt":r="< ";break;case"eq":r="= "}this.$query.val(r+n.trim(i[2]))}else u=new RegExp(this.field+"\\s+(ge|le|ne|eq|gt|lt)\\s+([0-9]*.[0-9]+|[0-9]+)\\s+and\\s+"+this.field+"\\s+(ge|le|ne|eq|gt|lt)\\s+([0-9]*.[0-9]+|[0-9]+)","g"),i=u.exec(t),i!=undefined&&i.length==5&&this.$query.val(n.trim(i[2])+" - "+n.trim(i[4]))},getValue:function(){var r=this.$query.val(),t,i;if(this.valid()?this.$query.removeClass("error"):this.$query.addClass("error"),r!=null&&r.length>=2&&r!=this.watermark()){if(t=/\s*(>=|<=|<>|=|>|<)\s*([0-9]*\.[0-9]+|[0-9]+)/g.exec(n.trim(r)),t!=undefined&&t.length==3){i="eq";switch(n.trim(t[1])){case">=":i=" ge ";break;case"<=":i=" le ";break;case"<>":i=" ne ";break;case">":i=" gt ";break;case"<":i=" lt ";break;case"=":i=" eq "}return"("+this.field+i+this.getNormalizedValue(n.trim(t[2]))+")"}if(t=/([0-9]*\.[0-9]+|[0-9]+)(\s*-\s*)([0-9]*\.[0-9]+|[0-9]+)/g.exec(n.trim(r)),t!=undefined&&t.length==4)return"("+this.field+" ge "+this.getNormalizedValue(n.trim(t[1]))+" and "+this.field+" le "+this.getNormalizedValue(n.trim(t[3]))+")"}return null},valid:function(){return this.$query.val().match(/\s*(>=|<=|<>|=|>|<)\s*([0-9]*\.[0-9]+|[0-9]+)/g)?!0:this.$query.val().match(/([0-9]*\.[0-9]+|[0-9]+)(\s*-\s*)([0-9]*\.[0-9]+|[0-9]+)/g)?!0:this.$query.val()==this.watermark()?!0:!1},watermark:function(){return"e.g. <3"},help:function(){return"Type any [= or < or > or <= or >=] + number or [number - number] for range and then press Enter."},getNormalizedValue:function(n){var t=n;return typeof parseFloat!="function"?n:(t=parseFloat(t),typeof t.toString!="function")?n:t.toString()}});t.DatetimeFilter=function(n,i,r,u,f){t.AbstractFilter.call(this,n,i,r,u,f)};t.DatetimeFilter.prototype=n.extend({},t.AbstractFilter.prototype,{match:function(){return!1},getPattern:function(){return/\s*(>=|<=|<>|=|>|<)\s*(never|[0-9]{4,}\s*-\s*[0-9]{1,2}\s*-\s*[0-9]{1,2}\s*[0-9]{1,2}\s*:\s*[0-9]{1,2}\s*:\s*[0-9]{1,2}\s*|[0-9]{4,}\s*-\s*[0-9]{1,2}\s*-\s*[0-9]{1,2}\s*)/g},getValue:function(){var u=this.$query.val(),r,t,i,f;if(this.valid()?this.$query.removeClass("error"):this.$query.addClass("error"),u!=null&&u.length>=2&&u!=this.watermark()&&(r=this.getPattern().exec(n.trim(u)),r!=undefined&&r.length==3)){t="eq";switch(n.trim(r[1])){case">=":t=" ge ";break;case"<=":t=" le ";break;case"<>":t=" ne ";break;case">":t=" gt ";break;case"<":t=" lt ";break;case"=":t=" eq "}if(i=n.trim(r[2]),i==="never"){if(i="null",t===" gt ")t=" ne ";else if(t===" lt "||t===" le ")t=" eq ";else if(t===" ge ")return null}else f=new Date(i.replace(/\s+/g,"T")),i="cast("+f.format("yyyy-mm-ddThh:nn:ss.fffZ")+",Edm.DateTimeOffset)";return"("+this.field+t+i+")"}return null},valid:function(){return this.$query.val().match(this.getPattern())?!0:this.$query.val()==this.watermark()?!0:!1},watermark:function(){return"e.g. >= 2014-06-25 15:02:32"},help:function(){return"Type any [= or < or > or <= or >=] + datetime and then press Enter."}});r.prototype={listen:function(){this.$all.change(n.proxy(this.all,this))},all:function(){var t=this.$all.prop("checked");n(":checkbox",this.$list).each(function(){n(this).prop("checked",t)});this.$text.text(t?"Deselect all":"Select all")},show:function(i,r,u,f){if(this.$list.empty(),i.length>0){var e=this;this.$all.prop("checked",u);this.$text.text(u?"Deselect all":"Select all");n(i).each(function(i,o){var s=n(e.item),h,c;h=r!=null&&r[o]!=null?r[o]:o;n(".title",s).html(f!=null?t.highlight(h,f):h);c=n("input",s);c.prop("checked",u);c.prop("value",o);e.$list.append(s)});this.$element.show()}},hide:function(){this.$element.hide();this.$list.empty()},selected:function(){var t=[];return n(":checked",this.$list).each(function(i,r){t.push(n(r).attr("value"))}),t}};t.MultipleSelector=function(t){this.$filter=t.$element;this.$element=n("<div>").addClass("selector").hide();this.selected=new r("selected");this.$element.append(this.selected.$element);this.found=new r("found");this.$element.append(this.found.$element);this.$ok=n("<a>").addClass("btn").attr({href:"#",role:"button"}).text("Ok");this.$cancel=n("<a>").addClass("btn").attr({href:"#",role:"button"}).text("Cancel");this.$actions=n("<div>").addClass("actions").append(this.$ok).append(this.$cancel);this.$element.append(this.$actions);this.items=[];this.mouseover=!1;this.listen()};t.MultipleSelector.prototype={listen:function(){this.$element.on("focusin",n.proxy(this.focusin,this)).on("mouseenter",n.proxy(this.mouseenter,this)).on("focusout",n.proxy(this.focusout,this)).on("mouseleave",n.proxy(this.mouseleave,this));this.$ok.on("click",n.proxy(this.ok,this));this.$cancel.on("click",n.proxy(this.cancel,this))},mouseenter:function(){this.mouseover=!0},mouseleave:function(){this.mouseover=!1},focusin:function(){this.mouseover=!0},focusout:function(){this.mouseover=!1;var n=this;window.setTimeout(function(){n.mouseover||n.hide()},500)},ok:function(){this.items=n.merge(this.selected.selected(),this.found.selected());this.$element.trigger("filter.multiple.ok")},cancel:function(){this.$element.trigger("filter.multiple.cancel")},show:function(n,t,i){this.items.length>0&&this.selected.show(this.items,i,!0);n.length>0&&this.found.show(n,i,!1,t);(this.items.length>0||n.length>0)&&(this.$actions.show(),this.$element.show())},hide:function(){this.selected.hide();this.found.hide();this.$actions.hide();this.$element.hide()}};t.MultipleFilter=function(n,i,r,u,f,e){this.selector=new t.MultipleSelector(this);this.short=!1;this.useContains=!1;this.dataProvider=e;t.AbstractFilter.call(this,n,i,r,u,f)};t.MultipleFilter.prototype=n.extend({},t.AbstractFilter.prototype,{dataProvider:null,match:function(n){var t;return t=this.useContains?new RegExp("contains\\(\\s+"+this.field+"\\s+,\\s+'([^']+)'\\s+\\)","g"):new RegExp(this.field+"\\s+eq\\s+'([^']+)'","g"),t.test(n)},listen:function(){this.$container.attr("short")&&(this.short=!0);this.$container.attr("useContains")&&(this.useContains=!0);this.$query.on("focus",n.proxy(this.focus,this)).on("keyup",n.proxy(this.keyup,this)).on("blur",n.proxy(this.blur,this));this.$clear.on("click",n.proxy(this.clear,this));this.selector.$element.on("filter.multiple.ok",n.proxy(this.go,this)).on("filter.multiple.cancel",n.proxy(this.cancel,this))},cancel:function(){this.hide()},go:function(){this.hide();this.search()},blur:function(){var n=this;window.setTimeout(function(){n.selector.mouseover||n.hide()},500)},message:function(){this.selector.items.length>0?this.$query.val("Selected: "+this.selector.items.length):this.$query.val(this.watermark())},hide:function(){this.message();this.selector.hide()},lookup:function(){var u=this.$query,f=this.selector,r=this.field,v=this.substitutions,e=this.dataProvider,a=function(t){var e,i;t.length>0&&(e=n.extend({},u.position(),{height:u[0].offsetHeight}),f.$element.insertAfter(u).css({top:e.top-8,left:e.left}),i=[],n.each(t,function(t,u){u[r]===""&&(u[r]="(Blank)");n.inArray(u[r],i)==-1&&n.inArray(u[r],f.items)==-1&&i.push(u[r])}),f.show(i,u.val(),v))},h,o,c,s,l;u.val().length!=0||this.short?e?(h=[],typeof e=="function"?o=e():Array.isArray(e)&&(o=e),o&&(n.each(o,function(n,t){var i={};i[r]=t;h.push(i)}),a(h))):(c="&$filter=",s="startswith(tolower("+r+"), tolower('"+t.odata.escapeParam(u.val())+"'))",s+=" or ",s+="contains(tolower("+r+"),tolower('"+t.odata.escapeParam(u.val())+"'))",c+=encodeURIComponent(s),l="/api/odata/"+cmt3.conference.name+"/"+this.model+"?$select="+r,this.short||(l+=c),i.request({requestUri:l},function(n){a(n.value)})):f.items.length==0?f.hide():f.found.hide()},reject:function(){this.hide();this.message()},focus:function(){this.$query.val("");this.selector.show([]);this.short&&this.lookup()},keyup:function(n){switch(n.keyCode){case 40:case 38:case 16:case 17:case 18:case 13:case 9:break;case 27:this.reject();break;default:this.lookup()}n.stopPropagation();n.preventDefault()},reset:function(){this.selector.items=[];this.hide()},state:function(n){return n&&(this.selector.items=n==this.watermark()?[]:n),this.selector.items},setValue:function(n){for(var f,e,r=n.split(" or "),u=[],i=0;i<r.length;i++)f=this.useContains?new RegExp("contains\\(\\s+"+this.field+"\\s+,\\s+'([^']+)'\\s+\\)","g"):new RegExp(this.field+"\\s+eq\\s+'([^']+)'","g"),e=f.exec(r[i].trim()),u.push(t.odata.unescapeParam(e[1]));this.state(u);this.message()},getValue:function(){var r=this,i="",u;return u=this.useContains?function(n,u){i+=(i==""?"":" or ")+"contains("+r.field+",'"+t.odata.escapeParam(u)+"')"}:function(n,u){i+=(i==""?"":" or ")+r.field+" eq '"+t.odata.escapeParam(u)+"'"},n.each(this.selector.items,function(n,t){u(n,t!=="(Blank)"?t:"")}),i==""?null:"("+i+")"},watermark:function(){return"сlick here..."},help:function(){return"Focus on this text box and select options and then press Enter."}});t.ComposedFilter=function(n,i,r,u,f){t.AbstractFilter.call(this,n,i,r,u,f)};t.ComposedFilter.prototype=n.extend({},t.AbstractFilter.prototype,{match:function(){return!1},getValue:function(){return null}});t.YesNoFilter=function(n,i,r,u,f){t.MultipleFilter.call(this,n,i,r,u,f,function(){return["Yes","No"]})};t.YesNoFilter.prototype=n.extend({},t.MultipleFilter.prototype);t.TrueFalseFilter=function(n,i,r,u,f){t.MultipleFilter.call(this,n,i,r,u,f||{"true":"Yes","false":"No"},function(){return["true","false"]})};t.TrueFalseFilter.prototype=n.extend({},t.MultipleFilter.prototype,{getValue:function(){var i=this,t="";return n.each(this.selector.items,function(n,r){r!=="(Blank)"&&(t+=(t===""?"":" or ")+i.field+" eq "+r)}),t===""?null:"("+t+")"},setValue:function(n){for(var u,f,i=n.split(" or "),r=[],t=0;t<i.length;t++)u=new RegExp(this.field+"\\s+eq\\s+(true|false)","g"),f=u.exec(i[t].trim()),r.push(f[1]);this.state(r);this.message()}});ko.bindingHandlers.filter={update:function(n,i,r,u,f){var e=i(),o=e.bindingContext||f.$data,h=e.property,c=e.substitutions,l=e.dataProvider,a=e.doNotLower,v=t.capitalize(e.type)+"Filter",y=o.controller,s=new window.app[v](o.$element,n,y,h,c,l);s.hasOwnProperty("doNotLower")&&(s.doNotLower=a);o.filters||(o.filters=[]);o.filters.push(s)}}})(window.jQuery,window.app,window.OData),function(n,t,i){"use strict";function u(){var n=this;n.id=t.autoMap();n.name=t.autoMap();n.submissionCount=t.autoMap();n.statuses=[];n.selectedStatus=ko.observable()}function r(n,r,u,f){var e=this,h,c,s,l,a,o;for(e.id=n.Id,e.title=n.Title,e.abstract=n.Abstract.htmlMultiLineEncode(),e.authors={primary:n.Author},e.authorList=n.Authors,e.numberOfUnregisteredAuthors=n.NumberOfUnregisteredAuthors,e.track={name:n.Track,id:n.TrackId},e.isSingleTrackConference=n.IsSingleTrackConference,e.subjects={primary:n.PrimarySubject,secondary:n.SecondarySubject},e.status=n.Status,e.statusPropertyIsRevision=n.StatusPropertyIsRevision,e.originalSubmissionId=n.OriginalSubmissionId,e.hasRevision=ko.observable(n.HasRevision),e.numberOfFiles=n.NumberOfFiles,e.numberOfSupplementaryFiles=n.NumberOfSupplementaryFiles,e.isReviewReadOnly=ko.observable(n.IsReviewReadOnly),e.isMetaReviewReadOnly=ko.observable(n.IsMetaReviewReadOnly),e.isCameraReady=ko.observable(n.IsCameraReady),e.isCameraReadyPosted=n.IsCameraReadyPosted,e.isPresentation=ko.observable(n.IsPresentation),e.inplaceRevisionSubmitted=ko.observable(n.InplaceRevisionSubmitted),e.isAuthorFeedback=n.IsAuthorFeedback,e.isAuthorFeedbackPosted=n.IsAuthorFeedbackPosted,e.authorFeedbackId=n.AuthorFeedbackId,e.conflicts=n.Conflicts,e.disputedConflicts=n.DisputedConflicts,e.reviewerList=n.Reviewers,e.assigned=n.Assigned,e.completed=n.Completed,e.percentage=n.Percentage,e.bids=n.Bids,e.metaReviewerList=n.MetaReviewers,e.metaReviewers=n.MetaReviewersJson?JSON.parse(n.MetaReviewersJson):[],e.metaAssigned=n.MetaAssigned,e.metaCompleted=n.MetaCompleted,e.metaPercentage=n.MetaPercentage,e.metaBids=n.MetaBids,e.seniorMetaReviewerList=n.SeniorMetaReviewers,e.seniorMetaReviewers=n.SeniorMetaReviewersJson?JSON.parse(n.SeniorMetaReviewersJson):[],e.numberOfSeniorMetaReviewers=n.NumberOfSeniorMetaReviewers,e.numberOfSeniorMetaReviewerRatings=n.NumberOfSeniorMetaReviewerRatings,e.avgSeniorMetaReviewerRating=n.AvgSeniorMetaReviewerRating,e.numberOfReviewerNotes=n.NumberOfReviewerNotes,e.numberOfMetaReviewerNotes=n.NumberOfMetaReviewerNotes,e.numberOfSeniorMetaReviewerNotes=n.NumberOfSeniorMetaReviewerNotes,e.numberOfSharedRecommendations=n.NumberOfSharedRecommendations,e.sharedRecommendations=n.SharedRecommendationsJson?JSON.parse(n.SharedRecommendationsJson):[],e.discussion={messages:n.Messages,enabled:ko.observable(n.DiscussionEnabled)},e.completedReviewRating=n.CompletedReviewRating,e.percentageReviewRating=n.PercentageReviewRating,e.isReviewReadOnlyText=ko.pureComputed(function(){return e.isReviewReadOnly()?"Yes":"No"}),e.isMetaReviewReadOnlyText=ko.pureComputed(function(){return e.isMetaReviewReadOnly()?"Yes":"No"}),e.inplaceRevisionSubmittedText=ko.pureComputed(function(){return e.statusPropertyIsRevision?e.inplaceRevisionSubmitted()?"Yes":"No":""}),e.hasRevisionText=ko.pureComputed(function(){return e.statusPropertyIsRevision?e.hasRevision()?"Yes":"No":""}),e.isAuthorFeedbackText=ko.pureComputed(function(){return e.isAuthorFeedback?"Yes":"No"}),e.isAuthorFeedbackPostedText=ko.pureComputed(function(){return e.isAuthorFeedbackPosted?"Yes":"No"}),e.isCameraReadyText=ko.pureComputed(function(){return e.isCameraReady()?"Yes":"No"}),e.isCameraReadyPostedText=ko.pureComputed(function(){return e.isCameraReadyPosted?"Yes":"No"}),e.isPresentationText=ko.pureComputed(function(){return e.isPresentation()?"Yes":"No"}),e.revisionTracks=f,e.chairNoteColumns=[],n.CNQ01Id!==null?e.chairNoteColumns.push(new t.QuestionResponseColumn(n.CNQ01Id,n.CNQ01Text)):e.chairNoteColumns.push(null),n.CNQ02Id!==null?e.chairNoteColumns.push(new t.QuestionResponseColumn(n.CNQ02Id,n.CNQ02Text)):e.chairNoteColumns.push(null),n.CNQ03Id!==null?e.chairNoteColumns.push(new t.QuestionResponseColumn(n.CNQ03Id,n.CNQ03Text)):e.chairNoteColumns.push(null),n.CNQ04Id!==null?e.chairNoteColumns.push(new t.QuestionResponseColumn(n.CNQ04Id,n.CNQ04Text)):e.chairNoteColumns.push(null),n.CNQ05Id!==null?e.chairNoteColumns.push(new t.QuestionResponseColumn(n.CNQ05Id,n.CNQ05Text)):e.chairNoteColumns.push(null),n.CNQ06Id!==null?e.chairNoteColumns.push(new t.QuestionResponseColumn(n.CNQ06Id,n.CNQ06Text)):e.chairNoteColumns.push(null),n.CNQ07Id!==null?e.chairNoteColumns.push(new t.QuestionResponseColumn(n.CNQ07Id,n.CNQ07Text)):e.chairNoteColumns.push(null),n.CNQ08Id!==null?e.chairNoteColumns.push(new t.QuestionResponseColumn(n.CNQ08Id,n.CNQ08Text)):e.chairNoteColumns.push(null),h=[],c=!1,s=0;s<u.length;s++)l=e.chairNoteColumns[s],h.push(l),l&&(c=!0);for(e.chairNoteColumns=h,e.noteLinkText=c?"Edit Note":"Add Note",e.aggregateColumns=[],s=0;s<r.length;s++)a=r[s],o="Q0"+a.Order,a.IsMeta&&(o="M"+o),n[o+"Id"]!==null?e.aggregateColumns.push(new t.AggregateColumn(o,n[o+"Id"],n[o+"Avg"],n[o+"Min"],n[o+"Max"],n[o+"Spread"])):e.aggregateColumns.push(new t.AggregateColumn(o,null,null,null,null,null));e.revisionClick=function(n,r){var u={requestUri:t.odata.getUrl(t.odata.entitySet.submissions,null,"Revision"),method:"POST",data:{Request:{SubmissionId:n,RevisionTrackId:r}}};i.request(u,function(i){e.hasRevision=!0;t.addMessage("Created revision id={1} for submission id={0}.".format(n,i.value))},function(n){i.defaultError(n)})}}function f(r,f){var o=f,e=this;e.tracks=ko.observableArray();e.submitEnabled=ko.computed(function(){var t,n;if(e.tracks().length<=0)return!1;for(t=!0,n=0;n<e.tracks().length;n++)t=t&&e.tracks()[n].selectedStatus()!==undefined&&typeof e.tracks()[n].selectedStatus()[0]!="undefined";return t});e.filter=null;e.changeStatus=function(){for(var f,h,c,s=[],u=0;u<e.tracks().length;u++)f=e.tracks()[u],s.push({TrackId:f.id,StatusId:f.selectedStatus()[0]});h={TrackStatusMap:s,Filter:e.filter};c={requestUri:t.odata.getUrl(t.odata.entitySet.trackStatuses,null,"BulkChangeStatus"),method:"POST",data:{Request:h}};i.request(c,function(){o.refresh();setTimeout(function(){t.addMessage("The status of selected submissions have been changed.")},500);n(r).modal("hide")})};e.bind=function(){ko.applyBindings(e,r)};e.editInDialog=function(f){i.read(t.odata.getUrl(t.odata.entitySet.trackStatuses+"?filter="+encodeURIComponent(f)+"&$expand=Statuses"),function(i){var o,s,c,h,l,a;for(e.tracks.removeAll(),o=0;o<i.value.length;o++){for(s=i.value[o],c=t.autoMap(new u,s),h=0;h<s.Statuses.length;h++)l=s.Statuses[h],a=t.autoMap(new t.SubmissionStatus,l),c.statuses.push(a);e.tracks.push(c)}e.filter=f;n(r).modal("show")})}}function e(r,u){var e=u,f=this;f.id=ko.observable("");f.title=ko.observable("");f.trackName=ko.observable("");f.isSingleTrackConference=ko.observable(!0);f.deleteSubmission=function(){var u={requestUri:t.odata.getUrl(t.odata.entitySet.submissions,f.id()),method:"DELETE",showProgressIndicator:!1};i.request(u,function(){n(r).modal("hide");e.refresh();setTimeout(function(){t.addMessage("Submission {0} has been deleted.".format(f.id()))},500)})};f.bind=function(){ko.applyBindings(f,r)};f.editInDialog=function(t){f.id(t.id);f.title(t.title);f.trackName(t.track.name);f.isSingleTrackConference(t.isSingleTrackConference);n(r).modal("show")}}r.prototype={setEnable:function(n){var r=!n.discussion.enabled(),u={requestUri:t.odata.getUrl(t.odata.entitySet.submissions,null,"EnableDisableDiscussion"),method:"POST",showProgressIndicator:!0,data:{Enable:r,SubmissionId:n.id}};i.request(u,function(){n.discussion.enabled(r);t.addMessage("Author feedback for submission {0} has been {1}!".format(n.id,r?"enabled":"disabled"))})}};t.SubmissionPage=function(i,r,u,o,s,h,c,l,a){var v=this,y,p;v.toggleableColumnsContainer=new t.ToggleableColumnsContainer(v.key);v.tracks=u;v.defaultTrackId=o;v.questions=s;v.chairNoteQuestions=h;v.statusNames=c;v.hasRevisionTracks=l;v.hasSeniorMetaReviewer=a;v.$element=n(i);v.conference=window.cmt3.conference.name;v.page=ko.observable(1);v.top=ko.observable(25);v.sort=ko.observable("Id");v.controller=r;v.filters=[];v._total=ko.observable(0);v.selected=ko.observable(0);v.submissions=ko.observableArray();v.status=ko.observable();v.editingStatus=ko.observable(!1);v.isCameraReady=ko.observable();v.listen();v.Pager=ko.pager(v.selected,v.top);v.Pager().CurrentPage.subscribe(function(){v.page(v.Pager().CurrentPage());v.show()});y=null;v.deleteSubmission=function(n){y===null&&(y=new e(document.getElementById("deleteSubmissionDialog"),v),y.bind());y.editInDialog(n)};p=null;v.changeStatus=function(n){p===null&&(p=new f(document.getElementById("changeStatusDialog"),v),p.bind());p.editInDialog(n)};v.allowSupplementaryMaterial=ko.computed(function(){for(var n in v.tracks)if(v.tracks[n].settings.allowSupplementaryMaterial)return!0;return!1});v.trackArray=ko.computed(function(){var n=[];for(var t in v.tracks)n.push(v.tracks[t]);return n.sort(function(n,t){return n.order<t.order?-1:n.order>t.order?1:n.name.toLowerCase()<t.name.toLowerCase()?-1:n.name.toLowerCase()>t.name.toLowerCase()?1:0})});v.allowInplaceRevision=ko.computed(function(){for(var n in v.tracks)if(v.tracks[n].settings.allowInplaceRevision)return!0;return!1});v.trackNamesProvider=function(){var t=[];return n.each(v.tracks,function(n,i){t.push(i.name)}),t};v.statusNamesProvider=function(){var n=v.statusNames;return n.sort(),n};v.reviewerAllowedToCompareSubmission=ko.computed(function(){for(var n in v.tracks)if(v.tracks[n].settings.reviewerAllowedToCompareSubmission)return!0;return!1});v.metaReviewerAllowedToCompareSubmission=ko.computed(function(){for(var n in v.tracks)if(v.tracks[n].settings.metaReviewerAllowedToCompareSubmission)return!0;return!1});v.metaReviewerEnabled=ko.computed(function(){for(var n in v.tracks)if(v.tracks[n].settings.metaReviewerEnabled)return!0;return!1});v.cameraReadyEnabled=ko.computed(function(){for(var n in v.tracks)if(v.tracks[n].settings.cameraReadyEnabled)return!0;return!1});v.authorFeedbackEnabled=ko.computed(function(){for(var n in v.tracks)if(v.tracks[n].settings.authorFeedbackEnabled)return!0;return!1});v.subjectAreaConfigured=ko.computed(function(){for(var n in v.tracks)if(v.tracks[n].settings.subjectAreaConfigured)return!0;return!1});v.inplaceRevisionEnabled=ko.computed(function(){for(var n in v.tracks)if(v.tracks[n].settings.inplaceRevisionEnabled)return!0;return!1})};t.SubmissionPage.prototype={key:"submissions",listen:function(){var t=this;n(document).on("data.filter",function(){t.Pager().CurrentPage()<2?t.show():t.Pager().CurrentPage(1)})},getDefaultTrackId:function(){return this.defaultTrackId},getFilter:function(){var t="";return n.each(this.filters,function(n,i){i.getValue()&&(t+=t===""?i.getValue():" and "+i.getValue())}),t},show:function(u,f,e,o,s){var h=this,c=function(u){var c=f?f:h.sort(),l=e?e:h.getFilter(),a=o?o:h.skip(),v=typeof s!="undefined"&&s!==null?s:h.top(),p=c?"&$orderby="+c:"",w=v?"&$top="+v:"",b=a?"&$skip="+a:"",y=l?"&$filter="+encodeURIComponent(l):"",k={headers:{Accept:"application/json"},requestUri:"/api/odata/"+h.conference+"/$batch",showProgressIndicator:!u,method:"POST",data:{requests:[{url:"/api/odata/"+h.conference+"/"+h.controller+"?"+(u?"$count=true&$top=0"+y:p+y+b+w),method:"GET",headers:{Accept:"application/json"}}]}};return i.request(k,function(i){var f,y,e,o,s;t.page.saveState("submissions",{sort:c,top:v,skip:a,filter:l});f=i.responses[0].body;u?(s=f["@odata.count"],h._total()===0&&h._total(s),h.selected(s),h.toggleableColumnsContainer&&h.toggleableColumnsContainer.loadState()):(y=f.value,e=[],n.each(h.tracks,function(n,t){e[t.id]=t}),o=[],n.each(y,function(t,i){var u=[];i.Revisions!==""&&n.each(i.Revisions.split(";"),function(n,t){var i=e[parseInt(t)];i!==null&&u.push(i)});o.push(new r(i,h.questions,h.chairNoteQuestions,u))}),h.submissions(o))},function(n){window.cmt3.logger.log(n.message)},i.batchHandler)};(h.initialized||u)&&n.when(c(!1),c(!0)).done(function(){n("html,body").scrollTop(0)})},scroll:function(){n(window).scrollTop()===n(document).height()-n(window).height()&&self.show()},selectStatus:function(t,i){var r=n(i.target),f=ko.contextFor(i.target),u=n(n("#statusTemplate").text());r.hide();r.after(u);f.$parent.getStatuses(t.id,t.track.id,r,u).done(function(n){ko.applyBindings(n,u[0])})},getStatuses:function(r,u,f,e){var o=n.Deferred();return i.read(t.odata.getUrl(t.odata.entitySet.submissionStatuses),function(n){for(var v,s,c,l=[],a=[],h=0;h<n.value.length;h++)v=n.value[h],s=t.autoMap(new t.SubmissionStatus,v),s.trackId===u&&(l.push(s),a[s.id]=s);c={options:ko.observableArray(l),selectedStatus:ko.observable()};c.selectedStatus.subscribe(function(n){var t={requestUri:"/api/odata/"+window.cmt3.conference.name+"/Submissions("+r+")",method:"PATCH",headers:{Prefer:"return-content"},progressIndicatorTimeout:0,data:{StatusId:n[0]}};i.request(t,function(n){e.remove();f.text(a[n.StatusId].name);f.show()})});o.resolve(c)}),o.promise()},importChairNotes:function(i,r){var u=r.target,f=n(u).attr("order"),e="/"+window.cmt3.conference.name+"/Submission/ImportChairNote?order="+f;t.url.navigateTo(e)},changeIsReviewReadOnly:function(t,i){var r=n(i.target),e=ko.contextFor(i.target),u=n(n("#isReviewReadOnlyTemplate").text()),f;r.hide();r.after(u);f=e.$parent.getIsReviewReadOnly(t.id,r,u);ko.applyBindings(f,u[0])},getIsReviewReadOnly:function(n,t,r){var u=[{name:"Yes",id:!0},{name:"No",id:!1}],f={options:ko.observableArray(u),selectedOption:ko.observable()};return f.selectedOption.subscribe(function(f){var e={requestUri:"/api/odata/"+window.cmt3.conference.name+"/Submissions("+n+")",method:"PATCH",headers:{Prefer:"return-content"},progressIndicatorTimeout:0,data:{IsReviewReadOnly:f[0]}};i.request(e,function(n){r.remove();t.text(n.IsReviewReadOnly?u[0].name:u[1].name);t.show()})}),f},changeIsMetaReviewReadOnly:function(t,i){var r=n(i.target),e=ko.contextFor(i.target),u=n(n("#isReviewReadOnlyTemplate").text()),f;r.hide();r.after(u);f=e.$parent.getIsMetaReviewReadOnly(t.id,r,u);ko.applyBindings(f,u[0])},getIsMetaReviewReadOnly:function(n,t,r){var u=[{name:"Yes",id:!0},{name:"No",id:!1}],f={options:ko.observableArray(u),selectedOption:ko.observable()};return f.selectedOption.subscribe(function(f){var e={requestUri:"/api/odata/"+window.cmt3.conference.name+"/Submissions("+n+")",method:"PATCH",headers:{Prefer:"return-content"},progressIndicatorTimeout:0,data:{IsMetaReviewReadOnly:f[0]}};i.request(e,function(n){r.remove();t.text(n.IsMetaReviewReadOnly?u[0].name:u[1].name);t.show()})}),f},changeIsAuthorFeedback:function(t,i){var r=n(i.target),e=ko.contextFor(i.target),u=n(n("#isAuthorFeedbackTemplate").text()),f;r.hide();r.after(u);f=e.$parent.getIsAuthorFeedback(t.id,r,u);ko.applyBindings(f,u[0])},getIsAuthorFeedback:function(n,t,r){var u=[{name:"Yes",id:!0},{name:"No",id:!1}],f={options:ko.observableArray(u),selectedOption:ko.observable()};return f.selectedOption.subscribe(function(f){var e={requestUri:"/api/odata/"+window.cmt3.conference.name+"/Submissions("+n+")",method:"PATCH",headers:{Prefer:"return-content"},progressIndicatorTimeout:0,data:{IsAuthorFeedback:f[0]}};i.request(e,function(n){r.remove();t.text(n.IsAuthorFeedback?u[0].name:u[1].name);t.show()})}),f},changeIsCameraReady:function(t,i){var r=n(i.target),f=ko.contextFor(i.target),u=n(n("#isCameraReadyTemplate").text()),e;r.hide();r.after(u);e=f.$parent.getIsCameraReady(t.id,r,u,f.$data);ko.applyBindings(e,u[0])},getIsCameraReady:function(n,t,r,u){var f={options:ko.observableArray([{name:"Yes",id:!0},{name:"No",id:!1}]),selectedOption:ko.observable()};return f.selectedOption.subscribe(function(f){var e={requestUri:"/api/odata/"+window.cmt3.conference.name+"/Submissions("+n+")",method:"PATCH",headers:{Prefer:"return-content"},progressIndicatorTimeout:0,data:{IsCameraReady:f[0]}};i.request(e,function(n){r.remove();u.isCameraReady(n.IsCameraReady);t.show()})}),f},changeIsPresentation:function(t,i){var r=n(i.target),f=ko.contextFor(i.target),u=n(n("#isPresentationTemplate").text()),e;r.hide();r.after(u);e=f.$parent.getIsPresentation(t.id,r,u,f.$data);ko.applyBindings(e,u[0])},getIsPresentation:function(n,r,u,f){var e={options:ko.observableArray([{name:"Yes",id:!0},{name:"No",id:!1}]),selectedOption:ko.observable()};return e.selectedOption.subscribe(function(e){var s="Id eq {0}".format(n),o=e[0],h={requestUri:t.odata.getUrl(t.odata.entitySet.presentations,null,"BulkEnableDisablePresentation"),method:"POST",progressIndicatorTimeout:0,data:{Filter:s,Enable:o}};i.request(h,function(){u.remove();f.isPresentation(o);r.show()})}),e},showAbstract:function(t,i){var f=ko.contextFor(i.target).$parent,r=n(i.target),u=r.next();u.is(":visible")?(u.hide(),r.text("Show abstract")):(u.show(),r.text("Hide abstract"))},email:function(i,r){var u=r.target,l=ko.contextFor(u),o=parseInt(n(u).attr("sid")),a=n(u).attr("recipientType"),s=n(u).attr("all"),h=n(u).attr("checkNote"),e,c,f;e=o?"Id eq {0}".format(o):l.$root.getFilter();c="/"+window.cmt3.conference.name+"/Submission/SendEmail/"+a;f={filter:e.length>0?e:null};s&&(f.all=s);h&&(f.checkNote=h);t.url.navigateTo(c,f)},bulkEnableDisablePresentation:function(r,u,f){var e=f?"enabling":"disabling",c;if(confirm("Bulk {0} Presentation will be performed for selected items.".format(e))){var o=u.target,l=ko.contextFor(o),s=parseInt(n(o).attr("sid")),h;h=s?"Id eq {0}".format(s):l.$root.getFilter();c={requestUri:t.odata.getUrl(t.odata.entitySet.presentations,null,"BulkEnableDisablePresentation"),method:"POST",showProgressIndicator:!0,data:{Filter:h,Enable:f}};i.request(c,function(){t.addMessage("Bulk {0} Presentation has been completed successfully.".format(e));location.reload()})}},bulkEnableDisableCameraReady:function(r,u,f){var e=f?"enabling":"disabling",c;if(confirm("Bulk {0} Camera Ready will be performed for selected items.".format(e))){var o=u.target,l=ko.contextFor(o),s=parseInt(n(o).attr("sid")),h;h=s?"Id eq {0}".format(s):l.$root.getFilter();c={requestUri:t.odata.getUrl(t.odata.entitySet.cameraReadySubmissions,null,"BulkEnableDisableCameraReady"),method:"POST",showProgressIndicator:!0,data:{Filter:h,Enable:f}};i.request(c,function(){t.addMessage("Bulk {0} Camera Ready has been completed successfully.".format(e));location.reload()})}},bulkEnableDisableAuthorFeedback:function(r,u,f){var e=f?"enabling":"disabling",c;if(confirm("Bulk {0} author feedback will be performed for selected items.".format(e))){var o=u.target,l=ko.contextFor(o),s=parseInt(n(o).attr("sid")),h;h=s?"Id eq {0}".format(s):l.$root.getFilter();c={requestUri:t.odata.getUrl(t.odata.entitySet.authorFeedbacks,null,"BulkEnableDisableAuthorFeedback"),method:"POST",showProgressIndicator:!0,data:{Filter:h,Enable:f}};i.request(c,function(){t.addMessage("Bulk {0} author feedback has been completed successfully.".format(e));location.reload()})}},bulkDeleteAssign:function(r,u,f){var e=f===t.enums.assignmentType.reviewer?"reviewer":f===t.enums.assignmentType.metaReviewer?"meta-reviewer":"senior meta-reviewer",c;if(confirm("Bulk delete {0} assignment will be performed for selected items.".format(e))){var o=u.target,l=ko.contextFor(o),s=parseInt(n(o).attr("sid")),h;h=s?"Id eq {0}".format(s):l.$root.getFilter();c={requestUri:t.odata.getUrl(t.odata.entitySet.submissions,null,"BulkDeleteAssignment"),method:"POST",showProgressIndicator:!0,data:{Filter:h,Type:f}};i.request(c,function(){t.addMessage("Bulk delete {0} assignment has been completed successfully.".format(e));location.reload()})}},bulkDeleteSubmissions:function(r,u){var s;if(confirm("Bulk delete submissions will be performed for selected items.")){var f=u.target,h=ko.contextFor(f),e=parseInt(n(f).attr("sid")),o;o=e?"Id eq {0}".format(e):h.$root.getFilter();s={requestUri:t.odata.getUrl(t.odata.entitySet.submissions,null,"BulkDeleteSubmissions"),method:"POST",showProgressIndicator:!0,data:{Filter:o}};i.request(s,function(){t.addMessage("Bulk delete submissions has been completed successfully.");location.reload()})}},bulkEnableDisableDiscussion:function(r,u,f){var e=f?"enabling":"disabling",c;if(confirm("Bulk {0} discussion will be performed for selected items.".format(e))){var o=u.target,l=ko.contextFor(o),s=parseInt(n(o).attr("sid")),h;h=s?"Id eq {0}".format(s):l.$root.getFilter();c={requestUri:t.odata.getUrl(t.odata.entitySet.submissions,null,"BulkEnableDisableDiscussion"),method:"POST",showProgressIndicator:!0,data:{Filter:h,Enable:f}};i.request(c,function(){t.addMessage("Bulk {0} discussion has been completed successfully.".format(e));location.reload()})}},bulkEnableDisableReviewReadOnly:function(r,u,f,e){var o=f?"enabling":"disabling",l;if(confirm("Bulk {0} {1} readOnly will be performed for selected submissions.".format(o,e?"meta-review":"review"))){var s=u.target,a=ko.contextFor(s),h=parseInt(n(s).attr("sid")),c;c=h?"Id eq {0}".format(h):a.$root.getFilter();l={requestUri:t.odata.getUrl(t.odata.entitySet.submissions,null,e?"BulkEnableDisableMetaReviewReadOnly":"BulkEnableDisableReviewReadOnly"),method:"POST",showProgressIndicator:!0,data:{Filter:c,Enable:f}};i.request(l,function(){t.addMessage("Bulk {0} {1} readOnly has been completed successfully.".format(o,e?"meta-review":"review"));location.reload()})}},bulkEnableAuthorFeedback:function(n,t){this.bulkEnableDisableAuthorFeedback(n,t,!0)},bulkDisableAuthorFeedback:function(n,t){this.bulkEnableDisableAuthorFeedback(n,t,!1)},bulkEnableDiscussion:function(n,t){this.bulkEnableDisableDiscussion(n,t,!0)},bulkDisableDiscussion:function(n,t){this.bulkEnableDisableDiscussion(n,t,!1)},exportReproducibilityResponsesForSubmission:function(n,t){this.exportReproducibilityResponses(n,t,!1)},exportReproducibilityResponsesForCameraReady:function(n,t){this.exportReproducibilityResponses(n,t,!0)},bulkEnableCameraReady:function(n,t){this.bulkEnableDisableCameraReady(n,t,!0)},bulkDisableCameraReady:function(n,t){this.bulkEnableDisableCameraReady(n,t,!1)},bulkEnablePresentation:function(n,t){this.bulkEnableDisablePresentation(n,t,!0)},bulkDisablePresentation:function(n,t){this.bulkEnableDisablePresentation(n,t,!1)},bulkDeleteReviewerAssignment:function(n,i){this.bulkDeleteAssign(n,i,t.enums.assignmentType.reviewer)},bulkDeleteMetaReviewerAssignment:function(n,i){this.bulkDeleteAssign(n,i,t.enums.assignmentType.metaReviewer)},bulkDeleteSeniorMetaReviewerAssignment:function(n,i){this.bulkDeleteAssign(n,i,t.enums.assignmentType.seniorMetaReviewer)},bulkEnableReviewReadOnly:function(n,t){this.bulkEnableDisableReviewReadOnly(n,t,!0,!1)},bulkDisableReviewReadOnly:function(n,t){this.bulkEnableDisableReviewReadOnly(n,t,!1,!1)},bulkEnableMetaReviewReadOnly:function(n,t){this.bulkEnableDisableReviewReadOnly(n,t,!0,!0)},bulkDisableMetaReviewReadOnly:function(n,t){this.bulkEnableDisableReviewReadOnly(n,t,!1,!0)},exportMetaReviews:function(i,r){var u=r.target,h=ko.contextFor(u),f=parseInt(n(u).attr("sid")),e,o,s;e=f?"Id eq {0}".format(f):h.$root.getFilter();o="/api/odata/"+window.cmt3.conference.name+"/SubmissionViews/ExportMetaReviews";s={Filter:e};t.page.post(o,s)},exportReviews:function(i,r){var u=r.target,h=ko.contextFor(u),f=parseInt(n(u).attr("sid")),e,o,s;e=f?"Id eq {0}".format(f):h.$root.getFilter();o="/api/odata/"+window.cmt3.conference.name+"/SubmissionViews/ExportReviews";s={Filter:e};t.page.post(o,s)},exportDiscussions:function(i,r){var u=r.target,h=ko.contextFor(u),f=parseInt(n(u).attr("sid")),e,o,s;e=f?"Id eq {0}".format(f):h.$root.getFilter();o="/api/odata/"+window.cmt3.conference.name+"/SubmissionViews/ExportDiscussions";s={Filter:e};t.page.post(o,s)},exportReviewsSnapshot:function(i,r){var u=r.target,h=ko.contextFor(u),f=parseInt(n(u).attr("sid")),e,o,s;e=f?"Id eq {0}".format(f):h.$root.getFilter();o="/api/odata/"+window.cmt3.conference.name+"/SubmissionViews/ExportReviewsSnapshot";s={Filter:e};t.page.post(o,s)},exportNotes:function(i,r,u){var e=r.target,l=ko.contextFor(e),o=parseInt(n(e).attr("sid")),s,f,h,c;s=o?"Id eq {0}".format(o):l.$root.getFilter();f=null;u===t.enums.userRole.reviewer?f="ExportReviewerNotes":u===t.enums.userRole.metaReviewer?f="ExportMetaReviewerNotes":u===t.enums.userRole.seniorMetaReviewer&&(f="ExportSeniorMetaReviewerNotes");h="/api/odata/"+window.cmt3.conference.name+"/SubmissionViews/"+f;c={Filter:s};t.page.post(h,c)},exportReviewerNotes:function(n,i){this.exportNotes(n,i,t.enums.userRole.reviewer)},exportMetaReviewerNotes:function(n,i){this.exportNotes(n,i,t.enums.userRole.metaReviewer)},exportSeniorMetaReviewerNotes:function(n,i){this.exportNotes(n,i,t.enums.userRole.seniorMetaReviewer)},exportCameraReadySubmissions:function(i,r){var u=r.target,h=ko.contextFor(u),f=parseInt(n(u).attr("sid")),e,o,s;e=f?"Id eq {0}".format(f):h.$root.getFilter();o="/api/odata/"+window.cmt3.conference.name+"/CameraReadySubmissionViews/Export";s={Filter:e};t.page.post(o,s)},exportSubmissions:function(i,r){var u=r.target,h=ko.contextFor(u),f=parseInt(n(u).attr("sid")),e,o,s;e=f?"Id eq {0}".format(f):h.$root.getFilter();o="/api/odata/"+window.cmt3.conference.name+"/SubmissionViews/Export";s={Filter:e};t.page.post(o,s)},exportSubmissionsAsTSV:function(i,r){var u=r.target,f=ko.contextFor(u),e=parseInt(n(u).attr("sid")),o,s,h;o=e?"Id eq {0}".format(e):f.$root.getFilter();s="/api/odata/"+window.cmt3.conference.name+"/SubmissionViews/ExportAsTSV";h={Filter:o,TrackId:f.$root.getDefaultTrackId()};t.page.post(s,h)},exportACMXml:function(i,r){var u=r.target,f=ko.contextFor(u),e=parseInt(n(u).attr("sid")),c=n(u).attr("data-tid")&&parseInt(n(u).attr("data-tid"))||f.$root.getDefaultTrackId(),o,s,h;o=e?"Id eq {0}".format(e):f.$root.getFilter();s="/api/odata/"+window.cmt3.conference.name+"/SubmissionViews/ExportACMXml";h={Filter:o,TrackId:c};t.page.post(s,h)},exportAuthorFeedback:function(i,r){var u=r.target,h=ko.contextFor(u),f=parseInt(n(u).attr("sid")),e,o,s;e=f?"Id eq {0}".format(f):h.$root.getFilter();o="/api/odata/"+window.cmt3.conference.name+"/SubmissionViews/ExportAuthorFeedback";s={Filter:e};t.page.post(o,s)},downloadFiles:function(r,u){var f=u.target,h=n(f).attr("href"),e=parseInt(n(f).attr("sid")),c=ko.contextFor(f),o,s;o=e?"Id eq {0}".format(e):c.$root.getFilter();s={requestUri:t.odata.getUrl(t.odata.entitySet.submissionViews,null,"GetIds"),method:"POST",showProgressIndicator:!0,data:{Filter:o}};i.request(s,function(n){var i=n.value.join("/"),r={Ids:i};t.page.post(h,r)});u.preventDefault()},exportBidsToExcel:function(){var n="/api/odata/"+window.cmt3.conference.name+"/BiddingModels/ExportExcel";t.page.post(n,{})},exportBidsToExcelWithAssignments:function(){var n="/api/odata/"+window.cmt3.conference.name+"/BiddingModels/ExportExcelWithAssignments";t.page.post(n,{})},exportMetaBidsToExcel:function(){var n="/api/odata/"+window.cmt3.conference.name+"/MetaBiddingModels/ExportExcel";t.page.post(n,{})},exportMetaBidsToExcelWithAssignments:function(){var n="/api/odata/"+window.cmt3.conference.name+"/MetaBiddingModels/ExportExcelWithAssignments";t.page.post(n,{})},exportMetaBidsToXml:function(){var n="/api/odata/"+window.cmt3.conference.name+"/MetaBiddingModels/ExportXml";t.page.post(n,{})},exportBidsToXml:function(){var n="/api/odata/"+window.cmt3.conference.name+"/BiddingModels/ExportXml";t.page.post(n,{})},exportMetaAssignmentsToXml:function(){var n="/api/odata/"+window.cmt3.conference.name+"/Submissions/ExportMetaAssignmentsXml";t.page.post(n,{})},exportSeniorMetaAssignmentsToXml:function(){var n="/api/odata/"+window.cmt3.conference.name+"/Submissions/ExportSeniorMetaAssignmentsXml";t.page.post(n,{})},exportAssignmentsToXml:function(){var n="/api/odata/"+window.cmt3.conference.name+"/Submissions/ExportAssignmentsXml";t.page.post(n,{})},exportReviewerConflicts:function(){var n="/api/odata/"+window.cmt3.conference.name+"/Submissions/ExportReviewerConflicts";t.page.post(n,{})},exportMetaReviewerConflicts:function(){var n="/api/odata/"+window.cmt3.conference.name+"/Submissions/ExportMetaReviewerConflicts";t.page.post(n,{})},exportReviewerRelevances:function(){var n="/api/odata/"+window.cmt3.conference.name+"/Submissions/ExportReviewerRelevances";t.page.post(n,{})},exportMetaReviewerRelevances:function(){var n="/api/odata/"+window.cmt3.conference.name+"/Submissions/ExportMetaReviewerRelevances";t.page.post(n,{})},exportSeniorMetaReviewerConflicts:function(){var n="/api/odata/"+window.cmt3.conference.name+"/Submissions/ExportSeniorMetaReviewerConflicts";t.page.post(n,{})},exportReviewerSuggestions:function(){var n="/api/odata/"+window.cmt3.conference.name+"/Submissions/ExportReviewerSuggestions";t.page.post(n,{})},exportReviewRatings:function(){var n="/api/odata/"+window.cmt3.conference.name+"/Submissions/ExportReviewRatings";t.page.post(n,{})},exportMetaReviewerRecommendations:function(){var n="/api/odata/"+window.cmt3.conference.name+"/Submissions/ExportMetaReviewerRecommendations";t.page.post(n,{})},exportSeniorMetaReviewerRatings:function(){var n="/api/odata/"+window.cmt3.conference.name+"/Submissions/ExportSeniorMetaReviewerRatings";t.page.post(n,{})},exportReviewerSubmissionComparisons:function(n,i){var r=t.GetEventFilter(i),u=t.odata.getUrl(t.odata.entitySet.submissionModels,null,"ExportReviewerSubmissionComparisons"),f={Filter:r};t.page.post(u,f)},exportMetaReviewerSubmissionComparisons:function(n,i){var r=t.GetEventFilter(i),u=t.odata.getUrl(t.odata.entitySet.submissionModels,null,"ExportMetaReviewerSubmissionComparisons"),f={Filter:r};t.page.post(u,f)},exportReproducibilityResponses:function(n,i,r){var u="/api/odata/"+window.cmt3.conference.name+"/Submissions/ExportReproducibilityResponses",f={IsCameraReady:r};t.page.post(u,f)},bulkChangeStatus:function(n,i){var r=t.GetEventFilter(i);this.changeStatus(r)},stub:function(){alert("Sorry, this feature is not implemented yet.")},reset:function(){n.each(this.filters,function(n,t){t.reset()});this.show()},size:function(t,i){var r,u,f;n("a",".show").removeClass("btn-success").css("color","#999999");n(i.currentTarget).addClass("btn-success").css("color","white");r=n(i.target).attr("size");u=parseInt(r);this.top(u);f=this.Pager().CurrentPage();this.Pager().CurrentPage(1);f===1&&this.show()},skip:function(){return(this.page()-1)*this.top()},prev:function(){this.top()!==0&&this.page()!==1&&(this.page(this.page()-1),this.show())},next:function(){this.top()===0||this.page()>this.selected()/this.top()||(this.page(this.page()+1),this.show())},setSort:function(t,i){var r=n(i.target),u=r.attr("data-sort");(u===null||u===undefined)&&(r=n(r.context.parentNode),u=r.attr("data-sort"));r.hasClass("selected")?this.sort().match(" desc$")?(this.sort(u+" asc"),r.find("i").removeClass("icon-arrow-down"),r.find("i").addClass("icon-arrow-up"),r.attr("aria-sort","ascending")):(this.sort(u+" desc"),r.find("i").removeClass("icon-arrow-up"),r.find("i").addClass("icon-arrow-down"),r.attr("aria-sort","descending")):(n("th[data-sort]").each(function(){n(this).find("i").removeClass("icon-arrow-up");n(this).find("i").removeClass("icon-arrow-down");n(this).removeClass("selected");r.removeAttr("aria-sort")}),r.find("i").removeClass("icon-arrow-down"),r.find("i").addClass("icon-arrow-up"),r.attr("aria-sort","ascending"),r.addClass("selected"),this.sort(u+" asc"));this.show()},refresh:function(){this.show()}}}(window.jQuery,window.app,window.OData),function(n,t,i){"use strict";function r(r,u){var f=this;f.oldPassword=ko.observable("").extend({required:!0,minLength:6}).autoMap();f.newPassword=ko.observable("").extend({required:!0,minLength:10}).autoMap();f.confirmPassword=ko.observable("").extend({required:!0,minLength:10,equal:{params:f.newPassword,message:"Passwords must be equal."}});f.showValidationWarning=ko.observable(!1);f.changePassword=function(){var u=!0,e=ko.validation.group(f,{deep:!0}),o,s;if(e().length>0&&(e.showAllMessages(),u=!1),!u){f.showValidationWarning(!0);return}o={OldPassword:f.oldPassword(),NewPassword:f.newPassword()};s={requestUri:t.odata.getGlobalUrl(t.odata.entitySet.users,null,"ChangePassword"),method:"POST",data:{Request:o}};i.request(s,function(){n(r).modal("hide");t.addMessage("Password has been changed.")},function(n){if(n.response.statusCode==403){var i=t.getODataErrorMessage(n).message;t.addMessage(i,"Change password failed:","error")}else t.addMessage("Change password failed.",null,"error")})};f.bind=function(){ko.applyBindings(f,r)};f.showDialog=function(){f.showValidationWarning(!1);f.oldPassword("");f.oldPassword.isModified(!1);f.newPassword("");f.newPassword.isModified(!1);f.confirmPassword("");f.confirmPassword.isModified(!1);n(r).modal("show");setTimeout(function(){n(u).focus()},600)}}t.userPassword=function(){var n=this,t,i;n.options={elementId:"userPassword"};t=null;n.changePassword=function(){t==null&&(t=new r(document.getElementById("changePasswordDialog"),document.getElementById("changePasswordDialog-oldPasswordTextbox"),n),t.bind());t.showDialog()};i=document.getElementById(n.options.elementId);i&&ko.applyBindings(n,i)}}(window.jQuery,window.app,window.OData),function(n){"use strict";var t=function(n,t){this.name=n;this.code=t},i=[new t("Afghanistan","AF"),new t("Åland Islands","AX"),new t("Albania","AL"),new t("Algeria","DZ"),new t("American Samoa","AS"),new t("Andorra","AD"),new t("Angola","AO"),new t("Anguilla","AI"),new t("Antarctica","AQ"),new t("Antigua and Barbuda","AG"),new t("Argentina","AR"),new t("Armenia","AM"),new t("Aruba","AW"),new t("Ascension Island","AC"),new t("Australia","AU"),new t("Austria","AT"),new t("Azerbaijan","AZ"),new t("Bahamas","BS"),new t("Bahrain","BH"),new t("Bangladesh","BD"),new t("Barbados","BB"),new t("Belarus","BY"),new t("Belgium","BE"),new t("Belize","BZ"),new t("Benin","BJ"),new t("Bermuda","BM"),new t("Bhutan","BT"),new t("Bolivia","BO"),new t("Bonaire","BQ"),new t("Bosnia and Herzegovina","BA"),new t("Botswana","BW"),new t("Bouvet Island","BV"),new t("Brazil","BR"),new t("British Indian Ocean Territory","IO"),new t("British Virgin Islands","VG"),new t("Brunei","BN"),new t("Bulgaria","BG"),new t("Burkina Faso","BF"),new t("Burundi","BI"),new t("Cabo Verde","CV"),new t("Cambodia","KH"),new t("Cameroon","CM"),new t("Canada","CA"),new t("Cayman Islands","KY"),new t("Central African Republic","CF"),new t("Chad","TD"),new t("Chile","CL"),new t("China","CN"),new t("Christmas Island","CX"),new t("Cocos (Keeling) Islands","CC"),new t("Colombia","CO"),new t("Comoros","KM"),new t("Congo","CG"),new t("Congo (DRC)","CD"),new t("Cook Islands","CK"),new t("Costa Rica","CR"),new t("Côte d'Ivoire","CI"),new t("Croatia","HR"),new t("Cuba","CU"),new t("Curaçao","CW"),new t("Cyprus","CY"),new t("Czechia","CZ"),new t("Denmark","DK"),new t("Djibouti","DJ"),new t("Dominica","DM"),new t("Dominican Republic","DO"),new t("Ecuador","EC"),new t("Egypt","EG"),new t("El Salvador","SV"),new t("Equatorial Guinea","GQ"),new t("Eritrea","ER"),new t("Estonia","EE"),new t("Ethiopia","ET"),new t("Falkland Islands","FK"),new t("Faroe Islands","FO"),new t("Fiji","FJ"),new t("Finland","FI"),new t("France","FR"),new t("French Guiana","GF"),new t("French Polynesia","PF"),new t("French Southern Territories","TF"),new t("Gabon","GA"),new t("Gambia, The","GM"),new t("Georgia","GE"),new t("Germany","DE"),new t("Ghana","GH"),new t("Gibraltar","GI"),new t("Greece","GR"),new t("Greenland","GL"),new t("Grenada","GD"),new t("Guadeloupe","GP"),new t("Guam","GU"),new t("Guatemala","GT"),new t("Guernsey","GG"),new t("Guinea","GN"),new t("Guinea-Bissau","GW"),new t("Guyana","GY"),new t("Haiti","HT"),new t("Heard Island and McDonald Islands","HM"),new t("Honduras","HN"),new t("Hong Kong SAR","HK"),new t("Hungary","HU"),new t("Iceland","IS"),new t("India","IN"),new t("Indonesia","ID"),new t("Iran","IR"),new t("Iraq","IQ"),new t("Ireland","IE"),new t("Isle of Man","IM"),new t("Israel","IL"),new t("Italy","IT"),new t("Jamaica","JM"),new t("Jan Mayen","SJ"),new t("Japan","JP"),new t("Jersey","JE"),new t("Jordan","JO"),new t("Kazakhstan","KZ"),new t("Kenya","KE"),new t("Kiribati","KI"),new t("Korea","KR"),new t("Kosovo","XK"),new t("Kuwait","KW"),new t("Kyrgyzstan","KG"),new t("Laos","LA"),new t("Latvia","LV"),new t("Lebanon","LB"),new t("Lesotho","LS"),new t("Liberia","LR"),new t("Libya","LY"),new t("Liechtenstein","LI"),new t("Lithuania","LT"),new t("Luxembourg","LU"),new t("Macao SAR","MO"),new t("Madagascar","MG"),new t("Malawi","MW"),new t("Malaysia","MY"),new t("Maldives","MV"),new t("Mali","ML"),new t("Malta","MT"),new t("Marshall Islands","MH"),new t("Martinique","MQ"),new t("Mauritania","MR"),new t("Mauritius","MU"),new t("Mayotte","YT"),new t("Mexico","MX"),new t("Micronesia","FM"),new t("Moldova","MD"),new t("Monaco","MC"),new t("Mongolia","MN"),new t("Montenegro","ME"),new t("Montserrat","MS"),new t("Morocco","MA"),new t("Mozambique","MZ"),new t("Myanmar","MM"),new t("Namibia","NA"),new t("Nauru","NR"),new t("Nepal","NP"),new t("Netherlands","NL"),new t("Netherlands Antilles (Former)","AN"),new t("New Caledonia","NC"),new t("New Zealand","NZ"),new t("Nicaragua","NI"),new t("Niger","NE"),new t("Nigeria","NG"),new t("Niue","NU"),new t("Norfolk Island","NF"),new t("North Macedonia","MK"),new t("North Korea","KP"),new t("Northern Mariana Islands","MP"),new t("Norway","NO"),new t("Oman","OM"),new t("Pakistan","PK"),new t("Palau","PW"),new t("Palestinian Authority","PS"),new t("Panama","PA"),new t("Papua New Guinea","PG"),new t("Paraguay","PY"),new t("Peru","PE"),new t("Philippines","PH"),new t("Pitcairn Islands","PN"),new t("Poland","PL"),new t("Portugal","PT"),new t("Puerto Rico","PR"),new t("Qatar","QA"),new t("Republic of Côte d'Ivoire","CI"),new t("Réunion","RE"),new t("Romania","RO"),new t("Russia","RU"),new t("Rwanda","RW"),new t("Saba","XS"),new t("Saint Barthélemy","BL"),new t("Saint Kitts and Nevis","KN"),new t("Saint Lucia","LC"),new t("Saint Martin","MF"),new t("Saint Pierre and Miquelon","PM"),new t("Saint Vincent and the Grenadines","VC"),new t("Samoa","WS"),new t("San Marino","SM"),new t("São Tomé and Príncipe","ST"),new t("Saudi Arabia","SA"),new t("Senegal","SN"),new t("Serbia","RS"),new t("Serbia, Montenegro","YU"),new t("Seychelles","SC"),new t("Sierra Leone","SL"),new t("Singapore","SG"),new t("Sint Eustatius","XE"),new t("Sint Maarten","SX"),new t("Slovakia","SK"),new t("Slovenia","SI"),new t("Solomon Islands","SB"),new t("Somalia","SO"),new t("South Africa","ZA"),new t("South Georgia and the South Sandwich Islands","GS"),new t("South Sudan","SS"),new t("Spain","ES"),new t("Sri Lanka","LK"),new t("St Helena, Ascension, and Tristan da Cunha","SH"),new t("Sudan","SD"),new t("Suriname","SR"),new t("Svalbard","SJ"),new t("Swaziland","SZ"),new t("Sweden","SE"),new t("Switzerland","CH"),new t("Syria","SY"),new t("Taiwan","TW"),new t("Tajikistan","TJ"),new t("Tanzania","TZ"),new t("Thailand","TH"),new t("Timor-Leste","TL"),new t("Togo","TG"),new t("Tokelau","TK"),new t("Tonga","TO"),new t("Trinidad and Tobago","TT"),new t("Tristan da Cunha","TA"),new t("Tunisia","TN"),new t("Turkey","TR"),new t("Turkmenistan","TM"),new t("Turks and Caicos Islands","TC"),new t("Tuvalu","TV"),new t("U.S. Outlying Islands","UM"),new t("U.S. Virgin Islands","VI"),new t("Uganda","UG"),new t("Ukraine","UA"),new t("United Arab Emirates","AE"),new t("United Kingdom","UK"),new t("United States","US"),new t("Uruguay","UY"),new t("Uzbekistan","UZ"),new t("Vanuatu","VU"),new t("Vatican City","VA"),new t("Venezuela","VE"),new t("Vietnam","VN"),new t("Wallis and Futuna","WF"),new t("Yemen","YE"),new t("Zambia","ZM"),new t("Zimbabwe","ZW")];n.countries={getCountries:function(){return i},getCountryNameByCode:function(n){var t=_.find(i,function(t){return t.code==n});return t===undefined||t==null?"":t.name}}}(window.app),function(n,t){"use strict";t.SortableColumnViewModel=function(n,t,i,r,u){var f=this;f.key=n;f.title=t;f.property=ko.observable(i);f.direction=ko.observable(r);f.isVisible=ko.observable(!0);f.hide=function(){f.isVisible(!1)};f.show=function(){f.isVisible(!0)};f.sort=function(){f.direction(f.direction()==="asc"?"desc":"asc");u&&typeof u=="function"&&u(f)}};ko.bindingHandlers.sortableColumn={init:function(i,r,u,f,e){var b=e.$data,s=ko.unwrap(r())||{},v=s.key,c=s.title,k=s.isToggleable,p=s.property,d=s.direction,l=s.callback,g=s.callbackContext,o=s.tableContext||b,nt=n(i),tt=nt.text().trim(),it=function(n){if(o&&o.sortableColumns){for(var t in o.sortableColumns)t!==n.property()&&o.sortableColumns[t].direction(null);l&&typeof l=="function"&&l.call(g||o,n)}},a=new t.SortableColumnViewModel(v,c||tt,p,d,it),h,y,w;return o.sortableColumns||(o.sortableColumns={}),o.sortableColumns[p]=a,c&&(l?n(i).append(n('<a href="#" class="sortlink"><\/a>').text(c)):n(i).append(n("<span><\/span>").text(c))),v&&k&&o.toggleableColumnsContainer&&(h=o.toggleableColumnsContainer,h.toggleableColumns||(h.toggleableColumns=ko.observable({})),h.toggleableColumns()[v]=a,h.toggleableColumns.valueHasMutated(),n(i).addClass("toggleable-column"),y=n('<a href="#" class="column-visibility-button">Hide<\/a>'),y.click(function(){return a.isVisible(!1),h.toggleableColumns.valueHasMutated(),h.saveState(),!1}),n(i).append(y)),c&&l&&(w=n("<i>").addClass("icon").attr("data-bind","css: {'icon-arrow-up': direction() === 'asc', 'icon-arrow-down': direction() === 'desc'}"),n(i).addClass("sortable").append(w).click(a.sort)),ko.applyBindingsToDescendants(a,i),{controlsDescendantBindings:!0}}}}(window.jQuery,window.app),function(n,t){"use strict";t.ToggleableColumnsContainer=function(n){var t=this;t.storageKey=n};t.ToggleableColumnsContainer.prototype={storageKey:null,toggleableColumns:ko.observable({}),defaultHiddenColumnKeys:null,setDefaultHiddenColumnKeys:function(n){var t=this;t.defaultHiddenColumnKeys=n},isColumnVisible:function(n){var t=this,i;return t.defaultHiddenColumnKeys&&t.defaultHiddenColumnKeys.indexOf(n)!==-1?!1:(i=t.toggleableColumns&&t.toggleableColumns(),!i||!i[n]||i[n].isVisible()===!0)},getHiddenColumnKeys:function(){var i=this,t=[];return n.each(i.toggleableColumns(),function(n,i){!i.isVisible()&&i.key&&t.push(i.key)}),t},hiddenColumns:function(){var i=this,t=[];return n.each(i.toggleableColumns(),function(n,i){i&&typeof i.isVisible=="function"&&!i.isVisible()&&t.push(i)}),t},numberOfHiddenColumns:function(){var n=this;return n.hiddenColumns().length},restoreHiddenColumns:function(){var t=this;n.each(t.toggleableColumns(),function(n,t){t&&typeof t.isVisible=="function"&&t.isVisible(!0)});t.saveState()},saveState:function(){var n=this;n.storageKey&&t.page.appendToState(n.storageKey,{hiddenColumnKeys:n.getHiddenColumnKeys()})},loadState:function(){var n=this,i,r,e,u,f;if(n.storageKey&&(i=t.page.loadState(n.storageKey),r=i&&i.hiddenColumnKeys,r&&r.length)){for(e=n.toggleableColumns(),u=0;u<r.length;u++)f=e[i.hiddenColumnKeys[u]],f&&f.isVisible(!1);n.toggleableColumns.valueHasMutated()}}}}(window.jQuery,window.app),function(n,t,i){"use strict";n.QuestionDependency=function(n){var t=this;t.questionById={};t.dependentQuestions=[];t.dependentChoicesByQuestionId={};t.questionsByDependentChoiceId={};t.appliedDependentChoicesByQuestionId={};t.hiddenQuestionIds={};var r=function(i){var u=t.questionsByDependentChoiceId[i],f,r,o,e;if(u&&u.length!==0)for(f=0;f<u.length;f++)(r=u[f],t.appliedDependentChoicesByQuestionId[r]||(t.appliedDependentChoicesByQuestionId[r]=[]),o=t.appliedDependentChoicesByQuestionId[r].indexOf(i),o>-1)||(t.appliedDependentChoicesByQuestionId[r].length===0&&(n.getQuestionDiv(r).fadeIn(1e3),e=t.questionById[r],e.required()&&(e.validationEnabled=!0),t.hiddenQuestionIds[r]&&delete t.hiddenQuestionIds[r]),t.appliedDependentChoicesByQuestionId[r].push(i))},u=function(i){var f=t.questionsByDependentChoiceId[i],e,r,o,u;if(f&&f.length!==0)for(e=0;e<f.length;e++)(r=f[e],t.appliedDependentChoicesByQuestionId[r]&&t.appliedDependentChoicesByQuestionId[r].length!==0)&&(o=t.appliedDependentChoicesByQuestionId[r].indexOf(i),o>-1&&(t.appliedDependentChoicesByQuestionId[r].splice(o,1),t.appliedDependentChoicesByQuestionId[r].length===0&&(n.getQuestionDiv(r).fadeOut(1e3),t.hiddenQuestionIds[r]=!0,u=t.questionById[r],u.selectedChoiceIds([]),t.dependentQuestions.indexOf(u)>-1&&(u.required()&&(u.validationEnabled=!1),u.answer(null)))))},f=function(n,t){t.status==="added"?r(t.value):t.status==="deleted"&&u(t.value)},e=function(n,t,i){u(i);r(t)};t.hasDependency=function(){return t.dependentQuestions.length>0};t.isHidden=function(n){return t.hiddenQuestionIds[n]};t.loadQuestions=function(n){for(var u,i,f,r=0;r<n.length;r++)if(i=n[r],t.questionById[i.id]=i,i.conditionQuestionChoiceIds.length>0)for(t.dependentChoicesByQuestionId[i.id]=i.conditionQuestionChoiceIds,u=0;u<i.conditionQuestionChoiceIds.length;u++)f=i.conditionQuestionChoiceIds[u],t.questionsByDependentChoiceId[f]||(t.questionsByDependentChoiceId[f]=[]),t.questionsByDependentChoiceId[f].push(i.id);for(r=0;r<n.length;r++)for(i=n[r],u=0;u<i.choices.length;u++)if(t.questionsByDependentChoiceId[i.choices[u].id]){t.dependentQuestions.push(i);break}};t.init=function(){var l,u,o,s,a,h,c,r;i.subscribeChoicesChanged(t.dependentQuestions,f);i.subscribeAnswerChanged(t.dependentQuestions,e);for(l in t.dependentChoicesByQuestionId)n.getQuestionDiv(l).hide(),t.hiddenQuestionIds[l]=!0;for(u=0;u<t.dependentQuestions.length;u++)if(o=t.dependentQuestions[u].selectedChoiceIds.peek(),o)for(s=0;s<o.length;s++)if(a=o[s],h=t.questionsByDependentChoiceId[a],h)for(c=0;c<h.length;c++)r=h[c],t.appliedDependentChoicesByQuestionId[r]||(t.appliedDependentChoicesByQuestionId[r]=[]),t.appliedDependentChoicesByQuestionId[r].length===0&&(n.getQuestionDiv(r).show(),delete t.hiddenQuestionIds[r]),t.appliedDependentChoicesByQuestionId[r].push(a)}}}(window.app,window.jQuery,new window.app.QuestionService),function(n,t,i){"use strict";t.Page=function(n,i){t.Page(n,i,null)};t.Page=function(t,i,r){var u=this;u.$element=n(t);u.conference=window.cmt3.conference!=undefined?window.cmt3.conference.name:null;u.page=ko.observable(1);u.top=ko.observable(25);u.sort=ko.observable("FirstName");u.controller=i;u.params=r;u.filters=[];u._total=ko.observable(0);u.selected=ko.observable(0);u.items=ko.observableArray();u.listen();u.Pager=ko.pager(u.selected,u.top);u.Pager().CurrentPage.subscribe(function(){u.page(u.Pager().CurrentPage());u.show()})};t.Page.prototype={listen:function(){var t=this;n(document).on("data.filter",function(){t.Pager().CurrentPage()<2?t.show():t.Pager().CurrentPage(1)})},getFilter:function(){var t="";return n.each(this.filters,function(n,i){i.getValue()&&(t+=t==""?i.getValue():" and "+i.getValue())}),t},setDefaultSort:function(n){var t=this;t.sort(n)},show:function(){var t=this,r="&$orderby="+this.sort(),u=this.top()!=0?"&$top="+this.top():"",f=this.skip()!=0?"&$skip="+this.skip():"",e=this.getFilter()!=""?"&$filter="+encodeURIComponent(this.getFilter()):"",o={headers:{Accept:"application/json"},requestUri:"/api/odata"+(this.conference!=null?"/"+this.conference+"/":"/")+"$batch",method:"POST",data:{requests:[{url:"/api/odata"+(this.conference!=null?"/"+this.conference+"/":"/")+t.controller+"?"+(t.params==null||t.params==undefined||t.params==""?"":t.params+"&")+"$count=true"+r+e+f+u,method:"GET",headers:{Accept:"application/json"}}]}};return i.request(o,function(i){var r=i.responses[0].body,u=r["@odata.count"],e=r.value,f=[];n.each(e,function(n,i){f.push(t.createItem(i))});t.items(f);t._total()==0&&t._total(u);t.selected(u)},function(n){window.cmt3.logger.log(n.message)},i.batchHandler)},createItem:function(){alert("not implemented")},scroll:function(){n(window).scrollTop()==n(document).height()-n(window).height()&&self.show()},post:function(n,t,i){var r,f,u;i=i||"post";r=document.createElement("form");r.setAttribute("method",i);r.setAttribute("action",n);for(f in t)t.hasOwnProperty(f)&&(u=document.createElement("input"),u.setAttribute("type","hidden"),u.setAttribute("name",f),u.setAttribute("value",t[f]),r.appendChild(u));document.body.appendChild(r);r.submit();document.body.removeChild(r)},stub:function(){alert("Sorry, this feature is not implemented yet.")},reset:function(){n.each(this.filters,function(n,t){t.reset()});this.show()},size:function(t,i){var r,u,f;n("a",".show").removeClass("btn-success").css("color","#999999");n(i.currentTarget).addClass("btn-success").css("color","white");r=n(i.target).attr("size");u=parseInt(r);this.top(u);f=this.Pager().CurrentPage();this.Pager().CurrentPage(1);f===1&&this.show()},skip:function(){return(this.page()-1)*this.top()},prev:function(){this.top()!=0&&this.page()!=1&&(this.page(this.page()-1),this.show())},next:function(){this.top()==0||this.page()>this.selected()/this.top()||(this.page(this.page()+1),this.show())},setSort:function(t,i){var r=n(i.target),u=r.attr("data-sort");(u==null||u==undefined)&&(r=n(r.context.parentNode),u=r.attr("data-sort"));r.hasClass("selected")?this.sort().match(" desc$")?(this.sort(u+" asc"),r.find("i").removeClass("icon-arrow-down"),r.find("i").addClass("icon-arrow-up")):(this.sort(u+" desc"),r.find("i").removeClass("icon-arrow-up"),r.find("i").addClass("icon-arrow-down")):(n("th[data-sort]").each(function(){n(this).find("i").removeClass("icon-arrow-up");n(this).find("i").removeClass("icon-arrow-down");n(this).removeClass("selected")}),r.find("i").removeClass("icon-arrow-down"),r.find("i").addClass("icon-arrow-up"),r.addClass("selected"),this.sort(u+" asc"));this.show()}}}(window.jQuery,window.app,window.OData),function(n,t,i){n.EmailProgressViewModel=function(r,u){function e(i){var r={},o;r[u?"SessionIds":"SessionId"]=i;o={requestUri:n.odata.getUrl(n.odata.entitySet.emails,null,u?"GetBulkProgress":"GetProgress"),method:"POST",showProgressIndicator:!1,data:r};t.request(o,function(t){f.totalCount(t.TotalCount);f.successCount(t.SuccessCount);f.errorCount(t.ErrorCount);f.totalCount()>0&&f.successCount()+f.errorCount()==f.totalCount()?setTimeout(function(){f.done(!0)},n.settings.queryProgressDelay):setTimeout(function(){e(i)},n.settings.queryProgressDelay)},function(){setTimeout(function(){e(i)},n.settings.queryProgressDelay)})}var f=this;f.totalCount=ko.observable(0);f.successCount=ko.observable(0);f.errorCount=ko.observable(0);f.progress=ko.computed(function(){return f.totalCount()==0?0:((f.successCount()+f.errorCount())/f.totalCount()*100).toFixed(0)+"%"});f.done=ko.observable(!1);f.showInDialog=function(n){f.totalCount(0);f.successCount(0);f.errorCount(0);f.done(!1);i(r).modal("show");e(n)};f.bind=function(){ko.applyBindings(f,r)}}}(window.app,window.OData,window.$),function(n,t){"use strict";t.DataTable=function(){var i=this;i.savedState=i.loadState();i.total=ko.observable(0);i.page=ko.observable(i.savedState.page);i.top=ko.observable(i.savedState.top);i.skip=ko.computed(function(){return(i.page()-1)*i.top()});i.pager=ko.pager(i.total,i.top);i.pager().CurrentPage(i.page());i.pager().CurrentPage.subscribe(function(){i.page(i.pager().CurrentPage());i.loadData()});i.filters=[];i.sortableColumns={};i.toggleableColumnsContainer=new t.ToggleableColumnsContainer(i.getStorageKey());i.sorting=ko.observable(i.savedState.sorting);n(document).on("data.filter",function(){i.pager().CurrentPage()<2?i.loadData():i.pager().CurrentPage(1)})};t.DataTable.prototype={getStorageKey:function(){return null},getDefaultSorting:function(){return null},getDefaultState:function(){var n=this;return{page:1,top:25,sorting:n.getDefaultSorting(),filters:[]}},loadState:function(){var n=this,t;return!sessionStorage||!(t=n.getStorageKey())?n.getDefaultState():JSON.parse(sessionStorage.getItem(t))||n.getDefaultState()},applyState:function(){var t=this,i;if(n.each(t.sortableColumns,function(n,i){i.property()!==t.savedState.sorting.property?i.direction(null):i.direction(t.savedState.sorting.direction)}),t.savedState&&t.savedState.sorting&&t.savedState.sorting.property&&t.sortableColumns&&t.sortableColumns[t.savedState.sorting.property])for(i in t.sortableColumns)t.sortableColumns[i].direction(i!==t.savedState.sorting.property?null:t.savedState.sorting.direction);n.each(t.savedState.filters,function(i,r){n.each(t.filters,function(n,t){t.field===r.property&&t.setValue(r.value)})})},saveState:function(){var t=this,i,r,u,f;sessionStorage&&(i=t.getStorageKey())&&(r=[],n.each(t.filters,function(n,t){var i=t.getValue();i&&r.push({property:t.field,value:i})}),u={page:t.page(),top:t.top(),sorting:t.sorting(),filters:r},f=t.loadState(i),sessionStorage.setItem(i,JSON.stringify(n.extend({},f,u))))},size:function(n){this.top(n);this.loadData()},sort:function(n){this.sorting({property:n.property(),direction:n.direction()});this.loadData()},resetFilters:function(){n.each(this.filters,function(n,t){t.reset()});this.pager().CurrentPage()<2?this.loadData():this.pager().CurrentPage(1)},refresh:function(){this.loadData()},loadData:function(){}}}(window.jQuery,window.app),function(n,t,i){"use strict";function e(n){var i=this,u,f;i.userRoles=[];i.userTags=[];u=function(n){var f={},t,u,e;if(n){for(t=0;t<n.length;t++)u=f[n[t].Role],u||(u=[]),n[t].ObjectId!==null&&n[t].ObjectType==="Track"&&u.push(n[t].ObjectId),f[n[t].Role]=u;for(e in r)f[e]&&i.userRoles.push(new o(r[e],f[e]))}};f=function(){var n,r;if(i.userTags=[],n=i.userTagJson&&JSON.parse(i.userTagJson),n)for(r=0;r<n.length;r++)i.userTags.push(t.autoMap(new t.UserTag,n[r]))};n?(i.id=n.Id,i.firstName=n.FirstName,i.middleInitial=n.MiddleInitial,i.lastName=n.LastName,i.email=n.Email,i.organization=n.Organization,i.country=n.Country,i.lastLoginDate=n.LastLoginDate,i.isFederation=n.IsFederation,i.googleScholarId=n.GoogleScholarId,i.semanticScholarId=n.SemanticScholarId,i.dblpId=n.DblpId,i.externalProfileEntered=n.ExternalProfileEntered,i.conflictDomainsEntered=n.ConflictDomainsEntered,i.individualConflictsEntered=n.IndividualConflictsEntered,i.userInformationEntered=n.UserInformationEntered,i.userTagJson=n.UserTagJson,u(n.Permissions),f()):(i.id=t.autoMap(),i.firstName=t.autoMap(),i.middleInitial=t.autoMap(),i.lastName=t.autoMap(),i.email=t.autoMap(),i.organization=t.autoMap(),i.country=t.autoMap(),i.lastLoginDate=t.autoMap(),i.isFederation=t.autoMap(),i.googleScholarId=t.autoMap(),i.semanticScholarId=t.autoMap(),i.dblpId=t.autoMap(),i.externalProfileEntered=t.autoMap(),i.conflictDomainsEntered=t.autoMap(),i.individualConflictsEntered=t.autoMap(),i.userInformationEntered=t.autoMap(),i.userTagJson=t.autoMap());i.googleScholarUrl=function(){return t.enums.externalProfile.googleScholar.format(i.googleScholarId)};i.semanticScholarUrl=function(){return t.enums.externalProfile.semanticScholar.format(i.semanticScholarId)};i.dblpUrl=function(){return t.enums.externalProfile.dblp.format(i.dblpId)};i.individualConflictsEnteredText=ko.pureComputed(function(){return i.individualConflictsEntered===!0?"Yes":"No"});i.userInformationEnteredText=ko.pureComputed(function(){return i.userInformationEntered===!0?"Yes":"No"});i.readFromJson=function(n){return t.autoMap(i,n),n&&n.Permissions&&n.Permissions&&u(n.Permissions),f(),i};i.lastLoginDateFormatted=function(){return t.formatUndefinableDateTime(i.lastLoginDate)};i.isReviewer=function(){var n=!1;return i.userRoles.forEach(function(i){n=n||i.role.name===t.enums.userRole.reviewer}),n};i.isMetaReviewer=function(){var n=!1;return i.userRoles.forEach(function(i){n=n||i.role.name===t.enums.userRole.metaReviewer}),n}}function o(n,t){var i=this,r;for(i.role=n,i.tracks=[],r=0;r<t.length;r++)i.tracks.push(f[t[r]]);i.tracks.sort(h);i.showTrackCount=function(){return i.tracks.length>0&&i.role.showTracks&&u===null}}function c(){this.name=t.autoMap();this.allowEdit=t.autoMap();this.showTracks=!1}function s(n,t){var i=this,r,o,e;i.role=n.role;i.tracks=ko.observableArray();i.originalTrackIds=[];i.availableTracks=ko.observableArray();for(r in f){for(o=!0,e=0;e<n.tracks.length;e++)if(n.tracks[e]&&r===n.tracks[e].id.toString()){o=!1;break}o?i.availableTracks.push(f[r]):(i.tracks.push(f[r]),i.originalTrackIds.push(r))}i.addTrack=function(n){i.tracks.push(n);i.availableTracks.remove(n)};i.removeTrack=function(n){i.tracks.remove(n);i.tracks().length===0&&t(i);i.availableTracks.push(n);i.availableTracks.sort(h)};i.showTracks=function(){return i.role.showTracks&&(u===null||u!==null&&i.tracks().length>0)}}function l(r){var u=this,f;u.id=ko.observable().autoMap();u.email=ko.observable().extend({required:!0,email:!0}).autoMap();u.firstName=ko.observable().autoMap();u.middleInitial=ko.observable().autoMap();u.lastName=ko.observable().autoMap();u.organization=ko.observable().autoMap();u.isSearching=ko.observable();u.searchedEmail=ko.observable();f=null;u.userFound=ko.computed(function(){return u.id()>0});u.userNotFound=ko.computed(function(){return u.id()===0});u.search=function(){var n=ko.validation.group([u.email]),r;if(n().length>0){n.showAllMessages();return}u.isSearching(!0);u.searchedEmail(u.email());r={requestUri:t.odata.getGlobalUrl(t.odata.entitySet.users,null,"SearchByEmail"),method:"POST",showProgressIndicator:!1,data:{Email:u.searchedEmail()}};i.read(r,function(n){t.autoMap(u,n);u.isSearching(!1)},function(n){u.isSearching(!1);n.response.statusCode===404?u.id(0):i.defaultError(n)})};u.addUser=function(){var o,s;n(r).modal("hide");o=new e;u.userFound()?(s={requestUri:t.odata.getUrl(t.odata.entitySet.users,null,"GetUserByEmail"),method:"POST",showProgressIndicator:!1,data:{Email:u.searchedEmail()}},i.read(s,function(n){o.readFromJson(n);f.resolve(o)},function(n){n.response.statusCode===404?f.resolve(t.autoMap(o,u)):i.defaultError(n)})):(o=t.autoMap(o,{}),o.email=u.searchedEmail(),f.resolve(o))};u.bind=function(){ko.applyBindings(u,r)};u.editInDialog=function(){return u.id(null),u.email(""),u.email.isModified(!1),u.firstName(""),u.lastName(""),u.organization(""),u.searchedEmail(""),n(r).modal("show"),f=n.Deferred(),f.promise()}}function a(e){function l(n,t){return{Role:n,ObjectId:t,ObjectType:"Track"}}function a(n,t){function s(n,t){for(var u,r,f=[],i=0;i<n.length;i++){for(u=!0,r=0;r<t.length;r++)if(n[i]===t[r].id.toString()){u=!1;break}u&&f.push(n[i])}return f}for(var e,i,o,u,f=[],r=0;r<n.length;r++){for(e=!0,i=0;i<t.length;i++)if(n[r]===t[i].role.name){for(o=s(t[i].originalTrackIds,t[i].tracks()),u=0;u<o.length;u++)f.push(l(n[r],o[u]));e=!1;break}e&&f.push(l(n[r],null))}return f}function v(n,t){function c(n,t){for(var u,r,f=[],i=0;i<t.length;i++){for(u=!0,r=0;r<n.length;r++)if(n[r]===t[i].id){u=!1;break}u&&f.push(t[i].id)}return f}for(var s,r,h,f,e,o,u=[],i=0;i<t.length;i++){for(s=!0,r=0;r<n.length;r++)if(n[r]===t[i].role.name){for(h=c(t[i].originalTrackIds,t[i].tracks()),f=0;f<h.length;f++)u.push(l(n[r],h[f]));s=!1;break}if(s)if(e=c([],t[i].tracks()),e.length===0)u.push(l(t[i].role.name,null));else for(o=0;o<e.length;o++)u.push(l(t[i].role.name,e[o]))}return u}var h=this,c;h.id=null;h.email=ko.observable().extend({required:!0,email:!0,maxLength:200}).autoMap();h.firstName=ko.observable().extend({required:!0,maxLength:200}).autoMap();h.middleInitial=ko.observable().extend({maxLength:10}).autoMap();h.lastName=ko.observable().extend({required:!0,maxLength:200}).autoMap();h.organization=ko.observable().extend({required:!0,maxLength:200}).autoMap();h.createNew=ko.observable();c=null;h.showTracks=function(){return u===null};h.userRoles=ko.observableArray();h.originalRoleNames=[];h.availableRoles=ko.observableArray();h.addRole=function(n){var t=new s(new o(n,[]),h.removeRole);u!==null&&n.showTracks&&t.addTrack(f[u.id]);h.userRoles.push(t);h.availableRoles.remove(n)};h.removeRole=function(n){h.userRoles.remove(n);h.availableRoles.push(n.role);h.availableRoles.sort(function(n,t){return n.name===t.name?0:n.name<t.name?-1:1})};h.editInDialog=function(i){var f,o,u;h.id=i.id;t.autoMap(h,i);h.createNew(!i.id);h.userRoles.removeAll();h.availableRoles.removeAll();h.originalRoleNames=[];for(f in r){for(o=!0,u=0;u<i.userRoles.length;u++)if(f===i.userRoles[u].role.name){o=!1;h.userRoles.push(new s(i.userRoles[u],h.removeRole));h.originalRoleNames.push(i.userRoles[u].role.name);break}o&&r[f].allowEdit&&h.availableRoles.push(r[f])}return n(e).modal("show"),c=n.Deferred(),c.promise()};h.save=function(){var r=!0,f,u,o,s,l,y;for(h.createNew()&&(f=ko.validation.group(h),f().length>0&&(f.showAllMessages(),r=!1),h.userRoles().length===0&&(r=!1)),u=0;u<h.userRoles().length;u++)if(o=h.userRoles()[u],o.showTracks()&&o.tracks().length===0){r=!1;break}r&&(h.createNew()?(l=t.autoMap(h),y={requestUri:t.odata.getUrl(t.odata.entitySet.users),method:"POST",headers:{Prefer:"return-content"},data:l},s=i.request(y,function(n){h.id=n.Id})):s=n.Deferred().resolve().promise(),s.done(function(){var u=a(h.originalRoleNames,h.userRoles()),f=v(h.originalRoleNames,h.userRoles()),r,o;u.length>0||f.length>0?(o={requestUri:t.odata.getUrl(t.odata.entitySet.users,h.id,"ModifyPermissions"),method:"POST",data:{Request:{Add:f,Remove:u}}},r=i.request(o,function(){})):r=n.Deferred().resolve().promise();r.done(function(){n(e).modal("hide");t.addMessage("User '{0} {1}' saved!".format(h.firstName(),h.lastName()));c&&c.resolve()})}))};h.bind=function(){ko.applyBindings(h,e)}}function v(r){var u=this,f=null;u.password=ko.observable("").extend({required:!0,minLength:10}).autoMap();u.confirmPassword=ko.observable("").extend({required:!0,minLength:10,equal:{params:u.password,message:"Passwords must match."}});u.resetPassword=function(){var e,o;if(f){if(e=ko.validation.group(u),e().length>0){e.showAllMessages();return}o={requestUri:t.odata.getUrl("Users",f.id,"ResetPassword"),method:"POST",data:{Password:u.password()}};i.request(o,function(){n(r).modal("hide");t.addMessage("Password for user {0} {1} was reset.".format(f.firstName,f.lastName))})}};u.bind=function(){ko.applyBindings(u,r)};u.editInDialog=function(t){u.password("");u.password.isModified(!1);u.confirmPassword("");u.confirmPassword.isModified(!1);f=t;n(r).modal("show")}}function h(n,t){return n.name===t.name?0:n.name<t.name?-1:1}var f,r,u;t.UserPage=function(o,s,h,y,p,w,b,k){function it(n){g===null&&(g=new a(document.getElementById("editDialog")),g.bind());g.editInDialog(n).done(rt)}function rt(){d.show()}t.Page.call(this,o,s);var d=this,g=null,nt=null,tt=null;f=h||{};r=y||{};u=p||null;d.requireConflictDomains=w;d.requireIndividualConflict=b;d.requireUserInformation=k;d.isGlobal=ko.observable(window.cmt3.conference===undefined);d.users=ko.observableArray();d.createItem=function(n){return new e(n)};d.edit=function(n){it(n)};d.addUser=function(){nt===null&&(nt=new l(document.getElementById("userSearchDialog")),nt.bind());nt.editInDialog().done(function(n){it(n)})};d.email=function(n,i){var r=t.GetEventFilter(i),u="/"+window.cmt3.conference.name+"/User/SendEmail";t.url.navigateTo(u,{filter:r.length>0?r:null})};d.importDomainConflicts=function(){var n="/"+window.cmt3.conference.name+"/User/ImportDomainConflicts";t.url.navigateTo(n)};d.importUserTags=function(){var n="/"+window.cmt3.conference.name+"/User/ImportUserTags";t.url.navigateTo(n,{roleValue:1})};d.exportUserInformation=function(n,i){var r=t.GetEventFilter(i),u="/api/odata/"+window.cmt3.conference.name+"/Users/ExportUserInformation",f={Filter:r};t.page.post(u,f)};d.exportTabDelimited=function(n,i){var r=t.GetEventFilter(i),u="/api/odata/"+window.cmt3.conference.name+"/Users/ExportTabDelimited",f={Filter:r};t.page.post(u,f)};d.impersonate=function(r){if(confirm("Are you sure to impersonate as {0} {1}?".format(r.firstName,r.lastName))){var u={requestUri:t.odata.getUrl("Users",r.id,"Impersonate"),method:"POST"};i.request(u,function(n){t.odata.processRedirectResponse(n)},function(i){var r=n.parseJSON(i.response.body).error.message;t.addMessage(r,null,"error")})}};d.resetPassword=function(n){tt===null&&(tt=new v(document.getElementById("resetPasswordDialog")),tt.bind());tt.editInDialog(n)};d.show=function(){d.isGlobal()?t.Page.prototype.show.call(d):t.Page.prototype.show.call(d)}};t.UserPage.prototype=Object.create(t.Page.prototype)}(window.jQuery,window.app,window.OData),function(n,t,i){"use strict";function f(){var n=this;n.name=t.autoMap();n.city=t.autoMap();n.country=t.autoMap();n.urlSegmentName=t.autoMap();n.startDate=t.autoMap();n.externalUrl=t.autoMap();n.emailChairsUrl=ko.pureComputed(function(){return"/"+this.urlSegmentName+"/Email/Chairs"},n);n.startDateString=function(){return n.startDate.getMonth()+1+"/"+n.startDate.getDate()+"/"+n.startDate.getFullYear()};n.url=function(){return i.protocol+"//"+i.host+u.conferenceRoot.format(n.urlSegmentName)}}function r(n,i){return new t.ServerList({entitySet:{isGlobal:!0,entitySet:n},filter:i,localFilter:function(n,t){return t=t.toLowerCase(),n.name.toLowerCase().indexOf(t)>-1||n.city.toLowerCase().indexOf(t)>-1||n.country.toLowerCase().indexOf(t)>-1||n.urlSegmentName.toLowerCase().indexOf(t)>-1?n:null},itemConstructor:function(n){return t.autoMap(new f,n)},odataFilter:function(n){return"contains(tolower(Name),tolower('{0}')) or contains(tolower(City),tolower('{0}')) or contains(tolower(Country),tolower('{0}')) or contains(tolower(UrlSegmentName),tolower('{0}'))".format(t.odata.escapeParam(n))},odataOrderByFields:"EndDate desc"})}function e(i){function f(n){return u.conferenceList.getItems(u.conferences,n).done(function(){u.showMore.updateCount(u.conferenceList.getTotalCount(),u.conferences().length)})}var u=this;u.showAllConferences=i;u.conferences=ko.observableArray();u.filterString=ko.observable("").extend({throttle:500});u.filterString.subscribe(function(){f(1)});u.showMore=new t.ShowMore(function(n){return u.conferenceList.addItems(u.conferences,n).done(function(){u.showMore.updateCount(u.conferenceList.getTotalCount(),u.conferences().length)})});u.init=function(){var i=n.Deferred();return u.filterFunction=function(){return u.filterString()},u.initModel=function(){u.myConferencesTitle="My Conferences ({0})".format(u.myConferencesCount);u.allConferencesTitle="All Conferences";u.myConferences=ko.observable(!0);u.allConferences=ko.observable(!1);u.conferenceList=r(t.odata.entitySet.myConferences,u.filterFunction);u.myConferencesClick=function(){u.conferenceList=r(t.odata.entitySet.myConferences,u.filterFunction);u.myConferences(!0);u.allConferences(!1);f(1)};u.allConferencesClick=function(){u.conferenceList=r(t.odata.entitySet.conferences,u.filterFunction);u.myConferences(!1);u.allConferences(!0);f(1)};u.bindTo=function(n){ko.applyBindingsAndShow(u,n)};i.resolve()},u.conferenceList=r(t.odata.entitySet.myConferences,u.filterFunction),f(1).done(function(){u.myConferencesCount=u.conferenceList.getTotalCount();u.initModel()}),i.promise()}}var u;t.conferenceRecent=function(n,t,i){u=n;var r=new e(t);r.init().done(function(){r.bindTo(i)})}}(window.jQuery,window.app,window.location),function(n,t,i,r,u,f,e){"use strict";function o(n,t){this.value=n;this.caption=t===null||t===undefined?n:t}function l(i,r,u){function o(){return e.loadQuestionsDirect(r,u).done(function(n){f.questions(n);for(var r,t,u,i=0;i<n.length;i++)if(t=n[i],f.questionById[t.id]=t,t.conditionQuestionChoiceIds.length>0)for(f.dependentChoicesByQuestionId[t.id]=t.conditionQuestionChoiceIds,r=0;r<t.conditionQuestionChoiceIds.length;r++)u=t.conditionQuestionChoiceIds[r],f.questionsByDependentChoiceId[u]||(f.questionsByDependentChoiceId[u]=[]),f.questionsByDependentChoiceId[u].push(t.id);for(i=0;i<n.length;i++)for(t=n[i],r=0;r<t.choices.length;r++)if(f.questionsByDependentChoiceId[t.choices[r].id]){f.dependentQuestions.push(t);break}})}var f=this;f.questions=ko.observableArray();f.questionById={};f.dependentQuestions=[];f.dependentChoicesByQuestionId={};f.questionsByDependentChoiceId={};f.appliedDependentChoicesByQuestionId={};f.hiddenQuestionIds={};f.show=function(){f.questions([]);t.showProgress();o().done(function(){n(i).modal("show")}).always(t.hideProgress)};f.hide=function(){n(i).modal("hide");f.questions([])}}function s(){var n=this;n.id=t.autoMap();n.title=t.autoMap();n.required=t.autoMap();n.isLocked=t.autoMap();n.visibleToAuthor=t.autoMap();n.visibleToAuthorDuringFeedback=t.autoMap();n.visibleToAuthorAfterNotification=t.autoMap();n.visibleToReviewer=t.autoMap();n.visibleToMetaReviewer=t.autoMap();n.visibleToOtherReviewer=t.autoMap();n.visibleToSeniorMetaReviewer=t.autoMap();n.order=ko.observable().autoMap();n.questionType=t.autoMap();n.questionTypeName=t.autoMap();n.optionsType=t.autoMap();n.optionsTypeName=t.autoMap();n.details=t.autoMap();n.additionalInfo=t.autoMap();n.choices=[];n.commentLength=t.autoMap()}function a(){var n=this;n.id=t.autoMap();n.name=t.autoMap()}function v(){var n=this;n.id=t.autoMap();n.name=t.autoMap()}function h(){var n=this;n.id=t.autoMap();n.text=t.autoMap();n.value=t.autoMap()}function c(n,i){var r=this;r.id=n.id;r.text=ko.observable(n.text).extend({required:!0}).autoMap();r.value=ko.observable(n.value==null?"":n.value.toString()).extend({required:{onlyIf:function(){return i.questionType()==t.enums.questionType.optionsWithValue}},pattern:{params:/^-?\d{1,5}$/,message:"Value must be an interger."}}).autoMap()}function y(r,u,f){var e=this;e.tracks=ko.observableArray();e.selectedTracks=ko.observableArray();e.editInDialog=function(){i.read(t.odata.getUrl(t.odata.entitySet.tracks,{orderby:"Order"}),function(i){for(var s,o=[],f=0;f<i.value.length;f++)i.value[f].Id!=u&&(s=t.autoMap(new t.Track,i.value[f]),o.push(s));e.tracks(o);e.selectedTracks([]);n(r).modal("show")})};e.save=function(){var o,s;e.selectedTracks().length!=0&&(o=t.autoMap(e),o.TrackId=u,o.ToTrackIds=e.selectedTracks(),o.FormType=f,s={requestUri:t.odata.getUrl(t.odata.entitySet.questions,null,"CopyQuestionsFromTrack"),method:"POST",data:{Request:o}},i.request(s,function(){n(r).modal("hide");t.addMessage("Questions copied!")}))};e.bind=function(){ko.applyBindings(e,r)}}function p(r,u,f){function l(){return i.read(t.odata.getUrl(t.odata.entitySet.questionTypes),function(i){e.questionTypes=n.map(i.value,function(n){return t.autoMap(new a,n)})})}function y(){return i.read(t.odata.getUrl(t.odata.entitySet.optionsTypes),function(i){e.optionsTypes=n.map(i.value,function(n){return t.autoMap(new v,n)})})}var e=this,s;e.id=null;e.form=u;e.formType=f;e.title=ko.observable().extend({required:{onlyIf:function(){return e.form.formType===t.enums.formType.submission||e.form.formType===t.enums.formType.cameraready}}}).autoMap();e.questionType=ko.observable().autoMap();e.optionsType=ko.observable().autoMap();e.required=ko.validatedObservable().autoMap();e.isLocked=ko.validatedObservable().autoMap();e.visibleToAuthor=ko.observable().autoMap();e.visibleToAuthorDuringFeedback=ko.observable().autoMap();e.visibleToAuthorAfterNotification=ko.observable().autoMap();e.visibleToReviewer=ko.observable().autoMap();e.visibleToMetaReviewer=ko.observable().autoMap();e.visibleToOtherReviewer=ko.observable().autoMap();e.visibleToSeniorMetaReviewer=ko.observable().autoMap();e.order=ko.observable().autoMap();e.details=ko.observable().extend({required:!0}).autoMap();e.additionalInfo=ko.observable("").autoMap();e.commentLength=ko.observable().autoMap();e.commentLengthOptions=[new o(125),new o(500),new o(1e3),new o(2e3),new o(3e3),new o(4e3),new o(5e3),new o(6e3),new o(7e3),new o(8e3),new o(null,"Unlimited")];e.questionTypes=[];e.optionsTypes=[];e.createNew=ko.observable();s=null;e.choices=ko.observableArray();e.addChoice=function(){var n=new c(t.autoMap(new h,{}),e),i=new Number(e.choices().length>0?e.choices()[e.choices().length-1].value():null);n.value(isNaN(i)?null:(i+1).toString());n.value.isModified(!1);e.choices.push(n);e.showChoicesValidationMessage(!1)};e.removeChoice=function(n){e.choices.remove(n)};e.showChoicesValidationMessage=ko.observable(!1);e.editInDialog=function(i){e.id=i.id;t.autoMap(e,i);e.showChoicesValidationMessage(!1);e.createNew(!i.id);e.createNew()&&(e.questionTypes.length>0&&e.questionType(e.questionTypes[0].id),e.optionsTypes.length>0&&e.optionsType(e.optionsTypes[0].id));e.choices.removeAll();for(var u=0;u<i.choices.length;u++)e.choices.push(new c(i.choices[u],e));return n(r).modal("show"),s=n.Deferred(),s.promise()};e.save=function(){var c=!0,l=ko.validation.group(e,{deep:!0}),f,o,h,a;if(l().length>0&&(l.showAllMessages(),c=!1),(e.questionType()===t.enums.questionType.options||e.questionType()===t.enums.questionType.optionsWithValue||e.questionType()===t.enums.questionType.optionsWithOther||e.questionType()===t.enums.questionType.optionsWithUserInput)&&e.choices().length<2&&(e.showChoicesValidationMessage(!0),c=!1),c){if(f=t.autoMap(e),e.questionType()===t.enums.questionType.optionsWithOther&&(f.OptionsType=t.enums.optionsType.radioButtonList),e.createNew()?f.FormId=u.id:f.Id=e.id,f.Choices=[],e.questionType()===t.enums.questionType.options||e.questionType()===t.enums.questionType.optionsWithValue||e.questionType()===t.enums.questionType.optionsWithOther||e.questionType()===t.enums.questionType.optionsWithUserInput)for(o=0;o<e.choices().length;o++)h=t.autoMap(e.choices()[o]),e.questionType()===t.enums.questionType.options&&(h.Value=null),h.Order=o+1,h.Id=e.choices()[o].id,f.Choices.push(h);a={requestUri:t.odata.getUrl(t.odata.entitySet.questions,e.createNew()?null:e.id),method:e.createNew()?"POST":"PUT",data:f};i.request(a,function(){n(r).modal("hide");t.addMessage("Question '{0}' saved!".format(e.title()||e.details()));s&&s.resolve()},function(n){n.response.statusCode===409?t.addMessage("Choice(s) that you are trying to delete is being used by papers, please contact CMT.",null,"error"):i.defaultError(n)})}};e.bind=function(){return n.when(l(),y()).done(function(){e.formType===t.enums.formType.chairnote||e.formType===t.enums.formType.reviewernote||e.formType===t.enums.formType.metareviewernote||e.formType===t.enums.formType.seniormetareviewernote?e.questionTypes=e.questionTypes.filter(function(n){return n.id===t.enums.questionType.comment||n.id===t.enums.questionType.options}):e.formType===t.enums.formType.reproducibility?(e.questionTypes=e.questionTypes.filter(function(n){return n.id===t.enums.questionType.optionsWithUserInput}),e.optionsTypes=e.optionsTypes.filter(function(n){return n.id===t.enums.optionsType.checkboxList})):e.formType===t.enums.formType.userinformation?(e.questionTypes=e.questionTypes.filter(function(n){return n.id===t.enums.questionType.agreement||n.id===t.enums.questionType.comment||n.id===t.enums.questionType.options||n.id===t.enums.questionType.optionsWithOther}),e.optionsTypes=e.optionsTypes.filter(function(n){return n.id!==t.enums.optionsType.dropDown&&n.id!==t.enums.optionsType.listBox})):e.questionTypes=e.questionTypes.filter(function(n){return n.id!==t.enums.questionType.optionsWithUserInput&&n.id!==t.enums.questionType.optionsWithOther});ko.applyBindings(e,r)})}}function w(e,o,c){function tt(){v=new t.ServerList({entitySet:t.odata.entitySet.questions,filter:function(){return a.filterString()},localFilter:function(n,t){return t=t.toLowerCase(),n.title.toLowerCase().indexOf(t)>-1||n.details.toLowerCase().indexOf(t)>-1?n:null},itemConstructor:function(n){for(var r=t.autoMap(new s,n),u=n.Choices,i=0;i<u.length;i++)r.choices.push(t.autoMap(new h,u[i]));return r},odataFilter:function(n){return"FormId eq {1} and (contains(tolower(Title),'{0}') or contains(tolower(Details),'{0}'))".format(n,b.id)},odataOrderByFields:"Order"})}function g(n){w?w.editInDialog(n).done(nt):(w=new p(r.getElementById("editDialog"),b,e),w.bind().done(w.editInDialog(n).done(nt)))}function d(n){return v.getItems(a.questions,n).done(function(){a.showMore.updateCount(v.getTotalCount(),a.questions().length)})}function nt(){v.clear();d(a.questions().length<t.settings.pageSize?1:a.questions().length/t.settings.pageSize)}var a=this,w=null,b=null,k=null,v=null;a.showMore=new t.ShowMore(function(n){return v.addItems(a.questions,n).done(function(){a.showMore.updateCount(v.getTotalCount(),a.questions().length)})});a.questions=ko.observableArray();a.filterString=ko.observable("").extend({throttle:500});a.formType=e;a.preview=ko.observable();a.showPreview=function(){var n=a.preview();n&&n.show()};a.delete=function(n){if(u("Are you sure you want to delete the question?")){var r={requestUri:t.odata.getUrl(t.odata.entitySet.questions,n.id),method:"DELETE"};i.request(r,function(){a.questions.remove(n);a.showMore.removeOne()},function(n){n.response.statusCode===409?t.addMessage("Question that you are trying to delete is being used by papers, please contact CMT.",null,"error"):i.defaultError(n)})}};a.edit=function(n){g(n)};a.addQuestion=function(){var n=a.formType===t.enums.formType.review;g(t.autoMap(new s,{visibleToOtherReviewer:n,CommentLength:8e3,required:a.formType!==t.enums.formType.reproducibility}))};a.copyQuestions=function(){k===null&&(k=new y(document.getElementById("copyDialog"),o,e),k.bind());k.editInDialog()};a.filterString.subscribe(function(){d(1)});a.swapQuestionsAndSave=function(n,r){var u={Id1:a.questions()[n].id,Id2:a.questions()[r].id},f={requestUri:t.odata.getUrl(t.odata.entitySet.questions,null,"SwapOrder"),method:"POST",data:{Request:u}};i.request(f,function(){var t=a.questions()[n];a.questions()[n]=a.questions()[r];a.questions()[r]=t;t=a.questions()[n].order();a.questions()[n].order(a.questions()[r].order());a.questions()[r].order(t);a.questions.valueHasMutated()},function(n){i.defaultError(n)})};a.moveQuestionUp=function(n){n<=0||a.swapQuestionsAndSave(n,n-1)};a.moveQuestionDown=function(n){n>=a.questions().length-1||a.swapQuestionsAndSave(n,n+1)};a.bindTo=function(t){f.loadForm(a.formType,o).done(function(i){i&&(b=i,a.preview(new l(r.getElementById("previewDialog"),a.formType,b.id)),tt(),d(1).done(function(){ko.applyBindingsAndShow(a,t);c?n("#menuNotes").addClass("in"):n("#menuForms").addClass("in")}))})}}t.formQuestion=function(n,t,i){new w(n,t,i).bindTo("questionListForm")}}(window.jQuery,window.app,window.OData,window.document,window.confirm,new window.app.FormService,new window.app.QuestionService),function(n,t,i,r,u,f,e,o){"use strict";function h(){var t=this;t.id=n.autoMap();t.originalName=n.autoMap();t.size=n.autoMap();t.formattedSize=n.autoMap();t.uploadDate=n.autoMap();t.downloadLink=n.autoMap()}function c(n,t,i,r,u){var f=this;f.id=n;f.title=t;f.trackId=i;f.trackName=r;f.isSingleTrackConference=u}function l(l,a,v,y,p,w,b,k){function nt(){function c(){var u=r.stringify(e.getAnswersJson(d.questions)),i,f;if(d.lastDraft===u){d.setAutoSaveTimer();return}i=n.autoMap(d);i.SubmissionId=d.submission.id;i.Id=d.draftId||0;i.Draft=u;f={requestUri:n.odata.getUrl(n.odata.entitySet.reviewDrafts),method:"POST",headers:{Prefer:"return-content"},showProgressIndicator:!1,data:i};t.request(f,function(n){d.draftId=n.Id;d.lastDraftErrorDate(null);d.lastDraftDate((new Date).toLocaleString());d.lastDraft=u},function(){d.lastDraftErrorDate((new Date).toLocaleString())}).always(d.setAutoSaveTimer)}function v(){var n=!0;return d.files().length>d.settings.reviewMaxFileNumber&&(d.showFilesMaxErrorMessage(!0),n=!1),d.files().length<d.settings.reviewMinFileNumber&&(d.showFilesMinErrorMessage(!0),n=!1),n}function l(t){var e,r,f,u;if(d.files().length+t.length>d.settings.reviewMaxFileNumber){n.addMessage("You can upload up to {0} files only.".format(d.settings.reviewMaxFileNumber),null,"error");return}for(e=[],r=0;r<d.files().length;r++)e[d.files()[r].originalName.toLowerCase()]=!0;for(r=0;r<t.length;r++)f=t[r],y(f,e)&&(d.uploading(d.uploading()+1),u=i.ajaxSettings.xhr(),u.open("POST",s.fileUpload,!0),u.setRequestHeader("Accept","application/json"),u.setRequestHeader("File-Name",encodeURIComponent(f.name)),u.send(f),u.addEventListener("load",function(t){t.target.status==200?a(t.target.responseText):n.processXmlHttpRequestError(t.target);d.uploading(d.uploading()-1)},!1))}function y(t,i){var u=t.name.toLowerCase(),r;if(i[u]===undefined)i[u]=!0;else return n.addMessage("Found at least two files with the same name: '{0}'.".format(t.name),null,"error"),!1;if(t.size>d.settings.reviewMaxFileSize*1048576)return n.addMessage("File '{0}' is bigger than maximum allowed size of {1} Mb.".format(t.name,d.settings.reviewMaxFileSize),null,"error"),!1;var f=t.name.substr(t.name.lastIndexOf(".")+1).toLowerCase(),e=d.settings.reviewAllowedFileTypes.split(","),o=!1;for(r=0;r<e.length;r++)if(e[r].trim().toLowerCase()==f){o=!0;break}return o?!0:(n.addMessage("File '{0}' has type '{1}' which is not accepted. We accept '{2}' only.".format(t.name,f,d.settings.reviewAllowedFileTypes),null,"error"),!1)}function a(t){var r,i;try{r=ko.utils.parseJson(t)}catch(u){n.processException(u);return}i=n.autoMap(new h,r);i.uploadDate=new Date(i.uploadDate);isNaN(i.uploadDate)&&(i.uploadDate=new Date);d.files.push(i)}d.showFilesMinErrorMessage=ko.observable(!1);d.showFilesMaxErrorMessage=ko.observable(!1);d.questions=[];d.submittedAnswersJson=null;d.autoSaveTimerId=null;d.draftId=null;d.loadedDraftDate=ko.observable();d.lastDraftDate=ko.observable();d.lastDraftErrorDate=ko.observable(null);d.lastDraft=null;d.setAutoSaveTimer=function(){return d.autoSaveTimerId&&f(d.autoSaveTimerId),d.autoSaveTimerId=u(c,n.settings.autoSaveDelay),!0};d.revertDraft=function(){ot();d.submittedAnswersJson!=null&&(e.unsubscribeAnswerChanged(d.questions),e.setAnswersFromJson(d.questions,d.submittedAnswersJson),d.setAutoSaveTimer());d.loadedDraftDate(null)};d.files=ko.observableArray();d.removeFile=function(n){d.files.remove(n)};d.uploading=ko.observable(0);d.uploadFile=function(){var n=i('<input type="file" accept="*" multiple="" />');n.on("change",function(){l(this.files)});n.trigger("click")};d.canUploadMoreFiles=ko.computed({read:function(){return d.uploading()==0&&d.files().length<d.settings.reviewMaxFileNumber},deferEvaluation:!0});d.xhrUploadSupported=function(){return o};d.fileUploadDragOver=function(n,t){d.canUploadMoreFiles()&&i(t.target).addClass("dragOver")};d.fileUploadDragLeave=function(n,t){d.canUploadMoreFiles()&&i(t.target).removeClass("dragOver")};d.fileUploadDrop=function(n,t){if(d.canUploadMoreFiles()){var i=t.originalEvent.dataTransfer.files;l(i);d.fileUploadDragLeave(n,t)}};d.uploadSingleFile=function(n,t){t.target.value!=""&&t.target.form.submit()};d.parseSingleUploadResult=function(n,t){a(t.target.contentDocument.body.innerText)};d.forceSave=function(){c()};d.save=function(){for(var f=!0,c=[],o,h,i,u,l,r=0;r<d.questions.length;r++)o=d.questions[r],g.isHidden(o.id)||c.push(o);if(h=ko.validation.group(c,{deep:!0}),h().length>0&&(h.showAllMessages(),f=!1),v()||(f=!1),f){for(i=n.autoMap(d),i.SubmissionId=d.submission.id,d.createNew||(i.Id=d.id),i.Files=[],u=0;u<d.files().length;u++)i.Files.push(d.files()[u].id);i.Answers=e.getAnswersJson(d.questions.filter(n=>!g.isHidden(n.id)));l={requestUri:n.odata.getUrl(n.odata.entitySet.reviews,d.createNew?null:d.id),method:d.createNew?"POST":"PUT",progressIndicatorTimeout:0,data:i};t.request(l,function(){n.url.navigateTo(s.returnConsole)})}}}function ut(r){return i.Deferred(function(i){if(r.Files.length==0){i.resolve();return}var u=n.odata.getUrl(n.odata.entitySet.files,{filter:n.odata.buildContainsQuery("Id",r.Files)});t.read({requestUri:u,showProgressIndicator:!1},function(t){for(var u=[],r=0;r<t.value.length;r++)u.push(n.autoMap(new h,t.value[r]));d.files(u);i.resolve()})}).promise()}function tt(){return i.Deferred(function(i){var r=n.odata.getUrl(n.odata.entitySet.reviewSettings,d.submission.trackId);t.read({requestUri:r,showProgressIndicator:!1},function(t){n.autoMap(d.settings,t);i.resolve()})}).promise()}function it(){return i.Deferred(function(t){e.loadQuestionsDirect(n.enums.formType.review,d.formId).done(function(n){d.questions=n;g.loadQuestions(n);t.resolve()})}).promise()}function ft(){return i.Deferred(function(i){var r=n.odata.getUrl(n.odata.entitySet.reviews,d.id);t.read({requestUri:r,showProgressIndicator:!1},function(t){n.autoMap(d,t);i.resolve(t)})}).promise()}function rt(u){return i.Deferred(function(i){var f=n.odata.getUrl(n.odata.entitySet.reviewDrafts,null,"GetBySubmissionIdAndReviewerId");t.read({requestUri:f,showProgressIndicator:!1,data:{SubmissionId:d.submission.id,ReviewerId:d.reviewerId},method:"POST"},function(n){if(!n){u&&e.setAnswersFromJson(d.questions,u.Answers);i.resolve(!1);return}d.loadedDraftDate(n.UpdateDate.toLocaleString());d.draftId=n.Id;var t=r.parse(n.Draft);e.setAnswersFromJson(d.questions,t);u&&(d.submittedAnswersJson=u.Answers);i.resolve(!0)},function(n){if(n.response.statusCode===404){u&&e.setAnswersFromJson(d.questions,u.Answers);i.resolve(!1);return}t.defaultError(n)})}).promise()}function et(){return i.Deferred(function(n){nt();i.when(ft(),tt(),it()).done(function(t){i.when(ut(t),rt(t)).done(function(){n.resolve()})})}).promise()}function ot(){if(!d.draftId)return i.Deferred().resolve().promise();var u={requestUri:n.odata.getUrl(n.odata.entitySet.reviewDrafts,d.draftId),method:"DELETE",showProgressIndicator:!1};return t.request(u,function(){d.draftId=null;d.lastDraftDate(null);d.lastDraftErrorDate(null);d.lastDraft=r.stringify(e.getAnswersJson(d.questions))})}var d=this,g=new n.QuestionDependency(d);d.id=l;d.formId=b;d.reviewerId=n.autoMap();d.updateDate=n.autoMap();d.settings={welcomeMessage:n.autoMap(),reviewMinFileNumber:n.autoMap(),reviewMaxFileNumber:n.autoMap(),reviewAllowedFileTypes:n.autoMap(),reviewMaxFileSize:n.autoMap()};d.submission=new c(a,y,p,w,k);d.createNew=!d.id;d.hasBranchingQuestions=function(){return g.hasDependency()};d.getQuestionDiv=function(n){return i("#rq_"+n)};d.bindTo=function(t){n.showProgress();var f=i.Deferred(),u;d.createNew?(n.autoMap(d,{reviewerId:v}),u=i.Deferred(),nt(),i.when(tt(),it()).done(function(){rt(null).done(function(){u.resolve()})})):u=et();u.promise().done(function(){ko.applyBindingsAndShow(d,t);g.init();d.lastDraft=r.stringify(e.getAnswersJson(d.questions));d.setAutoSaveTimer();f.resolve()});f.always(n.hideProgress)}}var s;n.reviewDetails=function(n,t,i,r,u,f,e,o,h,c){s=h;new l(n,t,i,r,u,f,e,o).bindTo(c)}}(window.app,window.OData,window.jQuery,window.JSON,window.setTimeout,window.clearTimeout,new window.app.QuestionService,window.FileReader!=undefined),function(n,t,i){"use strict";function r(){var t=this;t.id=n.autoMap();t.originalName=n.autoMap();t.size=n.autoMap();t.formattedSize=n.autoMap();t.uploadDate=n.autoMap();t.downloadLink=n.autoMap()}function u(){var t=this;t.order=n.autoMap();t.details=n.autoMap();t.answers=[]}function f(){var t=this;t.text=n.autoMap();t.value=n.autoMap()}function e(e){function s(){return t.read(n.odata.getUrl(n.odata.entitySet.reviewViews,o.id),function(t){var e,h,s,i,c,l;for(n.autoMap(o,t),i=0;i<t.Questions.length;i++){for(e=t.Questions[i],h=n.autoMap(new u,e),s=0;s<e.Answers.length;s++)h.answers.push(n.autoMap(new f,e.Answers[s]));o.questions.push(h)}for(i=0;i<t.Files.length;i++)c=t.Files[i],l=n.autoMap(new r,c),o.files.push(l)})}var o=this;o.id=e;o.trackName=n.autoMap();o.submissionTitle=n.autoMap();o.submissionId=n.autoMap();o.isSingleTrackConference=n.autoMap();o.questions=[];o.files=[];o.print=function(){i()};o.bindTo=function(n){s().done(function(){ko.applyBindingsAndShow(o,n)})}}n.reviewView=function(n){new e(n).bindTo("reviewForm")}}(window.app,window.OData,window.print),function(n,t,i){"use strict";function r(){var t=this;t.order=n.autoMap();t.details=n.autoMap();t.answers=[]}function u(){var t=this;t.text=n.autoMap();t.value=n.autoMap()}function f(f,e){function s(){var i;return f===n.enums.noteType.reviewer?i=n.odata.entitySet.reviewerNoteViews:f===n.enums.noteType.metaReviewer?i=n.odata.entitySet.metaReviewerNoteViews:f===n.enums.noteType.seniorMetaReviewer&&(i=n.odata.entitySet.seniorMetaReviewerNoteViews),t.read(n.odata.getUrl(i,o.id),function(t){var i,f,s,e;for(n.autoMap(o,t),i=0;i<t.Questions.length;i++){for(f=t.Questions[i],s=n.autoMap(new r,f),e=0;e<f.Answers.length;e++)s.answers.push(n.autoMap(new u,f.Answers[e]));o.questions.push(s)}})}var o=this;o.id=e;o.trackName=n.autoMap();o.submissionTitle=n.autoMap();o.submissionId=n.autoMap();o.isSingleTrackConference=n.autoMap();o.questions=[];o.print=function(){i()};o.bindTo=function(n){s().done(function(){ko.applyBindingsAndShow(o,n)})}}n.noteView=function(n,t,i){new f(n,t).bindTo(i)}}(window.app,window.OData,window.print),function(n,t,i){"use strict";function r(r){function f(){return t.read(n.odata.getUrl(n.odata.entitySet.tracks,{orderby:"Order"}),function(t){for(var r,f=[],e=u.selectedTrackId()||n.cookies.getValue("trackId"),o=!1,i=0;i<t.value.length;i++)r=n.autoMap(new n.Track,t.value[i]),f.push(r),r.id===e&&(o=!0);u.tracks(f);u.selectedTrackId(o?e:u.tracks().length===1?u.tracks()[0].id:null);u.selectedTrackId.subscribe(function(t){n.cookies.setValue("trackId",t,0,"/")})})}var u=this;u.tracks=ko.observableArray();u.selectedTrackId=ko.observable(r);u.isTrackChair=ko.observable(!1);u.trackChanged=function(t,i){var e=i.target.parentNode.parentNode,u=$(e).find("li[class|='active']"),r,f;u.length===0?n.url.navigateTo("/"+window.cmt3.conference.name+"/Settings/Index"):(r=u[0].childNodes[0],f=r&&r.attributes["data-section-scope"]&&r.attributes["data-section-scope"].value,f!=="conference"&&r.click())};u.bindTo=function(n){$.when(f(),i.getCurrentRoleDescriptor().done(function(n){u.isTrackChair(n.role==="TrackChair")})).done(function(){ko.applyBindingsAndShow(u,n)})}}n.settingsMenu=function(n){new r(n).bindTo("leftMenu")}}(window.app,window.OData,new window.app.RoleService),function(n,t,i,r,u){"use strict";function f(){var n=this;n.id=t.autoMap();n.name=t.autoMap();n.parentSubjectAreaId=t.autoMap();n.isChild=function(){return n.parentSubjectAreaId!=null};n.isVirtualRoot=function(){return n.id==null}}function e(r,u){var f=this;f.tracks=ko.observableArray();f.selectedTracks=ko.observableArray();f.editInDialog=function(){i.read(t.odata.getUrl(t.odata.entitySet.tracks,{orderby:"Order"}),function(i){for(var s,o=[],e=0;e<i.value.length;e++)i.value[e].Id!=u&&(s=t.autoMap(new t.Track,i.value[e]),o.push(s));f.tracks(o);f.selectedTracks([]);n(r).modal("show")})};f.save=function(){var e,o;f.selectedTracks().length!=0&&(e=t.autoMap(f),e.TrackId=u,e.ToTrackIds=f.selectedTracks(),o={requestUri:t.odata.getUrl(t.odata.entitySet.subjectAreas,null,"CopySubjectAreasFromTrack"),method:"POST",data:{Request:e}},i.request(o,function(){n(r).modal("hide");t.addMessage("Subject areas copied!")}))};f.bind=function(){ko.applyBindings(f,r)}}function o(r,u){var f=this,e;f.id=null;f.name=ko.observable().extend({required:!0}).autoMap();f.parentSubjectAreaId=ko.observable();f.createNew=ko.observable();e=null;f.editInDialog=function(i){return f.id=i.id,t.autoMap(f,i),f.parentSubjectAreaId(i.parentSubjectAreaId),f.createNew(i.id==null),n(r).modal("show"),e=n.Deferred(),e.promise()};f.save=function(){var s=ko.validation.group(f),o,h;if(s().length>0){s.showAllMessages();return}o=t.autoMap(f);o.TrackId=u;f.createNew()?o.ParentSubjectAreaId=f.parentSubjectAreaId():o.Id=f.id;h={requestUri:t.odata.getUrl(t.odata.entitySet.subjectAreas,f.createNew()?null:f.id),method:f.createNew()?"POST":"PUT",data:o};i.request(h,function(){n(r).modal("hide");t.addMessage("Subject area '{0}' saved!".format(f.name()));e&&e.resolve()})};f.bind=function(){ko.applyBindings(f,r)}}function s(s){function p(n){l==null&&(l=new o(r.getElementById("editDialog"),s),l.bind());l.editInDialog(n).done(w)}function v(n,i){return y[i?"addItems":"getItems"](c,n).done(function(){for(var n,r=c.length>0?c[0].isChild()?null:c[0].id:null,i=0;i<c.length;i++)n=c[i],n.isChild()&&(r==null||r!=n.parentSubjectAreaId)&&(c.splice(i,0,t.autoMap(new f,{name:""})),i++,r=n.parentSubjectAreaId),n.isChild()||(r=n.id);h.subjectAreas(c);h.showMore.updateCount(y.getTotalCount(),h.subjectAreas().length)})}function w(){y.clear();v(h.subjectAreas().length<t.settings.pageSize?1:h.subjectAreas().length/t.settings.pageSize)}var h=this,l=null,a=null,y=new t.ServerList({entitySet:t.odata.entitySet.subjectAreas,filter:function(){return h.filterString().toLowerCase()},localFilter:function(n,t){return t=t.toLowerCase(),n.name.toLowerCase().indexOf(t)>-1?n:null},itemConstructor:function(n){return t.autoMap(new f,n)},odataFilter:function(n){return"TrackId eq "+s+" and contains(tolower(Name),'{0}')".format(t.odata.escapeParam(n))},odataOrderByFields:"FlatIndex"}),c;h.showMore=new t.ShowMore(function(n){v(n,!0)});h.subjectAreas=ko.observableArray();h.filterString=ko.observable("").extend({throttle:500});h.delete=function(n){if(u("Are you sure you want to delete the subject area?")){var r={requestUri:t.odata.getUrl(t.odata.entitySet.subjectAreas,n.id),method:"DELETE"};i.request(r,function(){h.subjectAreas.remove(n);h.showMore.removeOne()},function(n){n.response.statusCode==409?t.addMessage("Subject area that you are trying to delete is being used by papers, please contact CMT.",null,"error"):i.defaultError(n)})}};h.edit=function(n){p(n)};h.addChild=function(n){p(t.autoMap(new f,{parentSubjectAreaId:n.id}))};h.addRoot=function(){p(t.autoMap(new f,{}))};h.copySubjectAreas=function(){a===null&&(a=new e(document.getElementById("copyDialog"),s),a.bind());a.editInDialog()};h.filterString.subscribe(function(){v(1)});c=[];h.bindTo=function(t){v(1).done(function(){ko.applyBindingsAndShow(h,t);n("#menuSiteFeatures").addClass("in")})}}t.settingsSubjectArea=function(n){new s(n).bindTo("subjectAreaListForm")}}(window.jQuery,window.app,window.OData,window.document,window.confirm),function(n,t,i){"use strict";function r(r,u){function h(n){i.read(t.odata.getUrl(t.odata.entitySet.submissionSettings,r),function(i){t.autoMap(f,i);n()})}var f=this,e,o,s;for(f.allowAuthorToDeleteSubmisionAfterSubmissionDeadline=ko.observable(!1).autoMap(),f.allowOnlyPrimaryContactAuthorToDeleteSubmision=ko.observable(!1).autoMap(),f.showWelcomeInstructionOnAuthorConsole=ko.observable(!1).autoMap(),f.allowAuthorToSeeDeskRejectStatus=ko.observable(!1).autoMap(),f.allowAuthorToSeeReviewingDataForWithdrawn=ko.observable(!1).autoMap(),f.abstractAllowed=ko.observable(!1).autoMap(),f.abstractAllowed.subscribe(function(n){n||f.abstractRequired(!1)}),f.abstractMaxLength=ko.observable(0).autoMap(),f.abstractRequired=ko.observable(!1).autoMap(),f.disableCoAuthors=ko.observable(!1).autoMap(),f.editAuthorsNotAllowed=ko.observable(!1).autoMap(),f.disableTitleInstruction=ko.observable(!1).autoMap(),f.titleMapping=ko.observable(null).autoMap(),f.fileUploadTitleMapping=ko.observable(null).autoMap(),f.showTipUnderFiles=ko.observable(!1).autoMap(),f.specialLayout=ko.observable(!1).autoMap(),f.submissionMinFileNumber=ko.observable(0).autoMap(),f.submissionMaxFileNumber=ko.observable(0).autoMap(),f.submissionAllowedFileTypes=ko.observable("").extend({required:!0,pattern:{params:/^ *(?:\w+(?: *, *[^$])?)+ *$/,message:"Value must be comma seprated list."}}).autoMap(),f.submissionMaxFileSize=ko.observable(0).autoMap(),f.supplementaryAllowed=ko.observable(!1).autoMap(),f.supplementaryAllowedFileTypes=ko.observable("").extend({required:{onlyIf:function(){return f.supplementaryAllowed()}},pattern:{params:/^ *(?:\w+(?: *, *[^$])?)+ *$/,message:"Value must be comma seprated list."}}).autoMap(),f.supplementaryMinFileNumber=ko.observable(0).autoMap(),f.supplementaryMaxFileNumber=ko.observable(0).autoMap(),f.supplementaryMaxFileSize=ko.observable(0).autoMap(),f.inplaceRevisionAllowed=ko.observable(!1).autoMap(),f.inplaceRevisionAllowedFileTypes=ko.observable("").extend({required:{onlyIf:function(){return f.inplaceRevisionAllowed()}},pattern:{params:/^ *(?:\w+(?: *, *[^$])?)+ *$/,message:"Value must be comma seprated list."}}).autoMap(),f.inplaceRevisionMinFileNumber=ko.observable(0).autoMap(),f.inplaceRevisionMaxFileNumber=ko.observable(0).autoMap(),f.inplaceRevisionMaxFileSize=ko.observable(0).autoMap(),f.secondarySubjectAreaAllowed=ko.observable(!1).autoMap(),f.secondarySubjectAreaLimited=ko.observable(!1).autoMap(),f.secondarySubjectAreaMaxNumber=ko.observable(0).autoMap(),f.immediateParentSelectionAllowed=ko.observable(!1).autoMap(),f.showNoneOfTheAboveSubjectArea=ko.observable(!1).autoMap(),f.showNoneOfTheAboveSubjectArea.subscribe(function(n){n&&(f.customPrimarySubjectAreaAllowed(!1),f.customSecondarySubjectAreaAllowed(!1))}),f.customPrimarySubjectAreaAllowed=ko.observable(!1).autoMap(),f.customSecondarySubjectAreaAllowed=ko.observable(!1).autoMap(),f.externalReviewerMatchingRequirementRequired=ko.observable(!1).autoMap(),f.welcomeMessage=ko.observable("").extend({maxLength:t.settings.submissionWelcomeInstructionChars}).autoMap(),f.welcomeMessageCharsLeft=ko.computed(function(){return Math.max(t.settings.submissionWelcomeInstructionChars-f.welcomeMessage().length,0)}),f.instructionAfterSubmission=ko.observable(null).autoMap(),f.referenceAllowed=ko.observable(!1).autoMap(),f.referenceInstruction=ko.observable(null).autoMap(),f.referenceMinNumber=ko.observable(0).autoMap(),f.referenceMaxNumber=ko.observable(0).autoMap(),f.referenceAllowedFileTypes=ko.observable(null).autoMap(),f.referenceMinFileNumber=ko.observable(0).autoMap(),f.referenceMaxFileNumber=ko.observable(0).autoMap(),f.referenceMaxFileSize=ko.observable(0).autoMap(),f.numbers=ko.utils.range(0,10),f.possibleLengthes=[],e=1;e<10;e++)f.possibleLengthes.push(e*1e3);o={};for(s in u)o[s.toLowerCase()]=u[s].map(function(n){return{value:n.Value,text:n.Text}});f.fileSizes=o;f.save=function(){var n=ko.validation.group(f),u,e;return n().length>0?(n.showAllMessages(),!1):(u=t.autoMap(f),e={requestUri:t.odata.getUrl(t.odata.entitySet.submissionSettings,r),method:"PUT",data:u},i.request(e,function(){t.addMessage("Submission settings have been saved!")}),!1)};f.bindTo=function(t){function i(){ko.applyBindingsAndShow(f,t);n("#menuSiteFeatures").addClass("in")}h(i)}}t.settingsSubmission=function(n,t){new r(n,t).bindTo("submissionSettingsForm")}}(window.jQuery,window.app,window.OData),function(n,t,i){"use strict";function r(r,u){function s(n){i.read(t.odata.getUrl(t.odata.entitySet.cameraReadySubmissionSettings,r),function(i){t.autoMap(f,i);n()})}var f=this,e,o;f.cameraReadySubmissionMinFileNumber=ko.observable(0).autoMap();f.cameraReadySubmissionMaxFileNumber=ko.observable(0).autoMap();f.cameraReadySubmissionAllowedFileTypes=ko.observable("").extend({required:!0,pattern:{params:/^ *(?:\w+(?: *, *[^$])?)+ *$/,message:"Value must be comma seprated list."}}).autoMap();f.cameraReadySubmissionMaxFileSize=ko.observable(0).autoMap();f.registrationRequired=ko.observable(!1).autoMap();f.publicationTitle=ko.observable("").autoMap();f.publicationSourceCode=ko.observable("").extend({pattern:{params:/^[0-9]{5}$/,message:"Value must be 5 digits."}}).autoMap();f.editCameraReadyAuthorsNotAllowed=ko.observable(!1).autoMap();f.changeCameraReadyAuthorOrderAllowed=ko.observable(!1).autoMap();f.allowMetaReviewerToViewCameraReady=ko.observable(!1).autoMap();f.allowSeniorMetaReviewerToViewCameraReady=ko.observable(!1).autoMap();f.requireReproducibilityCheckListForCameraReady=ko.observable(!1).autoMap();f.welcomeMessage=ko.observable("").extend({maxLength:t.settings.submissionWelcomeInstructionChars}).autoMap();f.welcomeMessageCharsLeft=ko.computed(function(){return Math.max(t.settings.submissionWelcomeInstructionChars-f.welcomeMessage().length,0)});f.numbers=ko.utils.range(1,10);e={};for(o in u)e[o.toLowerCase()]=u[o].map(function(n){return{value:n.Value,text:n.Text}});f.fileSizes=e;f.save=function(){var n=ko.validation.group(f),u,e;return n().length>0?(n.showAllMessages(),!1):(u=t.autoMap(f),e={requestUri:t.odata.getUrl(t.odata.entitySet.cameraReadySubmissionSettings,r),method:"PATCH",data:u},i.request(e,function(){t.addMessage("Camera Ready Submission settings have been saved!")}),!1)};f.bindTo=function(t){function i(){ko.applyBindingsAndShow(f,t);n("#menuSiteFeatures").addClass("in")}s(i)}}t.settingsCameraReadySubmission=function(n,t,i){new r(n,t).bindTo(i)}}(window.jQuery,window.app,window.OData),function(n,t,i){"use strict";function r(r){function e(n){i.read(t.odata.getUrl(t.odata.entitySet.authorFeedbackSettings,r),function(i){t.autoMap(u,i);n()})}var u=this,f;for(u.disableReviewSnapshotDuringFeedback=ko.observable(0).autoMap(),u.requestAllPapersForFeedback=ko.observable(0).autoMap(),u.authorFeedbackMinFileNumber=ko.observable(0).autoMap(),u.authorFeedbackMaxFileNumber=ko.observable(0).autoMap(),u.authorFeedbackAllowedFileTypes=ko.observable("").extend({required:!0,pattern:{params:/^ *(?:\w+(?: *, *[^$])?)+ *$/,message:"Value must be comma seprated list."}}).autoMap(),u.authorFeedbackMaxFileSize=ko.observable(0).autoMap(),u.visibleToReviewer=ko.observable(0).autoMap(),u.visibleToMetaReviewer=ko.observable(0).autoMap(),u.isAuthorFeedbackCommentingEnabled=ko.observable(0).autoMap(),u.authorFeedbackCommentMaxThreads=ko.observable(0).autoMap(),u.numbers=ko.utils.range(0,10),u.numberOfCommentThreads=ko.utils.range(1,5),u.possibleLengthes=[],f=1;f<10;f++)u.possibleLengthes.push(f*1e3);u.fileSizes=[{value:1,text:"1 MB"},{value:3,text:"3 MB"},{value:5,text:"5 MB"},{value:10,text:"10 MB"},{value:20,text:"20 MB"},{value:50,text:"50 MB"},{value:100,text:"100 MB"}];u.save=function(){var n=ko.validation.group(u),f,e;return n().length>0?(n.showAllMessages(),!1):(f=t.autoMap(u),e={requestUri:t.odata.getUrl(t.odata.entitySet.authorFeedbackSettings,r),method:"PUT",data:f},i.request(e,function(){t.addMessage("AuthorFeedback settings have been saved!")}),!1)};u.bindTo=function(t){function i(){ko.applyBindingsAndShow(u,t);n("#menuSiteFeatures").addClass("in")}e(i)}}t.settingsAuthorFeedback=function(n,t){new r(n).bindTo(t)}}(window.jQuery,window.app,window.OData),function(n,t,i){"use strict";function r(r){function f(n){i.read(t.odata.getUrl(t.odata.entitySet.conflictSettings,r),function(i){t.autoMap(u,i);n()})}var u=this;u.requireIndividualConflict=ko.observable().autoMap();u.editIndividualConflictsNotAllowed=ko.observable().autoMap();u.editConflictAllowed=ko.observable().autoMap();u.disputeConflictAllowed=ko.observable().autoMap();u.requireConflictDomains=ko.observable().autoMap();u.editPersonalConflictDomainsNotAllowed=ko.observable().autoMap();u.newPersonalConflictDomainsAllowed=ko.observable().autoMap();u.newIndividualConflictsAllowed=ko.observable().autoMap();u.requireSubmissionConflictDomains=ko.observable().autoMap();u.enableDblpConflict=ko.observable().autoMap();u.doNotComputeNewDblpConflicts=ko.observable().autoMap();u.disableMetaReviewerGroupConflict=ko.observable().autoMap();u.save=function(){var n=t.autoMap(u),f={requestUri:t.odata.getUrl(t.odata.entitySet.conflictSettings,r),method:"PATCH",data:n};return i.request(f,function(){t.addMessage("Conflict settings have been saved!")}),!1};u.bindTo=function(t){function i(){ko.applyBindingsAndShow(u,t);n("#menuSiteFeatures").addClass("in")}f(i)}}t.settingsConflict=function(n,t){new r(n).bindTo(t)}}(window.jQuery,window.app,window.OData),function(n,t,i){"use strict";function r(r){function e(n){i.read(t.odata.getUrl(t.odata.entitySet.reviewSettings,r),function(i){t.autoMap(u,i);n()})}var u=this,f;for(u.reviewMinFileNumber=ko.observable(0).autoMap(),u.reviewMaxFileNumber=ko.observable(0).autoMap(),u.reviewAllowedFileTypes=ko.observable("").extend({required:!0,pattern:{params:/^ *(?:\w+(?: *, *[^$])?)+ *$/,message:"Value must be comma seprated list."}}).autoMap(),u.reviewMaxFileSize=ko.observable(0).autoMap(),u.reviewFileVisibleToAuthor=ko.observable(!1).autoMap(),u.showReviewerIdentityToOtherReviewer=ko.observable(!1).autoMap(),u.allowReviewersToDiscussAllPapers=ko.observable(!1).autoMap(),u.allowReviewerToSeeReviewingDataOnlyAfterSubmitting=ko.observable(!1).autoMap(),u.allowReviewerToSeeReviewingDataAfterReviewing=ko.observable(!1).autoMap(),u.allowBiddingOnlyForSuggestedSubmissions=ko.observable(!1).autoMap(),u.notifyOtherReviewersForReviewUpdateDuringDiscussion=ko.observable(!1).autoMap(),u.notifyMetaReviewersForReviewUpdateDuringDiscussion=ko.observable(!1).autoMap(),u.allowReviewUpdateDuringDiscussion=ko.observable(!1).autoMap(),u.isBlind=ko.observable().autoMap(),u.enableAllPapersForDiscussion=ko.observable(!1).autoMap(),u.welcomeMessage=ko.observable("").extend({maxLength:t.settings.reviewWelcomeInstructionChars}).autoMap(),u.welcomeMessageCharsLeft=ko.pureComputed(function(){return Math.max(t.settings.reviewWelcomeInstructionChars-(this.welcomeMessage()==null?0:this.welcomeMessage().length),0)},u),u.enabledReviewAggregateColumn=ko.observable().autoMap(),u.allowInvitedReviewerToSetQuota=ko.observable().autoMap(),u.autopromoteToReviewer=ko.observable().autoMap(),u.reviewerInviteExpirationDays=ko.observable().extend({digit:!0,min:1}).autoMap(),u.maximumNumberOfEagerBidsForReviewer=ko.observable(null).extend({required:!1,digit:!0,min:0}).autoMap(),u.maximumNumberOfEagerBidsForReviewer.subscribe(function(n){n===""&&u.maximumNumberOfEagerBidsForReviewer(null)}),u.enableExternalReviewer=ko.observable().autoMap(),u.showExternalReviewerIdentityToOtherReviewer=ko.observable().autoMap(),u.allowReviewerToSeeStatusBeforeNotification=ko.observable().autoMap(),u.allowOnlyRevisionForReviewing=ko.observable().autoMap(),u.hideNonRevisionPapersDuringReviewing=ko.observable().autoMap(),u.showInlineReviewForMetaReviewer=ko.observable().autoMap(),u.showInlineReviewForSeniorMetaReviewer=ko.observable().autoMap(),u.requireReviewerSubjectArea=ko.observable().autoMap(),u.showOutOfQuotaReviewerDuringAssignment=ko.observable().autoMap(),u.doNotAllowReviewerToPostDiscussion=ko.observable().autoMap(),u.doNotAllowReviewerToEditNote=ko.observable().autoMap(),u.doNotEnableReviewerNote=ko.observable().autoMap(),u.hideDeskRejectPapersFromReviewer=ko.observable().autoMap(),u.allowReviewerToCompareSubmission=ko.observable().autoMap(),u.numbers=ko.utils.range(0,10),u.possibleLengthes=[],f=1;f<10;f++)u.possibleLengthes.push(f*1e3);u.fileSizes=[{value:1,text:"1 MB"},{value:3,text:"3 MB"},{value:5,text:"5 MB"},{value:10,text:"10 MB"},{value:20,text:"20 MB"},{value:50,text:"50 MB"},{value:100,text:"100 MB"}];u.save=function(){var n=ko.validation.group(u),f,e;return n().length>0?(n.showAllMessages(),!1):(f=t.autoMap(u),e={requestUri:t.odata.getUrl(t.odata.entitySet.reviewSettings,r),method:"PATCH",data:f},i.request(e,function(){t.addMessage("Review settings have been saved!")}),!1)};u.bindTo=function(t){function i(){ko.applyBindingsAndShow(u,t);n("#menuSiteFeatures").addClass("in")}e(i)}}t.settingsReview=function(n){new r(n).bindTo("reviewSettingsForm")}}(window.jQuery,window.app,window.OData),function(n,t,i){"use strict";function r(n){var t=this;t.Id=n.Id;t.Text=n.Text}function u(u,f){function a(n){i.read(t.odata.getUrl(t.odata.entitySet.metaReviewSettings,u),function(i){t.autoMap(e,i);e.Attributes((i.MetaReviewerConsoleDefaultHiddenColumns||"").split(";"));n()})}var e=this,h,o;for(e.metaReviewMinFileNumber=ko.observable(0).autoMap(),e.metaReviewMaxFileNumber=ko.observable(0).autoMap(),e.metaReviewAllowedFileTypes=ko.observable("").extend({required:!0,pattern:{params:/^ *(?:\w+(?: *, *[^$])?)+ *$/,message:"Value must be comma separated list."}}).autoMap(),e.metaReviewMaxFileSize=ko.observable(0).autoMap(),e.metaReviewFileVisibleToAuthor=ko.observable(!1).autoMap(),e.showMetaReviewerIdentityToReviewer=ko.observable(!1).autoMap(),e.showReviewerIdentityToMetaReviewer=ko.observable(!1).autoMap(),e.showMetaReviewerIdentityToOtherMetaReviewer=ko.observable(!1).autoMap(),e.allowMetaReviewerToAssignSubmissionToReviewer=ko.observable(!0).autoMap(),e.allowMetaReviewerToViewPaperStatus=ko.observable(!0).autoMap(),e.suggestionsEnabled=ko.observable(!0).autoMap(),e.editSuggestionNotAllowed=ko.observable(!0).autoMap(),e.isBlindToMetaReviewer=ko.observable().autoMap(),e.allowMetaReviewerToEnableDiscussion=ko.observable().autoMap(),e.allowMetaReviewerToEnableAuthorFeedback=ko.observable().autoMap(),e.allowMetaReviewerToInviteReviewers=ko.observable().autoMap(),e.allowMetaReviewerToAddReviewers=ko.observable().autoMap(),e.allowMetaReviewerToShareReviewer=ko.observable().autoMap(),e.allowMetaReviewerToSeeOtherMetaReview=ko.observable().autoMap(),e.allowMetaReviewerToEmailAuthor=ko.observable().autoMap(),e.allowMetaReviewerToRateReview=ko.observable().autoMap(),e.requireMetaReviewerSubjectArea=ko.observable().autoMap(),e.allowMetaBiddingOnlyForSuggestedSubmissions=ko.observable().autoMap(),e.includeConflictingReviewersInCandidateList=ko.observable().autoMap(),e.showInlineMetaReviewForMetaReviewer=ko.observable().autoMap(),e.showInlineMetaReviewForSeniorMetaReviewer=ko.observable().autoMap(),e.showInlineMetaReviewerNoteForSeniorMetaReviewer=ko.observable().autoMap(),e.allowMetaReviewerToSeeReviewingDataAfterReviewing=ko.observable().autoMap(),e.hideDeskRejectPapersFromMetaReviewer=ko.observable().autoMap(),e.doNotAllowMetaReviewerToEmailReviewer=ko.observable().autoMap(),e.metaWelcomeMessage=ko.observable("").extend({maxLength:t.settings.metaReviewWelcomeInstructionChars}).autoMap(),e.metaWelcomeMessageCharsLeft=ko.pureComputed(function(){return Math.max(t.settings.metaReviewWelcomeInstructionChars-(this.metaWelcomeMessage()===null?0:this.metaWelcomeMessage().length),0)},e),e.enabledMetaReviewAggregateColumn=ko.observable().autoMap(),e.autopromoteToMetaReviewer=ko.observable().autoMap(),e.metaReviewerInviteExpirationDays=ko.observable().extend({digit:!0,min:1}).autoMap(),e.doNotAllowMetaReviewerToEditNote=ko.observable().autoMap(),e.doNotEnableMetaReviewerNote=ko.observable().autoMap(),e.doNotAllowSharedMetaReviewerToEditRecommendation=ko.observable().autoMap(),e.allowMetaReviewerToCompareSubmission=ko.observable().autoMap(),e.numbers=ko.utils.range(0,10),e.possibleLengthes=[],o=1;o<10;o++)e.possibleLengthes.push(o*1e3);if(e.fileSizes=[{value:1,text:"1 MB"},{value:3,text:"3 MB"},{value:5,text:"5 MB"},{value:10,text:"10 MB"},{value:20,text:"20 MB"},{value:50,text:"50 MB"},{value:100,text:"100 MB"}],e.Attributes=ko.observableArray([]),h=[{Id:"track-column",Text:"Track"},{Id:"subject-areas-column",Text:"Subject Area"},{Id:"suggestions-column",Text:"Suggestion"},{Id:"review-column",Text:"Review"},{Id:"reviewer-note-column",Text:"Reviewer Note"},{Id:"meta-reviewer-note-column",Text:"Meta-Reviewer Note"},{Id:"meta-review-column",Text:"Meta-Review"},{Id:"discussion-feedback-column",Text:"Discussion & Feedback"}],f)for(o=0;o<f.length;o++){var s=f[o],c="question-"+(s.IsMeta?"MQ":"Q")+(s.Order<10?"0":"")+s.Order+"-column",l=(s.IsMeta?"[M] ":"[R] ")+(s.Title.length>38?s.Title.substring(0,35)+"...":s.Title);h.push({Id:c,Text:l})}e.availableAttributes=ko.observableArray([]);e.availableAttributes(ko.utils.arrayMap(h,function(n){return new r(n)}));e.save=function(){var r=ko.validation.group(e),n,f;return r().length>0?(r.showAllMessages(),!1):(n=t.autoMap(e),n.MetaReviewerConsoleDefaultHiddenColumns=e.Attributes().join(";"),f={requestUri:t.odata.getUrl(t.odata.entitySet.metaReviewSettings,u),method:"PUT",data:n},i.request(f,function(){t.addMessage("Meta-Review settings have been saved!")}),!1)};e.bindTo=function(t){function i(){ko.applyBindingsAndShow(e,t);n("#menuSiteFeatures").addClass("in")}a(i)}}t.settingsMetaReview=function(n,t){new u(n,t).bindTo("metaReviewSettingsForm")}}(window.jQuery,window.app,window.OData),function(n,t,i){"use strict";function r(n){var t=this;t.Id=n.Id;t.Text=n.Text}function u(u,f){function a(n){i.read(t.odata.getUrl(t.odata.entitySet.seniorMetaReviewSettings,u),function(i){t.autoMap(e,i);e.Attributes((i.SeniorMetaReviewerConsoleDefaultHiddenColumns||"").split(";"));n()})}var e=this,h,s;if(e.requireSeniorMetaReviewerSubjectArea=ko.observable().autoMap(),e.isBlindToSeniorMetaReviewer=ko.observable().autoMap(),e.allowSeniorMetaReviewerToViewPaperStatus=ko.observable().autoMap(),e.allowSeniorMetaReviewerToChangePaperStatus=ko.observable().autoMap(),e.allowSeniorMetaReviewerToRateSubmission=ko.observable().autoMap(),e.allowSeniorMetaReviewerToEnterRatingComment=ko.observable().autoMap(),e.allowSeniorMetaReviewerToEmailAuthor=ko.observable().autoMap(),e.assignSubmissionToSMRThroughMR=ko.observable().autoMap(),e.doNotUseSMRConflict=ko.observable().autoMap(),e.isInheritSMRConflictEnabled=ko.observable().autoMap(),e.doNotAllowSeniorMetaReviewerToEditNote=ko.observable().autoMap(),e.doNotEnableSeniorMetaReviewerNote=ko.observable().autoMap(),e.doNotAllowSeniorMetaReviewerToEditReviewAssignment=ko.observable().autoMap(),e.doNotAllowSeniorMetaReviewerToEditMetaReviewAssignment=ko.observable().autoMap(),e.doNotAllowSeniorMetaReviewerToEnableDiscussion=ko.observable().autoMap(),e.hideDeskRejectPapersFromSeniorMetaReviewer=ko.observable().autoMap(),e.allowSeniorMetaReviewerToInviteReviewers=ko.observable().autoMap(),e.Attributes=ko.observableArray([]),h=[{Id:"authors-column",Text:"Authors"},{Id:"track-column",Text:"Track"},{Id:"subject-areas-column",Text:"Subject Area"},{Id:"review-column",Text:"Review"},{Id:"reviewer-note-column",Text:"Reviewer Note"},{Id:"meta-review-column",Text:"Meta-Review"},{Id:"meta-reviewer-note-column",Text:"Meta-Reviewer Note"},{Id:"senior-meta-reviewer-note-column",Text:"Senior Meta-Reviewer Note"},{Id:"discussion-column",Text:"Discussion"},{Id:"author-feedback-requested-column",Text:"Author Feedback Requested"},{Id:"author-feedback-submitted-column",Text:"Author Feedback Submitted"},{Id:"status-column",Text:"Status"},{Id:"senior-reviewer-rating-column",Text:"Senior Meta-Reviewer Rating"},{Id:"review-rating-column",Text:"Review Rating"}],f)for(s=0;s<f.length;s++){var o=f[s],c="question-"+(o.IsMeta?"MQ":"Q")+(o.Order<10?"0":"")+o.Order+"-column",l=(o.IsMeta?"[M] ":"[R] ")+(o.Title.length>38?o.Title.substring(0,35)+"...":o.Title);h.push({Id:c,Text:l})}e.availableAttributes=ko.observableArray([]);e.availableAttributes(ko.utils.arrayMap(h,function(n){return new r(n)}));e.save=function(){var r=ko.validation.group(e),n,f;return r().length>0?(r.showAllMessages(),!1):(n=t.autoMap(e),n.SeniorMetaReviewerConsoleDefaultHiddenColumns=e.Attributes().join(";"),f={requestUri:t.odata.getUrl(t.odata.entitySet.seniorMetaReviewSettings,u),method:"PUT",data:n},i.request(f,function(){t.addMessage("Senior Meta-Review settings have been saved!")}),!1)};e.bindTo=function(t){function i(){ko.applyBindingsAndShow(e,t);n("#menuSiteFeatures").addClass("in")}a(i)}}t.settingsSeniorMetaReview=function(n,t){new u(n,t).bindTo("seniorMetaReviewSettingsForm")}}(window.jQuery,window.app,window.OData),function(n,t,i){function r(n){function u(){return i.read(t.odata.getUrl(t.odata.entitySet.iThenticateSettings,n),function(n){t.autoMap(r,n)})}var r=this;r.isEnabled=ko.observable().autoMap();r.fileDepositOption=ko.observable().autoMap();r.showAdditionalFields=ko.pureComputed(function(){return r.isEnabled()});r.save=function(){var u={requestUri:t.odata.getUrl(t.odata.entitySet.iThenticateSettings,n),method:"PATCH",data:{IsEnabled:r.isEnabled(),FileDepositOption:r.fileDepositOption()}};return i.request(u,function(){t.addMessage("iThenticate settings have been saved!")}),!1};r.bindTo=function(n){u().done(function(){ko.applyBindingsAndShow(r,n)})}}t.settingsIThenticatePage=function(t,i){n("#menuSiteFeatures").addClass("in");new r(t).bindTo(i)}}(window.jQuery,window.app,window.OData),function(n,t,i){"use strict";function u(t,i,r){function e(){o();f=u.isAssigned.subscribe(s)}function o(){f&&typeof f.dispose=="function"&&f.dispose()}function s(){u.initialState===undefined?u.initialState=u.isAssigned():h.call(u)}function h(){var i=this,r;i.isToggleInProgress(!0);r={UserId:i.id};r.Type=i.isAssigned()?"Assign":"Remove";OData.request({requestUri:n.odata.getUrl(n.odata.entitySet.submissions,t,(i.isSenior?"Senior":"")+(i.isMeta?"MetaAssign":"Assign")),method:"POST",showProgressIndicator:!1,data:{Request:r}},function(){i.isAssigned()===i.initialState?u.css(""):u.css(i.isAssigned()?"success":"error")},function(t){o();u.isAssigned(!u.isAssigned());e();n.addErrorMessage("Unable to edit assignment for '"+i.firstName+" "+i.lastName+"'. "+n.odata.getErrorMessage(t))}).always(function(){i.isToggleInProgress(!1)})}var u=this,f;u.id=n.autoMap();u.name=n.autoMap();u.firstName=n.autoMap();u.lastName=n.autoMap();u.email=n.autoMap();u.organization=n.autoMap();u.primarySubjectArea=n.autoMap();u.secondarySubjectAreas=n.autoMap();u.hiddenNumber=n.autoMap();u.bid=n.autoMap();u.relevance=n.autoMap();u.minSuggestionRank=n.autoMap();u.suggestionsJson=n.autoMap();u.tpmsRank=n.autoMap();u.trackSubmissionCount=0;u.trackSubmissionQuota=null;u.conferenceSubmissionCount=0;u.isMeta=i;u.isSenior=r;u.userType=n.autoMap();u.isAssigned=ko.observable().autoMap();u.googleScholarId=n.autoMap();u.semanticScholarId=n.autoMap();u.dblpId=n.autoMap();u.externalProfileEntered=n.autoMap();u.googleScholarUrl=function(){return n.enums.externalProfile.googleScholar.format(u.googleScholarId)};u.semanticScholarUrl=function(){return n.enums.externalProfile.semanticScholar.format(u.semanticScholarId)};u.dblpUrl=function(){return n.enums.externalProfile.dblp.format(u.dblpId)};u.suggestions=function(){var f=[],t=u.suggestionsJson?JSON.parse(u.suggestionsJson):[],i,r;if(t&&t.length>0)for(i=0;i<t.length;i++)(r=t[i],r)&&f.push(new n.Suggestion(r));return f};u.initialState=undefined;u.css=ko.observable("");u.isToggleInProgress=ko.observable(!1);e()}function r(t,i,r,u){var f=this;f.submissionId=t;f.showAssignedOnly=ko.observable("false");f.showAssignedOnly.subscribe(f.loadData,f);f.reviewers=ko.observableArray([]);f.isMeta=i;f.isSenior=r;f.userTypes=u;f.userTypesProvider=function(){return f.userTypes};n.DataTable.call(f)}function f(i){var r=this;r.id=i;r.trackId=ko.observable().autoMap();r.trackName=ko.observable().autoMap();r.title=ko.observable().autoMap();r.isSingleTrackConference=ko.observable().autoMap();r.primarySubjectAreas=ko.observableArray([]);r.secondarySubjectAreas=ko.observableArray([]);r.loadData=function(){var u=n.odata.getUrl(n.odata.entitySet.submissionViews,i,"GetSimpleView");return t.request({requestUri:u,showProgressIndicator:!1,method:"POST",headers:{"Content-Type":"application/json"}},function(t){n.autoMap(r,t);r.primarySubjectAreas(JSON.parse(t.PrimarySubjectAreas));r.secondarySubjectAreas(JSON.parse(t.SecondarySubjectAreas))})}}function e(t,u,e,o,s){var h=this;n.showProgress();h.submission=new f(t);h.table=new r(t,e,o,s);ko.applyBindings(h,i.getElementById(u));$.when(h.table.loadData(!0),h.submission.loadData()).then(function(){$("#"+u).show()}).always(n.hideProgress)}r.prototype=$.extend({},n.DataTable.prototype,{getDefaultSorting:function(){return{property:"IsAssigned",direction:"desc"}},loadData:function(i){var r,o,s;i=i===!0;r=this;i&&r.applyState();var e=r.sorting(),h=e?"&$orderby="+encodeURIComponent(e.property+" "+e.direction):"",c=r.skip()?"&$skip="+r.skip():"",l=r.top()?"&$top="+r.top():"",f="";return $.each(r.filters,function(n,t){t.getValue()&&(f+=f?" and "+t.getValue():t.getValue())}),r.showAssignedOnly()==="true"&&(f+=(f?" and":"")+" IsAssigned eq true"),f&&(f="&$filter="+encodeURIComponent(f)),o={method:"GET",headers:{Accept:"application/json"},requestUri:n.odata.getUrl(n.odata.entitySet.submissions,r.submissionId,(r.isSenior?"Senior":"")+(r.isMeta?"MetaReviewers":"Reviewers"))+"?$count=true"+f+h+c+l,showProgressIndicator:!i},s=t.request(o,function(t){var o,e,i,f;for(r.total(t["@odata.count"]||0),o=[],e=0;e<t.value.length;e++)i=t.value[e],f=n.autoMap(new u(r.submissionId,r.isMeta,r.isSenior),i),f.trackSubmissionCount=i.TrackCount,f.trackSubmissionQuota=i.Quota,f.conferenceSubmissionCount=i.AllTracksCount,o.push(f);r.reviewers(o);r.saveState()},function(t){n.addErrorMessage(n.odata.getErrorMessage(t))}),s}});n.submissionAssignReviewers=function(n,t,i,r,u){new e(n,t,i,r,u)}}(window.app,window.OData,window.document),function(n,t,i,r){"use strict";function e(){var t=this;t.id=n.autoMap();t.name=n.autoMap();t.description=n.autoMap()}function o(){var t=this;t.id=n.autoMap();t.markedBySystem=n.autoMap()}function s(t,u){function o(){s();e=f.isChecked.subscribe(h)}function s(){e&&typeof e.dispose=="function"&&e.dispose()}function h(){f.initialState===undefined?f.initialState=f.isChecked():c.call(f)}function c(){var t=this,e,h,c;t.isToggleInProgress(!0);e={UserId:f.reviewer.id,ReasonId:f.id()};e.Type=t.isChecked()?"Add":"Remove";h=i.Deferred(function(n){r.setTimeout(n.resolve,500)});c=OData.request({requestUri:n.odata.getUrl(n.odata.entitySet.submissions,u,"ModifyConflict"),method:"POST",showProgressIndicator:!1,data:{Request:e}},function(){},function(t){s();f.isChecked(!f.isChecked());o();n.addErrorMessage("Unable to edit conflict."+n.odata.getErrorMessage(t))});i.when(c,h).always(function(){t.isToggleInProgress(!1)})}var f=this,e;f.reviewer=t;f.id=ko.observable().autoMap();f.name=n.autoMap();f.isChecked=ko.observable();f.isMarkedBySystem=ko.observable(!1);f.enabled=ko.observable(!0);f.isAutoConflict=ko.computed(function(){return f.id()>=100||f.isMarkedBySystem()});f.isEnabled=ko.computed(function(){return f.enabled()&&!f.isAutoConflict()});f.initialState=undefined;f.isToggleInProgress=ko.observable(!1);o()}function h(t,i){var r=this;r.id=n.autoMap();r.firstName=n.autoMap();r.lastName=n.autoMap();r.email=n.autoMap();r.organization=n.autoMap();r.isEditingConflictsAllowed=n.autoMap();r.hasConflicts=ko.pureComputed(function(){return r.reviewerCheckedConflictReasons().length>0});r.hasConflictsText=ko.pureComputed(function(){return r.hasConflicts().toYesNo()});r.selectedConflictReasons={};r.reviewerConflictReasons=ko.pureComputed(function(){for(var u,e,o=[],f=0;f<i.length;f++)u=n.autoMap(new s(r,t),i[f]),e=r.selectedConflictReasons[u.id()],e?(u.isChecked(!0),u.isMarkedBySystem(e.markedBySystem)):u.isChecked(!1),o.push(u);return o});r.reviewerCheckedConflictReasons=ko.pureComputed(function(){for(var i=[],t=r.reviewerConflictReasons(),n=0;n<t.length;n++)t[n].isChecked()&&i.push(t[n]);return i})}function u(t,i,r){var u=this;u.submissionId=t;u.showEmail=r;u.reviewers=ko.observableArray([]);u.conflictReasons=i;u.conflictReasonProvider=function(){var t=[""],n;if(i){for(n=0;n<i.length;n++)t.push(i[n].name);return t}};n.DataTable.call(u)}function c(r,f,o,s,h,c,l){function v(){var i={requestUri:n.odata.getUrl(n.odata.entitySet.conflictReasons),method:"GET",headers:{"Content-Type":"application/json"},showProgressIndicator:!1};return t.request(i,function(t){for(var r,i=0;i<t.value.length;i++)r=n.autoMap(new e,t.value[i]),a.conflictReasons.push(r),a.conflictReasonsHash[r.id]=r})}var a=this;a.id=r;a.trackId=o;a.trackName=s;a.title=f;a.isSingleTrackConference=h;a.instructionForSubmissionConflict=c;a.conflictReasons=[];a.conflictReasonsHash={};a.submissionConflictDataTable=new u(r,a.conflictReasons,l);a.returnTrue=function(){return!0};a.bindTo=function(t){n.showProgress();i.when(a.submissionConflictDataTable.loadData(!0),v()).done(function(){ko.applyBindingsAndShow(a,t)}).always(n.hideProgress)}}var f;u.prototype=i.extend({},n.DataTable.prototype,{getDefaultSorting:function(){return{property:"HasConflicts",direction:"desc"}},loadData:function(r){var u,s,c;r=r===!0;u=this;r&&u.applyState();var e=u.sorting(),l=e.property!=="FirstName"?",FirstName asc":"",a=e?"&$orderby="+encodeURIComponent(e.property+" "+e.direction+l):"",v=u.skip()?"&$skip="+u.skip():"",y=u.top()?"&$top="+u.top():"",f="";return i.each(u.filters,function(n,t){t.getValue()&&(f+=f?" and "+t.getValue():t.getValue())}),f&&(f="&$filter="+encodeURIComponent(f)),s={method:"GET",headers:{Accept:"application/json"},requestUri:n.odata.getUrl(n.odata.entitySet.submissions,u.submissionId,"ConflictSelections")+"?$count=true"+f+a+v+y,showProgressIndicator:!r},c=t.request(s,function(t){var e,r,i,s,f,c;for(u.total(t["@odata.count"]||0),e=[],r=0;r<t.value.length;r++){if(i=t.value[r],s=n.autoMap(new h(u.submissionId,u.conflictReasons),i),i.ConflictReasons)for(f=0;f<i.ConflictReasons.length;f++)c=i.ConflictReasons[f],s.selectedConflictReasons[c.Id]=n.autoMap(new o,c);e.push(s)}u.reviewers(e);u.saveState()},function(t){n.addErrorMessage(n.odata.getErrorMessage(t))}),c}});n.submissionConflict=function(t,i,r,u,e,o,s,h){f=s;var l=n.cookies.getValue(".ROLE"),a=l==="Chair"||l==="TrackChair"||l==="SeniorMetaReviewer";new c(t,i,r,u,e,o,a).bindTo(h)}}(window.app,window.OData,window.jQuery,window),function(n,t,i,r,u,f,e){"use strict";function o(){var t=this;t.userId=n.autoMap();t.authorId=n.autoMap();t.email=n.autoMap();t.firstName=n.autoMap();t.lastName=n.autoMap();t.organization=n.autoMap();t.countryCode=n.autoMap();t.countryName=n.autoMap();t.isPrimary=n.autoMap();t.fullName=ko.pureComputed(function(){return t.firstName+" "+t.lastName})}function c(t){var i=this;i.email=ko.observable().extend({email:!0,required:!0,validation:{validator:function(n,t){for(var i=0;i<t.length;i++)if(t[i].email===n)return!1;return!0},message:"Author with the same email already exists.",params:t}});i.isEmailInvalid=ko.observable(!1);i.firstName=ko.observable().extend({required:{message:"First Name is required."},maxLength:200});i.lastName=ko.observable().extend({required:{message:"Last Name is required."},maxLength:200});i.organization=ko.observable().extend({required:{message:"Organization is required."},maxLength:200});i.availableCountries=ko.observable(n.countries.getCountries());i.countryCode=ko.observable().extend({required:{message:"Country is required."}});i.isSearching=ko.observable(!1);i.notFound=ko.observable(!1);i.cancelAdd=function(){i.email("");i.email.isModified(!1);i.firstName("");i.firstName.isModified(!1);i.lastName("");i.lastName.isModified(!1);i.organization("");i.organization.isModified(!1);i.countryCode(undefined);i.countryCode.isModified(!1);i.notFound(!1);i.isEmailInvalid(!1)}}function h(){var t=this;t.id=n.autoMap();t.name=n.autoMap();t.parentSubjectAreaId=n.autoMap();t.isChild=function(){return t.parentSubjectAreaId!==null};t.isPrimary=ko.observable();t.isSecondary=ko.observable();t.checkBoxId=function(){return"primary"+t.id};t.allowParentSelection=!0;t.specialType=null;t.customValue=ko.observable(null).extend({required:{onlyIf:function(){return t.isPrimary()||t.isSecondary()}}})}function l(){var t=this;t.id=n.autoMap();t.originalName=n.autoMap();t.size=n.autoMap();t.formattedSize=n.autoMap();t.uploadDate=n.autoMap();t.downloadLink=n.autoMap()}function a(){var n=this}function v(v,y,p,w,b,k,d,g,nt,tt,it,rt,ut,ft,et){function ht(){function h(){var n=!0;return ot.files().length>ot.settings.submissionMaxFileNumber&&(ot.showFilesMaxErrorMessage(!0),n=!1),n}function a(){var n=!0;return ot.references().length>ot.settings.referenceMaxNumber&&(ot.showReferencesMaxErrorMessage(!0),n=!1),ot.references().length<ot.settings.referenceMinNumber&&(ot.showReferencesMinErrorMessage(!0),n=!1),n}function v(){var t=ot.authors(),i,n,r;if(ot.isAuthorRole()&&!ot.createNew&&ot.settings.editAuthorsNotAllowed&&t.length===0)return!0;for(i=!1,n=0;n<t.length;n++)if(t[n].email===ot.primaryEmail()){i=!0;break}return r=!0,i||(ot.showPrimaryAuthorErrorMessage(!0),r=!1),r}function y(){if(!ft)return ot.showConferenceRequestChairsErrorMessage(!1),!0;var n=ot.conferenceRequestChairs().length>0;return n||ot.showConferenceRequestChairsErrorMessage(!0),n}function p(){var i,r,n,t,u;if(ot.subjectAreas.length===0)return!0;for(i=[],r=!1,n=0;n<ot.subjectAreas.length;n++)(ot.subjectAreas[n].specialType==="customPrimary"||ot.subjectAreas[n].specialType==="customSecondary")&&i.push(ot.subjectAreas[n].customValue),ot.subjectAreas[n].isPrimary()&&(r=!0);return t=!0,u=ko.validation.group(i),u().length>0&&(u.showAllMessages(),t=!1),r||(ot.showSubjectAreasErrorMessage(!0),t=!1),t}function r(t){var o,r,f,u;if(ot.files().length+t.length>ot.settings.submissionMaxFileNumber){n.addMessage("You can upload up to {0} files only.".format(ot.settings.submissionMaxFileNumber),null,"error");return}for(o=[],r=0;r<ot.files().length;r++)o[ot.files()[r].originalName.toLowerCase()]=!0;for(r=0;r<t.length;r++)f=t[r],w(f,o)&&(ot.uploading(ot.uploading()+1),u=i.ajaxSettings.xhr(),u.open("POST",s.fileUpload,!0),u.setRequestHeader("Accept","application/json"),u.setRequestHeader("File-Name",encodeURIComponent(f.name)),u.send(f),u.addEventListener("load",function(t){t.target.status===200?e(t.target.responseText):n.processXmlHttpRequestError(t.target);ot.uploading(ot.uploading()-1)},!1))}function w(t,i){var u=t.name.toLowerCase(),r;if(i[u]===undefined)i[u]=!0;else return n.addMessage("Found at least two files with the same name: '{0}'.".format(t.name),null,"error"),!1;if(t.size>ot.settings.submissionMaxFileSize*1048576)return n.addMessage("File '{0}' is bigger than maximum allowed size of {1} Mb.".format(t.name,ot.settings.submissionMaxFileSize),null,"error"),!1;var f=t.name.substr(t.name.lastIndexOf(".")+1).toLowerCase(),e=ot.settings.submissionAllowedFileTypes.split(","),o=!1;for(r=0;r<e.length;r++)if(e[r].trim().toLowerCase()===f){o=!0;break}return o?!0:(n.addMessage("File '{0}' has type '{1}' which is not accepted. We accept '{2}' only.".format(t.name,f,ot.settings.submissionAllowedFileTypes),null,"error"),!1)}function e(t){var r,i;try{r=ko.utils.parseJson(t)}catch(u){n.processException(u);return}i=n.autoMap(new l,r);i.uploadDate=new Date(i.uploadDate);isNaN(i.uploadDate)&&(i.uploadDate=new Date);ot.files.push(i)}ot.title=ko.observable().extend({required:!0,maxLength:1e3}).autoMap();ot.abstract=ko.observable("").extend({required:{onlyIf:function(){return ot.settings.abstractAllowed&&ot.settings.abstractRequired}},maxLength:ot.settings.abstractMaxLength}).autoMap();ot.abstractCharsLeft=ko.computed(function(){return Math.max(ot.settings.abstractMaxLength-ot.abstract().length,0)});ot.statusId=n.autoMap();ot.submissionListUrl=null;ot.authorizeSendingSubmissionToTpms=ko.observable().extend({requiredCheckbox:{message:"Your agreement is required.",onlyIf:function(){return ot.trackSettings.isTpmsEnabled}}}).autoMap();ot.authorizeSendingSubmissionToIThenticate=ko.observable().extend({requiredCheckbox:{message:"Your agreement is required.",onlyIf:function(){return ot.trackSettings.isIThenticateEnabled}}}).autoMap();ot.submissionConflictDomainsRaw=ko.observable().extend({required:{message:"Domain conflicts are required.",onlyIf:function(){return ot.trackSettings.isSubmissionConflictDomainsRequired}}}).autoMap();ot.showPrimaryAuthorErrorMessage=ko.observable(!1);ot.showFilesMaxErrorMessage=ko.observable(!1);ot.showReferencesMinErrorMessage=ko.observable(!1);ot.showReferencesMaxErrorMessage=ko.observable(!1);ot.removeAuthor=function(n){ot.authors.remove(n)};ot.moveAuthorUp=function(n){var t=ot.authors.indexOf(n);ot.authors.remove(n);ot.authors.splice(t-1,0,n)};ot.moveAuthorDown=function(n){var t=ot.authors.indexOf(n);ot.authors.remove(n);ot.authors.splice(t+1,0,n)};ot.addAuthor=function(t){var r=ko.validation.group([t.email,t.firstName,t.lastName,t.organization,t.countryCode]),i;if(r().length>0){r.showAllMessages();t.isEmailInvalid(!t.email.isValid());return}i=n.autoMap(new o,{isPrimary:!1,email:t.email(),firstName:t.firstName(),lastName:t.lastName(),organization:t.organization(),countryCode:t.countryCode(),countryName:n.countries.getCountryNameByCode(t.countryCode())});ot.authors.push(i);ot.authors().length===1&&(ot.primaryEmail(i.email),ot.showPrimaryAuthorErrorMessage(!1));t.cancelAdd()};ot.newAuthor=new c(ot.authors);ot.searchAuthorByEmail=function(i){var r=ko.validation.group([i.email]),u;if(r().length>0){i.isEmailInvalid(!0);r.showAllMessages();return}i.isEmailInvalid(!1);i.isSearching(!0);u={requestUri:n.odata.getGlobalUrl(n.odata.entitySet.users,null,"SearchByEmail"),method:"POST",showProgressIndicator:!1,data:{Email:i.email()}};t.read(u,function(t){var r=n.autoMap(new o,t);r.userId=t.Id;ot.authors.push(r);ot.authors().length===1&&(ot.primaryEmail(r.email),ot.showPrimaryAuthorErrorMessage(!1));i.cancelAdd();i.isSearching(!1)},function(r){i.isSearching(!1);r.response.statusCode===n.enums.httpStatusCodes.failure.notFound?ot.newAuthor.notFound(!0):t.defaultError(r)})};ot.showConferenceRequestChairsErrorMessage=ko.observable(!1);ot.removeChair=function(n){ot.conferenceRequestChairs.remove(n);ot.conferenceRequestChairs().length===0&&ot.showConferenceRequestChairsErrorMessage(!0)};ot.newConferenceRequestChair=new c(ot.conferenceRequestChairs);ot.searchConferenceRequestChairByEmail=function(i){var r=ko.validation.group([i.email]),u;if(r().length>0){i.isEmailInvalid(!0);r.showAllMessages();return}i.isEmailInvalid(!1);i.isSearching(!0);u={requestUri:n.odata.getGlobalUrl(n.odata.entitySet.users,null,"SearchByEmail"),method:"POST",showProgressIndicator:!1,data:{Email:i.email()}};t.read(u,function(t){var r=n.autoMap(new o,t);r.userId=t.Id;ot.conferenceRequestChairs.push(r);ot.conferenceRequestChairs().length>0&&ot.showConferenceRequestChairsErrorMessage(!1);i.cancelAdd();i.isSearching(!1)},function(r){i.isSearching(!1);r.response.statusCode===n.enums.httpStatusCodes.failure.notFound?ot.newConferenceRequestChair.notFound(!0):t.defaultError(r)})};ot.subjectAreas=[];ot.subjectAreaPairs=function(){return n.computeSubjectAreaColumnPairs(ot.subjectAreas)};ot.showSubjectAreasErrorMessage=ko.observable(!1);ot.subjectAreaSectionClassName=function(){return ot.subjectAreas.length<40?"small-subjectarea-section":"large-subjectarea-section"};ot.showValidationWarning=ko.observable(!1);ot.references=ko.observableArray();ot.removeReference=function(n){ot.references.remove(n)};ot.addReference=function(t){var i=ko.validation.group([t.email,t.firstName,t.lastName,t.organization,t.countryCode]),r;if(i().length>0){i.showAllMessages();t.isEmailInvalid(!t.email.isValid());return}r=n.autoMap(new o,{email:t.email(),firstName:t.firstName(),lastName:t.lastName(),organization:t.organization(),countryCode:t.countryCode(),countryName:n.countries.getCountryNameByCode(t.countryCode())});ot.references.push(r);t.cancelAdd()};ot.newReference=new c(ot.references);ot.searchReferenceByEmail=function(i){var r=ko.validation.group([i.email]),u;if(r().length>0){i.isEmailInvalid(!0);r.showAllMessages();return}i.isEmailInvalid(!1);i.isSearching(!0);u={requestUri:n.odata.getGlobalUrl(n.odata.entitySet.users,null,"SearchByEmail"),method:"POST",showProgressIndicator:!1,data:{Email:i.email()}};t.read(u,function(t){var r=n.autoMap(new o,t);r.userId=t.Id;ot.references.push(r);i.cancelAdd();i.isSearching(!1)},function(r){i.isSearching(!1);r.response.statusCode===n.enums.httpStatusCodes.failure.notFound?ot.newReference.notFound(!0):t.defaultError(r)})};ot.files=ko.observableArray();ot.removeFile=function(n){ot.files.remove(n)};ot.uploading=ko.observable(0);ot.uploadFile=function(){var n=i('<input type="file" accept="*" multiple="" />');n.on("change",function(){r(this.files)});n.trigger("click")};ot.canUploadMoreFiles=ko.computed(function(){return ot.uploading()===0&&ot.files().length<ot.settings.submissionMaxFileNumber});ot.xhrUploadSupported=function(){return u};ot.fileUploadDragOver=function(n,t){ot.canUploadMoreFiles()&&i(t.target).addClass("dragOver")};ot.fileUploadDragLeave=function(n,t){ot.canUploadMoreFiles()&&i(t.target).removeClass("dragOver")};ot.fileUploadDrop=function(n,t){if(ot.canUploadMoreFiles()){var i=t.originalEvent.dataTransfer.files;r(i);ot.fileUploadDragLeave(n,t)}};ot.uploadSingleFile=function(n,t){t.target.value!==""&&t.target.form.submit()};ot.parseSingleUploadResult=function(n,t){e(t.target.contentDocument.body.innerText)};ot.submissionQuestions=[];ot.reproQuestions=[];ot.save=function(){function ft(i){var r=n.autoMap(i),u;return delete r.UserId,delete r.AuthorId,delete r.IsPrimary,u={requestUri:n.odata.getUrl(n.odata.entitySet.users,null,"AddCoAuthor"),method:"POST",data:{Request:r}},t.request(u,function(n){it[i.email]=n.value},function(i){if(i.response.statusCode==n.enums.httpStatusCodes.failure.conflict)n.addMessage(r,"Please click Cancel and use the email box to select author.","error");else if(i.response.statusCode==n.enums.httpStatusCodes.failure.badRequest){var r=n.getODataErrorMessage(i).message;n.addMessage(r,"Author information invalid:","error")}else t.defaultError(i)})}var o=!0,l=ko.validation.group(ot,{deep:!1}),k,u,d,g,nt,tt,r,c,e,ut,w,it,rt,b;for(l().length>0&&(l.showAllMessages(),o=!1),v()||(o=!1),y()||(o=!1),p()||(o=!1),ot.settings.referenceAllowed&&!a()&&(o=!1),h()||(o=!1),k=[],u=0;u<ot.submissionQuestions.length;u++)d=ot.submissionQuestions[u],st.isHidden(d.id)||k.push(d);for(l=ko.validation.group(k,{deep:!0}),l().length>0&&(l.showAllMessages(),o=!1),g=[],u=0;u<ot.reproQuestions.length;u++)for(nt=ot.reproQuestions[u],c=0;c<nt.choices.length;c++)g.push(nt.choices[c]);if(tt=ko.validation.group(g,{deep:!0}),tt().length>0&&(tt.showAllMessages(),o=!1),!o){ot.showValidationWarning(!0);return}for(r=n.autoMap(ot),ot.createNew?(r.TrackId=ot.trackId,r.StatusId=0):r.Id=ot.id,r.SubjectAreas=[],r.NoneOfAboveSubjectArea=!1,r.CustomPrimarySubjectArea=null,r.CustomSecondarySubjectArea=null,c=0;c<ot.subjectAreas.length;c++)e=ot.subjectAreas[c],(e.isPrimary()||e.isSecondary())&&(e.specialType===null?(ut={SubjectAreaId:e.id,IsPrimary:e.isPrimary()},r.SubjectAreas.push(ut)):e.specialType==="noneOfAbove"?r.NoneOfAboveSubjectArea=!0:e.specialType==="customPrimary"?r.CustomPrimarySubjectArea=e.customValue():e.specialType==="customSecondary"&&(r.CustomSecondarySubjectArea=e.customValue()));for(r.Files=[],w=0;w<ot.files().length;w++)r.Files.push(ot.files()[w].id);if(r.Answers=f.getAnswersJson(ot.submissionQuestions.filter(n=>!st.isHidden(n.id))),r.ReproducibilityAnswers=f.getAnswersJson(ot.reproQuestions),it={},rt=[],!ot.isAuthorRole()||ot.createNew||!ot.settings.editAuthorsNotAllowed)for(u=0;u<ot.authors().length;u++)b=ot.authors()[u],b.userId||b.authorId||rt.push(ft(b));i.when.apply(i,rt).done(function(){var i,u,o,f,h,e,c,l;if(r.Authors=[],r.ConferenceRequestChairs=[],r.References=[],!ot.isAuthorRole()||ot.createNew||!ot.settings.editAuthorsNotAllowed)for(i=0;i<ot.authors().length;i++)u=ot.authors()[i],u.userId||u.authorId||(u.authorId=it[u.email]),o={Order:i+1,IsPrimary:u.email===ot.primaryEmail(),UserId:u.userId,AuthorId:u.authorId,Email:u.email},r.Authors.push(o);for(i=0;i<ot.conferenceRequestChairs().length;i++)f=ot.conferenceRequestChairs()[i],h={UserId:f.userId,Email:f.email},r.ConferenceRequestChairs.push(h);for(i=0;i<ot.references().length;i++)e=ot.references()[i],c={UserId:e.userId,Email:e.email},r.References.push(c);l={requestUri:n.odata.getUrl(n.odata.entitySet.submissions,ot.createNew?null:ot.id),method:ot.createNew?"POST":"PATCH",headers:{Prefer:"return-content"},progressIndicatorTimeout:0,data:r};t.request(l,function(t){ot.editConflictAllowed?n.url.navigateTo(s.submissionConflict.format(t.Id)):n.url.navigateTo(s.submissionSummary.format(t.Id))})})}}function ct(t){return i.Deferred(function(){var y,h,p,tt,w,it,b,r,k,c,l,d;n.autoMap(ot,t);var i,e,u,s,v={},g=[],nt=[];if(t.AuthorsJson)for(y=JSON.parse(t.AuthorsJson),i=0;i<y.length;i++)h=n.autoMap(new o,y[i]),ot.authors.push(h),h.isPrimary&&ot.primaryEmail(h.email);if(t.ConferenceRequestChairsJson)for(p=JSON.parse(t.ConferenceRequestChairsJson),i=0;i<p.length;i++)tt=n.autoMap(new o,p[i]),ot.conferenceRequestChairs.push(tt);if(t.ReferencesJson)for(w=JSON.parse(t.ReferencesJson),i=0;i<w.length;i++)it=n.autoMap(new o,w[i]),ot.references.push(it);if(t.PrimarySubjectAreaId&&(v[t.PrimarySubjectAreaId]=!0),t.SecondarySubjectAreasJson)for(b=JSON.parse(t.SecondarySubjectAreasJson),i=0;i<b.length;i++)v[b[i].SubjectAreaId]=!1;for(i=0;i<ot.subjectAreas.length;i++)r=ot.subjectAreas[i],k=v[r.id],k?r.isPrimary(!0):k===!1&&r.isSecondary(!0),r.specialType==="noneOfAbove"&&t.NoneOfAboveSubjectArea&&r.isPrimary(!0),r.specialType==="customPrimary"&&t.CustomPrimarySubjectArea!==null&&(r.isPrimary(!0),r.customValue(t.CustomPrimarySubjectArea)),r.specialType==="customSecondary"&&t.CustomSecondarySubjectArea!==null&&(r.isSecondary(!0),r.customValue(t.CustomSecondarySubjectArea));if(t.QuestionAnswersJson)for(c=JSON.parse(t.QuestionAnswersJson),i=0;i<c.length;i++)if(s=c[i].Answers,s)for(e=0;e<s.length;e++)u=new a,u.QuestionId=c[i].Id,u.Text=s[e].Text,u.QuestionChoiceId=s[e].QuestionChoiceId,g.push(u);if(f.setAnswersFromJson(ot.submissionQuestions,g),t.ReproducibilityQuestionAnswersJson)for(l=JSON.parse(t.ReproducibilityQuestionAnswersJson),i=0;i<l.length;i++)if(s=l[i].Answers,s)for(e=0;e<s.length;e++)u=new a,u.QuestionId=l[i].Id,u.QuestionChoiceId=s[e].QuestionChoiceId,d=JSON.parse(s[e].Text),u.Answer=d.Answer,u.Comment=d.Comment,nt.push(u);f.setAnswersFromJson(ot.reproQuestions,nt);n.url.hash.getValue()==="saved"&&(n.url.hash.remove(),n.addMessage("Submission '{0}' saved!".format(ot.title())))}).promise()}function lt(){return f.loadQuestionsDirect(n.enums.formType.submission,ot.submissionFormId).done(function(n){ot.submissionQuestions=n;st.loadQuestions(n)})}function at(){return f.loadQuestionsDirect(n.enums.formType.reproducibility,ot.reproFormId).done(function(n){var t,r,i;for(ot.reproQuestions=n,t=0;t<n.length;t++)for(r=n[t],i=0;i<r.choices.length;i++)r.choices[i].requireAnswer(!0)})}function vt(){e.getCurrentRoleDescriptor().done(function(t){ot.submissionListUrl=t.submissionListUrl;ot.isAuthorRole(ot.role===n.enums.userRole.author)})}function yt(t){function o(n){n||(this.customValue(null),this.customValue.isModified(!1))}function e(n){n.isPrimary.subscribe(function(n){n&&(ot.showSubjectAreasErrorMessage(!1),s(this),this.isSecondary(!1))},n);n.isSecondary.subscribe(function(n){var t,i;if(n){if(ot.settings.secondarySubjectAreaLimited&&(t=c(),t>ot.settings.secondarySubjectAreaMaxNumber)){i=this;r(function(){i.isSecondary(!1)},0);return}this.isPrimary(!1)}},n);ot.subjectAreas.push(n)}function s(n){for(var t=0;t<ot.subjectAreas.length;t++)ot.subjectAreas[t].isPrimary()&&ot.subjectAreas[t]!==n&&ot.subjectAreas[t].isPrimary(!1)}function c(){for(var t=0,n=0;n<ot.subjectAreas.length;n++)ot.subjectAreas[n].isSecondary()&&++t;return t}var u,i,f;if(t){for(u=null,f=0;f<t.length;f++)i=n.autoMap(new h,t[f]),u!==null&&u.id===i.parentSubjectAreaId&&!ot.settings.immediateParentSelectionAllowed&&u.allowParentSelection&&(u.allowParentSelection=!1),i.parentSubjectAreaId===null&&(u=i),e(i);ot.settings.showNoneOfTheAboveSubjectArea&&(i=new h,i.specialType="noneOfAbove",e(i));ot.settings.customPrimarySubjectAreaAllowed&&(i=new h,i.specialType="customPrimary",i.isPrimary.subscribe(o,i),e(i));ot.settings.customSecondarySubjectAreaAllowed&&ot.settings.secondarySubjectAreaAllowed&&(i=new h,i.specialType="customSecondary",i.isSecondary.subscribe(o,i),e(i))}}function pt(i){if(i.length===0)return!0;var r=n.odata.getUrl(n.odata.entitySet.files,{filter:n.odata.buildContainsQuery("Id",i)});return t.read({requestUri:r,showProgressIndicator:!1},function(t){for(var r=[],i=0;i<t.value.length;i++)r.push(n.autoMap(new l,t.value[i]));ot.files(r)})}function wt(){return ot.createNew?i.Deferred().resolve(null).promise():i.Deferred(function(i){var r={requestUri:n.odata.getUrl(n.odata.entitySet.submissionViews,ot.id,"GetSummaryView"),headers:{"Content-Type":"application/json"},showProgressIndicator:!1,method:"POST"};t.read(r,function(n){i.resolve(n)})}).promise()}var ot=this,st=new n.QuestionDependency(ot);ot.id=v;ot.createNew=!v;ot.trackId=y;ot.trackName=p;ot.submissionFormId=w;ot.reproFormId=b;ot.editConflictAllowed=k;ot.isSingleTrackConference=d;ot.role=g;ot.fileIds=tt;ot.titleTitle="Title";ot.fileUploadTitle="Files";ot.isAuthor=ko.observable(!1);ot.isAuthorRole=ko.observable(!1);ot.authors=ko.observableArray();ot.primaryEmail=ko.observable();ot.createNewSubmissionText=et&&et.CreateNewSubmissionText?et.CreateNewSubmissionText:"Create new submission";ot.editSubmissionText=et&&et.EditSubmissionText?et.EditSubmissionText:"Edit Submission";ot.conferenceRequestChairs=ko.observableArray();ot.settings={welcomeMessage:n.autoMap(),abstractAllowed:n.autoMap(),abstractMaxLength:n.autoMap(),abstractRequired:n.autoMap(),showNoneOfTheAboveSubjectArea:n.autoMap(),secondarySubjectAreaAllowed:n.autoMap(),secondarySubjectAreaLimited:n.autoMap(),secondarySubjectAreaMaxNumber:n.autoMap(),immediateParentSelectionAllowed:n.autoMap(),customPrimarySubjectAreaAllowed:n.autoMap(),customSecondarySubjectAreaAllowed:n.autoMap(),submissionMinFileNumber:n.autoMap(),submissionMaxFileNumber:n.autoMap(),submissionAllowedFileTypes:n.autoMap(),submissionMaxFileSize:n.autoMap(),referenceMinNumber:n.autoMap(),referenceMaxNumber:n.autoMap(),referenceAllowed:n.autoMap(),referenceAdditionalRequirement:n.autoMap(),disableCoAuthors:n.autoMap(),disableTitleInstruction:n.autoMap(),titleMapping:n.autoMap(),fileUploadTitleMapping:n.autoMap(),showTipUnderFiles:n.autoMap(),editAuthorsNotAllowed:n.autoMap()};n.autoMap(ot.settings,it);ot.settings.titleMapping!==null&&(ot.titleTitle=ot.settings.titleMapping);ot.settings.fileUploadTitleMapping!==null&&(ot.fileUploadTitle=ot.settings.fileUploadTitleMapping);ot.trackSettings=nt;ot.currentProfile=n.autoMap(new o,ut);ot.currentProfile.userId=ut.Id;ot.createNew&&ot.role===n.enums.userRole.author?(ot.authors([ot.currentProfile]),ft&&ot.conferenceRequestChairs([ot.currentProfile]),ot.primaryEmail(ot.currentProfile.email),ot.isAuthor(!0)):ot.isAuthor(!1);ot.hasBranchingQuestions=function(){return st.hasDependency()};ot.doNotAllowEditAuthorList=function(){return(ot.settings.editAuthorsNotAllowed||ot.settings.disableCoAuthors)&&ot.isAuthorRole()};ot.getQuestionDiv=function(n){return i("#sq_"+n)};ot.bindTo=function(t){n.showProgress();var r=i.Deferred();ht();yt(rt);i.when(wt(),lt(),at(),vt(),pt(ot.fileIds)).done(function(n){ot.createNew||ct(n);ko.applyBindingsAndShow(ot,t);st.init();r.resolve()});r.always(n.hideProgress)}}var s;n.submissionDetails=function(n,t,i,r,u,f,e,o,h,c,l,a,y,p,w,b){s=h;new v(n,t,i,r,u,f,e,o,c,l,a,y,p,w,b).bindTo("submissionForm")}}(window.app,window.OData,window.jQuery,window.setTimeout,window.FileReader!==undefined,new window.app.QuestionService,new window.app.RoleService),function(n,t,i,r,u,f,e){"use strict";function o(){var t=this;t.userId=n.autoMap();t.authorId=n.autoMap();t.email=n.autoMap();t.firstName=n.autoMap();t.lastName=n.autoMap();t.organization=n.autoMap();t.countryCode=n.autoMap();t.countryName=n.autoMap();t.isPrimary=n.autoMap()}function c(t){var i=this;i.email=ko.observable().extend({required:!0,email:!0,validation:{validator:function(n,t){for(var i=0;i<t.length;i++)if(t[i].email===n)return!1;return!0},message:"Author with the same email already exists.",params:t}});i.isEmailInvalid=ko.observable(!1);i.firstName=ko.observable().extend({required:{message:"First Name is required."},maxLength:200});i.lastName=ko.observable().extend({required:{message:"Last Name is required."},maxLength:200});i.organization=ko.observable().extend({required:{message:"Organization is required."},maxLength:200});i.availableCountries=ko.observable(n.countries.getCountries());i.countryCode=ko.observable().extend({required:{message:"Country is required."}});i.isSearching=ko.observable(!1);i.notFound=ko.observable(!1);i.cancelAdd=function(){i.email("");i.email.isModified(!1);i.firstName("");i.firstName.isModified(!1);i.lastName("");i.lastName.isModified(!1);i.organization("");i.organization.isModified(!1);i.countryCode(undefined);i.countryCode.isModified(!1);i.notFound(!1);i.isEmailInvalid(!1)}}function h(){var t=this;t.id=n.autoMap();t.originalName=n.autoMap();t.size=n.autoMap();t.formattedSize=n.autoMap();t.uploadDate=n.autoMap();t.downloadLink=n.autoMap()}function l(){var n=this}function a(r,a,v,y,p,w,b,k,d,g,nt){function rt(){function l(){var n=!0;return tt.files().length>tt.settings.cameraReadySubmissionMaxFileNumber&&(tt.showFilesMaxErrorMessage(!0),n=!1),tt.files().length<tt.settings.cameraReadySubmissionMinFileNumber&&(tt.showFilesMinErrorMessage(!0),n=!1),n}function a(){var r=tt.authors(),t,n,i;if(tt.isAuthorRole()&&tt.settings.editCameraReadyAuthorsNotAllowed&&!tt.settings.changeCameraReadyAuthorOrderAllowed)return!0;for(t=!1,n=0;n<r.length;n++)if(r[n].email===tt.primaryEmail()){t=!0;break}return i=!0,t||(tt.showPrimaryAuthorErrorMessage(!0),i=!1),i}function r(t){var o,r,f,u;if(tt.files().length+t.length>tt.settings.cameraReadySubmissionMaxFileNumber){n.addMessage("You can upload up to {0} files only.".format(tt.settings.cameraReadySubmissionMaxFileNumber),null,"error");return}for(o=[],r=0;r<tt.files().length;r++)o[tt.files()[r].originalName.toLowerCase()]=!0;for(r=0;r<t.length;r++)f=t[r],v(f,o)&&(tt.uploading(tt.uploading()+1),u=i.ajaxSettings.xhr(),u.open("POST",s.fileUpload,!0),u.setRequestHeader("Accept","application/json"),u.setRequestHeader("File-Name",encodeURIComponent(f.name)),u.send(f),u.addEventListener("load",function(t){t.target.status===200?e(t.target.responseText):n.processXmlHttpRequestError(t.target);tt.uploading(tt.uploading()-1)},!1))}function v(t,i){var u=t.name.toLowerCase(),r;if(i[u]===undefined)i[u]=!0;else return n.addMessage("Found at least two files with the same name: '{0}'.".format(t.name),null,"error"),!1;if(t.size>tt.settings.cameraReadySubmissionMaxFileSize*1048576)return n.addMessage("File '{0}' is bigger than maximum allowed size of {1} Mb.".format(t.name,tt.settings.cameraReadySubmissionMaxFileSize),null,"error"),!1;var f=t.name.substr(t.name.lastIndexOf(".")+1).toLowerCase(),e=tt.settings.cameraReadySubmissionAllowedFileTypes.split(","),o=!1;for(r=0;r<e.length;r++)if(e[r].trim().toLowerCase()===f){o=!0;break}return o?!0:(n.addMessage("File '{0}' has type '{1}' which is not accepted. We accept '{2}' only.".format(t.name,f,tt.settings.cameraReadySubmissionAllowedFileTypes),null,"error"),!1)}function e(t){var r,i;try{r=ko.utils.parseJson(t)}catch(u){n.processException(u);return}i=n.autoMap(new h,r);i.uploadDate=new Date(i.uploadDate);isNaN(i.uploadDate)&&(i.uploadDate=new Date);tt.files.push(i)}tt.title=ko.observable().extend({required:!0,maxLength:1e3}).autoMap();tt.abstract=ko.observable("").extend({required:{onlyIf:function(){return tt.settings.abstractAllowed&&tt.settings.abstractRequired}},maxLength:tt.settings.abstractMaxLength}).autoMap();tt.abstractCharsLeft=ko.computed(function(){return Math.max(tt.settings.abstractMaxLength-tt.abstract().length,0)});tt.submissionListUrl=null;tt.showPrimaryAuthorErrorMessage=ko.observable(!1);tt.showFilesMinErrorMessage=ko.observable(!1);tt.showFilesMaxErrorMessage=ko.observable(!1);tt.removeAuthor=function(n){tt.authors.remove(n)};tt.moveAuthorUp=function(n){var t=tt.authors.indexOf(n);tt.authors.remove(n);tt.authors.splice(t-1,0,n)};tt.moveAuthorDown=function(n){var t=tt.authors.indexOf(n);tt.authors.remove(n);tt.authors.splice(t+1,0,n)};tt.addAuthor=function(t){var r=ko.validation.group([t.email,t.firstName,t.lastName,t.organization,t.countryCode]),i;if(r().length>0){r.showAllMessages();t.isEmailInvalid(!t.email.isValid());return}i=n.autoMap(new o,{isPrimary:!1,email:t.email(),firstName:t.firstName(),lastName:t.lastName(),organization:t.organization(),countryCode:t.countryCode(),countryName:n.countries.getCountryNameByCode(t.countryCode())});tt.authors.push(i);tt.authors().length===1&&(tt.primaryEmail(i.email),tt.showPrimaryAuthorErrorMessage(!1));t.cancelAdd()};tt.newAuthor=new c(tt.authors);tt.searchAuthorByEmail=function(i){var r=ko.validation.group([i.email]),u;if(r().length>0){i.isEmailInvalid(!0);r.showAllMessages();return}i.isEmailInvalid(!1);i.isSearching(!0);u={requestUri:n.odata.getGlobalUrl(n.odata.entitySet.users,null,"SearchByEmail"),method:"POST",showProgressIndicator:!1,data:{Email:i.email()}};t.read(u,function(t){var r=n.autoMap(new o,t);r.userId=t.Id;tt.authors.push(r);tt.authors().length===1&&(tt.primaryEmail(r.email),tt.showPrimaryAuthorErrorMessage(!1));i.cancelAdd();i.isSearching(!1)},function(r){i.isSearching(!1);r.response.statusCode===n.enums.httpStatusCodes.failure.notFound?tt.newAuthor.notFound(!0):t.defaultError(r)})};tt.showValidationWarning=ko.observable(!1);tt.files=ko.observableArray();tt.removeFile=function(n){tt.files.remove(n)};tt.uploading=ko.observable(0);tt.uploadFile=function(){var n=i('<input type="file" accept="*" multiple="" />');n.on("change",function(){r(this.files)});n.trigger("click")};tt.canUploadMoreFiles=ko.computed(function(){return tt.uploading()===0&&tt.files().length<tt.settings.cameraReadySubmissionMaxFileNumber});tt.xhrUploadSupported=function(){return u};tt.fileUploadDragOver=function(n,t){tt.canUploadMoreFiles()&&i(t.target).addClass("dragOver")};tt.fileUploadDragLeave=function(n,t){tt.canUploadMoreFiles()&&i(t.target).removeClass("dragOver")};tt.fileUploadDrop=function(n,t){if(tt.canUploadMoreFiles()){var i=t.originalEvent.dataTransfer.files;r(i);tt.fileUploadDragLeave(n,t)}};tt.uploadSingleFile=function(n,t){t.target.value!==""&&t.target.form.submit()};tt.parseSingleUploadResult=function(n,t){e(t.target.contentDocument.body.innerText)};tt.submissionQuestions=[];tt.reproQuestions=[];tt.save=function(){function nt(i){var r=n.autoMap(i),u;return delete r.UserId,delete r.AuthorId,delete r.IsPrimary,u={requestUri:n.odata.getUrl(n.odata.entitySet.users,null,"AddCoAuthor"),method:"POST",data:{Request:r}},t.request(u,function(n){d[i.email]=n.value},function(i){if(i.response.statusCode==n.enums.httpStatusCodes.failure.conflict)n.addMessage(r,"Please click Cancel and use the email box to select author.","error");else if(i.response.statusCode==n.enums.httpStatusCodes.failure.badRequest){var r=n.getODataErrorMessage(i).message;n.addMessage(r,"Author information invalid:","error")}else t.defaultError(i)})}var e=!0,o=ko.validation.group(tt,{deep:!1}),y,p,w,b,h,k,u,c,d,g,r,v;for(o().length>0&&(o.showAllMessages(),e=!1),a()||(e=!1),l()||(e=!1),y=[],r=0;r<tt.submissionQuestions.length;r++)p=tt.submissionQuestions[r],it.isHidden(p.id)||y.push(p);for(o=ko.validation.group(y,{deep:!0}),o().length>0&&(o.showAllMessages(),e=!1),w=[],r=0;r<tt.reproQuestions.length;r++)for(b=tt.reproQuestions[r],h=0;h<b.choices.length;h++)w.push(b.choices[h]);if(k=ko.validation.group(w,{deep:!0}),k().length>0&&(k.showAllMessages(),e=!1),!e){tt.showValidationWarning(!0);return}for(u=n.autoMap(tt),u.Id=tt.id,u.Files=[],c=0;c<tt.files().length;c++)u.Files.push(tt.files()[c].id);if(u.Answers=f.getAnswersJson(tt.submissionQuestions.filter(n=>!it.isHidden(n.id))),u.ReproducibilityAnswers=f.getAnswersJson(tt.reproQuestions),d={},g=[],!tt.isAuthorRole()||!tt.settings.editCameraReadyAuthorsNotAllowed||tt.settings.changeCameraReadyAuthorOrderAllowed)for(r=0;r<tt.authors().length;r++)v=tt.authors()[r],v.userId||v.authorId||g.push(nt(v));i.when.apply(i,g).done(function(){var r,i,f,e;if(u.Authors=[],!tt.isAuthorRole()||!tt.settings.editCameraReadyAuthorsNotAllowed||tt.settings.changeCameraReadyAuthorOrderAllowed)for(r=0;r<tt.authors().length;r++)i=tt.authors()[r],i.userId||i.authorId||(i.authorId=d[i.email]),f={Order:r+1,IsPrimary:i.email===tt.primaryEmail(),UserId:i.userId,AuthorId:i.authorId,Email:i.email},u.Authors.push(f);e={requestUri:n.odata.getUrl(n.odata.entitySet.cameraReadySubmissions,tt.id),method:"PUT",headers:{Prefer:"return-content"},progressIndicatorTimeout:0,data:u};t.request(e,function(t){n.url.navigateTo(s.cameraReadySubmissionSummary.format(t.Id))})})}}function ut(t){return i.Deferred(function(){var e,r,u,i,o;if(n.autoMap(tt,t),ft(t.Authors),f.setAnswersFromJson(tt.submissionQuestions,t.Answers),e=[],t.ReproducibilityAnswers)for(r=0;r<t.ReproducibilityAnswers.length;r++)u=t.ReproducibilityAnswers[r],i=new l,i.QuestionId=u.QuestionId,i.QuestionChoiceId=u.QuestionChoiceId,o=JSON.parse(u.Text),i.Answer=o.Answer,i.Comment=o.Comment,e.push(i);f.setAnswersFromJson(tt.reproQuestions,e);n.url.hash.getValue()==="saved"&&(n.url.hash.remove(),n.addMessage("CameraReadySubmission '{0}' saved!".format(tt.title)))}).promise()}function ft(t){for(var r,u,f=[],i=0;i<t.length;i++)r=t[i],u=n.autoMap(new o,r),f.push(u),r.IsPrimary&&tt.primaryEmail(u.email);tt.authors(f)}function et(){return f.loadQuestionsDirect(n.enums.formType.cameraready,tt.submissionFormId).done(function(n){tt.submissionQuestions=n;it.loadQuestions(n)})}function ot(){return tt.trackSettings.requireRepro?f.loadQuestionsDirect(n.enums.formType.reproducibility,tt.reproFormId).done(function(n){var t,r,i;for(tt.reproQuestions=n,t=0;t<n.length;t++)for(r=n[t],i=0;i<r.choices.length;i++)r.choices[i].requireAnswer(!0)}):!0}function st(){e.getCurrentRoleDescriptor().done(function(t){tt.submissionListUrl=t.submissionListUrl;tt.isAuthorRole(tt.role===n.enums.userRole.author)})}function ht(i){if(i.length===0)return!0;var r=n.odata.getUrl(n.odata.entitySet.files,{filter:n.odata.buildContainsQuery("Id",i)});return t.read({requestUri:r,showProgressIndicator:!1},function(t){for(var r=[],i=0;i<t.value.length;i++)r.push(n.autoMap(new h,t.value[i]));tt.files(r)})}function ct(){return i.Deferred(function(i){t.read(n.odata.getUrl(n.odata.entitySet.cameraReadySubmissions,tt.id),function(n){i.resolve(n)})}).promise()}var tt=this,it=new n.QuestionDependency(tt);tt.id=r;tt.isPosted=n.autoMap();tt.trackName=v;tt.submissionFormId=y;tt.reproFormId=p;tt.isSingleTrackConference=w;tt.role=b;tt.fileIds=d;tt.trackId=a;tt.titleTitle="Title";tt.isAuthor=ko.observable(!1);tt.isAuthorRole=ko.observable(!1);tt.authors=ko.observableArray();tt.primaryEmail=ko.observable();tt.settings={welcomeMessage:n.autoMap(),cameraReadySubmissionMinFileNumber:n.autoMap(),cameraReadySubmissionMaxFileNumber:n.autoMap(),cameraReadySubmissionAllowedFileTypes:n.autoMap(),cameraReadySubmissionMaxFileSize:n.autoMap(),abstractAllowed:n.autoMap(),abstractMaxLength:n.autoMap(),abstractRequired:n.autoMap(),disableCoAuthors:n.autoMap(),disableTitleInstruction:n.autoMap(),titleMapping:n.autoMap(),showTipUnderFiles:n.autoMap(),editCameraReadyAuthorsNotAllowed:n.autoMap(),changeCameraReadyAuthorOrderAllowed:n.autoMap()};n.autoMap(tt.settings,g);tt.settings.titleMapping!==null&&(tt.titleTitle=tt.settings.titleMapping);tt.trackSettings=k;tt.currentProfile=n.autoMap(new o,nt);tt.currentProfile.userId=nt.Id;tt.isAuthor(!0);tt.hasBranchingQuestions=function(){return it.hasDependency()};tt.getQuestionDiv=function(n){return i("#sq_"+n)};tt.bindTo=function(t){n.showProgress();var r=i.Deferred();rt();i.when(ct(),et(),ot(),st(),ht(tt.fileIds)).done(function(n){ut(n);ko.applyBindingsAndShow(tt,t);it.init();r.resolve()});r.always(n.hideProgress)}}var s;n.cameraReadySubmissionDetails=function(n,t,i,r,u,f,e,o,h,c,l,v,y){s=o;new a(n,t,i,r,u,f,e,h,c,l,v).bindTo(y)}}(window.app,window.OData,window.jQuery,window.setTimeout,window.FileReader!==undefined,new window.app.QuestionService,new window.app.RoleService),function(n,t,i){function u(){var t=this;t.id=n.autoMap();t.originalName=n.autoMap();t.downloadLink=ko.pureComputed(function(){return"/api/{0}/Files/{1}".format(i.conference.name,t.id)})}function f(t,i){var r=this;r.id=n.autoMap();r.title=n.autoMap();r.abstract=n.autoMap();r.isPrimary=n.autoMap();r.isAbstractVisible=ko.observable(!1);r.toggleAbstract=function(){return r.isAbstractVisible(!r.isAbstractVisible()),!1};r.trackId=n.autoMap();r.trackName=n.autoMap();r.reviewCount=0;r.metaReviewCount=0;r.statusId=n.autoMap();r.statusName=n.autoMap();r.isCameraReady=n.autoMap();r.isCameraReadyPosted=n.autoMap();r.isAuthorFeedback=n.autoMap();r.isAuthorFeedbackPosted=n.autoMap();r.authorFeedbackId=n.autoMap();r.chairNoteId=n.autoMap();r.hasRevision=n.autoMap();r.originalSubmissionId=n.autoMap();r.cameraReadyLinkTitle=function(){return r.isCameraReadyPosted?"Edit Camera Ready Submission":"Create Camera Ready Submission"};r.viewUrl=function(){return t.submissionSummary.format(r.id)};r.viewRevisionUrl=function(){return r.originalSubmissionId&&t.submissionSummary.format(r.originalSubmissionId)};r.editUrl=function(){return t.submissionDetails.format(r.id)};r.editRevisionUrl=function(n){return t.submissionDetails.format(n)};r.editAuthorFeedbackLinkTitle=function(){return r.authorFeedbackId!==null?"Edit Author Feedback":"Post Author Feedback"};r.viewReviewsSnapshotTitle=function(){return"View Reviews"};r.viewMetaReviewsTitle=function(){return"View Meta-Reviews"};r.editAuthorFeedbackUrl=function(){return r.authorFeedbackId===null?t.authorFeedbackCreate.format(r.id):t.authorFeedbackDetails.format(r.authorFeedbackId)};r.viewAuthorFeedbackUrl=function(){return t.authorFeedbackSummary.format(r.authorFeedbackId)};r.editCameraReadyUrl=function(){return t.cameraReadySubmissionDetails.format(r.id)};r.viewCameraReadyUrl=function(){return t.cameraReadySubmissionSummary.format(r.id)};r.conflictUrl=function(){return t.submissionConflict.format(r.id)};r.viewReviewsUrl=function(){return t.submissionReviews.format(r.id)};r.viewMetaReviewsUrl=function(){return t.submissionMetaReviews.format(r.id)};r.viewChairNoteUrl=function(){return t.submissionChairNote.format(r.chairNoteId)};r.viewReviewsSnapshotUrl=function(){return i.disableReviewSnapshotDuringFeedback?r.viewReviewsUrl():t.submissionReviewsSnapshot.format(r.id)};r.crossTrackRevisionLinkVisible=function(){return r.statusId!==0&&i.allowAuthorNotification&&i.hasRevisionTracks&&!r.hasRevision&&i.statuses[r.statusId].isMajorRevision};r.reviewLinkVisible=function(){return i.reviewQuestionVisibleToAuthorCount>0&&r.statusId!==0&&(i.allowAuthorNotification&&i.statuses[r.statusId].reviewVisibleToAuthor||i.statuses[r.statusId].isDeskReject&&i.allowAuthorToSeeDeskRejectStatus||i.statuses[r.statusId].isWithdrawn&&i.allowAuthorToSeeReviewingDataForWithdrawn)};r.metaReviewLinkVisible=function(){return i.metaReviewQuestionVisibleToAuthorCount>0&&r.statusId!==0&&(i.allowAuthorNotification&&i.statuses[r.statusId].metaReviewVisibleToAuthor||i.statuses[r.statusId].isDeskReject&&i.allowAuthorToSeeDeskRejectStatus||i.statuses[r.statusId].isWithdrawn&&i.allowAuthorToSeeReviewingDataForWithdrawn)};r.chairNoteLinkVisible=function(){return r.chairNoteId&&i.chairNoteQuestionVisibleToAuthorCount>0&&r.statusId!==0&&(i.allowAuthorNotification||i.statuses[r.statusId].isDeskReject&&i.allowAuthorToSeeDeskRejectStatus||i.statuses[r.statusId].isWithdrawn&&i.allowAuthorToSeeReviewingDataForWithdrawn)};r.editLinkVisible=function(){return i.allowEditSubmission};r.deleteLinkVisible=function(){return(r.statusId===0||!i.statuses[r.statusId].isWithdrawn)&&(i.allowEditSubmission||i.allowAuthorToDeleteSubmisionAfterSubmissionDeadline)&&(!i.allowOnlyPrimaryContactAuthorToDeleteSubmision||r.isPrimary)};r.deleteLinkText=function(){return i.allowEditSubmission?"Delete Submission":i.allowAuthorToDeleteSubmisionAfterSubmissionDeadline?"Withdraw Submission":""};r.deleteConfirmTextFormat=function(){return i.allowEditSubmission?"You will not be able to revert this action. Are you sure you want to delete submission #{0}?":i.allowAuthorToDeleteSubmisionAfterSubmissionDeadline?"You will not be able to revert this action. Are you sure you want to withdraw submission #{0} ?":""};r.submitCopyrightFormUrlIsVisible=function(){return i.ecfRegistrationEnabled&&r.editCameraReadyLinkVisible()};r.editCameraReadyLinkVisible=function(){return i.allowCameraReadySubmission&&r.isCameraReady};r.editAuthorFeedbackLinkVisible=function(){return i.allowAuthorFeedback&&r.isAuthorFeedback};r.viewAuthorFeedbackLinkVisible=function(){return r.authorFeedbackId!==null};r.submitCopyrightFormUrl=function(){return t.copyrightForm.format(r.id)};r.uploadSupplementaryLinkVisible=function(){return i.allowSupplementaryMaterial};r.uploadSupplementaryUrl=function(){return t.supplementaryDetails.format(r.id)};r.uploadInplaceRevisionLinkVisible=function(){return r.statusId!==0&&i.allowAuthorNotification&&i.allowInplaceRevision&&i.statuses[r.statusId].isRevision};r.uploadInplaceRevisionUrl=function(){return t.inplaceRevisionDetails.format(r.id)};r.supplementaryLinkTitle=function(){return r.supplementaryFiles.length>0?"Edit Supplementary Material":"Upload Supplementary Material"};r.inplaceRevisionLinkTitle=function(){return r.revisionFiles.length>0?"Edit Revision":"Upload Revision"};r.crossTrackRevisionClick=function(){if(confirm('Have you completed revising paper {0}? Click "OK" only when you are ready to submit revision.'.format(r.id))){var t={requestUri:n.odata.getUrl(n.odata.entitySet.submissions,null,"RevisionAuthor"),method:"POST",data:{Request:r.id}};OData.request(t,function(t){n.addMessage("Created revision id={1} for submission id={0}.".format(r.id,t.value));window.location=r.editRevisionUrl(t.value)},function(n){OData.defaultError(n)})}};r.emailMetaReviewerLinkVisible=function(){return i.allowMetaReviewerToEmailAuthor};r.emailMetaReviewerUrl=function(){return t.emailMetaReviewer.format(r.id)};r.emailSeniorMetaReviewerLinkVisible=function(){return i.allowSeniorMetaReviewerToEmailAuthor};r.emailSeniorMetaReviewerUrl=function(){return t.emailSeniorMetaReviewer.format(r.id)};r.files=[];r.cameraReadyFiles=[];r.supplementaryFiles=[];r.revisionFiles=[];r.missingSubmissionFile=ko.pureComputed(function(){return r.files.length<i.submissionMinFileNumber});r.missingSupplementaryFile=ko.pureComputed(function(){return i.requireSupplementaryMaterial&&r.supplementaryFiles.length<i.supplementaryMinFileNumber})}function e(){var t=this;t.reviewVisibleToAuthor=n.autoMap();t.metaReviewVisibleToAuthor=n.autoMap();t.isRevision=n.autoMap();t.isMajorRevision=n.autoMap();t.isDeskReject=n.autoMap();t.isWithdrawn=n.autoMap()}function o(t){var i=this;i.id=n.autoMap();i.name=n.autoMap();i.createUrl=function(){return t.submissionCreate.format(i.id)};i.allowNewSubmission=n.autoMap();i.allowEditSubmission=n.autoMap();i.allowAuthorNotification=n.autoMap();i.allowMetaReviewerToEmailAuthor=n.autoMap();i.allowSeniorMetaReviewerToEmailAuthor=n.autoMap();i.allowAuthorToSeeDeskRejectStatus=n.autoMap();i.allowAuthorToSeeReviewingDataForWithdrawn=n.autoMap();i.editConflictAllowed=n.autoMap();i.allowCameraReadySubmission=n.autoMap();i.allowAuthorFeedback=n.autoMap();i.reviewQuestionVisibleToAuthorCount=n.autoMap();i.metaReviewQuestionVisibleToAuthorCount=n.autoMap();i.chairNoteQuestionVisibleToAuthorCount=n.autoMap();i.allowSupplementaryMaterial=n.autoMap();i.allowInplaceRevision=n.autoMap();i.hasRevisionTracks=n.autoMap();i.disableReviewSnapshotDuringFeedback=n.autoMap();i.allowAuthorToDeleteSubmisionAfterSubmissionDeadline=n.autoMap();i.allowOnlyPrimaryContactAuthorToDeleteSubmision=n.autoMap();i.ecfRegistrationEnabled=n.autoMap();i.submissionMinFileNumber=n.autoMap();i.supplementaryMinFileNumber=n.autoMap();i.requireSupplementaryMaterial=n.autoMap();i.statuses=[]}function r(i,r,u){function s(t,i){for(var u,r,s,h=0;h<i.length;h++){for(u=i[h],r=n.autoMap(new o(t),u),r.allowNewSubmission&&f.showCreateNewSubmission(!0),r.allowAuthorNotification&&f.reviewColumnVisible(!0),r.allowEditSubmission&&f.editSubmissionVisible(!0),r.allowCameraReadySubmission&&f.editCameraReadySubmissionVisible(!0),r.allowAuthorFeedback&&f.editAuthorFeedbackVisible(!0),(f.editSubmissionVisible()||r.allowAuthorToDeleteSubmisionAfterSubmissionDeadline||r.allowSupplementaryMaterial||f.editCameraReadySubmissionVisible()||f.editAuthorFeedbackVisible()||f.reviewColumnVisible())&&f.editColumnVisible(!0),s=0;s<u.StatusReviewVisibility.length;s++)r.statuses[u.StatusReviewVisibility[s].SubmissionStatusId]=n.autoMap(new e,u.StatusReviewVisibility[s]);f.tracks.push(r);f.tracksHash[r.id]=r}}var f=this;f.tracksHash={};f.tracks=[];f.pageUrls=i;f.authorConsoleCustomNotice=u&&u.AuthorConsoleCustomNotice;f.createNewSubmissionText=u&&u.CreateNewSubmissionText?u.CreateNewSubmissionText:"Create new submission";f.paperIDText=u&&u.PaperIDText?u.PaperIDText:"Paper ID";f.submissions=ko.observableArray([]);f.trackNamesProvider=ko.pureComputed(function(){var n=[];for(var t in f.tracks)f.tracks.hasOwnProperty(t)&&n.push(f.tracks[t].name);return n});f.showCreateNewSubmission=ko.observable(!1);f.editColumnVisible=ko.observable(!1);f.editSubmissionVisible=ko.observable(!1);f.editCameraReadySubmissionVisible=ko.observable(!1);f.reviewColumnVisible=ko.observable(!1);f.editAuthorFeedbackVisible=ko.observable(!1);f.authorFeedbackEntered=ko.observable(!1);f.editConflictAllowed=function(n){return f.tracksHash[n.trackId].editConflictAllowed};f.delete=function(i){if(confirm(i.deleteConfirmTextFormat().format(i.id))){var r,u=f.tracksHash[i.trackId];u.allowEditSubmission?(r={requestUri:n.odata.getUrl(n.odata.entitySet.submissions,i.id),method:"DELETE"},t.request(r,function(){f.submissions.remove(i)})):u.allowAuthorToDeleteSubmisionAfterSubmissionDeadline&&(r={requestUri:n.odata.getUrl(n.odata.entitySet.submissions,null,"Withdraw"),method:"POST",data:{Request:i.id}},t.request(r,function(n){n.value&&window.location.reload()},function(n){OData.defaultError(n)}))}};f.showWelcomeMessage=function(){$(document.getElementById("welcomeMessageDialog")).modal("show")};s(i,r);n.DataTable.call(f)}r.prototype=$.extend({},n.DataTable.prototype,{getDefaultSorting:function(){return{property:"Id",direction:"asc"}},getFilterString:function(){var t=this,n="";return $.each(t.filters,function(t,i){i.getValue()&&(n+=n?" and "+i.getValue():i.getValue())}),n},loadData:function(i){var r,s;i=i===!0;r=this;i&&r.applyState();var o=r.sorting(),h=o?"&$orderby="+encodeURIComponent(o.property+" "+o.direction):"",c=r.skip()?"&$skip="+r.skip():"",l=r.top()?"&$top="+r.top():"",e=r.getFilterString();return e&&(e="&$filter="+encodeURIComponent(e)),s={method:"GET",headers:{Accept:"application/json"},requestUri:n.odata.getUrl(n.odata.entitySet.submissionAuthorViews)+"?$count=true"+h+e+c+l,showProgressIndicator:!i},t.request(s,function(t){var v=t.value,a,l,e,c;for(r.total(t["@odata.count"]||0),a=[],l=0;l<v.length;l++){var o=v[l],y=o.TrackId,s=r.tracks&&r.tracksHash[y],i=n.autoMap(new f(r.pageUrls,s),o),h=o.SubmissionFilesJson&&JSON.parse(o.SubmissionFilesJson)||[];for(e=0;e<h.length;e++){if(c=n.autoMap(new u,h[e]),h[e].IsSubmissionFile){i.files.push(c);continue}if(h[e].IsSupplementaryFile){i.supplementaryFiles.push(c);continue}if(h[e].IsCameraReadyFile){i.cameraReadyFiles.push(c);continue}if(h[e].IsRevisionFile){i.revisionFiles.push(c);continue}}s&&i.statusId!==0&&s.statuses[i.statusId]&&(s.statuses[i.statusId].isDeskReject&&s.allowAuthorToSeeDeskRejectStatus||s.statuses[i.statusId].isWithdrawn)&&r.reviewColumnVisible(!0);i.authorFeedbackId&&r.authorFeedbackEntered(!0);i.reviewCount=o.NumberOfReviews;i.metaReviewCount=o.NumberOfMetaReviews;a.push(i)}r.submissions(a);r.saveState()},function(t){n.addErrorMessage(n.odata.getErrorMessage(t))}).done(function(){$("html,body").scrollTop(0)})}});n.authorSubmissionsPage=function(n,t,i,u){var f=new r(t,i,u);f.loadData().done(function(){ko.applyBindingsAndShow(f,n)})}}(window.app,window.OData,window.cmt3),function(n,t,i){"use strict";function f(){var t=this;t.id=n.autoMap();t.originalName=n.autoMap();t.size=n.autoMap();t.formattedSize=n.autoMap();t.uploadDate=n.autoMap();t.downloadLink=n.autoMap()}function r(){var t=this;t.order=n.autoMap();t.details=n.autoMap();t.answers=[]}function u(){var t=this;t.text=n.autoMap();t.value=n.autoMap()}function e(){var t=this;t.firstName=n.autoMap();t.lastName=n.autoMap();t.nickname=n.autoMap();t.name=n.autoMap();t.email=n.autoMap();t.organization=n.autoMap()}function o(){var t=this;t.ratingOptionName=n.autoMap();t.ratingOptionValue=n.autoMap()}function s(i,r){var u=this;u.id=n.autoMap();u.reviewerNumber=n.autoMap();u.reviewerName=n.autoMap();u.reviewerId=n.autoMap();u.externalReviewerName=n.autoMap();u.userType=n.autoMap();u.isSubmitted=n.autoMap();u.previousVersion=n.autoMap();u.ratingOptions=i;u.reviewRatingId=ko.observable(r);u.questions=[];u.files=[];u.ratings=[];u.deleteReview=function(){if(u.id&&u.reviewerName&&confirm("You will not be able to revert this action. Are you sure you want to delete review submitted by {0}?".format(u.reviewerName))){var i={requestUri:n.odata.getUrl(n.odata.entitySet.reviews,u.id),method:"DELETE"};t.request(i,function(){window.location.reload()},function(n){OData.defaultError(n)})}};u.reviewRatingId.subscribe(function(t){var i={requestUri:"/api/odata/"+window.cmt3.conference.name+"/ReviewRatings",method:"POST",headers:{Prefer:"return-content"},progressIndicatorTimeout:0,data:{ReviewId:u.id,ReviewRatingOptionId:t||null}};OData.request(i,function(){n.addMessage("Review rating saved")},function(){n.addMessage("Unable to save review rating",null,"error")})})}function h(t){var i=this;i.id=ko.observable();i.title=ko.observable();i.questions=ko.observableArray();i.reviewerNumber=ko.observableArray();i.reviewerName=ko.observableArray();i.previousVersion=ko.observableArray();i.newerVersion=ko.observableArray();i.updateDate=ko.observableArray();i.bind=function(){ko.applyBindings(i,t)};i.showPrevious=function(){i.previousVersion()&&i.loadQuestions(i.previousVersion())};i.showNewer=function(){i.newerVersion()&&i.loadQuestions(i.newerVersion())};i.loadQuestions=function(f){OData.read(n.odata.getUrl(n.odata.entitySet.reviewVersionViews,f),function(f){var h,o,c,e,s;if(i.questions([]),i.id(f.SubmissionId),i.title(f.SubmissionTitle),i.reviewerNumber(f.ReviewerNumber),i.reviewerName(f.ReviewerName),i.previousVersion(f.PreviousVersion),i.newerVersion(f.NewerVersion),i.updateDate(f.UpdateDate),f.Questions)for(e=0;e<f.Questions.length;e++){if(h=n.autoMap(new r,f.Questions[e]),o=f.Questions[e].Answers,o)for(s=0;s<o.length;s++)c=n.autoMap(new u,o[s]),h.answers.push(c);i.questions.push(h)}$(t).modal("show")})};i.editInDialog=function(n){i.loadQuestions(n.previousVersion)}}function c(c,l){function y(){return t.read(n.odata.getUrl(n.odata.entitySet.submissions,a.id,"Reviews"),function(t){for(var i,c,h,w,k,b,nt,tt,d,g,it,v,y=[],p=0;p<t.value.length;p++){for(i=t.value[p],p===0&&(a.trackName=i.TrackName,a.title=i.SubmissionTitle,a.isSingleTrackConference=i.IsSingleTrackConference),c=n.autoMap(new s(l,i.ReviewRatingId||undefined),i),h=0;h<i.Questions.length;h++){for(w=i.Questions[h],k=n.autoMap(new r,w),b=0;b<w.Answers.length;b++)k.answers.push(n.autoMap(new u,w.Answers[b]));c.questions.push(k)}for(h=0;h<i.Files.length;h++)nt=i.Files[h],tt=n.autoMap(new f,nt),c.files.push(tt);for(h=0;h<i.ReviewRatings.length;h++)d=i.ReviewRatings[h],g=n.autoMap(new o,d),g.user=n.autoMap(new e,d.User),c.ratings.push(g);c.reviewerNumber>0?a.reviews.push(c):y.push(c)}for(it=a.reviews.length===0?1:a.reviews[a.reviews.length-1].reviewerNumber+1,v=0;v<y.length;v++)y[v].reviewerNumber=it++,a.reviews.push(y[v])})}var a=this,v;a.id=c;a.trackName=null;a.title=null;a.isSingleTrackConference=null;a.reviews=[];a.print=function(){i()};v=null;a.reviewVersion=function(n){v===null&&(v=new h(document.getElementById("reviewVersionDialog")),v.bind());v.editInDialog(n)};a.bindTo=function(n){y().done(function(){ko.applyBindingsAndShow(a,n)})}}n.submissionReviews=function(n,t){new c(n,t).bindTo("submissionForm")}}(window.app,window.OData,window.print),function(n,t,i){"use strict";function r(){var t=this;t.order=n.autoMap();t.details=n.autoMap();t.answers=[]}function u(){var t=this;t.text=n.autoMap();t.value=n.autoMap()}function f(){var t=this;t.userNumber=n.autoMap();t.userName=n.autoMap();t.isSubmitted=n.autoMap();t.questions=[];t.files=[]}function e(e,o,s){function c(){return t.read(n.odata.getUrl(n.odata.entitySet.submissions,h.id,h.isMetaReviewer?h.isSenior?"SeniorMetaReviewerNotes":"MetaReviewerNotes":"ReviewerNotes"),function(t){for(var i,e,l,a,y,v,p,o,s=[],c=0;c<t.value.length;c++){for(i=t.value[c],c===0&&(h.trackName=i.TrackName,h.title=i.SubmissionTitle,h.isSingleTrackConference=i.IsSingleTrackConference),e=n.autoMap(new f,i),h.isSenior?(e.userName=i.SeniorMetaReviewerName,e.userNumber=i.SeniorMetaReviewerNumber):h.isMetaReviewer?(e.userName=i.MetaReviewerName,e.userNumber=i.MetaReviewerNumber):(e.userName=i.ReviewerName,e.userNumber=i.ReviewerNumber),l=0;l<i.Questions.length;l++){for(a=i.Questions[l],y=n.autoMap(new r,a),v=0;v<a.Answers.length;v++)y.answers.push(n.autoMap(new u,a.Answers[v]));e.questions.push(y)}e.userNumber>0?h.userNotes.push(e):s.push(e)}for(p=h.userNotes.length===0?1:h.userNotes[h.userNotes.length-1].userNumber+1,o=0;o<s.length;o++)s[o].userNumber=p++,h.userNotes.push(s[o])})}var h=this;h.isMetaReviewer=e;h.isSenior=o;h.id=s;h.trackName=null;h.title=null;h.isSingleTrackConference=null;h.userNotes=[];h.print=function(){i()};h.bindTo=function(n){c().done(function(){ko.applyBindingsAndShow(h,n)})}}n.submissionUserNotes=function(n,t,i){new e(n,t,i).bindTo("submissionForm")}}(window.app,window.OData,window.print),function(n,t,i){"use strict";function r(r){function f(){return t.read(n.odata.getUrl(n.odata.entitySet.submissions,u.id,"Reviews"),function(t){for(var s=[],r,h,o,i,f,c,l,a,v,y,e=0;e<t.value.length;e++){for(i=t.value[e],e===0&&(u.trackName=i.TrackName,u.title=i.SubmissionTitle,u.isSingleTrackConference=i.IsSingleTrackConference),f=n.autoMap(new n.Review,i),r=0;r<i.Questions.length;r++){for(c=i.Questions[r],l=n.autoMap(new n.Question,c),h=0;h<c.Answers.length;h++)l.answers.push(n.autoMap(new n.QuestionAnswer,c.Answers[h]));f.questions.push(l)}for(r=0;r<i.Files.length;r++)a=i.Files[r],v=n.autoMap(new n.File,a),f.files.push(v);f.reviewerNumber>0?u.reviews.push(f):s.push(f)}for(y=u.reviews.length===0?1:u.reviews[u.reviews.length-1].reviewerNumber+1,o=0;o<s.length;o++)s[o].reviewerNumber=y++,u.reviews.push(s[o])})}function e(){return t.read(n.odata.getUrl(n.odata.entitySet.submissions,u.id,"MetaReviews"),function(t){for(var s=[],r,h,o,i,f,c,l,a,v,y,e=0;e<t.value.length;e++){for(i=t.value[e],e===0&&(u.trackName=i.TrackName,u.title=i.SubmissionTitle,u.isSingleTrackConference=i.IsSingleTrackConference),f=n.autoMap(new n.MetaReview,i),r=0;r<i.Questions.length;r++){for(c=i.Questions[r],l=n.autoMap(new n.Question,c),h=0;h<c.Answers.length;h++)l.answers.push(n.autoMap(new n.QuestionAnswer,c.Answers[h]));f.questions.push(l)}for(r=0;r<i.Files.length;r++)a=i.Files[r],v=n.autoMap(new n.File,a),f.files.push(v);f.metaReviewerNumber>0?u.metaReviews.push(f):s.push(f)}for(y=u.metaReviews.length===0?1:u.metaReviews[u.metaReviews.length-1].metaReviewerNumber+1,o=0;o<s.length;o++)s[o].metaReviewerNumber=y++,u.metaReviews.push(s[o])})}function o(){return t.read(n.odata.getUrl(n.odata.entitySet.discussionMessages,{id:"{0}".format(n.odata.escapeParam(u.id)),orderby:"Date desc"}),function(t){for(var r,i=0;i<t.value.length;i++)r=t.value[i],u.messages.push(new n.MessageList(r))})}function s(){return $.Deferred(function(i){var r=n.odata.getUrl(n.odata.entitySet.authorFeedbackViews,null,"GetBySubmissionId");t.read({requestUri:r,showProgressIndicator:!1,data:{Id:u.id},method:"POST"},function(t){var r,f,o,e,s,h;for(u.feedbackId=t.Id,r=0;r<t.Questions.length;r++){for(f=t.Questions[r],o=n.autoMap(new n.Question,f),e=0;e<f.Answers.length;e++)o.answers.push(n.autoMap(new n.QuestionAnswer,f.Answers[e]));u.feedbackQuestions.push(o)}for(r=0;r<t.Files.length;r++)s=t.Files[r],h=n.autoMap(new n.File,s),u.feedbackFiles.push(h);i.resolve(!0)},function(n){n.response.statusCode===404?u.feedbackId=0:t.defaultError(n);i.resolve(!1)})}).promise()}var u=this;u.id=r;u.feedbackId=0;u.trackName=null;u.title=null;u.isSingleTrackConference=null;u.reviews=[];u.metaReviews=[];u.messages=[];u.feedbackQuestions=[];u.feedbackFiles=[];u.print=function(){i()};u.bindTo=function(n){$.when(f(),e(),o(),s()).done(function(){ko.applyBindingsAndShow(u,n)})}}n.submissionReviewingDetails=function(n){new r(n).bindTo("submissionForm")}}(window.app,window.OData,window.print),function(n,t,i){"use strict";function r(){var t=this;t.id=n.autoMap();t.originalName=n.autoMap();t.size=n.autoMap();t.formattedSize=n.autoMap();t.uploadDate=n.autoMap();t.downloadLink=n.autoMap()}function u(){var t=this;t.order=n.autoMap();t.details=n.autoMap();t.answers=[]}function f(){var t=this;t.text=n.autoMap();t.value=n.autoMap()}function e(){var t=this;t.reviewerNumber=n.autoMap();t.reviewerName=n.autoMap();t.userType=n.autoMap();t.questions=[];t.files=[]}function o(o){function h(){return t.read(n.odata.getUrl(n.odata.entitySet.reviewSnapshotAuthorViews,{filter:"SubmissionId eq {0}".format(n.odata.escapeParam(s.id)),orderby:"ReviewerNumber"}),function(t){for(var i,h,v,p,y,o,w,b,k,c,l=[],a=0;a<t.value.length;a++){for(i=t.value[a],a==0&&(s.trackName=i.TrackName,s.title=i.SubmissionTitle,s.isSingleTrackConference=i.IsSingleTrackConference),h=n.autoMap(new e,i),o=0;o<i.Questions.length;o++){for(v=i.Questions[o],p=n.autoMap(new u,v),y=0;y<v.Answers.length;y++)p.answers.push(n.autoMap(new f,v.Answers[y]));h.questions.push(p)}for(o=0;o<i.Files.length;o++)w=i.Files[o],b=n.autoMap(new r,w),h.files.push(b);h.reviewerNumber>0?s.reviews.push(h):l.push(h)}for(k=s.reviews.length==0?1:s.reviews[s.reviews.length-1].reviewerNumber+1,c=0;c<l.length;c++)l[c].reviewerNumber=k++,s.reviews.push(l[c])})}var s=this;s.id=o;s.trackName=null;s.title=null;s.isSingleTrackConference=null;s.reviews=[];s.print=function(){i()};s.bindTo=function(n){h().done(function(){ko.applyBindingsAndShow(s,n)})}}n.submissionReviewsSnapshot=function(n){new o(n).bindTo("submissionForm")}}(window.app,window.OData,window.print),function(n,t,i,r,u){"use strict";function c(){var t=this;t.email=n.autoMap();t.name=n.autoMap();t.id=n.autoMap()}function f(){var t=this;t.id=n.autoMap();t.name=n.autoMap();t.subject=n.autoMap();t.body=n.autoMap();t.createStub=function(n){return t.id=0,t.name=n,t.subject="",t.body="",t}}function l(r,u,f){function a(i,r){var u={SubmissionFilter:e,All:s,CheckNote:h,RecipientType:o,Skip:i,Top:r},f={requestUri:n.odata.getUrl(n.odata.entitySet.emails,null,"SubmissionGetRecipients"),method:"POST",data:{Request:u}};return t.request(f,function(t){for(var r=t.value,i=0;i<r.length;i++)l.recipients.push(n.autoMap(new c,r[i]));l.showAllVisible(l.recipientCount>l.recipients().length)})}var l=this;l.recipients=ko.observableArray();l.recipientCount=u;l.showAllVisible=ko.observable(!1);l.showInDialog=function(){i(r).modal("show")};l.showAll=function(){a(10,null)};l.removeRecipient=function(n){l.recipients.remove(n);l.recipientCount--;f.removeRecipient(n)};l.bind=function(){return a(0,10).done(function(){ko.applyBindings(l,r)})}}function a(n){var t=this,r=null;t.name=ko.observable().extend({required:!0});t.editInDialog=function(){return r=i.Deferred(),t.name(""),t.name.isModified(!1),i(n).modal("show"),r.promise()};t.bind=function(){ko.applyBindings(t,n)};t.saveTemplate=function(){var u=ko.validation.group(t);if(u().length>0){u.showAllMessages();return}r&&r.resolve(t.name());i(n).modal("hide")}}function v(u){var f=this,e=null,o;f.fromEmail=ko.observable().autoMap();f.fromName=ko.observable().autoMap();f.toEmail=ko.observable().autoMap();f.toName=ko.observable().autoMap();f.ccEmail=ko.observable().autoMap();f.recipientCount=ko.observable().autoMap();f.subject=ko.observable().autoMap();f.body=ko.observable("").autoMap();o=null;f.showInDialog=function(t,r){n.autoMap(f,t);o=r;i(u).modal("show")};f.sendEmails=function(){var f={requestUri:n.odata.getUrl(n.odata.entitySet.emails,null,"SubmissionSend"),method:"POST",data:{Request:o}};t.request(f,function(t){var f=t.value;i(u).modal("hide");e||(e=new n.EmailProgressViewModel(r.getElementById("showProgressDialog")),e.bind());e.showInDialog(f)})};f.bind=function(){ko.applyBindings(f,u)}}function y(c){function d(n,t){w||(w=new v(r.getElementById("previewEmailDialog")),w.bind());w.showInDialog(n,t)}function k(){var n=ko.validation.group(y);return n().length>0?(n.showAllMessages(),!1):!0}function g(){var i=n.autoMap(y),r;return i.SubmissionFilter=e,i.RecipientType=o,i.All=s,i.CheckNote=h,r={requestUri:n.odata.getUrl(n.odata.entitySet.emails,null,"SubmissionCountRecipients"),method:"POST",data:{Request:i}},t.request(r,function(n){y.recipientCount(n.value)})}function nt(){return t.read(n.odata.getUrl(n.odata.entitySet.emailTemplates,{orderby:"Name"}),function(t){y.templates.push((new f).createStub("Select predefined template…"));y.templates.push((new f).createStub("Create new…"));for(var i=0;i<t.value.length;i++)y.templates.push(n.autoMap(new f,t.value[i]))})}var y=this,w=null,b=null,p=null;y.from=c;y.ccEmail=ko.observable("").extend({email:!0,maxLength:200}).autoMap();y.ccSMR=ko.observable(!1).autoMap();y.recipientCount=ko.observable(0);y.templates=ko.observableArray();y.selectedTemplate=ko.observable();y.selectedTemplate.subscribe(function(n){y.subject(n.subject);y.subject.isModified(!1);y.body(n.body);y.body.isModified(!1)});y.subject=ko.observable("").extend({required:!0}).autoMap();y.body=ko.observable("").extend({required:!0}).autoMap();y.showPlaceholders=ko.observable(!1);y.showRecipients=function(){alert(y.recipients)};y.deleteRecipientIds=[];y.removeRecipient=function(n){y.deleteRecipientIds.push(n.id);y.recipientCount(y.recipientCount()-1)};y.previewEmail=function(){var i,r;k()&&(i=n.autoMap(y),i.SubmissionFilter=e,i.RecipientType=o,i.All=s,i.CheckNote=h,i.DeleteRecipientIds=y.deleteRecipientIds.join("/"),r={requestUri:n.odata.getUrl(n.odata.entitySet.emails,null,"SubmissionPreview"),method:"POST",data:{Request:i}},t.request(r,function(n){n.recipientCount=y.recipientCount();d(n,i)}))};y.saveTemplate=function(){var i,r;k()&&(i=n.autoMap(y),delete i.CcEmail,delete i.CcSMR,i.Name=y.selectedTemplate().name,r={requestUri:n.odata.getUrl(n.odata.entitySet.emailTemplates,y.selectedTemplate().id),method:"PUT",headers:{Prefer:"return-content"},data:i},t.request(r,function(t){y.selectedTemplate().subject=t.Subject;y.selectedTemplate().body=t.Body;n.addMessage("Template '{0}' saved.".format(y.selectedTemplate().name))}))};y.saveTemplateAs=function(){if(k()){var i=n.autoMap(y);delete i.CcEmail;delete i.CcSMR;b||(b=new a(r.getElementById("newTemplateNameDialog")),b.bind());b.editInDialog().done(function(r){i.Name=r;var u={requestUri:n.odata.getUrl(n.odata.entitySet.emailTemplates),method:"POST",headers:{Prefer:"return-content"},data:i};t.request(u,function(t){var i=n.autoMap(new f,t);y.templates.push(i);y.selectedTemplate(i);n.addMessage("Template '{0}' created.".format(r))})})}};y.removeTemplate=function(){if(y.selectedTemplate().id&&u("Are you sure you want to delete the template?")){var i={requestUri:n.odata.getUrl(n.odata.entitySet.emailTemplates,y.selectedTemplate().id),method:"DELETE"};t.request(i,function(){n.addMessage("Temmplate '{0}' removed.".format(y.selectedTemplate().name));y.templates.remove(y.selectedTemplate())})}};y.showRecipients=function(){p?p.showInDialog():(p=new l(r.getElementById("showRecipientsDialog"),y.recipientCount(),y),p.bind().done(function(){p.showInDialog()}))};y.bindTo=function(n){i.when(g(),nt()).done(function(){ko.applyBindingsAndShow(y,n)})}}var e=n.url===undefined?null:n.url.queryString.getValue("filter"),o=n.url===undefined?-1:parseInt(n.url.getUrlParts()[n.url.getUrlParts().length-1]),s=n.url===undefined?!0:n.url.queryString.getValue("all")==="true",h=n.url===undefined?!1:n.url.queryString.getValue("checkNote")==="true";n.submissionSendEmail=function(n){new y(n).bindTo("sendEmailForm")}}(window.app,window.OData,window.jQuery,window.document,window.confirm,window.setTimeout),function(n,t,i){"use strict";function f(){var t=this;t.firstName=ko.observable().autoMap();t.lastName=ko.observable().autoMap();t.organization=ko.observable().autoMap();t.email=n.autoMap();t.isPrimary=n.autoMap();t.authorId=n.autoMap();t.fullName=ko.pureComputed(function(){return t.firstName()+" "+t.lastName()})}function e(){var t=this;t.email=n.autoMap();t.firstName=n.autoMap();t.lastName=n.autoMap();t.organization=n.autoMap();t.fullName=ko.pureComputed(function(){return t.firstName+" "+t.lastName})}function o(t){var i=this;i.userId=n.autoMap();i.email=n.autoMap();i.firstName=n.autoMap();i.lastName=n.autoMap();i.isReferenceUploaded=n.autoMap();i.fullName=ko.pureComputed(function(){return i.firstName+" "+i.lastName});i.downloadLink=ko.pureComputed(function(){return"/api/{0}/ReferenceFile/{1}/{2}".format(window.cmt3.conference.name,t,i.userId)})}function s(){var t=this;t.fileId=n.autoMap();t.originalName=n.autoMap();t.size=n.autoMap();t.updated=n.autoMap();t.fileLabelId=n.autoMap();t.fileLabel=n.autoMap();t.formattedSize=ko.pureComputed(function(){return t.size.formatSize()});t.localeUploadDate=ko.pureComputed(function(){return new Date(t.updated).toLocaleString()});t.downloadLink=ko.pureComputed(function(){return"/api/{0}/Files/{1}".format(window.cmt3.conference.name,t.fileId)})}function r(){var t=this;t.id=n.autoMap();t.title=n.autoMap();t.heading=n.autoMap();t.answers=[];t.details=null}function u(){var t=this;t.answer=n.autoMap();t.customData=null;t.yesNo=ko.pureComputed(function(){return t.customData.Answer==="yes"?"Yes":t.customData.Answer==="no"?"No":"Not Applicable"});t.comment=ko.pureComputed(function(){return t.customData.Comment&&t.customData.Comment.htmlMultiLineEncode()})}function h(){var t=this;t.reason=n.autoMap()}function c(){var t=this;t.email=n.autoMap();t.firstName=n.autoMap();t.lastName=n.autoMap();t.reasons=[]}function l(l,a,v){function p(){var i={requestUri:n.odata.getUrl(n.odata.entitySet.submissionViews,y.id,"GetSummaryView"),headers:{"Content-Type":"application/json"},method:"POST"};return t.read(i,function(t){var i,l,v,p,a,w,b,d,g,nt,tt,it,k,rt,ut;if(t){if(n.autoMap(y,t),t.SubmissionFilesJson)for(w=JSON.parse(t.SubmissionFilesJson),i=0;i<w.length;i++){if(b=n.autoMap(new s,w[i]),w[i].IsSubmissionFile){y.files.push(b);continue}if(w[i].IsRevisionFile){y.revisionFiles.push(b);continue}if(w[i].IsSupplementaryFile){y.supplementaryFiles.push(b);continue}}if(t.SecondarySubjectAreasJson)for(d=JSON.parse(t.SecondarySubjectAreasJson),i=0;i<d.length;i++)y.secondarySubjectAreas.push(d[i].FullName);if(t.AuthorsJson)for(g=JSON.parse(t.AuthorsJson),i=0;i<g.length;i++)y.authors.push(n.autoMap(new f,g[i]));if(t.ConferenceRequestChairsJson)for(nt=JSON.parse(t.ConferenceRequestChairsJson),i=0;i<nt.length;i++)y.conferenceRequestChairs.push(n.autoMap(new e,nt[i]));if(t.ReferencesJson)for(tt=JSON.parse(t.ReferencesJson),i=0;i<tt.length;i++)y.references.push(n.autoMap(new o(y.id),tt[i]));if(t.QuestionAnswersJson)for(v=JSON.parse(t.QuestionAnswersJson),i=0;i<v.length;i++){if(p=n.autoMap(new r,v[i]),a=v[i].Answers,a)for(l=0;l<a.length;l++)p.answers.push(n.autoMap(new u,a[l]));p.details=y.submissionQuestionMap[p.id];y.submissionQuestions.push(p)}if(t.ReproducibilityQuestionAnswersJson)for(v=JSON.parse(t.ReproducibilityQuestionAnswersJson),i=0;i<v.length;i++){if(p=n.autoMap(new r,v[i]),a=v[i].Answers,a)for(l=0;l<a.length;l++)it=n.autoMap(new u,a[l]),it.customData=JSON.parse(a[l].Text),p.answers.push(it);y.reproQuestions.push(p)}if(t.ConflictsJson)for(k=JSON.parse(t.ConflictsJson),i=0;i<k.length;i++){for(rt=n.autoMap(new c,k[i]),ut=k[i].ConflictWithReason,l=0;l<ut.length;l++)rt.reasons.push(n.autoMap(new h,ut[l]));y.conflicts.push(rt)}}})}var y=this;y.id=l;y.submissionQuestionMap=a;y.acmConferenceAlias=v;y.conferenceName=n.autoMap();y.trackName=n.autoMap();y.title=n.autoMap();y.abstract=n.autoMap();y.primarySubjectArea=n.autoMap();y.created=n.autoMap();y.updated=n.autoMap();y.isSingleTrackConference=n.autoMap();y.submissionConflictDomainsRaw=n.autoMap();y.instructionAfterSubmission=n.autoMap();y.titleMapping=ko.observable(null).autoMap();y.idTitle=ko.computed(function(){var n=y.titleMapping();return n?"ID":"Paper ID"});y.titleTitle=ko.computed(function(){var n=y.titleMapping();return n?n:"Paper Title"});y.acmCallForParticipationUrl=function(){return v?"https://community.acm.org/"+v+"/demographics":""};y.authors=[];y.conferenceRequestChairs=[];y.references=[];y.secondarySubjectAreas=[];y.files=[];y.supplementaryFiles=[];y.revisionFiles=[];y.submissionQuestions=[];y.reproQuestions=[];y.conflicts=[];y.print=function(){i()};y.emailTo=ko.observable("currentUser");y.returnTrue=function(){return!0};y.sendEmail=function(){var i={EmailToCurrentUser:y.emailTo()==="currentUser"},r={requestUri:n.odata.getUrl(n.odata.entitySet.submissions,y.id,"SendEmail"),method:"POST",headers:{Prefer:"return-content"},data:i};t.request(r,function(t){if(t)for(var i=0;i<t.value.length;i++)n.addMessage("Error sending email to {0}.".format(t.value[i]),null,"error");else n.addMessage("Emails sent.")})};y.updateAuthor=function(i){var r={AuthorId:i.authorId,FirstName:i.firstName(),LastName:i.lastName(),Organization:i.organization()},u={requestUri:n.odata.getUrl(n.odata.entitySet.submissions,y.id,"ModifyAuthor"),method:"POST",headers:{Prefer:"return-content"},data:{Request:r}};t.request(u,function(){n.addMessage("Update successful.")},function(t){n.addErrorMessage("Unable to edit author."+n.odata.getErrorMessage(t))})};y.bindTo=function(n){p().done(function(){ko.applyBindingsAndShow(y,n)})}}n.submissionSummary=function(n,t,i){new l(n,t,i).bindTo("submissionForm")}}(window.app,window.OData,window.print,window.jQuery,new window.app.RoleService),function(n,t,i){"use strict";function f(){var t=this;t.email=n.autoMap();t.name=n.autoMap();t.isPrimary=n.autoMap()}function e(){var t=this;t.id=n.autoMap();t.originalName=n.autoMap();t.size=n.autoMap();t.formattedSize=n.autoMap();t.uploadDate=n.autoMap();t.downloadLink=n.autoMap()}function r(){var t=this;t.title=n.autoMap();t.heading=n.autoMap();t.answers=[]}function u(){var t=this;t.text=n.autoMap();t.value=n.autoMap();t.customData=null;t.yesNo=ko.pureComputed(function(){return t.customData.Answer==="yes"?"Yes":t.customData.Answer==="no"?"No":"Not Applicable"});t.comment=ko.pureComputed(function(){return t.customData.Comment&&t.customData.Comment.htmlMultiLineEncode()})}function o(o){function h(){return t.read(n.odata.getUrl(n.odata.entitySet.cameraReadySubmissionViews,s.id),function(t){var i,o,h,c,l;for(n.autoMap(s,t),i=0;i<t.Files.length;i++)s.files.push(n.autoMap(new e,t.Files[i]));for(i=0;i<t.Authors.length;i++)s.authors.push(n.autoMap(new f,t.Authors[i]));for(i=0;i<t.Questions.length;i++){for(h=t.Questions[i],c=n.autoMap(new r,h),o=0;o<h.Answers.length;o++)c.answers.push(n.autoMap(new u,h.Answers[o]));s.questions.push(c)}for(i=0;i<t.ReproducibilityQuestions.length;i++){for(h=t.ReproducibilityQuestions[i],c=n.autoMap(new r,h),o=0;o<h.Answers.length;o++)l=n.autoMap(new u,h.Answers[o]),l.customData=JSON.parse(h.Answers[o].CustomData),c.answers.push(l);s.reproQuestions.push(c)}})}var s=this;s.id=o;s.conferenceName=n.autoMap();s.trackName=n.autoMap();s.title=n.autoMap();s.abstract=n.autoMap();s.isSingleTrackConference=n.autoMap();s.isEditAllowed=n.autoMap();s.authors=[];s.files=[];s.questions=[];s.reproQuestions=[];s.print=function(){i()};s.returnTrue=function(){return!0};s.bindTo=function(n){h().done(function(){ko.applyBindingsAndShow(s,n)})}}n.cameraReadySubmissionSummary=function(n,t){new o(n).bindTo(t)}}(window.app,window.OData,window.print,window.jQuery,new window.app.RoleService),function(n,t,i,r,u){"use strict";function s(n){var t=this;t.email=n.Email;t.name=n.MiddleInitial==null||n.MiddleInitial==""?n.FirstName+" "+n.LastName:n.FirstName+" "+n.MiddleInitial+" "+n.LastName}function e(){var t=this;t.id=n.autoMap();t.name=n.autoMap();t.subject=n.autoMap();t.body=n.autoMap();t.createStub=function(n){return t.id=0,t.name=n,t.subject="",t.body="",t}}function h(r,u){function h(i,r){var u=n.odata.entitySet.userModels,h;return f==n.enums.inviteType.reviewer?u=n.odata.entitySet.manageInviteReviewers:f==n.enums.inviteType.metaReviewer?u=n.odata.entitySet.manageInviteMetaReviewers:f==n.enums.inviteType.seniorMetaReviewer&&(u=n.odata.entitySet.manageInviteSeniorMetaReviewers),h=n.odata.getUrl(u,{filter:o,skip:i,top:r}),t.read(h,function(n){for(var t,r={},i=0;i<n.value.length;i++)t=n.value[i],r[t.Email]||(r[t.Email]=!0,e.recipients.push(new s(t)));e.showAllVisible(e.recipientCount>e.recipients().length)})}var e=this;e.recipients=ko.observableArray();e.recipientCount=u;e.showAllVisible=ko.observable(!1);e.showInDialog=function(){i(r).modal("show")};e.showAll=function(){h(10,null)};e.bind=function(){return h(0,10).done(function(){ko.applyBindings(e,r)})}}function c(n){var t=this,r=null;t.name=ko.observable().extend({required:!0});t.editInDialog=function(){return r=i.Deferred(),t.name(""),t.name.isModified(!1),i(n).modal("show"),r.promise()};t.bind=function(){ko.applyBindings(t,n)};t.saveTemplate=function(){var u=ko.validation.group(t);if(u().length>0){u.showAllMessages();return}r&&r.resolve(t.name());i(n).modal("hide")}}function l(u){var f=this,e=null,o;f.fromEmail=ko.observable().autoMap();f.fromName=ko.observable().autoMap();f.toEmail=ko.observable().autoMap();f.toName=ko.observable().autoMap();f.recipientCount=ko.observable().autoMap();f.subject=ko.observable().autoMap();f.body=ko.observable("").autoMap();o=null;f.showInDialog=function(t,r){n.autoMap(f,t);o=r;i(u).modal("show")};f.sendEmails=function(){var f={requestUri:n.odata.getUrl(n.odata.entitySet.emails,null,"UserSend"),method:"POST",data:{Request:o}};t.request(f,function(t){var f=t.value;i(u).modal("hide");e||(e=new n.EmailProgressViewModel(r.getElementById("showProgressDialog")),e.bind());e.showInDialog(f)})};f.bind=function(){ko.applyBindings(f,u)}}function a(s){function b(n,t){y||(y=new l(r.getElementById("previewEmailDialog")),y.bind());y.showInDialog(n,t)}function w(){var n=ko.validation.group(a);return n().length>0?(n.showAllMessages(),!1):!0}function k(){var i=n.autoMap(a),r;return i.UserFilter=o,i.InviteType=f,r={requestUri:n.odata.getUrl(n.odata.entitySet.emails,null,"UserCountRecipients"),method:"POST",data:{Request:i}},t.request(r,function(n){a.recipientCount=n.value})}function d(){return t.read(n.odata.getUrl(n.odata.entitySet.emailTemplates,{orderby:"Name"}),function(t){a.templates.push((new e).createStub("Select predefined template…"));a.templates.push((new e).createStub("Create new…"));for(var i=0;i<t.value.length;i++)a.templates.push(n.autoMap(new e,t.value[i]))})}var a=this,y=null,p=null,v=null;a.from=s;a.recipientCount=0;a.templates=ko.observableArray();a.selectedTemplate=ko.observable();a.selectedTemplate.subscribe(function(n){a.subject(n.subject);a.subject.isModified(!1);a.body(n.body);a.body.isModified(!1)});a.subject=ko.observable("").extend({required:!0}).autoMap();a.body=ko.observable("").extend({required:!0}).autoMap();a.showPlaceholders=ko.observable(!1);a.showRecipients=function(){alert(a.recipients)};a.previewEmail=function(){var i,r;w()&&(i=n.autoMap(a),i.UserFilter=o,i.InviteType=f,r={requestUri:n.odata.getUrl(n.odata.entitySet.emails,null,"UserPreview"),method:"POST",data:{Request:i}},t.request(r,function(n){n.recipientCount=a.recipientCount;b(n,i)}))};a.saveTemplate=function(){var i,r;w()&&(i=n.autoMap(a),i.Name=a.selectedTemplate().name,r={requestUri:n.odata.getUrl(n.odata.entitySet.emailTemplates,a.selectedTemplate().id),method:"PUT",headers:{Prefer:"return-content"},data:i},t.request(r,function(t){a.selectedTemplate().subject=t.Subject;a.selectedTemplate().body=t.Body;n.addMessage("Template '{0}' saved.".format(a.selectedTemplate().name))}))};a.saveTemplateAs=function(){if(w()){var i=n.autoMap(a);p||(p=new c(r.getElementById("newTemplateNameDialog")),p.bind());p.editInDialog().done(function(r){i.Name=r;var u={requestUri:n.odata.getUrl(n.odata.entitySet.emailTemplates),method:"POST",headers:{Prefer:"return-content"},data:i};t.request(u,function(t){var i=n.autoMap(new e,t);a.templates.push(i);a.selectedTemplate(i);n.addMessage("Template '{0}' created.".format(r))})})}};a.removeTemplate=function(){if(a.selectedTemplate().id&&u("Are you sure you want to delete the template?")){var i={requestUri:n.odata.getUrl(n.odata.entitySet.emailTemplates,a.selectedTemplate().id),method:"DELETE"};t.request(i,function(){n.addMessage("Temmplate '{0}' removed.".format(a.selectedTemplate().name));a.templates.remove(a.selectedTemplate())})}};a.showRecipients=function(){v?v.showInDialog():(v=new h(r.getElementById("showRecipientsDialog"),a.recipientCount),v.bind().done(function(){v.showInDialog()}))};a.bindTo=function(n){i.when(k(),d()).done(function(){ko.applyBindingsAndShow(a,n)})}}var o=n.url==undefined?null:n.url.queryString.getValue("filter"),f=n.url==undefined?null:n.url.queryString.getValue("inviteType");n.userSendEmail=function(n,t){new a(n).bindTo(t)}}(window.app,window.OData,window.jQuery,window.document,window.confirm,window.setTimeout),function(n){"use strict";n.switchToLinkedUser=function(t){var i={requestUri:n.odata.getGlobalUrl(n.odata.entitySet.users,t,"SwitchToLinkedUser"),method:"POST"};OData.request(i,function(t){n.odata.processRedirectResponse(t)})};n.removeLinkedUser=function(t,i){if(confirm("Are you sure to remove linked account {0}?".format(i))){var r={requestUri:n.odata.getGlobalUrl(n.odata.entitySet.users,t,"RemoveLinkedUser"),method:"POST"};OData.request(r,function(){n.addMessage("Linked account removed.",null,"success","text",!0);window.location.reload()})}}}(window.app,window.document),function(n,t){"use strict";function i(i){var r=this;r.email=ko.observable("").extend({required:!0,email:!0}).autoMap();r.password=ko.observable("").extend({required:!0,minLength:6}).autoMap();r.loginInvalid=ko.observable(!1);r.showVerifyEmail=ko.observable(!1);r.error=ko.observable("");r.login=function(){var i;if(r.loginInvalid(!1),r.showVerifyEmail(!1),i=ko.validation.group(r),i().length>0)return i.showAllMessages(),!1;var f=n.autoMap(r),u=n.url.queryString.getValue("ReturnUrl"),e={requestUri:n.odata.getUrl(n.odata.entitySet.users,null,"Login")+(u?"?ReturnUrl="+encodeURIComponent(u):""),method:"POST",data:{Request:f}};return t.request(e,function(t){n.odata.processRedirectResponse(t)},function(i){if(i.response.statusCode==401||i.response.statusCode==403){r.loginInvalid(!0);var u=n.getODataErrorMessage(i);r.error(u.message);u.errorCode=="EmailNotVerified"&&r.showVerifyEmail(!0)}else t.defaultError(i)}),!1};r.bindTo=function(n){ko.applyBindingsAndShow(r,n);$(i).focus()}}n.userLogin=function(){new i(document.getElementById("emailTextbox")).bindTo("loginForm")}}(window.app,window.OData),function(n,t,i){"use strict";function u(){var u=this;u.email=ko.observable("").extend({required:!0,email:!0,validation:{async:!0,message:"Email is already being used.",validator:function(i,r,f){var e={requestUri:n.odata.getGlobalUrl(n.odata.entitySet.users,null,"IsFederationEmail"),method:"POST",showProgressIndicator:!1,data:{Email:i}};t.request(e,function(r){if(r.value)u.emailIsValidating(!1),f(!1);else{var e={requestUri:n.odata.getGlobalUrl(n.odata.entitySet.users,null,"CheckIfAccountExists"),method:"POST",showProgressIndicator:!1,data:{Email:i}};t.request(e,function(n){f(!n.value)},function(n){u.emailIsValidating(!1);t.defaultError(n)})}},function(n){u.emailIsValidating(!1);t.defaultError(n)})}}}).autoMap();u.email.isValidating.subscribe(function(n){u.emailIsValidating(n)});u.emailIsValidating=ko.observable(!1);u.password=ko.observable("").extend({required:!0,minLength:10}).autoMap();u.passwordHadFocus=ko.observable(!1);u.passwordHasFocus=ko.computed({read:function(){return u.passwordHadFocus()},write:function(n){n&&u.passwordHadFocus(!0)},owner:this});u.confirmPassword=ko.observable("").extend({required:!0,minLength:6,equal:{params:u.password,message:"Passwords must be equal."}});u.firstName=ko.observable("").extend({required:!0,maxLength:200}).autoMap();u.middleInitial=ko.observable("").extend({pattern:/^.*$/,maxLength:10}).autoMap();u.lastName=ko.observable("").extend({required:!0,maxLength:200}).autoMap();u.nickname=ko.observable("").extend({pattern:/^.*$/,maxLength:100}).autoMap();u.organization=ko.observable("").extend({required:!0,maxLength:200}).autoMap();u.phoneNumber=ko.observable("").extend({pattern:/^\+?(?:[0-9 \-]+|\([0-9]+\))+$/,maxLength:100}).autoMap();u.alternateEmail=ko.observable("").extend({email:!0,maxLength:200}).autoMap();u.agreementAccepted=ko.observable(!1).extend({equal:{params:!0,message:"You must accept agreement to continue."}}).autoMap();u.availableCountries=ko.observable(n.countries.getCountries());u.countryCode=ko.observable().extend({required:!0}).autoMap();u.googleScholarId=ko.observable("").extend({pattern:/^[-_0-9A-Za-z]{12}$/,maxLength:12}).autoMap();u.semanticScholarId=ko.observable("").extend({pattern:/^[1-9]\d*$/,maxLength:12}).autoMap();u.dblpId=ko.observable("").extend({pattern:/^\d{2,3}\/\d+(-\d+)?|[a-z]\/[a-zA-Z][0-9A-Za-z]*(-\d+)?$/,maxLength:50}).autoMap();u.captcha=new i.createViewModel;u.register=function(){var f=ko.validation.group(u),i,e;if(f().length>0){f.showAllMessages();return}i=n.autoMap(u);i.ValidateCaptchaRequest=u.captcha.getRequestModel();e={requestUri:n.odata.getUrl(n.odata.entitySet.users,{ReturnUrl:document.getElementById("returnUrl").value},"Register"),method:"POST",data:{Request:i}};t.request(e,function(){window.location=r},function(i){if(i.response.statusCode==403){var r=n.getODataErrorMessage(i).message;n.addMessage(r,"Registration failed:","error")}else t.defaultError(i);u.captcha.getNew(!1)})};u.bindTo=function(n){ko.applyBindingsAndShow(u,n);u.captcha.getNew(!1)}}var r;n.userRegister=function(n,t){r=n;(new u).bindTo(t)}}(window.app,window.OData,new window.app.CaptchaService),function(n,t,i){"use strict";function u(){var u=this;u.email=ko.observable("").extend({required:!0,email:!0,validation:{async:!0,message:"Invalid user account or you are trying to verify email for external user.",validator:function(i,r,f){var e={requestUri:n.odata.getGlobalUrl(n.odata.entitySet.users,null,"IsFederationEmail"),method:"POST",showProgressIndicator:!1,data:{Email:i}};t.request(e,function(r){if(r.value)u.emailIsValidating(!1),f(!1);else{var e={requestUri:n.odata.getGlobalUrl(n.odata.entitySet.users,null,"CheckIfAccountExists"),method:"POST",showProgressIndicator:!1,data:{Email:i}};t.request(e,function(n){n.value||u.emailIsValidating(!1);f(n.value)},function(){f(!1)})}},function(){f(!1)})}}}).autoMap();u.email.isValidating.subscribe(function(n){u.emailIsValidating(n)});u.emailIsValidating=ko.observable(!1);u.captcha=new i.createViewModel;u.verify=function(){var f=ko.validation.group(u),i,e;if(f().length>0){f.showAllMessages();return}i=n.autoMap(u);i.ValidateCaptchaRequest=u.captcha.getRequestModel();e={requestUri:n.odata.getUrl(n.odata.entitySet.users,{ReturnUrl:document.getElementById("returnUrl").value},"VerifyEmail"),method:"POST",data:{Request:i}};t.request(e,function(){window.location=r},function(i){if(i.response.statusCode==404){var r=n.getODataErrorMessage(i).message;n.addMessage(r,"Verify Email failed:","error")}else t.defaultError(i)}).always(function(){u.captcha.getNew(!1)})};u.bindTo=function(n){ko.applyBindingsAndShow(u,n);u.captcha.getNew(!1)}}var r;n.userVerify=function(n,t){r=n;(new u).bindTo(t)}}(window.app,window.OData,new window.app.CaptchaService),function(n,t,i){"use strict";function u(){var u=this;u.email=ko.observable("").extend({required:!0,email:!0,validation:{async:!0,message:"Invalid user account.",validator:function(i,r,f){var e={requestUri:n.odata.getGlobalUrl(n.odata.entitySet.users,null,"CheckIfAccountExists"),method:"POST",showProgressIndicator:!1,data:{Email:i}};t.request(e,function(n){n.value||u.emailIsValidating(!1);f(n.value)},function(){f(!1)})}}}).autoMap();u.email.isValidating.subscribe(function(n){u.emailIsValidating(n)});u.emailIsValidating=ko.observable(!1);u.captcha=new i.createViewModel;u.linkToAccount=function(){var f=ko.validation.group(u),i,e;if(f().length>0){f.showAllMessages();return}i=n.autoMap(u);i.ValidateCaptchaRequest=u.captcha.getRequestModel();e={requestUri:n.odata.getUrl(n.odata.entitySet.users,null,"RequestLinkToAccount"),method:"POST",data:{Request:i}};t.request(e,function(){window.location=r+"?linkto="+encodeURIComponent(u.email())},function(i){if(i.response.statusCode==404){var r=n.getODataErrorMessage(i).message;n.addMessage(r,"Link to Account failed:","error")}else t.defaultError(i)}).always(function(){u.captcha.getNew(!1)})};u.bindTo=function(n){ko.applyBindingsAndShow(u,n);u.captcha.getNew(!1)}}var r;n.linkToAccount=function(n,t){r=n;(new u).bindTo(t)}}(window.app,window.OData,new window.app.CaptchaService),function(n,t,i){"use strict";function r(r){var u=this;u.useCaptcha=r;r&&(u.captcha=new i.createViewModel);u.email=ko.observable("").extend({required:{params:!0,message:"Email is required."},email:!0,validation:{async:!0,message:"Invalid user account.",validator:function(i,r,f){var e={requestUri:n.odata.getGlobalUrl(n.odata.entitySet.users,null,"IsFederationEmail"),method:"POST",showProgressIndicator:!1,data:{Email:i}};t.request(e,function(r){if(r.value)u.emailIsValidating(!1),f(!1);else{var e={requestUri:n.odata.getGlobalUrl(n.odata.entitySet.users,null,"CheckIfAccountExists"),method:"POST",showProgressIndicator:!1,data:{Email:i}};t.request(e,function(n){n.value||u.emailIsValidating(!1);f(n.value)},function(){f(!1)})}},function(){f(!1)})}}}).autoMap();u.email.isValidating.subscribe(function(n){u.emailIsValidating(n)});u.emailIsValidating=ko.observable(!1);u.reset=function(){var r=ko.validation.group(u),i,f;if(r().length>0){r.showAllMessages();return}i=n.autoMap(u);u.useCaptcha&&(i.ValidateCaptchaRequest=u.captcha.getRequestModel());f={requestUri:n.odata.getUrl(n.odata.entitySet.users,null,"ResetPassword"),method:"POST",data:{Request:i}};t.request(f,function(){n.addMessage("Password has been reset and sent to you. Please check your email.")},function(i){if(i.response.statusCode===404){var r=n.getODataErrorMessage(i).message;n.addMessage(r,"Reset password failed:","error")}else t.defaultError(i);u.useCaptcha&&u.captcha.getNew(!1)})};u.bindTo=function(n){ko.applyBindingsAndShow(u,n);r&&u.captcha.getNew(!1)}}n.resetPassword=function(n,t){new r(n).bindTo(t)}}(window.app,window.OData,new window.app.CaptchaService),function(n,t,i){"use strict";function r(r){function f(){var t=[],i,n,r;if(u.publicationUrlsMultiLine())for(i=u.publicationUrlsMultiLine().split(/[\r\n]+/),n=0;n<i.length;n++)r=i[n].trim(),r&&t.push(r);return t.length>0?JSON.stringify(t):null}var u=this;u.firstName=ko.observable("").extend({required:!0,minLength:1,maxLength:200}).autoMap();u.middleInitial=ko.observable("").extend({maxLength:10}).autoMap();u.lastName=ko.observable("").extend({required:!0,minLength:1,maxLength:200}).autoMap();u.nickname=ko.observable("").extend({maxLength:200}).autoMap();u.organization=ko.observable("").extend({required:!0,minLength:1,maxLength:200}).autoMap();u.availableCountries=ko.observable(t.countries.getCountries());u.countryCode=ko.observable().extend({required:!0}).autoMap();u.googleScholarId=ko.observable("").extend({pattern:/^[-_0-9A-Za-z]{12}$/,maxLength:12}).autoMap();u.semanticScholarId=ko.observable("").extend({pattern:/^[1-9]\d*$/,maxLength:12}).autoMap();u.dblpId=ko.observable("").extend({pattern:/^\d{2,3}\/\d+(-\d+)?|[a-z]\/[a-zA-Z][0-9A-Za-z]*(-\d+)?$/,maxLength:50}).autoMap();u.publicationEmails=ko.observable("").extend({maxLength:1e3}).autoMap();u.publicationUrlsMultiLine=ko.observable("").extend({maxLength:4e3}).autoMap();u.doNotEmail=ko.observable(!1).autoMap();u.showPublicationUrlsErrorMessage=ko.observable(!1);u.showValidationWarning=ko.observable(!1);u.changeProfile=function(){var e=!0,o=ko.validation.group(u,{deep:!0}),s,h;if(o().length>0&&(o.showAllMessages(),e=!1),!e){u.showValidationWarning(!0);return}s={FirstName:u.firstName(),MiddleInitial:u.middleInitial(),LastName:u.lastName(),Nickname:u.nickname(),Organization:u.organization(),CountryCode:u.countryCode(),CountryName:t.countries.getCountryNameByCode(u.countryCode()),GoogleScholarId:u.googleScholarId(),SemanticScholarId:u.semanticScholarId(),DblpId:u.dblpId(),PublicationEmails:u.publicationEmails(),PublicationUrls:f(),DoNotEmail:u.doNotEmail()};h={requestUri:t.odata.getGlobalUrl(t.odata.entitySet.users,null,"ChangeProfile"),method:"POST",data:{Request:s}};i.request(h,function(){n(r).modal("hide");t.addMessage("Profile has been updated.")},function(n){if(n.response.statusCode==403||n.response.statusCode==400){var i=t.getODataErrorMessage(n).message;t.addMessage(i,"Update profile failed:","error")}else t.addMessage("Update profile failed.",null,"error")})};u.bind=function(){ko.applyBindings(u,r)};u.showDialog=function(t){if(u.showValidationWarning(!1),u.firstName(t.firstName),u.firstName.isModified(!1),u.middleInitial(t.middleInitial),u.lastName(t.lastName),u.lastName.isModified(!1),u.nickname(t.nickname),u.organization(t.organization),u.organization.isModified(!1),u.countryCode(t.countryCode),u.countryCode.isModified(!1),u.googleScholarId(t.googleScholarId),u.semanticScholarId(t.semanticScholarId),u.dblpId(t.dblpId),u.publicationEmails(t.publicationEmails),u.doNotEmail(t.doNotEmail),t.PublicationUrls){var i=JSON.parse(t.PublicationUrls);u.publicationUrlsMultiLine(i.join("\r\n"))}n(r).modal("show")}}function u(n){var t=this;t.email=n.Email;t.firstName=n.FirstName;t.lastName=n.LastName;t.organization=n.Organization;t.middleInitial=n.MiddleInitial;t.nickname=n.Nickname;t.countryCode=n.CountryCode;t.googleScholarId=n.GoogleScholarId;t.semanticScholarId=n.SemanticScholarId;t.dblpId=n.DblpId;t.publicationEmails=n.PublicationEmails;t.PublicationUrls=n.PublicationUrls;t.doNotEmail=n.DoNotEmail}t.userProfile=function(){function o(){return i.request({requestUri:t.odata.getUrl(t.odata.entitySet.users,null,"GetCurrentProfile"),method:"GET"},function(t){n.userProfile=new u(t)})}var n=this,f,e;n.options={elementId:"userProfile"};f=null;n.userProfile=null;n.changeProfile=function(){f==null&&(f=new r(document.getElementById("userProfileDialog"),n),f.bind());o().done(function(){f.showDialog(n.userProfile)})};e=document.getElementById(n.options.elementId);e&&ko.applyBindings(n,e)}}(window.jQuery,window.app,window.OData),function(n,t,i){"use strict";function r(r,u){var f=this;f.currentEmail=ko.observable("").extend({required:!0}).autoMap();f.newEmail=ko.observable("").extend({required:!0,email:!0,maxLength:200}).autoMap();f.confirmEmail=ko.observable("").extend({required:!0,equal:{params:f.newEmail,message:"Emails must be equal."}});f.showValidationWarning=ko.observable(!1);f.changeEmail=function(){var u=!0,e=ko.validation.group(f,{deep:!0}),o,s;if(e().length>0&&(e.showAllMessages(),u=!1),!u){f.showValidationWarning(!0);return}o={CurrentEmail:f.currentEmail(),NewEmail:f.newEmail()};s={requestUri:t.odata.getGlobalUrl(t.odata.entitySet.users,null,"ChangeEmail"),method:"POST",data:{Request:o}};i.request(s,function(){n(r).modal("hide");t.addMessage("Account email change request has been sent to your inbox for the new account email. Please check your email to complete the request.")},function(n){if(n.response.statusCode==403){var i=t.getODataErrorMessage(n).message;t.addMessage(i,"Change Email failed:","error")}else t.addMessage("Change Email failed.",null,"error")})};f.bind=function(){ko.applyBindings(f,r)};f.showDialog=function(){f.showValidationWarning(!1);f.currentEmail("");f.currentEmail.isModified(!1);f.newEmail("");f.newEmail.isModified(!1);f.confirmEmail("");f.confirmEmail.isModified(!1);n(r).modal("show");setTimeout(function(){n(u).focus()},600)}}t.userEmail=function(){var n=this,t,i;n.options={elementId:"userEmail"};t=null;n.changeEmail=function(){t==null&&(t=new r(document.getElementById("changeEmailDialog"),document.getElementById("changeEmailDialog-currentEmailTextbox"),n),t.bind());t.showDialog()};i=document.getElementById(n.options.elementId);i&&ko.applyBindings(n,i)}}(window.jQuery,window.app,window.OData),function(n){function i(i,r){var u=this;u.CurrentPage=t(1);u.TotalItemCount=i;u.PageSize=r;u.PageSlide=t(2);u.LastPage=n.computed(function(){if(u.PageSize()>0&&u.TotalItemCount()>0){var n=u.TotalItemCount()%u.PageSize(),t=(u.TotalItemCount()-n)/u.PageSize();return n>0&&t++,t}return 1});u.HasNextPage=n.computed(function(){return u.CurrentPage()<u.LastPage()});u.HasPrevPage=n.computed(function(){return u.CurrentPage()>1});u.FirstItemIndex=n.computed(function(){return u.TotalItemCount()==0?0:u.PageSize()*(u.CurrentPage()-1)+1});u.LastItemIndex=n.computed(function(){return u.TotalItemCount()==0?0:u.PageSize()>0?Math.min(u.FirstItemIndex()+u.PageSize()-1,u.TotalItemCount()):u.TotalItemCount()});u.ThisPageCount=n.computed(function(){var n=u.LastItemIndex()%u.PageSize();return n>0?n:u.PageSize()});u.Pages=n.computed(function(){var f=u.LastPage(),n=Math.max(1,u.CurrentPage()-u.PageSlide()),t=Math.min(f,u.CurrentPage()+u.PageSlide()),r,i;for(n=Math.max(1,Math.min(t-2*u.PageSlide(),n)),t=Math.min(f,Math.max(n+2*u.PageSlide(),t)),r=[],i=n;i<=t;i++)r.push(i);return r})}var t=function(t){var i=n.observable(t);return n.dependentObservable({read:function(){return i()},write:function(n){var t=parseFloat(n);i(isNaN(t)?n:t)}})};n.pager=function(t,r){var u=new i(t,r);return n.observable(u)}}(ko),function(n,t,i){"use strict";function u(t,i,r){function e(){o();f=u.isAssigned.subscribe(s)}function o(){f&&typeof f.dispose=="function"&&f.dispose()}function s(){u.initialState===undefined?u.initialState=u.isAssigned():h.call(u)}function h(){var i=this,f;i.isToggleInProgress(!0);f={UserId:t};f.Type=i.isAssigned()?"Assign":"Remove";OData.request({requestUri:n.odata.getUrl(n.odata.entitySet.submissions,i.id,i.isMeta?r?"SeniorMetaAssign":"MetaAssign":"Assign"),method:"POST",showProgressIndicator:!1,data:{Request:f}},function(){i.isAssigned()===i.initialState?u.css(""):u.css(i.isAssigned()?"success":"error")},function(t){o();u.isAssigned(!u.isAssigned());e();n.addErrorMessage("Unable to edit assignment for '"+i.title+"'. "+n.odata.getErrorMessage(t))}).always(function(){i.isToggleInProgress(!1)})}var u=this,f;u.isMeta=i;u.isSenior=r;u.id=n.autoMap();u.title=n.autoMap();u.trackName=n.autoMap();u.authors=n.autoMap();u.primarySubjectArea=n.autoMap();u.secondarySubjectAreas=n.autoMap();u.bid=n.autoMap();u.relevance=n.autoMap();u.tpmsRank=n.autoMap();u.assignmentsNumber=n.autoMap();u.isAssigned=ko.observable().autoMap();u.isSubmitted=ko.observable().autoMap();u.isSubmittedText=ko.pureComputed(function(){return u.isSubmitted()?"Yes":"No"});u.initialState=undefined;u.css=ko.observable("");u.isToggleInProgress=ko.observable(!1);e()}function r(t,i,r){var u=this;u.userId=t;u.isMeta=i;u.isSenior=r;u.showAssignedOnly=ko.observable("false");u.track=ko.observable();u.trackChangeSubscription=null;u.submissions=ko.observableArray([]);u.showAssignedOnly.subscribe(u.loadData,u);n.DataTable.call(u)}function f(t,i){var r=this;r.trackId=n.autoMap();r.trackName=n.autoMap();r.isTpmsEnabled=n.autoMap();r.quota=n.autoMap();r.primarySubjectAreas=n.autoMap();r.secondarySubjectAreas=n.autoMap();r.isSelected=ko.observable(i);r.selectTrack=function(){t.selectTrack(r)}}function e(i,r,u){var e=this;e.firstName=ko.observable().autoMap();e.lastName=ko.observable().autoMap();e.email=ko.observable().autoMap();e.organization=ko.observable().autoMap();e.tracks=ko.observableArray();e.selectedTrack=ko.observable(null);e.fullName=ko.pureComputed(function(){return e.firstName()+" "+e.lastName()});e.selectTrack=function(n){for(var t,u=n.trackId,r=e.tracks(),i=0;i<r.length;i++)t=r[i],t.trackId===u?(t.isSelected(!0),e.selectedTrack(n)):t.isSelected(!1)};e.loadData=function(){var o=n.odata.getUrl(r?u?n.odata.entitySet.seniorMetaReviewerBiddingViews:n.odata.entitySet.metaReviewerViews:n.odata.entitySet.reviewerViews,i,r?u?"GetSeniorMetaReviewerSimpleView":"GetMetaReviewerSimpleView":"GetReviewerSimpleView");return t.request({requestUri:o,showProgressIndicator:!1,method:"POST",headers:{"Content-Type":"application/json"}},function(t){var r,u,i;if(n.autoMap(e,t),r=[],t.TrackData){for(u=JSON.parse(t.TrackData),i=0;i<u.length;i++)r.push(n.autoMap(new f(e,i==0),u[i]));e.tracks(r);e.selectTrack(r[0])}})}}function o(t,u,f,o){var s=this;n.showProgress();s.user=new e(t,u,f);s.table=new r(t,u,f);ko.applyBindings(s,i.getElementById(o));$.when(s.user.loadData()).then(function(){return s.table.track(s.user.selectedTrack()),s.table.loadData(!0)}).then(function(){s.table.subscribeToTrackChange();s.user.selectedTrack.subscribe(function(n){s.table.track(n)});$("#"+o).show()}).always(n.hideProgress)}r.prototype=$.extend({},n.DataTable.prototype,{getDefaultSorting:function(){return{property:"IsAssigned",direction:"desc"}},subscribeToTrackChange:function(){var n=this;n.trackChangeSubscription||(n.trackChangeSubscription=n.track.subscribe(n.loadData,n))},loadData:function(i){var r,e,s;i=i===!0;r=this;i&&r.applyState();var o=r.sorting(),h=o?"&$orderby="+encodeURIComponent(o.property+" "+o.direction):"",c=r.skip()?"&$skip="+r.skip():"",l=r.top()?"&$top="+r.top():"",f="";return $.each(r.filters,function(n,t){t.getValue()&&(f+=f?" and "+t.getValue():t.getValue())}),r.showAssignedOnly()==="true"&&(f+=(f?" and":"")+" IsAssigned eq true"),e=r.track()&&r.track().trackId,typeof e=="number"&&e>0&&(f+=(f?" and":"")+" TrackId eq "+e),f&&(f="&$filter="+encodeURIComponent(f)),s={method:"GET",headers:{Accept:"application/json"},requestUri:n.odata.getUrl(r.isMeta?r.isSenior?n.odata.entitySet.seniorMetaReviewerSubmissionViews:n.odata.entitySet.metaReviewerSubmissionViews:n.odata.entitySet.reviewerSubmissionViews,r.userId)+"?$count=true"+f+h+c+l,showProgressIndicator:!i},t.request(s,function(t){var f,i,e,o;for(r.total(t["@odata.count"]||0),f=[],i=0;i<t.value.length;i++)e=t.value[i],o=n.autoMap(new u(r.userId,r.isMeta,r.isSenior),e),f.push(o);r.submissions(f);r.saveState()},function(t){n.addErrorMessage(n.odata.getErrorMessage(t))})}});n.reviewerAssignSubmissions=function(n,t,i,r){new o(n,t,i,r)}}(window.app,window.OData,window.document),function(n,t){"use strict";function i(t){var i=this;i.trackId=n.autoMap();i.trackName=n.autoMap();i.quota=ko.observable(t).extend({digit:!0,min:0,max:65536}).extend({trackChanges:!0})}function r(r,u,f){function o(){var r=f?n.odata.getUrl(n.odata.entitySet.reviewerViews,e.id,"GetReviewerSimpleView"):n.odata.getUrl(n.odata.entitySet.metaReviewerViews,e.id,"GetMetaReviewerSimpleView"),u={requestUri:r,method:"POST"};return t.request(u,function(t){var o=JSON.parse(t.TrackData),u,r,f;for(n.autoMap(e,t),u=[],r=0;r<o.length;r++)f=o[r],u.push(n.autoMap(new i(f.Quota),f));e.tracks(u)})}var e=this;e.singleTrackMode=u;e.id=r;e.email=n.autoMap();e.firstName=n.autoMap();e.lastName=n.autoMap();e.name=ko.pureComputed(function(){return e.firstName+" "+e.lastName});e.showValidationWarning=ko.observable(!1);e.tracks=ko.observableArray([]);e.save=function(){var o=!0,s=ko.validation.group(e,{deep:!0}),r,u,t,i,h;if(s().length>0&&(s.showAllMessages(),o=!1),!o){e.showValidationWarning(!0);return}for(r=[],u=e.tracks(),t=0;t<u.length;t++)i=u[t],i.quota.isChanged()&&r.push({TrackId:i.trackId,Quota:parseInt(i.quota()),ForReviewer:f});h={requestUri:n.odata.getUrl(n.odata.entitySet.users,e.id,"QuotaSettings"),method:"POST",headers:{Accept:"application/json"},data:{Request:{Quotas:r}}};OData.request(h,function(){n.addMessage("Quota successfully saved.")})};e.bindTo=function(n){o().done(function(){ko.applyBindingsAndShow(e,n)})}}n.reviewerTrackSettings=function(n,t,i,u){new r(n,t,i).bindTo(u)}}(window.app,window.OData),function(n,t,i){"use strict";function r(n){this.id=n.Id;this.sentOn=n.SentOn;this.emailStatus=n.EmailStatus;this.fromEmail=n.FromEmail;this.fromName=n.FromName;this.fromRole=n.FromRole;this.toEmail=n.ToEmail;this.toName=n.ToName;this.subject=n.Subject;this.body=n.Body;this.sentOnDateFormatted=function(){return t.formatUndefinableDateTime(this.sentOn)}}t.EmailMessagesPage=function(i,r){var u=this;u.$element=n(i);u.conference=window.cmt3.conference.name;u.page=ko.observable(1);u.top=ko.observable(25);u.sort=ko.observable("Id");u.controller=r;u.filters=[];u._total=ko.observable(0);u.selected=ko.observable(0);u.emailMessages=ko.observableArray();u.listen();u.Pager=ko.pager(u.selected,u.top);u.Pager().CurrentPage.subscribe(function(){u.page(u.Pager().CurrentPage());u.show()});u.roleNamesProvider=function(){var i=[],n=t.enums.userRole;for(var r in n)n.hasOwnProperty(r)&&i.push(n[r]);return i}};t.EmailMessagesPage.prototype={listen:function(){var t=this;n(document).on("data.filter",function(){t.Pager().CurrentPage()<2?t.show():t.Pager().CurrentPage(1)})},getFilter:function(){var t="";return n.each(this.filters,function(n,i){i.getValue()&&(t+=t==""?i.getValue():" and "+i.getValue())}),t},show:function(){var u=this;if(u.initialized){var f=u.sort(),e=u.top(),o=u.skip(),s=u.getFilter(),h=f?"&$orderby="+f:"",c=e?"&$top="+e:"",l=o?"&$skip="+o:"",a=s?"&$filter="+encodeURIComponent(s):"",v={headers:{Accept:"application/json"},requestUri:"/api/odata/"+this.conference+"/$batch",method:"POST",data:{requests:[{url:"/api/odata/"+this.conference+"/"+u.controller+"?$count=true"+h+a+l+c,method:"GET",headers:{Accept:"application/json"}}]}};i.request(v,function(i){t.page.saveState("emailmessages",{sort:f,top:e,skip:o,filter:s});var h=i.responses[0].body,c=h["@odata.count"],a=h.value,l=[];n.each(a,function(n,t){l.push(new r(t))});u.emailMessages(l);u._total()==0&&u._total(c);u.selected(c);n("html,body").scrollTop(0)},function(n){window.cmt3.logger.log(n.message)},i.batchHandler)}},scroll:function(){n(window).scrollTop()==n(document).height()-n(window).height()&&self.show()},reset:function(){n.each(this.filters,function(n,t){t.reset()});this.show()},size:function(t,i){var r,u,f;n("a",".show").removeClass("btn-success").css("color","#999999");n(i.currentTarget).addClass("btn-success").css("color","white");r=n(i.target).attr("size");u=parseInt(r);this.top(u);f=this.Pager().CurrentPage();this.Pager().CurrentPage(1);f===1&&this.show()},skip:function(){return(this.page()-1)*this.top()},prev:function(){this.top()!=0&&this.page()!=1&&(this.page(this.page()-1),this.show())},next:function(){this.top()==0||this.page()>this.selected()/this.top()||(this.page(this.page()+1),this.show())},setSort:function(t,i){var r=n(i.target),u=r.attr("data-sort");(u==null||u==undefined)&&(r=n(r.context.parentNode),u=r.attr("data-sort"));r.hasClass("selected")?this.sort().match(" desc$")?(this.sort(u+" asc"),r.find("i").removeClass("icon-arrow-down"),r.find("i").addClass("icon-arrow-up")):(this.sort(u+" desc"),r.find("i").removeClass("icon-arrow-up"),r.find("i").addClass("icon-arrow-down")):(n("th[data-sort]").each(function(){n(this).find("i").removeClass("icon-arrow-up");n(this).find("i").removeClass("icon-arrow-down");n(this).removeClass("selected")}),r.find("i").removeClass("icon-arrow-down"),r.find("i").addClass("icon-arrow-up"),r.addClass("selected"),this.sort(u+" asc"));this.show()},refresh:function(){this.show()}}}(window.jQuery,window.app,window.OData),function(n,t){"use strict";function i(i,r){function f(){return t.read(n.odata.getUrl(n.odata.entitySet.emailMessages,u.id),function(t){n.autoMap(u,t)})}var u=this;u.id=i;u.sentOn=n.autoMap();u.emailStatus=n.autoMap();u.fromEmail=n.autoMap();u.fromName=n.autoMap();u.toEmail=n.autoMap();u.toName=n.autoMap();u.subject=n.autoMap();u.body=n.autoMap();u.emailHistoryUrl=r;u.sentOnDateFormatted=function(){return n.formatUndefinableDateTime(u.sentOn)};u.bindTo=function(n){f().done(function(){ko.applyBindingsAndShow(u,n)})}}n.emailMessageSummary=function(n,t,r){new i(n,t).bindTo(r)}}(window.app,window.OData,window.print),function(n,t,i,r){"use strict";function u(n,t,i,r){return"{0} {1} {2} <{3}>".format(n,t==null?"":t,i,r)}function f(n){var t=this;t.name=u(n.firstName,n.middleInitial,n.lastName,n.email)}function e(n){function r(n,i){for(var o,u=0,e=0,r=0;r<t.users().length;r++)o=t.users()[r],u<n?u++:(i==null||e<i)&&(t.recipients.push(new f(o)),e++);t.showAllVisible(t.users().length>t.recipients().length)}var t=this;t.recipients=ko.observableArray();t.showAllVisible=ko.observable(!1);t.users=ko.observableArray();t.showInDialog=function(u){t.recipients.removeAll();t.users.removeAll();for(var f=0;f<u().length;f++)t.users.push(u()[f]);r(0,10);i(n).modal("show")};t.showAll=function(){r(10,null)};t.bind=function(){ko.applyBindings(t,n)}}function o(f,o){function h(n){s.previewFromEmail(n.FromEmail);s.previewFromName(n.FromName);s.previewToEmail(n.ToEmail);s.previewToName(n.ToName);s.previewSubject(n.Subject);s.previewBody(n.Body)}function c(){return t.request({requestUri:n.odata.getUrl(n.odata.entitySet.users,null,"GetCurrentProfile"),method:"GET"},function(n){s.from(n.Email);s.fromFirstName(n.FirstName);s.fromLastName(n.LastName)})}function l(){var i="Invite "+(s.inviteType===n.enums.inviteType.seniorMetaReviewer?"senior meta-reviewer":s.inviteType===n.enums.inviteType.metaReviewer?"meta-reviewer":"reviewer");return t.request({requestUri:n.odata.getUrl(n.odata.entitySet.emailTemplates,null,"GetByName"),data:{Name:i},method:"POST"},function(n){s.subject(n.Subject);s.body(n.Body);s.engineType=n.EngineType})}function a(){return t.read(n.odata.getUrl(n.odata.entitySet.tracks,{orderby:"Name"}),function(t){for(var r,u=[],f=n.cookies.getValue("trackId"),e=!1,i=0;i<t.value.length;i++)r=n.autoMap(new n.Track,t.value[i]),u.push(r),r.id==f&&(e=!0);s.tracks(u);s.selectedTrackId(e?f:s.tracks()[0].id);s.selectedTrackId.subscribe(function(t){n.cookies.setValue("trackId",t,0,"/")})})}var s=this;s.bulkInvite=f;s.inviteType=o;s.isFileUploaded=ko.observable(!1);s.users=ko.observableArray();s.normalUsers=ko.observableArray();s.hasError=ko.observable(!1);s.errorText=ko.observable();s.uploading=ko.observable(!1);s.previewFromEmail=ko.observable();s.previewFromName=ko.observable();s.previewToEmail=ko.observable();s.previewToName=ko.observable();s.previewSubject=ko.observable();s.previewBody=ko.observable("");s.selectedIndex=ko.observable(0);s.isPreviousEnabled=ko.pureComputed(function(){return this.bulkInvite&&this.selectedIndex()>0},s);s.isNextEnabled=ko.pureComputed(function(){return this.bulkInvite&&this.selectedIndex()+1<this.normalUsers().length},s);s.previousClick=function(){if(s.selectedIndex()>0){s.selectedIndex(s.selectedIndex()-1);var n=s.getPreviewRequest();t.request(n,function(n){h(n)})}};s.nextClick=function(){if(s.selectedIndex()+1<s.normalUsers().length){s.selectedIndex(s.selectedIndex()+1);var n=s.getPreviewRequest();t.request(n,function(n){h(n)})}};s.from=ko.observable(null);s.fromFirstName=ko.observable(null);s.fromMiddleInitial=ko.observable(null);s.fromLastName=ko.observable(null);s.fromFull=ko.pureComputed(function(){return u(this.fromFirstName(),this.fromMiddleInitial(),this.fromLastName(),this.from())},s);s.showRecipientsVm=null;s.to=ko.observable(null).extend({required:!0,email:!0,maxLength:200});s.toFirstName=ko.observable(null).extend({required:!0,maxLength:200});s.toMiddleInitial=ko.observable(null).extend({maxLength:10});s.toLastName=ko.observable(null).extend({required:!0,maxLength:200});s.toOrganization=ko.observable(null).extend({maxLength:200});s.userId=ko.observable(null);s.inviteeId=ko.observable(null);s.uploadFile=function(n,t){t.target.value!=""&&(s.uploading(!0),t.target.form.submit())};s.parseUploadResult=function(){var t=i.parseJSON(i("#singleFileUploadFrame").contents().text()),r,n,u;if(s.users.removeAll(),s.normalUsers.removeAll(),s.hasError(t.HasError),s.errorText(t.ErrorText),!s.hasError())for(r=0;r<t.Models.length;r++)n=t.Models[r],u={email:n.Email,firstName:n.FirstName,lastName:n.LastName,middleInitial:n.MiddleInitial,organization:n.Organization,notice:n.Note,hasError:n.HasError,rawData:n.RawData},s.users.push(u),u.hasError||s.normalUsers.push(u);s.isFileUploaded(!0);s.uploading(!1)};s.toFull=ko.computed(function(){return s.userId()==null&&s.inviteeId()==null?null:u(s.toFirstName(),s.toMiddleInitial(),s.toLastName(),s.to())});s.isSearching=ko.observable();s.searched=ko.observable(!1);s.userFound=ko.computed(function(){return(s.userId()!=null||s.inviteeId()!=null)&&s.searched()&&!s.to.isModified()});s.userNotFound=ko.computed(function(){return s.userId()==null&&s.inviteeId()==null&&s.searched()&&!s.to.isModified()});s.addUser=function(){var r=ko.validation.group([s.to,s.toFirstName,s.toLastName,s.toOrganization,s.toMiddleInitial]),i,u;if(r().length>0){r.showAllMessages();s.to.isModified(!1);return}return i={FirstName:s.toFirstName(),LastName:s.toLastName(),MiddleInitial:s.toMiddleInitial(),Organization:s.toOrganization(),Email:s.to()},delete i.MiddleInitial,u={requestUri:n.odata.getUrl(n.odata.entitySet.users,null,"AddInvitee"),method:"POST",data:{Request:i}},t.request(u,function(n){s.inviteeId(n.value)},function(i){if(i.response.statusCode==n.enums.httpStatusCodes.failure.conflict)n.addMessage(r,"Please enter user email in the email box to search again.","error");else if(i.response.statusCode==n.enums.httpStatusCodes.failure.badRequest){var r=n.getODataErrorMessage(i).message;n.addMessage(r,"User information invalid:","error")}else t.defaultError(i)})};s.search=function(){var t=ko.validation.group([s.to]),i;if(t().length>0){t.showAllMessages();return}s.isSearching(!0);i={requestUri:n.odata.getUrl(n.odata.entitySet.users,null,"SearchInviteeByEmail"),method:"POST",showProgressIndicator:!1,data:{Email:s.to()}};OData.read(i,function(n){s.userId(n.UserId);s.inviteeId(n.InviteeId);s.to(n.Email);s.toFirstName(n.FirstName);s.toMiddleInitial(n.MiddleInitial);s.toLastName(n.LastName);s.toOrganization(n.Organization);s.isSearching(!1);s.searched(!0);s.to.isModified(!1)},function(n){s.isSearching(!1);n.response.statusCode==404?(s.userId(null),s.inviteeId(null),s.toFirstName(null),s.toFirstName.isModified(!1),s.toMiddleInitial(null),s.toLastName(null),s.toLastName.isModified(!1),s.toOrganization(null),s.toOrganization.isModified(!1),s.searched(!0),s.to.isModified(!1)):OData.defaultError(n)})};s.tracks=ko.observableArray();s.selectedTrackId=ko.observable();s.subject=ko.observable("").extend({required:!0}).autoMap();s.body=ko.observable("").extend({required:!0}).autoMap();s.engineType=null;s.showPlaceholders=ko.observable(!1);s.getModel=function(){return{TrackId:s.selectedTrackId(),UserId:s.userId(),InviteeId:s.inviteeId(),SubjectTemplate:s.subject(),BodyTemplate:s.body(),EngineType:s.engineType,InviteType:s.inviteType}};s.getBulkPreviewModel=function(){var n=s.normalUsers()[s.selectedIndex()];return{UserFirstName:n.firstName,UserMiddleInitial:n.middleInitial,UserLastName:n.lastName,UserOrganization:n.firstName,UserEmail:n.email,TrackId:s.selectedTrackId(),SubjectTemplate:s.subject(),BodyTemplate:s.body(),EngineType:s.engineType,InviteType:s.inviteType}};s.getBulkModel=function(){for(var n,r,i=[],t=0;t<s.normalUsers().length;t++)n=s.normalUsers()[t],r={FirstName:n.firstName,MiddleInitial:n.middleInitial,LastName:n.lastName,Organization:n.organization,Email:n.email},i.push(r);return{Users:i,TrackId:s.selectedTrackId(),SubjectTemplate:s.subject(),BodyTemplate:s.body(),EngineType:s.engineType,InviteType:s.inviteType}};s.getPreviewRequest=function(){var t;return t=s.bulkInvite?s.getBulkPreviewModel():s.getModel(),{requestUri:n.odata.getUrl(n.odata.entitySet.users,null,s.bulkInvite?"InviteReviewersPreview":"InviteReviewerPreview"),method:"POST",data:{Request:t}}};s.previewInvite=function(n){s.selectedIndex(0);var i=s.getPreviewRequest();t.request(i,function(t){h(t);n()})};s.sendInvite=function(i){var r,u;r=s.bulkInvite?s.getBulkModel():s.getModel();u={requestUri:n.odata.getUrl(n.odata.entitySet.users,null,s.bulkInvite?"InviteReviewers":"InviteReviewer"),method:"POST",data:{Request:r}};t.request(u,function(){i()})};s.showRecipients=function(){s.showRecipientsVm==null&&(s.showRecipientsVm=new e(r.getElementById("showRecipientsDialog")),s.showRecipientsVm.bind());s.showRecipientsVm.showInDialog(s.normalUsers)};s.bindTo=function(n){i.when(c(),a(),l()).done(function(){ko.setupWizardSteps(s,5);s.fwdButtonTitles[2]="Preview";s.fwdButtonTitles[3]="Send";s.tracks().length<2&&s.steps[0].skip(!0);s.mayGoFwd=function(){return s.currentStep()!=1?!0:s.bulkInvite?s.isFileUploaded()&&s.normalUsers().length>0:(s.userId()!=null||s.inviteeId()!=null)&&!s.to.isModified()};s.mayGoBack=function(){return s.currentStep()!=4};s.beforeNextStepInvoked=function(n){return s.currentStep()==2?(s.previewInvite(n),!1):s.currentStep()==3?(s.sendInvite(n),!1):!0};s.startOver();ko.applyBindingsAndShow(s,n)})}}n.inviteReviewer=function(n,t,i){new o(n,t).bindTo(i)}}(window.app,window.OData,window.jQuery,window.document),function(n,t,i){"use strict";function r(n,t,i,r){return"{0} {1} {2} <{3}>".format(n,t===null?"":t,i,r)}function u(u){function e(n){f.previewFromEmail(n.FromEmail);f.previewFromName(n.FromName);f.previewToEmail(n.ToEmail);f.previewToName(n.ToName);f.previewSubject(n.Subject);f.previewBody(n.Body)}function o(){return t.request({requestUri:n.odata.getUrl(n.odata.entitySet.users,null,"GetCurrentProfile"),method:"GET"},function(n){f.from(n.Email);f.fromFirstName(n.FirstName);f.fromLastName(n.LastName)})}function s(){return t.request({requestUri:n.odata.getUrl(n.odata.entitySet.emailTemplates,null,"GetByName"),data:{Name:"Invite reviewer for submission"},method:"POST"},function(n){f.subject(n.Subject);f.body(n.Body);f.engineType=n.EngineType})}var f=this;f.submissionId=u;f.users=ko.observableArray();f.hasError=ko.observable(!1);f.errorText=ko.observable();f.previewFromEmail=ko.observable();f.previewFromName=ko.observable();f.previewToEmail=ko.observable();f.previewToName=ko.observable();f.previewSubject=ko.observable();f.previewBody=ko.observable("");f.selectedIndex=ko.observable(0);f.from=ko.observable(null);f.fromFirstName=ko.observable(null);f.fromMiddleInitial=ko.observable(null);f.fromLastName=ko.observable(null);f.fromFull=ko.pureComputed(function(){return r(this.fromFirstName(),this.fromMiddleInitial(),this.fromLastName(),this.from())},f);f.showRecipientsVm=null;f.to=ko.observable(null).extend({required:!0,email:!0,maxLength:200});f.toFirstName=ko.observable(null).extend({required:!0,maxLength:200});f.toMiddleInitial=ko.observable(null).extend({maxLength:10});f.toLastName=ko.observable(null).extend({required:!0,maxLength:200});f.toOrganization=ko.observable(null).extend({maxLength:200});f.userId=ko.observable(null);f.inviteeId=ko.observable(null);f.toFull=ko.computed(function(){return f.userId()==null&&f.inviteeId()==null?null:r(f.toFirstName(),f.toMiddleInitial(),f.toLastName(),f.to())});f.isSearching=ko.observable();f.searched=ko.observable(!1);f.userFound=ko.computed(function(){return(f.userId()!=null||f.inviteeId()!=null)&&f.searched()&&!f.to.isModified()});f.userNotFound=ko.computed(function(){return f.userId()==null&&f.inviteeId()==null&&f.searched()&&!f.to.isModified()});f.addUser=function(){var r=ko.validation.group([f.to,f.toFirstName,f.toLastName,f.toOrganization,f.toMiddleInitial]),i,u;if(r().length>0){r.showAllMessages();f.to.isModified(!1);return}return i={FirstName:f.toFirstName(),LastName:f.toLastName(),MiddleInitial:f.toMiddleInitial(),Organization:f.toOrganization(),Email:f.to()},delete i.MiddleInitial,u={requestUri:n.odata.getUrl(n.odata.entitySet.users,null,"AddInvitee"),method:"POST",data:{Request:i}},t.request(u,function(n){f.inviteeId(n.value)},function(i){if(i.response.statusCode==n.enums.httpStatusCodes.failure.conflict)n.addMessage(r,"Please enter user email in the email box to search again.","error");else if(i.response.statusCode==n.enums.httpStatusCodes.failure.badRequest){var r=n.getODataErrorMessage(i).message;n.addMessage(r,"User information invalid:","error")}else t.defaultError(i)})};f.search=function(){var t=ko.validation.group([f.to]),i;if(t().length>0){t.showAllMessages();return}f.isSearching(!0);i={requestUri:n.odata.getUrl(n.odata.entitySet.users,null,"SearchInviteeByEmail"),method:"POST",showProgressIndicator:!1,data:{Email:f.to()}};OData.read(i,function(n){f.userId(n.UserId);f.inviteeId(n.InviteeId);f.to(n.Email);f.toFirstName(n.FirstName);f.toMiddleInitial(n.MiddleInitial);f.toLastName(n.LastName);f.toOrganization(n.Organization);f.isSearching(!1);f.searched(!0);f.to.isModified(!1)},function(n){f.isSearching(!1);n.response.statusCode===404?(f.userId(null),f.inviteeId(null),f.toFirstName(null),f.toFirstName.isModified(!1),f.toMiddleInitial(null),f.toLastName(null),f.toLastName.isModified(!1),f.toOrganization(null),f.toOrganization.isModified(!1),f.searched(!0),f.to.isModified(!1)):OData.defaultError(n)})};f.subject=ko.observable("").extend({required:!0}).autoMap();f.body=ko.observable("").extend({required:!0}).autoMap();f.engineType=null;f.showPlaceholders=ko.observable(!1);f.getModel=function(){return{SubmissionId:f.submissionId,UserId:f.userId(),InviteeId:f.inviteeId(),SubjectTemplate:f.subject(),BodyTemplate:f.body(),EngineType:f.engineType}};f.getPreviewRequest=function(){var t=f.getModel();return{requestUri:n.odata.getUrl(n.odata.entitySet.users,null,"InviteReviewerForSubmissionPreview"),method:"POST",data:{Request:t}}};f.previewInvite=function(n){f.selectedIndex(0);var i=f.getPreviewRequest();t.request(i,function(t){e(t);n()})};f.sendInvite=function(i){var r=f.getModel(),u={requestUri:n.odata.getUrl(n.odata.entitySet.users,null,"InviteReviewerForSubmission"),method:"POST",data:{Request:r}};t.request(u,function(){i()})};f.bindTo=function(n){i.when(o(),s()).done(function(){ko.setupWizardSteps(f,4);f.fwdButtonTitles[1]="Preview";f.fwdButtonTitles[2]="Send";f.mayGoFwd=function(){return(f.userId()!=null||f.inviteeId()!=null)&&!f.to.isModified()};f.mayGoBack=function(){return f.currentStep()!==3};f.beforeNextStepInvoked=function(n){return f.currentStep()===1?(f.previewInvite(n),!1):f.currentStep()===2?(f.sendInvite(n),!1):!0};f.startOver();ko.applyBindingsAndShow(f,n)})}}n.inviteReviewerForSubmission=function(n,t){new u(n).bindTo(t)}}(window.app,window.OData,window.jQuery),function(n,t,i){"use strict";function r(r,u){function e(n){switch(n){case 1:return"Accept";case 2:return"Decline";default:return"Not responded"}}function o(){var t=i("#reviewerInvitationResponseConfirmationDialog"),n=i.Deferred();t.find(".btn-primary").off("click").click(function(){n.resolve(!0);n=null;t.modal("hide")});t.on("hidden",function(){n&&n.resolve(!1)});return t.modal("show"),n.promise()}function s(){return t.request({requestUri:n.odata.getUrl(n.odata.entitySet.manageReviewerInvites,null,"GetByUniqueId"),data:{UniqueId:r},method:"POST"},function(n){f.inviteType=n.InviteType;f.conferenceName=n.ConferenceName;f.trackName=n.TrackName;f.isSingleTrackConference(n.IsSingleTrackConference);f.isExpired(n.IsExpired);f.userNotRegistered(n.UserNotRegistered);f.comment(n.Comment);f.quota(n.Quota);switch(n.Status){case"Accepted":f.currentStatus(1);break;case"Declined":f.currentStatus(2);break;default:f.currentStatus(0)}})}var f=this;f.isExpired=ko.observable(!1);f.userNotRegistered=ko.observable(!1);f.currentStatus=ko.observable(0);f.newStatus=ko.observable(0);f.comment=ko.observable("");f.quota=ko.observable(null).extend({required:!1,digit:!0,min:1}).autoMap();f.quota.subscribe(function(n){n===""&&f.quota(null)});f.isSingleTrackConference=ko.observable(!1);f.conferenceName="";f.trackName="";f.commentMaxLength=256;f.commentCharsLeft=ko.computed(function(){return Math.max(f.commentMaxLength-f.comment().length,0)});f.inviteType=n.enums.inviteType.reviewer;f.isResponded=ko.computed(function(){return f.currentStatus()!==0});f.isAccepted=ko.computed(function(){return f.currentStatus()===1});f.isDeclined=ko.computed(function(){return f.currentStatus()===2});f.furtherStatus=ko.computed(function(){switch(f.currentStatus()){case 1:return 2;case 2:return 1;default:return 1}});f.currentStatusName=ko.computed(function(){return e(f.currentStatus())});f.newStatusName=ko.computed(function(){return e(f.newStatus())});f.furtherStatusName=ko.computed(function(){return e(f.furtherStatus())});f.changeStatusTo=function(u){var e=i.Deferred();return f.newStatus(u),o().done(function(i){if(!i){n.addMessage("NOTE: Response has not been changed.",null,"info");return}t.request({requestUri:n.odata.getUrl(n.odata.entitySet.manageReviewerInvites,null,"Respond"),data:{Request:{UniqueId:r,Accepted:u===1}},method:"POST"},function(){f.currentStatus(u);e.resolve()}).fail(function(){e.reject()})}),e.promise()};f.changeStatus=function(){var n=f.furtherStatus();f.changeStatusTo(n)};f.changeToDecline=function(){f.changeStatusTo(2)};f.submitOptional=function(){return t.request({requestUri:n.odata.getUrl(n.odata.entitySet.manageReviewerInvites,null,"UpdateFeedback"),data:{Request:{UniqueId:r,Quota:f.quota(),Comment:f.comment()}},method:"POST"},function(){n.addMessage("Feedback has been saved successfully.")})};f.bindTo=function(n){s().done(function(){ko.applyBindingsAndShow(f,n);f.isExpired()||f.userNotRegistered()||!u||f.currentStatus()===u||f.changeStatusTo(u)}).fail(function(){})}}n.invitation=function(n,t,i){new r(n,t).bindTo(i)}}(window.app,window.OData,window.jQuery),function(n,t,i){"use strict";function r(){var n=this;n.id=t.autoMap();n.name=t.autoMap()}function u(n,r){var u=this;u.convertStatus=function(n){switch(n){case"Accepted":return 1;case"Declined":return 2;default:return 0}};u.id=n.ReviewerInvitationId;u.userId=n.UserId;u.trackId=n.TrackId;u.created=n.Created;u.expiration=n.Expiration;u.firstName=n.FirstName;u.lastName=n.LastName;u.email=n.Email;u.organization=n.Organization;u.comment=n.Comment;u.track=n.TrackName;u.status=ko.observable(u.convertStatus(n.Status));u.statusName=n.Status;u.isReviewerLogical=ko.observable(n.IsInRole=="Yes");u.isReviewer=ko.computed(function(){return u.isReviewerLogical()?"Yes":"No"});u.showAddAsReviewer=u.status()==1&&!u.isReviewerLogical();u.expirationDateFormatted=function(){return t.formatUndefinableDateTime(u.expiration)};u.createdDateFormatted=function(){return t.formatUndefinableDateTime(u.created)};u.addAsReviewer=function(){return i.request({requestUri:t.odata.getUrl(t.odata.entitySet.manageInviteReviewers,null,r.inviteType===t.enums.inviteType.seniorMetaReviewer?"AddAsSeniorMetaReviewer":r.inviteType===t.enums.inviteType.metaReviewer?"AddAsMetaReviewer":"AddAsReviewer"),data:{Request:{TrackId:u.trackId,UserId:u.userId}},method:"POST"},function(){r.refresh()})};u.deleteInvite=function(){return i.request({requestUri:t.odata.getUrl(t.odata.entitySet.manageInviteReviewers,u.id),method:"DELETE"},function(){r.refresh()})}}t.ManageReviewerInvitationsPage=function(t,i,r,u){var f=this;f.inviteType=r;f.$element=n(t);f.conference=window.cmt3.conference.name;f.page=ko.observable(1);f.top=ko.observable(25);f.sort=ko.observable("Created desc");f.controller=i;f.filters=[];f._total=ko.observable(0);f.selected=ko.observable(0);f.inviteReviewers=ko.observableArray();f.listen();f.Pager=ko.pager(f.selected,f.top);f.Pager().CurrentPage.subscribe(function(){f.page(f.Pager().CurrentPage());f.show()});f.trackNamesProvider=function(){return u};f.statusNamesProvider=function(){return["Accepted","Declined","Not responded"]}};t.ManageReviewerInvitationsPage.prototype={listen:function(){var t=this;n(document).on("data.filter",function(){t.Pager().CurrentPage()<2?t.show():t.Pager().CurrentPage(1)})},getFilter:function(){var t="";return n.each(this.filters,function(n,i){i.getValue()&&(t+=t==""?i.getValue():" and "+i.getValue())}),t},show:function(){var t=this;if(t.initialized){var r="&$orderby="+this.sort(),f=this.top()!=0?"&$top="+this.top():"",e=this.skip()!=0?"&$skip="+this.skip():"",o=this.getFilter()!=""?"&$filter="+encodeURIComponent(this.getFilter()):"",s={headers:{Accept:"application/json"},requestUri:"/api/odata/"+this.conference+"/$batch",method:"POST",data:{requests:[{url:"/api/odata/"+this.conference+"/"+t.controller+"?$count=true"+r+o+e+f+"&caller=manageinvitereviewer",method:"GET",headers:{Accept:"application/json"}}]}};i.request(s,function(i){var r=i.responses[0].body,f=r["@odata.count"],o=r.value,e=[];n.each(o,function(n,i){e.push(new u(i,t))});t.inviteReviewers(e);t._total()==0&&t._total(f);t.selected(f);n("html,body").scrollTop(0)},function(n){window.cmt3.logger.log(n.message)},i.batchHandler)}},scroll:function(){n(window).scrollTop()==n(document).height()-n(window).height()&&self.show()},reset:function(){n.each(this.filters,function(n,t){t.reset()});this.show()},size:function(t,i){var r,u,f;n("a",".show").removeClass("btn-success").css("color","#999999");n(i.currentTarget).addClass("btn-success").css("color","white");r=n(i.target).attr("size");u=parseInt(r);this.top(u);f=this.Pager().CurrentPage();this.Pager().CurrentPage(1);f===1&&this.show()},skip:function(){return(this.page()-1)*this.top()},prev:function(){this.top()!=0&&this.page()!=1&&(this.page(this.page()-1),this.show())},next:function(){this.top()==0||this.page()>this.selected()/this.top()||(this.page(this.page()+1),this.show())},setSort:function(t,i){var r=n(i.target),u=r.attr("data-sort");(u==null||u==undefined)&&(r=n(r.context.parentNode),u=r.attr("data-sort"));r.hasClass("selected")?this.sort().match(" desc$")?(this.sort(u+" asc"),r.find("i").removeClass("icon-arrow-down"),r.find("i").addClass("icon-arrow-up")):(this.sort(u+" desc"),r.find("i").removeClass("icon-arrow-up"),r.find("i").addClass("icon-arrow-down")):(n("th[data-sort]").each(function(){n(this).find("i").removeClass("icon-arrow-up");n(this).find("i").removeClass("icon-arrow-down");n(this).removeClass("selected")}),r.find("i").removeClass("icon-arrow-down"),r.find("i").addClass("icon-arrow-up"),r.addClass("selected"),this.sort(u+" asc"));this.show()},refresh:function(){this.show()},selectStatus:function(t,i){var r=n(i.target),f=ko.contextFor(i.target),u=n(n("#statusTemplate").text());r.hide();r.after(u);f.$parent.getStatuses(t,r,u).done(function(n){ko.applyBindings(n,u[0])})},getEventFilter:function(n,t){var r=t.target,u=ko.contextFor(r),i=n.id;return i?"ReviewerInvitationId eq {0}".format(i):u.$root.getFilter()},email:function(n,i){var u=i.target,f=ko.contextFor(u),r=this.getEventFilter(n,i),e="/"+window.cmt3.conference.name+"/User/SendEmail";t.url.navigateTo(e,{filter:r.length>0?r:null,inviteType:f.$root.inviteType})},exportInvites:function(n,i){var r=i.target,u=ko.contextFor(r),f=this.getEventFilter(n,i),e=t.odata.getUrl("Users",null,"ExportUserInvites"),o={InviteType:u.$root.inviteType,Filter:f};t.page.post(e,o)},resendInvites:function(n,i){var s=i.target,r=ko.contextFor(s),f=n.id,u,e,o;u=f?"ReviewerInvitationId eq {0}".format(f):r.$root.getFilter();e=r.$root.inviteType===t.enums.inviteType.seniorMetaReviewer?"SeniorMetaResend":r.$root.inviteType===t.enums.inviteType.metaReviewer?"MetaResend":"Resend";o="/"+window.cmt3.conference.name+"/ReviewerInvite/"+e;t.url.navigateTo(o,{filter:u.length>0?u:null})},deleteInvites:function(n,r){var o,s;if(confirm("Bulk deletion will be performed for selected items.")){var h=r.target,u=ko.contextFor(h),f=n.id,e;return e=f?"ReviewerInvitationId eq {0}".format(f):u.$root.getFilter(),o={InvitesFilter:e,InviteType:u.$root.inviteType},s={requestUri:t.odata.getUrl(t.odata.entitySet.emails,null,"DeleteInvites"),method:"POST",data:{Request:o}},i.request(s,function(){t.addMessage("Bulk deletion has been completed successfully.");location.reload()})}},getStatuses:function(u,f,e){var o=n.Deferred();return i.read(t.odata.getUrl(t.odata.entitySet.inviteStatusModels),function(n){for(var v,s,c,l=[],a=[],h=0;h<n.value.length;h++)v=n.value[h],s=t.autoMap(new r,v),l.push(s),a[s.id]=s;c={options:ko.observableArray(l),selectedStatus:ko.observable()};c.selectedStatus.subscribe(function(n){var r=n[0],o={requestUri:t.odata.getUrl(t.odata.entitySet.manageReviewerInvites,null,"SetStatus"),method:"POST",showProgressIndicator:!0,data:{Request:{StatusId:r,ReviewerInvitationId:u.id}}};i.request(o,function(n){var i=n.value,t=a[r].name;e.remove();f.text(t);u.statusName=t;u.status(r);u.isReviewerLogical(i);f.show()})});o.resolve(c)}),o.promise()}}}(window.jQuery,window.app,window.OData),function(n,t){"use strict";function i(i){function u(){return t.request({requestUri:n.odata.getUrl(n.odata.entitySet.manageReviewerInvitesForSubmission,null,"GetByUniqueId"),data:{UniqueId:i},method:"POST"},function(n){r.conferenceName=n.ConferenceName;r.submissionId=n.SubmissionId;r.submissionTitle=n.SubmissionTitle;r.isExpired(n.IsExpired);r.userNotRegistered(n.UserNotRegistered);r.comment(n.Comment);switch(n.Status){case"Accepted":r.currentStatus(1);break;case"Declined":r.currentStatus(2);break;default:r.currentStatus(0)}})}var r=this;r.isExpired=ko.observable(!1);r.userNotRegistered=ko.observable(!1);r.currentStatus=ko.observable(0);r.conflictDomains=ko.observable("");r.comment=ko.observable("");r.conferenceName="";r.title="";r.commentMaxLength=512;r.commentCharsLeft=ko.computed(function(){return Math.max(r.commentMaxLength-r.comment().length,0)});r.isResponded=ko.computed(function(){return r.currentStatus()!==0});r.isDeclined=ko.computed(function(){return r.currentStatus()===2});r.getStatusName=function(n){switch(n){case 1:return"Accept";case 2:return"Decline";default:return"Not responded"}};r.currentStatusName=ko.computed(function(){return r.getStatusName(r.currentStatus())});r.decline=function(){return t.request({requestUri:n.odata.getUrl(n.odata.entitySet.manageReviewerInvitesForSubmission,null,"Decline"),data:{Request:{UniqueId:i}},method:"POST"},function(){r.currentStatus(2);r.conflictDomains("")})};r.accept=function(){return t.request({requestUri:n.odata.getUrl(n.odata.entitySet.manageReviewerInvitesForSubmission,null,"AcceptWithConflictsAndComment"),data:{Request:{UniqueId:i,DomainNames:r.conflictDomains(),Comment:r.comment()}},method:"POST"},function(){r.currentStatus(1);n.addMessage("Invite has been accepted.")},t.defaultError)};r.update=function(){return t.request({requestUri:n.odata.getUrl(n.odata.entitySet.manageReviewerInvitesForSubmission,null,"UpdateComment"),data:{Request:{UniqueId:i,Comment:r.comment()}},method:"POST"},function(){n.addMessage("Comment has been updated.")},t.defaultError)};r.bindTo=function(n){u().done(function(){ko.applyBindingsAndShow(r,n)}).fail(function(){})}}n.invitationForSubmission=function(n,t){new i(n).bindTo(t)}}(window.app,window.OData),function(n,t,i){"use strict";function r(n){var i=this;i.id=n.Id;i.submissionId=n.SubmissionId;i.title=n.Title;i.userId=n.UserId;i.trackId=n.TrackId;i.created=n.Created;i.expiration=n.Expiration;i.firstName=n.FirstName;i.lastName=n.LastName;i.email=n.Email;i.organization=n.Organization;i.comment=n.Comment;i.track=n.TrackName;i.status=n.Status;i.statusName=function(){return t.enums.inviteStatusOptionsSubstitutions[i.status]};i.expirationDateFormatted=function(){return t.formatUndefinableDateTime(i.expiration)};i.createdDateFormatted=function(){return t.formatUndefinableDateTime(i.created)}}t.ManageReviewerInvitationForSubmissionPage=function(t,i,r){var u=this;u.inviteType=r;u.$element=n(t);u.conference=window.cmt3.conference.name;u.page=ko.observable(1);u.top=ko.observable(25);u.sort=ko.observable("Created desc");u.controller=i;u.filters=[];u._total=ko.observable(0);u.selected=ko.observable(0);u.inviteReviewers=ko.observableArray();u.listen();u.Pager=ko.pager(u.selected,u.top);u.Pager().CurrentPage.subscribe(function(){u.page(u.Pager().CurrentPage());u.show()})};t.ManageReviewerInvitationForSubmissionPage.prototype={listen:function(){var t=this;n(document).on("data.filter",function(){t.Pager().CurrentPage()<2?t.show():t.Pager().CurrentPage(1)})},getFilter:function(){var t="";return n.each(this.filters,function(n,i){i.getValue()&&(t+=t===""?i.getValue():" and "+i.getValue())}),t},show:function(){var t=this;if(t.initialized){var u="&$orderby="+this.sort(),f=this.top()!==0?"&$top="+this.top():"",e=this.skip()!==0?"&$skip="+this.skip():"",o=this.getFilter()!==""?"&$filter="+encodeURIComponent(this.getFilter()):"",s={headers:{Accept:"application/json"},requestUri:"/api/odata/"+this.conference+"/$batch",method:"POST",data:{requests:[{url:"/api/odata/"+this.conference+"/"+t.controller+"?$count=true"+u+o+e+f+"&caller=manageinvitereviewerforsubmission",method:"GET",headers:{Accept:"application/json"}}]}};i.request(s,function(i){var u=i.responses[0].body,f=u["@odata.count"],o=u.value,e=[];n.each(o,function(n,i){e.push(new r(i,t))});t.inviteReviewers(e);t._total()===0&&t._total(f);t.selected(f);n("html,body").scrollTop(0)},function(n){window.cmt3.logger.log(n.message)},i.batchHandler)}},scroll:function(){n(window).scrollTop()===n(document).height()-n(window).height()&&self.show()},reset:function(){n.each(this.filters,function(n,t){t.reset()});this.show()},size:function(t,i){var r,u,f;n("a",".show").removeClass("btn-success").css("color","#999999");n(i.currentTarget).addClass("btn-success").css("color","white");r=n(i.target).attr("size");u=parseInt(r);this.top(u);f=this.Pager().CurrentPage();this.Pager().CurrentPage(1);f===1&&this.show()},skip:function(){return(this.page()-1)*this.top()},prev:function(){this.top()!==0&&this.page()!==1&&(this.page(this.page()-1),this.show())},next:function(){this.top()===0||this.page()>this.selected()/this.top()||(this.page(this.page()+1),this.show())},setSort:function(t,i){var r=n(i.target),u=r.attr("data-sort");(u===null||u===undefined)&&(r=n(r.context.parentNode),u=r.attr("data-sort"));r.hasClass("selected")?this.sort().match(" desc$")?(this.sort(u+" asc"),r.find("i").removeClass("icon-arrow-down"),r.find("i").addClass("icon-arrow-up")):(this.sort(u+" desc"),r.find("i").removeClass("icon-arrow-up"),r.find("i").addClass("icon-arrow-down")):(n("th[data-sort]").each(function(){n(this).find("i").removeClass("icon-arrow-up");n(this).find("i").removeClass("icon-arrow-down");n(this).removeClass("selected")}),r.find("i").removeClass("icon-arrow-down"),r.find("i").addClass("icon-arrow-up"),r.addClass("selected"),this.sort(u+" asc"));this.show()},refresh:function(){this.show()}}}(window.jQuery,window.app,window.OData),function(n,t,i,r,u){"use strict";function f(){var t=this;t.id=n.autoMap();t.name=n.autoMap();t.subject=n.autoMap();t.body=n.autoMap();t.createStub=function(n,i){return t.id=i,t.name=n,t.subject="",t.body="",t}}function e(r){function s(){var n=ko.validation.group(e);return n().length>0?(n.showAllMessages(),!1):!0}function h(){return t.read(n.odata.getUrl(n.odata.entitySet.emailTemplates,{orderby:"Name"}),function(t){e.selectedTemplate(e.templates()[0]);e.templates.splice(2,e.templates().length-2);for(var i=0;i<t.value.length;i++)e.templates.push(n.autoMap(new f,t.value[i]))})}var e=this,o=null;e.templates=ko.observableArray();e.templates.push((new f).createStub("Select predefined template…",-1));e.templates.push((new f).createStub("Create new…",0));e.selectedTemplate=ko.observable(e.templates()[0]);e.selectedTemplate.subscribe(function(n){n.id==0?e.name(""):(e.name(n.name),e.subject(n.subject),e.subject.isModified(!1),e.body(n.body),e.body.isModified(!1));e.name.isModified(!1)});e.subject=ko.observable("").extend({required:!0}).autoMap();e.body=ko.observable("").extend({required:!0}).autoMap();e.showPlaceholders=ko.observable(!1);e.name=ko.observable().extend({required:!0});e.close=function(){o&&o.resolve()};e.editInDialog=function(){return o=i.Deferred(),h().done(function(){i(r).modal("show");i(r).on("hidden",e.close)}),o.promise()};e.saveTemplate=function(){var i,r;s()&&(i=n.autoMap(e),i.Name=e.name(),e.selectedTemplate().id==0?(r={requestUri:n.odata.getUrl(n.odata.entitySet.emailTemplates),method:"POST",headers:{Prefer:"return-content"},data:i},t.request(r,function(t){var i=n.autoMap(new f,t);e.templates.push(i);e.selectedTemplate(i);n.addMessage("Template '{0}' created.".format(e.name()))})):(r={requestUri:n.odata.getUrl(n.odata.entitySet.emailTemplates,e.selectedTemplate().id),method:"PUT",headers:{Prefer:"return-content"},data:i},t.request(r,function(t){e.selectedTemplate().subject=t.Subject;e.selectedTemplate().body=t.Body;n.addMessage("Template '{0}' saved.".format(e.name()))})))};e.removeTemplate=function(){if(e.selectedTemplate().id&&u("Are you sure you want to delete the template?")){var i={requestUri:n.odata.getUrl(n.odata.entitySet.emailTemplates,e.selectedTemplate().id),method:"DELETE"};t.request(i,function(){n.addMessage("Temmplate '{0}' removed.".format(e.selectedTemplate().name));e.templates.remove(e.selectedTemplate())})}};e.bind=function(){ko.applyBindings(e,r)}}function o(){var n=this;n.previewFromName=ko.observable("");n.previewToName=ko.observable("");n.previewFromEmail=ko.observable("");n.previewToEmail=ko.observable("");n.previewSubject=ko.observable("");n.previewBody=ko.observable("");n.selectedEmailIndex=ko.observable(0);n.selectedSubmissionIndex=ko.observable(0);n.selectedIndex=ko.observable(0)}function s(n,t){var i=this,r;for(i.status=t,i.emailAllAuthors=[],r=0;r<n.EmailAllAuthors.length;r++)i.emailAllAuthors.push(n.EmailAllAuthors[r]);for(i.emailPrimaryContactOnly=[],r=0;r<n.EmailPrimaryContactOnly.length;r++)i.emailPrimaryContactOnly.push(n.EmailPrimaryContactOnly[r]);i.id=n.Id;i.email=ko.computed(function(){return i.status.track.root.emailingType()=="allAuthors"?i.emailAllAuthors:i.emailPrimaryContactOnly});i.emailCount=ko.computed(function(){return i.email().length})}function h(i,r){var u=this,f;for(u.track=r,u.submissions=ko.observableArray(),f=0;f<i.SubmissionSummaries.length;f++)u.submissions.push(new s(i.SubmissionSummaries[f],u));u.submissionCount=ko.computed(function(){return u.submissions().length});u.emailCount=ko.computed(function(){var n=0;return u.submissions().forEach(function(t){n+=t.emailCount()}),n});u.id=i.Id;u.name=i.Name;u.selectedTemplate=ko.observable();u.sessionId=ko.observable();u.preview=new o;u.loadPreview=function(){return t.request({requestUri:n.odata.getUrl(n.odata.entitySet.trackSummaries,null,"Preview"),data:{Request:{SubmissionId:u.submissions()[u.preview.selectedSubmissionIndex()].id,TemplateId:u.selectedTemplate().id,UserId:u.submissions()[u.preview.selectedSubmissionIndex()].email()[u.preview.selectedEmailIndex()]}},method:"POST"},function(n){u.preview.previewBody(n.Body);u.preview.previewSubject(n.Subject);u.preview.previewFromEmail(n.FromEmail);u.preview.previewFromName(n.FromName);u.preview.previewToEmail(n.ToEmail);u.preview.previewToName(n.ToName)})};u.previousClick=function(){u.preview.selectedEmailIndex()<=0&&(u.preview.selectedSubmissionIndex(u.preview.selectedSubmissionIndex()-1),u.preview.selectedEmailIndex(u.submissions()[u.preview.selectedSubmissionIndex()].emailCount()));u.preview.selectedEmailIndex(u.preview.selectedEmailIndex()-1);u.preview.selectedIndex(u.preview.selectedIndex()-1);u.loadPreview()};u.nextClick=function(){u.preview.selectedIndex(u.preview.selectedIndex()+1);u.preview.selectedEmailIndex(u.preview.selectedEmailIndex()+1);u.preview.selectedEmailIndex()>=u.submissions()[u.preview.selectedSubmissionIndex()].emailCount()&&(u.preview.selectedSubmissionIndex(u.preview.selectedSubmissionIndex()+1),u.preview.selectedEmailIndex(0));u.loadPreview()};u.isPreviousEnabled=function(){return u.preview.selectedIndex()>0};u.isNextEnabled=function(){return u.preview.selectedIndex()<u.emailCount()-1}}function c(n,t){var i=this,r;for(i.root=t,i.id=n.Id,i.name=n.Name,i.visibleToAuthorQuestionCount=n.VisibleToAuthorQuestionCount,i.isAuthorNotificationAlreadySent=n.IsAuthorNotificationAlreadySent,i.hasAwaitingDecision=n.HasAwaitingDecision,i.awaitingDecisionStatusName=n.AwaitingDecisionStatusName,i.isChecked=ko.observable(!1),i.statuses=ko.observableArray(),r=0;r<n.StatusSummaries.length;r++)i.statuses.push(new h(n.StatusSummaries[r],i));i.submissionCount=ko.computed(function(){var n=0;return i.statuses().forEach(function(t){n+=t.submissionCount()}),n});i.emailCount=ko.computed(function(){var n=0;return i.statuses().forEach(function(t){n+=t.emailCount()}),n})}function l(){var u=this;u.emailProgressVm=null;u.editTemplatesVm=null;u.templates=ko.observableArray();u.tracks=ko.observableArray();u.allTracksShown=ko.observable(!1);u.showAllTracks=function(){u.allTracksShown(!0)};u.editTemplatesInDialog=function(){u.editTemplatesVm||(u.editTemplatesVm=new e(r.getElementById("editTemplatesDialog")),u.editTemplatesVm.bind());u.editTemplatesVm.editInDialog().done(function(){u.loadTemplates()})};u.getEmailingTypeTitle=function(n){switch(n){case"primaryOnly":return"Primary Contact Authors Only";case"allAuthors":return"All Authors With Registered Account";default:return"Unknown"}};u.getEmailingTypeTitleForNotice=function(n){return u.getEmailingTypeTitle(n).toLowerCase()};u.emailingType=ko.observable("primaryOnly");u.emailingTypeTitleForNotice=ko.computed(function(){return u.getEmailingTypeTitleForNotice(u.emailingType())});u.emailingTypeTitle=ko.computed(function(){return u.getEmailingTypeTitle(u.emailingType())});u.totalEmailCount=ko.computed(function(){var n=0;return u.tracks().forEach(function(t){t.isChecked()&&(n+=t.emailCount())}),n});u.totalSubmissionCount=ko.computed(function(){var n=0;return u.tracks().forEach(function(t){t.isChecked()&&(n+=t.submissionCount())}),n});u.notificationHasSentAtLeastForOneTrack=ko.computed(function(){var n=!1;return u.tracks().forEach(function(t){n=n||t.isAuthorNotificationAlreadySent}),n});u.showAllTracksVisible=ko.computed(function(){return u.notificationHasSentAtLeastForOneTrack()&&!u.allTracksShown()});u.loadTrackSummaries=function(){return t.read(n.odata.getUrl(n.odata.entitySet.trackSummaries+"?$expand=StatusSummaries($expand=SubmissionSummaries)"),function(n){for(var t=0;t<n.value.length;t++)u.tracks.push(new c(n.value[t],u))})};u.loadTemplates=function(){return t.read(n.odata.getUrl(n.odata.entitySet.emailTemplates,{orderby:"Name"}),function(t){var r,i;for(u.templates().length<=0&&u.templates.push((new f).createStub("Select predefined template…",0)),i=0;i<u.tracks().length;i++)for(r=0;r<u.tracks()[i].statuses().length;r++)u.tracks()[i].statuses()[r].selectedTemplate(u.templates()[0]);for(u.templates().length>1&&u.templates.splice(1,u.templates().length-1),i=0;i<t.value.length;i++)u.templates.push(n.autoMap(new f,t.value[i]))})};u.send=function(){var i=[];return u.tracks().forEach(function(n){n.isChecked()&&n.statuses().forEach(function(n){n.submissions().forEach(function(t){t.emailCount()>0&&i.push({TemplateId:n.selectedTemplate().id,SubmissionId:t.id,Users:t.email()})})})}),t.request({requestUri:n.odata.getUrl(n.odata.entitySet.trackSummaries,null,"Send"),data:{Request:{Submissions:i}},method:"POST"},function(t){var i=[];t.TrackStatusSessions.forEach(function(n){var r=null,t;u.tracks().forEach(function(t){t.isChecked()&&t.id==n.TrackId&&(r=t)});t=null;r.statuses().forEach(function(i){i.emailCount()>0&&i.id==n.StatusId&&(t=i)});t.sessionId(n.SessionId);i.push(n.SessionId)});u.emailProgressVm||(u.emailProgressVm=new n.EmailProgressViewModel(r.getElementById("showProgressDialog"),!0),u.emailProgressVm.bind());u.emailProgressVm.showInDialog(i)},function(t){n.addErrorMessage(n.odata.getErrorMessage(t))})};u.bindTo=function(n){i.when(u.loadTemplates(),u.loadTrackSummaries()).done(function(){ko.setupWizardSteps(u,5);u.fwdButtonTitles[2]="Preview";u.fwdButtonTitles[3]="Send";u.mayGoFwd=function(){var n;return u.currentStep()==0?(n=!1,u.tracks().forEach(function(t){n=n||t.isChecked()}),n):u.currentStep()==1?(n=!0,u.tracks().forEach(function(t){t.isChecked()&&t.statuses().forEach(function(t){n=n&&t.selectedTemplate().id!=0})}),n):!0};u.mayGoBack=function(){return!0};u.beforeNextStepInvoked=function(n){if(u.currentStep()==2){var t=[];return u.tracks().forEach(function(n){n.isChecked()&&n.statuses().forEach(function(n){n.preview.selectedEmailIndex(0);n.preview.selectedSubmissionIndex(0);n.preview.selectedIndex(0);n.emailCount()>0&&t.push(n.loadPreview())})}),i.when.apply(null,t).done(n),!1}return u.currentStep()==3?(u.send().done(n),!1):!0};u.startOver();ko.applyBindingsAndShow(u,n)})}}n.authorNotification=function(n){(new l).bindTo(n)}}(window.app,window.OData,window.jQuery,window.document,window.confirm),function(n,t,i){"use strict";function r(n){this.id=n.Id;this.title=n.Title;this.trackName=n.TrackName;this.firstName=n.FirstName;this.lastName=n.LastName;this.organization=n.Organization;this.role=n.Role;this.dateTime=n.DateTime;this.activity=n.Activity;this.status=n.Status;this.comment=n.Comment;this.dateTimeFormatted=function(){return t.formatUndefinableDateTime(this.dateTime)}}t.AuditActivitiesPage=function(t,i,r){var u=this;u.$element=n(t);u.conference=window.cmt3.conference.name;u.page=ko.observable(1);u.top=ko.observable(25);u.sort=ko.observable("Id");u.controller=i;u.filters=[];u._total=ko.observable(0);u.selected=ko.observable(0);u.auditActivities=ko.observableArray();u.listen();u.Pager=ko.pager(u.selected,u.top);u.Pager().CurrentPage.subscribe(function(){u.page(u.Pager().CurrentPage());u.show()});u.trackNamesProvider=ko.pureComputed(function(){var n=[];for(var t in r)r.hasOwnProperty(t)&&n.push(r[t].name);return n})};t.AuditActivitiesPage.prototype={listen:function(){var t=this;n(document).on("data.filter",function(){t.Pager().CurrentPage()<2?t.show():t.Pager().CurrentPage(1)})},getFilter:function(){var t="";return n.each(this.filters,function(n,i){i.getValue()&&(t+=t==""?i.getValue():" and "+i.getValue())}),t},show:function(){var u=this;if(u.initialized){var f=u.sort(),e=u.top(),o=u.skip(),s=u.getFilter(),h=f?"&$orderby="+f:"",c=e?"&$top="+e:"",l=o?"&$skip="+o:"",a=s?"&$filter="+encodeURIComponent(s):"",v={headers:{Accept:"application/json"},requestUri:"/api/odata/"+this.conference+"/$batch",method:"POST",data:{requests:[{url:"/api/odata/"+this.conference+"/"+u.controller+"?$count=true"+h+a+l+c,method:"GET",headers:{Accept:"application/json"}}]}};i.request(v,function(i){t.page.saveState("audit",{sort:f,top:e,skip:o,filter:s});var h=i.responses[0].body,c=h["@odata.count"],a=h.value,l=[];n.each(a,function(n,t){l.push(new r(t))});u.auditActivities(l);u._total()==0&&u._total(c);u.selected(c);n("html,body").scrollTop(0)},function(n){window.cmt3.logger.log(n.message)},i.batchHandler)}},scroll:function(){n(window).scrollTop()==n(document).height()-n(window).height()&&self.show()},reset:function(){n.each(this.filters,function(n,t){t.reset()});this.show()},size:function(t,i){var r,u,f;n("a",".show").removeClass("btn-success").css("color","#999999");n(i.currentTarget).addClass("btn-success").css("color","white");r=n(i.target).attr("size");u=parseInt(r);this.top(u);f=this.Pager().CurrentPage();this.Pager().CurrentPage(1);f===1&&this.show()},skip:function(){return(this.page()-1)*this.top()},prev:function(){this.top()!=0&&this.page()!=1&&(this.page(this.page()-1),this.show())},next:function(){this.top()==0||this.page()>this.selected()/this.top()||(this.page(this.page()+1),this.show())},setSort:function(t,i){var r=n(i.target),u=r.attr("data-sort");(u==null||u==undefined)&&(r=n(r.context.parentNode),u=r.attr("data-sort"));r.hasClass("selected")?this.sort().match(" desc$")?(this.sort(u+" asc"),r.find("i").removeClass("icon-arrow-down"),r.find("i").addClass("icon-arrow-up")):(this.sort(u+" desc"),r.find("i").removeClass("icon-arrow-up"),r.find("i").addClass("icon-arrow-down")):(n("th[data-sort]").each(function(){n(this).find("i").removeClass("icon-arrow-up");n(this).find("i").removeClass("icon-arrow-down");n(this).removeClass("selected")}),r.find("i").removeClass("icon-arrow-down"),r.find("i").addClass("icon-arrow-up"),r.addClass("selected"),this.sort(u+" asc"));this.show()},refresh:function(){this.show()},exportActivitiesAsTSV:function(n,i){var r=this,u=t.GetEventFilter(i),f="/api/odata/"+r.conference+"/"+r.controller+"/ExportActivitiesAsTSV",e={Filter:u};t.page.post(f,e)}}}(window.jQuery,window.app,window.OData),function(n,t,i){"use strict";function u(r){function e(){o();f=u.isChecked.subscribe(s)}function o(){f&&typeof f.dispose=="function"&&f.dispose()}function s(){u.initialState===undefined?u.initialState=u.isChecked():h.call(u)}function h(){var f=this,s,h,c;f.isToggleInProgress(!0);s={ReasonId:u.id()};s.Type=f.isChecked()?"Add":"Remove";h=n.Deferred(function(n){window.setTimeout(n.resolve,500)});c=i.request({requestUri:t.odata.getUrl(t.odata.entitySet.submissions,r,"ModifyConflict"),method:"POST",showProgressIndicator:!1,data:{Request:s}},function(){},function(n){o();u.isChecked(!u.isChecked());e();t.addErrorMessage("Unable to edit conflict."+t.odata.getErrorMessage(n))});n.when(c,h).always(function(){f.isToggleInProgress(!1)})}var u=this,f;u.id=ko.observable().autoMap();u.name=t.autoMap();u.isChecked=ko.observable();u.initialState=undefined;u.isToggleInProgress=ko.observable(!1);e()}function f(){var n=this;n.title=t.autoMap();n.answers=[]}function e(){var n=this;n.answer=t.autoMap();n.customData=null;n.yesNo=ko.pureComputed(function(){return n.customData.Answer==="yes"?"Yes":n.customData.Answer==="no"?"No":"Not Applicable"});n.comment=ko.pureComputed(function(){return n.customData.Comment&&n.customData.Comment.htmlMultiLineEncode()})}function r(n){var i=this;n?(i.id=n.Id,i.firstName=n.FirstName,i.lastName=n.LastName,i.name=n.Name,i.email=n.Email,i.organization=n.Organization):(i.id=t.autoMap(),i.firstName=t.autoMap(),i.lastName=t.autoMap(),i.name=t.autoMap(),i.email=t.autoMap(),i.organization=t.autoMap());i.readFromJson=function(n){t.autoMap(i,n)}}function o(u,f){var e=this;e.parentVm=f;e.biddingModel=null;e.to=ko.observable(null).extend({required:!0,email:!0,maxLength:200});e.toFirstName=ko.observable(null).extend({required:!0,maxLength:200});e.toMiddleInitial=ko.observable(null).extend({maxLength:10});e.toLastName=ko.observable(null).extend({required:!0,maxLength:200});e.toOrganization=ko.observable(null).extend({required:!0,maxLength:200});e.userId=ko.observable(null);e.isSearching=ko.observable();e.searched=ko.observable(!1);e.userFound=ko.computed(function(){return e.userId()!==null&&e.searched()&&!e.to.isModified()});e.userNotFound=ko.computed(function(){return e.userId()===null&&e.searched()&&!e.to.isModified()});e.search=function(){var n=ko.validation.group([e.to]),r;if(n().length>0){n.showAllMessages();return}e.isSearching(!0);r={requestUri:t.odata.getGlobalUrl(t.odata.entitySet.users,null,"SearchByEmail"),method:"POST",showProgressIndicator:!1,data:{Email:e.to()}};i.read(r,function(n){e.userId(n.Id);e.to(n.Email);e.toFirstName(n.FirstName);e.toMiddleInitial(n.MiddleInitial);e.toLastName(n.LastName);e.toOrganization(n.Organization);e.isSearching(!1);e.searched(!0);e.to.isModified(!1)},function(n){e.isSearching(!1);n.response.statusCode===404?(e.userId(null),e.toFirstName(null),e.toFirstName.isModified(!1),e.toMiddleInitial(null),e.toLastName(null),e.toLastName.isModified(!1),e.toOrganization(null),e.toOrganization.isModified(!1),e.searched(!0),e.to.isModified(!1)):i.defaultError(n)})};e.assignOrRemove=function(f){var o={requestUri:t.odata.getUrl(t.odata.entitySet.reviews,null,"AssignExternalReviewer"),method:"POST",showProgressIndicator:!1,data:{Request:{SubmissionId:e.biddingModel.id,ExternalReviewerId:f}}};i.read(o,function(t){var i=new r;i.readFromJson(t);e.biddingModel.externalReviewer(i);n(u).modal("hide")},function(n){e.biddingModel.externalReviewer(null);i.defaultError(n)})};e.assign=function(){var n=e.userId();e.userId(null);e.isSearching(!1);e.searched(!1);e.to("");e.to.isModified(!1);e.assignOrRemove(n)};e.bind=function(){ko.applyBindings(e,u)};e.showDialog=function(){e.userId(null);e.isSearching(!1);e.searched(!1);n(u).modal("show")}}function s(n,f,e,o){var s=this,c,h,l,a;for(s.id=n.Id,s.title=n.Title,s.abstract=n.Abstract,s.originalSubmissionId=n.OriginalSubmissionId,s.track=n.Track,s.trackId=n.TrackId,s.primarySubject=n.PrimarySubject,s.secondarySubject=n.SecondarySubject,s.relevance=n.Relevance,s.tpmsRank=n.TpmsRank,s.customAffinityRank=n.CustomAffinityRank,s.bid=n.Bid,s.assigned=n.Assigned,s.reviewId=n.ReviewId,s.authorFeedbackId=n.AuthorFeedbackId,s.biddingEnabled=n.BiddingEnabled,s.reviewingEnabled=n.ReviewingEnabled,s.reviewingDisabled=n.ReviewingDisabled,s.isReviewReadOnly=n.IsReviewReadOnly,s.reviewingCompleted=n.ReviewingCompleted,s.discussionEnabled=n.DiscussionEnabled,s.doNotAllowReviewerToPostDiscussion=n.DoNotAllowReviewerToPostDiscussion,s.doNotAllowReviewerToEditNote=n.DoNotAllowReviewerToEditNote,s.doNotEnableReviewerNote=n.DoNotEnableReviewerNote,s.reproducibilityInfoRequired=n.ReproducibilityInfoRequired,s.feedbackComplete=n.FeedbackComplete,s.metaReviewingDisabled=n.MetaReviewingDisabled,s.submissionEnabledForDiscussion=n.SubmissionEnabledForDiscussion,s.allowReviewersToDiscussAllPapers=n.AllowReviewersToDiscussAllPapers,s.allowReviewerToSeeReviewingDataOnlyAfterSubmitting=n.AllowReviewerToSeeReviewingDataOnlyAfterSubmitting,s.allowReviewerToSeeReviewingDataAfterReviewing=n.AllowReviewerToSeeReviewingDataAfterReviewing,s.metaReviewAssigned=n.MetaReviewAssigned,s.metaReviewSubmitted=n.MetaReviewSubmitted,s.assignedSeniorMetaReviewer=n.AssignedSeniorMetaReviewer,s.filesUploaded=n.FilesUploaded,s.messages=n.Messages,s.enableExternalReviewer=n.EnableExternalReviewer,s.reviewerLabel=function(){return n.HiddenNumber?"Reviewer #"+n.HiddenNumber:""},s.externalReviewer=ko.observable(n.ExternalReviewer===null?null:new r(n.ExternalReviewer)),s.status=n.Status,s.statusPropertyIsRevision=n.StatusPropertyIsRevision,s.allowReviewUpdateDuringDiscussion=n.AllowReviewUpdateDuringDiscussion,s.allowOnlyRevisionForReviewing=n.AllowOnlyRevisionForReviewing,s.downloadLink=function(){return e.submissionFileWithSupplemental.format(s.id)},s.reviewerNoteId=n.ReviewerNoteId,s.reviewerNoteSubmitted=n.ReviewerNoteSubmitted,s.isViewOthersReviewsAvailable=n.IsViewOthersReviewsAvailable,s.isAuthorFeedbackAvailable=n.IsAuthorFeedbackAvailable,s.editReviewerNoteUrl=function(){return s.reviewerNoteId?e.reviewerNoteDetails.format(s.reviewerNoteId):e.reviewerNoteCreate.format(s.id)},s.editReviewerNoteText=function(){return s.reviewerNoteSubmitted?"Edit":"Add"},s.editReviewerNoteTooltip=function(){return s.reviewerNoteSubmitted?"Edit note":"Add note"},s.viewReviewerNoteUrl=function(){return s.reviewerNoteId?e.reviewerNoteView.format(s.reviewerNoteId):""},s.isConflictSelectedText=ko.pureComputed(function(){for(var n=0;n<s.reviewerConflictReasons.length;n++)if(s.reviewerConflictReasons[n].isChecked())return"Yes";return"No"}),s.chairNoteColumns=[],n.CNQ01Id!==null?s.chairNoteColumns.push(new t.QuestionResponseColumn(n.CNQ01Id,n.CNQ01Text)):s.chairNoteColumns.push(null),n.CNQ02Id!==null?s.chairNoteColumns.push(new t.QuestionResponseColumn(n.CNQ02Id,n.CNQ02Text)):s.chairNoteColumns.push(null),n.CNQ03Id!==null?s.chairNoteColumns.push(new t.QuestionResponseColumn(n.CNQ03Id,n.CNQ03Text)):s.chairNoteColumns.push(null),n.CNQ04Id!==null?s.chairNoteColumns.push(new t.QuestionResponseColumn(n.CNQ04Id,n.CNQ04Text)):s.chairNoteColumns.push(null),h=0,c=[],h=0;h<f.length;h++)c.push(s.chairNoteColumns[h]);if(s.chairNoteColumns=c,s.reviewerConflictReasons=[],o&&o.conflictDeclarationAllowedTracks&&o.conflictDeclarationAllowedTracks[s.trackId]===!0&&o.conflictReasons)for(h=0;h<o.conflictReasons.length;h++)l=o.conflictReasons[h],a=t.autoMap(new u(s.id),l),a.isChecked(n&&n.ConflictReasonIds&&n.ConflictReasonIds.indexOf(l.Id)>-1),s.reviewerConflictReasons.push(a);s.editReviewUrl=function(){return s.reviewId?e.reviewDetails.format(s.reviewId):e.reviewCreate.format(s.id)};s.viewReviewUrl=function(){return s.reviewId?e.reviewView.format(s.reviewId):null};s.viewMetaReviewsUrl=function(){return s.allowDiscussion()?e.metaReviews.format(s.id):null};s.allowDiscussion=function(){return s.isViewOthersReviewsAvailable};s.isActionApplicable=function(){return s.assigned&&s.reviewingEnabled||s.allowDiscussion()};s.viewAllReviewsUrl=function(){return s.allowDiscussion()?e.reviewViewAll.format(s.id):null};s.viewUrl=function(){return e.submissionSummary.format(s.id)};s.reviewingDetailsUrl=function(){return s.allowDiscussion()?e.reviewingDetailsUrl.format(s.id):null};s.viewOriginalUrl=function(){return s.originalSubmissionId?e.submissionSummary.format(s.originalSubmissionId):null};s.showFeed=function(){return e.feed.format(s.id)};s.viewAuthorFeedbackUrl=function(){return s.isAuthorFeedbackAvailable?e.feedback.format(s.authorFeedbackId):null};s.externalReviewerEmailUrl=function(){return e.externalReviewerEmail.format(s.id,s.externalReviewer().id)};s.metaReviewerEmailUrl=function(){return e.metaReviewerEmail.format(s.id)};s.seniorMetaReviewerEmailUrl=function(){return e.seniorMetaReviewerEmail.format(s.id)};s.removeExternalReviewer=function(){if(confirm("Remove external reviewer?".format(s.id))){var n={requestUri:t.odata.getUrl(t.odata.entitySet.reviews,null,"AssignExternalReviewer"),method:"POST",showProgressIndicator:!1,data:{Request:{SubmissionId:s.id,ExternalReviewerId:null}}};i.read(n,function(){t.addMessage("External reviewer has been removed succesfully.");s.externalReviewer(null)})}}}function h(r,u){var s=u,f=this,e,o;f.submissionCount=ko.observable(0);f.selectedBid=ko.observable(1);f.bidOptions=[{name:"Not Entered",id:1},{name:"Not Willing",id:2},{name:"In A Pinch",id:3},{name:"Willing",id:4},{name:"Eager",id:5}];f.submitEnabled=ko.computed(function(){return f.submissionCount()<=0?!1:f.selectedBid()!==null&&typeof f.selectedBid()!="undefined"});e=function(){return u.controller==="BiddingModels"||u.controller==="BiddingReviewModels"};o=function(){return u.controller==="ReviewModels"||u.controller==="BiddingReviewModels"};f.changeBid=function(){var u={Filter:f.filter,Bid:f.selectedBid(),ShowBidding:e(),ShowReviewing:o()},h={requestUri:t.odata.getUrl(t.odata.entitySet.biddingReviewModels,null,"BulkChangeBid"),method:"POST",showProgressIndicator:!0,data:{Request:u}};i.request(h,function(){s.refresh();setTimeout(function(){t.addMessage("The bid of selected submissions have been changed.")},500);n(r).modal("hide")})};f.bind=function(){ko.applyBindings(f,r)};f.filter=null;f.editInDialog=function(u){f.filter=u;var s={Filter:u,ShowBidding:e(),ShowReviewing:o()},h={requestUri:t.odata.getUrl(t.odata.entitySet.biddingReviewModels,null,"SubmissionCountFilteredBidding"),method:"POST",data:{Request:s}};i.request(h,function(t){f.submissionCount(t.value);f.selectedBid(null);n(r).modal("show")})}}function c(r,u){var s=u,f=this,e=function(){return u.controller==="BiddingModels"||u.controller==="BiddingReviewModels"},o=function(){return u.controller==="ReviewModels"||u.controller==="BiddingReviewModels"};f.bind=function(){ko.applyBindings(f,r)};f.editInDialog=function(u){var f={Filter:u,ShowBidding:e(),ShowReviewing:o()},s={requestUri:t.odata.getUrl(t.odata.entitySet.biddingReviewModels,null,"BidSummaryFilteredBidding"),method:"POST",data:{Request:f}};i.request(s,function(t){var i=t.value;n("#imagebids").html('<img src="data:image/png;base64,'+i+'" />');n(r).modal("show")})}}function l(r,u){var s=u,o=this;o.id=ko.observable();o.title=ko.observable();o.reproQuestions=ko.observableArray();o.bind=function(){ko.applyBindings(o,r)};o.editInDialog=function(u){o.reproQuestions([]);var s={requestUri:t.odata.getUrl(t.odata.entitySet.submissionViews,u,"GetSummaryView"),headers:{"Content-Type":"application/json"},method:"POST"};i.request(s,function(i){var c,l,u,a,s,h;if(o.id(i.Id),o.title(i.Title),i.ReproducibilityQuestionAnswersJson)for(c=JSON.parse(i.ReproducibilityQuestionAnswersJson),s=0;s<c.length;s++){if(l=t.autoMap(new f,c[s]),u=c[s].Answers,u)for(h=0;h<u.length;h++)a=t.autoMap(new e,u[h]),a.customData=JSON.parse(u[h].Text),l.answers.push(a);o.reproQuestions.push(l)}n(r).modal("show")})}}function a(r,u){var e=u,f=this;f.id=ko.observable();f.title=ko.observable();f.body=ko.observable();f.bind=function(){ko.applyBindings(f,r)};f.save=function(){var u={requestUri:t.odata.getUrl(t.odata.entitySet.authorFeedbackComments),headers:{"Content-Type":"application/json"},method:"POST",data:{SubmissionId:f.id(),Title:f.title(),Body:f.body()}};i.request(u,function(){t.addMessage("Author feedback comment saved.");n(r).modal("hide")})};f.editInDialog=function(t){f.id(t);n(r).modal("show")}}t.BiddingPage=function(t,i,r,u,f,e,s){var v=this,y,p,w,b;v.chairNoteQuestions=r;v.$element=n(t);v.conference=window.cmt3.conference.name;v.page=ko.observable(1);v.top=ko.observable(25);v.sort=ko.observable("Id");v.controller=i;v.filters=[];v._total=ko.observable(0);v.selected=ko.observable(0);v.biddingModels=ko.observableArray();v.reviewerConflictReasons=f.conflictReasons;v.bid=ko.observable();v.editingBid=ko.observable(!1);v.listen();v.Pager=ko.pager(v.selected,v.top);v.Pager().CurrentPage.subscribe(function(){v.page(v.Pager().CurrentPage());v.show()});v.pageUrls=u;v.params=f;v.bidNames=s;v.hasReviewerNoteQuestion=function(n){return e&&e.indexOf(n)!==-1};v.downloadSubmissionFileLink=function(){return v.pageUrls.submissionFile.format("")};v.submissionComparisonLink=function(){return v.pageUrls.submissionComparison.format("")};v.downloadAllLink=function(){return v.pageUrls.submissionFileWithSupplemental.format("")};v.importReviewsLink=function(){return v.pageUrls.importReviews};v.showWelcomeMessage=function(){n(document.getElementById("welcomeMessageDialog")).modal("show")};v.bidNamesProvider=function(){var n=v.bidNames;return n.sort(),n};v.assignExternalReviewerVm=null;v.showAssignExternalReviewerDialog=function(n){v.assignExternalReviewerVm===null&&(v.assignExternalReviewerVm=new o(document.getElementById("selectUserDialog"),v),v.assignExternalReviewerVm.bind());v.assignExternalReviewerVm.biddingModel=n;v.assignExternalReviewerVm.showDialog()};y=null;v.changeBid=function(n){y===null&&(y=new h(document.getElementById("changeBidDialog"),v),y.bind());y.editInDialog(n)};p=null;v.bidSummary=function(n){p===null&&(p=new c(document.getElementById("bidSummaryDialog"),v),p.bind());p.editInDialog(n)};w=null;v.reproducibilitySummary=function(n){w===null&&(w=new l(document.getElementById("reproducibilityDialog"),v),w.bind());w.editInDialog(n)};b=null;v.commentAuthorFeedback=function(n){b===null&&(b=new a(document.getElementById("authorFeedbackCommentDialog"),v),b.bind());b.editInDialog(n)}};t.BiddingPage.prototype={listen:function(){var t=this;n(document).on("data.filter",function(){t.Pager().CurrentPage()<2?t.show():t.Pager().CurrentPage(1)})},getFilter:function(){var t="";return n.each(this.filters,function(n,i){i.getValue()&&(t+=t===""?i.getValue():" and "+i.getValue())}),t},show:function(r,u,f,e,o){function c(r){var l=u?u:h.sort(),a=f?f:h.getFilter(),v=e?e:h.skip(),y=typeof o!="undefined"&&o!==null?o:h.top(),w=l?"&$orderby="+l:"",b=y?"&$top="+y:"",k=v?"&$skip="+v:"",p=a?"&$filter="+encodeURIComponent(a):"",d={headers:{Accept:"application/json"},requestUri:"/api/odata/"+h.conference+"/$batch",method:"POST",data:{requests:[{url:"/api/odata/"+h.conference+"/"+h.controller+"?"+(r?"$count=true&$top=0"+p:w+p+k+b),method:"GET",headers:{Accept:"application/json"}}]}},c=n.Deferred();return i.request(d,function(i){var u,e,f,o;t.page.saveState("biddings",{sort:l,top:y,skip:v,filter:a});u=i.responses[0].body;r?(o=u["@odata.count"],c.resolve(o)):(e=u.value,f=[],n.each(e,function(n,t){f.push(new s(t,h.chairNoteQuestions,h.pageUrls,h.params))}),c.resolve(f))},function(n){window.cmt3.logger.log(n.message);c.reject()},i.batchHandler),c.promise()}var h=this;(h.initialized||r)&&(t.showProgress(),n.when(c(!1),c(!0)).done(function(n,t){h._total()===0&&h._total(t);h.selected(t);h.biddingModels(n)}).always(t.hideProgress()))},scroll:function(){n(window).scrollTop()===n(document).height()-n(window).height()&&self.show()},selectBid:function(t,i){var u=n(i.target),e=ko.contextFor(i.target),r=n(n("#bidTemplate").text()),f;u.hide();u.after(r);f=e.$parent.getBids(t.id,u,r);ko.applyBindings(f,r[0]);r.find("select").focus()},getBids:function(n,t,r){var u=[{name:"Not Entered",id:1},{name:"Not Willing",id:2},{name:"In A Pinch",id:3},{name:"Willing",id:4},{name:"Eager",id:5}],f={options:ko.observableArray(u),selectedBid:ko.observable()};return f.selectedBid.subscribe(function(f){var e={requestUri:"/api/odata/"+window.cmt3.conference.name+"/BiddingModels("+n+")",method:"PATCH",headers:{Prefer:"return-content"},progressIndicatorTimeout:0,data:{BidId:f[0]}};i.request(e,function(n){r.remove();t.text(u[n.BidId-1].name);t.show()})}),f},post:function(n,t,i){var r,f,u;i=i||"post";r=document.createElement("form");r.setAttribute("method",i);r.setAttribute("action",n);for(f in t)t.hasOwnProperty(f)&&(u=document.createElement("input"),u.setAttribute("type","hidden"),u.setAttribute("name",f),u.setAttribute("value",t[f]),r.appendChild(u));document.body.appendChild(r);r.submit();document.body.removeChild(r)},stub:function(){alert("Sorry, this feature is not implemented yet.")},reset:function(){n.each(this.filters,function(n,t){t.reset()});this.show()},size:function(t,i){var r,u,f;n("a",".show").removeClass("btn-success").css("color","#999999");n(i.currentTarget).addClass("btn-success").css("color","white");r=n(i.target).attr("size");u=parseInt(r);this.top(u);f=this.Pager().CurrentPage();this.Pager().CurrentPage(1);f===1&&this.show()},skip:function(){return(this.page()-1)*this.top()},prev:function(){this.top()!==0&&this.page()!==1&&(this.page(this.page()-1),this.show())},next:function(){this.top()===0||this.page()>this.selected()/this.top()||(this.page(this.page()+1),this.show())},setSort:function(t,i){var r=n(i.target),u=r.attr("data-sort");(u===null||u===undefined)&&(r=n(r.context.parentNode),u=r.attr("data-sort"));r.hasClass("selected")?this.sort().match(" desc$")?(this.sort(u+" asc"),r.find("i").removeClass("icon-arrow-down"),r.find("i").addClass("icon-arrow-up")):(this.sort(u+" desc"),r.find("i").removeClass("icon-arrow-up"),r.find("i").addClass("icon-arrow-down")):(n("th[data-sort]").each(function(){n(this).find("i").removeClass("icon-arrow-up");n(this).find("i").removeClass("icon-arrow-down");n(this).removeClass("selected")}),r.find("i").removeClass("icon-arrow-down"),r.find("i").addClass("icon-arrow-up"),r.addClass("selected"),this.sort(u+" asc"));this.show()},refresh:function(){this.show()},showAbstract:function(t,i){var f=ko.contextFor(i.target).$parent,r=n(i.target),u=r.next();u.is(":visible")?(u.hide(),r.text("Show abstract")):(u.show(),r.text("Hide abstract"))},bulkChangeBid:function(n,i){var r=t.GetEventFilter(i);this.changeBid(r)},showBidSummary:function(n,i){var r=t.GetEventFilter(i);this.bidSummary(r)},showReproducibility:function(t,i){var r=i.target,u=ko.contextFor(r),f=parseInt(n(r).attr("sid"));u.$root.reproducibilitySummary(f)},showAuthorFeedbackComment:function(n,t){var r=t.target,i=ko.contextFor(r);i.$root.commentAuthorFeedback(i.$data.id)}}}(window.jQuery,window.app,window.OData),function(n,t,i){"use strict";function r(){var r=this;r.isFileUploaded=ko.observable(!1);r.hasError=ko.observable(!1);r.errorText=ko.observable();r.bids=ko.observableArray();r.normalBids=ko.observableArray();r.uploading=ko.observable(!1);r.fileName=ko.observable("");r.cancel=function(){window.location="/"+window.cmt3.conference.name+"/Submission/Manage"};r.getModel=function(){for(var n,u,i=[],t=0;t<r.normalBids().length;t++)n=r.normalBids()[t],u={Email:n.email,SubmissionId:n.id,BidValue:n.bidValue},i.push(u);return{Bids:i}};r.send=function(){var i=r.getModel(),u={requestUri:n.odata.getUrl(n.odata.entitySet.biddings,null,"Import"),method:"POST",data:{Request:i}};t.request(u,function(){window.location="/"+window.cmt3.conference.name+"/Submission/Manage"})};r.post=function(n,t,i){var r,f,u;i=i||"post";r=document.createElement("form");r.setAttribute("method",i);r.setAttribute("action",n);for(f in t)t.hasOwnProperty(f)&&(u=document.createElement("input"),u.setAttribute("type","hidden"),u.setAttribute("name",f),u.setAttribute("value",t[f]),r.appendChild(u));document.body.appendChild(r);r.submit();document.body.removeChild(r)};r.downloadTemplate=function(){var n="/api/odata/"+window.cmt3.conference.name+"/BiddingModels/GetImportTemplate";r.post(n,{})};r.uploadFile=function(n,t){t.target.value!=""&&(t.target.form.submit(),r.uploading(!0))};r.parseUploadResult=function(){var t=i.parseJSON(i("#singleFileUploadFrame").contents().text()),u,n,f;if(r.bids.removeAll(),r.normalBids.removeAll(),r.hasError(t.HasError),r.errorText(t.ErrorText),!r.hasError())for(u=0;u<t.Models.length;u++)n=t.Models[u],f={email:n.Email,id:n.Id,bid:n.Bid,bidValue:n.BidValue,status:n.Status,hasError:n.HasError,lineNumber:n.LineNumber},r.bids.push(f),f.hasError||r.normalBids.push(f);r.isFileUploaded(!0);r.uploading(!1);r.fileName("")};r.bindTo=function(n){ko.applyBindingsAndShow(r,n)}}n.importBids=function(n){(new r).bindTo(n)}}(window.app,window.OData,window.jQuery,window.document,window.confirm,window.setTimeout),function(n,t,i){"use strict";function r(t){var i=this;i.parent=t;i.assignments=ko.observableArray([]);n.DataTable.call(i)}function u(u,f){var e=this;e.isMetaReview=u;e.isSenior=f;e.table=new r(e);e.isFileUploaded=ko.observable(!1);e.hasError=ko.observable(!1);e.errorText=ko.observable();e.assignments=ko.observableArray();e.removeAssignments=ko.observableArray();e.normalAssignments=ko.observableArray();e.normalRemoveAssignments=ko.observableArray();e.uploading=ko.observable(!1);e.cancel=function(){window.location="/"+window.cmt3.conference.name+"/Submission/Manage"};e.getModel=function(){for(var t,u,f,i=[],r=[],n=0;n<e.normalAssignments().length;n++)t=e.normalAssignments()[n],u={Email:t.email,SubmissionId:t.id},i.push(u);for(n=0;n<e.normalRemoveAssignments().length;n++)f=e.normalRemoveAssignments()[n].id,r.push(f);return{Assignments:i,RemoveAssignments:r}};e.send=function(){var i=e.getModel(),r={requestUri:n.odata.getUrl(n.odata.entitySet.submissions,null,e.isMetaReview?e.isSenior?"ImportSeniorMetaAssignmentsXml":"ImportMetaAssignmentsXml":"ImportAssignmentsXml"),method:"POST",data:{Request:i}};t.request(r,function(){window.location="/"+window.cmt3.conference.name+"/Submission/Manage"})};e.post=function(n,t,i){var r,f,u;i=i||"post";r=document.createElement("form");r.setAttribute("method",i);r.setAttribute("action",n);for(f in t)t.hasOwnProperty(f)&&(u=document.createElement("input"),u.setAttribute("type","hidden"),u.setAttribute("name",f),u.setAttribute("value",t[f]),r.appendChild(u));document.body.appendChild(r);r.submit();document.body.removeChild(r)};e.downloadTemplate=function(){var n="/api/odata/"+window.cmt3.conference.name+"/Submissions/"+(e.isMetaReview?e.isSenior?"GetSeniorMetaAssignmentImportTemplate":"GetMetaAssignmentImportTemplate":"GetAssignmentImportTemplate");e.post(n,{})};e.uploadFile=function(n,t){t.target.value!=""&&(e.uploading(!0),t.target.form.submit())};e.parseUploadResult=function(){var t=i.parseJSON(i("#singleFileUploadFrame").contents().text()),r,n,u,f;if(e.assignments.removeAll(),e.normalAssignments.removeAll(),e.normalRemoveAssignments.removeAll(),e.hasError(t.HasError),e.errorText(t.ErrorText),!e.hasError()){for(r=0;r<t.Models.length;r++)n=t.Models[r],n.Email==null?(u={id:n.Id,title:n.Title,status:n.Status,hasError:n.HasError,lineNumber:n.LineNumber},e.removeAssignments.push(u),u.hasError||e.normalRemoveAssignments.push(u)):(f={email:n.Email,id:n.Id,title:n.Title,status:n.Status,hasError:n.HasError,lineNumber:n.LineNumber},e.assignments.push(f),f.hasError||e.normalAssignments.push(f));e.table.loadData(!0)}e.isFileUploaded(!0);e.uploading(!1)};e.bindTo=function(n){ko.applyBindingsAndShow(e,n)}}r.prototype=i.extend({},n.DataTable.prototype,{getStorageKey:function(){return"ImportAssignmentTable"},loadData:function(n){var t,i;n=n===!0;t=this;n&&t.applyState();i=t.top()>0?t.parent.assignments().slice(t.skip(),t.skip()+t.top()):t.parent.assignments();t.total(t.parent.assignments().length);t.assignments(i)}});n.importAssignments=function(n,t,i){new u(n,t).bindTo(i)}}(window.app,window.OData,window.jQuery,window.document),function(n,t,i){"use strict";function u(){var u=this;u.isFileUploaded=ko.observable(!1);u.hasError=ko.observable(!1);u.errorText=ko.observable();u.assignments=ko.observableArray();u.normalAssignments=ko.observableArray();u.uploading=ko.observable(!1);u.getModel=function(){for(var t,f,i=[],n=0;n<u.normalAssignments().length;n++)t=u.normalAssignments()[n],f={SeniorMetaReviewerEmail:t.seniorMetaReviewerEmail,MetaReviewerEmail:t.metaReviewerEmail},i.push(f);return{Assignments:i,TrackId:r}};u.send=function(){var i=u.getModel(),f={requestUri:n.odata.getUrl(n.odata.entitySet.users,null,"ImportSeniorMetaAssignments"),method:"POST",data:{Request:i}};t.request(f,function(){window.location="/"+window.cmt3.conference.name+"/User/SeniorMetaReviewers?trackId="+r})};u.downloadTemplate=function(){var t="/api/odata/"+window.cmt3.conference.name+"/Users/GetImportSeniorMetaAssignmentTemplate";n.page.post(t,{})};u.uploadFile=function(n,t){t.target.value!==""&&(u.uploading(!0),t.target.form.submit())};u.parseUploadResult=function(){var t=i.parseJSON(i("#singleFileUploadFrame").contents().text()),r,n,f;if(u.assignments.removeAll(),u.normalAssignments.removeAll(),u.hasError(t.HasError),u.errorText(t.ErrorText),!u.hasError())for(r=0;r<t.Models.length;r++)n=t.Models[r],f={seniorMetaReviewerEmail:n.SeniorMetaReviewerEmail,metaReviewerEmail:n.MetaReviewerEmail,status:n.Status,notice:n.ErrorText,hasError:n.HasError,rawData:n.RawData,lineNumber:n.LineNumber},u.assignments.push(f),f.hasError||u.normalAssignments.push(f);u.isFileUploaded(!0);u.uploading(!1)};u.bindTo=function(n){ko.applyBindingsAndShow(u,n)}}var r=n.url===undefined?null:n.url.queryString.getValue("trackId");n.importSeniorMetaAssignments=function(n){(new u).bindTo(n)}}(window.app,window.OData,window.jQuery,window.document,window.confirm,window.setTimeout),function(n,t,i){"use strict";function r(r,u){var f=this;f.isFileUploaded=ko.observable(!1);f.hasError=ko.observable(!1);f.errorText=ko.observable();f.quotas=ko.observableArray();f.normalQuotas=ko.observableArray();f.uploading=ko.observable(!1);f.getModel=function(){for(var t,e,i=[],n=0;n<f.normalQuotas().length;n++)t=f.normalQuotas()[n],e={Email:t.email,Quota:t.quota},i.push(e);return{Quotas:i,TrackId:r,ForReviewer:u}};f.send=function(){var i=f.getModel(),e={requestUri:n.odata.getUrl(n.odata.entitySet.users,null,"ImportUserQuotas"),method:"POST",data:{Request:i}};t.request(e,function(){window.location=u?"/"+window.cmt3.conference.name+"/User/Reviewers?trackId="+r:"/"+window.cmt3.conference.name+"/User/MetaReviewers?trackId="+r})};f.downloadTemplate=function(){var t="/api/odata/"+window.cmt3.conference.name+"/Users/GetImportUserQuotasTemplate";n.page.post(t,{})};f.uploadFile=function(n,t){t.target.value!==""&&(f.uploading(!0),t.target.form.submit())};f.parseUploadResult=function(){var t=i.parseJSON(i("#singleFileUploadFrame").contents().text()),r,n,u;if(f.quotas.removeAll(),f.normalQuotas.removeAll(),f.hasError(t.HasError),f.errorText(t.ErrorText),!f.hasError())for(r=0;r<t.Models.length;r++)n=t.Models[r],u={email:n.Email,quota:n.Quota,status:n.Status,notice:n.ErrorText,hasError:n.HasError,rawData:n.RawData,lineNumber:n.LineNumber},f.quotas.push(u),u.hasError||f.normalQuotas.push(u);f.isFileUploaded(!0);f.uploading(!1)};f.bindTo=function(n){ko.applyBindingsAndShow(f,n)}}n.importUserQuotas=function(n,t,i){new r(t,i).bindTo(n)}}(window.app,window.OData,window.jQuery),function(n,t,i){"use strict";function r(r){var u=this;u.isFileUploaded=ko.observable(!1);u.hasError=ko.observable(!1);u.errorText=ko.observable();u.tags=ko.observableArray();u.normalTags=ko.observableArray();u.uploading=ko.observable(!1);u.getModel=function(){for(var t,r,i=[],n=0;n<u.normalTags().length;n++)t=u.normalTags()[n],r={Email:t.email,Tag:t.tag},i.push(r);return{Tags:i}};u.send=function(){var i=u.getModel(),f={requestUri:n.odata.getUrl(n.odata.entitySet.users,null,"ImportUserTags"),method:"POST",data:{Request:i}};t.request(f,function(){window.location=r})};u.cancel=function(){window.location=r};u.downloadTemplate=function(){var t="/api/odata/"+window.cmt3.conference.name+"/Users/GetImportUserTagsTemplate";n.page.post(t,null,"GET")};u.uploadFile=function(n,t){t.target.value!==""&&(u.uploading(!0),t.target.form.submit())};u.parseUploadResult=function(){var t=i.parseJSON(i("#singleFileUploadFrame").contents().text()),r,n,f;if(u.tags.removeAll(),u.normalTags.removeAll(),u.hasError(t.HasError),u.errorText(t.ErrorText),!u.hasError())for(r=0;r<t.Models.length;r++)n=t.Models[r],f={email:n.Email,tag:n.Tag,status:n.Status,notice:n.ErrorText,hasError:n.HasError,rawData:n.RawData,lineNumber:n.LineNumber},u.tags.push(f),f.hasError||u.normalTags.push(f);u.isFileUploaded(!0);u.uploading(!1)};u.bindTo=function(n){ko.applyBindingsAndShow(u,n)}}n.importUserTags=function(n,t){new r(t).bindTo(n)}}(window.app,window.OData,window.jQuery),function(n,t,i){"use strict";function r(r){var u=this;u.isFileUploaded=ko.observable(!1);u.hasError=ko.observable(!1);u.errorText=ko.observable();u.userTypes=ko.observableArray();u.normalUserTypes=ko.observableArray();u.uploading=ko.observable(!1);u.getModel=function(){for(var t,r,i=[],n=0;n<u.normalUserTypes().length;n++)t=u.normalUserTypes()[n],r={Email:t.email,UserType:t.userType},i.push(r);return{UserTypes:i}};u.send=function(){var i=u.getModel(),f={requestUri:n.odata.getUrl(n.odata.entitySet.users,null,"ImportUserTypes"),method:"POST",data:{Request:i}};t.request(f,function(){window.location=r})};u.cancel=function(){window.location=r};u.downloadTemplate=function(){var t="/api/odata/"+window.cmt3.conference.name+"/Users/GetImportUserTypesTemplate";n.page.post(t,null,"GET")};u.uploadFile=function(n,t){t.target.value!==""&&(u.uploading(!0),t.target.form.submit())};u.parseUploadResult=function(){var t=i.parseJSON(i("#singleFileUploadFrame").contents().text()),r,n,f;if(u.userTypes.removeAll(),u.normalUserTypes.removeAll(),u.hasError(t.HasError),u.errorText(t.ErrorText),!u.hasError())for(r=0;r<t.Models.length;r++)n=t.Models[r],f={email:n.Email,userType:n.UserType,status:n.Status,notice:n.ErrorText,hasError:n.HasError,rawData:n.RawData,lineNumber:n.LineNumber},u.userTypes.push(f),f.hasError||u.normalUserTypes.push(f);u.isFileUploaded(!0);u.uploading(!1)};u.bindTo=function(n){ko.applyBindingsAndShow(u,n)}}n.importUserTypes=function(n,t){new r(t).bindTo(n)}}(window.app,window.OData,window.jQuery),function(n,t,i){"use strict";function r(){var r=this;r.isFileUploaded=ko.observable(!1);r.hasError=ko.observable(!1);r.errorText=ko.observable();r.userDomainConflicts=ko.observableArray();r.normalUserDomainConflicts=ko.observableArray();r.uploading=ko.observable(!1);r.getModel=function(){for(var t,u,i=[],n=0;n<r.normalUserDomainConflicts().length;n++)t=r.normalUserDomainConflicts()[n],u={Email:t.email,DomainConflicts:t.domainConflicts},i.push(u);return{UserDomainConflicts:i}};r.send=function(){var i=r.getModel(),u={requestUri:n.odata.getUrl(n.odata.entitySet.users,null,"ImportDomainConflicts"),method:"POST",data:{Request:i}};t.request(u,function(){window.location="/"+window.cmt3.conference.name+"/User/Index"})};r.downloadTemplate=function(){var t="/api/odata/"+window.cmt3.conference.name+"/Users/GetImportDomainConflictsTemplate";n.page.post(t,{})};r.uploadFile=function(n,t){t.target.value!==""&&(r.uploading(!0),t.target.form.submit())};r.parseUploadResult=function(){var t=i.parseJSON(i("#singleFileUploadFrame").contents().text()),u,n,f;if(r.userDomainConflicts.removeAll(),r.normalUserDomainConflicts.removeAll(),r.hasError(t.HasError),r.errorText(t.ErrorText),!r.hasError())for(u=0;u<t.Models.length;u++)n=t.Models[u],f={email:n.Email,domainConflicts:n.DomainConflicts,status:n.Status,notice:n.ErrorText,hasError:n.HasError,rawData:n.RawData,lineNumber:n.LineNumber},r.userDomainConflicts.push(f),f.hasError||r.normalUserDomainConflicts.push(f);r.isFileUploaded(!0);r.uploading(!1)};r.bindTo=function(n){ko.applyBindingsAndShow(r,n)}}n.importDomainConflicts=function(n){(new r).bindTo(n)}}(window.app,window.OData,window.jQuery,window.document,window.confirm,window.setTimeout),function(n,t,i){"use strict";function r(){var r=this;r.isFileUploaded=ko.observable(!1);r.hasError=ko.observable(!1);r.errorText=ko.observable();r.bids=ko.observableArray();r.normalBids=ko.observableArray();r.uploading=ko.observable(!1);r.cancel=function(){window.location="/"+window.cmt3.conference.name+"/Submission/Manage"};r.getModel=function(){for(var n,u,i=[],t=0;t<r.normalBids().length;t++)n=r.normalBids()[t],u={Email:n.email,SubmissionId:n.id,BidValue:n.bidValue},i.push(u);return{Bids:i}};r.downloadTemplate=function(){var n="/api/odata/"+window.cmt3.conference.name+"/BiddingModels/GetImportTabDelimitedTemplate";r.post(n,{})};r.send=function(){var i=r.getModel(),u={requestUri:n.odata.getUrl(n.odata.entitySet.biddings,null,"Import"),method:"POST",data:{Request:i}};t.request(u,function(){window.location="/"+window.cmt3.conference.name+"/Submission/Manage"})};r.post=function(n,t,i){var r,f,u;i=i||"post";r=document.createElement("form");r.setAttribute("method",i);r.setAttribute("action",n);for(f in t)t.hasOwnProperty(f)&&(u=document.createElement("input"),u.setAttribute("type","hidden"),u.setAttribute("name",f),u.setAttribute("value",t[f]),r.appendChild(u));document.body.appendChild(r);r.submit();document.body.removeChild(r)};r.uploadFile=function(n,t){t.target.value!=""&&(r.uploading(!0),t.target.form.submit())};r.parseUploadResult=function(){var t=i.parseJSON(i("#singleFileUploadFrame").contents().text()),u,n,f;if(r.bids.removeAll(),r.normalBids.removeAll(),r.hasError(t.HasError),r.errorText(t.ErrorText),!r.hasError())for(u=0;u<t.Models.length;u++)n=t.Models[u],f={email:n.Email,id:n.Id,bid:n.Bid,bidValue:n.BidValue,status:n.Status,hasError:n.HasError,rawData:n.RawData,lineNumber:n.LineNumber},r.bids.push(f),f.hasError||r.normalBids.push(f);r.isFileUploaded(!0);r.uploading(!1)};r.bindTo=function(n){ko.applyBindingsAndShow(r,n)}}n.importBidsFromTabDelimitedFile=function(n){(new r).bindTo(n)}}(window.app,window.OData,window.jQuery,window.document,window.confirm,window.setTimeout),function(n,t,i){"use strict";function r(r){var u=this;u.isFileUploaded=ko.observable(!1);u.hasError=ko.observable(!1);u.errorText=ko.observable();u.notes=ko.observableArray();u.normalNotes=ko.observableArray();u.uploading=ko.observable(!1);u.cancel=function(){window.location="/"+window.cmt3.conference.name+"/Submission/Manage"};u.getModel=function(){for(var t,r,i=[],n=0;n<u.normalNotes().length;n++)t=u.normalNotes()[n],r={SubmissionId:t.submissionId,Note:t.note},i.push(r);return{Notes:i}};u.downloadTemplate=function(){var t=n.odata.getUrl(n.odata.entitySet.chairNotes,null,"GetImportTabDelimitedTemplate")+"(order="+r+")";n.page.post(t,null,"GET")};u.send=function(){var i=u.getModel(),f={requestUri:n.odata.getUrl(n.odata.entitySet.chairNotes,null,"Import"),method:"POST",data:{Order:r,Request:i}};t.request(f,function(){window.location="/"+window.cmt3.conference.name+"/Submission/Manage"})};u.uploadFile=function(n,t){t.target.value!=""&&(u.uploading(!0),t.target.form.submit())};u.parseUploadResult=function(){var t=i.parseJSON(i("#singleFileUploadFrame").contents().text()),r,n,f;if(u.notes.removeAll(),u.normalNotes.removeAll(),u.hasError(t.HasError),u.errorText(t.ErrorText),!u.hasError())for(r=0;r<t.Models.length;r++)n=t.Models[r],f={submissionId:n.SubmissionId,note:n.Note,noteHtml:n.Note.htmlMultiLine(),status:n.Status,hasError:n.HasError,rawData:n.RawData,lineNumber:n.LineNumber},u.notes.push(f),f.hasError||u.normalNotes.push(f);u.isFileUploaded(!0);u.uploading(!1)};u.bindTo=function(n){ko.applyBindingsAndShow(u,n)}}n.importChairNotesFromTabDelimited=function(n,t){new r(n).bindTo(t)}}(window.app,window.OData,window.jQuery),function(n,t,i){"use strict";function u(){var t=this;t.id=n.autoMap();t.name=n.autoMap();t.firstName=n.autoMap();t.lastName=n.autoMap();t.email=n.autoMap();t.organization=n.autoMap();t.primarySubjectArea=n.autoMap();t.secondarySubjectAreas=n.autoMap();t.bid=n.autoMap();t.userType=n.autoMap();t.isAssigned=n.autoMap();t.changeBidVm=null;t.isAssignedText=ko.pureComputed(function(){return t.isAssigned?"Yes":"No"})}function r(t,i){var r=this;r.seniorMetaReviewerId=t;r.metaReviewers=ko.observableArray([]);r.track=ko.observable();r.trackChangeSubscription=null;r.userTypes=i;r.userTypesProvider=function(){return r.userTypes};n.DataTable.call(r)}function f(t,i){var r=this;r.trackId=n.autoMap();r.trackName=n.autoMap();r.biddingEnabled=n.autoMap();r.isSelected=ko.observable(i);r.selectTrack=function(){t.selectTrack(r)}}function e(i){var r=this;r.tracks=ko.observableArray();r.selectedTrack=ko.observable(null);r.selectTrack=function(n){for(var t,f=n.trackId,u=r.tracks(),i=0;i<u.length;i++)t=u[i],t.trackId===f?(t.isSelected(!0),r.selectedTrack(n)):t.isSelected(!1)};r.loadData=function(){var u=n.odata.getUrl(n.odata.entitySet.seniorMetaReviewerBiddingViews,i,"GetSeniorMetaReviewerSimpleView");return t.request({requestUri:u,showProgressIndicator:!1,method:"POST",headers:{"Content-Type":"application/json"}},function(t){var u,e,i;if(n.autoMap(r,t),u=[],t.TrackData){for(e=JSON.parse(t.TrackData),i=0;i<e.length;i++)u.push(n.autoMap(new f(r,i==0),e[i]));r.tracks(u);r.selectTrack(u[0])}})}}function o(t,i){var u=i,r=this;r.userCount=ko.observable(0);r.selectedBid=ko.observable(1);r.bidOptions=[{name:"Not Entered",id:1},{name:"Not Willing",id:2},{name:"In A Pinch",id:3},{name:"Willing",id:4},{name:"Eager",id:5}];r.submitEnabled=ko.computed(function(){return r.userCount()<=0?!1:r.selectedBid()!=null&&typeof r.selectedBid()!="undefined"});r.changeBid=function(){var i={Filter:r.filter,Bid:r.selectedBid(),UserId:u.seniorMetaReviewerId,TrackId:u.track()&&u.track().trackId},f={requestUri:n.odata.getUrl(n.odata.entitySet.seniorMetaReviewerBiddingModels,null,"BulkChangeBid"),method:"POST",showProgressIndicator:!0,data:{Request:i}};OData.request(f,function(){u.refresh();setTimeout(function(){n.addMessage("The bid for selected users have been changed.")},500);$(t).modal("hide")})};r.bind=function(){ko.applyBindings(r,t)};r.filter=null;r.editInDialog=function(i){r.filter=i;var f={Filter:i,UserId:u.seniorMetaReviewerId},e={requestUri:n.odata.getUrl(n.odata.entitySet.seniorMetaReviewerBiddingModels,null,"UserCountFilteredBidding"),method:"POST",data:{Request:f}};OData.request(e,function(n){r.userCount(n.value);r.selectedBid(null);$(t).modal("show")})}}function s(t,u,f,o){var s=this;n.showProgress();s.user=new e(t);s.table=new r(t,f);s.url=ko.pureComputed(function(){var n=s.user.selectedTrack();return n?o+"?trackId="+n.trackId:null});s.biddingEnabled=ko.pureComputed(function(){var n=s.user.selectedTrack();return n?n.biddingEnabled:!1});ko.applyBindings(s,i.getElementById(u));$.when(s.user.loadData()).then(function(){return s.table.track(s.user.selectedTrack()),s.table.loadData(!0)}).then(function(){s.table.subscribeToTrackChange();s.user.selectedTrack.subscribe(function(n){s.table.track(n)});$("#"+u).show()}).always(n.hideProgress)}r.prototype=$.extend({},n.DataTable.prototype,{getStorageKey:function(){return"SeniorMetaReviewerBidding"},getDefaultSorting:function(){return{property:"FirstName",direction:"asc"}},subscribeToTrackChange:function(){var n=this;n.trackChangeSubscription||(n.trackChangeSubscription=n.track.subscribe(n.loadData,n))},selectBid:function(n,t){var r=$(t.target),f=ko.contextFor(t.target),i=$($("#bidTemplate").text()),u;r.hide();r.after(i);u=f.$parent.getBids(n.id,r,i);ko.applyBindings(u,i[0]);i.find("select").focus()},getBids:function(t,i,r){var u=this,f=[{name:"Not Entered",id:1},{name:"Not Willing",id:2},{name:"In A Pinch",id:3},{name:"Willing",id:4},{name:"Eager",id:5}],e={options:ko.observableArray(f),selectedBid:ko.observable()};return e.selectedBid.subscribe(function(e){var o={requestUri:n.odata.getUrl(n.odata.entitySet.seniorMetaReviewerBiddingModels,t),method:"PATCH",headers:{Prefer:"return-content"},progressIndicatorTimeout:0,data:{UserId:u.seniorMetaReviewerId,BidId:e[0],TrackId:u.track().trackId}};OData.request(o,function(n){r.remove();i.text(f[n.BidId-1].name);i.show()})}),e},getFilter:function(){var i=this,n="",t;return $.each(i.filters,function(t,i){i.getValue()&&(n+=n?" and "+i.getValue():i.getValue())}),t=i.track()&&i.track().trackId,typeof t=="number"&&t>0&&(n+=(n?" and":"")+" TrackId eq "+t),n},loadData:function(i){var r,o,s;i=i===!0;r=this;i&&r.applyState();var e=r.sorting(),h=e?"&$orderby="+encodeURIComponent(e.property+" "+e.direction):"",c=r.skip()?"&$skip="+r.skip():"",l=r.top()?"&$top="+r.top():"",f=r.getFilter();return f&&(f="&$filter="+encodeURIComponent(f)),o={method:"GET",headers:{Accept:"application/json"},requestUri:n.odata.getUrl(n.odata.entitySet.seniorMetaReviewerBiddingViews,r.seniorMetaReviewerId)+"?$count=true"+f+h+c+l,showProgressIndicator:!i},s=t.request(o,function(t){var f,i,e;for(r.total(t["@odata.count"]||0),f=[],i=0;i<t.value.length;i++)e=n.autoMap(new u,t.value[i]),f.push(e);r.metaReviewers(f);r.saveState()},function(t){n.addErrorMessage(n.odata.getErrorMessage(t))}),s},bulkChangeBid:function(){var n=this,t=n.getFilter();n.changeBidVm==null&&(n.changeBidVm=new o(i.getElementById("changeBidDialog"),n),n.changeBidVm.bind());n.changeBidVm.editInDialog(t)},email:function(){var t=this,i=t.getFilter(),r="/"+window.cmt3.conference.name+"/SeniorMetaReviewer/SendEmailToMetaReviewers";n.url.navigateTo(r,{filter:i.length>0?i:null,userId:t.seniorMetaReviewerId})}});n.seniorMetaReviewerBidding=function(n,t,i,r){new s(n,t,i,r)}}(window.app,window.OData,window.document),function(n,t,i){"use strict";function u(t){function u(){f();r=i.isAssigned.subscribe(e)}function f(){r&&typeof r.dispose=="function"&&r.dispose()}function e(){i.initialState===undefined?i.initialState=i.isAssigned():o.call(i)}function o(){var r=this,e;r.isToggleInProgress(!0);e={UserId:r.id,TrackId:r.trackId};e.Type=r.isAssigned()?"Assign":"Remove";OData.request({requestUri:n.odata.getUrl(n.odata.entitySet.seniorMetaReviewerBiddingModels,t,"Assign"),method:"POST",showProgressIndicator:!1,data:{Request:e}},function(){r.isAssigned()===r.initialState?i.css(""):i.css(r.isAssigned()?"success":"error")},function(t){f();i.isAssigned(!i.isAssigned());u();n.addErrorMessage("Unable to edit assignment for '"+r.firstName+" "+r.lastName+"'. "+n.odata.getErrorMessage(t))}).always(function(){r.isToggleInProgress(!1)})}var i=this,r;i.trackId=n.autoMap();i.id=n.autoMap();i.name=n.autoMap();i.firstName=n.autoMap();i.lastName=n.autoMap();i.email=n.autoMap();i.organization=n.autoMap();i.primarySubjectArea=n.autoMap();i.secondarySubjectAreas=n.autoMap();i.bid=n.autoMap();i.assignmentsNumberWithinTrack=n.autoMap();i.isAssigned=ko.observable().autoMap();i.initialState=undefined;i.css=ko.observable("");i.isToggleInProgress=ko.observable(!1);u()}function r(t){var i=this;i.userId=t;i.showAssignedOnly=ko.observable("false");i.showAssignedOnly.subscribe(i.loadData,i);i.metaReviewers=ko.observableArray([]);i.track=ko.observable();i.trackChangeSubscription=null;n.DataTable.call(i)}function f(t,i){var r=this;r.trackId=n.autoMap();r.trackName=n.autoMap();r.primarySubjectAreas=n.autoMap();r.secondarySubjectAreas=n.autoMap();r.isSelected=ko.observable(i);r.selectTrack=function(){t.selectTrack(r)}}function e(i){var r=this;r.firstName=ko.observable().autoMap();r.lastName=ko.observable().autoMap();r.email=ko.observable().autoMap();r.organization=ko.observable().autoMap();r.tracks=ko.observableArray();r.selectedTrack=ko.observable(null);r.fullName=ko.pureComputed(function(){return r.firstName()+" "+r.lastName()});r.selectTrack=function(n){for(var t,f=n.trackId,u=r.tracks(),i=0;i<u.length;i++)t=u[i],t.trackId===f?(t.isSelected(!0),r.selectedTrack(n)):t.isSelected(!1)};r.loadData=function(){var u=n.odata.getUrl(n.odata.entitySet.seniorMetaReviewerBiddingViews,i,"GetSeniorMetaReviewerSimpleView");return t.request({requestUri:u,showProgressIndicator:!1,method:"POST",headers:{"Content-Type":"application/json"}},function(t){var u,e,i;if(n.autoMap(r,t),u=[],t.TrackData){for(e=JSON.parse(t.TrackData),i=0;i<e.length;i++)u.push(n.autoMap(new f(r,i==0),e[i]));r.tracks(u);r.selectTrack(u[0])}})}}function o(t,u){var f=this;n.showProgress();f.user=new e(t);f.table=new r(t);ko.applyBindings(f,i.getElementById(u));$.when(f.user.loadData()).then(function(){return f.table.track(f.user.selectedTrack()),f.table.loadData(!0)}).then(function(){f.table.subscribeToTrackChange();f.user.selectedTrack.subscribe(function(n){f.table.track(n)});$("#"+u).show()}).always(n.hideProgress)}r.prototype=$.extend({},n.DataTable.prototype,{getDefaultSorting:function(){return{property:"IsAssigned",direction:"desc"}},subscribeToTrackChange:function(){var n=this;n.trackChangeSubscription||(n.trackChangeSubscription=n.track.subscribe(n.loadData,n))},loadData:function(i){var r,e,s,h;i=i===!0;r=this;i&&r.applyState();var o=r.sorting(),c=o?"&$orderby="+encodeURIComponent(o.property+" "+o.direction):"",l=r.skip()?"&$skip="+r.skip():"",a=r.top()?"&$top="+r.top():"",f="";return $.each(r.filters,function(n,t){t.getValue()&&(f+=f?" and "+t.getValue():t.getValue())}),r.showAssignedOnly()==="true"&&(f+=(f?" and":"")+" IsAssigned eq true"),e=r.track()&&r.track().trackId,typeof e=="number"&&e>0&&(f+=(f?" and":"")+" TrackId eq "+e),f&&(f="&$filter="+encodeURIComponent(f)),s={method:"GET",headers:{Accept:"application/json"},requestUri:n.odata.getUrl(n.odata.entitySet.seniorMetaReviewerBiddingViews,r.userId)+"?$count=true"+f+c+l+a,showProgressIndicator:!i},h=t.request(s,function(t){var f,i,e,o;for(r.total(t["@odata.count"]||0),f=[],i=0;i<t.value.length;i++)e=t.value[i],o=n.autoMap(new u(r.userId),e),f.push(o);r.metaReviewers(f);r.saveState()},function(t){n.addErrorMessage(n.odata.getErrorMessage(t))}),h}});n.seniorMetaReviewerAssignMetaReviewers=function(n,t){new o(n,t)}}(window.app,window.OData,window.document),function(n,t,i,r,u){function o(t,u,e){function h(){var n=ko.validation.group(o.group());return n().length>0?(n.showAllMessages(),!1):!0}var o=this,s;o.group=ko.observable();o.tracks=e;o.addEditText=ko.pureComputed(function(){var n=o.group();return n&&n.groupId()?"Edit":"Add"});s=n(i.getElementById(t));o.addEditGroup=function(n){n=n&&n.constructor===f?r.autoMap(new f(u.trackId,e),n):new f(u.trackId,e);o.group(n);s.modal("show")};o.save=function(){if(h()){var t=o.group();t&&typeof t.save=="function"&&(r.showProgress(),n.when(t.save()).then(function(){return s.modal("hide"),u.show()}).always(r.hideProgress))}}}function f(n,t){var i=this;i.groupId=ko.observable(0).autoMap();i.groupName=ko.observable("").extend({required:!0}).autoMap();i.trackId=ko.observable(n>0?n:undefined).extend({required:!0,onlyIf:function(){return i.isTrackSelectionVisible()}}).autoMap();i.isImplicit=ko.observable(!1).autoMap();i.isEnabled=ko.observable(!1).autoMap();i.track=r.autoMap();i.tracks=ko.observable(t);i.numberOfMetaReviewers=r.autoMap();i.metaReviewersJson=r.autoMap();i.isTrackSelectionVisible=ko.pureComputed(function(){var t=i.groupId();return(!n||n<=0)&&(!t||t<1)});i.isImplicitText=ko.pureComputed(function(){return i.isImplicit()===!0?"Yes":"No"});i.isEnabledText=ko.pureComputed(function(){return i.isEnabled()===!0?"Yes":"No"});i.metaReviewers=ko.pureComputed(function(){return i.metaReviewersJson?JSON.parse(i.metaReviewersJson):[]});i.save=function(){var n=i.groupId(),t={method:n?"PATCH":"POST",requestUri:r.odata.getUrl(r.odata.entitySet.trackMetaReviewerGroups,n?n:null),showProgressIndicator:!1,data:{GroupName:i.groupName(),TrackId:i.trackId(),IsImplicit:i.isImplicit(),IsEnabled:i.isEnabled()}};return u.request(t)};i.remove=function(){var n={method:"DELETE",requestUri:r.odata.getUrl(r.odata.entitySet.trackMetaReviewerGroups,i.groupId()),showProgressIndicator:!1};return u.request(n)}}function e(i,u,e,s){var h,l,c,a;if(r.Page.call(this,i,r.odata.entitySet.trackMetaReviewerGroups,"key="+(e||-1)),h=this,h.trackId=e,h.createItem=function(n){return r.autoMap(new f,n)},h.addEditDialog=new o(u,h,s),h.changeTrack=function(n){var i="/"+t.cmt3.conference.name+"/User/MetaReviewerGroups";n.id>=0&&(i=i+"?trackId="+n.id);t.location=i},h.removeGroup=function(i){if(!i||i.constructor!==f||!t.confirm("Are you sure you want to remove this group?"))return!1;r.showProgress();n.when(i.remove()).then(function(){return h.show()}).always(r.hideProgress)},h.tracks=ko.observableArray(),h.selectedTrack=ko.observable(),l=null,s.length>1?(l=new r.Track,l.id=-1,l.name="<All Tracks>"):s.length>0&&(l=r.autoMap(new r.Track,s[0]),h.trackId=l.id),h.tracks.push(l),h.selectedTrack(l),s.length>1){for(c=0;c<s.length;c++)a=r.autoMap(new r.Track,s[c]),h.tracks.push(a);for(c=0;c<h.tracks().length;c++)if(h.trackId===h.tracks()[c].id){h.selectedTrack(h.tracks()[c]);break}h.selectedTrackSubscription=h.selectedTrack.subscribe(h.changeTrack)}h.trackNamesProvider=ko.pureComputed(function(){var n=[];for(var t in s)s.hasOwnProperty(t)&&n.push(s[t].name);return n})}e.prototype=Object.create(r.Page.prototype);r.metaReviewerGroupsPage=function(n,t,i,r,u){var f=new e(t,i,r,u);ko.applyBindingsAndShow(f,n);f.setDefaultSort("GroupName");f.show()}}($,window,document,window.app,window.OData),function(n,t,i){"use strict";function r(n){var i=this;n?(i.id=n.Id,i.firstName=n.FirstName,i.middleInitial=n.MiddleInitial,i.lastName=n.LastName,i.email=n.Email,i.organization=n.Organization):(i.id=t.autoMap(),i.firstName=t.autoMap(),i.middleInitial=t.autoMap(),i.lastName=t.autoMap(),i.email=t.autoMap(),i.organization=t.autoMap());i.readFromJson=function(n){return t.autoMap(i,n),i}}function u(n,r){var u=this,f,e;if(n?(u.id=n.Id,u.metaReviewerId=n.MetaReviewerId,u.firstName=n.FirstName,u.middleInitial=n.MiddleInitial,u.lastName=n.LastName,u.email=n.Email,u.organization=n.Organization,u.numberOfBids=n.NumberOfBids,u.numberOfAssignment=n.NumberOfAssignment,u.numberOfCompleted=n.NumberOfCompleted,u.percentageOfCompleted=n.PercentageOfCompleted,u.numberOfNotes=n.NumberOfNotes,u.percentageOfCompletedNote=n.PercentageOfCompletedNote,u.numberOfComparisons=n.NumberOfComparisons,u.conflictDomainsEntered=n.ConflictDomainsEntered,u.individualConflictsEntered=n.IndividualConflictsEntered,u.quota=n.Quota,u.userType=n.UserType,u.subjectAreaSelected=n.SubjectAreaSelected,u.primarySubject=n.PrimarySubject,u.secondarySubject=n.SecondarySubject,u.numberOfReviewRatings=n.NumberOfReviewRatings,u.avgReviewRating=n.AvgReviewRating,u.googleScholarId=n.GoogleScholarId,u.semanticScholarId=n.SemanticScholarId,u.dblpId=n.DblpId,u.externalProfileEntered=n.ExternalProfileEntered,u.userTagJson=n.UserTagJson):(u.id=t.autoMap(),u.firstName=t.autoMap(),u.middleInitial=t.autoMap(),u.lastName=t.autoMap(),u.email=t.autoMap(),u.organization=t.autoMap(),u.quota=n.Quota,u.numberOfBids=t.autoMap(),u.numberOfAssignment=t.autoMap(),u.numberOfCompleted=t.autoMap(),u.percentageOfCompleted=t.autoMap(),u.numberOfNotes=t.autoMap(),u.percentageOfCompletedNote=t.autoMap(),u.numberOfComparisons=t.autoMap(),u.conflictDomainsEntered=n.autoMap(),u.individualConflictsEntered=n.autoMap(),u.userType=t.autoMap(),u.subjectAreaSelected=t.autoMap(),u.primarySubject=t.autoMap(),u.secondarySubject=t.autoMap(),u.numberOfReviewRatings=t.autoMap(),u.avgReviewRating=t.autoMap(),u.googleScholarId=t.autoMap(),u.semanticScholarId=t.autoMap(),u.dblpId=t.autoMap(),u.externalProfileEntered=t.autoMap(),u.userTagJson=t.autoMap()),u.userTags=[],f=u.userTagJson&&JSON.parse(u.userTagJson),f)for(e=0;e<f.length;e++)u.userTags.push(t.autoMap(new t.UserTag,f[e]));u.googleScholarUrl=function(){return t.enums.externalProfile.googleScholar.format(u.googleScholarId)};u.semanticScholarUrl=function(){return t.enums.externalProfile.semanticScholar.format(u.semanticScholarId)};u.dblpUrl=function(){return t.enums.externalProfile.dblp.format(u.dblpId)};u.individualConflictsEnteredText=ko.pureComputed(function(){return u.individualConflictsEntered===!0?"Yes":"No"});u.readFromJson=function(n){t.autoMap(u,n)};u.exportBids=function(){var n=t.odata.getUrl("BiddingModels",null,"ExportToTabDelimitedFile"),i={UserId:u.id,TrackId:r.selectedTrackId()};t.page.post(n,i)};u.importBids=function(){window.location=r.importUrl+"?userId="+u.id};u.impersonate=function(n){if(confirm("Are you sure to impersonate as {0} {1}?".format(n.firstName,n.lastName))){var r={requestUri:t.odata.getUrl("Users",n.id,"Impersonate"),method:"POST"};i.request(r,function(n){t.odata.processRedirectResponse(n)})}};u.removeReviewer=function(n){r.removeReviewer(n)}}function f(r,u){var e=u,f=this;f.filter=null;f.userCount=ko.observable(0);f.selectedUserType=ko.observable("");f.userTypes=e.userTypes;f.submitEnabled=ko.computed(function(){return f.userCount()<=0?!1:f.selectedUserType()!==null&&typeof f.selectedUserType()!="undefined"});f.changeUserType=function(){var u={Filter:f.filter,UserTypeOptionId:f.selectedUserType(),TrackId:e.selectedTrackId()},o={requestUri:t.odata.getUrl(e.controller,null,"BulkChangeUserType"),method:"POST",showProgressIndicator:!0,data:{Request:u}};i.request(o,function(){e.refresh();setTimeout(function(){t.addMessage("The user types of selected reviewers have been changed.")},500);n(r).modal("hide")})};f.bind=function(){ko.applyBindings(f,r)};f.editInDialog=function(t){f.filter=t;var u=t?"&$filter="+encodeURIComponent(t):"";i.read({requestUri:"/api/odata/"+window.cmt3.conference.name+"/"+e.controller+"?key="+e.selectedTrackId()+"&$count=true"+u,dataType:"json"},function(t){f.userCount(t["@odata.count"]);f.selectedUserType("");n(r).modal("show")})}}function e(r,u){var e=u,f=this;f.reviewerCount=ko.observable(0);f.filter=null;f.quota=ko.observable(0).extend({digit:!0,min:0,max:9999}).extend({trackChanges:!0});f.showValidationWarning=ko.observable(!1);f.submitEnabled=ko.computed(function(){return f.reviewerCount()>0});f.changeQuota=function(){var u=!0,o=ko.validation.group(f,{deep:!0}),s,h;if(o().length>0&&(o.showAllMessages(),u=!1),!u){f.showValidationWarning(!0);return}s={Filter:f.filter,Quota:f.quota(),TrackId:e.selectedTrackId()};h={requestUri:t.odata.getUrl(t.odata.entitySet.trackReviewers,null,"BulkChangeQuota"),method:"POST",showProgressIndicator:!0,data:{Request:s}};i.request(h,function(){e.refresh();setTimeout(function(){t.addMessage("The quota of selected reviewers have been changed.")},500);n(r).modal("hide")})};f.bind=function(){ko.applyBindings(f,r)};f.editInDialog=function(t,i){f.filter=t;f.reviewerCount(i);n(r).modal("show")}}t.ReviewersStatPage=function(o,s,h,c,l,a,v,y,p,w,b){function ot(u){var f=this,e;f.id=ko.observable().autoMap();f.email=ko.observable().extend({required:!0,email:!0}).autoMap();f.firstName=ko.observable().autoMap();f.middleInitial=ko.observable().autoMap();f.lastName=ko.observable().autoMap();f.organization=ko.observable().autoMap();f.isSearching=ko.observable();f.searchedEmail=ko.observable();f.searchResult=ko.observable();e=null;f.userFound=ko.computed(function(){return f.id()>0});f.userNotFound=ko.computed(function(){return f.id()===0});f.search=function(){var n=ko.validation.group([f.email]),u;if(n().length>0){n.showAllMessages();return}f.isSearching(!0);f.searchedEmail(f.email());u={requestUri:t.odata.getGlobalUrl(t.odata.entitySet.users,null,"SearchByEmail"),method:"POST",showProgressIndicator:!1,data:{Email:f.searchedEmail()}};i.read(u,function(n){t.autoMap(f,n);f.searchResult((new r).readFromJson(n))},function(n){n.response.statusCode===404?(f.id(0),f.searchResult(null)):i.defaultError(n)}).always(function(){f.isSearching(!1)})};f.addReviewer=function(){n(u).modal("hide");var i=new r;f.userFound()?e.resolve(f.searchResult()):(i=t.autoMap(i,{}),i.email=f.searchedEmail(),e.resolve(i))};f.bind=function(){ko.applyBindings(f,u)};f.editInDialog=function(){return f.id(null),f.email(""),f.email.isModified(!1),f.firstName(""),f.lastName(""),f.organization(""),f.searchedEmail(""),n(u).modal("show"),e=n.Deferred(),e.promise()}}function st(n,t){var i=t;return n!==null&&n.length>0&&(isNaN(n)||(i=parseInt(n))),i}function ht(n){return n.Name}function ft(n,r){var f=function(n){return{Role:"Reviewer",ObjectId:n,ObjectType:"Track"}},u={},e;return r?(u.Add=[f(g)],u.Remove=[]):(u.Add=[],u.Remove=[f(g)]),e={requestUri:t.odata.getUrl(t.odata.entitySet.users,n,"ModifyPermissions"),method:"POST",data:{Request:u}},i.request(e,function(){})}var k=this,g=st(h,null),nt,tt,ut,it,d,et,rt;for(g===null?t.Page.call(k,o,s,"key=-1"):t.Page.call(k,o,s,"key="+g),k.importUrl=c,k.requireConflictDomains=v,k.requireIndividualConflict=y,k.allowMetaReviewerToRateReview=p,k.allowReviewerToCompareSubmission=w,k.userTypes=b,k.userTypesProvider=function(){return k.userTypes.map(ht)},nt=null,k.changeQuota=function(n,t){nt===null&&(nt=new e(document.getElementById("changeQuotaDialog"),k),nt.bind());nt.editInDialog(n,t)},k.bulkChangeQuota=function(n,i){var r=i.target,u=ko.contextFor(r),f=t.GetEventFilter(i);k.changeQuota(f,u.$root.Pager().TotalItemCount())},tt=null,k.openAddReviewerDialog=function(){tt===null&&(tt=new ot(document.getElementById("userSearchDialog")),tt.bind());tt.editInDialog().done(function(i){var u,r;i.id?u=ft(i.id,!0):(r=n.Deferred(),n.when(createUser(i)).then(function(n){i=n;ft(n.id,!0).done(r.resolve).fail(r.reject)}),u=r.promise());u.done(function(){k.show();t.addMessage("User '{0} {1}' saved.".format(i.firstName,i.lastName))})})},k.removeReviewer=function(n){var i="Are you sure you want to remove reviewer {0} {1}".format(n.firstName,n.lastName);n.numberOfAssignment>0&&(i+=" who is assigned to {0} paper{1}".format(n.numberOfAssignment,n.numberOfAssignment>1?"s":""),n.numberOfCompleted>0&&(i+=" and has submitted {0} review{1}".format(n.numberOfCompleted,n.numberOfCompleted>1?"s":"")));i+="?";confirm(i)&&ft(n.id,!1).done(function(){k.show();t.addMessage("Reviewer has been successfully removed.")})},k.trackId=g,k.createItem=function(n){return new u(n,k)},k.changeTrack=function(n){var t="/"+window.cmt3.conference.name+"/User/Reviewers";n.id>=0&&(t=t+"?trackId="+n.id);window.location=t},k.tracks=ko.observableArray(),k.selectedTrack=ko.observable(),k.isTrackSelectionVisible=ko.pureComputed(function(){return a===t.enums.reviewersStatPageMode.chair?k.tracks().length>2:k.tracks().length>1}),k.selectedTrackId=ko.pureComputed(function(){var t=k.selectedTrack(),n;return t&&t.id>0?t.id:(n=k.tracks(),n=n&&n.filter(function(n){return n.id>0}),n&&n.length===1)?n[0].id:-1}),k.exportReviewers=function(n,i){var r=t.GetEventFilter(i),u=t.odata.getUrl("TrackReviewers",null,"ExportTrackReviewers"),f={TrackId:k.selectedTrackId(),Filter:r};t.page.post(u,f)},k.exportReviewerQuotas=function(){var n="/api/odata/"+window.cmt3.conference.name+"/Users/ExportUserQuotas",i={TrackId:k.selectedTrackId(),ForReviewer:!0};t.page.post(n,i)},k.exportReviewerSubjectAreas=function(){var n="/api/odata/"+window.cmt3.conference.name+"/Users/ExportUserSubjectAreas",i={TrackId:k.selectedTrackId(),ForReviewer:!0,ForSeniorMetaReviewer:!1};t.page.post(n,i)},k.exportReviewerRelevances=function(){var n="/api/odata/"+window.cmt3.conference.name+"/Users/ExportUserRelevances",i={TrackId:k.selectedTrackId(),ForReviewer:!0};t.page.post(n,i)},k.importUserQuotas=function(){var n="/"+window.cmt3.conference.name+"/Reviewer/ImportQuotas";t.url.navigateTo(n,{trackId:k.trackId})},k.importUserTypes=function(){var n="/"+window.cmt3.conference.name+"/User/ImportUserTypes";t.url.navigateTo(n,{roleValue:2})},k.importUserTags=function(){var n="/"+window.cmt3.conference.name+"/User/ImportUserTags";t.url.navigateTo(n,{roleValue:2})},ut=[],a===t.enums.reviewersStatPageMode.chair&&(it=new t.Track,it.id=-1,it.name="<All Tracks>",ut.push(it),k.selectedTrack(it)),d=0;d<l.length;d++)et=t.autoMap(new t.Track,l[d]),ut.push(et);for(k.tracks(ut),d=0;d<k.tracks().length;d++)if(k.trackId===k.tracks()[d].id){k.selectedTrack(k.tracks()[d]);break}k.refresh=function(){k.show()};k.selectedTrackSubscription=k.selectedTrack.subscribe(k.changeTrack);k.users=ko.observableArray();k.email=function(n,i){var r=t.GetEventFilter(i),u="/"+window.cmt3.conference.name+"/Reviewer/SendEmail";t.url.navigateTo(u,{filter:r.length>0?r:null,trackId:k.trackId<0?null:k.trackId})};k.show=function(){t.Page.prototype.show.call(k)};k.bulkChangeUserType=function(n,i){var r=t.GetEventFilter(i);this.changeUserType(r)};rt=null;k.changeUserType=function(n){rt===null&&(rt=new f(document.getElementById("changeUserTypeDialog"),k),rt.bind());rt.editInDialog(n)}};t.ReviewersStatPage.prototype=Object.create(t.Page.prototype)}(window.jQuery,window.app,window.OData),function(n,t,i,r,u,f,e,o){"use strict";function h(){var t=this;t.id=n.autoMap();t.originalName=n.autoMap();t.size=n.autoMap();t.formattedSize=n.autoMap();t.uploadDate=n.autoMap();t.downloadLink=n.autoMap()}function c(n,t,i,r,u){var f=this;f.id=n;f.title=t;f.trackId=i;f.trackName=r;f.isSingleTrackConference=u}function l(l,a,v,y,p,w,b){function d(){function a(){var u=r.stringify(e.getAnswersJson(k.questions)),i,f;if(k.lastDraft===u){k.setAutoSaveTimer();return}i=n.autoMap(k);i.SubmissionId=k.submission.id;i.Id=k.draftId||0;i.Draft=r.stringify(e.getAnswersJson(k.questions));f={requestUri:n.odata.getUrl(n.odata.entitySet.authorFeedbackDrafts),method:"POST",headers:{Prefer:"return-content"},showProgressIndicator:!1,data:i};t.request(f,function(n){k.draftId=n.Id;k.lastDraftErrorDate(null);k.lastDraftDate((new Date).toLocaleString());k.lastDraft=u},function(){k.lastDraftErrorDate((new Date).toLocaleString())}).always(k.setAutoSaveTimer)}function v(){var n=!0;return k.files().length>k.settings.authorFeedbackMaxFileNumber&&(k.showFilesMaxErrorMessage(!0),n=!1),k.files().length<k.settings.authorFeedbackMinFileNumber&&(k.showFilesMinErrorMessage(!0),n=!1),n}function c(t){var e,r,f,u;if(k.files().length+t.length>k.settings.authorFeedbackMaxFileNumber){n.addMessage("You can upload up to {0} files only.".format(k.settings.authorFeedbackMaxFileNumber),null,"error");return}for(e=[],r=0;r<k.files().length;r++)e[k.files()[r].originalName.toLowerCase()]=!0;for(r=0;r<t.length;r++)f=t[r],y(f,e)&&(k.uploading(k.uploading()+1),u=i.ajaxSettings.xhr(),u.open("POST",s.fileUpload,!0),u.setRequestHeader("Accept","application/json"),u.setRequestHeader("File-Name",encodeURIComponent(f.name)),u.send(f),u.addEventListener("load",function(t){t.target.status==200?l(t.target.responseText):n.processXmlHttpRequestError(t.target);k.uploading(k.uploading()-1)},!1))}function y(t,i){var u=t.name.toLowerCase(),r;if(i[u]===undefined)i[u]=!0;else return n.addMessage("Found at least two files with the same name: '{0}'.".format(t.name),null,"error"),!1;if(t.size>k.settings.authorFeedbackMaxFileSize*1048576)return n.addMessage("File '{0}' is bigger than maximum allowed size of {1} Mb.".format(t.name,k.settings.authorFeedbackMaxFileSize),null,"error"),!1;var f=t.name.substr(t.name.lastIndexOf(".")+1).toLowerCase(),e=k.settings.authorFeedbackAllowedFileTypes.split(","),o=!1;for(r=0;r<e.length;r++)if(e[r].trim().toLowerCase()==f){o=!0;break}return o?!0:(n.addMessage("File '{0}' has type '{1}' which is not accepted. We accept '{2}' only.".format(t.name,f,k.settings.authorFeedbackAllowedFileTypes),null,"error"),!1)}function l(t){var r,i;try{r=ko.utils.parseJson(t)}catch(u){n.processException(u);return}i=n.autoMap(new h,r);i.uploadDate=new Date(i.uploadDate);isNaN(i.uploadDate)&&(i.uploadDate=new Date);k.files.push(i)}k.showFilesMinErrorMessage=ko.observable(!1);k.showFilesMaxErrorMessage=ko.observable(!1);k.questions=[];k.submittedAnswersJson=null;k.autoSaveTimerId=null;k.draftId=null;k.loadedDraftDate=ko.observable();k.lastDraftDate=ko.observable();k.lastDraftErrorDate=ko.observable(null);k.lastDraft=null;k.setAutoSaveTimer=function(){return k.autoSaveTimerId&&f(k.autoSaveTimerId),k.autoSaveTimerId=u(a,n.settings.autoSaveDelay),!0};k.revertDraft=function(){it();k.submittedAnswersJson!=null&&(e.unsubscribeAnswerChanged(k.questions),e.setAnswersFromJson(k.questions,k.submittedAnswersJson),e.subscribeAnswerChanged(k.questions,k.setAutoSaveTimer));k.loadedDraftDate(null)};k.files=ko.observableArray();k.removeFile=function(n){k.files.remove(n)};k.uploading=ko.observable(0);k.uploadFile=function(){var n=i('<input type="file" accept="*" multiple="" />');n.on("change",function(){c(this.files)});n.trigger("click")};k.canUploadMoreFiles=ko.computed({read:function(){return k.uploading()==0&&k.files().length<k.settings.authorFeedbackMaxFileNumber},deferEvaluation:!0});k.xhrUploadSupported=function(){return o};k.fileUploadDragOver=function(n,t){k.canUploadMoreFiles()&&i(t.target).addClass("dragOver")};k.fileUploadDragLeave=function(n,t){k.canUploadMoreFiles()&&i(t.target).removeClass("dragOver")};k.fileUploadDrop=function(n,t){if(k.canUploadMoreFiles()){var i=t.originalEvent.dataTransfer.files;c(i);k.fileUploadDragLeave(n,t)}};k.uploadSingleFile=function(n,t){t.target.value!=""&&t.target.form.submit()};k.parseSingleUploadResult=function(n,t){l(t.target.contentDocument.body.innerText)};k.save=function(){var f=!0,o=ko.validation.group(k.questions,{deep:!0}),r,u,h;if(o().length>0&&(o.showAllMessages(),f=!1),v()||(f=!1),f){for(r=n.autoMap(k),r.SubmissionId=k.submission.id,k.createNew||(r.Id=k.id),r.Files=[],u=0;u<k.files().length;u++)r.Files.push(k.files()[u].id);r.Answers=e.getAnswersJson(k.questions);h={requestUri:n.odata.getUrl(n.odata.entitySet.authorFeedbacks,k.createNew?null:k.id),method:k.createNew?"POST":"PUT",progressIndicatorTimeout:0,data:r};i.when(t.request(h,function(){}),it()).done(function(){n.url.navigateTo(s.submissionList)})}}}function rt(r){return i.Deferred(function(i){if(r.length==0){i.resolve();return}var u=n.odata.getUrl(n.odata.entitySet.files,{filter:n.odata.buildContainsQuery("Id",r)});t.read({requestUri:u,showProgressIndicator:!1},function(t){for(var u=[],r=0;r<t.value.length;r++)u.push(n.autoMap(new h,t.value[r]));k.files(u);i.resolve()})}).promise()}function g(){return i.Deferred(function(i){var r=n.odata.getUrl(n.odata.entitySet.authorFeedbackSettings,k.submission.trackId);t.read({requestUri:r,showProgressIndicator:!1},function(t){n.autoMap(k.settings,t);i.resolve()})}).promise()}function nt(){return i.Deferred(function(t){e.loadQuestionsDirect(n.enums.formType.authorfeedback,k.formId).done(function(n){k.questions=n;t.resolve()})}).promise()}function tt(){return i.Deferred(function(i){var u=n.odata.getUrl(n.odata.entitySet.authorFeedbackDrafts,null,"GetBySubmissionId");t.read({requestUri:u,showProgressIndicator:!1,data:{Id:k.submission.id},method:"POST"},function(n){if(!n){i.resolve(!1);return}k.loadedDraftDate(n.UpdateDate.toLocaleString());k.draftId=n.Id;var t=r.parse(n.Draft);e.setAnswersFromJson(k.questions,t);i.resolve(!0)},function(n){if(n.response.statusCode==404){i.resolve(!1);return}t.defaultError(n)})}).promise()}function ut(){return i.Deferred(function(r){var u=n.odata.getUrl(n.odata.entitySet.authorFeedbacks,k.id);t.read({requestUri:u,showProgressIndicator:!1},function(t){n.autoMap(k,t);d();i.when(g(),rt(t.Files),nt()).done(function(){tt().done(function(n){n?k.submittedAnswersJson=t.Answers:e.setAnswersFromJson(k.questions,t.Answers);r.resolve()})})})}).promise()}function it(){if(!k.draftId)return i.Deferred().resolve().promise();var u={requestUri:n.odata.getUrl(n.odata.entitySet.authorFeedbackDrafts,k.draftId),method:"DELETE",showProgressIndicator:!1};return t.request(u,function(){k.draftId=null;k.lastDraftDate(null);k.lastDraftErrorDate(null);k.lastDraft=r.stringify(e.getAnswersJson(k.questions))})}var k=this;k.id=l;k.formId=w;k.updateDate=n.autoMap();k.settings={requestAllPapersForFeedback:n.autoMap(),authorFeedbackMinFileNumber:n.autoMap(),authorFeedbackMaxFileNumber:n.autoMap(),authorFeedbackAllowedFileTypes:n.autoMap(),authorFeedbackMaxFileSize:n.autoMap()};k.submission=new c(a,v,y,p,b);k.createNew=!k.id;k.bindTo=function(t){n.showProgress();var f=i.Deferred(),u;k.createNew?(n.autoMap(k,{}),u=i.Deferred(),d(),i.when(g(),nt()).done(function(){tt().done(function(){u.resolve()})})):u=ut();u.promise().done(function(){ko.applyBindingsAndShow(k,t);k.lastDraft=r.stringify(e.getAnswersJson(k.questions));k.setAutoSaveTimer();f.resolve()});f.always(n.hideProgress)}}var s;n.authorFeedbackDetails=function(n,t,i,r,u,f,e,o,h){s=o;new l(n,t,i,r,u,f,e).bindTo(h)}}(window.app,window.OData,window.jQuery,window.JSON,window.setTimeout,window.clearTimeout,new window.app.QuestionService,window.FileReader!=undefined),function(n,t,i){"use strict";function r(n){var i=$("#"+n),t=$.Deferred();i.find(".btn-primary").off("click").click(function(){t.resolve(!0);t=null;i.modal("hide")});i.on("hidden",function(){t&&t.resolve(!1)});return i.modal("show"),t.promise()}function u(){var t=this;t.id=n.autoMap();t.originalName=n.autoMap();t.size=n.autoMap();t.formattedSize=n.autoMap();t.uploadDate=n.autoMap();t.downloadLink=n.autoMap()}function f(){var t=this;t.order=n.autoMap();t.details=n.autoMap();t.answers=[]}function e(){var t=this;t.text=n.autoMap();t.value=n.autoMap()}function o(i,u,f){var e=this;e.isReplyAvailable=n.autoMap();e.comments=ko.observableArray();e.isReplying=ko.observable(!1);e.lastCommentId=ko.observable(null).autoMap();e.replyBody=ko.observable("");e.post=function(){r(u).done(function(r){if(!r){n.addMessage("NOTE: Posting was not successful.",null,"info");return}n.showProgress();var u={requestUri:n.odata.getUrl(n.odata.entitySet.authorFeedbackComments),showProgressIndicator:!1,headers:{"Content-Type":"application/json"},method:"POST",data:{SubmissionId:i,ReplyTo:e.lastCommentId(),Body:e.replyBody()}};t.request(u,function(){n.addMessage("Post successfully saved.");(f&&f()||$.Deferred(function(n){n.resolve()}).promise()).always(function(){n.hideProgress();e.isReplying(!1);e.replyBody("")})}).fail(n.hideProgress)})}}function s(){var t=this;t.title=n.autoMap();t.text=n.autoMap();t.submitterLabel=n.autoMap();t.posted=ko.observable().autoMap();t.postedFormatted=ko.pureComputed(function(){return t.posted().toLocaleString()})}function h(h,c){function a(i){return t.read({requestUri:n.odata.getUrl(n.odata.entitySet.authorFeedbackViews,l.id),showProgressIndicator:i},function(t){var i,h,y,w,b,v,p,r;for(n.autoMap(l,t),i=0;i<t.Questions.length;i++){for(h=t.Questions[i],y=n.autoMap(new f,h),r=0;r<h.Answers.length;r++)y.answers.push(n.autoMap(new e,h.Answers[r]));l.questions.push(y)}for(i=0;i<t.Files.length;i++)w=t.Files[i],b=n.autoMap(new u,w),l.files.push(b);for(l.commentThreads([]),i=0;i<t.CommentThreads.length;i++){for(v=t.CommentThreads[i],p=n.autoMap(new o(l.submissionId,c,a),v),r=0;r<v.Comments.length;r++)p.comments.push(n.autoMap(new s,v.Comments[r]));l.commentThreads.push(p)}})}var l=this;l.id=h;l.trackName=n.autoMap();l.submissionTitle=n.autoMap();l.submissionId=n.autoMap();l.isSingleTrackConference=n.autoMap();l.isCommentingEnabled=ko.observable(!1).autoMap();l.isCommentingAvailable=ko.observable(!1).autoMap();l.isCommenting=ko.observable(!1);l.newCommentTitle=ko.observable("");l.newCommentText=ko.observable("");l.commentThreads=ko.observableArray();l.questions=[];l.files=[];l.print=function(){i()};l.postNewComment=function(){r(c).done(function(i){if(!i){n.addMessage("NOTE: Posting was not successful.",null,"info");return}n.showProgress();var r={requestUri:n.odata.getUrl(n.odata.entitySet.authorFeedbackComments),showProgressIndicator:!1,headers:{"Content-Type":"application/json"},method:"POST",data:{SubmissionId:l.submissionId,Title:l.newCommentTitle(),Body:l.newCommentText()}};t.request(r,function(){n.addMessage("Post successfully saved.");a(!1).always(function(){n.hideProgress();l.isCommenting(!1);l.newCommentTitle("");l.newCommentText("")})}).fail(n.hideProgress)})};l.bindTo=function(n){a(!0).done(function(){ko.applyBindingsAndShow(l,n)})}}n.authorFeedbackView=function(n,t,i){new h(n,i).bindTo(t)}}(window.app,window.OData,window.print),function(n,t,i,r,u,f,e){"use strict";function s(n,t,i,r,u){var f=this;f.id=n;f.title=t;f.trackId=i;f.trackName=r;f.isSingleTrackConference=u}function h(r,u,f,h,c,l,a){function y(){v.questions=[];v.submittedAnswersJson=null;v.save=function(){var u=!0,f=ko.validation.group(v.questions,{deep:!0}),r,s;(f().length>0&&(f.showAllMessages(),u=!1),u)&&(r=n.autoMap(v),r.SubmissionId=v.submission.id,v.createNew||(r.Id=v.id),r.Answers=e.getAnswersJson(v.questions),s={requestUri:n.odata.getUrl(n.odata.entitySet.chairNotes,v.createNew?null:v.id),method:v.createNew?"POST":"PUT",progressIndicatorTimeout:0,data:r},i.when(t.request(s,function(){})).done(function(){n.url.navigateTo(o.submissionList)}))}}function p(){return i.Deferred(function(t){e.loadQuestionsDirect(n.enums.formType.chairnote,v.formId).done(function(n){v.questions=n;t.resolve()})}).promise()}function w(){return i.Deferred(function(r){var u=n.odata.getUrl(n.odata.entitySet.chairNotes,v.id);t.read({requestUri:u,showProgressIndicator:!1},function(t){n.autoMap(v,t);y();i.when(p()).done(function(){e.setAnswersFromJson(v.questions,t.Answers);r.resolve()})})}).promise()}var v=this;v.id=r;v.formId=l;v.submission=new s(u,f,h,c,a);v.createNew=!v.id;v.bindTo=function(t){n.showProgress();var u=i.Deferred(),r;v.createNew?(r=i.Deferred(),y(),i.when(p()).done(function(){r.resolve()})):r=w();r.promise().done(function(){ko.applyBindingsAndShow(v,t);u.resolve()});u.always(n.hideProgress)}}var o;n.chairNoteDetails=function(n,t,i,r,u,f,e,s,c){o=s;new h(n,t,i,r,u,f,e).bindTo(c)}}(window.app,window.OData,window.jQuery,window.JSON,window.setTimeout,window.clearTimeout,new window.app.QuestionService),function(n,t,i){"use strict";function r(){var t=this;t.details=n.autoMap();t.answers=[]}function u(){var t=this;t.text=n.autoMap();t.value=n.autoMap()}function f(f){function o(){return t.read(n.odata.getUrl(n.odata.entitySet.chairNoteViews,e.id),function(t){var i,f,s,o;for(n.autoMap(e,t),i=0;i<t.Questions.length;i++){for(f=t.Questions[i],s=n.autoMap(new r,f),o=0;o<f.Answers.length;o++)s.answers.push(n.autoMap(new u,f.Answers[o]));e.questions.push(s)}})}var e=this;e.id=f;e.trackName=n.autoMap();e.submissionTitle=n.autoMap();e.submissionId=n.autoMap();e.isSingleTrackConference=n.autoMap();e.questions=[];e.print=function(){i()};e.bindTo=function(n){o().done(function(){ko.applyBindingsAndShow(e,n)})}}n.chairNoteView=function(n,t){new f(n).bindTo(t)}}(window.app,window.OData,window.print),function(n,t,i,r,u){"use strict";function o(n){if(!n||!n.toLowerCase().startsWith("https://scholar.google.com/citations"))return null;try{var i=new URL(n),t=i.searchParams.get("user");return e.test(t)&&t}catch(r){return null}}function h(n){var t=n.replace(/^(?:https:\/\/www.semanticscholar.org\/author\/)?(?:.*\/)?([1-9]\d*)$/gi,"$1");return s.test(t)&&t}function l(n){var t=n&&n.toLowerCase(),i;return!t||!t.startsWith("https://dblp.org/pid")&&!t.startsWith("https://dblp.uni-trier.de/")?null:(i=n.replace(/^https:\/\/((dblp.org)|(dblp.uni-trier.de))\/pid\//,""),c.test(i)&&i)}function f(n){var t=this;t.title=ko.observable();t.steps=ko.observableArray();t.successNote=ko.observable();t.openIdLinkFieldLabel=ko.observable();t.openIdLink=ko.observable();t.openId=ko.observable();t.apply=function(){n(t.openId())};t.isError=ko.observable(!1);t.getId=function(){t.isError(!1);t.openId(null);var n=t.extractOpenId(t.openIdLink());n?t.openId(n):t.isError(!0)}}function a(n){var t=this;f.call(t,n);t.title("Google Scholar Id");t.openIdLinkFieldLabel("Google Scholar Id Link");t.steps(['Type "your name google scholar" into search engine to find your Google Scholar Id link.','Copy the link into the box below and click "Get Id".','Click "Use this Id".']);this.extractOpenId=o}function v(n){var t=this;f.call(t,n);t.title("Semantic Scholar Id");t.openIdLinkFieldLabel("Semantic Scholar Id Link");t.steps(['Type "your name semantic scholar" into search engine to find your Semantic Scholar link.','Copy the link into the box below and click "Get Id".','Click "Use this Id".']);t.successNote('After claiming your Semantic Scholar profile, you can edit the profile to add or remove papers&nbsp;(<a href="https://www.semanticscholar.org/faq#author-claim" target="_blank">learn more<\/a>).');this.extractOpenId=h}function y(n){var t=this;f.call(t,n);t.title("DBLP Id");t.openIdLinkFieldLabel("DBLP Persistent URL Link");t.steps(['Go to the DBLP page <a href="https://dblp.org/" target="_blank">https://dblp.org/<\/a> or <a href="https://dblp.uni-trier.de/" target="_blank">https://dblp.uni-trier.de/<\/a>.','Type your name in dblp search box to find your page under "Home > Persons".','In "share bibliography" dropdown next to your name, find your persistent URL.<br /><img src="https://cmt3.research.microsoft.com/docs/help/general/images/external-profile/external-profile-dblp-share-icon.png" alt="find a persistent URL in share bibliography dropdown menu, next to your name" />','Copy the persistent URL into the box below and click "Get Id".','Click "Use this Id".']);this.extractOpenId=l}function p(n,t,i){var r=this;r.firstName=n;r.lastName=t;r.email=i;r.fullName=ko.pureComputed(function(){return r.firstName+" "+r.lastName})}function w(){var t=this;t.id=n.autoMap();t.name=n.autoMap();t.parentSubjectAreaId=n.autoMap();t.isChild=function(){return t.parentSubjectAreaId!==null};t.isPrimary=ko.observable();t.isSecondary=ko.observable();t.checkBoxId=function(){return"primary"+t.id};t.allowParentSelection=!0;t.specialType=null}function b(f,b,k,d,g,nt,tt,it){function ot(){function i(){var t=[],i,n,r;if(rt.publicationUrlsMultiLine())for(i=rt.publicationUrlsMultiLine().split(/[\r\n]+/),n=0;n<i.length;n++)r=i[n].trim(),r&&t.push(r);return t.length>0?JSON.stringify(t):null}function u(){var r,t,n,i;if(rt.publicationUrlsMultiLine())for(r=new RegExp("^(https?:\\/\\/)?((([a-z\\d]([a-z\\d-]*[a-z\\d])*)\\.?)+[a-z]{2,})(\\:\\d+)?(\\/[-a-z\\d%_.~+]*)*(\\?[;&amp;a-z\\d%_.~+=-]*)?(\\#[-a-z\\d_]*)?$","i"),t=rt.publicationUrlsMultiLine().split(/[\r\n]+/),n=0;n<t.length;n++)if(i=t[n].trim(),i&&!r.test(i))return rt.showPublicationUrlsErrorMessage(!0),!1;return!0}function f(){var i,r,n,t,u;if(rt.subjectAreas.length===0)return!0;for(i=[],r=!1,n=0;n<rt.subjectAreas.length;n++)(rt.subjectAreas[n].specialType==="customPrimary"||rt.subjectAreas[n].specialType==="customSecondary")&&i.push(rt.subjectAreas[n].customValue),rt.subjectAreas[n].isPrimary()&&(r=!0);return t=!0,u=ko.validation.group(i),u().length>0&&(u.showAllMessages(),t=!1),r||(rt.showSubjectAreasErrorMessage(!0),t=!1),t}rt.showValidationWarning=ko.observable(!1);rt.subjectAreas=[];rt.subjectAreaPairs=function(){return n.computeSubjectAreaColumnPairs(rt.subjectAreas)};rt.showPublicationUrlsErrorMessage=ko.observable(!1);rt.showSubjectAreasErrorMessage=ko.observable(!1);rt.questions=[];rt.save=function(){var w=ko.validation.group(rt),s,l,h,a,v,e,c,o,y,p;if(w().length>0){rt.showValidationWarning(!0);return}for(s=!0,u()||(s=!1),f()||(s=!1),l=[],h=0;h<rt.questions.length;h++)a=rt.questions[h],ut.isHidden(a.id)||l.push(a);if(v=ko.validation.group(l,{deep:!0}),v().length>0&&(v.showAllMessages(),s=!1),!s){rt.showValidationWarning(!0);return}for(e=n.autoMap(rt),e.UserId=rt.userId,rt.createNew||(e.Id=rt.id),e.SubjectAreas=[],c=0;c<rt.subjectAreas.length;c++)o=rt.subjectAreas[c],(o.isPrimary()||o.isSecondary())&&o.specialType===null&&(y={SubjectAreaId:o.id,IsPrimary:o.isPrimary()},e.SubjectAreas.push(y));e.Answers=r.getAnswersJson(rt.questions.filter(n=>!ut.isHidden(n.id)));e.PublicationUrls=i();delete e.PublicationUrlsMultiLine;p={requestUri:n.odata.getUrl(n.odata.entitySet.userInformationModels,rt.createNew?null:rt.id),method:rt.createNew?"POST":"PUT",progressIndicatorTimeout:0,data:e};t.request(p,function(){n.addMessage("User information saved.",null,"success","text",!0);tt?window.location=tt:window.location.reload()},t.defaultError)}}function et(t){return i.Deferred(function(i){rt.questions=r.parseQuestionsDirect(n.enums.formType.userinformation,t);ut.loadQuestions(rt.questions);i.resolve()}).promise()}function st(){return i.Deferred(function(i){var r=n.odata.getUrl(n.odata.entitySet.userInformationModels,rt.id);t.read({requestUri:r,showProgressIndicator:!1},function(t){if(n.autoMap(rt,t),t.PublicationUrls){var r=JSON.parse(t.PublicationUrls);rt.publicationUrlsMultiLine(r.join("\r\n"))}i.resolve(t)})}).promise()}function ht(t){function f(n){n.isPrimary.subscribe(function(n){n&&(rt.showSubjectAreasErrorMessage(!1),e(this),this.isSecondary(!1))},n);n.isSecondary.subscribe(function(n){var t,i;if(n){if(rt.settings.secondarySubjectAreaLimited&&(t=o(),t>rt.settings.secondarySubjectAreaMaxNumber)){i=this;setTimeout(function(){i.isSecondary(!1)},0);return}this.isPrimary(!1)}},n);rt.subjectAreas.push(n)}function e(n){for(var t=0;t<rt.subjectAreas.length;t++)rt.subjectAreas[t].isPrimary()&&rt.subjectAreas[t]!==n&&rt.subjectAreas[t].isPrimary(!1)}function o(){for(var t=0,n=0;n<rt.subjectAreas.length;n++)rt.subjectAreas[n].isSecondary()&&++t;return t}for(var i=null,r,u=0;u<t.length;u++)r=n.autoMap(new w,t[u]),i!==null&&i.id===r.parentSubjectAreaId&&!rt.settings.immediateParentSelectionAllowed&&i.allowParentSelection&&(i.allowParentSelection=!1),r.parentSubjectAreaId===null&&(i=r),f(r)}var rt=this,ut=new n.QuestionDependency(rt),ft;rt.id=f;rt.userId=b.UserId;rt.formId=k;rt.openIdHelper=ko.observable();rt.showOpenIdHelper=function(n,t){function e(t){n(t);i(f).modal("hide")}var f=u.getElementById(it),r;if(f){r=null;switch(t){case"GoogleScholarId":r=new a(e);break;case"SemanticScholarId":r=new v(e);break;case"DblpId":r=new y(e)}rt.openIdHelper(r);i(f).modal("show")}};rt.googleScholarId=ko.observable("").extend({pattern:e,maxLength:12,notify:"always"}).autoMap();rt.googleScholarIdFormatted=ko.computed({read:function(){return rt.googleScholarId()},write:function(n){rt.googleScholarId(o(n)||n)},owner:rt}).extend({notify:"always"});rt.googleScholarIdLink=ko.pureComputed(function(){return"https://scholar.google.com/citations?user="+rt.googleScholarId()});rt.googleScholarIdFormatted(b.GoogleScholarId);rt.semanticScholarId=ko.observable("").extend({pattern:s,maxLength:12,notify:"always"}).autoMap();rt.semanticScholarIdFormatted=ko.computed({read:function(){return rt.semanticScholarId()},write:function(n){rt.semanticScholarId(h(n)||n)},owner:rt}).extend({notify:"always"});rt.semanticScholarIdLink=ko.pureComputed(function(){return"https://www.semanticscholar.org/author/"+rt.semanticScholarId()});rt.semanticScholarIdFormatted(b.SemanticScholarId);rt.dblpId=ko.observable("").extend({pattern:c,maxLength:50,notify:"always"}).autoMap();rt.dblpIdFormatted=ko.computed({read:function(){return rt.dblpId()},write:function(n){rt.dblpId(l(n)||n)},owner:rt}).extend({notify:"always"});rt.dblpIdLink=ko.pureComputed(function(){return"https://dblp.org/pid/"+rt.dblpId()});rt.dblpIdFormatted(b.DblpId);rt.publicationEmails=ko.observable("").extend({maxLength:500}).autoMap();rt.publicationEmails(b.PublicationEmails);rt.publicationUrlsMultiLine=ko.observable("").extend({maxLength:8e3}).autoMap();b.PublicationUrls&&(ft=JSON.parse(b.PublicationUrls),rt.publicationUrlsMultiLine(ft.join("\r\n")));rt.settings={trackId:n.autoMap(),secondarySubjectAreaAllowed:n.autoMap(),secondarySubjectAreaLimited:n.autoMap(),secondarySubjectAreaMaxNumber:n.autoMap(),immediateParentSelectionAllowed:n.autoMap()};n.autoMap(rt.settings,d);rt.user=new p(b.FirstName,b.LastName,b.Email);rt.createNew=!rt.id;rt.hasBranchingQuestions=function(){return ut.hasDependency()};rt.getQuestionDiv=function(n){return i("#uiq_"+n)};rt.bindTo=function(t){n.showProgress();ot();ht(g);var f=i.Deferred(),u;rt.createNew?(u=i.Deferred(),i.when(et(nt)).done(function(){u.resolve()})):(u=i.Deferred(),i.when(st(),et(nt)).done(function(n){var f,t,i,e;for(r.setAnswersFromJson(rt.questions,n.Answers),f={},t=0;t<n.SubjectAreas.length;t++)i=n.SubjectAreas[t],f[i.SubjectAreaId]=i.IsPrimary;for(t=0;t<rt.subjectAreas.length;t++)i=rt.subjectAreas[t],e=f[i.id],e?i.isPrimary(!0):e===!1&&i.isSecondary(!0);u.resolve()}));u.promise().done(function(){ko.applyBindingsAndShow(rt,t);ut.init();f.resolve()});f.always(n.hideProgress)}}var e=/^[-_0-9A-Za-z]{12}$/,s=/^[1-9]\d*$/,c=/^\d{2,3}\/\d+(-\d+)?|[a-z]\/[a-zA-Z][0-9A-Za-z]*(-\d+)?$/;n.userInformationDetails=function(n,t,i,r,u,f,e,o,s){new b(n,t,i,r,u,f,e,o).bindTo(s)}}(window.app,window.OData,window.jQuery,new window.app.QuestionService,document),function(n,t,i){"use strict";function r(){function r(r){i.read(t.odata.getUrl(t.odata.entitySet.generalSettings),function(t){n.country(t.Country);n.city(t.City);n.conferenceFullName(t.ConferenceFullName);n.externalUrl(t.ExternalUrl);n.startDate(t.StartDate.format("mm/dd/yyyy"));n.endDate(t.EndDate.format("mm/dd/yyyy"));n.acmConferenceAlias(t.AcmConferenceAlias);n.acmConferenceYearAlias(t.AcmConferenceYearAlias);r()})}var n=this;n.country=ko.observable();n.city=ko.observable();n.conferenceFullName=ko.observable().extend({required:{message:"Conference Full Name is required."}});n.externalUrl=ko.observable();n.startDate=ko.observable();n.endDate=ko.observable();n.acmConferenceAlias=ko.observable("").extend({pattern:/^[A-Za-z]{3,}$/,maxLength:12,message:"Invalid Alias."}).autoMap();n.acmConferenceYearAlias=ko.observable("").extend({pattern:/^[A-Za-z]{3,}[0-9]{4}$/,maxLength:16,message:"Invalid Alias."}).autoMap();n.save=function(){var r=ko.validation.group(n),u,f;return r().length>0?(r.showAllMessages(),!1):(u={Country:n.country(),City:n.city(),ConferenceFullName:n.conferenceFullName(),ExternalUrl:n.externalUrl(),StartDate:new Date(n.startDate()).toISOString(),EndDate:new Date(n.endDate()).toISOString(),AcmConferenceAlias:n.acmConferenceAlias(),AcmConferenceYearAlias:n.acmConferenceYearAlias()},f={requestUri:t.odata.getUrl(t.odata.entitySet.generalSettings),method:"POST",data:u},i.request(f,function(){t.addMessage("Conference Details have been saved!")}),!1)};n.bindTo=function(t){function i(){ko.applyBindingsAndShow(n,t)}r(i)}}t.settingsGeneral=function(n){t.cookies.setValue("trackId",-1,0,"/");(new r).bindTo(n)}}(window.jQuery,window.app,window.OData),function(n,t,i){"use strict";function r(){function r(r){i.read(t.odata.getUrl(t.odata.entitySet.conferenceSessionSettings),function(i){t.autoMap(n,i);r()})}var n=this;n.allowDownloadCameraReadyFilesBySession=ko.observable(!1).autoMap();n.save=function(){var r=ko.validation.group(n),u,f;return r().length>0?(r.showAllMessages(),!1):(u=t.autoMap(n),f={requestUri:t.odata.getUrl(t.odata.entitySet.conferenceSessionSettings),method:"POST",data:u},i.request(f,function(){t.addMessage("Session settings have been saved!")}),!1)};n.bindTo=function(t){function i(){ko.applyBindingsAndShow(n,t)}r(i)}}t.settingsConferenceSession=function(n){t.cookies.setValue("trackId",-1,0,"/");(new r).bindTo(n)}}(window.jQuery,window.app,window.OData),function(n,t,i){"use strict";function r(){var t=this;t.id=n.autoMap();t.name=n.autoMap();t.checked=ko.observable(!0)}function u(){var u=this;u.isFileUploaded=ko.observable(!1);u.reviewers=ko.observableArray();u.normalReviewers=ko.observableArray();u.hasError=ko.observable(!1);u.errorText=ko.observable();u.uploading=ko.observable(!1);u.tracks=ko.observableArray();u.atLeastOneTrackSelected=ko.computed(function(){for(var t=!1,n=0;n<u.tracks().length;n++)t|=u.tracks()[n].checked();return t});u.loadTracks=function(){return t.read(n.odata.getUrl(n.odata.entitySet.tracks),function(t){for(var f,i=0;i<t.value.length;i++)f=n.autoMap(new r,t.value[i]),u.tracks.push(f)})};u.cancel=function(){window.location="/"+window.cmt3.conference.name+"/User/Reviewers"};u.getModel=function(){for(var t,e,i,r,f=[],n=0;n<u.normalReviewers().length;n++)t=u.normalReviewers()[n],e={FirstName:t.firstName,MiddleInitial:t.middleInitial,LastName:t.lastName,Organization:t.organization,Email:t.email},f.push(e);for(i=[],n=0;n<u.tracks().length;n++)r=u.tracks()[n],r.checked()&&i.push(r.id);return{Reviewers:f,Tracks:i,IsMeta:!1}};u.send=function(){if(u.atLeastOneTrackSelected()){var i=u.getModel(),r={requestUri:n.odata.getUrl(n.odata.entitySet.reviewers,null,"Import"),method:"POST",data:{Request:i}};t.request(r,function(){window.location="/"+window.cmt3.conference.name+"/User/Reviewers"})}};u.post=function(n,t,i){var r,f,u;i=i||"post";r=document.createElement("form");r.setAttribute("method",i);r.setAttribute("action",n);for(f in t)t.hasOwnProperty(f)&&(u=document.createElement("input"),u.setAttribute("type","hidden"),u.setAttribute("name",f),u.setAttribute("value",t[f]),r.appendChild(u));document.body.appendChild(r);r.submit();document.body.removeChild(r)};u.uploadFile=function(n,t){t.target.value!=""&&(u.uploading(!0),t.target.form.submit())};u.parseUploadResult=function(){var t=i.parseJSON(i("#singleFileUploadFrame").contents().text()),r,n,f;if(u.reviewers.removeAll(),u.normalReviewers.removeAll(),u.hasError(t.HasError),u.errorText(t.ErrorText),!u.hasError())for(r=0;r<t.Models.length;r++)n=t.Models[r],f={organization:n.Organization,email:n.Email,firstName:n.FirstName,lastName:n.LastName,middleInitial:n.MiddleInitial,notice:n.Note,rawData:n.RawData,hasError:n.HasError},u.reviewers.push(f),f.hasError||u.normalReviewers.push(f);u.isFileUploaded(!0);u.uploading(!1)};u.bindTo=function(n){u.loadTracks().done(function(){ko.applyBindingsAndShow(u,n)})}}n.importReviewers=function(n){(new u).bindTo(n)}}(window.app,window.OData,window.jQuery,window.document,window.confirm,window.setTimeout),function(n,t,i,r,u){"use strict";function h(n){var t=this;t.email=n.Email;t.name=n.MiddleInitial==null||n.MiddleInitial==""?n.FirstName+" "+n.LastName:n.FirstName+" "+n.MiddleInitial+" "+n.LastName}function o(){var t=this;t.id=n.autoMap();t.name=n.autoMap();t.subject=n.autoMap();t.body=n.autoMap();t.createStub=function(n){return t.id=0,t.name=n,t.subject="",t.body="",t}}function c(r,u,o,c){function a(i,r){var u="";if(c==="userId"){var a="&$filter="+f,v="&$skip="+i,y="&$top="+r;u=n.odata.getUrl(o,s)+"?$count=true"+a+v+y}else u=n.odata.getUrl(o,{key:e==null?-1:e,filter:f,skip:i,top:r});return t.read(u,function(n){for(var t,r={},i=0;i<n.value.length;i++)t=n.value[i],r[t.Id]||(r[t.Id]=!0,l.recipients.push(new h(t)));l.showAllVisible(l.recipientCount>l.recipients().length)})}var l=this;l.recipients=ko.observableArray();l.recipientCount=u;l.showAllVisible=ko.observable(!1);l.showInDialog=function(){i(r).modal("show")};l.showAll=function(){a(10,null)};l.bind=function(){return a(0,10).done(function(){ko.applyBindings(l,r)})}}function l(n){var t=this,r=null;t.name=ko.observable().extend({required:!0});t.editInDialog=function(){return r=i.Deferred(),t.name(""),t.name.isModified(!1),i(n).modal("show"),r.promise()};t.bind=function(){ko.applyBindings(t,n)};t.saveTemplate=function(){var u=ko.validation.group(t);if(u().length>0){u.showAllMessages();return}r&&r.resolve(t.name());i(n).modal("hide")}}function a(u,f){var e=this,o=null,s;e.fromEmail=ko.observable().autoMap();e.fromName=ko.observable().autoMap();e.toEmail=ko.observable().autoMap();e.toName=ko.observable().autoMap();e.ccEmail=ko.observable().autoMap();e.recipientCount=ko.observable().autoMap();e.subject=ko.observable().autoMap();e.body=ko.observable("").autoMap();s=null;e.showInDialog=function(t,r){n.autoMap(e,t);s=r;i(u).modal("show")};e.sendEmails=function(){var e={requestUri:f,method:"POST",data:{Request:s}};t.request(e,function(t){var f=t.value;i(u).modal("hide");o||(o=new n.EmailProgressViewModel(r.getElementById("showProgressDialog")),o.bind());o.showInDialog(f)})};e.bind=function(){ko.applyBindings(e,u)}}function v(s,h,v,y,p,w){function tt(n,t){d||(d=new a(r.getElementById("previewEmailDialog"),y),d.bind());d.showInDialog(n,t)}function nt(){var n=ko.validation.group(b);return n().length>0?(n.showAllMessages(),!1):!0}function it(){var i=n.autoMap(b),r;return i.UserFilter=f,i.TrackId=e,r={requestUri:v,method:"POST",data:{Request:i}},t.request(r,function(n){b.recipientCount=n.value})}function rt(){return t.read(n.odata.getUrl(n.odata.entitySet.emailTemplates,{orderby:"Name"}),function(t){b.templates.push((new o).createStub("Select predefined template…"));b.templates.push((new o).createStub("Create new…"));for(var i=0;i<t.value.length;i++)b.templates.push(n.autoMap(new o,t.value[i]))})}var b=this,d=null,g=null,k=null;b.from=s;b.ccEmail=ko.observable("").extend({email:!0,maxLength:200}).autoMap();b.ccSMR=ko.observable().autoMap(!1);b.recipientCount=0;b.templates=ko.observableArray();b.selectedTemplate=ko.observable();b.selectedTemplate.subscribe(function(n){b.subject(n.subject);b.subject.isModified(!1);b.body(n.body);b.body.isModified(!1)});b.subject=ko.observable("").extend({required:!0}).autoMap();b.body=ko.observable("").extend({required:!0}).autoMap();b.showPlaceholders=ko.observable(!1);b.showRecipients=function(){alert(b.recipients)};b.previewEmail=function(){var i,r;nt()&&(i=n.autoMap(b),i.UserFilter=f,i.TrackId=e,r={requestUri:h,method:"POST",data:{Request:i}},t.request(r,function(n){n.recipientCount=b.recipientCount;tt(n,i)}))};b.saveTemplate=function(){var i,r;nt()&&(i=n.autoMap(b),delete i.CcEmail,delete i.CcSMR,i.Name=b.selectedTemplate().name,r={requestUri:n.odata.getUrl(n.odata.entitySet.emailTemplates,b.selectedTemplate().id),method:"PUT",headers:{Prefer:"return-content"},data:i},t.request(r,function(t){b.selectedTemplate().subject=t.Subject;b.selectedTemplate().body=t.Body;n.addMessage("Template '{0}' saved.".format(b.selectedTemplate().name))}))};b.saveTemplateAs=function(){if(nt()){var i=n.autoMap(b);delete i.CcEmail;delete i.CcSMR;g||(g=new l(r.getElementById("newTemplateNameDialog")),g.bind());g.editInDialog().done(function(r){i.Name=r;var u={requestUri:n.odata.getUrl(n.odata.entitySet.emailTemplates),method:"POST",headers:{Prefer:"return-content"},data:i};t.request(u,function(t){var i=n.autoMap(new o,t);b.templates.push(i);b.selectedTemplate(i);n.addMessage("Template '{0}' created.".format(r))})})}};b.removeTemplate=function(){if(b.selectedTemplate().id&&u("Are you sure you want to delete the template?")){var i={requestUri:n.odata.getUrl(n.odata.entitySet.emailTemplates,b.selectedTemplate().id),method:"DELETE"};t.request(i,function(){n.addMessage("Temmplate '{0}' removed.".format(b.selectedTemplate().name));b.templates.remove(b.selectedTemplate())})}};b.showRecipients=function(){k?k.showInDialog():(k=new c(r.getElementById("showRecipientsDialog"),b.recipientCount,p,w),k.bind().done(function(){k.showInDialog()}))};b.bindTo=function(n){i.when(it(),rt()).done(function(){ko.applyBindingsAndShow(b,n)})}}var f=null,e=null,s=null;n.url==undefined||(f=n.url.queryString.getValue("filter"),e=n.url.queryString.getValue("trackId"),s=n.url.queryString.getValue("userId"));n.reviewerSendEmail=function(n,t,i,r,u,f){new v(n,t,i,r,u,f).bindTo("sendEmailForm")}}(window.app,window.OData,window.jQuery,window.document,window.confirm,window.setTimeout),function(n,t,i,r,u,f,e){"use strict";function s(){var t=this;t.userId=n.autoMap();t.email=n.autoMap();t.firstName=n.autoMap();t.lastName=n.autoMap();t.organization=n.autoMap();t.countryCode=n.autoMap();t.countryName=n.autoMap()}function a(t){var i=this;i.email=ko.observable().extend({required:!0,email:!0,validation:{validator:function(n,t){for(var i=0;i<t.length;i++)if(t[i].email==n)return!1;return!0},message:"Author with the same email already exists.",params:t}});i.isEmailInvalid=ko.observable(!1);i.firstName=ko.observable().extend({required:{message:"First Name is required."},maxLength:200});i.lastName=ko.observable().extend({required:{message:"Last Name is required."},maxLength:200});i.organization=ko.observable().extend({required:{message:"Organization is required."},maxLength:200});i.availableCountries=ko.observable(n.countries.getCountries());i.countryCode=ko.observable().extend({required:{message:"Country is required."}});i.isSearching=ko.observable(!1);i.notFound=ko.observable(!1);i.cancelAdd=function(){i.email("");i.email.isModified(!1);i.firstName("");i.firstName.isModified(!1);i.lastName("");i.lastName.isModified(!1);i.organization("");i.organization.isModified(!1);i.countryCode(undefined);i.countryCode.isModified(!1);i.notFound(!1);i.isEmailInvalid(!1)}}function h(){var t=this;t.id=n.autoMap();t.name=n.autoMap();t.parentSubjectAreaId=n.autoMap();t.isChild=function(){return t.parentSubjectAreaId!=null};t.isPrimary=ko.observable();t.isSecondary=ko.observable();t.checkBoxId=function(){return"primary"+t.id};t.allowParentSelection=!0;t.specialType=null;t.customValue=ko.observable(null).extend({required:{onlyIf:function(){return t.isPrimary()||t.isSecondary()}}})}function c(){var t=this;t.id=n.autoMap();t.originalName=n.autoMap();t.size=n.autoMap();t.formattedSize=n.autoMap();t.uploadDate=n.autoMap();t.downloadLink=n.autoMap()}function l(){return{welcomeMessage:n.autoMap(),abstractAllowed:n.autoMap(),abstractMaxLength:n.autoMap(),abstractRequired:n.autoMap(),showNoneOfTheAboveSubjectArea:n.autoMap(),secondarySubjectAreaAllowed:n.autoMap(),secondarySubjectAreaLimited:n.autoMap(),secondarySubjectAreaMaxNumber:n.autoMap(),immediateParentSelectionAllowed:n.autoMap(),customPrimarySubjectAreaAllowed:n.autoMap(),customSecondarySubjectAreaAllowed:n.autoMap(),submissionMinFileNumber:n.autoMap(),submissionMaxFileNumber:n.autoMap(),submissionAllowedFileTypes:n.autoMap(),submissionMaxFileSize:n.autoMap(),disableCoAuthors:n.autoMap(),disableTitleInstruction:n.autoMap(),titleMapping:n.autoMap(),fileUploadTitleMapping:n.autoMap(),showTipUnderFiles:n.autoMap()}}function v(v,y,p){function tt(){return t.read(n.odata.getUrl(n.odata.entitySet.submissionSettings,w.oldTrackId),function(t){n.autoMap(w.oldSettings,t)})}function it(){return t.read(n.odata.getUrl(n.odata.entitySet.submissionSettings,w.trackId),function(t){n.autoMap(w.settings,t);w.settings.titleMapping!=null&&(w.titleTitle=w.settings.titleMapping);w.settings.fileUploadTitleMapping!=null&&(w.fileUploadTitle=w.settings.fileUploadTitleMapping)})}function k(n){return n.substr(n.lastIndexOf(".")+1)}function d(n,t){for(var f=k(n).toLowerCase(),r=t.split(","),u=!1,i=0;i<r.length;i++)if(r[i].trim().toLowerCase()==f){u=!0;break}return u}function rt(){function h(){var n=!0;return w.files().length>w.settings.submissionMaxFileNumber&&(w.showFilesMaxErrorMessage(!0),n=!1),n}function l(){for(var t,i=!1,n=0;n<w.authors().length;n++)if(w.authors()[n].email==w.primaryEmail()){i=!0;break}return t=!0,i||(w.showPrimaryAuthorErrorMessage(!0),t=!1),t}function v(){var i,r,n,t,u;if(w.subjectAreas.length==0)return!0;for(i=[],r=!1,n=0;n<w.subjectAreas.length;n++)(w.subjectAreas[n].specialType=="customPrimary"||w.subjectAreas[n].specialType=="customSecondary")&&i.push(w.subjectAreas[n].customValue),w.subjectAreas[n].isPrimary()&&(r=!0);return t=!0,u=ko.validation.group(i),u().length>0&&(u.showAllMessages(),t=!1),r||(w.showSubjectAreasErrorMessage(!0),t=!1),t}function r(t){var s,r,f,u;if(w.files().length+t.length>w.settings.submissionMaxFileNumber){n.addMessage("You can upload up to {0} files only.".format(w.settings.submissionMaxFileNumber),null,"error");return}for(s=[],r=0;r<w.files().length;r++)s[w.files()[r].originalName.toLowerCase()]=!0;for(r=0;r<t.length;r++)f=t[r],y(f,s)&&(u=i.ajaxSettings.xhr(),u.open("POST",o.fileUpload,!0),u.setRequestHeader("Accept","application/json"),u.setRequestHeader("File-Name",encodeURIComponent(f.name)),u.send(f),u.addEventListener("load",function(t){t.target.status==200?e(t.target.responseText):n.processXmlHttpRequestError(t.target)},!1))}function y(t,i){var r=t.name.toLowerCase(),u;if(i[r]===undefined)i[r]=!0;else return n.addMessage("Found at least two files with the same name: '{0}'.".format(t.name),null,"error"),!1;return t.size>w.settings.submissionMaxFileSize*1048576?(n.addMessage("File '{0}' is bigger than maximum allowed size of {1} Mb.".format(t.name,w.settings.submissionMaxFileSize),null,"error"),!1):(u=d(t.name,w.settings.submissionAllowedFileTypes),!u)?(n.addMessage("File '{0}' has type '{1}' which is not accepted. We accept '{2}' only.".format(t.name,k(t.name),w.settings.submissionAllowedFileTypes),null,"error"),!1):!0}function e(t){var r,i;try{r=ko.utils.parseJson(t)}catch(u){n.processException(u);return}i=n.autoMap(new c,r);i.uploadDate=new Date(i.uploadDate);isNaN(i.uploadDate)&&(i.uploadDate=new Date);w.files.push(i)}w.title=ko.observable().extend({required:!0,maxLength:1e3}).autoMap();w.abstract=ko.observable("").extend({required:{onlyIf:function(){return w.settings.abstractAllowed&&w.settings.abstractRequired}},maxLength:w.settings.abstractMaxLength}).autoMap();w.abstractCharsLeft=ko.computed(function(){return Math.max(w.settings.abstractMaxLength-w.abstract().length,0)});w.trackName="";w.editConflictAllowed=!1;w.statusId=n.autoMap();w.submissionListUrl=null;w.authorizeSendingSubmissionToTpms=ko.observable().extend({requiredCheckbox:{message:"Your agreement is required.",onlyIf:function(){return w.trackSettings.isTpmsEnabled}}}).autoMap();w.authorizeSendingSubmissionToIThenticate=ko.observable().extend({requiredCheckbox:{message:"Your agreement is required.",onlyIf:function(){return w.trackSettings.isIThenticateEnabled}}}).autoMap();w.submissionConflictDomainsRaw=ko.observable().extend({required:{message:"Domain conflicts are required.",onlyIf:function(){return w.trackSettings.isSubmissionConflictDomainsRequired}}}).autoMap();w.isAuthor=ko.observable(!1);w.isAuthorRole=ko.observable(!1);w.authors=ko.observableArray();w.showPrimaryAuthorErrorMessage=ko.observable(!1);w.showFilesMaxErrorMessage=ko.observable(!1);w.primaryEmail=ko.observable();w.removeAuthor=function(n){w.authors.remove(n)};w.moveAuthorUp=function(n){var t=w.authors.indexOf(n);w.authors.remove(n);w.authors.splice(t-1,0,n)};w.moveAuthorDown=function(n){var t=w.authors.indexOf(n);w.authors.remove(n);w.authors.splice(t+1,0,n)};w.addAuthor=function(t){var r=ko.validation.group([t.email,t.firstName,t.lastName,t.organization,t.countryCode]),i;if(r().length>0){r.showAllMessages();t.isEmailInvalid(!t.email.isValid());return}i=n.autoMap(new s,{isPrimary:!1,email:t.email(),firstName:t.firstName(),lastName:t.lastName(),organization:t.organization(),countryCode:t.countryCode(),countryName:n.countries.getCountryNameByCode(t.countryCode())});w.authors.push(i);w.authors().length==1&&(w.primaryEmail(i.email),w.showPrimaryAuthorErrorMessage(!1));t.cancelAdd()};w.newAuthor=new a(w.authors);w.searchAuthorByEmail=function(i){var r=ko.validation.group([i.email]),u;if(r().length>0){i.isEmailInvalid(!0);r.showAllMessages();return}i.isEmailInvalid(!1);i.isSearching(!0);u={requestUri:n.odata.getGlobalUrl(n.odata.entitySet.users,null,"SearchByEmail"),method:"POST",showProgressIndicator:!1,data:{Email:i.email()}};t.read(u,function(t){var r=n.autoMap(new s,t);r.userId=t.Id;w.authors.push(r);w.authors().length==1&&(w.primaryEmail(r.email),w.showPrimaryAuthorErrorMessage(!1));i.cancelAdd();i.isSearching(!1)},function(n){i.isSearching(!1);n.response.statusCode==404?w.newAuthor.notFound(!0):t.defaultError(n)})};w.subjectAreas=[];w.subjectAreaPairs=function(){return n.computeSubjectAreaColumnPairs(w.subjectAreas)};w.showSubjectAreasErrorMessage=ko.observable(!1);w.showValidationWarning=ko.observable(!1);w.files=ko.observableArray();w.removeFile=function(n){w.files.remove(n)};w.uploadFile=function(){var n=i('<input type="file" accept="*" multiple="" />');n.on("change",function(){r(this.files)});n.trigger("click")};w.canUploadMoreFiles=ko.computed(function(){return w.files().length<w.settings.submissionMaxFileNumber});w.xhrUploadSupported=function(){return u};w.fileUploadDragOver=function(n,t){w.canUploadMoreFiles()&&i(t.target).addClass("dragOver")};w.fileUploadDragLeave=function(n,t){w.canUploadMoreFiles()&&i(t.target).removeClass("dragOver")};w.fileUploadDrop=function(n,t){if(w.canUploadMoreFiles()){var i=t.originalEvent.dataTransfer.files;r(i);w.fileUploadDragLeave(n,t)}};w.uploadSingleFile=function(n,t){t.target.value!=""&&t.target.form.submit()};w.parseSingleUploadResult=function(n,t){e(t.target.contentDocument.body.innerText)};w.questions=[];w.questionById={};w.dependentQuestions=[];w.dependentChoicesByQuestionId={};w.questionsByDependentChoiceId={};w.appliedDependentChoicesByQuestionId={};w.hiddenQuestionIds={};w.save=function(){function tt(i){var r=n.autoMap(i),u;return delete r.UserId,delete r.AuthorId,delete r.IsPrimary,u={requestUri:n.odata.getUrl(n.odata.entitySet.users,null,"AddCoAuthor"),method:"POST",data:{Request:r}},t.request(u,function(n){d[i.email]=n.value},function(i){if(i.response.statusCode==n.enums.httpStatusCodes.failure.conflict)n.addMessage(r,"Please click Cancel and use the email box to select author.","error");else if(i.response.statusCode==n.enums.httpStatusCodes.failure.badRequest){var r=n.getODataErrorMessage(i).message;n.addMessage(r,"Author information invalid:","error")}else t.defaultError(i)})}var s=!0,c=ko.validation.group(w,{deep:!1}),b,k,r,a,u,nt,y,d,g,e,p;for(c().length>0&&(c.showAllMessages(),s=!1),l()||(s=!1),v()||(s=!1),h()||(s=!1),b=[],e=0;e<w.questions.length;e++)k=w.questions[e],w.hiddenQuestionIds[k.id]||b.push(k);if(c=ko.validation.group(b,{deep:!0}),c().length>0&&(c.showAllMessages(),s=!1),!s){w.showValidationWarning(!0);return}for(r=n.autoMap(w),r.Id=w.id,r.TrackId=w.trackId,r.SubjectAreas=[],r.NoneOfAboveSubjectArea=!1,r.CustomPrimarySubjectArea=null,r.CustomSecondarySubjectArea=null,a=0;a<w.subjectAreas.length;a++)u=w.subjectAreas[a],(u.isPrimary()||u.isSecondary())&&(u.specialType==null?(nt={SubjectAreaId:u.id,IsPrimary:u.isPrimary()},r.SubjectAreas.push(nt)):u.specialType=="noneOfAbove"?r.NoneOfAboveSubjectArea=!0:u.specialType=="customPrimary"?r.CustomPrimarySubjectArea=u.customValue():u.specialType=="customSecondary"&&(r.CustomSecondarySubjectArea=u.customValue()));for(r.Files=[],y=0;y<w.files().length;y++)r.Files.push(w.files()[y].id);for(r.Answers=f.getAnswersJson(w.questions),d={},g=[],e=0;e<w.authors().length;e++)p=w.authors()[e],p.userId||p.authorId||g.push(tt(p));i.when.apply(i,g).done(function(){var u,i,f,e;for(r.Authors=[],r.References=[],u=0;u<w.authors().length;u++)i=w.authors()[u],i.userId||i.authorId||(i.authorId=d[i.email]),f={Order:u+1,IsPrimary:i.email==w.primaryEmail(),UserId:i.userId,AuthorId:i.authorId,Email:i.email},r.Authors.push(f);e={requestUri:n.odata.getUrl(n.odata.entitySet.submissions,w.id),method:"PUT",headers:{Prefer:"return-content"},progressIndicatorTimeout:0,data:r};t.request(e,function(t){w.editConflictAllowed?n.url.navigateTo(o.submissionConflict.format(t.Id)):n.url.navigateTo(o.submissionSummary.format(t.Id))})})}}function ut(t,r,u){return i.Deferred(function(f){n.autoMap(w,t);var e=et(),o=ct(t.Authors),s=i.Deferred(function(n){r.done(function(){n.resolve()})}).promise(),h=i.Deferred(function(n){u.done(function(){n.resolve()})}).promise(),c=lt(t.Files);i.when(e,o,s,h,c).done(function(){if(w.settings.disableCoAuthors){var n=w.authors.remove(function(n){return n.email!=w.primaryEmail()});n.length>0&&n.length<w.authors().length&&(w.authors(n),w.coAuthorsRemoved(!0))}w.abstract().length>w.settings.abstractMaxLength&&(w.abstract(w.abstract().substring(0,w.settings.abstractMaxLength-1)),w.abstractTrimmed(!0));w.files().length>w.settings.submissionMaxFileNumber&&w.filesDropped(!0);w.files().forEach(function(n){w.settings.submissionMaxFileSize*1048576<n.size&&w.filesDropped(!0);d(n.originalName,w.settings.submissionAllowedFileTypes)||w.filesDropped(!0)});w.filesDropped()&&w.files([]);f.resolve()});n.url.hash.getValue()=="saved"&&(n.url.hash.remove(),n.addMessage("Submission '{0}' saved!".format(w.title())))}).promise()}function ft(){return t.read(n.odata.getUrl(n.odata.entitySet.tracks,w.oldTrackId),function(n){w.oldTrackName=n.Name})}function et(){return t.read(n.odata.getUrl(n.odata.entitySet.tracks,w.trackId),function(n){w.trackName=n.Name;w.editConflictAllowed=n.EditConflictAllowed})}function ot(){return t.read(n.odata.getUrl("Tracks",{top:0,count:"true"}),function(n){w.isSingleTrackConference=n["@odata.count"]==1})}function st(){return t.request({requestUri:n.odata.getUrl(n.odata.entitySet.users,null,"GetCurrentProfile"),method:"GET"},function(t){t.UserId=t.Id;w.currentProfile=n.autoMap(new s,t)})}function ht(){return t.read(n.odata.getUrl(n.odata.entitySet.subjectAreas,{orderby:"FlatIndex",filter:"TrackId eq {0}".format(n.odata.escapeParam(w.trackId))}),function(t){function o(n){n||(this.customValue(null),this.customValue.isModified(!1))}function f(n){n.isPrimary.subscribe(function(n){n&&(w.showSubjectAreasErrorMessage(!1),s(this),this.isSecondary(!1))},n);n.isSecondary.subscribe(function(n){var t,i;if(n){if(w.settings.secondarySubjectAreaLimited&&(t=c(),t>w.settings.secondarySubjectAreaMaxNumber)){i=this;r(function(){i.isSecondary(!1)},0);return}this.isPrimary(!1)}},n);w.subjectAreas.push(n)}function s(n){for(var t=0;t<w.subjectAreas.length;t++)w.subjectAreas[t].isPrimary()&&w.subjectAreas[t]!=n&&w.subjectAreas[t].isPrimary(!1)}function c(){for(var t=0,n=0;n<w.subjectAreas.length;n++)w.subjectAreas[n].isSecondary()&&++t;return t}for(var u=null,i,e=0;e<t.value.length;e++)i=n.autoMap(new h,t.value[e]),u!=null&&u.id==i.parentSubjectAreaId&&!w.settings.immediateParentSelectionAllowed&&u.allowParentSelection&&(u.allowParentSelection=!1),i.parentSubjectAreaId==null&&(u=i),f(i);w.settings.showNoneOfTheAboveSubjectArea&&(i=new h,i.specialType="noneOfAbove",f(i));w.settings.customPrimarySubjectAreaAllowed&&(i=new h,i.specialType="customPrimary",i.isPrimary.subscribe(o,i),f(i));w.settings.customSecondarySubjectAreaAllowed&&w.settings.secondarySubjectAreaAllowed&&(i=new h,i.specialType="customSecondary",i.isSecondary.subscribe(o,i),f(i))})}function ct(r){for(var u=[],f=0;f<r.length;f++)u.push(r[f].UserId);return i.Deferred(function(i){if(!u.length){i.resolve();return}t.read(n.odata.getUrl("Users",{filter:n.odata.buildContainsQuery("Id",u)}),function(t){for(var o,u,f,h=[],e=0;e<r.length;e++)for(o=r[e],u=0;u<t.value.length;u++)if(o.UserId==t.value[u].Id){f=n.autoMap(new s,t.value[u]);f.userId=t.value[u].Id;h.push(f);o.IsPrimary&&w.primaryEmail(f.email);break}w.authors(h);i.resolve()})}).promise()}function lt(i){return i.length==0?!0:t.read(n.odata.getUrl(n.odata.entitySet.files,{filter:n.odata.buildContainsQuery("Id",i)}),function(t){for(var r=[],i=0;i<t.value.length;i++)r.push(n.autoMap(new c,t.value[i]));w.files(r)})}function at(){return i.Deferred(function(i){t.read(n.odata.getUrl(n.odata.entitySet.submissions,w.id),function(n){i.resolve(n)})}).promise()}var w=this;w.id=v;w.trackId=y;w.titleTitle="Title";w.fileUploadTitle="Files";w.oldTrackName="";w.currentProfile=null;w.settings=l();w.oldSettings=l();w.filesDropped=ko.observable(!1);w.abstractTrimmed=ko.observable(!1);w.coAuthorsRemoved=ko.observable(!1);w.trackSettings=p;w.choicesChange=function(n,t){t.status==="added"?g(t.value):t.status==="deleted"&&nt(t.value)};w.answerChange=function(n,t,i){nt(i);g(t)};var b=function(n){return i("#sq_"+n)},g=function(n){var i=w.questionsByDependentChoiceId[n],r,t,f,u;if(i&&i.length!==0)for(r=0;r<i.length;r++)(t=i[r],w.appliedDependentChoicesByQuestionId[t]||(w.appliedDependentChoicesByQuestionId[t]=[]),f=w.appliedDependentChoicesByQuestionId[t].indexOf(n),f>-1)||(w.appliedDependentChoicesByQuestionId[t].length===0&&(b(t).fadeIn(1e3),u=w.questionById[t],u.required()&&(u.validationEnabled=!0),w.hiddenQuestionIds[t]&&delete w.hiddenQuestionIds[t]),w.appliedDependentChoicesByQuestionId[t].push(n))},nt=function(n){var r=w.questionsByDependentChoiceId[n],u,t,f,i;if(r&&r.length!==0)for(u=0;u<r.length;u++)(t=r[u],w.appliedDependentChoicesByQuestionId[t]&&w.appliedDependentChoicesByQuestionId[t].length!==0)&&(f=w.appliedDependentChoicesByQuestionId[t].indexOf(n),f>-1&&(w.appliedDependentChoicesByQuestionId[t].splice(f,1),w.appliedDependentChoicesByQuestionId[t].length===0&&(b(t).fadeOut(1e3),w.hiddenQuestionIds[t]=!0,i=w.questionById[t],w.dependentQuestions.indexOf(i)>-1&&(i.required()&&(i.validationEnabled=!1),i.answer(null)))))};w.bindTo=function(t){at().done(function(r){r&&(w.oldTrackId=r.TrackId);i.when(it(),tt(),ft()).done(function(){var o;rt();var s=ht(),h=f.loadQuestions(n.enums.formType.submission,w.trackId).done(function(n){w.questions=n;for(var r,t,u,i=0;i<n.length;i++)if(t=n[i],w.questionById[t.id]=t,t.conditionQuestionChoiceIds.length>0)for(w.dependentChoicesByQuestionId[t.id]=t.conditionQuestionChoiceIds,r=0;r<t.conditionQuestionChoiceIds.length;r++)u=t.conditionQuestionChoiceIds[r],w.questionsByDependentChoiceId[u]||(w.questionsByDependentChoiceId[u]=[]),w.questionsByDependentChoiceId[u].push(t.id);for(i=0;i<n.length;i++)for(t=n[i],r=0;r<t.choices.length;r++)if(w.questionsByDependentChoiceId[t.choices[r].id]){w.dependentQuestions.push(t);break}}),u=i.Deferred();e.getCurrentRoleDescriptor().done(function(t){w.submissionListUrl=t.submissionListUrl;w.isAuthorRole(t.role==n.enums.userRole.author);st().done(function(){w.isAuthor(!1);u.resolve()})});o=i.when(ut(r,s,h),u,ot());o.done(function(){var s,i,r,u,h,e,o,n;ko.applyBindingsAndShow(w,t);f.subscribeChoicesChanged(w.dependentQuestions,w.choicesChange);f.subscribeAnswerChanged(w.dependentQuestions,w.answerChange);for(s in w.dependentChoicesByQuestionId)b(s).hide(),w.hiddenQuestionIds[s]=!0;for(i=0;i<w.dependentQuestions.length;i++)if(r=w.dependentQuestions[i].selectedChoiceIds.peek(),r)for(u=0;u<r.length;u++)if(h=r[u],e=w.questionsByDependentChoiceId[h],e)for(o=0;o<e.length;o++)n=e[o],w.appliedDependentChoicesByQuestionId[n]||(w.appliedDependentChoicesByQuestionId[n]=[]),w.appliedDependentChoicesByQuestionId[n].length===0&&(b(n).show(),delete w.hiddenQuestionIds[n]),w.appliedDependentChoicesByQuestionId[n].push(h)})})})}}var o;n.submissionChangeTrack=function(n,t,i,r){o=t;new v(n,i,r).bindTo("submissionForm")}}(window.app,window.OData,window.jQuery,window.setTimeout,window.FileReader!=undefined,new window.app.QuestionService,new window.app.RoleService),function(n,t,i){"use strict";function r(n){this.id=n.Id;this.title=n.Title;this.abstract=n.Abstract.htmlMultiLineEncode();this.authors={primary:n.Author};this.authorList=n.Authors;this.track={name:n.Track,id:n.TrackId};this.isSingleTrackConference=n.IsSingleTrackConference}t.DeletedSubmissionPage=function(t,i){var r=this;r.tracks=[];r.tracksLoaded=!1;r.$element=n(t);r.conference=window.cmt3.conference.name;r.page=ko.observable(1);r.top=ko.observable(25);r.sort=ko.observable("Id");r.controller=i;r.filters=[];r._total=ko.observable(0);r.selected=ko.observable(0);r.submissions=ko.observableArray();r.listen();r.Pager=ko.pager(r.selected,r.top);r.Pager().CurrentPage.subscribe(function(){r.page(r.Pager().CurrentPage());r.show()})};t.DeletedSubmissionPage.prototype={restore:function(n){var r=this,u={requestUri:t.odata.getUrl(t.odata.entitySet.deletedSubmissions,null,"Restore"),method:"POST",data:{Request:{SubmissionId:n}}};i.request(u,function(){t.addMessage("Submission (id={0}) has been restored.".format(n));r.show()})},bulkRestore:function(){var n=this,r={requestUri:t.odata.getUrl(t.odata.entitySet.deletedSubmissions,null,"BulkRestore"),method:"POST",data:{Request:{SubmissionFilter:n.getFilter()}}};confirm("Are you sure you want to restore selected submissions?")&&i.request(r,function(){t.addMessage("Selected submissions have been restored.");n.show()})},listen:function(){var t=this;n(document).on("data.filter",function(){t.Pager().CurrentPage()<2?t.show():t.Pager().CurrentPage(1)})},getFilter:function(){var t="";return n.each(this.filters,function(n,i){i.getValue()&&(t+=t==""?i.getValue():" and "+i.getValue())}),t},show:function(){function f(){var f=u.sort(),e=u.top(),o=u.skip(),s=u.getFilter(),h=f?"&$orderby="+f:"",c=e?"&$top="+e:"",l=o?"&$skip="+o:"",a=s?"&$filter="+encodeURIComponent(s):"",v={headers:{Accept:"application/json"},requestUri:"/api/odata/"+u.conference+"/$batch",method:"POST",data:{requests:[{url:"/api/odata/"+u.conference+"/"+u.controller+"?$count=true"+h+a+l+c,method:"GET",headers:{Accept:"application/json"}}]}};i.request(v,function(i){t.page.saveState("deleted_submissions",{sort:f,top:e,skip:o,filter:s});var h=i.responses[0].body,c=h["@odata.count"],a=h.value,l=[];n.each(a,function(n,t){l.push(new r(t))});u.submissions(l);u._total()==0&&u._total(c);u.selected(c);n("html,body").scrollTop(0)},function(n){window.cmt3.logger.log(n.message)},i.batchHandler)}var u=this;u.initialized&&(u.tracksLoaded?f():i.read(t.odata.getUrl(t.odata.entitySet.tracks),function(n){for(var r,i=0;i<n.value.length;i++)r=t.autoMap(new t.Track,n.value[i]),u.tracks.push(r);u.tracksLoaded=!0;f()}))},scroll:function(){n(window).scrollTop()==n(document).height()-n(window).height()&&self.show()},showAbstract:function(t,i){var f=ko.contextFor(i.target).$parent,r=n(i.target),u=r.next();u.is(":visible")?(u.hide(),r.text("Show abstract")):(u.show(),r.text("Hide abstract"))},post:function(n,t,i){var r,f,u;i=i||"post";r=document.createElement("form");r.setAttribute("method",i);r.setAttribute("action",n);for(f in t)t.hasOwnProperty(f)&&(u=document.createElement("input"),u.setAttribute("type","hidden"),u.setAttribute("name",f),u.setAttribute("value",t[f]),r.appendChild(u));document.body.appendChild(r);r.submit();document.body.removeChild(r)},stub:function(){alert("Sorry, this feature is not implemented yet.")},reset:function(){n.each(this.filters,function(n,t){t.reset()});this.show()},size:function(t,i){var r,u,f;n("a",".show").removeClass("btn-success").css("color","#999999");n(i.currentTarget).addClass("btn-success").css("color","white");r=n(i.target).attr("size");u=parseInt(r);this.top(u);f=this.Pager().CurrentPage();this.Pager().CurrentPage(1);f===1&&this.show()},skip:function(){return(this.page()-1)*this.top()},prev:function(){this.top()!=0&&this.page()!=1&&(this.page(this.page()-1),this.show())},next:function(){this.top()==0||this.page()>this.selected()/this.top()||(this.page(this.page()+1),this.show())},setSort:function(t,i){var r=n(i.target),u=r.attr("data-sort");(u==null||u==undefined)&&(r=n(r.context.parentNode),u=r.attr("data-sort"));r.hasClass("selected")?this.sort().match(" desc$")?(this.sort(u+" asc"),r.find("i").removeClass("icon-arrow-down"),r.find("i").addClass("icon-arrow-up")):(this.sort(u+" desc"),r.find("i").removeClass("icon-arrow-up"),r.find("i").addClass("icon-arrow-down")):(n("th[data-sort]").each(function(){n(this).find("i").removeClass("icon-arrow-up");n(this).find("i").removeClass("icon-arrow-down");n(this).removeClass("selected")}),r.find("i").removeClass("icon-arrow-down"),r.find("i").addClass("icon-arrow-up"),r.addClass("selected"),this.sort(u+" asc"));this.show()},refresh:function(){this.show()}}}(window.jQuery,window.app,window.OData),function(n,t,i,r,u,f){"use strict";function o(){var t=this;t.id=n.autoMap();t.originalName=n.autoMap();t.size=n.autoMap();t.formattedSize=n.autoMap();t.uploadDate=n.autoMap();t.downloadLink=n.autoMap()}function s(){var t=this;t.allowedFileTypes=n.autoMap();t.minFileNumber=n.autoMap();t.maxFileNumber=n.autoMap();t.maxFileSize=n.autoMap()}function h(t,r){var f=this;f.id=n.autoMap();f.name=n.autoMap();f.files=ko.observableArray();f.settings=n.autoMap(new s,r);f.initModel=function(){function r(r){var c,l,a,u,o;if(f.files().length+r.length>f.settings.maxFileNumber){n.addMessage("You can upload up to {0} files only.".format(f.settings.maxFileNumber),null,"error");return}for(c={},l=t.files(),u=0;u<l.length;u++)c[l[u].originalName.toLowerCase()]=!0;for(n.showProgress(),a=[],u=0;u<r.length;u++)o=r[u],h(o,c)&&a.push(i.Deferred(function(t){var r=i.ajaxSettings.xhr();r.open("POST",e.fileUpload,!0);r.setRequestHeader("Accept","application/json");r.setRequestHeader("File-Name",encodeURIComponent(o.name));r.send(o);r.addEventListener("load",function(i){i.target.status==200?(s(i.target.responseText),t.resolve()):(n.processXmlHttpRequestError(i.target),t.reject())},!1)}).promise());i.when.apply(i,a).always(n.hideProgress)}function h(t,i){var u=t.name.toLowerCase(),r;if(i[u]===undefined)i[u]=!0;else return n.addMessage("Found at least two files with the same name: '{0}'.".format(t.name),null,"error"),!1;if(t.size>f.settings.maxFileSize*1048576)return n.addMessage("File '{0}' is bigger than maximum allowed size of {1} Mb.".format(t.name,f.settings.maxFileSize),null,"error"),!1;var e=t.name.substr(t.name.lastIndexOf(".")+1).toLowerCase(),o=f.settings.allowedFileTypes.split(","),s=!1;for(r=0;r<o.length;r++)if(o[r].trim().toLowerCase()==e){s=!0;break}return s?!0:(n.addMessage("File '{0}' has type '{1}' which is not accepted. We accept '{2}' only.".format(t.name,e,f.settings.allowedFileTypes),null,"error"),!1)}function s(t){var r,i;try{r=ko.utils.parseJson(t)}catch(u){n.processException(u);return}i=n.autoMap(new o,r);i.uploadDate=new Date(i.uploadDate);isNaN(i.uploadDate)&&(i.uploadDate=new Date);f.files.push(i)}f.title=n.autoMap();f.validateFiles=function(){var n=!0;return f.files().length>f.settings.maxFileNumber&&(f.showFilesMaxErrorMessage(!0),n=!1),f.files().length<f.settings.minFileNumber&&(f.showFilesMinErrorMessage(!0),n=!1),n};f.showFilesMinErrorMessage=ko.observable(!1);f.showFilesMaxErrorMessage=ko.observable(!1);f.files=ko.observableArray();f.removeFile=function(n){f.files.remove(n)};f.uploadFile=function(){var n=i('<input type="file" accept="*" multiple="" />');n.on("change",function(){r(this.files)});n.trigger("click")};f.canUploadMoreFiles=ko.computed(function(){return f.files().length<f.settings.maxFileNumber});f.xhrUploadSupported=function(){return u};f.fileUploadDragOver=function(n,t){f.canUploadMoreFiles()&&i(t.target).addClass("dragOver")};f.fileUploadDragLeave=function(n,t){f.canUploadMoreFiles()&&i(t.target).removeClass("dragOver")};f.fileUploadDrop=function(n,t){if(f.canUploadMoreFiles()){var i=t.originalEvent.dataTransfer.files;r(i);f.fileUploadDragLeave(n,t)}};f.uploadSingleFile=function(n,t){t.target.value!=""&&t.target.form.submit()};f.parseSingleUploadResult=function(n,t){s(t.target.contentDocument.body.innerText)}}}function c(r,u,s,c,l,a,v){function k(i){if(i.length==0)return!0;var u=i.map(function(n){return n.FileId}),r=i.reduce(function(n,t){return n[t.FileId]=t.FileLabelId,n},{}),f=n.odata.getUrl(n.odata.entitySet.files,{filter:n.odata.buildContainsQuery("Id",u)});return t.read({requestUri:f,showProgressIndicator:!1},function(t){for(var f,u={},i=0;i<t.value.length;i++)u[r[t.value[i].Id]]||(u[r[t.value[i].Id]]=[]),u[r[t.value[i].Id]].push(n.autoMap(new o,t.value[i]));for(f in u)w[f]&&w[f].files(u[f])})}function d(){return i.Deferred(function(i){var r=n.odata.getUrl(n.odata.entitySet.supplementary,y.id);t.read({requestUri:r,showProgressIndicator:!1},function(n){i.resolve(n)})}).promise()}function g(){f.getCurrentRoleDescriptor().done(function(n){y.submissionListUrl=n.submissionListUrl})}var y=this,w,p,b;for(y.id=r,y.trackId=null,y.trackName=s,y.isSingleTrackConference=c,y.fileIds=l,y.titleTitle="Title",y.labels=ko.observableArray(),y.title=n.autoMap(),y.showValidationWarning=ko.observable(!1),y.submissionListUrl=null,y.files=ko.pureComputed(function(){return y.labels().reduce(function(n,t){return n.concat(t.files())},[])}),w={},p=0;p<v.length;p++)b=new h(y,v[p].Settings),y.labels.push(n.autoMap(b,v[p])),b.initModel(),w[v[p].Id]=b;y.settings={minFileNumber:n.autoMap(),maxFileNumber:n.autoMap(),allowedFileTypes:n.autoMap(),maxFileSize:n.autoMap()};n.autoMap(y.settings,a);y.save=function(){var o=!0,h=ko.validation.group(y,{deep:!0}),r,u,i,s,f,c;for(h().length>0&&(h.showAllMessages(),o=!1),r=y.labels(),i=0;i<r.length;i++)r[i].validateFiles()||(o=!1);if(!o){y.showValidationWarning(!0);return}for(u=n.autoMap(y),u.Id=y.id,u.Files=[],i=0;i<r.length;i++)for(s=r[i].files(),f=0;f<s.length;f++)u.Files.push({FileId:s[f].id,FileLabelId:r[i].id});c={requestUri:n.odata.getUrl(n.odata.entitySet.supplementary,y.id),method:"PUT",headers:{Prefer:"return-content"},progressIndicatorTimeout:0,data:u};t.request(c,function(t){n.url.navigateTo(e.submissionSummary.format(t.Id))})};y.bindTo=function(t){n.showProgress();var r=i.Deferred();i.when(d(),g(),k(y.fileIds)).done(function(i){n.autoMap(y,i);ko.applyBindingsAndShow(y,t);r.resolve()});r.always(n.hideProgress)}}var e;n.supplementaryDetails=function(n,t,i,r,u,f,o,s,h){e=u;new c(n,t,i,r,f,o,s).bindTo(h)}}(window.app,window.OData,window.jQuery,window.setTimeout,window.FileReader!=undefined,new window.app.RoleService),function(n,t,i,r,u,f){"use strict";function o(){var t=this;t.id=n.autoMap();t.originalName=n.autoMap();t.size=n.autoMap();t.formattedSize=n.autoMap();t.uploadDate=n.autoMap();t.downloadLink=n.autoMap()}function s(r,s,h,c,l,a){function y(){function s(){var n=!0;return v.files().length>v.settings.submissionMaxFileNumber&&(v.showFilesMaxErrorMessage(!0),n=!1),v.files().length<v.settings.submissionMinFileNumber&&(v.showFilesMinErrorMessage(!0),n=!1),n}function r(t){var o,s,r,u;if(v.files().length+t.length>v.settings.submissionMaxFileNumber){n.addMessage("You can upload up to {0} files only.".format(v.settings.submissionMaxFileNumber),null,"error");return}for(o=[],r=0;r<v.files().length;r++)o[v.files()[r].originalName.toLowerCase()]=!0;for(n.showProgress(),s=[],r=0;r<t.length;r++)u=t[r],h(u,o)&&s.push(i.Deferred(function(t){var r=i.ajaxSettings.xhr();r.open("POST",e.fileUpload,!0);r.setRequestHeader("Accept","application/json");r.setRequestHeader("File-Name",encodeURIComponent(u.name));r.send(u);r.addEventListener("load",function(i){i.target.status==200?(f(i.target.responseText),t.resolve()):(n.processXmlHttpRequestError(i.target),t.reject())},!1)}).promise());i.when.apply(i,s).always(n.hideProgress)}function h(t,i){var u=t.name.toLowerCase(),r;if(i[u]===undefined)i[u]=!0;else return n.addMessage("Found at least two files with the same name: '{0}'.".format(t.name),null,"error"),!1;if(t.size>v.settings.submissionMaxFileSize*1048576)return n.addMessage("File '{0}' is bigger than maximum allowed size of {1} Mb.".format(t.name,v.settings.submissionMaxFileSize),null,"error"),!1;var f=t.name.substr(t.name.lastIndexOf(".")+1).toLowerCase(),e=v.settings.submissionAllowedFileTypes.split(","),o=!1;for(r=0;r<e.length;r++)if(e[r].trim().toLowerCase()==f){o=!0;break}return o?!0:(n.addMessage("File '{0}' has type '{1}' which is not accepted. We accept '{2}' only.".format(t.name,f,v.settings.submissionAllowedFileTypes),null,"error"),!1)}function f(t){var r,i;try{r=ko.utils.parseJson(t)}catch(u){n.processException(u);return}i=n.autoMap(new o,r);i.uploadDate=new Date(i.uploadDate);isNaN(i.uploadDate)&&(i.uploadDate=new Date);v.files.push(i)}v.title=n.autoMap();v.submissionListUrl=null;v.showValidationWarning=ko.observable(!1);v.showFilesMinErrorMessage=ko.observable(!1);v.showFilesMaxErrorMessage=ko.observable(!1);v.files=ko.observableArray();v.removeFile=function(n){v.files.remove(n)};v.uploadFile=function(){var n=i('<input type="file" accept="*" multiple="" />');n.on("change",function(){r(this.files)});n.trigger("click")};v.canUploadMoreFiles=ko.computed(function(){return v.files().length<v.settings.submissionMaxFileNumber});v.xhrUploadSupported=function(){return u};v.fileUploadDragOver=function(n,t){v.canUploadMoreFiles()&&i(t.target).addClass("dragOver")};v.fileUploadDragLeave=function(n,t){v.canUploadMoreFiles()&&i(t.target).removeClass("dragOver")};v.fileUploadDrop=function(n,t){if(v.canUploadMoreFiles()){var i=t.originalEvent.dataTransfer.files;r(i);v.fileUploadDragLeave(n,t)}};v.uploadSingleFile=function(n,t){t.target.value!=""&&t.target.form.submit()};v.parseSingleUploadResult=function(n,t){f(t.target.contentDocument.body.innerText)};v.save=function(){var u=!0,f=ko.validation.group(v,{deep:!1}),i,r,o;if(f().length>0&&(f.showAllMessages(),u=!1),s()||(u=!1),!u){v.showValidationWarning(!0);return}for(i=n.autoMap(v),i.Id=v.id,i.Files=[],r=0;r<v.files().length;r++)i.Files.push(v.files()[r].id);o={requestUri:n.odata.getUrl(n.odata.entitySet.submissionFilesModel,v.id),method:"PUT",headers:{Prefer:"return-content"},progressIndicatorTimeout:0,data:i};t.request(o,function(t){n.url.navigateTo(e.submissionSummary.format(t.Id))})}}function p(i){if(i.length==0)return!0;var r=n.odata.getUrl(n.odata.entitySet.files,{filter:n.odata.buildContainsQuery("Id",i)});return t.read({requestUri:r,showProgressIndicator:!1},function(t){for(var r=[],i=0;i<t.value.length;i++)r.push(n.autoMap(new o,t.value[i]));v.files(r)})}function w(){return i.Deferred(function(i){var r=n.odata.getUrl(n.odata.entitySet.submissionFilesModel,v.id);t.read({requestUri:r,showProgressIndicator:!1},function(n){i.resolve(n)})}).promise()}function b(){f.getCurrentRoleDescriptor().done(function(n){v.submissionListUrl=n.submissionListUrl})}var v=this;v.id=r;v.trackId=null;v.trackName=h;v.isSingleTrackConference=c;v.fileIds=l;v.titleTitle="Title";v.settings={submissionMinFileNumber:n.autoMap(),submissionMaxFileNumber:n.autoMap(),submissionAllowedFileTypes:n.autoMap(),submissionMaxFileSize:n.autoMap()};n.autoMap(v.settings,a);v.bindTo=function(t){n.showProgress();var r=i.Deferred();y();i.when(w(),b(),p(v.fileIds)).done(function(i){n.autoMap(v,i);ko.applyBindingsAndShow(v,t);r.resolve()});r.always(n.hideProgress)}}var e;n.submissionFileDetails=function(n,t,i,r,u,f,o){e=u;new s(n,t,i,r,f,o).bindTo("submissionFileDetailsForm")}}(window.app,window.OData,window.jQuery,window.setTimeout,window.FileReader!=undefined,new window.app.RoleService),function(n,t,i,r,u,f){"use strict";function o(){var t=this;t.id=n.autoMap();t.originalName=n.autoMap();t.size=n.autoMap();t.formattedSize=n.autoMap();t.uploadDate=n.autoMap();t.downloadLink=n.autoMap()}function s(r){function h(){return t.read(n.odata.getUrl(n.odata.entitySet.submissionSettings,s.trackId),function(t){n.autoMap(s.settings,t);s.settings.titleMapping!=null&&(s.titleTitle=s.settings.titleMapping)})}function c(){function h(){var n=!0;return s.files().length>s.settings.inplaceRevisionMaxFileNumber&&(s.showFilesMaxErrorMessage(!0),n=!1),s.files().length<s.settings.inplaceRevisionMinFileNumber&&(s.showFilesMinErrorMessage(!0),n=!1),n}function r(t){var h,r,o,u;if(s.files().length+t.length>s.settings.inplaceRevisionMaxFileNumber){n.addMessage("You can upload up to {0} files only.".format(s.settings.inplaceRevisionMaxFileNumber),null,"error");return}for(h=[],r=0;r<s.files().length;r++)h[s.files()[r].originalName.toLowerCase()]=!0;for(r=0;r<t.length;r++)o=t[r],c(o,h)&&(u=i.ajaxSettings.xhr(),u.open("POST",e.fileUpload,!0),u.setRequestHeader("Accept","application/json"),u.setRequestHeader("File-Name",encodeURIComponent(o.name)),u.send(o),u.addEventListener("load",function(t){t.target.status==200?f(t.target.responseText):n.processXmlHttpRequestError(t.target)},!1))}function c(t,i){var u=t.name.toLowerCase(),r;if(i[u]===undefined)i[u]=!0;else return n.addMessage("Found at least two files with the same name: '{0}'.".format(t.name),null,"error"),!1;if(t.size>s.settings.inplaceRevisionMaxFileSize*1048576)return n.addMessage("File '{0}' is bigger than maximum allowed size of {1} Mb.".format(t.name,s.settings.inplaceRevisionMaxFileSize),null,"error"),!1;var f=t.name.substr(t.name.lastIndexOf(".")+1).toLowerCase(),e=s.settings.inplaceRevisionAllowedFileTypes.split(","),o=!1;for(r=0;r<e.length;r++)if(e[r].trim().toLowerCase()==f){o=!0;break}return o?!0:(n.addMessage("File '{0}' has type '{1}' which is not accepted. We accept '{2}' only.".format(t.name,f,s.settings.inplaceRevisionAllowedFileTypes),null,"error"),!1)}function f(t){var r,i;try{r=ko.utils.parseJson(t)}catch(u){n.processException(u);return}i=n.autoMap(new o,r);i.uploadDate=new Date(i.uploadDate);isNaN(i.uploadDate)&&(i.uploadDate=new Date);s.files.push(i)}s.title=n.autoMap();s.trackName="";s.submissionListUrl=null;s.showValidationWarning=ko.observable(!1);s.showFilesMinErrorMessage=ko.observable(!1);s.showFilesMaxErrorMessage=ko.observable(!1);s.files=ko.observableArray();s.removeFile=function(n){s.files.remove(n)};s.uploadFile=function(){var n=i('<input type="file" accept="*" multiple="" />');n.on("change",function(){r(this.files)});n.trigger("click")};s.canUploadMoreFiles=ko.computed(function(){return s.files().length<s.settings.inplaceRevisionMaxFileNumber});s.xhrUploadSupported=function(){return u};s.fileUploadDragOver=function(n,t){s.canUploadMoreFiles()&&i(t.target).addClass("dragOver")};s.fileUploadDragLeave=function(n,t){s.canUploadMoreFiles()&&i(t.target).removeClass("dragOver")};s.fileUploadDrop=function(n,t){if(s.canUploadMoreFiles()){var i=t.originalEvent.dataTransfer.files;r(i);s.fileUploadDragLeave(n,t)}};s.uploadSingleFile=function(n,t){t.target.value!=""&&t.target.form.submit()};s.parseSingleUploadResult=function(n,t){f(t.target.contentDocument.body.innerText)};s.save=function(){var u=!0,f=ko.validation.group(s,{deep:!1}),i,r,o;if(f().length>0&&(f.showAllMessages(),u=!1),h()||(u=!1),!u){s.showValidationWarning(!0);return}for(i=n.autoMap(s),i.Id=s.id,i.Files=[],r=0;r<s.files().length;r++)i.Files.push(s.files()[r].id);o={requestUri:n.odata.getUrl(n.odata.entitySet.inplaceRevision,s.id),method:"PUT",headers:{Prefer:"return-content"},progressIndicatorTimeout:0,data:i};t.request(o,function(t){n.url.navigateTo(e.submissionSummary.format(t.Id))})}}function l(t){return i.Deferred(function(r){n.autoMap(s,t);var u=a(),f=y(t.Files);i.when(u,f).done(function(){r.resolve()});n.url.hash.getValue()=="saved"&&(n.url.hash.remove(),n.addMessage("Revision '{0}' saved!".format(s.title)))}).promise()}function a(){return t.read(n.odata.getUrl(n.odata.entitySet.tracks,s.trackId),function(n){s.trackName=n.Name})}function v(){return t.read(n.odata.getUrl("Tracks",{top:0,count:"true"}),function(n){s.isSingleTrackConference=n["@odata.count"]==1})}function y(i){return i.length==0?!0:t.read(n.odata.getUrl(n.odata.entitySet.files,{filter:n.odata.buildContainsQuery("Id",i)}),function(t){for(var r=[],i=0;i<t.value.length;i++)r.push(n.autoMap(new o,t.value[i]));s.files(r)})}function p(){return i.Deferred(function(i){t.read(n.odata.getUrl(n.odata.entitySet.inplaceRevision,s.id),function(n){i.resolve(n)})}).promise()}var s=this;s.id=r;s.trackId=null;s.titleTitle="Title";s.settings={inplaceRevisionMinFileNumber:n.autoMap(),inplaceRevisionMaxFileNumber:n.autoMap(),inplaceRevisionAllowedFileTypes:n.autoMap(),inplaceRevisionMaxFileSize:n.autoMap(),titleMapping:n.autoMap()};s.bindTo=function(n){p().done(function(t){t&&(s.trackId=t.TrackId);h().done(function(){var r,u;c();r=i.Deferred();f.getCurrentRoleDescriptor().done(function(n){s.submissionListUrl=n.submissionListUrl;r.resolve()});u=i.when(r,l(t),v());u.done(function(){ko.applyBindingsAndShow(s,n)})})})}}var e;n.inplaceRevisionDetails=function(n,t,i){e=t;new s(n).bindTo(i)}}(window.app,window.OData,window.jQuery,window.setTimeout,window.FileReader!=undefined,new window.app.RoleService),function(n,t,i,r,u,f){"use strict";function o(){var t=this;t.id=n.autoMap();t.originalName=n.autoMap();t.size=n.autoMap();t.formattedSize=n.autoMap();t.uploadDate=n.autoMap();t.downloadLink=n.autoMap()}function s(r){function h(){var i=n.odata.getUrl(n.odata.entitySet.cameraReadySubmissionSettings,s.trackId);return t.read({requestUri:i,showProgressIndicator:!1},function(t){n.autoMap(s.settings,t);s.settings.titleMapping!=null&&(s.titleTitle=s.settings.titleMapping)})}function c(){function h(){var n=!0;return s.files().length>s.settings.copyrightMaxFileNumber&&(s.showFilesMaxErrorMessage(!0),n=!1),s.files().length<s.settings.copyrightMinFileNumber&&(s.showFilesMinErrorMessage(!0),n=!1),n}function r(t){var h,r,o,u;if(s.files().length+t.length>s.settings.copyrightMaxFileNumber){n.addMessage("You can upload up to {0} files only.".format(s.settings.copyrightMaxFileNumber),null,"error");return}for(h=[],r=0;r<s.files().length;r++)h[s.files()[r].originalName.toLowerCase()]=!0;for(r=0;r<t.length;r++)o=t[r],c(o,h)&&(s.uploading(s.uploading()+1),u=i.ajaxSettings.xhr(),u.open("POST",e.fileUpload,!0),u.setRequestHeader("Accept","application/json"),u.setRequestHeader("File-Name",encodeURIComponent(o.name)),u.send(o),u.addEventListener("load",function(t){t.target.status==200?f(t.target.responseText):n.processXmlHttpRequestError(t.target);s.uploading(s.uploading()-1)},!1))}function c(t,i){var u=t.name.toLowerCase(),r;if(i[u]===undefined)i[u]=!0;else return n.addMessage("Found at least two files with the same name: '{0}'.".format(t.name),null,"error"),!1;if(t.size>s.settings.copyrightMaxFileSize*1048576)return n.addMessage("File '{0}' is bigger than maximum allowed size of {1} Mb.".format(t.name,s.settings.copyrightMaxFileSize),null,"error"),!1;var f=t.name.substr(t.name.lastIndexOf(".")+1).toLowerCase(),e=s.settings.copyrightAllowedFileTypes.split(","),o=!1;for(r=0;r<e.length;r++)if(e[r].trim().toLowerCase()==f){o=!0;break}return o?!0:(n.addMessage("File '{0}' has type '{1}' which is not accepted. We accept '{2}' only.".format(t.name,f,s.settings.copyrightAllowedFileTypes),null,"error"),!1)}function f(t){var r,i;try{r=ko.utils.parseJson(t)}catch(u){n.processException(u);return}i=n.autoMap(new o,r);i.uploadDate=new Date(i.uploadDate);isNaN(i.uploadDate)&&(i.uploadDate=new Date);s.files.push(i)}s.title=n.autoMap();s.trackName="";s.submissionListUrl=null;s.showFilesMinErrorMessage=ko.observable(!1);s.showFilesMaxErrorMessage=ko.observable(!1);s.showValidationWarning=ko.observable(!1);s.files=ko.observableArray();s.removeFile=function(n){s.files.remove(n)};s.uploading=ko.observable(0);s.uploadFile=function(){var n=i('<input type="file" accept="*" multiple="" />');n.on("change",function(){r(this.files)});n.trigger("click")};s.canUploadMoreFiles=ko.computed(function(){return s.uploading()==0&&s.files().length<s.settings.copyrightMaxFileNumber});s.xhrUploadSupported=function(){return u};s.fileUploadDragOver=function(n,t){s.canUploadMoreFiles()&&i(t.target).addClass("dragOver")};s.fileUploadDragLeave=function(n,t){s.canUploadMoreFiles()&&i(t.target).removeClass("dragOver")};s.fileUploadDrop=function(n,t){if(s.canUploadMoreFiles()){var i=t.originalEvent.dataTransfer.files;r(i);s.fileUploadDragLeave(n,t)}};s.uploadSingleFile=function(n,t){t.target.value!=""&&t.target.form.submit()};s.parseSingleUploadResult=function(n,t){f(t.target.contentDocument.body.innerText)};s.save=function(){var u=!0,f=ko.validation.group(s,{deep:!1}),i,r,e;if(f().length>0&&(f.showAllMessages(),u=!1),h()||(u=!1),!u){s.showValidationWarning(!0);return}for(i=n.autoMap(s),i.Id=s.id,i.Files=[],r=0;r<s.files().length;r++)i.Files.push(s.files()[r].id);e={requestUri:n.odata.getUrl(n.odata.entitySet.copyrights,s.id),method:"PUT",headers:{Prefer:"return-content"},progressIndicatorTimeout:0,data:i};t.request(e,function(){n.url.navigateTo(s.submissionListUrl)})}}function l(t){return i.Deferred(function(r){n.autoMap(s,t);var u=a(),f=y(t.Files);i.when(u,f).done(function(){r.resolve()});n.url.hash.getValue()=="saved"&&(n.url.hash.remove(),n.addMessage("Copyright Form '{0}' saved!".format(s.title)))}).fail(function(){dfr.reject()}).promise()}function a(){var i=n.odata.getUrl(n.odata.entitySet.tracks,s.trackId);return t.read({requestUri:i,showProgressIndicator:!1},function(n){s.trackName=n.Name})}function v(){var i=n.odata.getUrl("Tracks",{top:0,count:"true"});return t.read({requestUri:i,showProgressIndicator:!1},function(n){s.isSingleTrackConference=n["@odata.count"]==1})}function y(i){if(i.length==0)return!0;var r=n.odata.getUrl(n.odata.entitySet.files,{filter:n.odata.buildContainsQuery("Id",i)});return t.read({requestUri:r,showProgressIndicator:!1},function(t){for(var r=[],i=0;i<t.value.length;i++)r.push(n.autoMap(new o,t.value[i]));s.files(r)})}function p(){return i.Deferred(function(i){var r=n.odata.getUrl(n.odata.entitySet.copyrights,s.id);t.read({requestUri:r,showProgressIndicator:!1},function(n){i.resolve(n)}).fail(function(){i.reject()})}).promise()}var s=this;s.id=r;s.titleTitle="Title";s.settings={copyrightMinFileNumber:n.autoMap(),copyrightMaxFileNumber:n.autoMap(),copyrightAllowedFileTypes:n.autoMap(),copyrightMaxFileSize:n.autoMap(),titleMapping:n.autoMap()};s.ecfUrl=function(){return e.ecf.format(s.id)};s.bindTo=function(t){n.showProgress();var r=i.Deferred();p().done(function(n){n&&(s.trackId=n.TrackId);h().done(function(){c();i.when(f.getCurrentRoleDescriptor(),l(n),v()).done(function(n){s.submissionListUrl=n.submissionListUrl;ko.applyBindingsAndShow(s,t)}).always(r.resolve)})});r.always(n.hideProgress)}}var e;n.copyrightDetails=function(n,t,i){e=t;new s(n).bindTo(i)}}(window.app,window.OData,window.jQuery,window.setTimeout,window.FileReader!=undefined,new window.app.RoleService),function(n,t,i,r,u,f){"use strict";function o(){var t=this;t.id=n.autoMap();t.originalName=n.autoMap();t.size=n.autoMap();t.formattedSize=n.autoMap();t.uploadDate=n.autoMap();t.downloadLink=n.autoMap()}function s(r){function h(){return t.read(n.odata.getUrl(n.odata.entitySet.submissionSettings,s.trackId),function(t){n.autoMap(s.settings,t);s.settings.titleMapping!=null&&(s.titleTitle=s.settings.titleMapping)})}function c(){function h(){var n=!0;return s.files().length>s.settings.referenceMaxFileNumber&&(s.showFilesMaxErrorMessage(!0),n=!1),s.files().length<s.settings.referenceMinFileNumber&&(s.showFilesMinErrorMessage(!0),n=!1),n}function r(t){var h,r,o,u;if(s.files().length+t.length>s.settings.referenceMaxFileNumber){n.addMessage("You can upload up to {0} files only.".format(s.settings.referenceMaxFileNumber),null,"error");return}for(h=[],r=0;r<s.files().length;r++)h[s.files()[r].originalName.toLowerCase()]=!0;for(r=0;r<t.length;r++)o=t[r],c(o,h)&&(u=i.ajaxSettings.xhr(),u.open("POST",e.fileUpload,!0),u.setRequestHeader("Accept","application/json"),u.setRequestHeader("File-Name",encodeURIComponent(o.name)),u.send(o),u.addEventListener("load",function(t){t.target.status==200?f(t.target.responseText):n.processXmlHttpRequestError(t.target)},!1))}function c(t,i){var u=t.name.toLowerCase(),r;if(i[u]===undefined)i[u]=!0;else return n.addMessage("Found at least two files with the same name: '{0}'.".format(t.name),null,"error"),!1;if(t.size>s.settings.referenceMaxFileSize*1048576)return n.addMessage("File '{0}' is bigger than maximum allowed size of {1} Mb.".format(t.name,s.settings.referenceMaxFileSize),null,"error"),!1;var f=t.name.substr(t.name.lastIndexOf(".")+1).toLowerCase(),e=s.settings.referenceAllowedFileTypes.split(","),o=!1;for(r=0;r<e.length;r++)if(e[r].trim().toLowerCase()==f){o=!0;break}return o?!0:(n.addMessage("File '{0}' has type '{1}' which is not accepted. We accept '{2}' only.".format(t.name,f,s.settings.referenceAllowedFileTypes),null,"error"),!1)}function f(t){var r,i;try{r=ko.utils.parseJson(t)}catch(u){n.processException(u);return}i=n.autoMap(new o,r);i.uploadDate=new Date(i.uploadDate);isNaN(i.uploadDate)&&(i.uploadDate=new Date);s.files.push(i)}s.title=n.autoMap();s.trackName="";s.showValidationWarning=ko.observable(!1);s.showFilesMinErrorMessage=ko.observable(!1);s.showFilesMaxErrorMessage=ko.observable(!1);s.files=ko.observableArray();s.removeFile=function(n){s.files.remove(n)};s.uploadFile=function(){var n=i('<input type="file" accept="*" multiple="" />');n.on("change",function(){r(this.files)});n.trigger("click")};s.canUploadMoreFiles=ko.computed(function(){return s.files().length<s.settings.referenceMaxFileNumber});s.xhrUploadSupported=function(){return u};s.fileUploadDragOver=function(n,t){s.canUploadMoreFiles()&&i(t.target).addClass("dragOver")};s.fileUploadDragLeave=function(n,t){s.canUploadMoreFiles()&&i(t.target).removeClass("dragOver")};s.fileUploadDrop=function(n,t){if(s.canUploadMoreFiles()){var i=t.originalEvent.dataTransfer.files;r(i);s.fileUploadDragLeave(n,t)}};s.uploadSingleFile=function(n,t){t.target.value!=""&&t.target.form.submit()};s.parseSingleUploadResult=function(n,t){f(t.target.contentDocument.body.innerText)};s.cancel=function(){n.url.navigateTo(e.referenceConsole)};s.save=function(){var u=!0,f=ko.validation.group(s,{deep:!1}),i,r,o;if(f().length>0&&(f.showAllMessages(),u=!1),h()||(u=!1),!u){s.showValidationWarning(!0);return}for(i=n.autoMap(s),i.Id=s.id,i.Files=[],r=0;r<s.files().length;r++)i.Files.push(s.files()[r].id);o={requestUri:n.odata.getUrl(n.odata.entitySet.referenceModels,s.id),method:"PUT",headers:{Prefer:"return-content"},progressIndicatorTimeout:0,data:i};t.request(o,function(){n.url.navigateTo(e.referenceConsole)})}}function l(t){return i.Deferred(function(r){n.autoMap(s,t);var u=a(),f=y(t.Files);i.when(u,f).done(function(){r.resolve()});n.url.hash.getValue()=="saved"&&(n.url.hash.remove(),n.addMessage("Reference '{0}' saved!".format(s.title)))}).promise()}function a(){return t.read(n.odata.getUrl(n.odata.entitySet.tracks,s.trackId),function(n){s.trackName=n.Name})}function v(){return t.read(n.odata.getUrl("Tracks",{top:0,count:"true"}),function(n){s.isSingleTrackConference=n["@odata.count"]==1})}function y(i){return i.length==0?!0:t.read(n.odata.getUrl(n.odata.entitySet.files,{filter:n.odata.buildContainsQuery("Id",i)}),function(t){for(var r=[],i=0;i<t.value.length;i++)r.push(n.autoMap(new o,t.value[i]));s.files(r)})}function p(){return i.Deferred(function(i){t.read(n.odata.getUrl(n.odata.entitySet.referenceModels,s.id),function(n){i.resolve(n)})}).promise()}var s=this;s.id=r;s.trackId=null;s.titleTitle="Title";s.settings={referenceMinFileNumber:n.autoMap(),referenceMaxFileNumber:n.autoMap(),referenceAllowedFileTypes:n.autoMap(),referenceMaxFileSize:n.autoMap(),titleMapping:n.autoMap()};s.bindTo=function(n){p().done(function(t){t&&(s.trackId=t.TrackId);h().done(function(){var r,u;c();r=i.Deferred();f.getCurrentRoleDescriptor().done(function(){r.resolve()});u=i.when(r,l(t),v());u.done(function(){ko.applyBindingsAndShow(s,n)})})})}}var e;n.referenceDetails=function(n,t,i){e=t;new s(n).bindTo(i)}}(window.app,window.OData,window.jQuery,window.setTimeout,window.FileReader!=undefined,new window.app.RoleService),function(n,t,i){"use strict";function r(){function r(r){i.read(t.odata.getUrl(t.odata.entitySet.userSettingsModels,-1),function(i){t.autoMap(n,i);r()})}var n=this;n.emailNotificationNewSubmission=ko.observable(!1).autoMap();n.emailNotificationUpdateSubmission=ko.observable(!1).autoMap();n.emailNotificationDeleteSubmission=ko.observable(!1).autoMap();n.emailNotificationDiscussion=ko.observable(!1).autoMap();n.ccChairsOnMyEmail=ko.observable(!1).autoMap();n.showOneMessagePerSession=ko.observable(!1).autoMap();n.seniorMetaReviewerEmailNotificationDiscussionOff=ko.observable(!1).autoMap();n.metaReviewerEmailNotificationDiscussionOff=ko.observable(!1).autoMap();n.metaReviewerEmailNotificationReviewOff=ko.observable(!1).autoMap();n.save=function(){var r=ko.validation.group(n),u,f;return r().length>0?(r.showAllMessages(),!1):(u=t.autoMap(n),f={requestUri:t.odata.getUrl(t.odata.entitySet.userSettingsModels,-1),method:"PUT",data:u},i.request(f,function(){t.addMessage("User settings have been saved!")}),!1)};n.bindTo=function(t){function i(){ko.applyBindingsAndShow(n,t)}r(i)}}t.userSettings=function(n){(new r).bindTo(n)}}(window.jQuery,window.app,window.OData),function(n,t,i,r,u){"use strict";function f(){var n=this;n.id=t.autoMap();n.name=t.autoMap();n.reviewVisibleToAuthor=t.autoMap();n.metaReviewVisibleToAuthor=t.autoMap();n.isRevision=t.autoMap();n.isDeskReject=t.autoMap();n.isWithdrawn=t.autoMap();n.isMajorRevision=t.autoMap();n.embedded=t.autoMap()}function e(r,u){var f=this,e;f.id=null;f.trackId=u;f.name=ko.observable().extend({required:"Please, enter a name"}).autoMap();f.reviewVisibleToAuthor=ko.observable().autoMap();f.metaReviewVisibleToAuthor=ko.observable().autoMap();f.embedded=ko.observable().autoMap();f.createNew=ko.observable();e=null;f.editInDialog=function(i){return f.id=i.id,t.autoMap(f,i),f.createNew(!i.id),n(r).modal("show"),e=n.Deferred(),e.promise()};f.save=function(){var s=!0,h=ko.validation.group(f,{deep:!0}),o,c;(h().length>0&&(h.showAllMessages(),s=!1),s)&&(o=t.autoMap(f),f.createNew()?o.TrackId=u:o.Id=f.id,c={requestUri:t.odata.getUrl(t.odata.entitySet.statuses,f.createNew()?null:f.id),method:f.createNew()?"POST":"PUT",data:o},i.request(c,function(){n(r).modal("hide");t.addMessage("Status '{0}' saved!".format(f.name()));e&&e.resolve()},function(n){i.defaultError(n)}))};f.bind=function(){ko.applyBindings(f,r)}}function o(o){function c(n){h||(h=new e(r.getElementById("editDialog"),s.trackId),h.bind());h.editInDialog(n).done(l)}function l(){return i.read(t.odata.getUrl(t.odata.entitySet.statuses+"?$filter=TrackId eq "+o),function(n){s.statuses.removeAll();for(var i=0;i<n.value.length;i++)s.statuses.push(t.autoMap(new f,n.value[i]))})}var s=this,h=null;s.trackId=o;s.statuses=ko.observableArray();s.delete=function(n){if(u("Are you sure you want to delete the status?")){var r={requestUri:t.odata.getUrl(t.odata.entitySet.statuses,n.id),method:"DELETE"};i.request(r,function(){s.statuses.remove(n)},function(n){n.response.statusCode==409?t.addMessage("Status that you are trying to delete is being used by papers, please contact CMT.",null,"error"):i.defaultError(n)})}};s.edit=function(n){c(n)};s.addStatus=function(){c(t.autoMap(new f,{ReviewVisibleToAuthor:!0,MetaReviewVisibleToAuthor:!0}))};s.bindTo=function(t){l().done(function(){ko.applyBindingsAndShow(s,t);n("#menuSiteFeatures").addClass("in")})}}t.formStatus=function(n,t){new o(n).bindTo(t)}}(window.jQuery,window.app,window.OData,window.document,window.confirm),function(n,t,i,r,u){"use strict";function f(){var n=this;n.id=t.autoMap();n.name=t.autoMap();n.visibleToAuthor=t.autoMap();n.visibleToMetaReviewer=t.autoMap()}function e(r){var u=this,f;u.id=null;u.name=ko.observable().extend({required:"Please, enter a name"}).autoMap();u.visibleToAuthor=ko.observable().autoMap();u.visibleToMetaReviewer=ko.observable().autoMap();u.createNew=ko.observable();f=null;u.editInDialog=function(i){return u.id=i.id,t.autoMap(u,i),u.createNew(!i.id),n(r).modal("show"),f=n.Deferred(),f.promise()};u.save=function(){var o=!0,s=ko.validation.group(u,{deep:!0}),e,h;(s().length>0&&(s.showAllMessages(),o=!1),o)&&(e=t.autoMap(u),u.createNew()||(e.Id=u.id),h={requestUri:t.odata.getUrl(t.odata.entitySet.userTypeOptions,u.createNew()?null:u.id),method:u.createNew()?"POST":"PUT",data:e},i.request(h,function(){n(r).modal("hide");t.addMessage("UserType '{0}' saved!".format(u.name()));f&&f.resolve()},function(n){i.defaultError(n)}))};u.bind=function(){ko.applyBindings(u,r)}}function o(){function h(n){s||(s=new e(r.getElementById("editDialog")),s.bind());s.editInDialog(n).done(c)}function c(){return i.read(t.odata.getUrl(t.odata.entitySet.userTypeOptions),function(n){o.userTypes.removeAll();for(var i=0;i<n.value.length;i++)o.userTypes.push(t.autoMap(new f,n.value[i]))})}var o=this,s=null;o.userTypes=ko.observableArray();o.delete=function(n){if(u("Are you sure?")){var r={requestUri:t.odata.getUrl(t.odata.entitySet.userTypeOptions,n.id),method:"DELETE"};i.request(r,function(){o.userTypes.remove(n)},function(n){n.response.statusCode==409?t.addMessage("User type that you are trying to delete is being used, please contact CMT.",null,"error"):i.defaultError(n)})}};o.edit=function(n){h(n)};o.addUserType=function(){h(t.autoMap(new f,{}))};o.bindTo=function(t){c().done(function(){ko.applyBindingsAndShow(o,t);n("#menuConferenceDetails").addClass("in")})}}t.formUserType=function(n){t.cookies.setValue("trackId",-1,0,"/");(new o).bindTo(n)}}(window.jQuery,window.app,window.OData,window.document,window.confirm),function(n,t,i){function r(r,u,f){function s(){var t={requestUri:n.odata.getUrl(n.odata.entitySet.userTypes,u),method:"GET"};i.request(t,function(n){e.userTypeOptionId(n.UserTypeOptionId)},function(n){n.response.statusCode!=404&&i.defaultError(n)})}var e=this;for(var o of f)if(o.Id===0){o.Name="(Blank)";break}e.userTypeOptions=f;e.userTypeOptionId=ko.observable("");e.save=function(){var t={requestUri:n.odata.getUrl(n.odata.entitySet.userTypes),method:"POST",data:{UserId:u,UserTypeOptionId:e.userTypeOptionId()}};i.request(t,function(){n.addMessage("User type saved.",null,"success","text",!0);window.location.reload()},i.defaultError)};s();ko.applyBindings(e,t.getElementById(r))}n.selectUserTypePage=function(n,t,i){new r(n,t,i)}}(window.app,window.document,window.OData),function(n,t,i,r){"use strict";function u(){function f(){var n=ko.validation.group(i);return n().length>0?(n.showAllMessages(),!1):!0}var i=this,u=null;i.subject=ko.observable("").extend({required:!0}).autoMap();i.body=ko.observable("").extend({required:!0}).autoMap();i.subject("PLEASE WRITE QUICK DESCRIPTION OF ISSUE HERE");i.sendEmail=function(){if(f()){var e=n.autoMap(i),o={requestUri:n.odata.getUrl(n.odata.entitySet.emails,null,"ChairsSend"),method:"POST",data:{Request:e}};t.request(o,function(t){var i=t.value;u||(u=new n.EmailProgressViewModel(r.getElementById("showProgressDialog")),u.bind());u.showInDialog(i)})}};i.bindTo=function(n){ko.applyBindingsAndShow(i,n)}}n.chairsSendEmail=function(n){(new u).bindTo(n)}}(window.app,window.OData,window.jQuery,window.document,window.confirm,window.setTimeout),function(n,t,i,r){"use strict";function u(){function f(){var n=ko.validation.group(i);return n().length>0?(n.showAllMessages(),!1):!0}var i=this,u=null;i.subject=ko.observable("").extend({required:!0}).autoMap();i.body=ko.observable("").extend({required:!0}).autoMap();i.subject("PLEASE WRITE QUICK DESCRIPTION OF ISSUE HERE");i.sendEmail=function(){if(f()){var e=n.autoMap(i),o={requestUri:n.odata.getUrl(n.odata.entitySet.emails,null,"SupportSend"),method:"POST",data:{Request:e}};t.request(o,function(t){var i=t.value;u||(u=new n.EmailProgressViewModel(r.getElementById("showProgressDialog")),u.bind());u.showInDialog(i)})}};i.bindTo=function(n){ko.applyBindingsAndShow(i,n)}}n.supportSendEmail=function(){(new u).bindTo("sendEmailForm")}}(window.app,window.OData,window.jQuery,window.document),function(n,t,i,r){"use strict";function u(u){var f=this,e=null,o;f.fromEmail=ko.observable().autoMap();f.fromName=ko.observable().autoMap();f.toEmail=ko.observable().autoMap();f.toName=ko.observable().autoMap();f.subject=ko.observable().autoMap();f.body=ko.observable("").autoMap();o=null;f.showInDialog=function(t,r){n.autoMap(f,t);o=r;i(u).modal("show")};f.sendEmail=function(){var f={requestUri:n.odata.getUrl(n.odata.entitySet.emails,null,"ExternalReviewerSend"),method:"POST",data:{Request:o}};t.request(f,function(t){var f=t.value;i(u).modal("hide");e||(e=new n.EmailProgressViewModel(r.getElementById("showProgressDialog")),e.bind());e.showInDialog(f)})};f.bind=function(){ko.applyBindings(f,u)}}function f(f,e){function h(n,t){s||(s=new u(r.getElementById("previewEmailDialog")),s.bind());s.showInDialog(n,t)}function c(){var n=ko.validation.group(o);return n().length>0?(n.showAllMessages(),!1):!0}function l(){return t.request({requestUri:n.odata.getUrl(n.odata.entitySet.emailTemplates,null,"GetByName"),data:{Name:"External reviewer"},method:"POST"},function(n){o.subject(n.Subject);o.body(n.Body)})}function a(){return t.request({requestUri:n.odata.getUrl(n.odata.entitySet.users,o.externalReviewerId)},function(n){o.to=n.FirstName+" "+n.LastName+" <"+n.Email+">"})}var o=this,s=null;o.submissionId=f;o.externalReviewerId=e;o.to=null;o.subject=ko.observable("").extend({required:!0}).autoMap();o.body=ko.observable("").extend({required:!0}).autoMap();o.showPlaceholders=ko.observable(!1);o.previewEmail=function(){var i,r;c()&&(i=n.autoMap(o),i.SubmissionId=o.submissionId,i.ExternalReviewerId=o.externalReviewerId,r={requestUri:n.odata.getUrl(n.odata.entitySet.emails,null,"ExternalReviewerPreview"),method:"POST",data:{Request:i}},t.request(r,function(n){h(n,i)}))};o.bindTo=function(n){i.when(a(),l()).done(function(){ko.applyBindingsAndShow(o,n)})}}n.externalReviewerSendEmail=function(n,t,i){new f(n,t).bindTo(i)}}(window.app,window.OData,window.jQuery,window.document,window.confirm,window.setTimeout),function(n,t,i,r){"use strict";function u(i){function e(){var n=ko.validation.group(u);return n().length>0?(n.showAllMessages(),!1):!0}var u=this,f=null;u.subject=ko.observable("").extend({required:!0}).autoMap();u.body=ko.observable("").extend({required:!0}).autoMap();u.subject(window.cmt3.conference.name+": Reviewer Inquiry About Paper #"+i);u.sendEmail=function(){var o,s;e()&&(o=n.autoMap(u),o.SubmissionId=i,s={requestUri:n.odata.getUrl(n.odata.entitySet.emails,null,"ReviewerSendMetaReviewer"),method:"POST",data:{Request:o}},t.request(s,function(t){var i=t.value;f||(f=new n.EmailProgressViewModel(r.getElementById("showProgressDialog")),f.bind());f.showInDialog(i)}))};u.bindTo=function(n){ko.applyBindingsAndShow(u,n)}}n.reviewerSendMetaReviewerEmail=function(n){new u(n).bindTo("sendEmailForm")}}(window.app,window.OData,window.jQuery,window.document),function(n,t,i,r){"use strict";function u(i,u){function o(){var n=ko.validation.group(f);return n().length>0?(n.showAllMessages(),!1):!0}var f=this,e=null;f.subject=ko.observable("").extend({required:!0}).autoMap();f.body=ko.observable("").extend({required:!0}).autoMap();f.subject(window.cmt3.conference.name+": Author Inquiry About Paper #"+i);f.sendEmail=function(){var s,h;o()&&(s=n.autoMap(f),s.SubmissionId=i,h={requestUri:n.odata.getUrl(n.odata.entitySet.emails,null,u?"AuthorSendSeniorMetaReviewer":"AuthorSendMetaReviewer"),method:"POST",data:{Request:s}},t.request(h,function(t){var i=t.value;e||(e=new n.EmailProgressViewModel(r.getElementById("showProgressDialog")),e.bind());e.showInDialog(i)}))};f.bindTo=function(n){ko.applyBindingsAndShow(f,n)}}n.authorSendMetaReviewerEmail=function(n,t,i){new u(n,t).bindTo(i)}}(window.app,window.OData,window.jQuery,window.document),function(n,t,i,r){"use strict";function u(i,u){function o(){var n=ko.validation.group(f);return n().length>0?(n.showAllMessages(),!1):!0}var f=this,e=null;f.subject=ko.observable("").extend({required:!0}).autoMap();f.body=ko.observable("").extend({required:!0}).autoMap();f.subject(window.cmt3.conference.name+" Paper #"+i);f.sendEmail=function(){var s,h;o()&&(s=n.autoMap(f),s.SubmissionId=i,h={requestUri:n.odata.getUrl(n.odata.entitySet.emails,null,u?"MetaReviewerSendSeniorMetaReviewer":"ReviewerSendSeniorMetaReviewer"),method:"POST",data:{Request:s}},t.request(h,function(t){var i=t.value;e||(e=new n.EmailProgressViewModel(r.getElementById("showProgressDialog")),e.bind());e.showInDialog(i)}))};f.bindTo=function(n){ko.applyBindingsAndShow(f,n)}}n.sendSeniorMetaReviewerEmail=function(n,t){new u(n,t).bindTo("sendEmailForm")}}(window.app,window.OData,window.jQuery,window.document),function(n,t,i,r){"use strict";function u(i){function e(){var n=ko.validation.group(u);return n().length>0?(n.showAllMessages(),!1):!0}var u=this,f=null;u.subject=ko.observable("").extend({required:!0}).autoMap();u.body=ko.observable("").extend({required:!0}).autoMap();u.subject(window.cmt3.conference.name+" Paper #"+i);u.sendEmail=function(){var o,s;e()&&(o=n.autoMap(u),o.SubmissionId=i,s={requestUri:n.odata.getUrl(n.odata.entitySet.emails,null,"MetaReviewerSendAuthor"),method:"POST",data:{Request:o}},t.request(s,function(t){var i=t.value;f||(f=new n.EmailProgressViewModel(r.getElementById("showProgressDialog")),f.bind());f.showInDialog(i)}))};u.bindTo=function(n){ko.applyBindingsAndShow(u,n)}}n.sendAuthorEmail=function(n,t){new u(n,t).bindTo("sendEmailForm")}}(window.app,window.OData,window.jQuery,window.document),function(n,t,i,r){"use strict";function u(i,u,f){function s(){var n=ko.validation.group(e);return n().length>0?(n.showAllMessages(),!1):!0}var e=this,o=null;e.subject=ko.observable("").extend({required:!0}).autoMap();e.body=ko.observable("").extend({required:!0}).autoMap();e.subject(window.cmt3.conference.name+" Paper #"+u);e.sendEmail=function(){var h,c;s()&&(h=n.autoMap(e),h.SubmissionId=u,h.ReviewerId=f,c={requestUri:n.odata.getUrl(n.odata.entitySet.emails,null,i===n.enums.trackUserType.reviewer?"SendReviewer":i===n.enums.trackUserType.metaReviewer?"SendMetaReviewer":null),method:"POST",data:{Request:h}},t.request(c,function(t){var i=t.value;o||(o=new n.EmailProgressViewModel(r.getElementById("showProgressDialog")),o.bind());o.showInDialog(i)}))};e.bindTo=function(n){ko.applyBindingsAndShow(e,n)}}n.sendReviewerEmail=function(n,t,i){new u(n,t,i).bindTo("sendEmailForm")}}(window.app,window.OData,window.jQuery,window.document),function(n,t,i,r){"use strict";function u(i,u,f){function s(){var n=ko.validation.group(e);return n().length>0?(n.showAllMessages(),!1):!0}var e=this,o=null;e.subject=ko.observable("").extend({required:!0}).autoMap();e.body=ko.observable("").extend({required:!0}).autoMap();e.subject(window.cmt3.conference.name+" Paper #"+i);e.sendEmail=function(){var h,c;s()&&(h=n.autoMap(e),h.SubmissionId=i,h.HiddenNumber=u,c={requestUri:n.odata.getUrl(n.odata.entitySet.emails,null,f?"SendAssignedMetaReviewer":"SendAssignedReviewer"),method:"POST",data:{Request:h}},t.request(c,function(t){var i=t.value;o||(o=new n.EmailProgressViewModel(r.getElementById("showProgressDialog")),o.bind());o.showInDialog(i)}))};e.bindTo=function(n){ko.applyBindingsAndShow(e,n)}}n.sendAssignedReviewerEmail=function(n,t,i){new u(n,t,i).bindTo("sendEmailForm")}}(window.app,window.OData,window.jQuery,window.document),function(n,t,i){"use strict";function r(){var r=this;r.isFileUploaded=ko.observable(!1);r.hasError=ko.observable(!1);r.errorText=ko.observable();r.changes=ko.observableArray();r.normalChanges=ko.observableArray();r.uploading=ko.observable(!1);r.cancel=function(){window.location="/"+window.cmt3.conference.name+"/Submission/Manage"};r.getModel=function(){for(var t,u,i=[],n=0;n<r.normalChanges().length;n++)t=r.normalChanges()[n],u={SubmissionId:t.id,NewStatusId:t.newStatusId},i.push(u);return{Changes:i}};r.send=function(){var i=r.getModel(),u={requestUri:n.odata.getUrl(n.odata.entitySet.submissions,null,"BulkChangePaperStatus"),method:"POST",data:{Request:i}};t.request(u,function(){window.location="/"+window.cmt3.conference.name+"/Submission/Manage"})};r.post=function(n,t,i){var r,f,u;i=i||"post";r=document.createElement("form");r.setAttribute("method",i);r.setAttribute("action",n);for(f in t)t.hasOwnProperty(f)&&(u=document.createElement("input"),u.setAttribute("type","hidden"),u.setAttribute("name",f),u.setAttribute("value",t[f]),r.appendChild(u));document.body.appendChild(r);r.submit();document.body.removeChild(r)};r.downloadTemplate=function(){var n="/api/odata/"+window.cmt3.conference.name+"/Submissions/GetBulkChangePaperStatusTemplate";r.post(n,{})};r.uploadFile=function(n,t){t.target.value!=""&&(r.uploading(!0),t.target.form.submit())};r.parseUploadResult=function(){var t=i.parseJSON(i("#singleFileUploadFrame").contents().text()),u,n,f;if(r.changes.removeAll(),r.normalChanges.removeAll(),r.hasError(t.HasError),r.errorText(t.ErrorText),!r.hasError())for(u=0;u<t.Models.length;u++)n=t.Models[u],f={id:n.Id,title:n.Title,currentStatusId:n.CurrentStatusId,newStatusId:n.NewStatusId,currentStatus:n.CurrentStatus,newStatus:n.NewStatus,status:n.Status,hasError:n.HasError,lineNumber:n.LineNumber},r.changes.push(f),f.hasError||r.normalChanges.push(f);r.isFileUploaded(!0);r.uploading(!1)};r.bindTo=function(n){ko.applyBindingsAndShow(r,n)}}n.bulkChangePaperStatus=function(n){(new r).bindTo(n)}}(window.app,window.OData,window.jQuery,window.document,window.confirm,window.setTimeout),function(n,t,i){"use strict";function r(r){function e(){o();f=u.isChecked.subscribe(s)}function o(){f&&typeof f.dispose=="function"&&f.dispose()}function s(){u.initialState===undefined?u.initialState=u.isChecked():h.call(u)}function h(){var f=this,s,h,c;f.isToggleInProgress(!0);s={ReasonId:u.id()};s.Type=f.isChecked()?"Add":"Remove";h=n.Deferred(function(n){window.setTimeout(n.resolve,500)});c=i.request({requestUri:t.odata.getUrl(t.odata.entitySet.submissions,r,"ModifyConflict"),method:"POST",showProgressIndicator:!1,data:{Request:s}},function(){},function(n){o();u.isChecked(!u.isChecked());e();t.addErrorMessage("Unable to edit conflict."+t.odata.getErrorMessage(n))});n.when(c,h).always(function(){f.isToggleInProgress(!1)})}var u=this,f;u.id=ko.observable().autoMap();u.name=t.autoMap();u.isChecked=ko.observable();u.initialState=undefined;u.isToggleInProgress=ko.observable(!1);e()}function u(){var n=this;n.id=t.autoMap();n.trackId=t.autoMap();n.name=t.autoMap()}function f(n){var i=this;i.id=t.autoMap();i.reviewerName=t.autoMap();i.hiddenNumber=t.autoMap();i.googleScholarId=t.autoMap();i.semanticScholarId=t.autoMap();i.dblpId=t.autoMap();i.googleScholarUrl=function(){return t.enums.externalProfile.googleScholar.format(i.googleScholarId)};i.semanticScholarUrl=function(){return t.enums.externalProfile.semanticScholar.format(i.semanticScholarId)};i.dblpUrl=function(){return t.enums.externalProfile.dblp.format(i.dblpId)};i.reviewPreview=n}function e(n){var i=this;i.id=t.autoMap();i.metaReviewerName=t.autoMap();i.hiddenNumber=t.autoMap();i.metaReviewPreview=n}function o(){var n=this;n.trackId=t.autoMap();n.groupId=t.autoMap();n.groupName=t.autoMap();n.isImplicit=t.autoMap();n.peerName=t.autoMap()}function s(n,u,s,h,c,l,a,v,y,p,w,b,k,d,g,nt,tt,it,rt,ut,ft){var et=this,ot,ui,ht,fi,gt,hi,ct,ni,ti,ii,ri,pt,ei,st,lt,at,vt,yt,wt,bt,ci,li,kt,dt,ai,vi,oi,si;for(et.id=n.Id,et.title=n.Title,et.abstract=n.Abstract,et.originalSubmissionId=n.OriginalSubmissionId,et.track=n.Track,et.trackId=n.TrackId,et.primarySubject=n.PrimarySubject,et.secondarySubject=n.SecondarySubject,et.relevance=n.Relevance,et.tpmsRank=n.TpmsRank,et.customAffinityRank=n.CustomAffinityRank,et.metaBid=n.MetaBid,et.assigned=n.Assigned,et.metaReviewId=n.MetaReviewId,et.authorFeedbackId=n.AuthorFeedbackId,et.isMetaReviewReadOnly=n.IsMetaReviewReadOnly,et.isAuthorFeedback=ko.observable(n.IsAuthorFeedback),et.isCameraReadyPosted=n.IsCameraReadyPosted,et.metaBiddingEnabled=n.MetaBiddingEnabled,et.metaReviewingEnabled=n.MetaReviewingEnabled,et.notificationComplete=n.NotificationComplete,et.discussionEnabled=n.DiscussionEnabled,et.assignedSeniorMetaReviewer=n.AssignedSeniorMetaReviewer,et.submissionEnabledForDiscussion=ko.observable(n.SubmissionEnabledForDiscussion),et.filesUploaded=n.FilesUploaded,et.messages=n.Messages,et.metaReviewers=n.MetaReviewersJson?JSON.parse(n.MetaReviewersJson):[],et.completed=n.Completed,et.percentage=n.Percentage,et.numberOfReviewerNotes=n.NumberOfReviewerNotes,et.assignment=n.Assignment,et.completedReviewRating=n.CompletedReviewRating,et.percentageReviewRating=n.PercentageReviewRating,et.metaReviewerNoteId=n.MetaReviewerNoteId,et.metaReviewerNoteSubmitted=n.MetaReviewerNoteSubmitted,et.allowMetaReviewerToSeeReviewingDataAfterReviewing=n.AllowMetaReviewerToSeeReviewingDataAfterReviewing,et.doNotAllowMetaReviewerToEditNote=n.DoNotAllowMetaReviewerToEditNote,et.doNotEnableMetaReviewerNote=n.DoNotShowMetaReviewerNote,et.showMetaReviewerIdentityToReviewer=h,et.showReviewerIdentityToMetaReviewer=c,et.showMetaReviewerIdentityToOtherMetaReviewer=l,et.suggestionsEnabled=a,et.editSuggestionNotAllowed=v,et.allowMetaReviewerToAssignSubmissionToReviewer=y,et.allowMetaReviewerToInviteReviewers=p,et.allowMetaReviewerToEnableDiscussion=w,et.allowMetaReviewerToEnableAuthorFeedback=b,et.allowMetaReviewerToSeeOtherMetaReview=k,et.allowMetaReviewerToEmailAuthor=d,et.doNotAllowSharedMetaReviewerToEditRecommendation=nt,et.doNotAllowMetaReviewerToEmailReviewer=g,et.reviewQuestions=ut,et.metaReviewQuestions=ft,et.sharedMetaReviewerRecommendation=ko.observable(n.SharedMetaReviewerRecommendation).autoMap(),et.sharedMetaReviewerRecommendationOptionId=ko.observable(n.SharedMetaReviewerRecommendationOptionId).autoMap(),et.agreeWithMetaReview=ko.observable(n.AgreeWithMetaReview).autoMap(),et.recommendationComment=ko.observable(n.RecommendationComment).autoMap(),et.chairNoteColumns=[],n.CNQ01Id!==null?et.chairNoteColumns.push(new t.QuestionResponseColumn(n.CNQ01Id,n.CNQ01Text)):et.chairNoteColumns.push(null),n.CNQ02Id!==null?et.chairNoteColumns.push(new t.QuestionResponseColumn(n.CNQ02Id,n.CNQ02Text)):et.chairNoteColumns.push(null),n.CNQ03Id!==null?et.chairNoteColumns.push(new t.QuestionResponseColumn(n.CNQ03Id,n.CNQ03Text)):et.chairNoteColumns.push(null),n.CNQ04Id!==null?et.chairNoteColumns.push(new t.QuestionResponseColumn(n.CNQ04Id,n.CNQ04Text)):et.chairNoteColumns.push(null),ot=0,ui=[],ot=0;ot<tt.length;ot++)ui.push(et.chairNoteColumns[ot]);for(et.chairNoteColumns=ui,ht={},n.MRNQ01Id!==null&&(ht[1]=new t.QuestionResponseColumn(n.MRNQ01Id,n.MRNQ01Text)),n.MRNQ02Id!==null&&(ht[2]=new t.QuestionResponseColumn(n.MRNQ02Id,n.MRNQ02Text)),n.MRNQ03Id!==null&&(ht[3]=new t.QuestionResponseColumn(n.MRNQ03Id,n.MRNQ03Text)),n.MRNQ04Id!==null&&(ht[4]=new t.QuestionResponseColumn(n.MRNQ04Id,n.MRNQ04Text)),n.MRNQ05Id!==null&&(ht[5]=new t.QuestionResponseColumn(n.MRNQ05Id,n.MRNQ05Text)),n.MRNQ06Id!==null&&(ht[6]=new t.QuestionResponseColumn(n.MRNQ06Id,n.MRNQ06Text)),n.MRNQ07Id!==null&&(ht[7]=new t.QuestionResponseColumn(n.MRNQ07Id,n.MRNQ07Text)),n.MRNQ08Id!==null&&(ht[8]=new t.QuestionResponseColumn(n.MRNQ08Id,n.MRNQ08Text)),n.MRNQ09Id!==null&&(ht[9]=new t.QuestionResponseColumn(n.MRNQ09Id,n.MRNQ09Text)),n.MRNQ10Id!==null&&(ht[10]=new t.QuestionResponseColumn(n.MRNQ10Id,n.MRNQ10Text)),fi=[],ot=0;ot<it.length;ot++)fi.push(ht[it[ot].Order]);if(et.metaReviewerNoteColumns=fi,et.aggregateColumns=[],et.sharedSubmissionInfo=[],gt=n.SharedSubmissionInfoJson&&JSON.parse(n.SharedSubmissionInfoJson),gt)for(ot=0;ot<gt.length;ot++)et.sharedSubmissionInfo.push(t.autoMap(new o,gt[ot]));for(ot=0;ot<rt.length;ot++)hi=rt[ot],ct="Q0"+hi.Order,n[ct+"Id"]!==null?et.aggregateColumns.push(new t.AggregateColumn(ct,n[ct+"Id"],n[ct+"Avg"],n[ct+"Min"],n[ct+"Max"],n[ct+"Spread"])):et.aggregateColumns.push(new t.AggregateColumn(ct,null,null,null,null,null));for(ni=n&&n.InlineReviewJson&&JSON.parse(n.InlineReviewJson)||[],ti={},ot=0;ot<ni.length;ot++)ti[ni[ot].HiddenNumber]=ni[ot];for(ii=n&&n.InlineMetaReviewJson&&JSON.parse(n.InlineMetaReviewJson)||[],ri={},ot=0;ot<ii.length;ot++)ri[ii[ot].HiddenNumber]=ii[ot];if(et.suggestions=[],pt=n.SuggestionsJson?JSON.parse(n.SuggestionsJson):[],pt&&pt.length>0)for(ot=0;ot<pt.length;ot++)(ei=pt[ot],ei)&&et.suggestions.push(new t.Suggestion(ei));if(st=0,wt=n.ReviewersJson?JSON.parse(n.ReviewersJson):[],et.reviewers=[],wt&&wt.length>0)for(ot=0;ot<wt.length;ot++)if(bt=wt[ot],bt){if(lt=[],et.reviewQuestions&&et.reviewQuestions.length>0){for(vt=ti[bt.HiddenNumber]&&ti[bt.HiddenNumber].Question||[],at={},st=0;st<vt.length;st++)yt=vt[st],at[yt.QuestionOrder]=yt;for(st=0;st<et.reviewQuestions.length;st++)ci=et.reviewQuestions[st],lt.push(at[ci.Order])}li=t.autoMap(new f(lt),bt);et.reviewers.push(li)}if(kt=n.MetaReviewersJson?JSON.parse(n.MetaReviewersJson):[],et.metaReviewers=[],kt&&kt.length>0)for(ot=0;ot<kt.length;ot++)if(dt=kt[ot],dt){if(lt=[],et.metaReviewQuestions&&et.metaReviewQuestions.length>0){for(vt=ri[dt.HiddenNumber]&&ri[dt.HiddenNumber].Question||[],at={},st=0;st<vt.length;st++)yt=vt[st],at[yt.QuestionOrder]=yt;for(st=0;st<et.metaReviewQuestions.length;st++)ai=et.metaReviewQuestions[st],lt.push(at[ai.Order])}vi=t.autoMap(new e(lt),dt);et.metaReviewers.push(vi)}if(et.status=n.Status,et.statusPropertyIsRevision=n.StatusPropertyIsRevision,et.allowOnlyRevisionForReviewing=n.AllowOnlyRevisionForReviewing,et.metaReviewerLabel=function(){return n.HiddenNumber?"Meta-Reviewer #"+n.HiddenNumber:""},et.metaReviewerTags=n.MetaReviewerTags,et.downloadLink=function(){return et.isShared()?u.sharedSubmissionFileWithSupplemental.format(et.id):u.submissionFileWithSupplemental.format(et.id)},et.editMetaReviewUrl=function(){return et.metaReviewId?u.metaReviewDetails.format(et.metaReviewId):u.metaReviewCreate.format(et.id)},et.editMetaReviewerNoteUrl=function(){return et.metaReviewerNoteId?u.metaReviewerNoteDetails.format(et.metaReviewerNoteId):u.metaReviewerNoteCreate.format(et.id)},et.editMetaReviewerNoteText=function(){return et.metaReviewerNoteSubmitted?"Edit":"Add"},et.editMetaReviewerNoteTooltip=function(){return et.reviewerNoteSubmitted?"Edit note":"Add note"},et.viewMetaReviewerNoteUrl=function(){return et.metaReviewerNoteId?u.metaReviewerNoteView.format(et.metaReviewerNoteId):""},et.editSuggestionsUrl=function(){return u.suggestions.format(et.id)},et.assignReviewersUrl=function(){return u.assignReviewers.format(et.id)},et.viewMetaReviewUrl=function(){return et.metaReviewId?u.metaReviewView.format(et.metaReviewId):null},et.isShared=ko.pureComputed(function(){return this.sharedSubmissionInfo&&this.sharedSubmissionInfo.length>0},et),et.allowDiscussion=ko.pureComputed(function(){return(this.assigned||this.isShared())&&this.submissionEnabledForDiscussion()&&(this.discussionEnabled||this.allowMetaReviewerToSeeReviewingDataAfterReviewing)},et),et.viewAllMetaReviewsUrl=function(){return et.allowMetaReviewerToSeeOtherMetaReview||et.isShared()?u.metaReviewViewAll.format(et.id):null},et.reviewingDetailsUrl=function(){return et.allowDiscussion()?u.reviewingDetailsUrl.format(et.id):null},et.viewUrl=function(){return u.submissionSummary.format(et.id)},et.viewOriginalUrl=function(){return et.originalSubmissionId?u.submissionSummary.format(et.originalSubmissionId):null},et.cameraReadySummaryUrl=function(){return u.cameraReadySummary.format(et.id)},et.inviteReviewerUrl=function(){return u.inviteReviewer.format(et.id)},et.reviewerEmailUrl=function(n){return u.reviewerEmail.format(et.id,n)},et.assignedReviewerEmailUrl=function(n){return u.assignedReviewerEmail.format(et.id,n)},et.metaReviewerEmailUrl=function(n){return u.metaReviewerEmail.format(et.id,n)},et.assignedMetaReviewerEmailUrl=function(n){return u.assignedMetaReviewerEmail.format(et.id,n)},et.seniorMetaReviewerEmailUrl=function(){return u.seniorMetaReviewerEmail.format(et.id)},et.canSendMetaReviewerEmail=function(n){return et.id!==n},et.authorEmailUrl=function(){return u.authorEmail.format(et.id)},et.showFeed=function(){return u.feed.format(et.id)},et.viewAuthorFeedbackUrl=function(){return et.authorFeedbackId&&(et.assigned||et.isShared())?u.feedback.format(et.authorFeedbackId):null},et.setAuthorFeedbackEnable=function(n){var r=!n.isAuthorFeedback(),u={requestUri:t.odata.getUrl(t.odata.entitySet.metaBiddingReviewModels,null,"EnableDisableAuthorFeedback"),method:"POST",showProgressIndicator:!0,data:{Enable:r,SubmissionId:n.id}};i.request(u,function(){n.isAuthorFeedback(r);t.addMessage("Author feedback for submission {0} has been {1}!".format(n.id,r?"enabled":"disabled"))})},et.setDiscussionEnable=function(n){var r=!n.submissionEnabledForDiscussion(),u={requestUri:t.odata.getUrl(t.odata.entitySet.submissions,null,"EnableDisableDiscussion"),method:"POST",showProgressIndicator:!0,data:{Enable:r,SubmissionId:n.id}};i.request(u,function(){n.submissionEnabledForDiscussion(r);t.addMessage("Author feedback for submission {0} has been {1}!".format(n.id,r?"enabled":"disabled"))})},et.emailReviewersUrl=function(n){var t="Id eq {0}".format(et.id);n.navigateEmailReviewersUrl(t,!1)},et.emailAllReviewersUrl=function(n){var t="Id eq {0}".format(et.id);n.navigateEmailReviewersUrl(t,!0)},et.isConflictSelectedText=ko.pureComputed(function(){for(var n=0;n<et.metaReviewerConflictReasons.length;n++)if(et.metaReviewerConflictReasons[n].isChecked())return"Yes";return"No"}),et.metaReviewerConflictReasons=[],s&&s.conflictDeclarationAllowedTracks&&s.conflictDeclarationAllowedTracks[et.trackId]===!0&&s.conflictReasons)for(ot=0;ot<s.conflictReasons.length;ot++)oi=s.conflictReasons[ot],si=t.autoMap(new r(et.id),oi),si.isChecked(n&&n.ConflictReasonIds&&n.ConflictReasonIds.indexOf(oi.Id)>-1),et.metaReviewerConflictReasons.push(si)}function h(r,u){var e=u,f=this;f.submissionCount=ko.observable(0);f.selectedMetaBid=ko.observable(1);f.metaBidOptions=[{name:"Not Entered",id:1},{name:"Not Willing",id:2},{name:"In A Pinch",id:3},{name:"Willing",id:4},{name:"Eager",id:5}];f.submitEnabled=ko.computed(function(){return f.submissionCount()<=0?!1:f.selectedMetaBid()!==null&&typeof f.selectedMetaBid()!="undefined"});f.changeMetaBid=function(){var o={Filter:f.filter,MetaBid:f.selectedMetaBid(),ShowMetaBidding:u.showMetaBidding(),ShowMetaReviewing:u.showMetaReviewing()},s={requestUri:t.odata.getUrl(t.odata.entitySet.metaBiddingReviewModels,null,"BulkChangeMetaBid"),method:"POST",showProgressIndicator:!0,data:{Request:o}};i.request(s,function(){e.refresh();setTimeout(function(){t.addMessage("The bid of selected submissions have been changed.")},500);n(r).modal("hide")})};f.bind=function(){ko.applyBindings(f,r)};f.filter=null;f.editInDialog=function(e){f.filter=e;var o={Filter:e,ShowMetaBidding:u.showMetaBidding(),ShowMetaReviewing:u.showMetaReviewing()},s={requestUri:t.odata.getUrl(t.odata.entitySet.metaBiddingReviewModels,null,"SubmissionCountFilteredMetaBidding"),method:"POST",data:{Request:o}};i.request(s,function(t){f.submissionCount(t.value);f.selectedMetaBid(null);n(r).modal("show")})}}function c(r,u){var e=u,f=this;f.submissionCount=ko.observable(0);f.bind=function(){ko.applyBindings(f,r)};f.editInDialog=function(f){var e={Filter:f,ShowMetaBidding:u.showMetaBidding(),ShowMetaReviewing:u.showMetaReviewing()},o={requestUri:t.odata.getUrl(t.odata.entitySet.metaBiddingReviewModels,null,"BidSummaryFilteredMetaBidding"),method:"POST",data:{Request:e}};i.request(o,function(t){var i=t.value;n("#imagemetabids").html('<img src="data:image/png;base64,'+i+'" />');n(r).modal("show")})}}t.MetaBiddingPage=function(r,f,e,o,s,l,a,v,y,p,w,b,k,d,g,nt,tt,it){function ot(r){var f=this;f.recommendationComment=ko.observable("").extend({maxLength:300});f.bind=function(){ko.applyBindings(f,r)};f.recommendationOptions=ko.observableArray([]);f.viewRecommendationOptions={};f.selectedSharedMetaReviewerRecommendation=ko.observable(null);f.sid=ko.observable(0);f.agreeWithMetaReview=ko.observable(!1);f.data=null;f.editInDialog=function(e){f.data=e;f.recommendationComment(e.recommendationComment());f.sid(e.id);f.recommendationOptions([]);f.viewRecommendationOptions={};f.agreeWithMetaReview(!1);i.read(t.odata.getUrl(t.odata.entitySet.sharedMetaReviewerRecommendationOptions+"?$filter=TrackId eq "+e.trackId),function(i){for(var h,s,o=0;o<i.value.length;o++)h=i.value[o],s=t.autoMap(new u,h),f.recommendationOptions.push(s),f.viewRecommendationOptions[s.id]=s;f.selectedSharedMetaReviewerRecommendation(e.sharedMetaReviewerRecommendationOptionId());f.agreeWithMetaReview(e.agreeWithMetaReview());n(r).modal("show")})};f.saveRecommendation=function(){var u={requestUri:t.odata.getUrl(t.odata.entitySet.submissions,null,"ChangeSharedMetaReviewerRecommendation"),method:"POST",showProgressIndicator:!0,data:{Request:{SubmissionId:f.sid(),RecommendationOptionId:f.selectedSharedMetaReviewerRecommendation()||null,AgreeWithMetaReview:f.agreeWithMetaReview(),RecommendationComment:f.recommendationComment()}}};i.request(u,function(t){t&&(f.data.sharedMetaReviewerRecommendation(f.viewRecommendationOptions[t.value].name),f.data.sharedMetaReviewerRecommendationOptionId(t.value),f.data.agreeWithMetaReview(f.agreeWithMetaReview()),f.data.recommendationComment(f.recommendationComment()));n(r).modal("hide")})}}var rt=this,ut,ft,et;rt.chairNoteQuestions=v;rt.metaReviewerNoteQuestions=y;rt.questions=p;rt.$element=n(r);rt.conference=window.cmt3.conference.name;rt.page=ko.observable(1);rt.top=ko.observable(25);rt.sort=ko.observable("Id");rt.controller=f;rt.metaReviewerId=l;rt.filters=[];rt._total=ko.observable(0);rt.selected=ko.observable(0);rt.metaBiddingModels=ko.observableArray();rt.metaBid=ko.observable();rt.editingMetaBid=ko.observable(!1);rt.listen();rt.Pager=ko.pager(rt.selected,rt.top);rt.Pager().CurrentPage.subscribe(function(){rt.page(rt.Pager().CurrentPage());rt.show()});rt.pageUrls=o;rt.showMetaReviewerIdentityToReviewer=ko.observable(!1);rt.showReviewerIdentityToMetaReviewer=ko.observable(!1);rt.showMetaReviewerIdentityToOtherMetaReviewer=ko.observable(!1);rt.suggestionsEnabled=ko.observable(!1);rt.allowMetaReviewerToEnableDiscussion=ko.observable(!1);rt.allowMetaReviewerToEnableAuthorFeedback=ko.observable(!1);rt.allowMetaReviewerToRateReview=ko.observable(!1);rt.doNotAllowSharedMetaReviewerToEditRecommendation=ko.observable(!1);rt.doNotAllowMetaReviewerToEmailReviewer=ko.observable(!1);rt.toggleableColumnsContainer=new t.ToggleableColumnsContainer(rt.key);rt.reviewQuestions=w;rt.metaReviewQuestions=k;rt.toggleableColumnsContainer.setDefaultHiddenColumnKeys(e);rt.showInlineReview=function(n){return b&&b.length>0&&(!n||b.indexOf(n)!==-1)};rt.showReviewingDataAfterReviewing=function(n){return nt&&nt.indexOf(n)!==-1};rt.hasMetaReviewerNoteQuestion=function(n){return it&&it.indexOf(n)!==-1};rt.hasReviewerNoteQuestion=function(n){return tt&&tt.indexOf(n)!==-1};rt.showInlineMetaReview=function(n){return d&&d.length>0&&(!n||d.indexOf(n)!==-1)};rt.showTags=function(){return g&&g.length>0};rt.tagOptionNamesProvider=function(){return g};rt.importMetaReviewsLink=function(){return rt.pageUrls.importMetaReviews};rt.downloadSubmissionFileLink=function(){return rt.isShared()?rt.pageUrls.sharedSubmissionFile.format(""):rt.pageUrls.submissionFile.format("")};rt.downloadAllLink=function(){return rt.isShared()?rt.pageUrls.sharedSubmissionFileWithSupplemental.format(""):rt.pageUrls.submissionFileWithSupplemental.format("")};rt.showWelcomeMessage=function(){n(document.getElementById("welcomeMessageDialog")).modal("show")};rt.submissionComparisonLink=function(){return rt.pageUrls.submissionComparison.format("")};ut=null;rt.changeMetaBid=function(n){ut===null&&(ut=new h(document.getElementById("changeMetaBidDialog"),rt),ut.bind());ut.editInDialog(n)};rt.isShared=function(){return rt.controller==="MetaSharedModels"};rt.showMetaBidding=function(){return rt.controller==="MetaBiddingModels"||rt.controller==="MetaBiddingReviewModels"};rt.showMetaReviewing=function(){return rt.controller==="MetaReviewModels"||rt.controller==="MetaBiddingReviewModels"};ft=null;rt.metaBidSummary=function(n){ft===null&&(ft=new c(document.getElementById("metaBidSummaryDialog"),rt),ft.bind());ft.editInDialog(n)};rt.params=s;rt.recommendationOptionsProvider=ko.pureComputed(function(){return a});et=null;rt.selectSharedMetaReviewerRecommendationWithComment=function(n){et===null&&(et=new ot(document.getElementById("editRecommendationDialog")),et.bind());et.editInDialog(n)}};t.MetaBiddingPage.prototype={key:"metabiddings",listen:function(){var t=this;n(document).on("data.filter",function(){t.Pager().CurrentPage()<2?t.show():t.Pager().CurrentPage(1)})},getFilter:function(){var t="";return n.each(this.filters,function(n,i){i.getValue()&&(t+=t===""?i.getValue():" and "+i.getValue())}),t},odataRequest:function(n,t,r){var u={headers:{Accept:"application/json"},requestUri:"/api/odata/"+this.conference+"/$batch",showProgressIndicator:r,method:"POST",data:{requests:[{url:n,method:"GET",headers:{Accept:"application/json"}}]}};i.request(u,function(n){var i=n.responses[0].body,r=i["@odata.count"],u=i.value;t(u,r)},function(n){window.cmt3.logger.log(n.message)},i.batchHandler)},show:function(){var i=this;if(i.initialized){t.showProgress();var r=i.sort(),u=i.top(),f=i.skip(),e=i.getFilter(),c=r?"&$orderby="+r:"",l=u?"&$top="+u:"",a=f?"&$skip="+f:"",v=e?"&$filter="+encodeURIComponent(e):"",o=new n.Deferred(function(){i.odataRequest("/api/odata/"+i.conference+"/"+i.controller+"?$count=true"+c+v+a+l,function(n,t){o.resolve({items:n,count:t})},!1)}),h=new n.Deferred(function(){i.odataRequest(t.odata.entitySet.metaReviewSettings,function(n,t){h.resolve({settings:n,settingsCount:t})},!1)});n.when(o,h).done(function(o,h){var vt=h.settings,yt=o.items;t.page.appendToState(i.key,{sort:r,top:u,skip:f,filter:e});var pt=[],et=[],c=[],l=[],a=[],ot=[],st=[],v=[],y=[],ht=[],ct=[],lt=[],p=[],at=[],w=[],b=[],k=!1,d=!1,g=!1,nt=!1,tt=!1,it=!1,rt=!1,ut=!1,ft=!1;n.each(vt,function(n,t){c[t.TrackId]=t.ShowMetaReviewerIdentityToReviewer;l[t.TrackId]=t.ShowReviewerIdentityToMetaReviewer;a[t.TrackId]=t.ShowMetaReviewerIdentityToOtherMetaReviewer;ot[t.TrackId]=t.AllowMetaReviewerToAssignSubmissionToReviewer;st[t.TrackId]=t.AllowMetaReviewerToInviteReviewers;v[t.TrackId]=t.AllowMetaReviewerToEnableDiscussion;y[t.TrackId]=t.AllowMetaReviewerToEnableAuthorFeedback;ht[t.TrackId]=t.AllowMetaReviewerToSeeOtherMetaReview;ct[t.TrackId]=t.AllowMetaReviewerToEmailAuthor;b[t.TrackId]=t.DoNotAllowMetaReviewerToEmailReviewer;lt[t.TrackId]=t.AllowMetaReviewerToRateReview;p[t.TrackId]=t.SuggestionsEnabled;at[t.TrackId]=t.EditSuggestionNotAllowed;w[t.TrackId]=t.DoNotAllowSharedMetaReviewerToEditRecommendation});n.each(yt,function(n,t){var r=new s(t,i.pageUrls,i.params,c[t.TrackId],l[t.TrackId],a[t.TrackId],p[t.TrackId],at[t.TrackId],ot[t.TrackId],st[t.TrackId],v[t.TrackId],y[t.TrackId],ht[t.TrackId],ct[t.TrackId],b[t.TrackId],w[t.TrackId],i.chairNoteQuestions,i.metaReviewerNoteQuestions,i.questions,i.reviewQuestions&&i.reviewQuestions[t.TrackId],i.metaReviewQuestions&&i.metaReviewQuestions[t.TrackId]);pt[r.id]=r;et.push(r);k=k|c[t.TrackId];d=d|l[t.TrackId];g=g|a[t.TrackId];nt=nt|p[t.TrackId];tt=tt|v[t.TrackId];it=it|y[t.TrackId];rt=rt|lt[t.TrackId];ut=ut|w[t.TrackId];ft=ft|b[t.TrackId]});i.showMetaReviewerIdentityToReviewer(k);i.showReviewerIdentityToMetaReviewer(d);i.showMetaReviewerIdentityToOtherMetaReviewer(g);i.suggestionsEnabled(nt);i.allowMetaReviewerToEnableDiscussion(tt);i.allowMetaReviewerToEnableAuthorFeedback(it);i.allowMetaReviewerToRateReview(rt);i.doNotAllowSharedMetaReviewerToEditRecommendation(ut);i.doNotAllowMetaReviewerToEmailReviewer(ft);i.metaBiddingModels(et);i._total()===0&&i._total(o.count);i.selected(o.count);i.toggleableColumnsContainer&&i.toggleableColumnsContainer.loadState();i.$element.show()}).always(t.hideProgress)}},scroll:function(){n(window).scrollTop()===n(document).height()-n(window).height()&&self.show()},selectMetaBid:function(t,i){var u=n(i.target),e=ko.contextFor(i.target),r=n(n("#metaBidTemplate").text()),f;u.hide();u.after(r);f=e.$parent.getMetaBids(t.id,u,r);ko.applyBindings(f,r[0]);r.find("select").focus()},getMetaBids:function(n,t,r){var u=[{name:"Not Entered",id:1},{name:"Not Willing",id:2},{name:"In A Pinch",id:3},{name:"Willing",id:4},{name:"Eager",id:5}],f={options:ko.observableArray(u),selectedMetaBid:ko.observable()};return f.selectedMetaBid.subscribe(function(f){var e={requestUri:"/api/odata/"+window.cmt3.conference.name+"/MetaBiddingModels("+n+")",method:"PATCH",headers:{Prefer:"return-content"},progressIndicatorTimeout:0,data:{MetaBidId:f[0]}};i.request(e,function(n){r.remove();t.text(u[n.MetaBidId-1].name);t.show()})}),f},post:function(n,t,i){var r,f,u;i=i||"post";r=document.createElement("form");r.setAttribute("method",i);r.setAttribute("action",n);for(f in t)t.hasOwnProperty(f)&&(u=document.createElement("input"),u.setAttribute("type","hidden"),u.setAttribute("name",f),u.setAttribute("value",t[f]),r.appendChild(u));document.body.appendChild(r);r.submit();document.body.removeChild(r)},stub:function(){alert("Sorry, this feature is not implemented yet.")},reset:function(){n.each(this.filters,function(n,t){t.reset()});this.show()},size:function(t,i){var r,u,f;n("a",".show").removeClass("btn-success").css("color","#999999");n(i.currentTarget).addClass("btn-success").css("color","white");r=n(i.target).attr("size");u=parseInt(r);this.top(u);f=this.Pager().CurrentPage();this.Pager().CurrentPage(1);f===1&&this.show()},skip:function(){return(this.page()-1)*this.top()},prev:function(){this.top()!==0&&this.page()!==1&&(this.page(this.page()-1),this.show())},next:function(){this.top()===0||this.page()>this.selected()/this.top()||(this.page(this.page()+1),this.show())},setSort:function(t,i){var r=n(i.target),u=r.attr("data-sort");(u===null||u===undefined)&&(r=n(r.context.parentNode),u=r.attr("data-sort"));r.hasClass("selected")?this.sort().match(" desc$")?(this.sort(u+" asc"),r.find("i").removeClass("icon-arrow-down"),r.find("i").addClass("icon-arrow-up")):(this.sort(u+" desc"),r.find("i").removeClass("icon-arrow-up"),r.find("i").addClass("icon-arrow-down")):(n("th[data-sort]").each(function(){n(this).find("i").removeClass("icon-arrow-up");n(this).find("i").removeClass("icon-arrow-down");n(this).removeClass("selected")}),r.find("i").removeClass("icon-arrow-down"),r.find("i").addClass("icon-arrow-up"),r.addClass("selected"),this.sort(u+" asc"));this.show()},refresh:function(){this.show()},showAbstract:function(t,i){var f=ko.contextFor(i.target).$parent,r=n(i.target),u=r.next();u.is(":visible")?(u.hide(),r.text("Show abstract")):(u.show(),r.text("Hide abstract"))},bulkChangeMetaBid:function(n,i){var r=t.GetEventFilter(i);this.changeMetaBid(r)},showMetaBidSummary:function(n,i){var r=t.GetEventFilter(i);this.metaBidSummary(r)},bulkEnableDisableAuthorFeedback:function(n,r,u){var f=u?"enabling":"disabling",e,o;confirm("Bulk author feedback {0} will be performed for selected items you are assigned to.".format(f))&&(e=t.GetEventFilter(r),o={requestUri:t.odata.getUrl(t.odata.entitySet.metaBiddingReviewModels,null,"BulkEnableDisableAuthorFeedback"),method:"POST",showProgressIndicator:!0,data:{Filter:e,Enable:u}},i.request(o,function(){t.addMessage("Bulk author feedback {0} has been completed successfully.".format(f));location.reload()}))},openAllReviews:function(n,r,u,f){var s=this,e=t.GetEventFilter(r),o={requestUri:t.odata.getUrl(t.odata.entitySet.metaBiddingReviewModels,null,"GetIds"),method:"POST",showProgressIndicator:!0,data:{Filter:e,Shared:f}};i.request(o,function(n){var i=n.value.join("/"),r="/"+window.cmt3.conference.name+"/Submission/"+(u?"AllReviewsSideBySide":"AllReviews");t.url.navigateTo(r,{ids:i})})},bulkEnableDisableDiscussion:function(n,r,u){var f=u?"enabled":"disabled",e,o;confirm("The selected assignments will be {0} for discussion.".format(f))&&(e=t.GetEventFilter(r),o={requestUri:t.odata.getUrl(t.odata.entitySet.metaBiddingReviewModels,null,"BulkDiscussionEnableDisable"),method:"POST",showProgressIndicator:!0,data:{Filter:e,Enable:u}},i.request(o,function(){t.addMessage("Bulk discussion {0} has been completed successfully.".format(f));location.reload()}))},exportReviewerSubmissionComparisons:function(n,i){var r=t.GetEventFilter(i),u=t.odata.getUrl(t.odata.entitySet.metaBiddingReviewModels,null,"ExportReviewerSubmissionComparisons"),f={Filter:r,Shared:!1};t.page.post(u,f)},navigateEmailReviewersUrl:function(n,i){var r="/"+window.cmt3.conference.name+"/Submission/SendEmail/3";t.url.navigateTo(r,{filter:n.length>0?n:null,all:i})},bulkEmailAllReviewers:function(n,i){var r=t.GetEventFilter(i);this.navigateEmailReviewersUrl(r,!0)},bulkEmailReviewers:function(n,i){var r=t.GetEventFilter(i);this.navigateEmailReviewersUrl(r,!1)},bulkEnableAuthorFeedback:function(n,t){this.bulkEnableDisableAuthorFeedback(n,t,!0)},bulkDisableAuthorFeedback:function(n,t){this.bulkEnableDisableAuthorFeedback(n,t,!1)},bulkEnableDiscussion:function(n,t){this.bulkEnableDisableDiscussion(n,t,!0)},bulkDisableDiscussion:function(n,t){this.bulkEnableDisableDiscussion(n,t,!1)},openAllReviewsPrinterFriendly:function(n,t){this.openAllReviews(n,t,!1,!1)},openAllReviewsSideBySide:function(n,t){this.openAllReviews(n,t,!0,!1)},openAllReviewsPrinterFriendlyShared:function(n,t){this.openAllReviews(n,t,!1,!0)},openAllReviewsSideBySideShared:function(n,t){this.openAllReviews(n,t,!0,!0)}}}(window.jQuery,window.app,window.OData),function(n,t,i){"use strict";function r(n,t){var i=this;i.meta=t;i.conference=window.cmt3.conference.name;i.controller=i.meta?"MetaPapersDetails":"PapersDetails";i._sort=ko.observable("Id");i._total=ko.observable(0);i._selected=ko.observable(0);i._items=ko.observableArray(n);i.filters=[];i.bind();i.start()}function u(n,t){var i=this;i.meta=t;i.conference=window.cmt3.conference.name;i.controller=i.controller=i.meta?"MetaReviewersDetails":"ReviewersDetails";i._sort=ko.observable("Id");i._total=ko.observable(0);i._selected=ko.observable(0);i._items=ko.observableArray(n);i.filters=[];i.bind();i.start()}t.ConfirmationPage=function(n){var t=this;t.meta=n;t.conference=window.cmt3.conference.name;t.start()};t.ConfirmationPage.prototype={prefix:function(){var n=this;return n.meta?"Meta":""},start:function(){var t=this;t.show("papers");n('a[data-toggle="tab"]').on("shown.bs.tab",function(i){t.filters=[];var r=n(i.target),u=r.attr("href"),f=u.substring(1);t.show(f)})},assign:function(){var t=this;n.when(n.ajax({url:"/"+t.conference+"/Assignment/{0}Assign".format(t.prefix()),dataType:"json"}))},go:function(n){var t=this;window.location="/"+t.conference+"/Assignment/"+n},again:function(){var t=this;n.when(n.ajax({type:"POST",url:"/"+t.conference+"/Assignment/{0}StartOver".format(t.prefix())})).done(function(n){n.code&&(n.code=="error"&&window.cmt3.logger.warn("[start] server return: "+n.message),n.code=="redirect"&&t.go(n.action));window.cmt3.logger.error("[start] unexpected response")}).fail(function(n){window.cmt3.logger.error("[batch] server side error: <"+n.status+"> "+n.statusText)})},update:function(){},show:function(i){var f=this;n.when(n.ajax({url:"/"+f.conference+"/Assignment/{0}".format(f.prefix())+t.capitalize(i)+"Detail",dataType:"json"})).done(function(e){if(e)if(e.code)e.code=="error"&&window.cmt3.logger.info("["+i+"] server said: "+e.message),e.code=="redirect"&&f.go(e.action),window.cmt3.logger.info("["+i+"] unexpected response");else{var h=t.capitalize(i)+"Detail",c=n("#"+i),o=n(c.text()),s=null;s=h==="PapersDetail"?new r(e,f.meta):new u(e,f.meta);n(".grid:visible").empty().append(o);ko.applyBindings(s,o[0]);window.cmt3.logger.info("["+i+"] view succefully changed")}else window.cmt3.logger.info("["+i+"] empty response")}).fail(function(n){window.cmt3.logger.error("["+i+"] server side error: "+n.status)})}};r.prototype={bind:function(){var t=this;n(document).on("data.filter",n.proxy(t.render,t))},start:function(){var n=this;i.read({requestUri:"/api/odata/"+n.conference+"/"+n.controller+"?$count=true&$top=0",dataType:"json"},function(t){n._total(t["@odata.count"])},function(n){window.cmt3.logger.error("[start] server side error: "+n.message)})},sort:function(t,i){var u=this,r=n(i.target),f=r.attr("sortby");r.hasClass("selected")?u._sort().match("desc$")?(u._sort(f+" asc"),r.find("i").removeClass("icon-chevron-down"),r.find("i").addClass("icon-chevron-up")):(u._sort(f+" desc"),r.find("i").removeClass("icon-chevron-up"),r.find("i").addClass("icon-chevron-down")):(n("th[sortby]").each(function(){n(u).find("i").removeClass("icon-chevron-up");n(u).find("i").removeClass("icon-chevron-down");n(u).removeClass("selected")}),r.find("i").removeClass("icon-chevron-down"),r.find("i").addClass("icon-chevron-up"),r.addClass("selected"),u._sort(f+" asc"));u.render()},getFilter:function(){var i=this,t="";return n.each(i.filters,function(n,i){i.getValue()&&(t+=t==""?i.getValue():" and "+i.getValue())}),t},render:function(){var t=this,r="&$orderby="+t._sort(),u=t.getFilter()!=""?"&$filter="+encodeURIComponent(t.getFilter()):"",f="$count=true"+r+u,e={method:"POST",requestUri:"/api/odata/"+t.conference+"/$batch",headers:{Accept:"application/json"},data:{requests:[{method:"GET",url:"/api/odata/"+t.conference+"/"+t.controller+"?"+f+"&$select=Id,Title,AssignedCount,NewCount&$expand=New($select=Email,Name),Assigned($select=Email,Name)",headers:{Accept:"application/json"}}]}};i.request(e,function(i){var r=i&&i.responses&&i.responses[0]&&i.responses[0].body,e=r&&r["@odata.count"],u=r&&r.value,f=!0;r?(e?(t._selected(e),t.saved=!1):(window.cmt3.logger.warn("[batch] can't calculate response count"),f=!1),u&&n.inArray(u)?(t._items([]),t._items(u),t.saved=!1):(window.cmt3.logger.warn("[batch] resquest doesn't contain data"),f=!1),f&&window.cmt3.logger.info("[batch] data updated successfully")):window.cmt3.logger.error("[batch] unexpected response")},function(n){window.cmt3.logger.error("[batch] server side error: "+n.message)},i.batchHandler)}};u.prototype={bind:function(){var t=this;n(document).on("data.filter",n.proxy(t.render,t))},start:function(){var n=this;i.read({requestUri:"/api/odata/"+n.conference+"/"+n.controller+"?$count=true&$select=Id",dataType:"json"},function(t){n._total(t["@odata.count"])},function(n){window.cmt3.logger.error("[start] server side error: "+n.message)})},sort:function(t,i){var u=this,r=n(i.target),f=r.attr("sortby");r.hasClass("selected")?u._sort().match("desc$")?(u._sort(f+" asc"),r.find("i").removeClass("icon-chevron-down"),r.find("i").addClass("icon-chevron-up")):(u._sort(f+" desc"),r.find("i").removeClass("icon-chevron-up"),r.find("i").addClass("icon-chevron-down")):(n("th[sortby]").each(function(){n(u).find("i").removeClass("icon-chevron-up");n(u).find("i").removeClass("icon-chevron-down");n(u).removeClass("selected")}),r.find("i").removeClass("icon-chevron-down"),r.find("i").addClass("icon-chevron-up"),r.addClass("selected"),u._sort(f+" asc"));u.render()},getFilter:function(){var i=this,t="";return n.each(i.filters,function(n,i){i.getValue()&&(t+=t==""?i.getValue():" and "+i.getValue())}),t},render:function(){var t=this,r="&$orderby="+t._sort(),u=t.getFilter()!=""?"&$filter="+encodeURIComponent(t.getFilter()):"",f="$count=true"+r+u,e={method:"POST",requestUri:"/api/odata/"+t.conference+"/$batch",headers:{Accept:"application/json"},data:{requests:[{method:"GET",url:"/api/odata/"+t.conference+"/"+t.controller+"?"+f+"&$select=Id,Name,Email,AssignedCount,NewCount&$expand=New($select=Id,Title),Assigned($select=Id,Title)",headers:{Accept:"application/json"}}]}};i.request(e,function(i){var r=i&&i.responses&&i.responses[0]&&i.responses[0].body,e=r&&r["@odata.count"],u=r&&r.value,f=!0;r?(e?(t._selected(e),t.saved=!1):(window.cmt3.logger.warn("[batch] can't calculate response count"),f=!1),u&&n.inArray(u)?(t._items([]),t._items(u),t.saved=!1):(window.cmt3.logger.warn("[batch] resquest doesn't contain data"),f=!1),f&&window.cmt3.logger.info("[batch] data updated successfully")):window.cmt3.logger.error("[batch] unexpected response")},function(n){window.cmt3.logger.error("[batch] server side error: "+n.message)},i.batchHandler)}}}(window.jQuery,window.app,window.OData),function(n,t,i){"use strict";function r(n){var t=this;t.id=n.Id;t.title=n.Title;t.track=n.Track;t.status=n.Status;t.assigned=n.Assigned;t.completed=n.Percentage}t.PapersPage=function(t,i,r){var u=this;u.meta=r;u.$element=n(t);u.conference=window.cmt3.conference.name;u.controller=i;u.scope="autoa";u.state={};u.filters=[];u.saved=!1;u._sort=ko.observable("Id");u._total=ko.observable(0);u._selected=ko.observable(0);u._items=ko.observableArray([]);u._assign=ko.observable(0);u._assign.hasError=ko.observable(!1);u._increase=ko.observable(0);u._increase.hasError=ko.observable(!1);u._direction=ko.observable("inc");u.bind();u.start()};t.PapersPage.prototype={getKey:function(){var n=this;return n.meta?"METAAUTOA_PAPERS_STATE":"AUTOA_PAPERS_STATE"},prefix:function(){var n=this;return n.meta?"Meta":""},bind:function(){var t=this;n(document).on("data.filter",n.proxy(t.render,t))},start:function(){var t=this;i.read({requestUri:"/api/odata/"+t.conference+"/"+t.controller+"?$count=true&$top=0",dataType:"json"},function(n){t._total(n["@odata.count"])},function(n){window.cmt3.logger.error("[start] server side error: "+n.message)});n.when(n.ajax({type:"GET",url:"/"+t.conference+"/Assignment/GetState",data:{scope:t.scope,key:t.getKey()},dataType:"json",contentType:"application/json; charset=utf-8"})).done(function(n){n.code?n.code=="error"&&window.cmt3.logger.info("[start] can't restore state: "+n.message):t.setState(n)}).done(function(){t.render()}).fail(function(n){window.cmt3.logger.error("[start] server side error: <"+n.status+"> "+n.statusText)})},setState:function(t){var i=this,r,u,f,e,o;return t?(r=JSON.parse(t.sort),r&&n.type(r)=="string"&&r.length>0?i._sort(r):window.cmt3.logger.info("[state] can't restore sort value"),u=JSON.parse(t.total),u&&n.isNumeric(u)?i._total(u):window.cmt3.logger.info("[state] can't restore total value"),f=JSON.parse(t.selected),f&&n.isNumeric(f)?i._selected(f):window.cmt3.logger.info("[state] can't restore selected value"),e=t.filters,(e,n.isArray(e))?n.each(i.filters,function(n,t){t.state(e[n])}):window.cmt3.logger.info("[state] can't restore filters"),o=JSON.parse(t.state),o&&n.type(o)=="object"?n.each(o,function(n,t){i.state[n]=ko.observable(t);i.state[n].hasError=ko.observable(!1)}):window.cmt3.logger.info("[state] can't restore ids value"),!0):!1},render:function(){var t=this,u="&$orderby="+t._sort(),f=t.getFilter()!=""?"&$filter="+encodeURIComponent(t.getFilter()):"",e="$count=true"+u+f,o={method:"POST",requestUri:"/api/odata/"+t.conference+"/$batch",headers:{Accept:"application/json"},data:{requests:[{method:"GET",url:"/api/odata/"+t.conference+"/"+t.controller+"?"+e,headers:{Accept:"application/json"}}]}};i.request(o,function(i){var u=i&&i.responses&&i.responses[0]&&i.responses[0].body,s=u&&u["@odata.count"],f=u&&u.value,e=!0,o;u?(s?(t._selected(s),t.saved=!1):(window.cmt3.logger.warn("[batch] can't calculate response count"),e=!1),f&&n.inArray(f)?(t._items([]),o=[],n.each(f,function(n,i){var u=i.Id;t.state[u]||(t.state[u]=ko.observable(i.Assigned),t.state[u].hasError=ko.observable(!1));o.push(new r(i))}),t._items(o),t.saved=!1):(window.cmt3.logger.warn("[batch] resquest doesn't contain data"),e=!1),e&&(t.save(),window.cmt3.logger.info("[batch] data updated successfully"))):window.cmt3.logger.error("[batch] unexpected response")},function(n){window.cmt3.logger.error("[batch] server side error: "+n.message)},i.batchHandler)},getState:function(){var t=this,i={sort:ko.toJSON(t._sort),total:ko.toJSON(t._total),selected:ko.toJSON(t._selected),state:ko.toJSON(t.state),filters:[]};return n.each(t.filters,function(n,t){i.filters.push(t.state())}),i},getFilter:function(){var i=this,t="";return n.each(i.filters,function(n,i){i.getValue()&&(t+=t==""?i.getValue():" and "+i.getValue())}),t},scroll:function(){var t=this;n(window).scrollTop()==n(document).height()-n(window).height()&&t.render()},resetFilters:function(){var t=this;n.each(t.filters,function(n,t){t.reset()});t.render()},sort:function(t,i){var u=this,r=n(i.target),f=r.attr("sortby");(f==null||f==undefined)&&(r=n(r.context.parentNode),f=r.attr("sortby"));r.hasClass("selected")?u._sort().match("desc$")?(u._sort(f+" asc"),r.find("i").removeClass("icon-chevron-down"),r.find("i").addClass("icon-chevron-up")):(u._sort(f+" desc"),r.find("i").removeClass("icon-chevron-up"),r.find("i").addClass("icon-chevron-down")):(n("th[sortby]").each(function(){n(u).find("i").removeClass("icon-chevron-up");n(u).find("i").removeClass("icon-chevron-down");n(u).removeClass("selected")}),r.find("i").removeClass("icon-chevron-down"),r.find("i").addClass("icon-chevron-up"),r.addClass("selected"),u._sort(f+" asc"));u.render()},next:function(){var i=this;n.when(i.submit(),i.saveState()).done(function(n){var r=n[0];if(r)switch(r.code){case"error":t.addMessage(r.message,"Appliction Error:","error");window.cmt3.logger.log("[next] server return: "+r.message);break;case"redirect":r.action?i.go(r.action):(t.addMessage("Server returns empty action to redirect. Please, contact your suystem administrator.","Appliction Error:","error"),window.cmt3.logger.log("[next] server return: no action to redirect"))}}).fail(function(n){t.addMessage(n.statusText,"System error:","error");window.cmt3.logger.error("[batch] server side error: <"+n.status+"> "+n.statusText)})},previous:function(){var n=this;n.go("Papers")},go:function(n){var t=this;window.location="/"+t.conference+"/Assignment/"+n},begin:function(){var t=this;n.when(n.ajax({type:"POST",url:"/"+t.conference+"/Assignment/{0}StartOver".format(t.prefix())})).done(function(n){n.code&&(n.code=="error"&&window.cmt3.logger.warn("[start] server return: "+n.message),n.code=="redirect"&&t.go(n.action));window.cmt3.logger.error("[start] unexpected response")}).fail(function(n){window.cmt3.logger.error("[batch] server side error: <"+n.status+"> "+n.statusText)})},submit:function(){var t=this;return n.ajax({type:"POST",url:"/"+t.conference+"/Assignment/{0}SavePapers".format(t.prefix()),data:JSON.stringify({papers:t.getResult()}),contentType:"application/json; charset=utf-8"})},assign:function(){var t=this,i=parseInt(t._assign());if(i<0||isNaN(i)){t._assign.hasError(!0);return}n.each(t._items(),function(n,r){var u=t.state[r.id];r.assigned>i?(u.hasError(!0),u(r.assigned)):(u(i),u.hasError(!1))});t.save();t._assign.hasError(!1)},increase:function(){var t=this,i=parseInt(t._increase());if(i<0||isNaN(i)){t._increase.hasError(!0);return}t._direction()=="dec"&&(i=0-i);n.each(t._items(),function(n,r){var u=t.state[r.id],f=parseInt(u()),e;if(f<0||isNaN(f)){u.hasError(!0);return}e=f+i;r.assigned>e?(u.hasError(!0),u(r.assigned)):(u(e),u.hasError(!1))});t.save();t._increase.hasError(!1)},blur:function(n,t){var r=ko.contextFor(t.target).$root,i=r.state[n.id],u=parseInt(i());n.assigned>u||isNaN(u)?i.hasError(!0):(r.save(),i.hasError(!1))},getResult:function(){var t=this,i=[];return n.each(t._items(),function(n,r){r.assigned<t.state[r.id]()&&i.push({Id:r.id,Assigned:r.assigned,Reviewers:t.state[r.id]()})}),i},saveState:function(){var t=this;return n.ajax({type:"POST",url:"/"+t.conference+"/Assignment/SetState",dataType:"json",data:{scope:t.scope,key:t.getKey(),value:JSON.stringify(t.getState())}})},save:function(){var t=this;n.when(t.saveState()).done(function(n){n.code?(n.code=="error"&&window.cmt3.logger.error("[batch] server return: "+n.message),n.code=="ok"&&window.cmt3.logger.info("[batch] state saved succefully!")):window.cmt3.logger.error("[batch] unexpected response: "+n)}).fail(function(n){window.cmt3.logger.error("[batch] server side error: <"+n.status+"> "+n.statusText)})}}}(window.jQuery,window.app,window.OData),function(n,t){"use strict";t.ProgressPage=function(n){var t=this;t.meta=n;t.timer=null;t.conference=window.cmt3.conference.name;t.progress=ko.observable(0);t.eta=ko.observable(null);t.error=ko.observable(!1);t.completed=ko.observable(!1);t.message=ko.observable("");t.listen();t.etaText=ko.pureComputed(function(){var n=t.eta();return n!=null?"ETA: "+n:null},t)};t.ProgressPage.prototype={prefix:function(){var n=this;return n.meta?"Meta":""},listen:function(){var t=this;t.timer=setInterval(n.proxy(t.update,t),1e3)},candidates:function(){var n=this;n.go("{0}Confirmation".format(n.prefix()))},previous:function(){var n=this;n.go("{0}Settings".format(n.prefix()))},go:function(n){var t=this;window.location="/"+t.conference+"/Assignment/"+n},begin:function(){var t=this;n.when(n.ajax({type:"POST",url:"/"+t.conference+"/Assignment/{0}StartOver".format(t.prefix())})).done(function(n){n.code&&(n.code=="error"&&window.cmt3.logger.warn("[start] server return: "+n.message),n.code=="redirect"&&t.go(n.action));window.cmt3.logger.error("[start] unexpected response")}).fail(function(n){window.cmt3.logger.error("[batch] server side error: <"+n.status+"> "+n.statusText)})},update:function(){var i=this;n.get("/"+i.conference+"/Assignment/{0}GetProgress".format(i.prefix())).done(function(n){n.code?n.code=="error":n.Progress&&(i.progress(n.Progress),i.eta(n.ETA),n.Progress>=100&&n.Progress==100&&(n.HasError&&(i.error(!0),n.Message&&t.addMessage(n.Message,"Calculation error:","error")),clearInterval(i.timer)))})}}}(window.jQuery,window.app),function(n,t,i){"use strict";function r(n){var t=this;t.id=n.Id;t.name=n.Name;t.surname=n.Surname;t.email=n.Email;t.tracks=n.Tracks;t.trackList=n.TrackList;t.assigned=n.Assigned;t.completed=n.Completed;t.percentage=n.Percentage;t.quota=n.Quota;t.quotaString=t.quota==null?"-":t.quota;t.userType=n.UserType;t.hasError=ko.observable(!1)}t.ReviewersPage=function(t,i,r,u){var f=this;f.meta=r;f.$element=n(t);f.conference=window.cmt3.conference.name;f.controller=i;f.scope="autoa";f.desc=!0;f.state={};f.filters=[];f.saved=!1;f._sort=ko.observable("Id");f._total=ko.observable(0);f._selected=ko.observable(0);f._items=ko.observableArray([]);f._assign=ko.observable(0);f._assign.hasError=ko.observable(!1);f._increase=ko.observable(0);f._increase.hasError=ko.observable(!1);f._direction=ko.observable("inc");f.bind();f.start();f.userTypes=u;f.userTypesProvider=function(){return f.userTypes}};t.ReviewersPage.prototype={getKey:function(){var n=this;return n.meta?"METAAUTOA_REVIEWERS_STATE":"AUTOA_REVIEWERS_STATE"},prefix:function(){var n=this;return n.meta?"Meta":""},bind:function(){var t=this;n(document).on("data.filter",n.proxy(t.render,t))},start:function(){var t=this;i.read({requestUri:"/api/odata/"+t.conference+"/"+t.controller+"?$count=true&$top=0",dataType:"json"},function(n){t._total(n["@odata.count"])},function(n){window.cmt3.logger.error("[start] server side error: "+n.message)});n.when(n.ajax({type:"GET",url:"/"+t.conference+"/Assignment/GetState",data:{scope:t.scope,key:t.getKey()},dataType:"json",contentType:"application/json; charset=utf-8"})).done(function(n){n.code?n.code=="error"&&window.cmt3.logger.info("[start] can't restore state: "+n.message):t.setState(n)}).done(function(){t.render()}).fail(function(n){window.cmt3.logger.error("[start] server side error: <"+n.status+"> "+n.statusText)})},setState:function(t){var i=this,r,u,f,e,o;return t?(r=JSON.parse(t.sort),r&&n.type(r)=="string"&&r.length>0?i._sort(r):window.cmt3.logger.info("[state] can't restore sort value"),u=JSON.parse(t.total),u&&n.isNumeric(u)?i._total(u):window.cmt3.logger.info("[state] can't restore total value"),f=JSON.parse(t.selected),f&&n.isNumeric(f)?i._selected(f):window.cmt3.logger.info("[state] can't restore selected value"),e=t.filters,(e,n.isArray(e))?n.each(i.filters,function(n,t){t.state(e[n])}):window.cmt3.logger.info("[state] can't restore filters"),o=JSON.parse(t.state),o&&n.type(o)=="object"?n.each(o,function(n,t){i.state[n]=ko.observable(t);i.state[n].hasError=ko.observable(!1)}):window.cmt3.logger.info("[state] can't restore ids value"),!0):!1},render:function(){var t=this,u="&$orderby="+t._sort(),f=t.getFilter()!=""?"&$filter="+encodeURIComponent(t.getFilter()):"",e="$count=true"+u+f,o={method:"POST",requestUri:"/api/odata/"+t.conference+"/$batch",headers:{Accept:"application/json"},data:{requests:[{method:"GET",url:"/api/odata/"+t.conference+"/"+t.controller+"?"+e,headers:{Accept:"application/json"}}]}};i.request(o,function(i){var u=i&&i.responses&&i.responses[0]&&i.responses[0].body,s=u&&u["@odata.count"],f=u&&u.value,e=!0,o;u?(s?(t._selected(s),t.saved=!1):(window.cmt3.logger.warn("[batch] can't calculate response count"),e=!1),f&&n.inArray(f)?(t._items([]),o=[],n.each(f,function(n,i){var u=i.Id;t.state[u]||(t.state[u]=ko.observable(i.Assigned),t.state[u].hasError=ko.observable(!1));o.push(new r(i))}),t._items(o),t.saved=!1):(window.cmt3.logger.warn("[batch] resquest doesn't contain data"),e=!1),e&&(t.save(),window.cmt3.logger.info("[batch] data updated successfully"))):window.cmt3.logger.error("[batch] unexpected response")},function(n){window.cmt3.logger.error("[batch] server side error: "+n.message)},i.batchHandler)},getState:function(){var t=this,i={sort:ko.toJSON(t._sort),total:ko.toJSON(t._total),selected:ko.toJSON(t._selected),state:ko.toJSON(t.state),filters:[]};return n.each(t.filters,function(n,t){i.filters.push(t.state())}),i},getFilter:function(){var i=this,t="";return n.each(i.filters,function(n,i){i.getValue()&&(t+=t==""?i.getValue():" and "+i.getValue())}),t},scroll:function(){var t=this;n(window).scrollTop()==n(document).height()-n(window).height()&&t.render()},resetFilters:function(){var t=this;n.each(t.filters,function(n,t){t.reset()});t.render()},sort:function(t,i){var u=this,r=n(i.target),f=r.attr("sortby");(f==null||f==undefined)&&(r=n(r.context.parentNode),f=r.attr("sortby"));r.hasClass("selected")?u._sort().match("desc$")?(u._sort(f+" asc"),r.find("i").removeClass("icon-chevron-down"),r.find("i").addClass("icon-chevron-up")):(u._sort(f+" desc"),r.find("i").removeClass("icon-chevron-up"),r.find("i").addClass("icon-chevron-down")):(n("th[sortby]").each(function(){n(u).find("i").removeClass("icon-chevron-up");n(u).find("i").removeClass("icon-chevron-down");n(u).removeClass("selected")}),r.find("i").removeClass("icon-chevron-down"),r.find("i").addClass("icon-chevron-up"),r.addClass("selected"),u._sort(f+" asc"));u.render()},next:function(){var t=this;n.when(t.submit(),t.saveState()).done(function(n){n[0]&&(n[0].code=="error"&&window.cmt3.logger.log("[next] server return: "+n[0].message),n[0].code=="redirect"&&t.go(n[0].action))}).fail(function(n){window.cmt3.logger.error("[batch] server side error: <"+n.status+"> "+n.statusText)})},previous:function(){var n=this;n.go("{0}Papers".format(n.prefix()))},go:function(n){var t=this;window.location="/"+t.conference+"/Assignment/"+n},begin:function(){var t=this;n.when(n.ajax({type:"POST",url:"/"+t.conference+"/Assignment/{0}StartOver".format(t.prefix())})).done(function(n){n.code&&(n.code=="error"&&window.cmt3.logger.warn("[start] server return: "+n.message),n.code=="redirect"&&t.go(n.action));window.cmt3.logger.error("[start] unexpected response")}).fail(function(n){window.cmt3.logger.error("[batch] server side error: <"+n.status+"> "+n.statusText)})},submit:function(){var t=this;return n.ajax({type:"POST",url:"/"+t.conference+"/Assignment/{0}SaveReviewers".format(t.prefix()),data:JSON.stringify({reviewers:t.getResult()}),contentType:"application/json; charset=utf-8"})},assign:function(){var t=this,i=parseInt(t._assign());if(i<0||isNaN(i)){t._assign.hasError(!0);return}n.each(t._items(),function(n,r){var u=t.state[r.id];r.assigned>i?(u.hasError(!0),u(r.assigned)):r.quota!=null&&r.assigned<=r.quota&&i>r.quota?(u.hasError(!0),u(r.quota)):(u(i),u.hasError(!1))});t.save();t._assign.hasError(!1)},increase:function(){var t=this,i=parseInt(t._increase());if(i<0||isNaN(i)){t._increase.hasError(!0);return}t._direction()=="dec"&&(i=0-i);n.each(t._items(),function(n,r){var u=t.state[r.id],e=parseInt(u()),f;if(e<0||isNaN(e)){u.hasError(!0);return}f=e+i;r.assigned>f?(u.hasError(!0),u(r.assigned)):r.quota!=null&&r.assigned<=r.quota&&f>r.quota?(u.hasError(!0),u(r.quota)):(u(f),u.hasError(!1))});t.save();t._increase.hasError(!1)},blur:function(n,t){var u=ko.contextFor(t.target).$root,i=u.state[n.id],r=parseInt(i());n.assigned>r||isNaN(r)?i.hasError(!0):n.quota!=null&&n.assigned<=n.quota&&r>n.quota?(i.hasError(!0),i(n.quota)):(u.save(),i.hasError(!1))},getResult:function(){var t=this,i=[];return n.each(t._items(),function(n,r){i.push({Id:r.id,Assigned:r.assigned,Papers:t.state[r.id]()})}),i},saveState:function(){var t=this;return n.ajax({type:"POST",url:"/"+t.conference+"/Assignment/SetState",dataType:"json",data:{scope:t.scope,key:t.getKey(),value:JSON.stringify(t.getState())}})},save:function(){var t=this;n.when(t.saveState()).done(function(n){n.code?(n.code=="error"&&window.cmt3.logger.error("[batch] server return: "+n.message),n.code=="ok"&&window.cmt3.logger.info("[batch] state saved succefully!")):window.cmt3.logger.error("[batch] unexpected response: "+n)}).fail(function(n){window.cmt3.logger.error("[batch] server side error: <"+n.status+"> "+n.statusText)})}}}(window.jQuery,window.app,window.OData),function(n,t){"use strict";t.SettingsPage=function(n){var t=this;t.meta=n;t.conference=window.cmt3.conference.name;t.customWeights=ko.observable("default");t.customWeights.subscribe(t.checkWeights,t);t.bids=ko.observable("");t.bids.hasError=ko.observable(!1);t.suggestions=ko.observable("");t.suggestions.hasError=ko.observable(!1);t.relevance=ko.observable("");t.relevance.hasError=ko.observable(!1);t.tpms=ko.observable("");t.tpms.hasError=ko.observable(!1);t.loadBalanced=ko.observable(!0);t.loadBalanced.subscribe(t.resetBalanceFactor,t);t.balanceFactor=ko.observable(1);t.balanceFactor.hasError=ko.observable(!1);t.showWeightDetails=ko.observable(!0);t.showAssignmentsDetails=ko.observable(!0);t.valid=ko.observable(!0)};t.SettingsPage.prototype={prefix:function(){var n=this;return n.meta?"Meta":""},run:function(){var i=this,s;if(i.validate()){var r=-1,u=-1,f=-1,e=-1,o=-1;i.customWeights()=="custom"&&(r=i.bids()?parseFloat(i.bids()):-1,u=i.suggestions()?parseFloat(i.suggestions()):-1,f=i.relevance()?parseFloat(i.relevance()):-1,e=i.tpms()?parseFloat(i.tpms()):-1,o=i.balanceFactor()?parseFloat(i.balanceFactor()):1);s={bids:r,suggestions:u,relevance:f,tpms:e,loadBalanced:i.loadBalanced(),balanceFactor:o};n.ajax({type:"POST",url:"/"+i.conference+"/Assignment/{0}Run".format(i.prefix()),data:JSON.stringify(s),contentType:"application/json; charset=UTF-8"}).done(function(n){n.code=="error"&&(window.cmt3.logger.log(n.message),t.addMessage(n.message,"Application error:","error"));n.code=="redirect"&&(window.location="/"+i.conference+"/Assignment/"+n.action)}).fail(function(n){window.cmt3.logger.error("[run] server side error: <"+n.status+"> "+n.statusText);t.addMessage(n.message,"Application error:","error")})}},reviewers:function(){var n=this;window.location="/"+n.conference+"/Assignment/{0}Reviewers".format(n.prefix())},again:function(){var i=this;n.ajax({type:"POST",url:"/"+i.conference+"/Assignment/{0}StartOver".format(i.prefix())}).done(function(n){n.code=="error"&&(t.addMessage(n.message,"Application error:","error"),window.cmt3.logger.log(n.message));n.code=="redirect"&&(window.location="/"+i.conference+"/Assignment/"+n.action)})},resetBalanceFactor:function(){var n=this;n.balanceFactor(1);n.balanceFactor.hasError(!1)},resetWeights:function(){var n=this;n.bids("");n.suggestions("");n.relevance("");n.tpms("");n.bids.hasError(!1);n.suggestions.hasError(!1);n.relevance.hasError(!1);n.tpms.hasError(!1)},checkWeights:function(n){var t=this;n=="default"&&t.resetWeights();t.validate()},validate:function(){var t=this,i;return t.valid(!0),i=!0,t.customWeights()=="custom"&&(i=t.validateWeights()),i&&t.loadBalanced()&&(i=t.validateWeight(n("input.balanceFactor"))),i||t.valid(!1),i},validateWeights:function(){var i=this,t=!0;return n("input.weight").each(function(){var n=i.validateWeight.apply(i,[this]);t=t&&n}),t&&(t=i.validateWeightsSum()),t},validateWeight:function(t){var i=this,r=n(t).attr("id"),u=i[r](),f;return typeof u=="string"&&(u=u.trim()),u?(f=parseFloat(u),isNaN(f)?i.bad(r):f==0?i.good(r):f>0&&f<=1?i.good(r):i.bad(r)):i.good(r)},validateWeightsSum:function(){var t=0,i=this,r=!0;return(n.each(["bids","suggestions","relevance","tpms"],function(n,u){var f=i[u]().trim();f&&(r=!1,t+=parseFloat(f))}),r)?!1:t<=0||t>1?i.badSum():!0},badSum:function(){var i=this;return t.addMessage("The sum of 'Bids', 'Suggestions' and 'Relevance' must be greater than 0 and not greater than 1","Incorrect input:","error"),n.each(["bids","suggestions","relevance","tpms"],function(n,t){var r=i[t];r.hasError(!0)}),!1},bad:function(n){var i=this;return t.addMessage("Weight for the '"+t.capitalize(n)+"'  must be a numeric value between 0 and 1","Incorrect input:","error"),i[n].hasError(!0),!1},good:function(n){var t=this;return t[n].hasError(!1),!0}}}(window.jQuery,window.app),function(n){function t(n){var t=this;if(!n){t.currentRank=ko.observable(null);t.order=ko.observable(null);return}t.id=n.Id;t.order=ko.observable(n.Order);t.currentRank=ko.observable(t.order()==null?null:n.CurrentRank);t.userFirstName=n.UserFirstName;t.userLastName=n.UserLastName;t.userEmail=n.UserEmail;t.tpmsRank=n.TpmsRank;t.suggestionModel=null}function u(t){var i=this;i.id=t.Id;i.order=ko.observable(t.Order);i.currentRank=ko.observable(i.order()==null?null:t.CurrentRank);i.userFirstName=t.UserFirstName;i.userLastName=t.UserLastName;i.userEmail=t.UserEmail;i.userId=t.UserId;i.primarySubject=t.PrimarySubject;i.secondarySubject=t.SecondarySubject;i.relevance=t.Relevance;i.tpmsRank=t.TpmsRank;i.bid=t.Bid;i.numberOfPapersSuggested=ko.observable(t.NumberOfPapersSuggested);i.numberOfAssignment=t.NumberOfAssignment;i.addAsCandidateClicked=!1;i.userType=t.UserType;i.googleScholarId=t.GoogleScholarId;i.googleScholarUrl=function(){return n.enums.externalProfile.googleScholar.format(i.googleScholarId)};i.semanticScholarId=t.SemanticScholarId;i.semanticScholarUrl=function(){return n.enums.externalProfile.semanticScholar.format(i.semanticScholarId)};i.dblpId=t.DblpId;i.dblpUrl=function(){return n.enums.externalProfile.dblp.format(i.dblpId)}}function i(){var n=this;n.isTpmsEnabled=ko.observable(!1).autoMap()}function f(t){var r=this;r.id=t;r.trackId=ko.observable().autoMap();r.trackName=ko.observable().autoMap();r.title=ko.observable().autoMap();r.isSingleTrackConference=ko.observable().autoMap();r.primarySubjectAreas=ko.observableArray([]);r.secondarySubjectAreas=ko.observableArray([]);r.trackData=ko.observable(new i);r.loadData=function(){var u=n.odata.getUrl(n.odata.entitySet.submissionViews,t,"GetSimpleView");return OData.request({requestUri:u,showProgressIndicator:!1,method:"POST",headers:{"Content-Type":"application/json"}},function(t){n.autoMap(r,t);r.primarySubjectAreas(JSON.parse(t.PrimarySubjectAreas));r.secondarySubjectAreas(JSON.parse(t.SecondarySubjectAreas));r.trackData(n.autoMap(new i,t.TrackData?JSON.parse(t.TrackData):{}))})}}function r(n,t,i,r){var u=this;u.submissionId=t;u.submission=new f(t);u.metaReviewerId=i;u.userTypes=r;u.userTypesProvider=function(){return u.userTypes};u.$element=$(n);u.conference=window.cmt3.conference.name;u.page=ko.observable(1);u.top=ko.observable(25);u.sort=ko.observable("CurrentRank, UserFirstName, UserLastName, UserEmail");u.controller="SuggestionModels";u.filters=[];u._total=ko.observable(0);u.selected=ko.observable(0);u.suggestions=ko.observableArray();u.candidates=ko.observableArray();u.candidatesLoaded=!1;u.submissionDetailsLoaded=!1;u.listen();u.Pager=ko.pager(u.selected,u.top);u.Pager().CurrentPage.subscribe(function(){u.page(u.Pager().CurrentPage());u.show()})}r.prototype={addCandidate:function(i){var u=this,r=u.suggestions()[i],f;r.addAsCandidateClicked||(r.addAsCandidateClicked=!0,f={requestUri:n.odata.getUrl(n.odata.entitySet.suggestionModels,null,"AddCandidate"),method:"POST",showProgressIndicator:!1,data:{Request:{SubmissionId:u.submissionId,MetaReviewerId:u.metaReviewerId,UserId:r.userId}}},OData.request(f,function(n){var i=new t;r.id=n.SuggestionId;r.currentRank(u.candidates().length+1);r.order(n.Order);r.numberOfPapersSuggested(r.numberOfPapersSuggested()+1);i.id=r.id;i.order(r.order());i.currentRank(r.currentRank());i.suggestionModel=r;i.userFirstName=r.userFirstName;i.userLastName=r.userLastName;i.userEmail=r.userEmail;i.tpmsRank=r.tpmsRank;u.candidates().push(i);u.candidates.valueHasMutated()},function(n){r.addAsCandidateClicked=!1;OData.defaultError(n)}))},removeCandidate:function(t){var r=this,i=r.candidates()[t],u={requestUri:n.odata.getUrl(n.odata.entitySet.suggestionModels,i.id),method:"DELETE"};OData.request(u,function(){var n=i.suggestionModel,u,f;for(n!=null&&(n.id=0,n.currentRank(null),n.order(null),n.numberOfPapersSuggested(n.numberOfPapersSuggested()-1)),u=r.candidates(),u.splice(t,1),f=t;f<u.length;f++)i=u[f],n=i.suggestionModel,n!=null&&n.currentRank(n.currentRank()-1),i.currentRank(i.currentRank()-1);r.candidates.valueHasMutated();n&&(n.addAsCandidateClicked=!1)},function(n){OData.defaultError(n)})},updateSuggestion:function(n){var t=n.suggestionModel;t!=null&&(t.currentRank(n.currentRank()),t.order(n.order()))},swapCandidates:function(t,i,r,u){var f=this,e={Id1:t.id,Id2:i.id},o={requestUri:n.odata.getUrl(n.odata.entitySet.suggestionModels,null,"SwapOrder"),method:"POST",data:{Request:e}};OData.request(o,function(){var n=t.order(),e;t.order(i.order());i.order(n);n=t.currentRank();t.currentRank(i.currentRank());i.currentRank(n);f.updateSuggestion(t);f.updateSuggestion(i);e=f.candidates();e[r]=i;e[u]=t;f.candidates.valueHasMutated()},function(n){OData.defaultError(n)})},moveCandidateUp:function(n){if(!(n<=0)){var t=this,i=n,r=n-1,u=t.candidates()[i],f=t.candidates()[r];t.swapCandidates(u,f,i,r)}},moveCandidateDown:function(n){var t=this;if(!(n>=t.candidates().length-1)){var i=n,r=n+1,u=t.candidates()[i],f=t.candidates()[r];t.swapCandidates(f,u,r,i)}},listen:function(){var n=this;$(document).on("data.filter",function(){n.Pager().CurrentPage()<2?n.show():n.Pager().CurrentPage(1)})},getFilter:function(){var n="";return $.each(this.filters,function(t,i){i.getValue()&&(n+=n==""?i.getValue():" and "+i.getValue())}),n},odataRequest:function(n){var t=this;return $.Deferred(function(i){var r={headers:{Accept:"application/json"},showProgressIndicator:!1,requestUri:"/api/odata/"+t.conference+"/$batch",method:"POST",data:{requests:[{url:n,method:"GET",headers:{Accept:"application/json"}}]}};OData.request(r,function(n){var t=n.responses[0].body,r=t["@odata.count"],u=t.value;i.resolve({items:u,count:r})},function(n){window.cmt3.logger.log(n.message);i.reject(n)},OData.batchHandler)}).promise()},show:function(){var i=this,r;if(i.initialized){var f=function(){var n="&$orderby="+i.sort(),t=i.top()!=0?"&$top="+i.top():"",r=i.skip()!=0?"&$skip="+i.skip():"",u=i.getFilter()!=""?"&$filter="+encodeURIComponent(i.getFilter()):"";return i.odataRequest("/api/odata/"+i.conference+"/"+i.controller+"?key="+i.submissionId+"&metaReviewerId="+i.metaReviewerId+"&$count=true"+n+u+r+t+"&caller=suggestions")},e=function(){var r,n;return i.candidatesLoaded?(r=i.candidates(),$.Deferred(function(n){var t=[];$.each(r,function(n,i){t[i.id]=i;i.suggestionModel=null});n.resolve(t)}).promise()):(n=$.Deferred(),i.odataRequest("/api/odata/"+i.conference+"/"+i.controller+"?key="+i.submissionId+"&metaReviewerId="+i.metaReviewerId+"&$count=true&$filter="+encodeURIComponent("(Order ne null)")+"&caller=suggestions").done(function(r){var u=[];$.each(r.items,function(n,i){var r=new t(i);u[r.id]=r});i.candidatesLoaded=!0;n.resolve(u)}).fail(n.reject),n.promise())},o=function(n,t,r){var e,f;i.submissionDetailsLoaded=!0;e=[];$.each(t.items,function(n,t){var i=new u(t);e.push(i);i.currentRank()!=null&&r[i.id]!=null&&(r[i.id].suggestionModel=i)});f=[];$.each(r,function(n,t){t&&f.push(t)});f.sort(function(n,t){return n.currentRank()-t.currentRank()});i.candidates(f);i.suggestions(e);i._total()==0&&i._total(t.count);i.selected(t.count);i.$element.show()};n.showProgress();r=i.submissionDetailsLoaded?$.Deferred().resolve().promise():i.submission.loadData();$.when(r,f(),e()).done(o).always(n.hideProgress)}},scroll:function(){$(window).scrollTop()==$(document).height()-$(window).height()&&self.show()},post:function(n,t,i){var r,f,u;i=i||"post";r=document.createElement("form");r.setAttribute("method",i);r.setAttribute("action",n);for(f in t)t.hasOwnProperty(f)&&(u=document.createElement("input"),u.setAttribute("type","hidden"),u.setAttribute("name",f),u.setAttribute("value",t[f]),r.appendChild(u));document.body.appendChild(r);r.submit();document.body.removeChild(r)},reset:function(){$.each(this.filters,function(n,t){t.reset()});this.show()},size:function(n,t){var i,r,u;$("a",".show").removeClass("btn-success").css("color","#999999");$(t.currentTarget).addClass("btn-success").css("color","white");i=$(t.target).attr("size");r=parseInt(i);this.top(r);u=this.Pager().CurrentPage();this.Pager().CurrentPage(1);u===1&&this.show()},skip:function(){return(this.page()-1)*this.top()},prev:function(){this.top()!=0&&this.page()!=1&&(this.page(this.page()-1),this.show())},next:function(){this.top()==0||this.page()>this.selected()/this.top()||(this.page(this.page()+1),this.show())},setSort:function(n,t){var i=$(t.target),r=i.attr("data-sort");(r==null||r==undefined)&&(i=$(i.context.parentNode),r=i.attr("data-sort"));i.hasClass("selected")?this.sort().match(" desc$")?(this.sort(r+" asc"),i.find("i").removeClass("icon-arrow-down"),i.find("i").addClass("icon-arrow-up")):(this.sort(r+" desc"),i.find("i").removeClass("icon-arrow-up"),i.find("i").addClass("icon-arrow-down")):($("th[data-sort]").each(function(){$(this).find("i").removeClass("icon-arrow-up");$(this).find("i").removeClass("icon-arrow-down");$(this).removeClass("selected")}),i.find("i").removeClass("icon-arrow-down"),i.find("i").addClass("icon-arrow-up"),i.addClass("selected"),this.sort(r+" asc"));this.show()},refresh:function(){this.show()}};n.suggestionsPage=function(n,t,i,u){return new r(n,t,i,u)}}(window.app),function(n,t,i,r,u,f,e,o){"use strict";function h(){var t=this;t.id=n.autoMap();t.originalName=n.autoMap();t.size=n.autoMap();t.formattedSize=n.autoMap();t.uploadDate=n.autoMap();t.downloadLink=n.autoMap()}function c(n,t,i,r,u){var f=this;f.id=n;f.title=t;f.trackId=i;f.trackName=r;f.isSingleTrackConference=u}function l(l,a,v,y,p,w,b,k){function g(){function a(){var u=r.stringify(e.getAnswersJson(d.questions)),i,f;if(d.lastDraft===u){d.setAutoSaveTimer();return}i=n.autoMap(d);i.SubmissionId=d.submission.id;i.Id=d.draftId||0;i.Draft=u;f={requestUri:n.odata.getUrl(n.odata.entitySet.metaReviewDrafts),method:"POST",headers:{Prefer:"return-content"},showProgressIndicator:!1,data:i};t.request(f,function(n){d.draftId=n.Id;d.lastDraftErrorDate(null);d.lastDraftDate((new Date).toLocaleString());d.lastDraft=u},function(){d.lastDraftErrorDate((new Date).toLocaleString())}).always(d.setAutoSaveTimer)}function v(){var n=!0;return d.files().length>d.settings.metaReviewMaxFileNumber&&(d.showFilesMaxErrorMessage(!0),n=!1),d.files().length<d.settings.metaReviewMinFileNumber&&(d.showFilesMinErrorMessage(!0),n=!1),n}function c(t){var e,r,f,u;if(d.files().length+t.length>d.settings.metaReviewMaxFileNumber){n.addMessage("You can upload up to {0} files only.".format(d.settings.metaReviewMaxFileNumber),null,"error");return}for(e=[],r=0;r<d.files().length;r++)e[d.files()[r].originalName.toLowerCase()]=!0;for(r=0;r<t.length;r++)f=t[r],y(f,e)&&(d.uploading(d.uploading()+1),u=i.ajaxSettings.xhr(),u.open("POST",s.fileUpload,!0),u.setRequestHeader("Accept","application/json"),u.setRequestHeader("File-Name",encodeURIComponent(f.name)),u.send(f),u.addEventListener("load",function(t){t.target.status==200?l(t.target.responseText):n.processXmlHttpRequestError(t.target);d.uploading(d.uploading()-1)},!1))}function y(t,i){var u=t.name.toLowerCase(),r;if(i[u]===undefined)i[u]=!0;else return n.addMessage("Found at least two files with the same name: '{0}'.".format(t.name),null,"error"),!1;if(t.size>d.settings.metaReviewMaxFileSize*1048576)return n.addMessage("File '{0}' is bigger than maximum allowed size of {1} Mb.".format(t.name,d.settings.metaReviewMaxFileSize),null,"error"),!1;var f=t.name.substr(t.name.lastIndexOf(".")+1).toLowerCase(),e=d.settings.metaReviewAllowedFileTypes.split(","),o=!1;for(r=0;r<e.length;r++)if(e[r].trim().toLowerCase()==f){o=!0;break}return o?!0:(n.addMessage("File '{0}' has type '{1}' which is not accepted. We accept '{2}' only.".format(t.name,f,d.settings.metaReviewAllowedFileTypes),null,"error"),!1)}function l(t){var r,i;try{r=ko.utils.parseJson(t)}catch(u){n.processException(u);return}i=n.autoMap(new h,r);i.uploadDate=new Date(i.uploadDate);isNaN(i.uploadDate)&&(i.uploadDate=new Date);d.files.push(i)}d.showFilesMinErrorMessage=ko.observable(!1);d.showFilesMaxErrorMessage=ko.observable(!1);d.questions=[];d.submittedAnswersJson=null;d.autoSaveTimerId=null;d.draftId=null;d.loadedDraftDate=ko.observable();d.lastDraftDate=ko.observable();d.lastDraftErrorDate=ko.observable(null);d.lastDraft=null;d.setAutoSaveTimer=function(){return d.autoSaveTimerId&&f(d.autoSaveTimerId),d.autoSaveTimerId=u(a,n.settings.autoSaveDelay),!0};d.revertDraft=function(){st();d.submittedAnswersJson!=null&&(e.unsubscribeAnswerChanged(d.questions),e.setAnswersFromJson(d.questions,d.submittedAnswersJson),e.subscribeAnswerChanged(d.questions,d.setAutoSaveTimer));d.loadedDraftDate(null)};d.files=ko.observableArray();d.removeFile=function(n){d.files.remove(n)};d.uploading=ko.observable(0);d.uploadFile=function(){var n=i('<input type="file" accept="*" multiple="" />');n.on("change",function(){c(this.files)});n.trigger("click")};d.canUploadMoreFiles=ko.computed({read:function(){return d.uploading()==0&&d.files().length<d.settings.metaReviewMaxFileNumber},deferEvaluation:!0});d.xhrUploadSupported=function(){return o};d.fileUploadDragOver=function(n,t){d.canUploadMoreFiles()&&i(t.target).addClass("dragOver")};d.fileUploadDragLeave=function(n,t){d.canUploadMoreFiles()&&i(t.target).removeClass("dragOver")};d.fileUploadDrop=function(n,t){if(d.canUploadMoreFiles()){var i=t.originalEvent.dataTransfer.files;c(i);d.fileUploadDragLeave(n,t)}};d.uploadSingleFile=function(n,t){t.target.value!=""&&t.target.form.submit()};d.parseSingleUploadResult=function(n,t){l(t.target.contentDocument.body.innerText)};d.save=function(){var u=!0,f=ko.validation.group(d.questions,{deep:!0}),i,r,o;if(f().length>0&&(f.showAllMessages(),u=!1),v()||(u=!1),u){for(i=n.autoMap(d),i.SubmissionId=d.submission.id,d.createNew||(i.Id=d.id),i.Files=[],r=0;r<d.files().length;r++)i.Files.push(d.files()[r].id);i.Answers=e.getAnswersJson(d.questions);o={requestUri:n.odata.getUrl(n.odata.entitySet.metaReviews,d.createNew?null:d.id),method:d.createNew?"POST":"PUT",progressIndicatorTimeout:0,data:i};t.request(o,function(){n.url.navigateTo(s.returnConsole)})}}}function rt(r){return i.Deferred(function(i){if(r.Files.length==0){i.resolve();return}var u=n.odata.getUrl(n.odata.entitySet.files,{filter:n.odata.buildContainsQuery("Id",r.Files)});t.read({requestUri:u,showProgressIndicator:!1},function(t){for(var u=[],r=0;r<t.value.length;r++)u.push(n.autoMap(new h,t.value[r]));d.files(u);i.resolve()})}).promise()}function nt(){return i.Deferred(function(i){var r=n.odata.getUrl(n.odata.entitySet.metaReviewSettings,d.submission.trackId);t.read({requestUri:r,showProgressIndicator:!1},function(t){n.autoMap(d.settings,t);i.resolve()})}).promise()}function tt(){return i.when(ut(),ft()).done(function(){for(var t,i=[],n=0;n<d.questions.length;n++)t=d.questions[n],d.questionInvisibleByTagsMap[t.id]||i.push(t);d.questions=i})}function ut(){return i.Deferred(function(t){e.loadQuestionsDirect(n.enums.formType.metareview,d.formId).done(function(n){d.questions=n;t.resolve()})}).promise()}function ft(){return i.Deferred(function(i){var r=n.odata.getUrl(n.odata.entitySet.questionInvisibleByTags,{filter:"SubmissionId eq {0}".format(n.odata.escapeParam(d.submission.id))});t.read({requestUri:r,showProgressIndicator:!1},function(n){d.questionInvisibleByTagsMap={};d.questionInvisibleByTags=n.value;for(var t=0;t<d.questionInvisibleByTags.length;t++)d.questionInvisibleByTagsMap[d.questionInvisibleByTags[t].QuestionId]=d.questionInvisibleByTags[t];i.resolve(!0)})}).promise()}function et(){return i.Deferred(function(i){var r=n.odata.getUrl(n.odata.entitySet.metaReviews,d.id);t.read({requestUri:r,showProgressIndicator:!1},function(t){n.autoMap(d,t);i.resolve(t)})}).promise()}function it(u){return i.Deferred(function(i){var f=n.odata.getUrl(n.odata.entitySet.metaReviewDrafts,null,"GetBySubmissionIdAndMetaReviewerId");t.read({requestUri:f,showProgressIndicator:!1,data:{SubmissionId:d.submission.id,MetaReviewerId:d.metaReviewerId},method:"POST"},function(n){if(!n){u&&e.setAnswersFromJson(d.questions,u.Answers);i.resolve(!1);return}d.loadedDraftDate(n.UpdateDate.toLocaleString());d.draftId=n.Id;var t=r.parse(n.Draft);e.setAnswersFromJson(d.questions,t);u&&(d.submittedAnswersJson=u.Answers);i.resolve(!0)},function(n){if(n.response.statusCode===404){u&&e.setAnswersFromJson(d.questions,u.Answers);i.resolve(!1);return}t.defaultError(data)})}).promise()}function ot(){return i.Deferred(function(n){g();i.when(et(),nt(),tt()).done(function(t){i.when(rt(t),it(t)).done(function(){n.resolve()})})}).promise()}function st(){if(!d.draftId)return i.Deferred().resolve().promise();var u={requestUri:n.odata.getUrl(n.odata.entitySet.metaReviewDrafts,d.draftId),method:"DELETE",showProgressIndicator:!1};return t.request(u,function(){d.draftId=null;d.lastDraftDate(null);d.lastDraftErrorDate(null);d.lastDraft=r.stringify(e.getAnswersJson(d.questions))})}var d=this;d.id=l;d.formId=b;d.metaReviewerId=n.autoMap();d.updateDate=n.autoMap();d.settings={metaWelcomeMessage:n.autoMap(),metaReviewMinFileNumber:n.autoMap(),metaReviewMaxFileNumber:n.autoMap(),metaReviewAllowedFileTypes:n.autoMap(),metaReviewMaxFileSize:n.autoMap()};d.submission=new c(a,y,p,w,k);d.createNew=!d.id;d.bindTo=function(t){n.showProgress();var f=i.Deferred(),u;d.createNew?(n.autoMap(d,{metaReviewerId:v}),u=i.Deferred(),g(),i.when(nt(),tt()).done(function(){it().done(function(){u.resolve()})})):u=ot();u.promise().done(function(){ko.applyBindingsAndShow(d,t);d.lastDraft=r.stringify(e.getAnswersJson(d.questions));d.setAutoSaveTimer();f.resolve()});f.always(n.hideProgress)}}var s;n.metaReviewDetails=function(n,t,i,r,u,f,e,o,h,c){s=h;new l(n,t,i,r,u,f,e,o).bindTo(c)}}(window.app,window.OData,window.jQuery,window.JSON,window.setTimeout,window.clearTimeout,new window.app.QuestionService,window.FileReader!=undefined),function(n,t,i){"use strict";function r(){var t=this;t.id=n.autoMap();t.originalName=n.autoMap();t.size=n.autoMap();t.formattedSize=n.autoMap();t.uploadDate=n.autoMap();t.downloadLink=n.autoMap()}function u(){var t=this;t.order=n.autoMap();t.details=n.autoMap();t.answers=[]}function f(){var t=this;t.text=n.autoMap();t.value=n.autoMap()}function e(e){function s(){return t.read(n.odata.getUrl(n.odata.entitySet.metaReviewViews,o.id),function(t){var e,h,s,i,c,l;for(n.autoMap(o,t),i=0;i<t.Questions.length;i++){for(e=t.Questions[i],h=n.autoMap(new u,e),s=0;s<e.Answers.length;s++)h.answers.push(n.autoMap(new f,e.Answers[s]));o.questions.push(h)}for(i=0;i<t.Files.length;i++)c=t.Files[i],l=n.autoMap(new r,c),o.files.push(l)})}var o=this;o.id=e;o.trackName=n.autoMap();o.submissionTitle=n.autoMap();o.submissionId=n.autoMap();o.isSingleTrackConference=n.autoMap();o.questions=[];o.files=[];o.print=function(){i()};o.bindTo=function(n){s().done(function(){ko.applyBindingsAndShow(o,n)})}}n.metaReviewView=function(n,t){new e(n).bindTo(t)}}(window.app,window.OData,window.print),function(n,t,i,r,u){"use strict";function e(n,t,i,r,u){var f=this;f.id=n;f.title=t;f.trackId=i;f.trackName=r;f.isSingleTrackConference=u}function o(r,o,s,h,c,l,a,v){function w(){y.questions=[];y.submittedAnswersJson=null;y.save=function(){for(var s=!0,h=[],e,o,i,c,r=0;r<y.questions.length;r++)e=y.questions[r],p.isHidden(e.id)||h.push(e);(o=ko.validation.group(h,{deep:!0}),o().length>0&&(o.showAllMessages(),s=!1),s)&&(i=n.autoMap(y),i.SubmissionId=y.submission.id,y.createNew||(i.Id=y.id),i.Answers=u.getAnswersJson(y.questions.filter(n=>!p.isHidden(n.id))),c={requestUri:n.odata.getUrl(n.odata.entitySet.reviewerNotes,y.createNew?null:y.id),method:y.createNew?"POST":"PUT",progressIndicatorTimeout:0,data:i},t.request(c,function(){n.url.navigateTo(f.submissionReviewConsole)}))}}function b(){return i.when(k()).done(function(){for(var i,t=[],n=0;n<y.questions.length;n++)i=y.questions[n],t.push(i);y.questions=t})}function k(){return i.Deferred(function(t){u.loadQuestionsDirect(n.enums.formType.reviewernote,y.formId).done(function(n){y.questions=n;p.loadQuestions(n);t.resolve()})}).promise()}function d(){return i.Deferred(function(i){var r=n.odata.getUrl(n.odata.entitySet.reviewerNotes,y.id);t.read({requestUri:r,showProgressIndicator:!1},function(t){n.autoMap(y,t);i.resolve(t)})}).promise()}function g(){return i.Deferred(function(n){w();i.when(d(),b()).done(function(t){t&&u.setAnswersFromJson(y.questions,t.Answers);n.resolve()})}).promise()}var y=this,p=new n.QuestionDependency(y);y.id=r;y.formId=a;y.reviewerId=n.autoMap();y.updateDate=n.autoMap();y.submission=new e(o,h,c,l,v);y.createNew=!y.id;y.hasBranchingQuestions=function(){return p.hasDependency()};y.getQuestionDiv=function(n){return i("#nq_"+n)};y.bindTo=function(t){n.showProgress();var u=i.Deferred(),r;y.createNew?(n.autoMap(y,{reviewerId:s}),r=i.Deferred(),w(),i.when(b()).done(function(){r.resolve()})):r=g();r.promise().done(function(){ko.applyBindingsAndShow(y,t);p.init();u.resolve()});u.always(n.hideProgress)}}var f;n.reviewNoteDetails=function(n,t,i,r,u,e,s,h,c,l){f=c;new o(n,t,i,r,u,e,s,h).bindTo(l)}}(window.app,window.OData,window.jQuery,window.JSON,new window.app.QuestionService),function(n,t,i,r,u){"use strict";function e(n,t,i,r,u){var f=this;f.id=n;f.title=t;f.trackId=i;f.trackName=r;f.isSingleTrackConference=u}function o(r,o,s,h,c,l,a,v){function w(){y.questions=[];y.submittedAnswersJson=null;y.save=function(){for(var s=!0,h=[],e,o,i,c,r=0;r<y.questions.length;r++)e=y.questions[r],p.isHidden(e.id)||h.push(e);(o=ko.validation.group(h,{deep:!0}),o().length>0&&(o.showAllMessages(),s=!1),s)&&(i=n.autoMap(y),i.SubmissionId=y.submission.id,y.createNew||(i.Id=y.id),i.Answers=u.getAnswersJson(y.questions.filter(n=>!p.isHidden(n.id))),c={requestUri:n.odata.getUrl(n.odata.entitySet.metaReviewerNotes,y.createNew?null:y.id),method:y.createNew?"POST":"PUT",progressIndicatorTimeout:0,data:i},t.request(c,function(){n.url.navigateTo(f.submissionMetaReviewConsole)}))}}function b(){return i.when(k()).done(function(){for(var i,t=[],n=0;n<y.questions.length;n++)i=y.questions[n],t.push(i);y.questions=t})}function k(){return i.Deferred(function(t){u.loadQuestionsDirect(n.enums.formType.metareviewernote,y.formId).done(function(n){y.questions=n;p.loadQuestions(n);t.resolve()})}).promise()}function d(){return i.Deferred(function(i){var r=n.odata.getUrl(n.odata.entitySet.metaReviewerNotes,y.id);t.read({requestUri:r,showProgressIndicator:!1},function(t){n.autoMap(y,t);i.resolve(t)})}).promise()}function g(){return i.Deferred(function(n){w();i.when(d(),b()).done(function(t){t&&u.setAnswersFromJson(y.questions,t.Answers);n.resolve()})}).promise()}var y=this,p=new n.QuestionDependency(y);y.id=r;y.formId=a;y.metaReviewerId=n.autoMap();y.updateDate=n.autoMap();y.submission=new e(o,h,c,l,v);y.createNew=!y.id;y.hasBranchingQuestions=function(){return p.hasDependency()};y.getQuestionDiv=function(n){return i("#nq_"+n)};y.bindTo=function(t){n.showProgress();var u=i.Deferred(),r;y.createNew?(n.autoMap(y,{metaReviewerId:s}),r=i.Deferred(),w(),i.when(b()).done(function(){r.resolve()})):r=g();r.promise().done(function(){ko.applyBindingsAndShow(y,t);p.init();u.resolve()});u.always(n.hideProgress)}}var f;n.metaReviewNoteDetails=function(n,t,i,r,u,e,s,h,c,l){f=c;new o(n,t,i,r,u,e,s,h).bindTo(l)}}(window.app,window.OData,window.jQuery,window.JSON,new window.app.QuestionService),function(n,t,i,r,u){"use strict";function e(n,t,i,r,u){var f=this;f.id=n;f.title=t;f.trackId=i;f.trackName=r;f.isSingleTrackConference=u}function o(r,o,s,h,c,l,a,v){function w(){y.questions=[];y.submittedAnswersJson=null;y.save=function(){for(var s=!0,h=[],e,o,i,c,r=0;r<y.questions.length;r++)e=y.questions[r],p.isHidden(e.id)||h.push(e);(o=ko.validation.group(h,{deep:!0}),o().length>0&&(o.showAllMessages(),s=!1),s)&&(i=n.autoMap(y),i.SubmissionId=y.submission.id,y.createNew||(i.Id=y.id),i.Answers=u.getAnswersJson(y.questions.filter(n=>!p.isHidden(n.id))),c={requestUri:n.odata.getUrl(n.odata.entitySet.seniorMetaReviewerNotes,y.createNew?null:y.id),method:y.createNew?"POST":"PUT",progressIndicatorTimeout:0,data:i},t.request(c,function(){n.url.navigateTo(f.submissionSeniorMetaReviewConsole)}))}}function b(){return i.when(k()).done(function(){for(var i,t=[],n=0;n<y.questions.length;n++)i=y.questions[n],t.push(i);y.questions=t})}function k(){return i.Deferred(function(t){u.loadQuestionsDirect(n.enums.formType.seniormetareviewernote,y.formId).done(function(n){y.questions=n;p.loadQuestions(n);t.resolve()})}).promise()}function d(){return i.Deferred(function(i){var r=n.odata.getUrl(n.odata.entitySet.seniorMetaReviewerNotes,y.id);t.read({requestUri:r,showProgressIndicator:!1},function(t){n.autoMap(y,t);i.resolve(t)})}).promise()}function g(){return i.Deferred(function(n){w();i.when(d(),b()).done(function(t){t&&u.setAnswersFromJson(y.questions,t.Answers);n.resolve()})}).promise()}var y=this,p=new n.QuestionDependency(y);y.id=r;y.formId=a;y.seniorMetaReviewerId=n.autoMap();y.updateDate=n.autoMap();y.submission=new e(o,h,c,l,v);y.createNew=!y.id;y.hasBranchingQuestions=function(){return p.hasDependency()};y.getQuestionDiv=function(n){return i("#nq_"+n)};y.bindTo=function(t){n.showProgress();var u=i.Deferred(),r;y.createNew?(n.autoMap(y,{seniorMetaReviewerId:s}),r=i.Deferred(),w(),i.when(b()).done(function(){r.resolve()})):r=g();r.promise().done(function(){ko.applyBindingsAndShow(y,t);p.init();u.resolve()});u.always(n.hideProgress)}}var f;n.seniorMetaReviewNoteDetails=function(n,t,i,r,u,e,s,h,c,l){f=c;new o(n,t,i,r,u,e,s,h).bindTo(l)}}(window.app,window.OData,window.jQuery,window.JSON,new window.app.QuestionService),function(n,t,i){"use strict";function r(){var t=this;t.id=n.autoMap();t.originalName=n.autoMap();t.size=n.autoMap();t.formattedSize=n.autoMap();t.uploadDate=n.autoMap();t.downloadLink=n.autoMap()}function u(){var t=this;t.order=n.autoMap();t.details=n.autoMap();t.answers=[]}function f(){var t=this;t.text=n.autoMap();t.value=n.autoMap()}function e(){var i=this;i.id=n.autoMap();i.metaReviewerNumber=n.autoMap();i.metaReviewerId=n.autoMap();i.metaReviewerName=n.autoMap();i.userType=n.autoMap();i.isSubmitted=n.autoMap();i.questions=[];i.files=[];i.deleteMetaReview=function(){if(i.id&&i.metaReviewerName&&confirm("You will not be able to revert this action. Are you sure you want to delete meta-review submitted by {0}?".format(i.metaReviewerName))){var r={requestUri:n.odata.getUrl(n.odata.entitySet.metaReviews,i.id),method:"DELETE"};t.request(r,function(){window.location.reload()},function(n){OData.defaultError(n)})}}}function o(o){function h(){return t.read(n.odata.getUrl(n.odata.entitySet.submissions,s.id,"MetaReviews"),function(t){for(var i,h,o,v,p,y,w,b,k,c,l=[],a=0;a<t.value.length;a++){for(i=t.value[a],a===0&&(s.trackName=i.TrackName,s.title=i.SubmissionTitle,s.isSingleTrackConference=i.IsSingleTrackConference),h=n.autoMap(new e,i),o=0;o<i.Questions.length;o++){for(v=i.Questions[o],p=n.autoMap(new u,v),y=0;y<v.Answers.length;y++)p.answers.push(n.autoMap(new f,v.Answers[y]));h.questions.push(p)}for(o=0;o<i.Files.length;o++)w=i.Files[o],b=n.autoMap(new r,w),h.files.push(b);h.metaReviewerNumber>0?s.metaReviews.push(h):l.push(h)}for(k=s.metaReviews.length===0?1:s.metaReviews[s.metaReviews.length-1].metaReviewerNumber+1,c=0;c<l.length;c++)l[c].metaReviewerNumber=k++,s.metaReviews.push(l[c])})}var s=this;s.id=o;s.trackName=null;s.title=null;s.isSingleTrackConference=null;s.metaReviews=[];s.print=function(){i()};s.bindTo=function(n){h().done(function(){ko.applyBindingsAndShow(s,n)})}}n.submissionMetaReviews=function(n){new o(n).bindTo("submissionForm")}}(window.app,window.OData,window.print),function(n,t,i){"use strict";function r(n,r){var u=this,f,e;if(n?(u.id=n.Id,u.firstName=n.FirstName,u.middleInitial=n.MiddleInitial,u.lastName=n.LastName,u.email=n.Email,u.organization=n.Organization,u.numberOfBids=n.NumberOfBids,u.numberOfSuggestedSubmissions=n.NumberOfSuggestedSubmissions,u.numberOfSuggestedReviewers=n.NumberOfSuggestedReviewers,u.numberOfAssignment=n.NumberOfAssignment,u.numberOfCompleted=n.NumberOfCompleted,u.percentageOfCompleted=n.PercentageOfCompleted,u.numberOfNotes=n.NumberOfNotes,u.percentageOfCompletedNote=n.PercentageOfCompletedNote,u.numberOfComparisons=n.NumberOfComparisons,u.conflictDomainsEntered=n.ConflictDomainsEntered,u.individualConflictsEntered=n.IndividualConflictsEntered,u.userType=n.UserType,u.quota=n.Quota,u.subjectAreaSelected=n.SubjectAreaSelected,u.primarySubject=n.PrimarySubject,u.secondarySubject=n.SecondarySubject,u.seniorMetaReviewers=n.SeniorMetaReviewers,u.userTagJson=n.UserTagJson):(u.id=t.autoMap(),u.firstName=t.autoMap(),u.middleInitial=t.autoMap(),u.lastName=t.autoMap(),u.email=t.autoMap(),u.organization=t.autoMap(),u.numberOfBids=t.autoMap(),u.numberOfSuggestedSubmissions=t.autoMap(),u.numberOfSuggestedReviewers=t.autoMap(),u.numberOfAssignment=t.autoMap(),u.numberOfCompleted=t.autoMap(),u.percentageOfCompleted=t.autoMap(),u.numberOfNotes=t.autoMap(),u.percentageOfCompletedNote=t.autoMap(),u.numberOfComparisons=t.autoMap(),u.conflictDomainsEntered=t.autoMap(),u.individualConflictsEntered=t.autoMap(),u.userType=t.autoMap(),u.quota=t.autoMap(),u.subjectAreaSelected=t.autoMap(),u.primarySubject=t.autoMap(),u.secondarySubject=t.autoMap(),u.seniorMetaReviewers=t.autoMap(),u.userTagJson=t.autoMap()),u.userTags=[],f=u.userTagJson&&JSON.parse(u.userTagJson),f)for(e=0;e<f.length;e++)u.userTags.push(t.autoMap(new t.UserTag,f[e]));u.individualConflictsEnteredText=ko.pureComputed(function(){return u.individualConflictsEntered===!0?"Yes":"No"});u.exportBids=function(){var n=t.odata.getUrl("MetaBiddingModels",null,"ExportToTabDelimitedFile"),i={UserId:u.id,TrackId:r.selectedTrackId()};t.page.post(n,i)};u.impersonate=function(n){if(confirm("Are you sure to impersonate as {0} {1}?".format(n.firstName,n.lastName))){var r={requestUri:t.odata.getUrl("Users",n.id,"Impersonate"),method:"POST"};i.request(r,function(n){t.odata.processRedirectResponse(n)})}};u.removeMetaReviewer=function(n){r.removeMetaReviewer(n)}}function u(r,u){var e=u,f=this;f.filter=null;f.userCount=ko.observable(0);f.selectedUserType=ko.observable("");f.userTypes=e.userTypes;f.submitEnabled=ko.computed(function(){return f.userCount()<=0?!1:f.selectedUserType()!==null&&typeof f.selectedUserType()!="undefined"});f.changeUserType=function(){var u={Filter:f.filter,UserTypeOptionId:f.selectedUserType(),TrackId:e.selectedTrackId()},o={requestUri:t.odata.getUrl(e.controller,null,"BulkChangeUserType"),method:"POST",showProgressIndicator:!0,data:{Request:u}};i.request(o,function(){e.refresh();setTimeout(function(){t.addMessage("The user types of selected meta-reviewers have been changed.")},500);n(r).modal("hide")})};f.bind=function(){ko.applyBindings(f,r)};f.editInDialog=function(t){f.filter=t;var u=t?"&$filter="+encodeURIComponent(t):"";i.read({requestUri:"/api/odata/"+window.cmt3.conference.name+"/"+e.controller+"?key="+e.selectedTrackId()+"&$count=true"+u,dataType:"json"},function(t){f.userCount(t["@odata.count"]);f.selectedUserType("");n(r).modal("show")})}}t.MetaReviewersStatPage=function(n,f,e,o,s,h,c,l,a,v){function g(n,t){var i=t;return n!==null&&n.length>0&&(isNaN(n)||(i=parseInt(n))),i}function nt(n,r){var f=function(n){return{Role:"MetaReviewer",ObjectId:n,ObjectType:"Track"}},u={},e;return r?(u.Add=[f(w)],u.Remove=[]):(u.Add=[],u.Remove=[f(w)]),e={requestUri:t.odata.getUrl(t.odata.entitySet.users,n,"ModifyPermissions"),method:"POST",data:{Request:u}},i.request(e,function(){})}function tt(n){return n.Name}var w=g(e,null),y,b,d,p,k;for(w==null?t.Page.call(this,n,f,"key=-1"):t.Page.call(this,n,f,"key="+w),y=this,y.controller=f,y.removeMetaReviewer=function(n){var i="Are you sure you want to remove meta-reviewer {0} {1}".format(n.firstName,n.lastName);n.numberOfAssignment>0&&(i+=" who is assigned to {0} paper{1}".format(n.numberOfAssignment,n.numberOfAssignment>1?"s":""),n.numberOfCompleted>0&&(i+=" and has submitted {0} meta-review{1}".format(n.numberOfCompleted,n.numberOfCompleted>1?"s":"")));i+="?";confirm(i)&&nt(n.id,!1).done(function(){y.show();t.addMessage("Meta-Reviewer has been successfully removed.")})},y.trackId=w,y.requireConflictDomains=s,y.requireIndividualConflict=h,y.suggestionsEnabled=c,y.useSeniorMetaReviewer=l,y.allowMetaReviewerToCompareSubmission=a,y.userTypes=v,y.userTypesProvider=function(){return y.userTypes.map(tt)},y.createItem=function(n){return new r(n,y)},y.changeTrack=function(n){var t="/"+window.cmt3.conference.name+"/User/MetaReviewers";n.id>=0&&(t=t+"?trackId="+n.id);window.location=t},y.tracks=ko.observableArray(),y.selectedTrack=ko.observable(),y.selectedTrackId=ko.pureComputed(function(){var t=y.selectedTrack(),n;return t&&t.id>0?t.id:(n=y.tracks(),n=n&&n.filter(function(n){return n.id>0}),n&&n.length===1)?n[0].id:-1}),o.length>1&&(b=new t.Track,b.id=-1,b.name="<All Tracks>",y.tracks.push(b),y.selectedTrack(b)),p=0;p<o.length;p++)d=t.autoMap(new t.Track,o[p]),y.tracks.push(d);for(p=0;p<y.tracks().length;p++)if(y.trackId==y.tracks()[p].id){y.selectedTrack(y.tracks()[p]);break}y.refresh=function(){y.show()};y.selectedTrackSubscription=y.selectedTrack.subscribe(y.changeTrack);y.users=ko.observableArray();y.exportMetaReviewers=function(n,i){var r=t.GetEventFilter(i),u=t.odata.getUrl("TrackMetaReviewers",null,"ExportTrackMetaReviewers"),f={TrackId:y.selectedTrackId(),Filter:r};t.page.post(u,f)};y.exportMetaReviews=function(n,i){var r=t.GetEventFilter(i),f="/api/odata/"+window.cmt3.conference.name+"/SubmissionViews/ExportMetaReviews2",u;u=y.trackId!=null?{Filter:r,TrackId:y.trackId}:{Filter:r};t.page.post(f,u)};y.bulkChangeUserType=function(n,i){var r=t.GetEventFilter(i);this.changeUserType(r)};k=null;y.changeUserType=function(n){k===null&&(k=new u(document.getElementById("changeUserTypeDialog"),y,t),k.bind());k.editInDialog(n)};y.exportMetaReviewerQuotas=function(){var n="/api/odata/"+window.cmt3.conference.name+"/Users/ExportUserQuotas",i={TrackId:y.trackId,ForReviewer:!1};t.page.post(n,i)};y.exportMetaReviewerRelevances=function(){var n="/api/odata/"+window.cmt3.conference.name+"/Users/ExportUserRelevances",i={TrackId:y.selectedTrackId(),ForReviewer:!1};t.page.post(n,i)};y.exportMetaReviewerSubjectAreas=function(){var n="/api/odata/"+window.cmt3.conference.name+"/Users/ExportUserSubjectAreas",i={TrackId:y.selectedTrackId(),ForReviewer:!1,ForSeniorMetaReviewer:!1};t.page.post(n,i)};y.importUserQuotas=function(){var n="/"+window.cmt3.conference.name+"/MetaReviewer/ImportQuotas";t.url.navigateTo(n,{trackId:y.trackId})};y.importUserTypes=function(){var n="/"+window.cmt3.conference.name+"/User/ImportUserTypes";t.url.navigateTo(n,{roleValue:8})};y.importUserTags=function(){var n="/"+window.cmt3.conference.name+"/User/ImportUserTags";t.url.navigateTo(n,{roleValue:8})};y.email=function(n,i){var r=t.GetEventFilter(i),u="/"+window.cmt3.conference.name+"/MetaReviewer/SendEmail";t.url.navigateTo(u,{filter:r.length>0?r:null,trackId:y.trackId<0?null:y.trackId})};y.show=function(){t.Page.prototype.show.call(y)}};t.MetaReviewersStatPage.prototype=Object.create(t.Page.prototype)}(window.jQuery,window.app,window.OData),function(n,t,i){"use strict";function r(n){var r=this,u,f;if(n?(r.id=n.Id,r.firstName=n.FirstName,r.middleInitial=n.MiddleInitial,r.lastName=n.LastName,r.email=n.Email,r.organization=n.Organization,r.numberOfBids=n.NumberOfBids,r.numberOfAssignment=n.NumberOfAssignment,r.numberOfNotes=n.NumberOfNotes,r.numberOfRatings=n.NumberOfRatings,r.percentageOfCompletedNote=n.PercentageOfCompletedNote,r.percentageOfCompletedRating=n.PercentageOfCompletedRating,r.conflictDomainsEntered=n.ConflictDomainsEntered,r.individualConflictsEntered=n.IndividualConflictsEntered,r.userType=n.UserType,r.subjectAreaSelected=n.SubjectAreaSelected,r.primarySubject=n.PrimarySubject,r.secondarySubject=n.SecondarySubject,r.userTagJson=n.UserTagJson):(r.id=t.autoMap(),r.firstName=t.autoMap(),r.middleInitial=t.autoMap(),r.lastName=t.autoMap(),r.email=t.autoMap(),r.organization=t.autoMap(),r.numberOfAssignment=t.autoMap(),r.numberOfBids=t.autoMap(),r.numberOfNotes=t.autoMap(),r.numberOfRatings=t.autoMap(),r.percentageOfCompletedNote=t.autoMap(),r.percentageOfCompletedRating=t.autoMap(),r.conflictDomainsEntered=t.autoMap(),r.individualConflictsEntered=t.autoMap(),r.userType=t.autoMap(),r.subjectAreaSelected=t.autoMap(),r.primarySubject=t.autoMap(),r.secondarySubject=t.autoMap(),r.userTagJson=t.autoMap()),r.userTags=[],u=r.userTagJson&&JSON.parse(r.userTagJson),u)for(f=0;f<u.length;f++)r.userTags.push(t.autoMap(new t.UserTag,u[f]));r.individualConflictsEnteredText=ko.pureComputed(function(){return r.individualConflictsEntered===!0?"Yes":"No"});r.impersonate=function(n){if(confirm("Are you sure to impersonate as {0} {1}?".format(n.firstName,n.lastName))){var r={requestUri:t.odata.getUrl("Users",n.id,"Impersonate"),method:"POST"};i.request(r,function(n){t.odata.processRedirectResponse(n)})}}}function u(r,u){var e=u,f=this;f.filter=null;f.userCount=ko.observable(0);f.selectedUserType=ko.observable("");f.userTypes=e.userTypes;f.submitEnabled=ko.computed(function(){return f.userCount()<=0?!1:f.selectedUserType()!==null&&typeof f.selectedUserType()!="undefined"});f.changeUserType=function(){var u={Filter:f.filter,UserTypeOptionId:f.selectedUserType(),TrackId:e.selectedTrackId()},o={requestUri:t.odata.getUrl(e.controller,null,"BulkChangeUserType"),method:"POST",showProgressIndicator:!0,data:{Request:u}};i.request(o,function(){e.refresh();setTimeout(function(){t.addMessage("The user types of selected senior meta-reviewers have been changed.")},500);n(r).modal("hide")})};f.bind=function(){ko.applyBindings(f,r)};f.editInDialog=function(t){f.filter=t;var u=t?"&$filter="+encodeURIComponent(t):"";i.read({requestUri:"/api/odata/"+window.cmt3.conference.name+"/"+e.controller+"?key="+e.selectedTrackId()+"&$count=true"+u,dataType:"json"},function(t){f.userCount(t["@odata.count"]);f.selectedUserType("");n(r).modal("show")})}}t.SeniorMetaReviewersStatPage=function(n,f,e,o,s,h,c,l){function k(n,t){var i=t;return n!==null&&n.length>0&&(isNaN(n)||(i=parseInt(n))),i}function d(n){return n.Name}function g(n,r){var f=function(n){return{Role:"SeniorMetaReviewer",ObjectId:n,ObjectType:"Track"}},u={},e;return r?(u.Add=[f(p)],u.Remove=[]):(u.Add=[],u.Remove=[f(p)]),e={requestUri:t.odata.getUrl(t.odata.entitySet.users,n,"ModifyPermissions"),method:"POST",data:{Request:u}},i.request(e,function(){})}var p=k(e,null),a,y,v,b,w;if(p===null?t.Page.call(this,n,f,"key=-1"):t.Page.call(this,n,f,"key="+p),a=this,a.trackId=p,a.userTypes=l,a.userTypesProvider=function(){return a.userTypes.map(d)},a.requireConflictDomains=s,a.requireIndividualConflict=h,a.assignSubmissionIndirectlyToSMR=c,a.removeSeniorMetaReviewer=function(n){var i="Are you sure you want to remove senior meta-reviewer {0} {1}".format(n.firstName,n.lastName);n.numberOfAssignment>0&&(i+=a.assignSubmissionIndirectlyToSMR?" who is assigned to {0} meta-reviewer{1}".format(n.numberOfAssignment,n.numberOfAssignment>1?"s":""):" who is assigned to {0} paper{1}".format(n.numberOfAssignment,n.numberOfAssignment>1?"s":""));i+="?";confirm(i)&&g(n.id,!1).done(function(){a.show();t.addMessage("Senior Meta-Reviewer has been successfully removed.")})},a.createItem=function(n){return new r(n)},a.changeTrack=function(n){var t="/"+window.cmt3.conference.name+"/User/SeniorMetaReviewers";n.id>=0&&(t=t+"?trackId="+n.id);window.location=t},a.tracks=ko.observableArray(),a.selectedTrack=ko.observable(),y=null,o.length>1?(y=new t.Track,y.id=-1,y.name="<All Tracks>"):o.length>0&&(y=t.autoMap(new t.Track,o[0]),a.trackId=y.id),a.tracks.push(y),a.selectedTrack(y),a.selectedTrackId=ko.pureComputed(function(){var t=a.selectedTrack(),n;return t&&t.id>0?t.id:(n=a.tracks(),n=n&&n.filter(function(n){return n.id>0}),n&&n.length===1)?n[0].id:-1}),o.length>1){for(v=0;v<o.length;v++)b=t.autoMap(new t.Track,o[v]),a.tracks.push(b);for(v=0;v<a.tracks().length;v++)if(a.trackId===a.tracks()[v].id){a.selectedTrack(a.tracks()[v]);break}a.selectedTrackSubscription=a.selectedTrack.subscribe(a.changeTrack)}a.users=ko.observableArray();a.importUserTypes=function(){var n="/"+window.cmt3.conference.name+"/User/ImportUserTypes";t.url.navigateTo(n,{roleValue:256})};a.importUserTags=function(){var n="/"+window.cmt3.conference.name+"/User/ImportUserTags";t.url.navigateTo(n,{roleValue:256})};a.email=function(n,i){var r=t.GetEventFilter(i),u="/"+window.cmt3.conference.name+"/SeniorMetaReviewer/SendEmail";t.url.navigateTo(u,{filter:r.length>0?r:null,trackId:a.trackId<0?null:a.trackId})};a.importSeniorMetaReviewerAssignments=function(){var n="/"+window.cmt3.conference.name+"/SeniorMetaReviewer/ImportAssignments";t.url.navigateTo(n,{trackId:a.trackId})};a.exportSeniorMetaReviewerBids=function(){var n="/api/odata/"+window.cmt3.conference.name+"/Users/ExportSeniorMetaReviewerBids",i={TrackId:a.trackId};t.page.post(n,i)};a.exportSeniorMetaReviewerAssignments=function(){var n="/api/odata/"+window.cmt3.conference.name+"/Users/ExportSeniorMetaReviewerAssignments",i={TrackId:a.trackId};t.page.post(n,i)};a.exportSeniorMetaReviewerSubjectAreas=function(){var n="/api/odata/"+window.cmt3.conference.name+"/Users/ExportUserSubjectAreas",i={TrackId:a.trackId,ForReviewer:!1,ForSeniorMetaReviewer:!0};t.page.post(n,i)};a.show=function(){t.Page.prototype.show.call(a)};a.bulkChangeUserType=function(n,i){var r=t.GetEventFilter(i);this.changeUserType(r)};w=null;a.changeUserType=function(n){w===null&&(w=new u(document.getElementById("changeUserTypeDialog"),a,t),w.bind());w.editInDialog(n)};a.refresh=function(){a.show()}};t.SeniorMetaReviewersStatPage.prototype=Object.create(t.Page.prototype)}(window.jQuery,window.app,window.OData),function(n,t,i,r){"use strict";function f(u,f){var e=this,o=null;e.parent=f;e.fromEmail=ko.observable();e.fromName=ko.observable();e.toEmail=ko.observable();e.toName=ko.observable();e.subject=ko.observable();e.body=ko.observable("");e.previewIndex=ko.observable(0);e.showInDialog=function(){e.previewIndex(0);e.refreshPreview(function(){i(u).modal("show")})};e.isPreviousEnabled=ko.pureComputed(function(){return this.previewIndex()>0},e);e.isNextEnabled=ko.pureComputed(function(){return this.previewIndex()+1<this.parent.emails().length},e);e.previousClick=function(){e.previewIndex()>0&&(e.previewIndex(e.previewIndex()-1),e.refreshPreview())};e.nextClick=function(){e.previewIndex()+1<e.parent.emails().length&&(e.previewIndex(e.previewIndex()+1),e.refreshPreview())};e.refreshPreview=function(i){var r=e.parent.emails()[e.previewIndex()],u={InviteType:e.parent.inviteType,ReviewerInvitationId:r,Subject:e.parent.subject(),Body:e.parent.body()},f={requestUri:n.odata.getUrl(n.odata.entitySet.emails,null,"ResendInvitesPreview"),method:"POST",data:{Request:u}};t.request(f,function(n){e.fromEmail(n.FromEmail);e.fromName(n.FromName);e.toEmail(n.ToEmail);e.toName(n.ToName);e.subject(n.Subject);e.body(n.Body);i&&i()})};e.sendEmails=function(){for(var h,c,l,s=[],f=0;f<e.parent.emails().length;f++)h=e.parent.emails()[f],s.push(h);c={InviteType:e.parent.inviteType,Invites:s,Subject:e.parent.subject(),Body:e.parent.body()};l={requestUri:n.odata.getUrl(n.odata.entitySet.emails,null,"ResendInvites"),method:"POST",data:{Request:c}};t.request(l,function(t){var f=t.value;i(u).modal("hide");o||(o=new n.EmailProgressViewModel(r.getElementById("showProgressDialog")),o.bind());o.showInDialog(f)})};e.bind=function(){ko.applyBindings(e,u)}}function e(e,o){function c(){h||(h=new f(r.getElementById("previewEmailDialog"),s),h.bind());h.showInDialog()}function l(){var n=ko.validation.group(s);return n().length>0?(n.showAllMessages(),!1):!0}function a(){var i={InvitesFilter:u,InviteType:o},r={requestUri:n.odata.getUrl(n.odata.entitySet.emails,null,"ResendInvitesInfo"),method:"POST",data:{Request:i}};return t.request(r,function(n){for(var t=0;t<n.Invites.length;t++)s.emails.push(n.Invites[t]);s.subject(n.Subject);s.body(n.Body)})}var s=this,h=null;s.inviteType=o;s.from=e;s.subject=ko.observable("").extend({required:!0}).autoMap();s.body=ko.observable("").extend({required:!0}).autoMap();s.emails=ko.observableArray();s.showPlaceholders=ko.observable(!1);s.previewEnabled=ko.pureComputed(function(){return this.emails().length>0},s);s.previewEmail=function(){s.emails().length<=0||l()&&c()};s.bindTo=function(n){i.when(a()).done(function(){ko.applyBindingsAndShow(s,n)})}}var u=n.url==undefined?null:n.url.queryString.getValue("filter");n.resendInvites=function(n,t,i){new e(n,t).bindTo(i)}}(window.app,window.OData,window.jQuery,window.document);ExternalReviewPage.prototype={listen:function(){var n=this;$(document).on("data.filter",function(){n.Pager().CurrentPage()<2?n.show():n.Pager().CurrentPage(1)})},getFilter:function(){var n="";return $.each(this.filters,function(t,i){i.getValue()&&(n+=n==""?i.getValue():" and "+i.getValue())}),n},show:function(){var n=this;if(n.initialized){var t=n.sort(),i=n.top(),r=n.skip(),u=n.getFilter(),f=t?"&$orderby="+t:"",e=i?"&$top="+i:"",o=r?"&$skip="+r:"",s=u?"&$filter="+encodeURIComponent(u):"",h={headers:{Accept:"application/json"},requestUri:"/api/odata/"+this.conference+"/$batch",method:"POST",data:{requests:[{url:"/api/odata/"+this.conference+"/"+n.controller+"?$count=true"+f+s+o+e,method:"GET",headers:{Accept:"application/json"}}]}};OData.request(h,function(f){app.page.saveState("externalReviewModels",{sort:t,top:i,skip:r,filter:u});var e=f.responses[0].body,o=e["@odata.count"],h=e.value,s=[];$.each(h,function(t,i){s.push(new ExternalReviewModel(i,n.pageUrls))});n.externalReviewModels(s);n._total()==0&&n._total(o);n.selected(o);$("html,body").scrollTop(0)},function(n){window.cmt3.logger.log(n.message)},OData.batchHandler)}},scroll:function(){$(window).scrollTop()==$(document).height()-$(window).height()&&self.show()},post:function(n,t,i){var r,f,u;i=i||"post";r=document.createElement("form");r.setAttribute("method",i);r.setAttribute("action",n);for(f in t)t.hasOwnProperty(f)&&(u=document.createElement("input"),u.setAttribute("type","hidden"),u.setAttribute("name",f),u.setAttribute("value",t[f]),r.appendChild(u));document.body.appendChild(r);r.submit();document.body.removeChild(r)},stub:function(){alert("Sorry, this feature is not implemented yet.")},reset:function(){$.each(this.filters,function(n,t){t.reset()});this.show()},size:function(n,t){var i,r,u;$("a",".show").removeClass("btn-success").css("color","#999999");$(t.currentTarget).addClass("btn-success").css("color","white");i=$(t.target).attr("size");r=parseInt(i);this.top(r);u=this.Pager().CurrentPage();this.Pager().CurrentPage(1);u===1&&this.show()},skip:function(){return(this.page()-1)*this.top()},prev:function(){this.top()!=0&&this.page()!=1&&(this.page(this.page()-1),this.show())},next:function(){this.top()==0||this.page()>this.selected()/this.top()||(this.page(this.page()+1),this.show())},setSort:function(n,t){var i=$(t.target),r=i.attr("data-sort");(r==null||r==undefined)&&(i=$(i.context.parentNode),r=i.attr("data-sort"));i.hasClass("selected")?this.sort().match(" desc$")?(this.sort(r+" asc"),i.find("i").removeClass("icon-arrow-down"),i.find("i").addClass("icon-arrow-up")):(this.sort(r+" desc"),i.find("i").removeClass("icon-arrow-up"),i.find("i").addClass("icon-arrow-down")):($("th[data-sort]").each(function(){$(this).find("i").removeClass("icon-arrow-up");$(this).find("i").removeClass("icon-arrow-down");$(this).removeClass("selected")}),i.find("i").removeClass("icon-arrow-down"),i.find("i").addClass("icon-arrow-up"),i.addClass("selected"),this.sort(r+" asc"));this.show()},refresh:function(){this.show()},showAbstract:function(n,t){var u=ko.contextFor(t.target).$parent,i=$(t.target),r=i.next();r.is(":visible")?(r.hide(),i.text("Show abstract")):(r.show(),i.text("Hide abstract"))}},function(n,t,i){"use strict";function r(n){var t=this;t.number=n.Number;t.errorMessage=n.ErrorMessage}function u(n){var t=this,i;if(t.reviewId=n.ReviewId,t.submissionId=n.SubmissionId,t.title=n.Title,t.errorMessage=n.ErrorMessage,t.questions=[],n.BadQuestions!==null)for(i=0;i<n.BadQuestions.length;i++)t.questions.push(new r(n.BadQuestions[i]))}function f(n,t){var i=this;i.id=n.Id;i.title=n.Title;i.track=n.Track;i.selected=ko.observable(!1);i.enabled=t?n.MetaReviewingEnabled:n.ReviewingEnabled||n.DiscussionEnabled&&n.SubmissionEnabledForDiscussion}function e(r,e){function s(i){return t.request({requestUri:n.odata.getUrl((i?n.odata.entitySet.metaReviewModels:n.odata.entitySet.reviewModels)+"?$filter=Assigned eq true")},function(n){for(var t=0;t<n.value.length;t++)o.models.push(new f(n.value[t],i))})}var o=this;o.isMeta=r;o.models=ko.observableArray();o.isFileUploaded=ko.observable(!1);o.hasError=ko.observable(!1);o.errorText=ko.observable();o.uploading=ko.observable(!1);o.goodPapers=ko.observableArray();o.badPapers=ko.observableArray();o.file=ko.observable(null);o.getReviewUrl=function(n){return o.isMeta?e.metaReviewView.format(n):e.reviewView.format(n)};o.getSubmissionUrl=function(n){return e.submissionView.format(n)};o.uploadFile=function(n,t){t.target.value!==""&&(o.uploading(!0),t.target.form.submit())};o.parseUploadResult=function(){var n=i.parseJSON(i("#singleFileUploadFrame").contents().text()),t,r;if(o.goodPapers.removeAll(),o.badPapers.removeAll(),o.hasError(n.HasError),o.errorText(n.ErrorText),!o.hasError())for(t=0;t<n.Models.length;t++)r=new u(n.Models[t]),r.reviewId===null?o.badPapers.push(r):o.goodPapers.push(r);o.isFileUploaded(!0);o.uploading(!1);o.file(null)};o.downloadClick=function(){for(var i,r=[],t=0;t<o.models().length;t++)i=o.models()[t],i.selected()&&r.push(i.id);var u=r.join(","),f="/api2/"+window.cmt3.conference.name+"/ExportReviewTemplate",e={Ids:u,IsMeta:o.isMeta};n.page.post(f,e)};o.atLeastOneSubmissionSelected=ko.computed(function(){for(var t=!1,n=0;n<o.models().length;n++)t|=o.models()[n].selected();return t});o.bindTo=function(n){i.when(s(o.isMeta)).done(function(){ko.applyBindingsAndShow(o,n)})}}n.importReviews=function(n,t,i){new e(n,t).bindTo(i)}}(window.app,window.OData,window.jQuery,window.document,window.confirm,window.setTimeout),function(n,t,i){"use strict";function r(){var t=this;t.id=n.autoMap();t.name=n.autoMap();t.checked=ko.observable(!0)}function u(){var u=this;u.isFileUploaded=ko.observable(!1);u.metaReviewers=ko.observableArray();u.normalMetaReviewers=ko.observableArray();u.hasError=ko.observable(!1);u.errorText=ko.observable();u.uploading=ko.observable(!1);u.tracks=ko.observableArray();u.atLeastOneTrackSelected=ko.computed(function(){for(var t=!1,n=0;n<u.tracks().length;n++)t|=u.tracks()[n].checked();return t});u.loadTracks=function(){return t.read(n.odata.getUrl(n.odata.entitySet.tracks),function(t){for(var f,i=0;i<t.value.length;i++)f=n.autoMap(new r,t.value[i]),u.tracks.push(f)})};u.cancel=function(){window.location="/"+window.cmt3.conference.name+"/User/MetaReviewers"};u.getModel=function(){for(var t,e,i,r,f=[],n=0;n<u.normalMetaReviewers().length;n++)t=u.normalMetaReviewers()[n],e={FirstName:t.firstName,MiddleInitial:t.middleInitial,LastName:t.lastName,Organization:t.organization,Email:t.email},f.push(e);for(i=[],n=0;n<u.tracks().length;n++)r=u.tracks()[n],r.checked()&&i.push(r.id);return{Reviewers:f,Tracks:i,IsMeta:!0}};u.send=function(){if(u.atLeastOneTrackSelected()){var i=u.getModel(),r={requestUri:n.odata.getUrl(n.odata.entitySet.reviewers,null,"Import"),method:"POST",data:{Request:i}};t.request(r,function(){window.location="/"+window.cmt3.conference.name+"/User/MetaReviewers"})}};u.post=function(n,t,i){var r,f,u;i=i||"post";r=document.createElement("form");r.setAttribute("method",i);r.setAttribute("action",n);for(f in t)t.hasOwnProperty(f)&&(u=document.createElement("input"),u.setAttribute("type","hidden"),u.setAttribute("name",f),u.setAttribute("value",t[f]),r.appendChild(u));document.body.appendChild(r);r.submit();document.body.removeChild(r)};u.uploadFile=function(n,t){t.target.value!=""&&(u.uploading(!0),t.target.form.submit())};u.parseUploadResult=function(){var t=i.parseJSON(i("#singleFileUploadFrame").contents().text()),r,n,f;if(u.metaReviewers.removeAll(),u.normalMetaReviewers.removeAll(),u.hasError(t.HasError),u.errorText(t.ErrorText),!u.hasError())for(r=0;r<t.Models.length;r++)n=t.Models[r],f={organization:n.Organization,email:n.Email,firstName:n.FirstName,lastName:n.LastName,middleInitial:n.MiddleInitial,notice:n.Note,rawData:n.RawData,hasError:n.HasError},u.metaReviewers.push(f),f.hasError||u.normalMetaReviewers.push(f);u.isFileUploaded(!0);u.uploading(!1)};u.bindTo=function(n){u.loadTracks().done(function(){ko.applyBindingsAndShow(u,n)})}}n.importMetaReviewers=function(n){(new u).bindTo(n)}}(window.app,window.OData,window.jQuery,window.document,window.confirm,window.setTimeout),function(n,t,i){"use strict";function r(){var r=this;r.isFileUploaded=ko.observable(!1);r.hasError=ko.observable(!1);r.errorText=ko.observable();r.bids=ko.observableArray();r.normalBids=ko.observableArray();r.uploading=ko.observable(!1);r.cancel=function(){window.location="/"+window.cmt3.conference.name+"/Submission/Manage"};r.getModel=function(){for(var n,u,i=[],t=0;t<r.normalBids().length;t++)n=r.normalBids()[t],u={Email:n.email,SubmissionId:n.id,BidValue:n.bidValue},i.push(u);return{Bids:i}};r.send=function(){var i=r.getModel(),u={requestUri:n.odata.getUrl(n.odata.entitySet.metaBiddingModels,null,"Import"),method:"POST",data:{Request:i}};t.request(u,function(){window.location="/"+window.cmt3.conference.name+"/Submission/Manage"})};r.post=function(n,t,i){var r,f,u;i=i||"post";r=document.createElement("form");r.setAttribute("method",i);r.setAttribute("action",n);for(f in t)t.hasOwnProperty(f)&&(u=document.createElement("input"),u.setAttribute("type","hidden"),u.setAttribute("name",f),u.setAttribute("value",t[f]),r.appendChild(u));document.body.appendChild(r);r.submit();document.body.removeChild(r)};r.downloadTemplate=function(){var n="/api/odata/"+window.cmt3.conference.name+"/MetaBiddingModels/GetImportTemplate";r.post(n,{})};r.uploadFile=function(n,t){t.target.value!=""&&(r.uploading(!0),t.target.form.submit())};r.parseUploadResult=function(){var t=i.parseJSON(i("#singleFileUploadFrame").contents().text()),u,n,f;if(r.bids.removeAll(),r.normalBids.removeAll(),r.hasError(t.HasError),r.errorText(t.ErrorText),!r.hasError())for(u=0;u<t.Models.length;u++)n=t.Models[u],f={email:n.Email,id:n.Id,bid:n.Bid,bidValue:n.BidValue,status:n.Status,hasError:n.HasError,lineNumber:n.LineNumber},r.bids.push(f),f.hasError||r.normalBids.push(f);r.isFileUploaded(!0);r.uploading(!1)};r.bindTo=function(n){ko.applyBindingsAndShow(r,n)}}n.importMetaBids=function(n){(new r).bindTo(n)}}(window.app,window.OData,window.jQuery,window.document,window.confirm,window.setTimeout),function(n,t,i){"use strict";function r(n,t){var i=this;i.id=n.Id;i.title=n.Title;i.track=n.Track;i.referenceFiles=[];i.uploadReferenceUrl=function(){return t.referenceDetails.format(i.id)};i.uploadReferenceLinkVisible=function(){return!0};i.referenceLinkTitle=function(){return i.referenceFiles.length>0?"Update":"Upload"}}function u(){var n=this;n.id=t.autoMap();n.originalName=t.autoMap();n.size=t.autoMap();n.formattedSize=t.autoMap();n.uploadDate=t.autoMap();n.downloadLink=t.autoMap()}t.ReferencePage=function(t,i){var r=this;r.$element=n(t);r.conference=window.cmt3.conference.name;r.page=ko.observable(1);r.top=ko.observable(25);r.sort=ko.observable("Id");r.controller="ReferenceModels";r.filters=[];r._total=ko.observable(0);r.selected=ko.observable(0);r.referenceModels=ko.observableArray();r.listen();r.Pager=ko.pager(r.selected,r.top);r.Pager().CurrentPage.subscribe(function(){r.page(r.Pager().CurrentPage());r.show()});r.pageUrls=i;r.showWelcomeMessage=function(){n(document.getElementById("welcomeMessageDialog")).modal("show")}};t.ReferencePage.prototype={listen:function(){var t=this;n(document).on("data.filter",function(){t.Pager().CurrentPage()<2?t.show():t.Pager().CurrentPage(1)})},getFilter:function(){var t="";return n.each(this.filters,function(n,i){i.getValue()&&(t+=t==""?i.getValue():" and "+i.getValue())}),t},show:function(){var f=this;if(f.initialized){var e=f.sort(),o=f.top(),s=f.skip(),h=f.getFilter(),c=e?"&$orderby="+e:"",l=o?"&$top="+o:"",a=s?"&$skip="+s:"",v=h?"&$filter="+encodeURIComponent(h):"",y={headers:{Accept:"application/json"},requestUri:"/api/odata/"+this.conference+"/$batch",method:"POST",data:{requests:[{url:"/api/odata/"+this.conference+"/"+f.controller+"?$count=true"+c+v+a+l,method:"GET",headers:{Accept:"application/json"}}]}};i.request(y,function(i){t.page.saveState("referenceModels",{sort:e,top:o,skip:s,filter:h});var c=i.responses[0].body,l=c["@odata.count"],v=c.value,a=[];n.each(v,function(n,i){for(var o=new r(i,f.pageUrls),e=0;e<i.ReferenceFiles.length;e++)o.referenceFiles.push(t.autoMap(new u,i.ReferenceFiles[e]));a.push(o)});f.referenceModels(a);f._total()==0&&f._total(l);f.selected(l);n("html,body").scrollTop(0)},function(n){window.cmt3.logger.log(n.message)},i.batchHandler)}},scroll:function(){n(window).scrollTop()==n(document).height()-n(window).height()&&self.show()},post:function(n,t,i){var r,f,u;i=i||"post";r=document.createElement("form");r.setAttribute("method",i);r.setAttribute("action",n);for(f in t)t.hasOwnProperty(f)&&(u=document.createElement("input"),u.setAttribute("type","hidden"),u.setAttribute("name",f),u.setAttribute("value",t[f]),r.appendChild(u));document.body.appendChild(r);r.submit();document.body.removeChild(r)},stub:function(){alert("Sorry, this feature is not implemented yet.")},reset:function(){n.each(this.filters,function(n,t){t.reset()});this.show()},size:function(t,i){var r,u,f;n("a",".show").removeClass("btn-success").css("color","#999999");n(i.currentTarget).addClass("btn-success").css("color","white");r=n(i.target).attr("size");u=parseInt(r);this.top(u);f=this.Pager().CurrentPage();this.Pager().CurrentPage(1);f===1&&this.show()},skip:function(){return(this.page()-1)*this.top()},prev:function(){this.top()!=0&&this.page()!=1&&(this.page(this.page()-1),this.show())},next:function(){this.top()==0||this.page()>this.selected()/this.top()||(this.page(this.page()+1),this.show())},setSort:function(t,i){var r=n(i.target),u=r.attr("data-sort");(u==null||u==undefined)&&(r=n(r.context.parentNode),u=r.attr("data-sort"));r.hasClass("selected")?this.sort().match(" desc$")?(this.sort(u+" asc"),r.find("i").removeClass("icon-arrow-down"),r.find("i").addClass("icon-arrow-up")):(this.sort(u+" desc"),r.find("i").removeClass("icon-arrow-up"),r.find("i").addClass("icon-arrow-down")):(n("th[data-sort]").each(function(){n(this).find("i").removeClass("icon-arrow-up");n(this).find("i").removeClass("icon-arrow-down");n(this).removeClass("selected")}),r.find("i").removeClass("icon-arrow-down"),r.find("i").addClass("icon-arrow-up"),r.addClass("selected"),this.sort(u+" asc"));this.show()},refresh:function(){this.show()}}}(window.jQuery,window.app,window.OData),function(n,t,i,r){function f(t,r,u){function e(){var n=ko.validation.group(f);return n().length>0?(n.showAllMessages(),!1):!0}var f=this;f.parentViewModel=t;f.conflictViewModel=u;f.disputeReason=ko.observable(u.disputeReason).extend({required:!0});f.dispute=function(){if(e()){var u={requestUri:n.odata.getUrl(n.odata.entitySet.userDisputeConflicts),method:"POST",data:{SubmissionId:f.conflictViewModel.submissionId,DisputeReason:f.disputeReason()}};i.request(u,function(){$(r).modal("hide");t.refresh()},function(n){t.showODataError(n);t.refresh()})}};$(r).modal("show")}function s(t){var i=this;i.disputeId=t.DisputeId;i.submissionId=t.SubmissionId;i.submissionTitle=t.SubmissionTitle;i.submissionAuthors=t.SubmissionAuthors.split("\r\n");i.trackId=t.TrackId;i.trackName=t.TrackName;i.conflictReasons=t.ConflictReasons.split("\r\n");i.disputeStatus=ko.observable(t.DisputeStatus);i.disputeStatusText=ko.pureComputed(function(){return n.enums.disputedConflictStatus[i.disputeStatus()]||"Unknown"});i.disputeReason=t.DisputeReason}function h(t){var i=this;i.disputeId=t.DisputeId;i.submissionId=t.SubmissionId;i.submissionTitle=t.SubmissionTitle;i.submissionAuthors=t.SubmissionAuthors&&t.SubmissionAuthors.split("\r\n");i.trackId=t.TrackId;i.reviewerId=t.ReviewerId;i.reviewerName=t.ReviewerName;i.reviewerEmail=t.ReviewerEmail;i.reviewerOrganization=t.ReviewerOrganization;i.trackName=t.TrackName;i.conflictReasons=t.ConflictReasons&&t.ConflictReasons.split("\r\n");i.disputeStatus=ko.observable(t.DisputeStatus);i.disputeStatusText=ko.pureComputed(function(){return n.enums.disputedConflictStatus[i.disputeStatus()]||"Unknown"});i.disputeReason=t.DisputeReason}function u(n,i){var u=this,f;u.conference=r.name;u.savedState=u.loadState();u.submissionId=i;u.total=ko.observable(0);u.page=ko.observable(u.savedState.page);u.top=ko.observable(u.savedState.top);u.skip=ko.computed(function(){return(u.page()-1)*u.top()});u.pager=ko.pager(u.total,u.top);u.pager().CurrentPage.subscribe(function(){u.page(u.pager().CurrentPage());u.loadData()});u.conflicts=ko.observableArray();u.filters=[];u.sortableColumns={};u.sorting=ko.observable(u.savedState.sorting);$.each(u.sortableColumns,function(n,t){t.property()!==savedState.sorting.property?t.direction(null):t.direction(savedState.sorting.direction)});$(t).on("data.filter",function(){u.pager().CurrentPage()<2?u.loadData():u.pager().CurrentPage(1)});if(ko.applyBindingsAndShow(u,n),u.savedState&&u.savedState.sorting&&u.savedState.sorting.property&&u.sortableColumns&&u.sortableColumns[u.savedState.sorting.property])for(f in u.sortableColumns)u.sortableColumns[f].direction(f!==u.savedState.sorting.property?null:u.savedState.sorting.direction);$.each(u.savedState.filters,function(n,t){$.each(u.filters,function(n,i){i.field===t.property&&i.setValue(t.value)})});u.loadData()}function e(t,i,r){this.controller=n.odata.entitySet.chairDisputeConflicts;u.call(this,t,i);this.pageUrl=r}function o(t,i){this.controller=n.odata.entitySet.userDisputeConflicts;u.call(this,t);this.disputeDialogElementId=i}u.prototype={loadState:function(){var t=this,n={page:1,top:25,sorting:{property:"SubmissionId",direction:"asc"},filters:[]};return sessionStorage?JSON.parse(sessionStorage.getItem(t.controller))||n:n},saveState:function(){var n,t,i;sessionStorage&&(n=this,t=[],$.each(n.filters,function(n,i){var r=i.getValue();r&&t.push({property:i.field,value:r})}),i={page:n.page(),top:n.top(),sorting:n.sorting(),filters:t},sessionStorage.setItem(n.controller,JSON.stringify(i)))},size:function(n){this.top(n);this.loadData()},sort:function(n){this.sorting({property:n.property(),direction:n.direction()});this.loadData()},resetFilters:function(){$.each(this.filters,function(n,t){t.reset()});this.pager().CurrentPage()<2?this.loadData():this.pager().CurrentPage(1)},refresh:function(){this.loadData()},loadData:function(){var t=this,f=t.sorting(),o=f?"&$orderby="+encodeURIComponent(f.property+" "+f.direction):"",s=t.skip()?"&$skip="+t.skip():"",h=t.top()?"&$top="+t.top():"",u="",e;$.each(t.filters,function(n,t){t.getValue()&&(u+=u?" and "+t.getValue():t.getValue())});t.submissionId&&(u+=u?" and ":"",u+="(SubmissionId eq "+t.submissionId+")");u&&(u="&$filter="+encodeURIComponent(u));e={headers:{Accept:"application/json"},requestUri:"/api/odata/"+r.name+"/$batch",method:"POST",data:{requests:[{url:n.odata.getUrl(t.controller)+"?$count=true"+u+o+s+h,method:"GET",headers:{Accept:"application/json"}}]}};i.request(e,function(n){for(var r=n.responses[0].body,e=r["@odata.count"],u=r.value,f=[],i=0;i<u.length;i++)f.push(t.getConflictViewModel(u[i]));t.conflicts(f);t.total(e);t.saveState()},function(n){t.showODataError(n)},OData.batchHandler)},showODataError:function(t){var i,r;t&&t.response&&t.response.body&&(i=$.parseJSON(t.response.body),i&&i.error&&i.error.message)&&(r=i.error.message,n.addMessage(r,null,"error"))}};e.prototype=$.extend({},u.prototype,{getConflictViewModel:function(n){return new h(n)},changeStatus:function(t){var r=this,u;(t.disputeStatus()==="Kept"||t.disputeStatus()==="Deleted")&&(u={requestUri:n.odata.getUrl(n.odata.entitySet.chairDisputeConflicts,t.disputeId),method:"PATCH",data:{DisputeStatus:t.disputeStatus()}},i.request(u,function(){},function(n){r.showODataError(n);r.refresh()}))},emailReviewer:function(t){var i=this,r="Id eq {0}".format(t.reviewerId),u="/"+i.conference+"/User/SendEmail/";n.url.navigateTo(u,{filter:r,returnTo:i.pageUrl})},emailAuthors:function(t){var i=this,r="Id eq {0}".format(t.submissionId),u="/"+i.conference+"/Submission/SendEmail/2";n.url.navigateTo(u,{filter:r,returnTo:i.pageUrl})}});o.prototype=$.extend({},u.prototype,{getConflictViewModel:function(n){return new s(n)},dispute:function(n){var i=t.getElementById(this.disputeDialogElementId);this.disputeDialog?this.disputeDialog(new f(this,i,n)):(this.disputeDialog=ko.observable(new f(this,i,n)),ko.applyBindings(this.disputeDialog,i))},withdraw:function(t){var r=this,u={requestUri:n.odata.getUrl(n.odata.entitySet.userDisputeConflicts,t.disputeId),method:"DELETE"};i.request(u,function(){r.refresh()},function(n){r.showODataError(n);r.refresh()})}});n.userDisputeConflictsPage=function(n,t){new o(n,t)};n.chairManageDisputedConflictsPage=function(n,t,i){new e(n,t,i)}}(window.app,window.document,window.OData,window.cmt3.conference),function(n,t,i){function r(r,u){function e(){var t={requestUri:n.odata.getUrl(n.odata.entitySet.conflictDomains,u),method:"GET"};i.request(t,function(n){f.conflictDomains(n.DomainNames)},i.defaultError)}var f=this;f.conflictDomains=ko.observable();f.save=function(){var t={requestUri:n.odata.getUrl(n.odata.entitySet.conflictDomains),method:"POST",data:{UserId:u,DomainNames:f.conflictDomains()}};i.request(t,function(){n.addMessage("Domain conflicts saved.",null,"success","text",!0);window.location.reload()},i.defaultError)};e();ko.applyBindings(f,t.getElementById(r))}n.conflictDomainsPage=function(n,t){new r(n,t)}}(window.app,window.document,window.OData),function(n,t,i){"use strict";function u(t){function u(){f();r=i.isConflicting.subscribe(e)}function f(){r&&typeof r.dispose=="function"&&r.dispose()}function e(){i.initialState===undefined?i.initialState=i.isConflicting():o.call(i)}function o(){var r=this,e;r.isToggleInProgress(!0);e={UserId:r.id};e.Type=r.isConflicting()?"Add":"Remove";OData.request({requestUri:n.odata.getUrl(n.odata.entitySet.individualConflictViews,t,"Modify"),method:"POST",showProgressIndicator:!1,data:{Request:e}},function(){r.isConflicting()===r.initialState?i.css(""):i.css(r.isConflicting()?"success":"error")},function(t){f();i.isConflicting(!i.isConflicting());u();n.addErrorMessage("Unable to mark conflict with '"+r.firstName+" "+r.lastName+"'. "+n.odata.getErrorMessage(t))}).always(function(){r.isToggleInProgress(!1)})}var i=this,r;i.id=n.autoMap();i.name=n.autoMap();i.firstName=n.autoMap();i.lastName=n.autoMap();i.organization=n.autoMap();i.isConflicting=ko.observable().autoMap();i.initialState=undefined;i.css=ko.observable("");i.isToggleInProgress=ko.observable(!1);u()}function r(t){var i=this;i.userId=t;i.users=ko.observableArray([]);n.DataTable.call(i)}function f(t,u){var f=this;n.showProgress();f.table=new r(t);ko.applyBindings(f,i.getElementById(u));$.when(f.table.loadData(!0)).then(function(){$("#"+u).show()}).always(n.hideProgress)}r.prototype=$.extend({},n.DataTable.prototype,{getStorageKey:function(){return"IndividualConflicts"},getDefaultSorting:function(){return{property:"IsConflicting",direction:"desc"}},loadData:function(i){var r,o,s;i=i===!0;r=this;i&&r.applyState();var e=r.sorting(),h=e?"&$orderby="+encodeURIComponent(e.property+" "+e.direction):"",c=r.skip()?"&$skip="+r.skip():"",l=r.top()?"&$top="+r.top():"",f="";return $.each(r.filters,function(n,t){t.getValue()&&(f+=f?" and "+t.getValue():t.getValue())}),f&&(f="&$filter="+encodeURIComponent(f)),o={method:"GET",headers:{Accept:"application/json"},requestUri:n.odata.getUrl(n.odata.entitySet.individualConflictViews,r.userId)+"?$count=true"+f+h+c+l,showProgressIndicator:!i},s=t.request(o,function(t){var f,i,e,o;for(r.total(t["@odata.count"]||0),f=[],i=0;i<t.value.length;i++)e=t.value[i],o=n.autoMap(new u(r.userId),e),f.push(o);r.users(f);r.saveState()},function(t){n.addErrorMessage(n.odata.getErrorMessage(t))}),s}});n.individualConflicts=function(n,t){new f(n,t)}}(window.app,window.OData,window.document),function(n,t,i){function r(n){var t=this;t.id=n.Id;t.firstName=n.FirstName;t.lastName=n.LastName;t.email=n.Email;t.organization=n.Organization}function u(u,f,e,o,s,h){function a(n){var t=this;t.firstName=ko.observable().extend({required:{message:"First Name is required."},maxLength:200});t.lastName=ko.observable().extend({required:{message:"Last Name is required."},maxLength:200});t.organization=ko.observable().extend({required:{message:"Organization is required."},maxLength:200});t.email=ko.observable().extend({email:!0,required:{message:"Email is required."},maxLength:200,validation:{validator:function(n,t){for(var i=0;i<t.length;i++)if(t[i].email===n)return!1;return!0},message:"Author with the same email already exists.",params:n}});t.cancelAdd=function(){t.firstName("");t.firstName.isModified(!1);t.lastName("");t.lastName.isModified(!1);t.organization("");t.organization.isModified(!1);t.email("");t.email.isModified(!1)}}function v(){var t={requestUri:n.odata.getUrl(n.odata.entitySet.conflictDomains,f),method:"GET"};i.request(t,function(n){n.DomainNames&&c.conflictDomains(n.DomainNames)},i.defaultError)}function y(){var t=n.odata.getUrl(n.odata.entitySet.individualConflictViews,null,"GetConflictingUsersOnly");i.read({requestUri:t,showProgressIndicator:!1,data:{Id:f},method:"POST"},function(n){for(var u,t=[],i=0;i<n.value.length;i++)u=new r(n.value[i]),t.push(u);t.sort(function(n,t){return n.firstName.toLowerCase().localeCompare(t.firstName.toLowerCase())});c.conflictingUsers(t);c.conflictingUsers.valueHasMutated()},i.defaultError)}var c=this,l;c.allowEditConflictDomains=e;c.allowEditIndividualConflicts=o;c.oneChanceToEditConflicts=s;c.conflictDomains=ko.observable().extend({required:!0,maxLength:1e3}).autoMap();c.conflictingUsers=ko.observableArray();c.nonCMTConflictingUsers=ko.observableArray();l=h?$.parseJSON(h):[];c.nonCMTConflictingUsers(l);c.to=ko.observable(null).extend({required:{onlyIf:function(){return c.validationEnabled&&c.answer()!==""}},email:!0,maxLength:200});c.showValidationWarning=ko.observable(!1);c.isSearching=ko.observable();c.searched=ko.observable(!1);c.userFound=ko.observable(!1);c.userNotFound=ko.observable(!1);c.newNonCMTConflictUser=new a(c.nonCMTConflictingUsers);c.search=function(){var t=ko.validation.group([c.to]),i;if(t().length>0){t.showAllMessages();return}c.isSearching(!0);i={requestUri:n.odata.getGlobalUrl(n.odata.entitySet.users,null,"SearchByEmail"),method:"POST",showProgressIndicator:!1,data:{Email:c.to()}};OData.read(i,function(n){var i=new r(n),t=c.conflictingUsers();t.push(i);t.sort(function(n,t){return n.firstName.toLowerCase().localeCompare(t.firstName.toLowerCase())});c.conflictingUsers(t);c.conflictingUsers.valueHasMutated();c.userNotFound(!1);c.isSearching(!1);c.to(null)},function(n){c.isSearching(!1);n.response.statusCode===404?c.userNotFound(!0):OData.defaultError(n)})};c.removeConflictUser=function(n){var t=this,i=t.conflictingUsers();i.splice(n,1);t.conflictingUsers.valueHasMutated()};c.addNonCMTConflictUser=function(n){var i=ko.validation.group([n.firstName,n.lastName,n.email,n.organization]);if(i().length>0){i.showAllMessages();return}var u={FirstName:n.firstName(),LastName:n.lastName(),Email:n.email(),Organization:n.organization()},f=new r(u),t=c.nonCMTConflictingUsers();t.push(f);t.sort(function(n,t){return n.firstName.toLowerCase().localeCompare(t.firstName.toLowerCase())});c.nonCMTConflictingUsers(t);c.nonCMTConflictingUsers.valueHasMutated();n.cancelAdd()};c.removeNonCMTConflictUser=function(n){var t=this,i=t.nonCMTConflictingUsers();i.splice(n,1);t.nonCMTConflictingUsers.valueHasMutated()};c.confirmSave=function(){var n=!0,i=ko.validation.group(c,{deep:!1}),r;if(i().length>0&&(i.showAllMessages(),n=!1),!n){c.showValidationWarning(!0);return}c.showValidationWarning(!1);r=t.getElementById("saveConflictsDialog");$(r).modal("show")};c.save=function(){var e=!0,o=ko.validation.group(c,{deep:!1}),t,u,r,s;if(o().length>0&&(o.showAllMessages(),e=!1),!e){c.showValidationWarning(!0);return}if(c.showValidationWarning(!1),c.allowEditConflictDomains){if(t=null,c.allowEditIndividualConflicts){for(u=[],r=0;r<c.conflictingUsers().length;r++)u.push(c.conflictingUsers()[r].id);s={UserIds:u,WriteInConflicts:ko.toJSON(c.nonCMTConflictingUsers()),DomainNames:c.conflictDomains()};t={requestUri:n.odata.getUrl(n.odata.entitySet.individualConflictViews,f,"BulkAddIndividualConflict"),method:"POST",showProgressIndicator:!1,data:{Request:s}}}else t={requestUri:n.odata.getUrl(n.odata.entitySet.conflictDomains),method:"POST",data:{UserId:f,DomainNames:c.conflictDomains()}};i.request(t,function(){n.addMessage("Personal conflicts saved.",null,"success","text",!0);window.location.reload()},i.defaultError)}};$.when(v(),y()).done(function(){ko.applyBindings(c,t.getElementById(u))})}n.personalConflictsPage=function(n,t,i,r,f,e,o){new u(n,t,i,r,f,e,o)}}(window.app,window.document,window.OData),function(n,t,i,r){function u(){var n=this;n.Id=t.autoMap();n.Title=t.autoMap();n.Authors=t.autoMap();n.TrackId=t.autoMap();n.Track=t.autoMap();n.Status=t.autoMap();n.IsCameraReadyPosted=t.autoMap();n.NumberOfCameraReadyFiles=t.autoMap();n.CameraReadyFileUploadDate=t.autoMap();n.IsCopyrightFormPosted=t.autoMap();n.LastCameraReadyFileUploadDateFormatted=function(){return t.formatUndefinableDateTime(n.CameraReadyFileUploadDate)}}function f(f,e){function c(){var n={page:1,top:25,sorting:{property:"Id",direction:"asc"},filters:[]};return sessionStorage?JSON.parse(sessionStorage.getItem(o.controller))||n:n}function l(){var t,i;sessionStorage&&(t=[],n.each(o.filters,function(n,i){var r=i.getValue();r&&t.push({property:i.field,value:r})}),i={page:o.page(),top:o.top(),sorting:o.sorting(),filters:t},sessionStorage.setItem(o.controller,JSON.stringify(i)))}function s(){var r=o.sorting(),e=r?"&$orderby="+encodeURIComponent(r.property+" "+r.direction):"",s=o.skip()?"&$skip="+o.skip():"",h=o.top()?"&$top="+o.top():"",n=o.getFilterString(),f;n&&(n="&$filter="+encodeURIComponent(n));f={headers:{Accept:"application/json"},requestUri:"/api/odata/"+o.conference+"/$batch",method:"POST",data:{requests:[{url:t.odata.getUrl(t.odata.entitySet.proceedingEditorModels)+"?$count=true"+n+e+s+h,method:"GET",headers:{Accept:"application/json"}}]}};i.request(f,function(n){for(var r=n.responses[0].body,s=r["@odata.count"],f=r.value,e=[],i=0;i<f.length;i++)e.push(t.autoMap(new u,f[i]));o.submissions(e);o.total(s);l()},function(n){a(n)},OData.batchHandler)}function a(i){var r,u;i&&i.response&&i.response.body&&(r=n.parseJSON(i.response.body),r&&r.error&&r.error.message)&&(u=r.error.message,t.addMessage(u,null,"error"))}var o=this,h;o.tracks=e;o.conference=r.name;o.controller=t.odata.entitySet.proceedingEditorModels;o.savedState=c();o.total=ko.observable(0);o.page=ko.observable(o.savedState.page);o.top=ko.observable(o.savedState.top);o.skip=ko.computed(function(){return(o.page()-1)*o.top()});o.pager=ko.pager(o.total,o.top);o.pager().CurrentPage.subscribe(function(){o.page(o.pager().CurrentPage());s()});o.submissions=ko.observableArray();o.filters=[];o.sortableColumns={};o.sorting=ko.observable(o.savedState.sorting);n.each(o.sortableColumns,function(n,t){t.property()!==savedState.sorting.property?t.direction(null):t.direction(savedState.sorting.direction)});n(document).on("data.filter",function(){o.pager().CurrentPage()<2?s():o.pager().CurrentPage(1)});if(o.sort=function(n){o.sorting({property:n.property(),direction:n.direction()});s()},o.getFilterString=function(){var t="";return n.each(o.filters,function(n,i){i.getValue()&&(t+=t?" and "+i.getValue():i.getValue())}),t},o.resetFilters=function(){n.each(o.filters,function(n,t){t.reset()});o.pager().CurrentPage()<2?s():o.pager().CurrentPage(1)},o.refresh=function(){s()},o.size=function(n){o.top(n);s()},o.email=function(i,r){var u=r.target,c=ko.contextFor(u),e=parseInt(n(u).attr("sid")),h=n(u).attr("recipientType"),f,s;f=e?"Id eq {0}".format(e):o.getFilterString();s="/"+o.conference+"/Submission/SendEmail/"+h;t.url.navigateTo(s,{filter:f.length>0?f:null})},o.downloadFiles=function(i,r){var u=r.target,f=n(u).attr("href"),e=o.getFilterString(),s={requestUri:t.odata.getUrl(t.odata.entitySet.proceedingEditorModels,null,"GetIds"),method:"POST",showProgressIndicator:!0,data:{filter:e}};OData.request(s,function(n){var i=n.value.join("/"),r={Ids:i};t.page.post(f,r)});r.preventDefault()},o.exportCameraReadySubmissions=function(i,r){var u=r.target,c=ko.contextFor(u),f=parseInt(n(u).attr("sid")),e,s,h;e=f?"Id eq {0}".format(f):o.getFilterString();s="/api/odata/"+window.cmt3.conference.name+"/CameraReadySubmissionViews/Export";h={Filter:e};t.page.post(s,h)},ko.applyBindingsAndShow(o,f),o.savedState&&o.savedState.sorting&&o.savedState.sorting.property&&o.sortableColumns&&o.sortableColumns[o.savedState.sorting.property])for(h in o.sortableColumns)o.sortableColumns[h].direction(h!==o.savedState.sorting.property?null:o.savedState.sorting.direction);n.each(o.savedState.filters,function(t,i){n.each(o.filters,function(n,t){t.field===i.property&&t.setValue(i.value)})});s()}t.proceedingEditorList=function(n,t){new f(n,t)}}(window.jQuery,window.app,window.OData,window.cmt3.conference),function(n,t,i,r){function u(u,f){var e=this;e.userName=ko.observable("");e.password=ko.observable("");e.save=function(){var o={requestUri:t.odata.getUrl(t.odata.entitySet.tpmsSettings,null,"UpdateTpmsAuthentication"),method:"POST",data:{Request:{UserName:e.userName(),Password:e.password()}}};i.request(o,function(i){i.value===!0?(f&&typeof f=="function"&&f(!0),n(r.getElementById(u)).modal("hide")):t.addMessage("Unable to authenticate!",null,"error")})}}function f(f,e){function s(){var r=n.Deferred(),u={requestUri:t.odata.getUrl(t.odata.entitySet.tpmsSettings,null,"VerifyTpmsAuthentication"),method:"POST"};return i.request(u,function(n){r.resolve(n.value)},function(){r.reject()}),r.promise()}function h(n){i.read(t.odata.getUrl(t.odata.entitySet.tpmsSettings,f),function(i){t.autoMap(o,i);n()})}var o=this;o.isEnabled=ko.observable().autoMap();o.depositAuthor=ko.observable().autoMap();o.isEnsuringAuthentication=ko.observable().autoMap();o.showAdditionalFields=ko.pureComputed(function(){return o.isEnabled()&&!o.isEnsuringAuthentication()});o.isEnabled.subscribe(function(t){t&&(o.isEnsuringAuthentication(!0),s().done(function(t){if(!t){var i=r.getElementById(e);o.tpmsAuthenticationFormViewModel==null&&(o.tpmsAuthenticationFormViewModel=new u(e,function(n){n&&o.isEnabled(!0)}),ko.applyBindings(o.tpmsAuthenticationFormViewModel,i));n(i).modal("show");o.isEnabled(!1)}}).fail(function(){o.isEnabled(!1)}).always(function(){o.isEnsuringAuthentication(!1)}))});o.save=function(){var n={requestUri:t.odata.getUrl(t.odata.entitySet.tpmsSettings,f),method:"PATCH",data:{IsEnabled:o.isEnabled(),DepositAuthor:o.depositAuthor()}};return i.request(n,function(){t.addMessage("TPMS settings have been saved!")}),!1};o.bindTo=function(t){function i(){ko.applyBindingsAndShow(o,t);n("#menuSiteFeatures").addClass("in")}h(i)}}t.settingsTpmsPage=function(n,t,i){new f(n,i).bindTo(t)}}(window.jQuery,window.app,window.OData,window.document),function(n,t){function i(n){var t=this;t.successCount=ko.observable(null).autoMap();t.errorCount=ko.observable(null).autoMap();t.failedSubmissionIds=ko.observableArray(n);t.failedSubmissionIdsText=ko.pureComputed(function(){var n=t.failedSubmissionIds();return n&&n.join(", ")});t.totalCount=ko.observable(null).autoMap();t.finishedAt=ko.observable(null).autoMap();t.processedCount=ko.pureComputed(function(){return t.errorCount()+t.successCount()});t.percentage=ko.pureComputed(function(){var n=t.totalCount(),i=t.processedCount();return!n||i===null?null:Math.round(i/n*100)})}function r(){function e(){var u={requestUri:n.odata.getUrl(n.odata.entitySet.tpmsSubmissions,null,"GetProgress"),showProgressIndicator:!1,method:"POST"};return OData.request(u,function(t){r.progress(n.autoMap(new i(t.FailedSubmissionIds),t))},function(i){if((i&&i.response&&i.response.statusCode)===n.enums.httpStatusCodes.failure.notFound){r.progress(null);return}t.defaultError(i)})}function u(){e().done(function(){var n=r.progress()&&r.progress().finishedAt();f=n?null:setTimeout(u,1e3)})}var f,r=this;r.progress=ko.observable(null);r.visible=ko.pureComputed(function(){return r.progress()!=null});r.done=function(){var t={requestUri:n.odata.getUrl(n.odata.entitySet.tpmsSubmissions,null,"ClearProgress"),showProgressIndicator:!1,method:"POST"};OData.request(t,function(){r.progress(null)})};r.refresh=function(){u()};u()}function u(){var t=this;t.trackId=n.autoMap();t.trackName=n.autoMap();t.numberOfSubmissions=ko.observable(0).autoMap();t.checked=ko.observable(!1);t.isDisabled=ko.computed(function(){return t.numberOfSubmissions()<1})}function f(t){var i=this;i.submissionId=ko.observable().extend({required:!0,pattern:"^[0-9]+$"});i.progressViewModel=t;i.isSubmitDisabled=ko.pureComputed(function(){return!i.submissionId.isValid()});i.submit=function(){if(i.submissionId.isValid()){var t={requestUri:n.odata.getUrl(n.odata.entitySet.tpmsSubmissions,i.submissionId(),"SendSubmissionToTpms"),method:"POST"};return OData.request(t,function(){i.progressViewModel.refresh()})}}}function e(t){function r(){var n=i.tracks(),r=[],t;if(n.length===1&&!n[0].isDisabled())return r.push(n[0].trackId),r;for(t=0;t<n.length;t++)n[t].checked()&&!n[t].isDisabled()&&r.push(n[t].trackId);return r}function f(){var t={requestUri:n.odata.getUrl(n.odata.entitySet.tpmsSubmissions,null,"GetTpmsTracksInfo"),method:"POST"};return OData.request(t,function(t){for(var e,r=[],f=0;f<t.value.length;f++)e=n.autoMap(new u,t.value[f]),r.push(e);r.sort(function(n,t){return n.trackId<t.trackId?-1:n.trackId>t.trackId?1:0});i.tracks(r)})}var i=this;i.progressViewModel=t;i.isSingleTrackConference=ko.observable(!1);i.tracks=ko.observableArray([]);i.selectedCount=ko.computed(function(){return r().length});i.isSubmitDisabled=ko.computed(function(){return i.selectedCount()<1});i.isSingleTrackConference=ko.pureComputed(function(){return i.tracks().length<2});i.toggleAllChecked=ko.pureComputed({read:function(){for(var t=i.tracks(),n=0;n<t.length;n++)if(!t[n].checked()&&!t[n].isDisabled())return!1;return!0},write:function(){for(var r=!i.toggleAllChecked(),t=i.tracks(),n=0;n<t.length;n++)t[n].isDisabled()!==!0&&t[n].checked(r);return!1}});i.submit=function(){var t={requestUri:n.odata.getUrl(n.odata.entitySet.tpmsSubmissions,null,"SendSubmissionsToTpms"),method:"POST",data:{Request:{TrackIds:r()}}};return OData.request(t,function(){i.progressViewModel.refresh()})};f()}function o(){var n=this;n.progress=new r;n.submissions=new e(n.progress);n.submission=new f(n.progress);n.submissionsVisible=ko.pureComputed(function(){return!n.progress.visible()})}n.tpmsSubmissions=function(n){ko.applyBindings(new o,document.getElementById(n))}}(window.app,window.OData),function(n){function t(){var t=this;t.trackId=n.autoMap();t.trackName=n.autoMap();t.numberOfReviewers=n.autoMap();t.numberOfMetaReviewers=n.autoMap();t.numberOfSeniorMetaReviewers=n.autoMap();t.isReviewersChecked=ko.observable(!1);t.isMetaReviewersChecked=ko.observable(!1);t.isSeniorMetaReviewersChecked=ko.observable(!1);t.isReviewersDisabled=ko.pureComputed(function(){return t.numberOfReviewers<1});t.isMetaReviewersDisabled=ko.pureComputed(function(){return t.numberOfMetaReviewers<1});t.isSeniorMetaReviewersDisabled=ko.pureComputed(function(){return t.numberOfSeniorMetaReviewers<1})}function i(i){function u(){var i={requestUri:n.odata.getUrl(n.odata.entitySet.tpmsMatchingRequests,null,"GetTpmsReviewersTrackInfo"),method:"POST"};return OData.request(i,function(i){for(var e,u=[],f=0;f<i.value.length;f++)e=n.autoMap(new t,i.value[f]),u.push(e);u.sort(function(n,t){return n.trackId<t.trackId?-1:n.trackId>t.trackId?1:0});r.tracks(u)})}var r=this;r.tracks=ko.observableArray([]);r.isSingleTrackConference=ko.pureComputed(function(){return r.tracks().length<2});r.selectedTracksData=ko.pureComputed(function(){for(var n,i=r.tracks(),u=[],t=0;t<i.length;t++)n=i[t],(!n.isReviewersDisabled()&&n.isReviewersChecked()||!n.isMetaReviewersDisabled()&&n.isMetaReviewersChecked()||!n.isSeniorMetaReviewersDisabled()&&n.isSeniorMetaReviewersChecked())&&u.push({TrackId:n.trackId,IsReviewersChecked:n.isReviewersChecked(),IsMetaReviewersChecked:n.isMetaReviewersChecked(),IsSeniorMetaReviewersChecked:n.isSeniorMetaReviewersChecked()});return u});r.isSubmitDisabled=ko.pureComputed(function(){return r.selectedTracksData().length<1});r.submit=function(){for(var e,o,u=r.selectedTracksData(),f=[],t=0;t<u.length;t++)e=u[t],o={requestUri:n.odata.getUrl(n.odata.entitySet.tpmsMatchingRequests),method:"POST",data:e},f.push(OData.request(o,function(){}));$.when.apply($,f).then(function(){n.url.navigateTo(i,"requestSent")})};u()}n.tpmsSendMatchingRequest=function(n,t){ko.applyBindingsAndShow(new i(t),n)}}(window.app),function(n,t){function i(i){function u(n){return n?"Yes":"No"}$parent=i;var r=this;r.created=n.autoMap();r.id=n.autoMap();r.trackId=n.autoMap();r.isReviewersChecked=n.autoMap();r.isMetaReviewersChecked=n.autoMap();r.isSeniorMetaReviewersChecked=n.autoMap();r.isResultRetrieved=n.autoMap();r.isRetrievingResult=n.autoMap();r.lastRequestStatus=n.autoMap();r.track=ko.pureComputed(function(){return i.dictTrack[r.trackId]});r.statusMessage=ko.pureComputed(function(){if(r.isResultRetrieved)return"";switch(r.lastRequestStatus){case"Pending":return"TPMS result is not ready yet, please try again later.";case"Error":return"Error, please try again later or contact CMT support."}return""});r.createdFormatted=ko.pureComputed(function(){return n.formatUndefinableDateTime(r.created)});r.isReviewersCheckedText=ko.pureComputed(function(){return u(r.isReviewersChecked)});r.isMetaReviewersCheckedText=ko.pureComputed(function(){return u(r.isMetaReviewersChecked)});r.isSeniorMetaReviewersCheckedText=ko.pureComputed(function(){return u(r.isSeniorMetaReviewersChecked)});r.getScores=function(){var i={showProgressIndicator:!1,headers:{Accept:"application/json"},requestUri:n.odata.getUrl(n.odata.entitySet.tpmsMatchingRequests,r.id,"RetrieveScores"),method:"POST"};n.showProgress();t.request(i,function(t,i){i.statusCode===n.enums.httpStatusCodes.success.ok&&$parent.reload(!1);i.statusCode===n.enums.httpStatusCodes.success.noContent&&n.addMessage("TPMS result is not ready yet, please try again later.","","warning")}).always(n.hideProgress)}}function r(r){function f(r){var f={showProgressIndicator:r!==!1,headers:{Accept:"application/json"},requestUri:n.odata.getUrl("$batch"),method:"POST",data:{requests:[{url:n.odata.getUrl(n.odata.entitySet.tpmsMatchingRequests),method:"GET",headers:{Accept:"application/json"}}]}};return t.request(f,function(t){for(var o,s=t.responses[0].body,f=s.value,e=[],r=0;r<f.length;r++)o=n.autoMap(new i(u),f[r]),e.push(o);u.requests(e)},function(n){window.cmt3.logger.log(n.message)},t.batchHandler)}var u=this;u.dictTrack=r.reduce(function(n,t){return n[t.Id]=t.Name,n},{});u.requests=ko.observableArray([]);u.reload=function(n){return f(n)};n.url.hash.getValue()==="requestSent"&&(n.url.hash.remove(),n.addMessage("Request has been submitted to TPMS, please allow some time for the request to be processed."));f();setInterval(function(){f(!1)},6e4)}n.tpmsManageMatchingRequests=function(n,t){ko.applyBindings(new r(t),document.getElementById(n))}}(window.app,window.OData),function(n,t){function i(){var t=this;t.id=n.autoMap();t.name=n.autoMap();t.isChecked=ko.observable(!1)}function r(r){function e(n,i){var r=t.createElement("form"),f,u;if(r.setAttribute("method","post"),r.setAttribute("action",n),i)for(f=0;f<i.length;f++)u=t.createElement("input"),u.setAttribute("type","hidden"),u.setAttribute("name","tracks"),u.setAttribute("value",i[f]),r.appendChild(u);t.body.appendChild(r);r.submit();t.body.removeChild(r)}var u=this,f;for(u.type=ko.observable("reviewer"),u.tracks=[],f=0;f<r.length;f++)u.tracks.push(n.autoMap(new i,r[f]));u.tracks.length==1&&u.tracks[0].isChecked(!0);u.isDownloadButtonEnabled=ko.pureComputed(function(){if(!u.tracks||u.tracks.length<2)return!0;for(var n=0;n<u.tracks.length;n++)if(u.tracks[n].isChecked&&u.tracks[n].isChecked())return!0;return!1});u.download=function(){for(var i=[],t=0;t<u.tracks.length;t++)u.tracks[t].isChecked()&&i.push(u.tracks[t].id);e(n.odata.getUrl(n.odata.entitySet.tpmsScores,null,u.type()==="seniorMetaReviewer"?"DownloadSeniorMetaReviewerScores":u.type()==="metaReviewer"?"DownloadMetaReviewerScores":"DownloadReviewerScores"),i)}}n.tpmsDownloadScoresPage=function(n,i){ko.applyBindings(new r(i),t.getElementById(n))}}(window.app,window.document),function(n,t){"use strict";function i(){var i=this;i.id=n.autoMap();i.submissionId=n.autoMap();i.name=n.autoMap();i.track=n.autoMap();i.description=n.autoMap();i.presenters=n.autoMap();i.durationInMinutes=ko.observable().extend({required:!1,number:!0}).autoMap();i.sessionId=ko.observable().autoMap();i.session=n.autoMap();i.isAssigned=n.autoMap();i.isAssignedText=ko.pureComputed(function(){return i.isAssigned.toYesNo()});i.save=function(){var r=i.id,u={method:"PATCH",requestUri:n.odata.getUrl(n.odata.entitySet.presentations,r?r:null),showProgressIndicator:!1,data:{SessionId:$.isNumeric(i.sessionId())?i.sessionId():null,DurationInMinutes:$.isNumeric(i.durationInMinutes())?i.durationInMinutes():null}};return t.request(u)}}function r(){var t=this;t.presentations=ko.observableArray([]);n.DataTable.call(t)}function u(r,u){function o(){var t=this;t.id=n.autoMap();t.name=n.autoMap()}function s(){var i={method:"GET",headers:{Accept:"application/json"},requestUri:n.odata.getUrl(n.odata.entitySet.sessions)+"?$select=Id,Name"};return t.request(i).done(function(t){var r,u,i,e,s;if(t.value){for(r=t.value,u=[],i=0;i<r.length;i++)e=r[i],s=n.autoMap(new o,e),u.push(s);f.sessions(u)}})}var f=this,e;f.presentation=ko.observable();f.sessions=ko.observableArray();e=$(document.getElementById(r));f.edit=function(t){var r=f.sessions(),u=!r||r.length===0?s():$.Deferred().resolve().promise();u.done(function(){t=t&&t.constructor===i?n.autoMap(new i,t):new i(f);f.presentation(t);e.modal("show")})};f.save=function(){var t=f.presentation();t&&typeof t.save=="function"&&(n.showProgress(),$.when(t.save()).then(function(){return e.modal("hide"),u.loadData(!1,!0)}).always(n.hideProgress))}}function f(i){var f=this;f.table=new r;f.editDialog=new u(i,f.table);f.table.loadData();f.exportSessionPresentations=function(t,i){var r=f.table.getFilterForURIComponent(),u={method:"GET",headers:{Accept:"application/json"},requestUri:n.odata.getUrl(n.odata.entitySet.presentations)+"?$count=true&$select=Id"+r,showProgressIndicator:!0};OData.request(u,function(t){for(var f,e,o,r=t.value,u=[],i=0;i<r.length;i++)f=r[i],u.push(f.Id);e={PresentationIds:u.join(",")};o=n.odata.getUrl(n.odata.entitySet.presentations,null,"ExportPresentationSessions");n.page.post(o,e)});i.preventDefault()};f.bulkUnassignFromSession=function(){if(confirm("Bulk unassigning will be performed for selected presentations.")){var i=f.table.getFilterString(),r={requestUri:n.odata.getUrl(n.odata.entitySet.presentations,null,"BulkUnassignFromSession"),method:"POST",showProgressIndicator:!0,data:{Filter:i}};t.request(r,function(){n.addMessage("Bulk unassigning has been completed successfully.",null,"success","text",!0);location.reload()})}};f.bulkAutoAssign=function(){if(confirm("Automatic assignment will be performed for selected presentations.")){var i=f.table.getFilterString(),r={requestUri:n.odata.getUrl(n.odata.entitySet.presentations,null,"BulkAutoAssign"),method:"POST",showProgressIndicator:!0,data:{Filter:i}};t.request(r,function(t){t.value?n.addMessage("Automatic assignment has been completed successfully.",null,"success","text",!0):n.addMessage("Automatic assignment could not be completed.",null,"error","text",!0);location.reload()})}}}r.prototype=$.extend({},n.DataTable.prototype,{getDefaultSorting:function(){return{property:"Id",direction:"asc"}},getFilterString:function(){var t=this,n="";return $.each(t.filters,function(t,i){i.getValue()&&(n+=n?" and "+i.getValue():i.getValue())}),n},getFilterForURIComponent:function(){var t=this,n=t.getFilterString();return n&&(n="&$filter="+encodeURIComponent(n)),n},loadData:function(r){var u;r=r===!0;u=this;r&&u.applyState();var f=u.sorting(),e=f?"&$orderby="+encodeURIComponent(f.property+" "+f.direction):"",o=u.skip()?"&$skip="+u.skip():"",s=u.top()?"&$top="+u.top():"",h=u.getFilterForURIComponent(),c={method:"GET",headers:{Accept:"application/json"},requestUri:n.odata.getUrl(n.odata.entitySet.presentations)+"?$count=true"+h+e+o+s,showProgressIndicator:!r};return t.request(c,function(t){var f,r,e,o;for(u.total(t["@odata.count"]||0),f=[],r=0;r<t.value.length;r++)e=t.value[r],o=n.autoMap(new i,e),f.push(o);u.presentations(f);u.saveState()},function(t){n.addErrorMessage(n.odata.getErrorMessage(t))})}});n.sessionPlanningPresentationsPage=function(n,t){ko.applyBindingsAndShow(new f(t),n)}}(window.app,window.OData),function(n,t,i,r){function o(){var n=this;n.id=i.autoMap();n.name=i.autoMap()}function u(t){var u=this;u.id=ko.observable().autoMap();u.name=ko.observable().extend({required:!0}).autoMap();u.description=ko.observable().autoMap();u.start=ko.observable().autoMap();u.durationInMinutes=ko.observable().extend({required:!1,number:!0}).autoMap();u.end=ko.observable().autoMap();u.roomId=ko.observable().autoMap();u.roomName=ko.observable().autoMap();u.presentations=[];u.chair=ko.observable().autoMap();u.quota=ko.observable().extend({required:!1,number:!0}).autoMap();u.isSelected=ko.observable(t);u.save=function(){var t=u.id(),f=u.start(),e={method:t?"PATCH":"POST",requestUri:i.odata.getUrl(i.odata.entitySet.sessions,t?t:null),showProgressIndicator:!1,data:{Name:u.name(),Start:f&&f.length>0?f:null,RoomId:n.isNumeric(u.roomId())?u.roomId():null,DurationInMinutes:n.isNumeric(u.durationInMinutes())?u.durationInMinutes():null,Chair:u.chair(),Quota:n.isNumeric(u.quota())?u.quota():null}};return r.request(e)};u.remove=function(){var n={method:"DELETE",requestUri:i.odata.getUrl(i.odata.entitySet.sessions,u.id()),showProgressIndicator:!1};return r.request(n)}}function e(){var n=this;n.controller=i.odata.entitySet.sessions;n.sessions=ko.observableArray([]);i.DataTable.call(n)}function s(f,e){function c(){var n={method:"GET",headers:{Accept:"application/json"},requestUri:i.odata.getUrl(i.odata.entitySet.rooms)+"?$select=Id,Name"};return r.request(n).done(function(n){var r,u,t,f,e;if(n.value){for(r=n.value,u=[],t=0;t<r.length;t++)f=r[t],e=i.autoMap(new o,f),u.push(e);s.rooms(u)}})}var s=this,h;s.session=ko.observable();s.rooms=ko.observableArray();s.addEditText=ko.pureComputed(function(){var n=s.session();return n&&n.id()?"Edit":"Add"});h=n(t.getElementById(f));s.addEditSession=function(t){var r=s.rooms(),f=!r||r.length===0?c():n.Deferred().resolve().promise();f.done(function(){t=t&&t.constructor===u?i.autoMap(new u,t):new u(s);s.session(t);h.modal("show")})};s.save=function(){var t=s.session();t&&typeof t.save=="function"&&(i.showProgress(),n.when(t.save()).then(function(){return h.modal("hide"),e.loadData(!1,!0)}).always(i.hideProgress))}}function h(u){var e=this,o=n(t.getElementById(u));e.conflicts=ko.observableArray();e.sessions=ko.observableArray();e.delete=function(n){var t,r,i;if(f[n.id()]){for(t=e.sessions(),r=-1,i=0;i<t.length;i++)if(t[i].id()===n.id()){r=i;break}r>-1&&(t.splice(r,1),n.isSelected(!1),e.sessions(t));f[n.id()]=!1}};e.add=function(n){f[n.id()]||(e.sessions.push(n),n.isSelected(!0),f[n.id()]=n)};e.check=function(){for(var f,t=[],u=e.sessions(),n=0;n<u.length;n++)t.push(u[n].id());f={method:"POST",headers:{"Content-Type":"application/json",Accept:"application/json"},requestUri:i.odata.getUrl(i.odata.entitySet.sessions,null,"CheckConflicts"),data:{Request:{SessionIds:t}}};r.request(f).done(function(n){e.conflicts(n.value);o.modal("show")})}}function c(t,f){var o=this;o.table=new e;o.addEditDialog=new s(t,o.table);o.selectedSessions=new h(f);o.table.loadData();o.selectSession=function(n){if(!n||n.constructor!==u)return!1;o.selectedSessions.add(n)};o.deselectSession=function(n){if(!n||n.constructor!==u)return!1;o.selectedSessions.delete(n)};o.removeSession=function(t){if(!t||t.constructor!==u||!window.confirm("Are you sure you want to remove this session?"))return!1;i.showProgress();n.when(t.remove()).then(function(){return o.table.loadData(!1,!0)}).always(i.hideProgress)};o.invokeBulk=function(t,r){var u=r.target,f=n(u).attr("href"),e=o.table.getFilterForURIComponent(),s={method:"GET",headers:{Accept:"application/json"},requestUri:i.odata.getUrl(i.odata.entitySet.sessions)+"?$count=true&$select=Id"+e,showProgressIndicator:!0};OData.request(s,function(n){for(var e,o,s,r=n.value,u=[],t=0;t<r.length;t++)e=r[t],u.push(e.Id);o=u.join("/");s={Ids:o};i.page.post(f,s)});r.preventDefault()};o.exportSessionPresentations=function(n,t){var r=o.table.getFilterForURIComponent(),u={method:"GET",headers:{Accept:"application/json"},requestUri:i.odata.getUrl(i.odata.entitySet.sessions)+"?$count=true&$select=Id"+r,showProgressIndicator:!0};OData.request(u,function(n){for(var f,e,o,r=n.value,u=[],t=0;t<r.length;t++)f=r[t],u.push(f.Id);e={SessionIds:u.join(",")};o=i.odata.getUrl(i.odata.entitySet.sessions,null,"ExportSessionPresentations");i.page.post(o,e)});t.preventDefault()};o.bulkUnassignPresentation=function(){if(confirm("Bulk unassigning will be performed for selected sessions.")){var n=o.table.getFilterString(),t={requestUri:i.odata.getUrl(i.odata.entitySet.sessions,null,"BulkUnassignPresentation"),method:"POST",showProgressIndicator:!0,data:{Filter:n}};r.request(t,function(){i.addMessage("Bulk unassigning has been completed successfully.",null,"success","text",!0);location.reload()})}}}var f=[];e.prototype=n.extend({},i.DataTable.prototype,{getDefaultSorting:function(){return{property:"Id",direction:"asc"}},getFilterString:function(){var i=this,t="";return n.each(i.filters,function(n,i){i.getValue()&&(t+=t?" and "+i.getValue():i.getValue())}),t},getFilterForURIComponent:function(){var t=this,n=t.getFilterString();return n&&(n="&$filter="+encodeURIComponent(n)),n},loadData:function(n,t){var e;n=n===!0;e=this;n&&e.applyState();var o=e.sorting(),s=o?"&$orderby="+encodeURIComponent(o.property+" "+o.direction):"",h=e.skip()?"&$skip="+e.skip():"",c=e.top()?"&$top="+e.top():"",l=e.getFilterForURIComponent(),a={method:"GET",headers:{Accept:"application/json"},requestUri:i.odata.getUrl(i.odata.entitySet.sessions)+"?$count=true"+l+s+h+c,showProgressIndicator:!n&&!t};return r.request(a,function(n){var r,t,o,s;for(e.total(n["@odata.count"]||0),r=[],t=0;t<n.value.length;t++)o=n.value[t],s=i.autoMap(new u(f[o.Id]),o),r.push(s);e.sessions(r);e.saveState()},function(n){i.addErrorMessage(i.odata.getErrorMessage(n))})}});i.sessionPlanningSessionsPage=function(n,t,i){ko.applyBindingsAndShow(new c(t,i),n)}}($,document,window.app,window.OData),function(n,t,i,r,u){function f(){var t=this;t.id=ko.observable(0).autoMap();t.name=ko.observable("").extend({required:!0}).autoMap();t.size=ko.observable().extend({required:!1,number:!0}).autoMap();t.save=function(){var i=t.id(),f={method:i?"PATCH":"POST",requestUri:r.odata.getUrl(r.odata.entitySet.rooms,i?i:null),showProgressIndicator:!1,data:{Name:t.name(),Size:n.isNumeric(t.size())?t.size():null}};return u.request(f)};t.remove=function(){var n={method:"DELETE",requestUri:r.odata.getUrl(r.odata.entitySet.rooms,t.id()),showProgressIndicator:!1};return u.request(n)}}function e(){var n=this;n.rooms=ko.observableArray([]);r.DataTable.call(n)}function o(t,u){var e=this,o;e.room=ko.observable();e.addEditText=ko.pureComputed(function(){var n=e.room();return n&&n.id()?"Edit":"Add"});o=n(i.getElementById(t));e.addEditRoom=function(n){n=n&&n.constructor===f?r.autoMap(new f,n):new f(e);e.room(n);o.modal("show")};e.save=function(){var t=e.room();t&&typeof t.save=="function"&&(r.showProgress(),n.when(t.save()).then(function(){return o.modal("hide"),u.loadData(!1,!0)}).always(r.hideProgress))}}function s(i){var u=this;u.table=new e;u.addEditDialog=new o(i,u.table);u.table.loadData();u.removeRoom=function(i){if(!i||i.constructor!==f||!t.confirm("Are you sure you want to remove this room?"))return!1;r.showProgress();n.when(i.remove()).then(function(){return u.table.loadData(!1,!0)}).always(r.hideProgress)}}e.prototype=n.extend({},r.DataTable.prototype,{getDefaultSorting:function(){return{property:"Id",direction:"asc"}},loadData:function(t,i){var e,h,c;t=t===!0;e=this;t&&e.applyState();var s=e.sorting(),l=s?"&$orderby="+encodeURIComponent(s.property+" "+s.direction):"",a=e.skip()?"&$skip="+e.skip():"",v=e.top()?"&$top="+e.top():"",o="";return n.each(e.filters,function(n,t){t.getValue()&&(o+=o?" and "+t.getValue():t.getValue())}),o&&(o="&$filter="+encodeURIComponent(o)),h={method:"GET",headers:{Accept:"application/json"},requestUri:r.odata.getUrl(r.odata.entitySet.rooms)+"?$count=true"+o+l+a+v,showProgressIndicator:!t&&!i},c=u.request(h,function(n){var i,t,u,o;for(e.total(n["@odata.count"]||0),i=[],t=0;t<n.value.length;t++)u=n.value[t],o=r.autoMap(new f,u),i.push(o);e.rooms(i);e.saveState()},function(n){r.addErrorMessage(r.odata.getErrorMessage(n))}),c}});r.sessionPlanningRoomsPage=function(n,t){ko.applyBindingsAndShow(new s(t),n)}}($,window,document,window.app,window.OData),function(n){function t(n,t){var i=this;i.number=ko.observable(n);i.name=ko.observable(t);i.left=ko.pureComputed(function(){return i.number()*150+"px"})}function i(n){var t=this;t.hour=ko.observable(n);t.top=ko.pureComputed(function(){return t.hour()*60+"px"})}function r(){var r=this,u,f,n;for(r.rooms=ko.observableArray([]),r.hours=ko.observableArray([]),u=[],n=0;n<25;n++)u.push(new i(n));for(r.hours(u),f=[],n=0;n<5;n++)f.push(new t(n,"Room "+(n+1)));r.rooms(f)}n.sessionPlanningPreviewPage=function(n){ko.applyBindingsAndShow(new r,n)}}(window.app),function(n,t,i){function r(){var r=this;r.sessions=ko.observableArray([]);r.getStartDate=function(n){if(!n)return"?";var t=new Date(n);return new Intl.DateTimeFormat("en-US",{weekday:"short",month:"short",day:"2-digit",hour:"2-digit",minute:"2-digit",timeZone:"UTC",hour12:!1}).format(t)};r.getEndDate=function(n){if(!n)return"?";var t=new Date(n);return new Intl.DateTimeFormat("en-US",{hour:"2-digit",minute:"2-digit",timeZone:"UTC",hour12:!1}).format(t)};i.showProgress();n.get("/api/"+(t.cmt3&&t.cmt3.conference?t.cmt3.conference.name:null)+"/contents").done(function(n){r.sessions(n.Sessions)}).always(i.hideProgress)}i.sessionPlanningContentsPage=function(n){ko.applyBindingsAndShow(new r,n)}}($,window,window.app),function(n,t){"use strict";function i(){var t=this;t.id=n.autoMap();t.name=n.autoMap();t.parentSubjectAreaId=n.autoMap();t.isChild=function(){return t.parentSubjectAreaId!==null};t.isPrimary=ko.observable();t.isSecondary=ko.observable();t.checkBoxId=function(){return"primary"+t.id};t.allowParentSelection=!0;t.specialType=null}function r(r,u,f,e){function s(){function i(){var i,r,n,t,u;if(o.subjectAreas.length===0)return!0;for(i=[],r=!1,n=0;n<o.subjectAreas.length;n++)(o.subjectAreas[n].specialType==="customPrimary"||o.subjectAreas[n].specialType==="customSecondary")&&i.push(o.subjectAreas[n].customValue),o.subjectAreas[n].isPrimary()&&(r=!0);return t=!0,u=ko.validation.group(i),u().length>0&&(u.showAllMessages(),t=!1),r||(o.showSubjectAreasErrorMessage(!0),t=!1),t}o.showValidationWarning=ko.observable(!1);o.subjectAreas=[];o.subjectAreaPairs=function(){return n.computeSubjectAreaColumnPairs(o.subjectAreas)};o.showSubjectAreasErrorMessage=ko.observable(!1);o.save=function(){var l=ko.validation.group(o),e,s,f,u,h,c;if(l().length>0){o.showValidationWarning(!0);return}if(e=!0,i()||(e=!1),!e){o.showValidationWarning(!0);return}for(s=[],f=0;f<o.subjectAreas.length;f++)u=o.subjectAreas[f],(u.isPrimary()||u.isSecondary())&&u.specialType===null&&(h={SubjectAreaId:u.id,IsPrimary:u.isPrimary()},s.push(h));c={requestUri:n.odata.getUrl(n.odata.entitySet.sessions,null,"UpdateSubjectAreas"),method:"POST",showProgressIndicator:!0,data:{Request:{SessionId:r,SubjectAreas:s}}};t.request(c,function(){n.addMessage("Subject areas saved for session.",null,"success","text",!0);location.reload()})}}function h(t,r){function c(n){n.isPrimary.subscribe(function(n){n&&(o.showSubjectAreasErrorMessage(!1),l(this),this.isSecondary(!1))},n);n.isSecondary.subscribe(function(n){var t,i;if(n){if(o.settings.secondarySubjectAreaLimited&&(t=a(),t>o.settings.secondarySubjectAreaMaxNumber)){i=this;setTimeout(function(){i.isSecondary(!1)},0);return}this.isPrimary(!1)}},n);o.subjectAreas.push(n)}function l(n){for(var t=0;t<o.subjectAreas.length;t++)o.subjectAreas[t].isPrimary()&&o.subjectAreas[t]!==n&&o.subjectAreas[t].isPrimary(!1)}function a(){for(var t=0,n=0;n<o.subjectAreas.length;n++)o.subjectAreas[n].isSecondary()&&++t;return t}for(var s,u,h,e=null,f=0;f<t.length;f++)u=n.autoMap(new i,t[f]),e!==null&&e.id===u.parentSubjectAreaId&&!o.settings.immediateParentSelectionAllowed&&e.allowParentSelection&&(e.allowParentSelection=!1),u.parentSubjectAreaId===null&&(e=u),c(u);for(s={},f=0;f<r.length;f++)u=r[f],s[u.SubjectAreaId]=u.IsPrimary;for(f=0;f<o.subjectAreas.length;f++)u=o.subjectAreas[f],h=s[u.id],h?u.isPrimary(!0):h===!1&&u.isSecondary(!0)}var o=this;o.sessionId=r;o.settings={secondarySubjectAreaAllowed:n.autoMap(),secondarySubjectAreaLimited:n.autoMap(),secondarySubjectAreaMaxNumber:n.autoMap(),immediateParentSelectionAllowed:n.autoMap()};n.autoMap(o.settings,u);o.bindTo=function(n){s();h(f,e);ko.applyBindingsAndShow(o,n)}}n.sessionSubjectAreas=function(n,t,i,u,f){new r(n,t,i,u).bindTo(f)}}(window.app,window.OData,window.jQuery,document),function(n,t){function i(t){var i=this;i.id=n.autoMap();i.name=n.autoMap();i.reviewPreview=t}function r(){var t=this;t.id=n.autoMap();t.trackId=n.autoMap();t.name=n.autoMap()}function f(r,u,f,e,o,s,h,c,l){function v(t,r){for(var e,o,s,h,c,v,y,l=[],a=r&&JSON.parse(r)||[],u,f=0;f<a.length;f++){if(e=a[f],o=[],t=t||[],t.length>0){for(s=e.Question||[],h={},u=0;u<s.length;u++)c=s[u],h[c.QuestionOrder]=c;for(u=0;u<t.length;u++)v=t[u],o.push(h[v.Order]||[])}y=n.autoMap(new i(o),e);l.push(y)}return l}var a=this;a.questions=[];a.id=n.autoMap();a.title=n.autoMap();a.abstract=n.autoMap();a.authors=n.autoMap();a.primarySubject=n.autoMap();a.secondarySubject=n.autoMap();a.reviewersJson=n.autoMap();a.assigned=n.autoMap();a.completed=n.autoMap();a.percentage=n.autoMap();a.bids=n.autoMap();a.metaReviewersJson=n.autoMap();a.metaAssigned=n.autoMap();a.metaCompleted=n.autoMap();a.metaPercentage=n.autoMap();a.metaBids=n.autoMap();a.messages=n.autoMap();a.messagesRead=n.autoMap();a.discussionEnabled=ko.observable().autoMap();a.status=n.autoMap();a.seniorMetaReviewerRating=ko.observable().autoMap();a.seniorMetaReviewerRatingOptionId=ko.observable().autoMap();a.ratingComment=ko.observable("").autoMap();a.isAuthorFeedback=n.autoMap();a.isAuthorFeedbackPosted=n.autoMap();a.authorFeedbackId=n.autoMap();a.completedReviewRating=n.autoMap();a.percentageReviewRating=n.autoMap();a.numberOfReviewerNotes=n.autoMap();a.numberOfMetaReviewerNotes=n.autoMap();a.seniorMetaReviewerNoteSubmitted=n.autoMap();a.seniorMetaReviewerNoteId=n.autoMap();a.track=f;a.trackId=u;a.isAbstractVisible=ko.observable(!1);a.toggleAbstract=function(){return a.isAbstractVisible(!a.isAbstractVisible()),!1};a.isAuthorFeedbackText=ko.pureComputed(function(){return a.isAuthorFeedback?"Yes":"No"});a.isAuthorFeedbackPostedText=ko.pureComputed(function(){return a.isAuthorFeedbackPosted?"Yes":"No"});a.isCameraReadyPosted=n.autoMap();a.isCameraReadyPostedBool=ko.pureComputed(function(){return a.isCameraReadyPosted==="Yes"});a.reviewQuestions=ko.pureComputed(function(){return e});a.inlineReviews=ko.pureComputed(function(){return v(e,o)});a.metaReviewQuestions=ko.pureComputed(function(){return s});a.inlineMetaReviews=ko.pureComputed(function(){return v(s,h)});a.metaReviewerNoteQuestions=ko.pureComputed(function(){return c});a.inlineMetaReviewerNotes=ko.pureComputed(function(){return v(c,l)});a.hasSeniorMetaReviewerNoteQuestion=ko.pureComputed(function(){return f&&f.hasSeniorMetaReviewerNoteQuestion});a.showInlineReviewForSeniorMetaReviewer=ko.pureComputed(function(){return f&&f.showInlineReviewForSeniorMetaReviewer});a.showInlineMetaReviewForSeniorMetaReviewer=ko.pureComputed(function(){return f&&f.showInlineMetaReviewForSeniorMetaReviewer});a.showInlineMetaReviewerNoteForSeniorMetaReviewer=ko.pureComputed(function(){return f&&f.showInlineMetaReviewerNoteForSeniorMetaReviewer});a.allowSeniorMetaReviewerToEmailAuthor=ko.pureComputed(function(){return f&&f.allowSeniorMetaReviewerToEmailAuthor});a.allowSeniorMetaReviewerToViewPaperStatus=ko.pureComputed(function(){return f&&f.allowSeniorMetaReviewerToViewPaperStatus});a.allowSeniorMetaReviewerToChangePaperStatus=ko.pureComputed(function(){return f&&f.allowSeniorMetaReviewerToChangePaperStatus});a.allowSeniorMetaReviewerToRateSubmission=ko.pureComputed(function(){return f&&f.allowSeniorMetaReviewerToRateSubmission});a.allowSeniorMetaReviewerToEnterRatingComment=ko.pureComputed(function(){return f&&f.allowSeniorMetaReviewerToEnterRatingComment});a.allowSeniorMetaReviewerToInviteReviewers=ko.pureComputed(function(){return f&&f.allowSeniorMetaReviewerToInviteReviewers});a.doNotAllowSeniorMetaReviewerToEditNote=ko.pureComputed(function(){return f&&f.doNotAllowSeniorMetaReviewerToEditNote});a.doNotAllowSeniorMetaReviewerToEditReviewAssignment=ko.pureComputed(function(){return f&&f.doNotAllowSeniorMetaReviewerToEditReviewAssignment});a.doNotAllowSeniorMetaReviewerToEditMetaReviewAssignment=ko.pureComputed(function(){return f&&f.doNotAllowSeniorMetaReviewerToEditMetaReviewAssignment});a.doNotAllowSeniorMetaReviewerToEnableDiscussion=ko.pureComputed(function(){return f&&f.doNotAllowSeniorMetaReviewerToEnableDiscussion});a.doNotEnableReviewerNote=ko.pureComputed(function(){return f&&f.doNotEnableReviewerNote});a.doNotEnableMetaReviewerNote=ko.pureComputed(function(){return f&&f.doNotEnableMetaReviewerNote});a.doNotEnableSeniorMetaReviewerNote=ko.pureComputed(function(){return f&&f.doNotEnableSeniorMetaReviewerNote});a.reviewers=ko.pureComputed(function(){var f=[],t=a.reviewersJson?JSON.parse(a.reviewersJson):[],r,u,e;if(t&&t.length>0)for(r=0;r<t.length;r++)(u=t[r],u)&&(e=n.autoMap(new i,u),f.push(e));return f});a.metaReviewers=ko.pureComputed(function(){var f=[],t=a.metaReviewersJson?JSON.parse(a.metaReviewersJson):[],r,u,e;if(t&&t.length>0)for(r=0;r<t.length;r++)(u=t[r],u)&&(e=n.autoMap(new i,u),f.push(e));return f});a.editSeniorMetaReviewerNoteUrl=function(){return a.seniorMetaReviewerNoteId?r.seniorMetaReviewerNoteDetails.format(a.seniorMetaReviewerNoteId):r.seniorMetaReviewerNoteCreate.format(a.id)};a.editSeniorMetaReviewerNoteText=function(){return a.seniorMetaReviewerNoteSubmitted?"Edit":"Add"};a.editSeniorMetaReviewerNoteTooltip=function(){return a.seniorMetaReviewerNoteSubmitted?"Edit note":"Add note"};a.seniorMetaReviewerNoteSubmittedText=ko.pureComputed(function(){return a.seniorMetaReviewerNoteSubmitted?"Yes":"No"});a.viewSeniorMetaReviewerNoteUrl=function(){return a.seniorMetaReviewerNoteId?r.seniorMetaReviewerNoteView.format(a.seniorMetaReviewerNoteId):""};a.inviteReviewerUrl=function(n){return r.inviteReviewer.format(a.id,n)};a.reviewerEmailUrl=function(n){return r.reviewerEmail.format(a.id,n)};a.metaReviewerEmailUrl=function(n){return r.metaReviewerEmail.format(a.id,n)};a.PopulateAggregates=function(t,i){var f=this,u,e,r;for(f.aggregateColumns=[],u=0;u<t.length;u++)e=t[u],r="Q0"+e.Order,e.IsMeta&&(r="M"+r),i[r+"Id"]!=null?f.aggregateColumns.push(new n.AggregateColumn(r,i[r+"Id"],i[r+"Avg"],i[r+"Min"],i[r+"Max"],i[r+"Spread"])):f.aggregateColumns.push(new n.AggregateColumn(r,null,null,null,null,null))};a.PopulateSeniorMetaReviewerNoteColumns=function(t,i){var r={},f,u;for(i.SMRNQ01Id!==null&&(r[1]=new n.QuestionResponseColumn(i.SMRNQ01Id,i.SMRNQ01Text)),i.SMRNQ02Id!==null&&(r[2]=new n.QuestionResponseColumn(i.SMRNQ02Id,i.SMRNQ02Text)),i.SMRNQ03Id!==null&&(r[3]=new n.QuestionResponseColumn(i.SMRNQ03Id,i.SMRNQ03Text)),i.SMRNQ04Id!==null&&(r[4]=new n.QuestionResponseColumn(i.SMRNQ04Id,i.SMRNQ04Text)),i.SMRNQ05Id!==null&&(r[5]=new n.QuestionResponseColumn(i.SMRNQ05Id,i.SMRNQ05Text)),i.SMRNQ06Id!==null&&(r[6]=new n.QuestionResponseColumn(i.SMRNQ06Id,i.SMRNQ06Text)),i.SMRNQ07Id!==null&&(r[7]=new n.QuestionResponseColumn(i.SMRNQ07Id,i.SMRNQ07Text)),i.SMRNQ08Id!==null&&(r[8]=new n.QuestionResponseColumn(i.SMRNQ08Id,i.SMRNQ08Text)),i.SMRNQ09Id!==null&&(r[9]=new n.QuestionResponseColumn(i.SMRNQ09Id,i.SMRNQ09Text)),i.SMRNQ10Id!==null&&(r[10]=new n.QuestionResponseColumn(i.SMRNQ10Id,i.SMRNQ10Text)),i.SMRNQ11Id!==null&&(r[11]=new n.QuestionResponseColumn(i.SMRNQ11Id,i.SMRNQ11Text)),i.SMRNQ12Id!==null&&(r[12]=new n.QuestionResponseColumn(i.SMRNQ12Id,i.SMRNQ12Text)),i.SMRNQ13Id!==null&&(r[13]=new n.QuestionResponseColumn(i.SMRNQ13Id,i.SMRNQ13Text)),i.SMRNQ14Id!==null&&(r[14]=new n.QuestionResponseColumn(i.SMRNQ14Id,i.SMRNQ14Text)),i.SMRNQ15Id!==null&&(r[15]=new n.QuestionResponseColumn(i.SMRNQ15Id,i.SMRNQ15Text)),i.SMRNQ16Id!==null&&(r[16]=new n.QuestionResponseColumn(i.SMRNQ16Id,i.SMRNQ16Text)),i.SMRNQ17Id!==null&&(r[17]=new n.QuestionResponseColumn(i.SMRNQ17Id,i.SMRNQ17Text)),i.SMRNQ18Id!==null&&(r[18]=new n.QuestionResponseColumn(i.SMRNQ18Id,i.SMRNQ18Text)),i.SMRNQ19Id!==null&&(r[19]=new n.QuestionResponseColumn(i.SMRNQ19Id,i.SMRNQ19Text)),i.SMRNQ20Id!==null&&(r[20]=new n.QuestionResponseColumn(i.SMRNQ20Id,i.SMRNQ20Text)),i.SMRNQ21Id!==null&&(r[21]=new n.QuestionResponseColumn(i.SMRNQ21Id,i.SMRNQ21Text)),i.SMRNQ22Id!==null&&(r[22]=new n.QuestionResponseColumn(i.SMRNQ22Id,i.SMRNQ22Text)),i.SMRNQ23Id!==null&&(r[23]=new n.QuestionResponseColumn(i.SMRNQ23Id,i.SMRNQ23Text)),i.SMRNQ24Id!==null&&(r[24]=new n.QuestionResponseColumn(i.SMRNQ24Id,i.SMRNQ24Text)),i.SMRNQ25Id!==null&&(r[25]=new n.QuestionResponseColumn(i.SMRNQ25Id,i.SMRNQ25Text)),f=[],u=0;u<t.length;u++)f.push(r[t[u].Order]);a.seniorMetaReviewerNoteColumns=f};a.PopulateChairNoteColumns=function(t,i){var r={},f,u;for(i.CNQ01Id!==null&&(r[1]=new n.QuestionResponseColumn(i.CNQ01Id,i.CNQ01Text)),i.CNQ02Id!==null&&(r[2]=new n.QuestionResponseColumn(i.CNQ02Id,i.CNQ02Text)),i.CNQ03Id!==null&&(r[3]=new n.QuestionResponseColumn(i.CNQ03Id,i.CNQ03Text)),i.CNQ04Id!==null&&(r[4]=new n.QuestionResponseColumn(i.CNQ04Id,i.CNQ04Text)),i.CNQ05Id!==null&&(r[5]=new n.QuestionResponseColumn(i.CNQ05Id,i.CNQ05Text)),i.CNQ06Id!==null&&(r[6]=new n.QuestionResponseColumn(i.CNQ06Id,i.CNQ06Text)),i.CNQ07Id!==null&&(r[7]=new n.QuestionResponseColumn(i.CNQ07Id,i.CNQ07Text)),i.CNQ08Id!==null&&(r[8]=new n.QuestionResponseColumn(i.CNQ08Id,i.CNQ08Text)),f=[],u=0;u<t.length;u++)f.push(r[t[u].Order]);a.chairNoteColumns=f};a.setEnable=function(i){var r=!i.discussionEnabled(),u={requestUri:n.odata.getUrl(n.odata.entitySet.submissions,null,"EnableDisableDiscussion"),method:"POST",showProgressIndicator:!0,data:{Enable:r,SubmissionId:i.id}};t.request(u,function(){i.discussionEnabled(r);n.addMessage("Author feedback for submission {0} has been {1}!".format(i.id,r?"enabled":"disabled"))})}}function e(t){var i=this;i.ratingComment=ko.observable("").extend({maxLength:300});i.bind=function(){ko.applyBindings(i,t)};i.ratingOptions=ko.observableArray([]);i.viewRatingOptions={};i.selectedSeniorMetaReviewerRating=ko.observable(null);i.sid=ko.observable(0);i.data=null;i.editInDialog=function(u){i.data=u;i.ratingComment(u.ratingComment());i.sid(u.id);i.ratingOptions([]);i.viewRatingOptions={};OData.read(n.odata.getUrl(n.odata.entitySet.seniorMetaReviewerRatingOptions+"?$filter=TrackId eq "+u.trackId),function(f){for(var s,o,e=0;e<f.value.length;e++)s=f.value[e],o=n.autoMap(new r,s),i.ratingOptions.push(o),i.viewRatingOptions[o.id]=o;i.selectedSeniorMetaReviewerRating(u.seniorMetaReviewerRatingOptionId());$(t).modal("show")})};i.saveRating=function(){var r={requestUri:n.odata.getUrl(n.odata.entitySet.submissions,null,"ChangeSeniorMetaReviewerRating"),method:"POST",showProgressIndicator:!0,data:{Request:{SubmissionId:i.sid(),RatingOptionId:i.selectedSeniorMetaReviewerRating()||null,RatingComment:i.ratingComment()}}};OData.request(r,function(n){n&&(i.data.seniorMetaReviewerRating(i.viewRatingOptions[n.value].name),i.data.seniorMetaReviewerRatingOptionId(n.value),i.data.ratingComment(i.ratingComment()));$(t).modal("hide")})}}function u(t,i,r,u,f,o,s,h,c,l,a){var v=this,y;v.key=t;v.tracks=i;v.pageUrls=r;v.questions=o;v.reviewQuestions=s;v.metaReviewQuestions=h;v.metaReviewerNoteQuestions=c;v.seniorMetaReviewerNoteQuestions=l;v.chairNoteQuestions=a;v.submissions=ko.observableArray([]);v.editRatingVm=null;v.submissionStatusNamesProvider=ko.pureComputed(function(){return u});v.submissionSeniorMetaReviewerRatingOptionsProvider=ko.pureComputed(function(){return f});v.trackNamesProvider=ko.pureComputed(function(){var n=[];for(var t in i)i.hasOwnProperty(t)&&n.push(i[t].name);return n});v.reviewerAllowedToCompareSubmission=ko.computed(function(){for(var n in i)if(i.hasOwnProperty(n)&&i[n].allowReviewerToCompareSubmission)return!0;return!1});v.metaReviewerAllowedToCompareSubmission=ko.computed(function(){for(var n in i)if(i.hasOwnProperty(n)&&i[n].allowMetaReviewerToCompareSubmission)return!0;return!1});v.exportReviewerSubmissionComparisons=function(){var t=this,i=t.getFilterString(),r=n.odata.getUrl(n.odata.entitySet.submissionModels,null,"ExportReviewerSubmissionComparisons"),u={Filter:i};n.page.post(r,u)};v.exportMetaReviewerSubmissionComparisons=function(){var t=this,i=t.getFilterString(),r=n.odata.getUrl(n.odata.entitySet.submissionModels,null,"ExportMetaReviewerSubmissionComparisons"),u={Filter:i};n.page.post(r,u)};y=null;v.selectSeniorMetaReviewerRatingWithComment=function(n){y===null&&(y=new e(document.getElementById("editRatingDialog")),y.bind());y.editInDialog(n)};v.email=function(t,i){var c=this,r=i.target,e=parseInt($(r).attr("sid")),l=$(r).attr("recipientType"),o=$(r).attr("all"),s=$(r).attr("checkNote"),f,h,u;f=e?"Id eq {0}".format(e):c.getFilterString();h="/"+window.cmt3.conference.name+"/Submission/SendEmail/"+l;u={filter:f.length>0?f:null};o&&(u.all=o);s&&(u.checkNote=s);n.url.navigateTo(h,u)};v.downloadAllLink=function(){return r.submissionFile.format("")};v.downloadFiles=function(t,i){var f=this,e=i.target,o=$(e).attr("href"),r=f.getFilterString(),u;r&&(r="&$filter="+encodeURIComponent(r));u={method:"GET",headers:{Accept:"application/json"},requestUri:n.odata.getUrl(n.odata.entitySet.submissionModels)+"?$select=Id"+r,showProgressIndicator:!0};OData.request(u,function(t){for(var f,e,r=t.value,u=[],i=0;i<r.length;i++)u.push(r[i].Id);f=u.join("/");e={Ids:f};n.page.post(o,e)});i.preventDefault()};n.DataTable.call(v)}u.prototype=$.extend({},n.DataTable.prototype,{getStorageKey:function(){var n=this;return n.key},getDefaultSorting:function(){return{property:"Id",direction:"asc"}},getFilterString:function(){var t=this,n="";return $.each(t.filters,function(t,i){i.getValue()&&(n+=n?" and "+i.getValue():i.getValue())}),n},selectStatus:function(n,t){var i=$(t.target),u=ko.contextFor(t.target),r=$($("#statusTemplate").text());i.hide();i.after(r);u.$parent.getStatuses(n.id,n.track.id,i,r).done(function(n){ko.applyBindings(n,r[0])})},getStatuses:function(t,i,r,u){var f=$.Deferred();return OData.read(n.odata.getUrl(n.odata.entitySet.submissionStatuses),function(e){for(var a,o,h,c=[],l={},s=0;s<e.value.length;s++)a=e.value[s],o=n.autoMap(new n.SubmissionStatus,a),o.trackId==i&&(c.push(o),l[o.id]=o);h={options:ko.observableArray(c),selectedStatus:ko.observable()};h.selectedStatus.subscribe(function(i){var f={requestUri:n.odata.getUrl(n.odata.entitySet.submissions,null,"ChangeStatus"),method:"POST",showProgressIndicator:!0,data:{Request:{SubmissionId:t,StatusId:i[0]}}};OData.request(f,function(n){u.remove();r.text(l[n.value].name);r.show()})});f.resolve(h)}),f.promise()},selectSeniorMetaReviewerRating:function(n,t){var i=$(t.target),u=ko.contextFor(t.target),r=$($("#seniorMetaReviewerRatingTemplate").text());i.hide();i.after(r);u.$parent.getSeniorMetaReviewerRatingOptions(n.id,n.track.id,n.seniorMetaReviewerRatingOptionId,i,r).done(function(n){ko.applyBindings(n,r[0])})},getSeniorMetaReviewerRatingOptions:function(t,i,u,f,e){var o=$.Deferred();return OData.read(n.odata.getUrl(n.odata.entitySet.seniorMetaReviewerRatingOptions+"?$filter=TrackId eq "+i),function(i){for(var v,s,c,l=[],a={},h=0;h<i.value.length;h++)v=i.value[h],s=n.autoMap(new r,v),l.push(s),a[s.id]=s;c={options:ko.observableArray(l),selectedSeniorMetaReviewerRating:ko.observable(u())};c.selectedSeniorMetaReviewerRating.subscribe(function(i){if(i!=u()){var r={requestUri:n.odata.getUrl(n.odata.entitySet.submissions,null,"ChangeSeniorMetaReviewerRating"),method:"POST",showProgressIndicator:!0,data:{Request:{SubmissionId:t,RatingOptionId:i||null}}};OData.request(r,function(n){u(n&&n.value);e.remove();n?f.text(a[n.value].name):f.text("Not Rated");f.show()})}});o.resolve(c)}),o.promise()},loadData:function(i){var r,u;return i=i===!0,r=this,i&&r.applyState(),u=function(i){var e=r.sorting(),s=e?"&$orderby="+encodeURIComponent(e.property+" "+e.direction):"",h=r.skip()?"&$skip="+r.skip():"",c=r.top()?"&$top="+r.top():"",u=r.getFilterString(),o;return u&&(u="&$filter="+encodeURIComponent(u)),o={method:"GET",headers:{Accept:"application/json"},requestUri:n.odata.getUrl(n.odata.entitySet.submissionModels)+"?"+(i?"$count=true&$top=0"+u:s+u+h+c)},t.request(o,function(t){var h,o;if(i)r.total(t["@odata.count"]||0);else{for(h=[],o=0;o<t.value.length;o++){var u=t.value[o],e=u.TrackId,c=r.tracks&&r.tracks[e],l=r.reviewQuestions&&r.reviewQuestions[e],a=r.metaReviewQuestions&&r.metaReviewQuestions[e],v=r.metaReviewerNoteQuestions&&r.metaReviewerNoteQuestions[e],s=n.autoMap(new f(r.pageUrls,e,c,l,u.InlineReviewJson,a,u.InlineMetaReviewJson,v,u.InlineMetaReviewerNoteJson),u);s.PopulateAggregates(r.questions,u);s.PopulateSeniorMetaReviewerNoteColumns(r.seniorMetaReviewerNoteQuestions,u);s.PopulateChairNoteColumns(r.chairNoteQuestions,u);h.push(s)}r.submissions(h)}r.saveState()},function(t){n.addErrorMessage(n.odata.getErrorMessage(t))})},$.when(u(!1),u(!0)).done(function(){$("html,body").scrollTop(0)})},openAllReviews:function(t,i,r,u){var o=this,f=o.getFilterString(),e;f&&(f="&$filter="+encodeURIComponent(f));e={method:"GET",headers:{Accept:"application/json"},requestUri:n.odata.getUrl(n.odata.entitySet.submissionModels)+"?$select=Id"+f,showProgressIndicator:!0};OData.request(e,function(t){for(var o,s,f=t.value,e=[],i=0;i<f.length;i++)e.push(f[i].Id);o=e.join("/");s="/"+window.cmt3.conference.name+"/Submission/"+(r?u?"AllReviewsSideBySide":"AllReviews":"AllMetaReviews");n.url.navigateTo(s,{ids:o})})},openAllReviewsPrinterFriendly:function(n,t){this.openAllReviews(n,t,!0,!1)},openAllReviewsSideBySide:function(n,t){this.openAllReviews(n,t,!0,!0)},openAllMetaReviewsPrinterFriendly:function(n,t){this.openAllReviews(n,t,!1)}});n.seniorMetaReviewerSubmissionsPage=function(n,t,i,r,f,e,o,s,h,c,l,a,v){var y=new u(t,f,r,e,o,s,h,c,l,a,v),p;y.toggleableColumnsContainer&&y.toggleableColumnsContainer.setDefaultHiddenColumnKeys(i);p=document.getElementById(n);ko.applyBindings(y,p);y.loadData(!0).done(function(){y.toggleableColumnsContainer&&y.toggleableColumnsContainer.loadState();$(p).show()})}}(window.app,window.OData),function(n,t,i){"use strict";function r(r,u){var f=this;f.trackId=u;f.isFileUploaded=ko.observable(!1);f.users=ko.observableArray();f.normalUsers=ko.observableArray();f.hasError=ko.observable(!1);f.errorText=ko.observable();f.uploading=ko.observable(!1);f.userId=r;f.uploadFile=function(n,t){t.target.value!=""&&(f.uploading(!0),t.target.form.submit())};f.parseUploadResult=function(){var t=i.parseJSON(i("#singleFileUploadFrame").contents().text()),r,n,u;if(f.users.removeAll(),f.normalUsers.removeAll(),f.hasError(t.HasError),f.errorText(t.ErrorText),!f.hasError())for(r=0;r<t.Models.length;r++)n=t.Models[r],u={email:n.Email,userId:n.UserId,bid:n.Bid,notice:n.Note,hasError:n.HasError,rawData:n.RawData},f.users.push(u),u.hasError||f.normalUsers.push(u);f.isFileUploaded(!0);f.uploading(!1)};f.getModel=function(){for(var t,r,i=[],n=0;n<f.normalUsers().length;n++)t=f.normalUsers()[n],r={UserId:t.userId,Bid:t.bid},i.push(r);return{UserId:f.userId,TrackId:f.trackId,Bids:i}};f.send=function(){var i=f.getModel(),r={requestUri:n.odata.getUrl(n.odata.entitySet.seniorMetaReviewerBiddingModels,null,"Import"),method:"POST",data:{Request:i}};t.request(r,function(){window.location="/"+window.cmt3.conference.name+"/User/SeniorMetaBidding"})};f.bindTo=function(n){ko.applyBindingsAndShow(f,n)}}n.importSeniorMetaReviewerBids=function(n,t,i){new r(n,t).bindTo(i)}}(window.app,window.OData,window.jQuery,window.document,window.confirm),function(n,t,i){function u(t){function u(){f();r=i.isAssigned.subscribe(e)}function f(){r&&typeof r.dispose=="function"&&r.dispose()}function e(){i.initialState===undefined?i.initialState=i.isAssigned():o.call(i)}function o(){var r=this,e;r.isToggleInProgress(!0);e={UserId:r.userId};e.Type=r.isAssigned()?"Assign":"Remove";OData.request({requestUri:n.odata.getUrl(n.odata.entitySet.trackMetaReviewerGroups,t,"AssignMetaReviewer"),method:"POST",showProgressIndicator:!1,data:{Request:e}},function(){r.isAssigned()===r.initialState?i.css(""):i.css(r.isAssigned()?"success":"error")},function(t){f();i.isAssigned(!i.isAssigned());u();n.addErrorMessage("Unable to edit assignment for '"+r.firstName+" "+r.lastName+"'. "+n.odata.getErrorMessage(t))}).always(function(){r.isToggleInProgress(!1)})}var i=this,r;i.userId=n.autoMap();i.firstName=n.autoMap();i.lastName=n.autoMap();i.email=n.autoMap();i.organization=n.autoMap();i.primarySubjectArea=n.autoMap();i.secondarySubjectAreas=n.autoMap();i.quota=n.autoMap();i.trackSubmissionCount=n.autoMap();i.conferenceSubmissionCount=n.autoMap();i.userType=n.autoMap();i.isAssigned=ko.observable().autoMap();i.initialState=undefined;i.css=ko.observable("");i.isToggleInProgress=ko.observable(!1);u()}function r(t,i){var r=this;r.groupId=t;r.showAssignedOnly=ko.observable("false");r.showAssignedOnly.subscribe(r.loadData,r);r.metaReviewers=ko.observableArray([]);r.userTypes=i;r.userTypesProvider=function(){return r.userTypes};n.DataTable.call(r)}function f(i){var r=this;r.id=i;r.trackId=ko.observable().autoMap();r.track=ko.observable().autoMap();r.groupName=ko.observable().autoMap();r.isSingleTrackConference=ko.observable().autoMap();r.loadData=function(){var u=n.odata.getUrl(n.odata.entitySet.trackMetaReviewerGroups,i);return t.request({requestUri:u,showProgressIndicator:!1,method:"GET"},function(t){n.autoMap(r,t)})}}function e(t,u,e){var o=this;n.showProgress();o.metaReviewerGroup=new f(t);o.table=new r(t,e);ko.applyBindings(o,i.getElementById(u));$.when(o.table.loadData(!0),o.metaReviewerGroup.loadData()).then(function(){$("#"+u).show()}).always(n.hideProgress)}r.prototype=$.extend({},n.DataTable.prototype,{getStorageKey:function(){return"MetaReviewerGroupAssignMetaReviewers"},getDefaultSorting:function(){return{property:"IsAssigned",direction:"desc"}},loadData:function(i){var r,o,s;i=i===!0;r=this;i&&r.applyState();var e=r.sorting(),h=e?"&$orderby="+encodeURIComponent(e.property+" "+e.direction):"",c=r.skip()?"&$skip="+r.skip():"",l=r.top()?"&$top="+r.top():"",f="";return $.each(r.filters,function(n,t){t.getValue()&&(f+=f?" and "+t.getValue():t.getValue())}),r.showAssignedOnly()==="true"&&(f+=(f?" and":"")+" IsAssigned eq true"),f&&(f="&$filter="+encodeURIComponent(f)),o={method:"GET",headers:{Accept:"application/json"},requestUri:n.odata.getUrl(n.odata.entitySet.trackMetaReviewerGroups,r.groupId,"MetaReviewers")+"?$count=true"+f+h+c+l,showProgressIndicator:!i},s=t.request(o,function(t){var f,i,e,o;for(r.total(t["@odata.count"]||0),f=[],i=0;i<t.value.length;i++)e=t.value[i],o=n.autoMap(new u(r.groupId),e),f.push(o);r.metaReviewers(f);r.saveState()},function(t){n.addErrorMessage(n.odata.getErrorMessage(t))}),s}});n.metaReviewerGroupAssignMetaReviewers=function(n,t,i){new e(n,t,i)}}(window.app,window.OData,window.document),function(n,t,i){function u(){var i=this;i.id=n.autoMap();i.trackId=n.autoMap();i.trackName=n.autoMap();i.submissionId=n.autoMap();i.submissionTitle=n.autoMap();i.fileId=n.autoMap();i.fileName=n.autoMap();i.status=n.autoMap();i.percentMatch=n.autoMap();i.getSimilarityReport=function(){var r={method:"POST",headers:{Accept:"application/json","Content-Type":"application/json"},requestUri:n.odata.getUrl(n.odata.entitySet.iThenticateResults,i.id,"GetSimilarityReport"),showProgressIndicator:!0};t.request(r,function(n){window.location=n.value})}}function r(){var t=this;t.results=ko.observableArray([]);n.DataTable.call(t)}function f(t){var u=this;n.showProgress();u.table=new r;ko.applyBindings(u,document.getElementById(t));u.table.loadData(!0).done(function(){i("#"+t).show()}).always(n.hideProgress)}r.prototype=i.extend({},n.DataTable.prototype,{controller:n.odata.entitySet.iThenticateResults,getDefaultSorting:function(){return{property:"SubmissionId",direction:"asc"}},loadData:function(r){var f,s,h;r=r===!0;f=this;r&&f.applyState();var o=f.sorting(),c=o?"&$orderby="+encodeURIComponent(o.property+" "+o.direction):"",l=f.skip()?"&$skip="+f.skip():"",a=f.top()?"&$top="+f.top():"",e="";return i.each(f.filters,function(n,t){t.getValue()&&(e+=e?" and "+t.getValue():t.getValue())}),e&&(e="&$filter="+encodeURIComponent(e)),s={method:"GET",headers:{Accept:"application/json"},requestUri:n.odata.getUrl(f.controller)+"?$count=true"+e+c+l+a,showProgressIndicator:!r},h=t.request(s,function(t){var r,i;for(f.total(t["@odata.count"]||0),r=[],i=0;i<t.value.length;i++)r.push(n.autoMap(new u,t.value[i]));f.results(r);f.saveState()},function(t){n.addErrorMessage(n.odata.getErrorMessage(t))}),h}});n.iThenticateResultsPage=function(n){var t=new f(n)}}(window.app,window.OData,window.$),function(n){function t(){function u(){var i={requestUri:n.odata.getUrl(n.odata.entitySet.iThenticateRetrieveResults),showProgressIndicator:!1,method:"GET"};return OData.request(i,function(n){t.id(n.Id);t.startedAt(n.StartedAt);t.finishedAt(n.FinishedAt);t.pendingCount(n.PendingCount);t.doneCount(n.DoneCount);t.errorCount(n.ErrorCount)},function(i){if(i===n.enums.httpStatusCodes.failure.notFound){t.id(null);t.startedAt(null);t.finishedAt(null);t.pendingCount(null);t.doneCount(null);t.errorCount(null);return}})}function i(){u().done(function(){r=t.finished()?null:setTimeout(i,1e3)})}var r,t=this;t.id=ko.observable(null);t.startedAt=ko.observable(null);t.finishedAt=ko.observable(null);t.pendingCount=ko.observable(null);t.doneCount=ko.observable(null);t.errorCount=ko.observable(null);t.visible=ko.pureComputed(function(){return t.id()});t.finished=ko.pureComputed(function(){return t.id()&&t.finishedAt()});t.done=function(){var i={requestUri:n.odata.getUrl(n.odata.entitySet.iThenticateRetrieveResults,t.id()),showProgressIndicator:!1,method:"DELETE"};OData.request(i,function(){window.location.reload()})};t.refresh=function(){i()};i()}function i(i){var r=this;r.IThenticateRetrieveResultSession=ko.observable();r.progressDialog=new t;r.retrieveResults=function(){var t={requestUri:n.odata.getUrl(n.odata.entitySet.iThenticateRetrieveResults),showProgressIndicator:!1,method:"POST"};return OData.request(t).done(r.progressDialog.refresh)};ko.applyBindings(r,document.getElementById(i))}n.iThenticateRetrieveResultsPage=function(n){var t=new i(n)}}(window.app,window.OData,window.$),function(n){function t(){var n=this;n.successCount=ko.observable(null).autoMap();n.errorCount=ko.observable(null).autoMap();n.totalCount=ko.observable(null).autoMap();n.status=ko.observable(null).autoMap();n.finishedAt=ko.observable(null).autoMap();n.processedCount=ko.pureComputed(function(){return n.errorCount()+n.successCount()});n.percentage=ko.pureComputed(function(){var t=n.totalCount(),i=n.processedCount();return!t||i===null?null:Math.round(i/t*100)})}function i(){function f(){var r={requestUri:n.odata.getUrl(n.odata.entitySet.iThenticateSubmissions,null,"GetProgress"),showProgressIndicator:!1,method:"POST"};return OData.request(r,function(r){i.progress(n.autoMap(new t,r))},function(t){var r=t&&t.response&&t.response.statusCode;r===n.enums.httpStatusCodes.failure.notFound&&i.progress(null)})}function r(){f().done(function(){var n=i.progress()&&i.progress().finishedAt();u=n?null:setTimeout(r,1e3)})}var u,i=this;i.progress=ko.observable(null);i.visible=ko.pureComputed(function(){return i.progress()!=null});i.done=function(){var t={requestUri:n.odata.getUrl(n.odata.entitySet.iThenticateSubmissions,null,"ClearProgress"),showProgressIndicator:!1,method:"POST"};OData.request(t,function(){i.progress(null)})};i.refresh=function(){r()};r()}function r(){var t=this;t.trackId=n.autoMap();t.trackName=n.autoMap();t.statuses=n.autoMap()}function u(){var t=this;t.trackId=n.autoMap();t.trackName=n.autoMap();t.statusId=n.autoMap();t.statusName=n.autoMap();t.submissionsCount=n.autoMap();t.submissionFilesCount=n.autoMap();t.cameraReadyFilesCount=n.autoMap();t.checked=ko.observable(!1);t.isDisabled=ko.computed(function(){return t.submissionFilesCount<1})}function f(t){function f(){for(var t,n,u=i.tracks(),f=[],r=0;r<u.length;r++)for(t=u[r].statuses,n=0;n<t.length;n++)t[n].checked()&&!t[n].isDisabled()&&f.push({TrackId:t[n].trackId,StatusId:t[n].statusId,SendSubmissionFiles:!0});return f}function e(){var t={requestUri:n.odata.getUrl(n.odata.entitySet.iThenticateSubmissions),method:"GET"};return OData.request(t,function(t){for(var f,h,o=[],e={},s=0;s<t.value.length;s++)f=n.autoMap(new u,t.value[s]),e[f.trackId]?e[f.trackId].Statuses.push(f):e[f.trackId]={TrackId:f.trackId,TrackName:f.trackName,Statuses:[f]};for(h in e)e.hasOwnProperty(h)&&o.push(n.autoMap(new r,e[h]));o.sort(function(n,t){return n.trackId<t.trackId?-1:n.trackId>t.trackId?1:0});i.tracks(o)})}var i=this;i.progressViewModel=t;i.tracks=ko.observableArray([]);i.selectedCount=ko.computed(function(){return f().length});i.isSubmitDisabled=ko.computed(function(){return i.selectedCount()<1});i.isSingleTrackConference=ko.pureComputed(function(){return i.tracks().length<2});i.submit=function(){var t={requestUri:n.odata.getUrl(n.odata.entitySet.iThenticateSubmissions,null,"Send"),method:"POST",data:{Request:{Items:f()}}};return OData.request(t,function(){i.progressViewModel.refresh()})};e()}function e(){var n=this;n.progressDialog=new i;n.submissions=new f(n.progressDialog);n.submissionsVisible=ko.pureComputed(function(){return!n.progressDialog.visible()})}n.iThenticateSendSubmissions=function(n){ko.applyBindings(new e,document.getElementById(n))}}(window.app),function(n,t,i,r){function u(n,t,i){var r=this;r.id=ko.observable(0).autoMap();r.left=ko.observable(0).autoMap();r.right=ko.observable(0).autoMap();r.operator=ko.observable("").autoMap();r.leftTitle=ko.pureComputed(function(){var t=n[r.left()];return t&&t.title||"Unknown paper"});r.rightTitle=ko.pureComputed(function(){var t=n[r.right()];return t&&t.title||"Unknown paper"});r.operatorTitle=ko.pureComputed(function(){return t[r.operator()]});r.isEditable=ko.pureComputed(function(){var t=n[r.left()];return t&&i.has(t.id)})}function e(){var n=this;n.id=t.autoMap();n.title=t.autoMap()}function o(){var n=this;n.rowComparisons=ko.observableArray()}function f(n,t,i){var r=this;r.leftSubmissions=ko.pureComputed(function(){return(t||[]).map(function(t){return{id:t,title:n[t]&&n[t].title||"Unknown paper"}})});r.operatorTitle=i}function s(s,h,c){function w(t){var r=n(document.getElementById(t)),i=n.Deferred();r.find(".btn-primary").off("click").click(function(){i.resolve(!0);i=null;r.modal("hide")});r.on("hidden",function(){i&&i.resolve(!1)});return r.modal("show"),i.promise()}var l=this,a={},v={Comparable:"~",PreferredOver:">"},y=new Set,p=new Set(c);l.isEditing=ko.observable(!1);l.editViewModel=ko.observable(null);l.comparisons=ko.observableArray();l.submissions=ko.observableArray();l.toBeDeleted=ko.observable(null);l.aggregateComparisons=ko.observableArray();l.operators=ko.pureComputed(function(){return Object.keys(v).map(function(n){return{value:n,name:v[n]}})});l.add=function(){l.editViewModel(new u);l.isEditing(!0)};l.save=function(){l.aggregateComparisons([]);t.showProgress();var r=n.Deferred(),u=t.autoMap(l.editViewModel()),f={requestUri:t.odata.getUrl(h===t.enums.assignmentType.metaReviewer?t.odata.entitySet.metaReviewerSubmissionComparisons:t.odata.entitySet.reviewerSubmissionComparisons),method:"POST",showProgressIndicator:!1,headers:{Prefer:"return-content"},data:u};return i.request(f,function(){l.loadData(!1).done(function(){l.isEditing(!1);r.resolve()}).always(t.hideProgress)}).fail(t.hideProgress),r.promise()};l.delete=function(r){l.toBeDeleted(r);w(s).done(function(u){if(u){l.aggregateComparisons([]);t.showProgress();var f=n.Deferred(),e={requestUri:t.odata.getUrl(h===t.enums.assignmentType.metaReviewer?t.odata.entitySet.metaReviewerSubmissionComparisons:t.odata.entitySet.reviewerSubmissionComparisons,r.id()),showProgressIndicator:!1,method:"DELETE"};return i.request(e,function(){l.loadData(!1).done(function(){f.resolve()}).always(t.hideProgress)}).fail(t.hideProgress),f.promise()}})};l.showSummary=function(){var r={requestUri:t.odata.getUrl(h===t.enums.assignmentType.metaReviewer?t.odata.entitySet.metaReviewerSubmissionComparisons:t.odata.entitySet.reviewerSubmissionComparisons,null,"GetSummary"),method:"GET"};i.request(r,function(t){l.aggregateComparisons([]);var i=JSON.parse(t.value);n.each(i,function(n,t){for(var u,r=new o,i=0;i<t.length;i++)u=i==t.length-1?new f(a,t[i]):new f(a,t[i],">"),r.rowComparisons.push(u);l.aggregateComparisons.push(r)})})};l.loadData=function(f){var o={requestUri:"/api/odata/"+r.name+"/$batch",method:"POST",showProgressIndicator:f,data:{requests:[{url:t.odata.getUrl(h===t.enums.assignmentType.metaReviewer?t.odata.entitySet.metaReviewModels:t.odata.entitySet.reviewModels)+"?$select=Id,Title,TrackId",method:"GET",headers:{Accept:"application/json"}},{url:t.odata.getUrl(h===t.enums.assignmentType.metaReviewer?t.odata.entitySet.metaReviewerSubmissionComparisons:t.odata.entitySet.reviewerSubmissionComparisons),method:"GET",headers:{Accept:"application/json"}},]}};return i.request(o,function(i){var r=i&&i.responses&&i.responses[0]&&i.responses[0].body&&i.responses[0].body.value||[],f=i&&i.responses&&i.responses[1]&&i.responses[1].body&&i.responses[1].body.value||[];l.submissions([]);a={};y.clear();n.each(r,function(n,i){a[i.Id]=t.autoMap(new e,i);p.has(i.TrackId)&&(y.add(i.Id),l.submissions.push(a[i.Id]))});l.comparisons([]);n.each(f,function(n,i){l.comparisons.push(t.autoMap(new u(a,v,y),i))})})}}t.submissionComparison=function(n,t,i,r){var u=new s(t,i,r);u.loadData(!0).done(function(){ko.applyBindingsAndShow(u,n)})}}(window.jQuery,window.app,window.OData,window.cmt3.conference),function(n,t,i,r){"use strict";function u(){var n=this,t=!1;n.id=ko.observable(0).autoMap();n.name=ko.observable("").extend({required:!0}).autoMap();n.isEditing=ko.observable(!1);n.focus=function(){t=!0};n.isFocused=ko.pureComputed=function(){return t}}function f(){function e(){return i.read(t.odata.getUrl(t.odata.entitySet.tracks),function(i){var r=i&&i.value;n.each(r,function(n,i){var r=t.autoMap(new u,i);r.name.extend({trackChanges:!0});f.tracks.push(r)})})}var f=this;f.tracks=ko.observableArray([]);f.createNew=function(){if(confirm('Are you sure subject area is not the better option? Click "OK" only if you understand the complexity to manage tracks.')){var n=t.autoMap(new u,{});f.tracks.unshift(n);f.edit(n)}};f.edit=function(t){n.each(f.tracks(),function(n,i){i!==t&&f.cancel(i)});t.isEditing(!0);t.focus()};f.save=function(n){var f=ko.validation.group(n),u,e;if(f().length>0)return f.showAllMessages(),!1;u=t.autoMap(n);e={requestUri:t.odata.getUrl(t.odata.entitySet.tracks,u.Id),method:u.Id?"PATCH":"POST",headers:{Accept:"application/json"},data:u};i.request(e,function(){n.isEditing(!1);r.location.reload()})};f.delete=function(n){if(f.tracks().length==1){alert("Sorry, you cannot delete the only track in a conference.");return}if(confirm("Are you sure you want to delete this track?")){var u={requestUri:t.odata.getUrl(t.odata.entitySet.tracks,n.id()),method:"DELETE"};i.request(u,function(){r.location.reload()})}};f.cancel=function(n){if(n)if(n.id())n.name(n.name.originalValue),n.isEditing(!1);else{var t=f.tracks.indexOf(n);t>-1&&f.tracks.splice(t,1)}};f.bindTo=function(n){e().done(function(){ko.applyBindingsAndShow(f,n)})}}t.settingsTrackManagement=function(n){(new f).bindTo(n)}}(window.jQuery,window.app,window.OData,window),function(n,t,i){"use strict";function f(n,t){var i=this;i.hiddenNumber=n;i.reviewPreview=t}var u=function(n,i){var r=this;r.context=i;r.id=n.Id;r.reviewer=n.FirstName+" "+n.LastName;r.replyAuthor=n.ReplyAuthor;r.replyDate=n.ReplyDate;r.date=n.Date;r.topicId=n.TopicId;r.topic=n.Topic;r.message=n.Text.htmlMultiLineEncode();r.replying=ko.observable(!1);r.text=ko.observable();r.dateFormatted=function(){var n=r.date.toString();return n.substring(0,n.indexOf(".")).replace("T"," ")};r.replyDateFormatted=function(){if(r.replyDate){var n=r.replyDate.toString();return n.substring(0,n.indexOf(".")).replace("T"," ")}return""};r.deleteMessage=function(){if(r.id&&confirm("You will not be able to revert this action. Are you sure you want to delete the message?")){var n={requestUri:window.app.odata.getUrl(t.odata.entitySet.discussionMessages,null,"DeleteMessage"),method:"POST",data:{Id:r.id}};window.OData.request(n,function(){window.location.reload()},function(n){OData.defaultError(n)})}}},r;u.prototype={form:function(){var n=this;n.replying(!0)},reply:function(i,r){var u=this,o=u.context,f=n(r.target),e;t.disableLink(f);e={requestUri:window.app.odata.getUrl(t.odata.entitySet.discussionMessages,null,"Reply"),method:"POST",data:{TopicId:u.topicId,AnswerTo:u.id,Text:u.text()}};OData.request(e,function(){o.render();t.addMessage("Reply successfully saved.");t.enableLink(f)},function(n){t.addMessage(n.response.statusCode,"Error:","error");t.enableLink(f)})},cancel:function(){var n=this;n.text("");n.replying(!1)}};r=function(i){function u(){return OData.read(t.odata.getUrl(t.odata.entitySet.submissions,r.submissionId,"Reviews"),function(n){for(var o=[],i,h,e,u,f,c,l,a,v,y,s=0;s<n.value.length;s++){for(u=n.value[s],f=t.autoMap(new t.Review,u),i=0;i<u.Questions.length;i++){for(c=u.Questions[i],l=t.autoMap(new t.Question,c),h=0;h<c.Answers.length;h++)l.answers.push(t.autoMap(new t.QuestionAnswer,c.Answers[h]));f.questions.push(l)}for(i=0;i<u.Files.length;i++)a=u.Files[i],v=t.autoMap(new t.File,a),f.files.push(v);f.reviewerNumber>0?r._reviews.push(f):o.push(f)}for(y=r._reviews.length===0?1:r._reviews[r._reviews.length-1].reviewerNumber+1,e=0;e<o.length;e++)o[e].reviewerNumber=y++,r._reviews.push(o[e])})}var r=this;r.isCreatingNewTopic=ko.observable(!1);r.newTopicTitle=ko.observable("");r.newTopicText=ko.observable("");r.submissionId=parseInt(n("#sid").text());r._items=ko.observableArray();r._sort=ko.observable("Date desc");r._selected=ko.observable();r._filter=ko.observable("");r._reviewQuestions=i;r._reviewers=ko.observableArray();r._reviews=ko.observableArray();r.bindTo=function(n){r.render();ko.applyBindingsAndShow(r,n)};r.postNewTopic=function(i,u){var f=n(u.target),e;t.disableLink(f);e={requestUri:window.app.odata.getUrl(t.odata.entitySet.discussionMessages,null,"CreateTopic"),showProgressIndicator:!1,headers:{"Content-Type":"application/json"},method:"POST",data:{SubmissionId:r.submissionId,Title:r.newTopicTitle(),Description:r.newTopicText()}};OData.request(e,function(){r.render();r.isCreatingNewTopic(!1);r.newTopicTitle("");r.newTopicText("");t.addMessage("Topic successfully created.");t.enableLink(f)},function(n){t.addMessage(n.response.statusCode,"Error:","error");t.enableLink(f)})};r.cancelNewTopic=function(){r.isCreatingNewTopic(!1);r.newTopicTitle("");r.newTopicText("")};r.inlineReviewsLoaded=ko.observable(!1);r.inlineReviewsVisible=ko.observable(!1);r.toggleInlineReviews=function(){return r.inlineReviewsLoaded()?r.inlineReviewsVisible(!r.inlineReviewsVisible()):n.when(u()).done(function(){r.inlineReviewsLoaded(!0);r.inlineReviewsVisible(!0)}),!1}};r.prototype={render:function(){var r=this,e="&$orderby="+r._sort(),o=r.getFilter()!=""?"&$filter="+encodeURIComponent(r.getFilter()):"",s="$count=true"+e+o,h={method:"POST",requestUri:"/api/odata/"+i+"/$batch",headers:{Accept:"application/json"},data:{requests:[{method:"GET",url:"/api/odata/"+i.name+"/"+t.odata.entitySet.discussionMessages+"?id="+r.submissionId+"&"+s,headers:{Accept:"application/json"}},{method:"GET",url:t.odata.getUrl(t.odata.entitySet.reviewViews,null,"GetAggregatableReviews")+"(key="+r.submissionId+")",headers:{Accept:"application/json"}}]}};OData.request(h,function(t){var e=t&&t.responses&&t.responses[0]&&t.responses[0].body,l,o,a,s,v,h,i,y,p,w,b,k,c,d,g;if(e&&(l=e&&e["@odata.count"],o=e&&e.value,r._items([]),l&&r._selected(l),o&&n.inArray(o)&&(a=[],n.each(o,function(n,t){a.push(new u(t,r))}),r._items(a))),s=t&&t.responses&&t.responses[1]&&t.responses[1].body,s){for(v=s.value&&JSON.parse(s.value)||[],r._reviewers([]),k=[],h=0;h<v.length;h++){if(c=v[h],y=[],r._reviewQuestions&&r._reviewQuestions.length>0){for(w=c&&c.Question||[],p={},i=0;i<w.length;i++)b=w[i],p[b.QuestionOrder]=b;for(i=0;i<r._reviewQuestions.length;i++)d=r._reviewQuestions[i],y.push(p[d.Order])}g=new f(c.HiddenNumber,y);k.push(g)}r._reviewers(k)}},function(n){window.cmt3.logger.error("[batch] server side error: "+n.message)},OData.batchHandler)},getFilter:function(){var r=n(".search-box > input").val(),i,u;return r!="Search Discussion for text"&&r!=""?(i="",u=["Text","Topic","FirstName","LastName","Email"],n.each(u,function(n,u){i+=(i==""?"":" or ")+"contains(tolower("+u+"),tolower('"+t.odata.escapeParam(r)+"'))"}),i):""},sort:function(t,i){var f=this,r=n(i.target),u=r.attr("data-sort");(u==null||u==undefined)&&(r=n(r.context.parentNode),u=r.attr("data-sort"));r.hasClass("selected")?f._sort().match(" desc$")?(f._sort(u+" asc"),r.next().removeClass("icon-arrow-down"),r.next().addClass("icon-arrow-up")):(f._sort(u+" desc"),r.next().removeClass("icon-arrow-up"),r.next().addClass("icon-arrow-down")):(n("a[data-sort]").each(function(){n(this).next().removeClass("icon-arrow-up");n(this).next().removeClass("icon-arrow-down");n(this).removeClass("selected")}),r.next().removeClass("icon-arrow-down"),r.next().addClass("icon-arrow-up"),r.addClass("selected"),f._sort(u+" asc"));f.render()},search:function(n,t){var i=this;t.keyCode==13&&i.render()}};t.showDiscussion=function(n,t){new r(t).bindTo(n)}}(window.jQuery,window.app,window.cmt3.conference),function(n,t){function i(t,i,r){var u=this,t=t,e=null,f;i&&(f=t.availableFilters[i],f&&(e=new n.filtering[f.type](i,$.extend({},f.config,r))));u.filter=ko.observable(e);u.property=ko.observable(i);u.property.subscribe(function(i){if(i){var r=t.availableFilters[i];u.filter(new n.filtering[r.type](i,r.config))}});u.availableFilters=ko.pureComputed(function(){return Object.keys(t.availableFilters)});u.getFilterString=ko.pureComputed(function(){var n=u.filter();return n?u.filter().getFilterString():""})}function u(){var t=this;t.availableFilters={Id:{property:"Id",type:"NumericFilter"},Status:{property:"Status",type:"OptionsFilter",config:{options:["Awaiting Decision","Complete","Desk Reject"]}},Name:{property:"Name",type:"StringFilter"}};t.appliedFilters=ko.observableArray([new i(t,"Status",{operator:n.filtering.operators.is,value:"Awaiting Decision"})]);t.addFilter=function(){t.appliedFilters.push(new i(t))};t.updateFilter=function(){};t.removeFilter=function(n){var i=t.appliedFilters();i.splice(i.indexOf(n),1);t.appliedFilters(i)};t.getFilterString=function(){return t.appliedFilters().map(function(n){return n&&n.getFilterString()}).filter(function(n){return n&&n!==""}).join(" and ")}}function f(){var n=this;n.id=ko.observable().autoMap();n.title=ko.observable().autoMap();n.heading=ko.observable().autoMap();n.answers=ko.observableArray([]);n.details=null}function e(){var n=this;n.text=ko.observable().autoMap()}function r(){var t=this;t.id=n.autoMap();t.firstName=ko.observable().autoMap();t.lastName=ko.observable().autoMap();t.email=ko.observable().autoMap();t.organization=ko.observable().autoMap();t.textFormatted=ko.pureComputed(function(){return t.firstName()+" "+t.lastName()+" ("+t.organization()+") <"+t.email()+">"})}function o(t,i){function u(n){var t=n.match(/^(\d{1,2})\/(\d{1,2})\/(\d{4})$/),r;if(t){var u=parseInt(t[1],10),f=parseInt(t[2],10),i=parseInt(t[3],10);return u>12?null:(r=(new Date).getFullYear(),i<r||i>r+2)?null:new Date(i,u-1,f)}return null}var r=this,f;r.city=ko.observable().autoMap();r.country=ko.observable().autoMap();r.name=ko.observable().autoMap();r.shortName=ko.observable().extend({isEditable:!0}).autoMap();r.startDate=ko.observable().autoMap();r.endDate=ko.observable().autoMap();r.createSubmissionDeadline=ko.observable().autoMap();r.externalUrl=ko.observable().autoMap();r.logoBlobName=n.autoMap();r.Chairs=t;r.startDateFormatted=ko.pureComputed({read:function(){var n=r.startDate();return console.log(n),n&&n.format("mm/dd/yyyy")||null},write:function(n){var t=u(n);t&&(r.startDate(t),console.log(t))}});r.endDateFormatted=ko.pureComputed({read:function(){var n=r.endDate();return n&&n.format("mm/dd/yyyy")||null},write:function(n){var t=u(n);t&&r.endDate(t)}});r.createSubmissionDeadlineFormatted=ko.pureComputed({read:function(){var n=r.createSubmissionDeadline();return n&&n.format("mm/dd/yyyy")||null},write:function(n){var t=u(n);t&&r.createSubmissionDeadline(t)}});f=[];$.each(i||[],function(n,t){f.push(ko.observable(t))});r.tracks=ko.observableArray(f);r.addTrack=function(){r.tracks.push(ko.observable("Track "+(r.tracks().length+1)))};r.deleteTrack=function(n){var i,u,t,f;if(window.confirm("Are you sure?")){for(i=-1,u=r.tracks(),t=0;t<u.length;t++)if(f=u[t],typeof f=="function"&&f()===n){i=t;break}i!==-1&&r.tracks.splice(i,1)}}}function s(i){var r=this;r.id=n.autoMap();r.name=n.autoMap();r.status=n.autoMap();r.chairsJson=n.autoMap();r.chairs=ko.observableArray([]);r.requestors=ko.observableArray([]);r.questions=ko.observableArray([]);r.creationViewModel=ko.observable();r.isExpanded=ko.observable(!1);r.create=function(){var u,f,e;if(window.confirm("Are you sure?")){if(u=r.creationViewModel(),f=u.shortName().trim(),f.match(/(\S{1,})(\s{1,})(\S{1,})/)||!f.match(/(\d{4})/)){alert("Conference short name is invalid");return}return e={requestUri:n.odata.getGlobalUrl(n.odata.entitySet.conferenceRequests,null,"CreateConference"),method:"POST",data:{Request:{RequestId:r.id,ShortName:u.shortName().trim(),Name:u.name(),City:u.city(),Country:u.country(),StartDate:u.startDate(),EndDate:u.endDate(),CreateSubmissionDeadline:u.createSubmissionDeadline(),Chairs:u.Chairs,ExternalUrl:u.externalUrl(),LogoBlobName:u.logoBlobName,Tracks:u.tracks().map(function(n){return typeof n=="function"?n():null}).filter(function(n){return n!==null})}}},t.request(e,function(n){i.updateItem(r,n)})}};r.reject=function(){if(window.confirm("Are you sure?")){var u={requestUri:n.odata.getGlobalUrl(n.odata.entitySet.conferenceRequests,r.id,"Reject"),method:"POST"};t.request(u,function(n){i.updateItem(r,n)})}}}function h(){function c(){var r=i.filteringViewModel.getFilterString(),u="?$orderby=Created desc&$top=25",f;return r&&(u+="&$filter="+r),f={requestUri:n.odata.getGlobalUrl(n.odata.entitySet.conferenceRequests)+u},t.request(f)}function h(t){var u=n.autoMap(new s(i),t),p=n.autoMap(new o(t.ConferenceCreationModel.Chairs,t.ConferenceCreationModel.Tracks),t.ConferenceCreationModel),a,h,v,c,y,l;return u.creationViewModel(p),a=t.RequestorsJson&&JSON.parse(t.RequestorsJson),h=[],$.each(a,function(t,i){h.push(n.autoMap(new r,i))}),u.requestors(h),v=t.ChairsJson&&JSON.parse(t.ChairsJson),c=[],$.each(v,function(t,i){c.push(n.autoMap(new r,i))}),u.chairs(c),y=t.QuestionsJson&&JSON.parse(t.QuestionsJson),l=[],$.each(y,function(t,i){var r=n.autoMap(new f,i),o=i.Answers,u=[];$.each(o,function(t,i){u.push(n.autoMap(new e,i))});r.answers(u);l.push(r)}),u.questions(l),u}var i=this;i.filteringViewModel=new u;i.conferences=ko.observableArray([]);i.applyFilters=function(){i.reload()};i.reload=function(){return c().done(function(n){var t=[],r=n&&n.value||[];$.each(r,function(n,i){t.push(h(i))});i.conferences(t)})};i.updateItem=function(n,t){var u=i.conferences.indexOf(n),r;t?(r=h(t),i.conferences.splice(u,1,r)):i.reload()};i.initialize=function(n){i.reload().done(function(){ko.applyBindingsAndShow(i,n)})}}n.conferenceRequests=function(n){return(new h).initialize(n)}}(window.app,window.OData),function(n,t){function i(){var i=this;i.id=n.autoMap();i.firstName=n.autoMap();i.lastName=n.autoMap();i.email=n.autoMap();i.country=n.autoMap();i.reason=n.autoMap();i.status=n.autoMap();i.textFormatted=ko.pureComputed(function(){return i.firstName+" "+i.lastName+" <"+i.email+"> ("+i.country+")"});i.deleteAccount=function(){if(window.confirm("Are you sure?")){var r={requestUri:n.odata.getGlobalUrl(n.odata.entitySet.accountProcessingRequests,i.id,"Process"),method:"POST"};t.request(r,function(){window.location.reload();n.addMessage("Account deletion submitted for processing.")})}};i.cancelRequest=function(){if(window.confirm("Are you sure?")){var r={requestUri:n.odata.getGlobalUrl(n.odata.entitySet.accountProcessingRequests,i.id,"Cancel"),method:"POST"};t.request(r,function(){window.location.reload();n.addMessage("Account deletion request canceled.")})}}}function r(){function u(){return t.read(n.odata.getUrl(n.odata.entitySet.accountProcessingRequests),function(t){var u=[],f=t&&t.value||[];$.each(f,function(t,r){var f=n.autoMap(new i,r);u.push(f)});r.requests(u)})}var r=this;r.requests=ko.observableArray([]);r.bindTo=function(n){u().done(function(){ko.applyBindingsAndShow(r,n)})}}n.accountDeletionProcessing=function(n){return(new r).bindTo(n)}}(window.app,window.OData)

==> icde2022-reviews_files/json2 <==
var JSON;JSON||(JSON={}),(function(){"use strict";function i(n){return n<10?"0"+n:n}function f(n){return o.lastIndex=0,o.test(n)?'"'+n.replace(o,function(n){var t=s[n];return typeof t=="string"?t:"\\u"+("0000"+n.charCodeAt(0).toString(16)).slice(-4)})+'"':'"'+n+'"'}function r(i,e){var h,l,c,a,v=n,s,o=e[i];o&&typeof o=="object"&&typeof o.toJSON=="function"&&(o=o.toJSON(i)),typeof t=="function"&&(o=t.call(e,i,o));switch(typeof o){case"string":return f(o);case"number":return isFinite(o)?String(o):"null";case"boolean":case"null":return String(o);case"object":if(!o)return"null";n+=u,s=[];if(Object.prototype.toString.apply(o)==="[object Array]"){for(a=o.length,h=0;h<a;h+=1)s[h]=r(h,o)||"null";return c=s.length===0?"[]":n?"[\n"+n+s.join(",\n"+n)+"\n"+v+"]":"["+s.join(",")+"]",n=v,c}if(t&&typeof t=="object")for(a=t.length,h=0;h<a;h+=1)typeof t[h]=="string"&&(l=t[h],c=r(l,o),c&&s.push(f(l)+(n?": ":":")+c));else for(l in o)Object.prototype.hasOwnProperty.call(o,l)&&(c=r(l,o),c&&s.push(f(l)+(n?": ":":")+c));return c=s.length===0?"{}":n?"{\n"+n+s.join(",\n"+n)+"\n"+v+"}":"{"+s.join(",")+"}",n=v,c}}typeof Date.prototype.toJSON!="function"&&(Date.prototype.toJSON=function(){return isFinite(this.valueOf())?this.getUTCFullYear()+"-"+i(this.getUTCMonth()+1)+"-"+i(this.getUTCDate())+"T"+i(this.getUTCHours())+":"+i(this.getUTCMinutes())+":"+i(this.getUTCSeconds())+"Z":null},String.prototype.toJSON=Number.prototype.toJSON=Boolean.prototype.toJSON=function(){return this.valueOf()});var e=/[\u0000\u00ad\u0600-\u0604\u070f\u17b4\u17b5\u200c-\u200f\u2028-\u202f\u2060-\u206f\ufeff\ufff0-\uffff]/g,o=/[\\\"\x00-\x1f\x7f-\x9f\u00ad\u0600-\u0604\u070f\u17b4\u17b5\u200c-\u200f\u2028-\u202f\u2060-\u206f\ufeff\ufff0-\uffff]/g,n,u,s={"\b":"\\b","\t":"\\t","\n":"\\n","\f":"\\f","\r":"\\r",'"':'\\"',"\\":"\\\\"},t;typeof JSON.stringify!="function"&&(JSON.stringify=function(i,f,e){var o;n="",u="";if(typeof e=="number")for(o=0;o<e;o+=1)u+=" ";else typeof e=="string"&&(u=e);t=f;if(f&&typeof f!="function"&&(typeof f!="object"||typeof f.length!="number"))throw new Error("JSON.stringify");return r("",{"":i})}),typeof JSON.parse!="function"&&(JSON.parse=function(n,t){function r(n,i){var f,e,u=n[i];if(u&&typeof u=="object")for(f in u)Object.prototype.hasOwnProperty.call(u,f)&&(e=r(u,f),e!==undefined?u[f]=e:delete u[f]);return t.call(n,i,u)}var i;n=String(n),e.lastIndex=0,e.test(n)&&(n=n.replace(e,function(n){return"\\u"+("0000"+n.charCodeAt(0).toString(16)).slice(-4)}));if(/^[\],:{}\s]*$/.test(n.replace(/\\(?:["\\\/bfnrt]|u[0-9a-fA-F]{4})/g,"@").replace(/"[^"\\\n\r]*"|true|false|null|-?\d+(?:\.\d*)?(?:[eE][+\-]?\d+)?/g,"]").replace(/(?:^|:|,)(?:\s*\[)+/g,"")))return i=eval("("+n+")"),typeof t=="function"?r({"":i},""):i;throw new SyntaxError("JSON.parse");})})();


==> icde2022-reviews_files/knockoutValidation <==
!function(n){"function"==typeof require&&"object"==typeof exports&&"object"==typeof module?n(require("knockout"),exports):"function"==typeof define&&define.amd?define(["knockout","exports"],n):n(ko,ko.validation={})}(function(n,t){function c(n){var t="max"===n;return function(r,u){var o,h,s,f,e;if(i.utils.isEmptyVal(r))return!0;void 0===u.typeAttr?(h="text",o=u):(h=u.typeAttr,o=u.value);isNaN(o)||o instanceof Date||(h="number");switch(h.toLowerCase()){case"week":if(s=/^(\d{4})-W(\d{2})$/,f=r.match(s),null===f)throw new Error("Invalid value for "+n+" attribute for week input.  Should look like '2000-W33' http://www.w3.org/TR/html-markup/input.week.html#input.week.attrs.min");return e=o.match(s),e?t?f[1]<e[1]||f[1]===e[1]&&f[2]<=e[2]:f[1]>e[1]||f[1]===e[1]&&f[2]>=e[2]:!1;case"month":if(s=/^(\d{4})-(\d{2})$/,f=r.match(s),null===f)throw new Error("Invalid value for "+n+" attribute for month input.  Should look like '2000-03' http://www.w3.org/TR/html-markup/input.month.html#input.month.attrs.min");return e=o.match(s),e?t?f[1]<e[1]||f[1]===e[1]&&f[2]<=e[2]:f[1]>e[1]||f[1]===e[1]&&f[2]>=e[2]:!1;case"number":case"range":return t?!isNaN(r)&&parseFloat(r)<=parseFloat(o):!isNaN(r)&&parseFloat(r)>=parseFloat(o);default:return t?o>=r:r>=o}}}function y(n,t,r){return t.validator(n(),void 0===r.params?!0:f(r.params))?!0:(n.setError(i.formatMessage(r.message||t.message,f(r.params),n)),!1)}function p(n,t,r){n.isValidating(!0);var u=function(u){var e=!1,o="";return n.__valid__()?(u.message?(e=u.isValid,o=u.message):e=u,e||(n.error(i.formatMessage(o||r.message||t.message,f(r.params),n)),n.__valid__(e)),void n.isValidating(!1)):void n.isValidating(!1)};i.utils.async(function(){t.validator(n(),void 0===r.params?!0:f(r.params),u)})}var a,h,s,v;if("undefined"==typeof n)throw new Error("Knockout is required, please ensure it is loaded before loading this validation plug-in");n.validation=t;var i=n.validation,u=n.utils,f=u.unwrapObservable,e=u.arrayForEach,r=u.extend,l={registerExtenders:!0,messagesOnModified:!0,errorsAsTitle:!0,errorsAsTitleOnModified:!1,messageTemplate:null,insertMessages:!0,parseInputAttributes:!1,writeInputAttributes:!1,decorateInputElement:!1,decorateElementOnModified:!0,errorClass:null,errorElementClass:"validationElement",errorMessageClass:"validationMessage",allowHtmlMessages:!1,grouping:{deep:!1,observable:!0,live:!1},validate:{}},o=r({},l);o.html5Attributes=["required","pattern","min","max","step"];o.html5InputTypes=["email","number","date"];o.reset=function(){r(o,l)};i.configuration=o;i.utils=function(){var r=(new Date).getTime(),t={},n="__ko_validation__";return{isArray:function(n){return n.isArray||"[object Array]"===Object.prototype.toString.call(n)},isObject:function(n){return null!==n&&"object"==typeof n},isNumber:function(n){return!isNaN(n)},isObservableArray:function(n){return!!n&&"function"==typeof n.remove&&"function"==typeof n.removeAll&&"function"==typeof n.destroy&&"function"==typeof n.destroyAll&&"function"==typeof n.indexOf&&"function"==typeof n.replace},values:function(n){var t=[];for(var i in n)n.hasOwnProperty(i)&&t.push(n[i]);return t},getValue:function(n){return"function"==typeof n?n():n},hasAttribute:function(n,t){return null!==n.getAttribute(t)},getAttribute:function(n,t){return n.getAttribute(t)},setAttribute:function(n,t,i){return n.setAttribute(t,i)},isValidatable:function(n){return!!(n&&n.rules&&n.isValid&&n.isModified)},insertAfter:function(n,t){n.parentNode.insertBefore(t,n.nextSibling)},newId:function(){return r+=1},getConfigOptions:function(n){var t=i.utils.contextFor(n);return t||i.configuration},setDomData:function(r,u){var f=r[n];f||(r[n]=f=i.utils.newId());t[f]=u},getDomData:function(i){var r=i[n];if(r)return t[r]},contextFor:function(n){switch(n.nodeType){case 1:case 8:var t=i.utils.getDomData(n);if(t)return t;if(n.parentNode)return i.utils.contextFor(n.parentNode)}return void 0},isEmptyVal:function(n){return void 0===n?!0:null===n?!0:""===n?!0:void 0},getOriginalElementTitle:function(n){var t=i.utils.getAttribute(n,"data-orig-title"),r=n.title,u=i.utils.hasAttribute(n,"data-orig-title");return u?t:r},async:function(n){window.setImmediate?window.setImmediate(n):window.setTimeout(n,0)},forEach:function(n,t){if(i.utils.isArray(n))return e(n,t);for(var r in n)n.hasOwnProperty(r)&&t(n[r],r)}}}();a=function(){function c(n){e(n.subscriptions,function(n){n.dispose()});n.subscriptions=[]}function v(n){n.options.deep&&(e(n.flagged,function(n){delete n.__kv_traversed}),n.flagged.length=0);n.options.live||c(n)}function s(n,t){t.validatables=[];c(t);l(n,t);v(t)}function l(i,r,u){var e=[],f=i.peek?i.peek():i;i.__kv_traversed!==!0&&(r.options.deep&&(i.__kv_traversed=!0,r.flagged.push(i)),u=void 0!==u?u:r.options.deep?1:-1,n.isObservable(i)&&(i.errors||t.isValidatable(i)||i.extend({validatable:!0}),r.validatables.push(i),r.options.live&&t.isObservableArray(i)&&r.subscriptions.push(i.subscribe(function(){r.graphMonitor.valueHasMutated()}))),f&&!f._destroy&&(t.isArray(f)?e=f:t.isObject(f)&&(e=t.values(f))),0!==u&&t.forEach(e,function(t){!t||t.nodeType||n.isComputed(t)&&!t.rules||l(t,r,u+1)}))}function h(n){var i=[];return e(n,function(n){t.isValidatable(n)&&!n.isValid()&&i.push(n.error.peek())}),i}var a=0,o=i.configuration,t=i.utils;return{init:function(n,t){a>0&&!t||(n=n||{},n.errorElementClass=n.errorElementClass||n.errorClass||o.errorElementClass,n.errorMessageClass=n.errorMessageClass||n.errorClass||o.errorMessageClass,r(o,n),o.registerExtenders&&i.registerExtenders(),a=1)},reset:i.configuration.reset,group:function(i,f){f=r(r({},o.grouping),f);var l={options:f,graphMonitor:n.observable(),flagged:[],subscriptions:[],validatables:[]},c=null;return c=f.observable?n.computed(function(){return l.graphMonitor(),s(i,l),h(l.validatables)}):function(){return s(i,l),h(l.validatables)},c.showAllMessages=function(n){void 0===n&&(n=!0);c.forEach(function(i){t.isValidatable(i)&&i.isModified(n)})},c.isAnyMessageShown=function(){return!!c.find(function(n){return t.isValidatable(n)&&!n.isValid()&&n.isModified()})},c.filter=function(n){return n=n||function(){return!0},c(),u.arrayFilter(l.validatables,n)},c.find=function(n){return n=n||function(){return!0},c(),u.arrayFirst(l.validatables,n)},c.forEach=function(n){n=n||function(){};c();e(l.validatables,n)},c.map=function(n){return n=n||function(n){return n},c(),u.arrayMap(l.validatables,n)},c._updateState=function(n){if(!t.isObject(n))throw new Error("An object is required.");return i=n,f.observable?void l.graphMonitor.valueHasMutated():(s(n,l),h(l.validatables))},c},formatMessage:function(n,i,r){if(t.isObject(i)&&i.typeAttr&&(i=i.value),"function"==typeof n)return n(i,r);var u=f(i);return null==u&&(u=[]),t.isArray(u)||(u=[u]),n.replace(/{(\d+)}/gi,function(n,t){return"undefined"!=typeof u[t]?u[t]:n})},addRule:function(n,t){n.extend({validatable:!0});var i=!!u.arrayFirst(n.rules(),function(n){return n.rule&&n.rule===t.rule});return i||n.rules.push(t),n},addAnonymousRule:function(n,t){void 0===t.message&&(t.message="Error");t.onlyIf&&(t.condition=t.onlyIf);i.addRule(n,t)},addExtender:function(r){n.extenders[r]=function(n,u){return u&&(u.message||u.onlyIf)?i.addRule(n,{rule:r,message:u.message,params:t.isEmptyVal(u.params)?!0:u.params,condition:u.onlyIf}):i.addRule(n,{rule:r,params:u})}},registerExtenders:function(){if(o.registerExtenders)for(var t in i.rules)i.rules.hasOwnProperty(t)&&(n.extenders[t]||i.addExtender(t))},insertValidationMessage:function(n){var i=document.createElement("SPAN");return i.className=t.getConfigOptions(n).errorMessageClass,t.insertAfter(n,i),i},parseInputValidationAttributes:function(n,r){e(i.configuration.html5Attributes,function(u){var e,f;t.hasAttribute(n,u)&&(e=n.getAttribute(u)||!0,("min"===u||"max"===u)&&(f=n.getAttribute("type"),"undefined"!=typeof f&&f||(f="text"),e={typeAttr:f,value:e}),i.addRule(r(),{rule:u,params:e}))});var u=n.getAttribute("type");e(i.configuration.html5InputTypes,function(n){n===u&&i.addRule(r(),{rule:"date"===n?"dateISO":n,params:!0})})},writeInputValidationAttributes:function(t,r){var f=r(),o;f&&f.rules&&(o=f.rules(),e(i.configuration.html5Attributes,function(i){var r=u.arrayFirst(o,function(n){return n.rule&&n.rule.toLowerCase()===i.toLowerCase()});r&&n.computed({read:function(){var u=n.unwrap(r.params);"pattern"===r.rule&&u instanceof RegExp&&(u=u.source);t.setAttribute(i,u)},disposeWhenNodeIsRemoved:t})}),o=null)},makeBindingHandlerValidatable:function(t){var i=n.bindingHandlers[t].init;n.bindingHandlers[t].init=function(t,r,u,f,e){return i(t,r,u,f,e),n.bindingHandlers.validationCore.init(t,r,u,f,e)}},setRules:function(r,u){var e=function(r,u){var s,h,o,l;if(r&&u)for(s in u)if(u.hasOwnProperty(s)&&(h=u[s],r[s])){var a=r[s],c=f(a),y={},v={};for(o in h)h.hasOwnProperty(o)&&(i.rules[o]?y[o]=h[o]:v[o]=h[o]);if(n.isObservable(a)&&a.extend(y),c&&t.isArray(c))for(l=0;l<c.length;l++)e(c[l],v);else e(c,v)}};e(r,u)}}}();r(n.validation,a);i.rules={};i.rules.required={validator:function(n,t){var i;return void 0===n||null===n?!t:(i=n,"string"==typeof n&&(i=String.prototype.trim?n.trim():n.replace(/^\s+|\s+$/g,"")),t?(i+"").length>0:!0)},message:"This field is required."};i.rules.min={validator:c("min"),message:"Please enter a value greater than or equal to {0}."};i.rules.max={validator:c("max"),message:"Please enter a value less than or equal to {0}."};i.rules.minLength={validator:function(n,t){if(i.utils.isEmptyVal(n))return!0;var r=i.utils.isNumber(n)?""+n:n;return r.length>=t},message:"Please enter at least {0} characters."};i.rules.maxLength={validator:function(n,t){if(i.utils.isEmptyVal(n))return!0;var r=i.utils.isNumber(n)?""+n:n;return r.length<=t},message:"Please enter no more than {0} characters."};i.rules.pattern={validator:function(n,t){return i.utils.isEmptyVal(n)||null!==n.toString().match(t)},message:"Please check this value."};i.rules.step={validator:function(n,t){if(i.utils.isEmptyVal(n)||"any"===t)return!0;var r=100*n%(100*t);return Math.abs(r)<1e-5||Math.abs(1-r)<1e-5},message:"The value must increment by {0}."};i.rules.email={validator:function(n,t){return t?i.utils.isEmptyVal(n)||t&&/^((([a-z]|\d|[!#\$%&'\*\+\-\/=\?\^_`{\|}~]|[\u00A0-\uD7FF\uF900-\uFDCF\uFDF0-\uFFEF])+(\.([a-z]|\d|[!#\$%&'\*\+\-\/=\?\^_`{\|}~]|[\u00A0-\uD7FF\uF900-\uFDCF\uFDF0-\uFFEF])+)*)|((\x22)((((\x20|\x09)*(\x0d\x0a))?(\x20|\x09)+)?(([\x01-\x08\x0b\x0c\x0e-\x1f\x7f]|\x21|[\x23-\x5b]|[\x5d-\x7e]|[\u00A0-\uD7FF\uF900-\uFDCF\uFDF0-\uFFEF])|(\\([\x01-\x09\x0b\x0c\x0d-\x7f]|[\u00A0-\uD7FF\uF900-\uFDCF\uFDF0-\uFFEF]))))*(((\x20|\x09)*(\x0d\x0a))?(\x20|\x09)+)?(\x22)))@((([a-z]|\d|[\u00A0-\uD7FF\uF900-\uFDCF\uFDF0-\uFFEF])|(([a-z]|\d|[\u00A0-\uD7FF\uF900-\uFDCF\uFDF0-\uFFEF])([a-z]|\d|-|\.|_|~|[\u00A0-\uD7FF\uF900-\uFDCF\uFDF0-\uFFEF])*([a-z]|\d|[\u00A0-\uD7FF\uF900-\uFDCF\uFDF0-\uFFEF])))\.)+(([a-z]|[\u00A0-\uD7FF\uF900-\uFDCF\uFDF0-\uFFEF])|(([a-z]|[\u00A0-\uD7FF\uF900-\uFDCF\uFDF0-\uFFEF])([a-z]|\d|-|\.|_|~|[\u00A0-\uD7FF\uF900-\uFDCF\uFDF0-\uFFEF])*([a-z]|[\u00A0-\uD7FF\uF900-\uFDCF\uFDF0-\uFFEF])))$/i.test(n):!0},message:"Please enter a proper email address."};i.rules.date={validator:function(n,t){return t?i.utils.isEmptyVal(n)||t&&!/Invalid|NaN/.test(new Date(n)):!0},message:"Please enter a proper date."};i.rules.dateISO={validator:function(n,t){return t?i.utils.isEmptyVal(n)||t&&/^\d{4}[-/](?:0?[1-9]|1[012])[-/](?:0?[1-9]|[12][0-9]|3[01])$/.test(n):!0},message:"Please enter a proper date."};i.rules.number={validator:function(n,t){return t?i.utils.isEmptyVal(n)||t&&/^-?(?:\d+|\d{1,3}(?:,\d{3})+)?(?:\.\d+)?$/.test(n):!0},message:"Please enter a number."};i.rules.digit={validator:function(n,t){return t?i.utils.isEmptyVal(n)||t&&/^\d+$/.test(n):!0},message:"Please enter a digit."};i.rules.phoneUS={validator:function(n,t){return t?i.utils.isEmptyVal(n)?!0:"string"!=typeof n?!1:(n=n.replace(/\s+/g,""),t&&n.length>9&&n.match(/^(1-?)?(\([2-9]\d{2}\)|[2-9]\d{2})-?[2-9]\d{2}-?\d{4}$/)):!0},message:"Please specify a valid phone number."};i.rules.equal={validator:function(n,t){var r=t;return n===i.utils.getValue(r)},message:"Values must equal."};i.rules.notEqual={validator:function(n,t){var r=t;return n!==i.utils.getValue(r)},message:"Please choose another value."};i.rules.unique={validator:function(n,t){var r=i.utils.getValue(t.collection),e=i.utils.getValue(t.externalValue),f=0;return n&&r?(u.arrayFilter(r,function(i){n===(t.valueAccessor?t.valueAccessor(i):i)&&f++}),(e?1:2)>f):!0},message:"Please make sure the value is unique."},function(){i.registerExtenders()}();n.bindingHandlers.validationCore=function(){return{init:function(t,r){var u=i.utils.getConfigOptions(t),f=r(),e;(u.parseInputAttributes&&i.utils.async(function(){i.parseInputValidationAttributes(t,r)}),u.insertMessages&&i.utils.isValidatable(f))&&(e=i.insertValidationMessage(t),u.messageTemplate?n.renderTemplate(u.messageTemplate,{field:f},null,e,"replaceNode"):n.applyBindingsToNode(e,{validationMessage:f}));u.writeInputAttributes&&i.utils.isValidatable(f)&&i.writeInputValidationAttributes(t,r);u.decorateInputElement&&i.utils.isValidatable(f)&&n.applyBindingsToNode(t,{validationElement:f})}}}();i.makeBindingHandlerValidatable("value");i.makeBindingHandlerValidatable("checked");n.bindingHandlers.textInput&&i.makeBindingHandlerValidatable("textInput");i.makeBindingHandlerValidatable("selectedOptions");n.bindingHandlers.validationMessage={update:function(t,r){var e=r(),s=i.utils.getConfigOptions(t),h=(f(e),!1),c=!1,o,l,a;if(null===e||"undefined"==typeof e)throw new Error("Cannot bind validationMessage to undefined value. data-bind expression: "+t.getAttribute("data-bind"));h=e.isModified&&e.isModified();c=e.isValid&&e.isValid();o=null;(!s.messagesOnModified||h)&&(o=c?null:e.error);l=!s.messagesOnModified||h?!c:!1;a="none"!==t.style.display;s.allowHtmlMessages?u.setHtml(t,o):n.bindingHandlers.text.update(t,function(){return o});a&&!l?t.style.display="none":!a&&l&&(t.style.display="")}};n.bindingHandlers.validationElement={update:function(t,r,u){var e=r(),o=i.utils.getConfigOptions(t),h=(f(e),!1),s=!1,c;if(null===e||"undefined"==typeof e)throw new Error("Cannot bind validationElement to undefined value. data-bind expression: "+t.getAttribute("data-bind"));h=e.isModified&&e.isModified();s=e.isValid&&e.isValid();c=function(){var n={},t=!o.decorateElementOnModified||h?!s:!1;return n[o.errorElementClass]=t,n};n.bindingHandlers.css.update(t,c,u);o.errorsAsTitle&&n.bindingHandlers.attr.update(t,function(){var n=!o.errorsAsTitleOnModified||h,r=i.utils.getOriginalElementTitle(t);return n&&!s?{title:e.error,"data-orig-title":r}:!n||s?{title:r,"data-orig-title":null}:void 0})}};n.bindingHandlers.validationOptions=function(){return{init:function(n,t){var e=f(t()),u;e&&(u=r({},i.configuration),r(u,e),i.utils.setDomData(n,u))}}}();n.extenders.validation=function(n,t){return e(i.utils.isArray(t)?t:[t],function(t){i.addAnonymousRule(n,t)}),n};n.extenders.validatable=function(t,u){var o,f,s,e;return(i.utils.isObject(u)||(u={enable:u}),"enable"in u||(u.enable=!0),u.enable&&!i.utils.isValidatable(t))?(o=i.configuration.validate||{},f={throttleEvaluation:u.throttle||o.throttle},t.error=n.observable(null),t.rules=n.observableArray(),t.isValidating=n.observable(!1),t.__valid__=n.observable(!0),t.isModified=n.observable(!1),t.isValid=n.computed(t.__valid__),t.setError=function(n){var i=t.error.peek(),r=t.__valid__.peek();t.error(n);t.__valid__(!1);i===n||r||t.isValid.notifySubscribers()},t.clearError=function(){return t.error(null),t.__valid__(!0),t},s=t.subscribe(function(){t.isModified(!0)}),e=n.computed(r({read:function(){return t(),t.rules(),i.validateObservable(t),!0}},f)),r(e,f),t._disposeValidation=function(){t.isValid.dispose();t.rules.removeAll();s.dispose();e.dispose();delete t.rules;delete t.error;delete t.isValid;delete t.isValidating;delete t.__valid__;delete t.isModified;delete t.setError;delete t.clearError;delete t._disposeValidation}):u.enable===!1&&t._disposeValidation&&t._disposeValidation(),t};i.validateObservable=function(n){for(var r,t,u=0,f=n.rules(),e=f.length;e>u;u++)if(t=f[u],!t.condition||t.condition())if(r=t.rule?i.rules[t.rule]:t,r.async||t.async)p(n,r,t);else if(!y(n,r,t))return!1;return n.clearError(),!0};s={};i.defineLocale=function(n,t){return n&&t?(s[n.toLowerCase()]=t,t):null};i.locale=function(n){if(n){if(n=n.toLowerCase(),!s.hasOwnProperty(n))throw new Error("Localization "+n+" has not been loaded.");i.localize(s[n]);h=n}return h};i.localize=function(n){var r=i.rules;for(var t in n)r.hasOwnProperty(t)&&(r[t].message=n[t])},function(){var r={},n=i.rules;for(var t in n)n.hasOwnProperty(t)&&(r[t]=n[t].message);i.defineLocale("en-us",r)}();h="en-us";n.applyBindingsWithValidation=function(t,u,f){var e,o=document.body;u&&u.nodeType?(o=u,e=f):e=u;i.init();e&&(e=r(r({},i.configuration),e),i.utils.setDomData(o,e));n.applyBindings(t,o)};v=n.applyBindings;n.applyBindings=function(n,t){i.init();v(n,t)};n.validatedObservable=function(t,r){if(!r&&!i.utils.isObject(t))return n.observable(t).extend({validatable:!0});var u=n.observable(t);return u.errors=i.group(i.utils.isObject(t)?t:{},r),u.isValid=n.observable(0===u.errors().length),n.isObservable(u.errors)?u.errors.subscribe(function(n){u.isValid(0===n.length)}):n.computed(u.errors).subscribe(function(n){u.isValid(0===n.length)}),u.subscribe(function(n){i.utils.isObject(n)||(n={});u.errors._updateState(n);u.isValid(0===u.errors().length)}),u}})

==> icde2022-reviews_files/odatajs <==
/*
 * Licensed to the Apache Software Foundation (ASF) under one
 * or more contributor license agreements.  See the NOTICE file
 * distributed with this work for additional information
 * regarding copyright ownership.  The ASF licenses this file
 * to you under the Apache License, Version 2.0 (the
 * "License"); you may not use this file except in compliance
 * with the License.  You may obtain a copy of the License at
 *
 *   http://www.apache.org/licenses/LICENSE-2.0
 *
 * Unless required by applicable law or agreed to in writing,
 * software distributed under the License is distributed on an
 * "AS IS" BASIS, WITHOUT WARRANTIES OR CONDITIONS OF ANY
 * KIND, either express or implied.  See the License for the
 * specific language governing permissions and limitations
 * under the License.
 */

!function(){var a=function(a,b,c){a.version={major:4,minor:0,build:2},a.deferred=c("./lib/deferred.js"),a.utils=c("./lib/utils.js"),a.xml=c("./lib/xml.js"),a.oData=c("./lib/odata.js"),a.store=c("./lib/store.js"),a.cache=c("./lib/cache.js")},b={cache:function(a,b,c){"use strict";function d(a,b){var c=e(a,b),d=0,f=0;c&&(d=c.i-b.i,f=d+(a.c-A(a.d))),a.d=C(a.d,B(b.d,d,f))}function e(a,b){var c,d=a.i+a.c,e=b.i+b.c,f=a.i>b.i?a.i:b.i,g=d<e?d:e;return g>=f&&(c={i:f,c:g-f}),c}function f(a,b){if(void 0===a||"number"!=typeof a)throw{message:"'"+b+"' must be a number."};if(isNaN(a)||a<0||!isFinite(a))throw{message:"'"+b+"' must be greater than or equal to zero."}}function g(a,b){if(void 0!==a){if("number"!=typeof a)throw{message:"'"+b+"' must be a number."};if(isNaN(a)||a<=0||!isFinite(a))throw{message:"'"+b+"' must be greater than zero."}}}function h(a,b){if(void 0!==a&&("number"!=typeof a||isNaN(a)||!isFinite(a)))throw{message:"'"+b+"' must be a number."}}function i(a,b){var c,d;for(c=0,d=a.length;c<d;c++)if(a[c]===b)return a.splice(c,1),!0;return!1}function j(a){var b=0,c=typeof a;if("object"===c&&a)for(var d in a)b+=2*d.length+j(a[d]);else b="string"===c?2*a.length:8;return b}function k(a,b,c){return a=Math.floor(a/c)*c,b=Math.ceil((b+1)/c)*c,{i:a,c:b-a}}function l(a,b,c,d,e,f,g){var h,i,j=this;j.p=b,j.i=d,j.c=e,j.d=f,j.s=M,j.canceled=!1,j.pending=g,j.oncomplete=null,j.cancel=function(){if(c){var a=j.s;a!==L&&a!==K&&a!==J&&(j.canceled=!0,j.transition(J,h))}},j.complete=function(){v(j.s!==K,"DataCacheOperation.complete() - operation is in the end state",j),j.transition(K,h)},j.error=function(a){j.canceled||(v(j.s!==K,"DataCacheOperation.error() - operation is in the end state",j),v(j.s!==L,"DataCacheOperation.error() - operation is in the error state",j),j.transition(L,a))},j.run=function(a){i=a,j.transition(j.s,h)},j.wait=function(a){v(j.s!==K,"DataCacheOperation.wait() - operation is in the end state",j),j.transition(N,a)};var k=function(b,c,d){switch(b){case M:c!==F&&a(j,b,c,d);break;case N:a(j,b,c,d);break;case J:a(j,b,c,d),j.fireCanceled(),j.transition(K);break;case L:a(j,b,c,d),j.canceled=!0,j.fireRejected(d),j.transition(K);break;case K:j.oncomplete&&j.oncomplete(j),j.canceled||j.fireResolved(),a(j,b,c,d);break;default:var e=a(j,b,c,d);v(e,"Bad operation state: "+b+" cacheState: "+c,this)}};return j.transition=function(a,b){j.s=a,h=b,k(a,i,b)},j}function m(a){var b,c=F,e={counts:0,netReads:0,prefetches:0,cacheReads:0},g=[],h=[],m=[],n=0,p=!1,B=x(a.cacheSize,1048576),C=0,L=0,N=0,T=0===B,U=x(a.pageSize,50),V=x(a.prefetchSize,U),W="1.0",X=0,Y=a.source;"string"==typeof Y&&(Y=new r.ODataCacheSource(a)),Y.options=a;var Z=q.createStore(a.name,a.mechanism),$=this;$.onidle=a.idle,$.stats=e,$.count=function(){if(b)throw b;var a=y(),c=!1;if(p)return t(function(){a.resolve(C)}),a.promise();var d=Y.count(function(b){d=null,e.counts++,a.resolve(b)},function(b){d=null,a.reject(u(b,{canceled:c}))});return u(a.promise(),{cancel:function(){d&&(c=!0,d.abort(),d=null)}})},$.clear=function(){if(b)throw b;if(0===g.length){var a=y(),c=new l(oa,a,!1);return ha(c,g),a.promise()}return g[0].p},$.filterForward=function(a,b,c){return ea(a,b,c,!1)},$.filterBack=function(a,b,c){return ea(a,b,c,!0)},$.readRange=function(a,c){if(f(a,"index"),f(c,"count"),b)throw b;var d=y(),e=new l(qa,d,!0,a,c,{},0);return ha(e,h),u(d.promise(),{cancel:function(){e.cancel()}})},$.ToObservable=$.toObservable=function(){if(!o.inBrowser())throw{message:"Only in broser supported"};if(!window.Rx||!window.Rx.Observable)throw{message:"Rx library not available - include rx.js"};if(b)throw b;return new window.Rx.Observable(function(a){var b=!1,c=0,d=function(c){b||a.onError(c)},e=function(f){if(!b){var g,h;for(g=0,h=f.value.length;g<h;g++)a.onNext(f.value[g]);f.value.length<U?a.onCompleted():(c+=U,$.readRange(c,U).then(e,d))}};return $.readRange(c,U).then(e,d),{Dispose:function(){a.dispose(),b=!0}}})};var _=function(a){return function(c){b={message:a,error:c},v(0===m.length,"prefetchOperations.length === 0");var d,e;for(d=0,e=h.length;d<e;d++)h[d].fireRejected(b);for(d=0,e=g.length;d<e;d++)g[d].fireRejected(b);h=g=null}},aa=function(a){if(a!==c){c=a;var b,d,e=g.concat(h,m);for(b=0,d=e.length;b<d;b++)e[b].run(c)}},ba=function(){v(c===D||c===F,"DataCache.clearStore() - cache is not on the destroy or initialize state, current sate = "+c);var a=new z;return Z.clear(function(){n=0,p=!1,C=0,L=0,N=0,T=0===B,e={counts:0,netReads:0,prefetches:0,cacheReads:0},$.stats=e,Z.close(),a.resolve()},function(b){a.reject(b)}),a},ca=function(a){var b=i(g,a);b||(b=i(h,a))||i(m,a),X--,aa(E)},da=function(a){v(c!==D,"DataCache.fetchPage() - cache is on the destroy state"),v(c!==E,"DataCache.fetchPage() - cache is on the idle state");var b=new z,d=!1,e=Y.read(a,U,function(c){var d=A(c),e={i:a,c:d,d:c};b.resolve(e)},function(a){b.reject(a)});return u(b,{cancel:function(){e&&(e.abort(),d=!0,e=null)}})},ea=function(a,c,d,e){if(a=w(a),c=w(c),isNaN(a))throw{message:"'index' must be a valid number.",index:a};if(isNaN(c))throw{message:"'count' must be a valid number.",count:c};if(b)throw b;a=Math.max(a,0);var f=y(),g={};g.value=[];var h=!1,i=null,j=function(a,b){h||(c>0&&g.value.length>=c?f.resolve(g):i=$.readRange(a,b).then(function(h){h["@odata.context"]&&!g["@odata.context"]&&(g["@odata.context"]=h["@odata.context"]);for(var i=0,k=h.value.length;i<k&&(c<0||g.value.length<c);i++){var l=e?k-i-1:i,m=h.value[l];if(d(m)){var n={index:a+l,item:m};e?g.value.unshift(n):g.value.push(n)}}if(!e&&h.value.length<b||e&&a<=0)f.resolve(g);else{var o=e?Math.max(a-U,0):a+b;j(o,U)}},function(a){f.reject(a)}))},l=k(a,a,U),m=e?l.i:a,n=e?a-l.i+1:l.i+l.c-a;return j(m,n),u(f.promise(),{cancel:function(){i&&i.cancel(),h=!0}})},fa=function(){$.onidle&&0===X&&$.onidle()},ga=function(a){if(!p&&0!==V&&!T&&(v(c===G,"DataCache.prefetch() - cache is not on the read state, current state: "+c),0===m.length||m[0]&&-1!==m[0].c)){var b=new l(pa,null,!0,a,V,null,V);ha(b,m)}},ha=function(a,b){a.oncomplete=ca,b.push(a),X++,a.run(c)},ia=function(a){v(c!==D,"DataCache.readPage() - cache is on the destroy state");var b=!1,d=u(new z,{cancel:function(){b=!0}}),e=la(d,"Read page from store failure");return Z.contains(a,function(c){if(!b)return c?void Z.read(a,function(a,c){b||d.resolve(void 0!==c,c)},e):void d.resolve(!1)},e),d},ja=function(a,b){v(c!==D,"DataCache.savePage() - cache is on the destroy state"),v(c!==E,"DataCache.savePage() - cache is on the idle state");var d=!1,e=u(new z,{cancel:function(){d=!0}}),f=la(e,"Save page to store failure"),g=function(){e.resolve(!0)};if(b.c>0){var h=j(b);T=B>=0&&B<n+h,T?g():Z.addOrUpdate(a,b,function(){ma(b,h),ka(g,f)},f)}else ma(b,0),ka(g,f);return e},ka=function(a,b){var c={actualCacheSize:n,allDataLocal:p,cacheSize:B,collectionCount:C,highestSavedPage:L,highestSavedPageSize:N,pageSize:U,sourceId:Y.identifier,version:W};Z.addOrUpdate("__settings",c,a,b)},la=function(a){return function(){a.resolve(!1)}},ma=function(a,b){var c=a.c,d=a.i;0===c?L===d-U&&(C=L+N):(L=Math.max(L,d),L===d&&(N=c),n+=b,c<U&&!C&&(C=d+c)),p||C!==L+N||(p=!0)},na=function(a,b,c,d){var e=a.canceled&&b!==K;return e&&b===J&&d&&d.cancel&&d.cancel(),e},oa=function(a,b,c){var d=a.transition;if(c!==D)return aa(D),!0;switch(b){case M:d(O);break;case K:fa();break;case O:ba().then(function(){a.complete()}),a.wait();break;default:return!1}return!0},pa=function(a,b,c,d){if(!na(a,b,c,d)){var e=a.transition;if(c!==H)return c===D?b!==J&&a.cancel():c===E&&aa(H),!0;switch(b){case M:m[0]===a&&e(Q,a.i);break;case P:var f=a.pending;f>0&&(f-=Math.min(f,d.c)),p||0===f||d.c<U||T?a.complete():(a.pending=f,e(Q,d.i+U));break;default:return ra(a,b,c,d,!0)}}return!0},qa=function(a,b,f,g){if(!na(a,b,f,g)){var h=a.transition;if(f!==G&&b!==M)return f===D?b!==M&&a.cancel():f!==I&&(v(c==E||c===H,"DataCache.readStateMachine() - cache is not on the read or idle state."),aa(G)),!0;switch(b){case M:if(f===E||f===H)if(aa(G),a.c>=0){var i=k(a.i,a.c,U);h(Q,i.i)}else h(P,a);break;case P:d(a,g);var j=A(a.d);a.c===j||g.c<U?(e.cacheReads++,ga(g.i+g.c),a.complete()):h(Q,g.i+U);break;default:return ra(a,b,f,g,!1)}}return!0},ra=function(a,b,c,d,f){var g,h=a.error,i=a.transition,j=a.wait;switch(b){case K:fa();break;case Q:g=ia(d).then(function(b,c){a.canceled||(b?i(P,c):i(S,d))});break;case S:g=da(d).then(function(b){a.canceled||(f?e.prefetches++:e.netReads++,i(R,b))},h);break;case R:c!==I&&(aa(I),g=ja(d.i,d).then(function(b){a.canceled||(!b&&f&&(a.pending=0),i(P,d)),aa(E)}));break;default:return!1}return g&&(a.canceled?g.cancel():a.s===b&&j(g)),!0};return Z.read("__settings",function(a,b){if(s(b)){var c=b.version;if(!c||0!==c.indexOf("1."))return void _("Unsupported cache store version "+c)();U!==b.pageSize||Y.identifier!==b.sourceId?ba().then(function(){aa(E)},_("Unable to clear store during initialization")):(n=b.actualCacheSize,p=b.allDataLocal,B=b.cacheSize,C=b.collectionCount,L=b.highestSavedPage,N=b.highestSavedPageSize,W=c,aa(E))}else ka(function(){aa(E)},_("Unable to write settings during initialization."))},_("Unable to read settings from store.")),$}function n(a){if(g(a.pageSize,"pageSize"),h(a.cacheSize,"cacheSize"),h(a.prefetchSize,"prefetchSize"),!s(a.name))throw{message:"Undefined or null name",options:a};if(!s(a.source))throw{message:"Undefined source",options:a};return new m(a)}var o=c("./utils.js"),p=c("./deferred.js"),q=c("./store.js"),r=c("./cache/source.js"),s=o.assigned,t=o.delay,u=o.extend,v=o.djsassert,w=(o.isArray,o.normalizeURI,o.parseInt10),x=o.undefinedDefault,y=p.createDeferred,z=p.DjsDeferred,A=o.getJsonValueArraryLength,B=o.sliceJsonValueArray,C=o.concatJsonValueArray,D="destroy",E="idle",F="init",G="read",H="prefetch",I="write",J="cancel",K="end",L="error",M="start",N="wait",O="clear",P="done",Q="local",R="save",S="source";l.prototype.fireResolved=function(){var a=this.p;a&&(this.p=null,a.resolve(this.d))},l.prototype.fireRejected=function(a){var b=this.p;b&&(this.p=null,b.reject(a))},l.prototype.fireCanceled=function(){this.fireRejected({canceled:!0,message:"Operation canceled"})},a.estimateSize=j,a.createDataCache=n},source:function(a,b,c){"use strict";function d(a,b){return a+(a.indexOf("?")>=0?"&":"?")+b}function e(a,b){var c=a.indexOf("?"),d="";return c>=0&&(d=a.substr(c),a=a.substr(0,c)),"/"!==a[a.length-1]&&(a+="/"),a+b+d}function f(a,b){return{method:"GET",requestUri:a,user:b.user,password:b.password,enableJsonpCallback:b.enableJsonpCallback,callbackParameterName:b.callbackParameterName,formatQueryString:b.formatQueryString}}function g(a,b,c,d){return h(a,b,{},c,d)}function h(a,b,c,d,e){var g=f(a,b),i=k.request(g,function(f){var g=f["@odata.nextLink"];if(g){var j=a.indexOf(".svc/",0);-1!=j&&(g=a.substring(0,j+5)+g)}if(c.value&&f.value)c.value=c.value.concat(f.value);else for(var k in f)"@odata.nextLink"!=k&&(c[k]=f[k]);g?i=h(g,b,c,d,e):d(c)},e,void 0,b.httpClient,b.metadata);return{abort:function(){i.abort()}}}function i(a){var b=this,c=a.source;return b.identifier=m(encodeURI(decodeURI(c))),b.options=a,b.count=function(a,d){var g=b.options;return k.request(f(e(c,"$count"),g),function(b){var c=l(b.toString());isNaN(c)?d({message:"Count is NaN",count:c}):a(c)},d,void 0,g.httpClient,g.metadata)},b.read=function(a,e,f,h){return g(d(c,"$skip="+a+"&$top="+e),b.options,f,h)},b}var j=c("./../utils.js"),k=c("./../odata.js"),l=j.parseInt10,m=j.normalizeURICase;a.ODataCacheSource=i},deferred:function(a,b,c){"use strict";function d(a,b,c){return function(){return a[b].apply(a,arguments),c}}function e(){this._arguments=void 0,this._done=void 0,this._fail=void 0,this._resolved=!1,this._rejected=!1}function f(){return window.jQuery&&window.jQuery.Deferred?new window.jQuery.Deferred:new e}e.prototype={then:function(a,b){return a&&(this._done?this._done.push(a):this._done=[a]),b&&(this._fail?this._fail.push(b):this._fail=[b]),this._resolved?this.resolve.apply(this,this._arguments):this._rejected&&this.reject.apply(this,this._arguments),this},resolve:function(){if(this._done){var a,b;for(a=0,b=this._done.length;a<b;a++)this._done[a].apply(null,arguments);this._done=void 0,this._resolved=!1,this._arguments=void 0}else this._resolved=!0,this._arguments=arguments},reject:function(){if(this._fail){var a,b;for(a=0,b=this._fail.length;a<b;a++)this._fail[a].apply(null,arguments);this._fail=void 0,this._rejected=!1,this._arguments=void 0}else this._rejected=!0,this._arguments=arguments},promise:function(){var a={};return a.then=d(this,"then",a),a}},a.createDeferred=f,a.DjsDeferred=e},odata:function(a,b,c){"use strict";function d(a,b,c){var d,e;for(d=0,e=o.length;d<e&&!o[d][a](b,c);d++);if(d===e)throw{message:"no handler for data"}}var e=a.utils=c("./odata/odatautils.js"),f=a.handler=c("./odata/handler.js"),g=a.metadata=c("./odata/metadata.js"),h=a.net=c("./odata/net.js"),i=a.json=c("./odata/json.js");a.batch=c("./odata/batch.js");var j=c("./utils.js"),k=j.assigned,l=(j.defined,j.throwErrorCallback),m=(e.invokeRequest,f.MAX_DATA_SERVICE_VERSION),n=(e.prepareRequest,g.metadataParser),o=[i.jsonHandler,f.textHandler];a.defaultSuccess=function(a){window.alert(window.JSON.stringify(a))},a.defaultError=l,a.defaultHandler={read:function(a,b){a&&k(a.body)&&a.headers["Content-Type"]&&d("read",a,b)},write:function(a,b){d("write",a,b)},maxDataServiceVersion:m,accept:"application/json;q=0.9, */*;q=0.1"},a.defaultMetadata=[],a.read=function(b,c,d,e,f,g){var h;return h=b instanceof String||"string"==typeof b?{requestUri:b}:b,a.request(h,c,d,e,f,g)},a.request=function(b,c,d,f,g,k){c=c||a.defaultSuccess,d=d||a.defaultError,f=f||a.defaultHandler,g=g||h.defaultHttpClient,k=k||a.defaultMetadata,b.recognizeDates=j.defined(b.recognizeDates,i.jsonHandler.recognizeDates),b.callbackParameterName=j.defined(b.callbackParameterName,g.callbackParameterName,h.defaultHttpClient.callbackParameterName),b.formatQueryString=j.defined(b.formatQueryString,g.formatQueryString,h.defaultHttpClient.formatQueryString),b.enableJsonpCallback=j.defined(b.enableJsonpCallback,g.enableJsonpCallback,h.defaultHttpClient.enableJsonpCallback);var l={metadata:k,recognizeDates:b.recognizeDates,callbackParameterName:b.callbackParameterName,formatQueryString:b.formatQueryString,enableJsonpCallback:b.enableJsonpCallback};try{return e.prepareRequest(b,f,l),e.invokeRequest(b,c,d,f,g,l)}catch(a){if(a.bIsSuccessHandlerError)throw a;d(a)}},a.parseMetadata=function(a){return n(null,a)},a.batch.batchHandler.partHandler=a.defaultHandler,a.metadataHandler=g.metadataHandler,a.jsonHandler=i.jsonHandler},batch:function(a,b,c){"use strict";function d(){return Math.floor(65536*(1+Math.random())).toString(16).substr(1)}function e(a){return a+d()+"-"+d()+"-"+d()}function f(a){return a.handler.partHandler}function g(a){var b=a.boundaries;return b[b.length-1]}function h(a,b,c){return{__batchResponses:j(b,{boundaries:[c.contentType.properties.boundary],handlerContext:c})}}function i(a,b,c){if((c.contentType=c.contentType||x(D)).mediaType===D)return o(b,c)}function j(a,b){var c="--"+g(b);n(a,b,c),m(a,b);for(var d=[],e=null;"--"!==e&&b.position<a.length;){var h,i=k(a,b),o=x(i["Content-Type"]);if(o&&o.mediaType===D){b.boundaries.push(o.properties.boundary);try{h=j(a,b)}catch(d){d.response=l(a,b,c),h=[d]}d.push({__changeResponses:h}),b.boundaries.pop(),n(a,b,"--"+g(b))}else{if(!o||"application/http"!==o.mediaType)throw{message:"invalid MIME part type "};m(a,b);var p=l(a,b,c);try{p.statusCode>=200&&p.statusCode<=299?f(b.handlerContext).read(p,b.handlerContext):p={message:"HTTP request failed",response:p}}catch(a){p=a}d.push(p)}e=a.substr(b.position,2),m(a,b)}return d}function k(a,b){var c,d,e,f={};do{e=b.position,d=m(a,b),c=F.exec(d),null!==c?f[c[1]]=c[2]:b.position=e}while(d&&c);return B(f),f}function l(a,b,c){var d,e,f,g=b.position,h=E.exec(m(a,b));return h?(d=h[1],e=h[2],f=k(a,b),m(a,b)):b.position=g,{statusCode:d,statusText:e,headers:f,body:n(a,b,"\r\n"+c)}}function m(a,b){return n(a,b,"\r\n")}function n(a,b,c){var d=b.position||0,e=a.length;if(c){if(-1===(e=a.indexOf(c,d)))return null;b.position=e+c.length}else b.position=e;return a.substring(d,e)}function o(a,b){if(!z(a))throw{message:"Data is not a batch object."};var c,d,f=e("batch_"),g=a.__batchRequests,h="";for(c=0,d=g.length;c<d;c++)h+=p(f,!1)+q(g[c],b);return h+=p(f,!0),b.contentType.properties.boundary=f,h}function p(a,b){var c="\r\n--"+a;return b&&(c+="--"),c+"\r\n"}function q(a,b,c){var d,g=a.__changeRequests;if(w(g)){if(c)throw{message:"Not Supported: change set nested in other change set"};var h=e("changeset_");d="Content-Type: "+D+"; boundary="+h+"\r\n";var i,j;for(i=0,j=g.length;i<j;i++)d+=p(h,!1)+q(g[i],b,!0);d+=p(h,!0)}else{d="Content-Type: application/http\r\nContent-Transfer-Encoding: binary\r\n\r\n";var k=v({},b);k.handler=y,k.request=a,k.contentType=null,C(a,f(b),k),d+=r(a)}return d}function r(a){var b=(a.method?a.method:"GET")+" "+a.requestUri+" HTTP/1.1\r\n";for(var c in a.headers)a.headers[c]&&(b=b+c+": "+a.headers[c]+"\r\n");return b+="\r\n",a.body&&(b+=a.body),b}var s=c("./../utils.js"),t=c("./odatautils.js"),u=c("./handler.js"),v=s.extend,w=s.isArray,x=(s.trimString,u.contentType),y=u.handler,z=t.isBatch,A=u.MAX_DATA_SERVICE_VERSION,B=t.normalizeHeaders,C=t.prepareRequest,D="multipart/mixed",E=/^HTTP\/1\.\d (\d{3}) (.*)$/i,F=/^([^()<>@,;:\\"\/[\]?={} \t]+)\s?:\s?(.*)/;a.batchHandler=y(h,i,D,A),a.batchSerializer=i,a.writeRequest=r},handler:function(a,b,c){"use strict";function d(a){if(!a)return null;var b,c,d=a.split(";"),e={};for(b=1,c=d.length;b<c;b++){var f=d[b].split("=");e[v(f[0])]=f[1]}return{mediaType:v(d[0]),properties:e}}function e(a){if(a){var b,c=a.mediaType;for(b in a.properties)c+=";"+b+"="+a.properties[b];return c}}function f(a,b,c,d){var e={};return u(e,c),u(e,{contentType:a,dataServiceVersion:b,handler:d}),e}function g(a,b,c){if(a){var d=a.headers;d[b]||(d[b]=c)}}function h(a,b){if(a){var c=a.headers,d=c["OData-Version"];c["OData-Version"]=d?w(d,b):b}}function i(a,b){var c=a.headers;return c&&c[b]||void 0}function j(a){return d(i(a,"Content-Type"))}function k(a){var b=i(a,"OData-Version");if(b){var c=y.exec(b);if(c&&c.length)return c[1]}}function l(a,b){return a.accept.indexOf(b.mediaType)>=0}function m(a,b,c,d){if(!c||!c.headers)return!1;var e=j(c),g=k(c)||"",h=c.body;if(!t(h))return!1;if(l(a,e)){var i=f(e,g,d,a);return i.response=c,c.data=b(a,h,i),void 0!==c.data}return!1}function n(a,b,c,d){if(!c||!c.headers)return!1;var i=j(c),m=k(c);if(!i||l(a,i)){var n=f(i,m,d,a);if(n.request=c,c.body=b(a,c.data,n),void 0!==c.body)return h(c,n.dataServiceVersion||"4.0"),g(c,"Content-Type",e(n.contentType)),g(c,"OData-MaxVersion",a.maxDataServiceVersion),!0}return!1}function o(a,b,c,d){return{accept:c,maxDataServiceVersion:d,read:function(b,c){return m(this,a,b,c)},write:function(a,c){return n(this,b,a,c)}}}function p(a,b){return b}function q(a,b){return t(b)?b.toString():void 0}var r=c("./../utils.js"),s=c("./odatautils.js"),t=r.assigned,u=r.extend,v=r.trimString,w=s.maxVersion,x="4.0",y=/^\s?(\d+\.\d+);?.*$/;a.textHandler=o(p,q,"text/plain",x),a.contentType=d,a.contentTypeToString=e,a.handler=o,a.createReadWriteContext=f,a.fixRequestHeader=g,a.getRequestOrResponseHeader=i,a.getContentType=j,a.getDataServiceVersion=k,a.MAX_DATA_SERVICE_VERSION=x},json:function(a,b,c){function d(a,b,c){var d,e=J(c.recognizeDates,a.recognizeDates),f=c.metadata,g="string"==typeof b?JSON.parse(b):b;I(c.contentType)&&I(c.contentType.properties)&&(d=c.contentType.properties["odata.metadata"]);var h=N(d,1);return 0===h?g:1===h?k(g,f,e):2===h?i(g,f,e):g}function e(a,b,c){var d=c.dataServiceVersion||"4.0",e=c.contentType=c.contentType||pa;if(e&&e.mediaType===pa.mediaType){c.dataServiceVersion=$(d,"4.0");var g=f(b);if(g)return JSON.stringify(g,sa)}}function f(a){if(!a)return a;if(R(a))return a;if(K(a)){var b,c,d=[];for(b=0,c=a.length;b<c;b++)d[b]=f(a[b]);return d}var e={};for(var h in a)g(h)&&(e[h]=f(a[h]));return e}function g(a){if(!a)return!1;if(-1==a.indexOf("@odata."))return!0;var b,c;for(b=0,c=qa.length;b<c;b++){var d=qa[b];if(-1!=a.indexOf(d))return!0}return!1}function h(a,b){return{kind:a,type:b||null}}function i(a,b,c){var d;if(C.isObject(a))for(var e in a)if(a.hasOwnProperty(e)&&-1===e.indexOf("@"))if(C.isArray(a[e]))for(var f=0;f<a[e].length;++f)i(a[e][f],b,c);else if(C.isObject(a[e]))null!==a[e]&&(d=a[e+"@odata.type"],d?(d=d.substring(1),aa(d)||ba(d)||i(a[e],b,c)):i(a[e],b,c));else if(d=a[e+"@odata.type"],I(d))c&&t(a,e,d.substring(1));else{var g=typeof a[e];"string"===g?p(a,e,"String"):"boolean"===g?p(a,e,"Boolean"):"number"===g&&(a[e]%1==0?p(a,e,"Int32"):p(a,e,"Decimal"))}return a}function j(a,b,c,d,e){for(var f in a)if(-1===f.indexOf("@")){for(var g=b,h=a[f],i=Y(g.property,f);null===i&&void 0!==g.baseType;)g=U(g.baseType,d),i=Y(g.property,f);if(K(h)){S(i.type)?q(a,f,i.type.substring(11,i.type.length-1)):r(a,f,i.type);for(var j=0;j<h.length;j++)n(h[j],i,c,d,e)}else L(h)&&null!==h?n(h,i,c,d,e):(r(a,f,i.type),e&&s(a,f,i.type))}}function k(a,b,c){if(!I(b)||K(b))return a;var d=a[H],e=z(a,b);switch(e.detectedPayloadKind){case ja:return null!==e.type?m(a,e,d,b,c):r(a,"value",e.typeName);case ca:return l(a,b,e,d,c);case da:return m(a,e,d,b,c);case fa:return o(a,b,e,d,c);case ea:return null!==e.type?m(a,e,d,b,c):r(a,"value",e.typeName);case ga:case PAYLOADTYPE_LINKS:return a}return a}function l(a,b,c,d,e){var f,g,h,i=[],j=a.value;for(f=0,g=j.length;f<g;f++){var k=j[f];if(J(k["@odata.type"])){var l=k["@odata.type"].substring(1),n=U(l,b);h=m(k,{contentTypeOdata:c.contentTypeOdata,detectedPayloadKind:c.detectedPayloadKind,name:c.name,type:n,typeName:l},d,b,e)}else h=m(k,c,d,b,e);i.push(h)}return a.value=i,a}function m(a,b,c,d,e){p(a,"",b.typeName);for(var f=b.type;J(f)&&void 0===f.key&&void 0!==f.baseType;)f=U(f.baseType,d);if(void 0!==f.key){var g=b.name+A(a,f);a["@odata.id"]=c.substring(0,c.lastIndexOf("$metadata"))+g,a["@odata.editLink"]=g}return j(a,b.type,c,d,e),a}function n(a,b,c,d,e){var f=b.type;S(b.type)&&(f=b.type.substring(11,b.type.length-1)),p(a,"",b.type);var g=T(f,d);null!==g&&j(a,g,c,d,e)}function o(a,b,c,d,e){if(q(a,"",c.typeName),null!==c.type){var f,g,h,i=[],j=a.value;for(f=0,g=j.length;f<g;f++){var k=j[f];if(J(k["@odata.type"])){var l=k["@odata.type"].substring(1),n=U(l,b);h=m(k,{contentTypeOdata:c.contentTypeOdata,detectedPayloadKind:c.detectedPayloadKind,name:c.name,type:n,typeName:l},d,b,e)}else h=m(k,c,d,b,e);i.push(h)}a.value=i}return a}function p(a,b,c){var d=b+"@odata.type";void 0===a[d]&&(a[d]="#"+c)}function q(a,b,c){var d=b+"@odata.type";void 0===a[d]&&("Edm."===c.substring(0,4)?a[d]="#Collection("+c.substring(4)+")":a[d]="#Collection("+c+")")}function r(a,b,c){var d=b+"@odata.type";return void 0===a[d]&&("Edm."===c.substring(0,4)?a[d]="#"+c.substring(4):a[d]="#"+c),a}function s(a,b,c){"Edm.Date"===c?a[b]=D.parseDate(a[b],!0):"Edm.DateTimeOffset"===c?a[b]=D.parseDateTimeOffset(a[b],!0):"Edm.Duration"===c?a[b]=D.parseDuration(a[b],!0):"Edm.Time"===c&&(a[b]=D.parseTime(a[b],!0))}function t(a,b,c){"Date"===c?a[b]=D.parseDate(a[b],!0):"DateTimeOffset"===c?a[b]=D.parseDateTimeOffset(a[b],!0):"Duration"===c?a[b]=D.parseDuration(a[b],!0):"Time"===c&&(a[b]=D.parseTime(a[b],!0))}function u(a,b){switch(a=""+v(a,b),a=encodeURIComponent(a.replace("'","''")),b){case"Edm.Binary":return"X'"+a+"'";case"Edm.DateTime":return"datetime'"+a+"'";case"Edm.DateTimeOffset":return"datetimeoffset'"+a+"'";case"Edm.Decimal":return a+"M";case"Edm.Guid":return"guid'"+a+"'";case"Edm.Int64":return a+"L";case"Edm.Float":return a+"f";case"Edm.Double":return a+"D";case"Edm.Geography":return"geography'"+a+"'";case"Edm.Geometry":return"geometry'"+a+"'";case"Edm.Time":return"time'"+a+"'";case"Edm.String":return"'"+a+"'";default:return a}}function v(a,b){switch(b){case"Edm.Binary":return O(a);default:return a}}function w(a){var b;a<0?(b="-",a=-a):b="+";var c=Math.floor(a/60);return a-=60*c,b+Q(c,2)+":"+Q(a,2)}function x(a){var b=a&&ra.exec(a);if(b){var c=new Date(M(b[1]));if(b[2]){var d=M(b[3]);"-"===b[2]&&(d=-d);var e=c.getUTCMinutes();c.setUTCMinutes(e-d),c.__edmType="Edm.DateTimeOffset",c.__offset=w(d)}if(!isNaN(c.valueOf()))return c}}function y(a,b){var c={};if(-1===a.indexOf("/")){if(0===a.length)return c.detectedPayloadKind=ga,c;if("Edm.Null"===a)return c.detectedPayloadKind=ja,c.isNullProperty=!0,c;if("Collection($ref)"===a)return c.detectedPayloadKind=ia,c;if("$ref"===a)return c.detectedPayloadKind=ha,c}c.type=void 0,c.typeName=void 0;for(var d,e=a.split("/"),f=0;f<e.length;++f){var g=e[f];if(void 0===c.typeName){if(-1!==g.indexOf("(")){for(var h=g.length-2,i=1;i>0&&h>0;--h)"("==g.charAt(h)?i--:")"==g.charAt(h)&&i++;var j=g.substring(h+2,g.length-1);if(g=g.substring(0,h+1),C.startsWith(g,"Collection")){if(c.detectedPayloadKind=fa,c.typeName=j,null!==(d=U(c.typeName,b))){c.type=d;continue}if(null!==(d=T(c.typeName,b))){c.type=d;continue}c.type=null;continue}c.projection=j}if(B(g)){c.typeName=g,c.type=null,c.detectedPayloadKind=ja;continue}var k=X(b),l=W(k.entitySet,g);if(null!==l){c.typeName=l.entityType,c.type=U(c.typeName,b),c.name=g,c.detectedPayloadKind=ca;continue}var m=V(k.singleton,g);if(null!==m){c.typeName=m.entityType,c.type=U(c.typeName,b),c.name=g,c.detectedPayloadKind=da;continue}}else{if(C.endsWith(g,"$entity")&&c.detectedPayloadKind===ca){c.detectedPayloadKind=da;continue}if(-1!==g.indexOf(".")){if(c.typeName=g,null!==(d=U(c.typeName,b))){c.type=d;continue}if(null!==(d=T(c.typeName,b))){c.type=d;continue}}if(c.detectedPayloadKind===ca||c.detectedPayloadKind===da){var n=Y(c.type.property,g);if(null!==n){if(c.typeName=n.type,C.startsWith(n.type,"Collection")){c.detectedPayloadKind=fa;var o=n.type.substring(11,n.type.length-1);c.typeName=o,c.type=T(o,b),c.detectedPayloadKind=fa}else c.type=T(n.type,b),c.detectedPayloadKind=ea;c.name=g}continue}if("$delta"===g){c.deltaKind=ka;continue}if(C.endsWith(g,"/$deletedEntity")){c.deltaKind=la;continue}if(C.endsWith(g,"/$link")){c.deltaKind=ma;continue}if(C.endsWith(g,"/$deletedLink")){c.deltaKind=na;continue}}}return c}function z(a,b){var c=a[H];if(!c||"string"!=typeof c)return null;var d=c.lastIndexOf("#");return-1===d?h(ga):y(c.substring(d+1),b)}function A(a,b){var c,d,e=b.key.propertyRef;if(c="(",1==e.length)d=Y(b.property,e[0].name).type,c+=u(a[e[0].name],d);else for(var f=!0,g=0;g<e.length;g++)f?f=!1:c+=",",d=Y(b.property,e[g].name).type,c+=e[g].name+"="+u(a[e[g].name],d);return c+=")"}function B(a){return _(a)||aa(a)||ba(a)}var C=c("./../utils.js"),D=c("./odatautils.js"),E=c("./handler.js"),F="odata",G=F+".",H="@"+G+"context",I=C.assigned,J=C.defined,K=C.isArray,L=C.isObject,M=C.parseInt10,N=C.getFormatKind,O=C.convertByteArrayToHexString,P=(D.formatDateTimeOffset,D.formatDuration),Q=D.formatNumberWidth,R=(D.getCanonicalTimezone,D.handler,D.isComplex,D.isPrimitive),S=D.isCollectionType,T=D.lookupComplexType,U=D.lookupEntityType,V=D.lookupSingleton,W=D.lookupEntitySet,X=D.lookupDefaultEntityContainer,Y=D.lookupProperty,Z=D.MAX_DATA_SERVICE_VERSION,$=D.maxVersion,_=D.isPrimitiveEdmType,aa=D.isGeographyEdmType,ba=D.isGeometryEdmType,ca="f",da="e",ea="p",fa="c",ga="s",ha="erl",ia="erls",ja="v",ka="f",la="de",ma="l",na="dl",oa="application/json",pa=E.contentType(oa),qa=["@odata.id","@odata.type"],ra=/^\/Date\((-?\d+)(\+|-)?(\d+)?\)\/$/,sa=function(a,b){return b&&"Edm.Time"===b.__edmType?P(b):b},ta=E.handler(d,e,oa,Z);ta.recognizeDates=!1,a.createPayloadInfo=z,a.jsonHandler=ta,a.jsonParser=d,a.jsonSerializer=e,a.parseJsonDateString=x},metadata:function(a,b,c){"use strict";function d(a,b,c,d){return{attributes:a,elements:b,text:c||!1,ns:d}}function e(a){if(!a)return a;if(a.length>1){var b=a.substr(0,2);return b===b.toUpperCase()?a:a.charAt(0).toLowerCase()+a.substr(1)}return a.charAt(0).toLowerCase()}function f(a,b){var c=a.elements;if(!c)return null;var d,f;for(d=0,f=c.length;d<f;d++){var g=c[d],h=!1;if("*"===g.charAt(g.length-1)&&(h=!0,g=g.substr(0,g.length-1)),b===g){return{isArray:h,propertyName:e(g)}}}return null}function g(a){return a===y}function h(a){var b=r(a),c=s(a),d=B.elements[b];if(!d)return null;if(d.ns){if(c!==d.ns)return null}else if(!g(c))return null;var i={},j=d.attributes||[];return n(a,function(a){var b=r(a),c=s(a),d=a.value;if(c!==t){var f=null;g(c)||null===c?f="":c===z&&(f="m:"),null!==f&&(f+=b,m(j,f)&&(i[e(b)]=d))}}),o(a,function(a){var b=r(a),c=f(d,b);if(c)if(c.isArray){var e=i[c.propertyName];e||(e=[],i[c.propertyName]=e),e.push(h(a))}else i[c.propertyName]=h(a)}),d.text&&(i.text=q(a)),i}function i(a,b){var c=u(b);return h(p(c))||void 0}var j=c("./../utils.js"),k=c("./../xml.js"),l=c("./handler.js"),m=j.contains,n=(j.normalizeURI,k.xmlAttributes),o=k.xmlChildElements,p=k.xmlFirstChildElement,q=k.xmlInnerText,r=k.xmlLocalName,s=k.xmlNamespaceURI,t=(k.xmlNS,k.xmlnsNS),u=k.xmlParse,v=k.http+"docs.oasis-open.org/odata/",w=v+"ns",x=w+"/edmx",y=w+"/edm",z=w+"/metadata",A=l.MAX_DATA_SERVICE_VERSION,B={elements:{Action:d(["Name","IsBound","EntitySetPath"],["ReturnType","Parameter*","Annotation*"]),ActionImport:d(["Name","Action","EntitySet","Annotation*"]),Annotation:d(["Term","Qualifier","Binary","Bool","Date","DateTimeOffset","Decimal","Duration","EnumMember","Float","Guid","Int","String","TimeOfDay","AnnotationPath","NavigationPropertyPath","Path","PropertyPath","UrlRef"],["Binary","Bool","Date","DateTimeOffset","Decimal","Duration","EnumMember","Float","Guid","Int","String","TimeOfDay","And","Or","Not","Eq","Ne","Gt","Ge","Lt","Le","AnnotationPath","Apply","Cast","Collection","If","IsOf","LabeledElement","LabeledElementReference","Null","NavigationPropertyPath","Path","PropertyPath","Record","UrlRef","Annotation*"]),AnnotationPath:d(null,null,!0),Annotations:d(["Target","Qualifier"],["Annotation*"]),Apply:d(["Function"],["Binary*","Bool*","Date*","DateTimeOffset*","Decimal*","Duration*","EnumMember*","Float*","Guid*","Int*","String*","TimeOfDay*","And*","Or*","Not*","Eq*","Ne*","Gt*","Ge*","Lt*","Le*","AnnotationPath*","Apply*","Cast*","Collection*","If*","IsOf*","LabeledElement*","LabeledElementReference*","Null*","NavigationPropertyPath*","Path*","PropertyPath*","Record*","UrlRef*","Annotation*"]),And:d(null,["Binary","Bool","Date","DateTimeOffset","Decimal","Duration","EnumMember","Float","Guid","Int","String","TimeOfDay","And","Or","Not","Eq","Ne","Gt","Ge","Lt","Le","AnnotationPath","Apply","Cast","Collection","If","IsOf","LabeledElement","LabeledElementReference","Null","NavigationPropertyPath","Path","PropertyPath","Record","UrlRef","Annotation*"]),Or:d(null,["Binary","Bool","Date","DateTimeOffset","Decimal","Duration","EnumMember","Float","Guid","Int","String","TimeOfDay","And","Or","Not","Eq","Ne","Gt","Ge","Lt","Le","AnnotationPath","Apply","Cast","Collection","If","IsOf","LabeledElement","LabeledElementReference","Null","NavigationPropertyPath","Path","PropertyPath","Record","UrlRef","Annotation*"]),Not:d(null,["Binary","Bool","Date","DateTimeOffset","Decimal","Duration","EnumMember","Float","Guid","Int","String","TimeOfDay","And","Or","Not","Eq","Ne","Gt","Ge","Lt","Le","AnnotationPath","Apply","Cast","Collection","If","IsOf","LabeledElement","LabeledElementReference","Null","NavigationPropertyPath","Path","PropertyPath","Record","UrlRef","Annotation*"]),Eq:d(null,["Binary","Bool","Date","DateTimeOffset","Decimal","Duration","EnumMember","Float","Guid","Int","String","TimeOfDay","And","Or","Not","Eq","Ne","Gt","Ge","Lt","Le","AnnotationPath","Apply","Cast","Collection","If","IsOf","LabeledElement","LabeledElementReference","Null","NavigationPropertyPath","Path","PropertyPath","Record","UrlRef","Annotation*"]),Ne:d(null,["Binary","Bool","Date","DateTimeOffset","Decimal","Duration","EnumMember","Float","Guid","Int","String","TimeOfDay","And","Or","Not","Eq","Ne","Gt","Ge","Lt","Le","AnnotationPath","Apply","Cast","Collection","If","IsOf","LabeledElement","LabeledElementReference","Null","NavigationPropertyPath","Path","PropertyPath","Record","UrlRef","Annotation*"]),Gt:d(null,["Binary","Bool","Date","DateTimeOffset","Decimal","Duration","EnumMember","Float","Guid","Int","String","TimeOfDay","And","Or","Not","Eq","Ne","Gt","Ge","Lt","Le","AnnotationPath","Apply","Cast","Collection","If","IsOf","LabeledElement","LabeledElementReference","Null","NavigationPropertyPath","Path","PropertyPath","Record","UrlRef","Annotation*"]),Ge:d(null,["Binary","Bool","Date","DateTimeOffset","Decimal","Duration","EnumMember","Float","Guid","Int","String","TimeOfDay","And","Or","Not","Eq","Ne","Gt","Ge","Lt","Le","AnnotationPath","Apply","Cast","Collection","If","IsOf","LabeledElement","LabeledElementReference","Null","NavigationPropertyPath","Path","PropertyPath","Record","UrlRef","Annotation*"]),Lt:d(null,["Binary","Bool","Date","DateTimeOffset","Decimal","Duration","EnumMember","Float","Guid","Int","String","TimeOfDay","And","Or","Not","Eq","Ne","Gt","Ge","Lt","Le","AnnotationPath","Apply","Cast","Collection","If","IsOf","LabeledElement","LabeledElementReference","Null","NavigationPropertyPath","Path","PropertyPath","Record","UrlRef","Annotation*"]),Le:d(null,["Binary","Bool","Date","DateTimeOffset","Decimal","Duration","EnumMember","Float","Guid","Int","String","TimeOfDay","And","Or","Not","Eq","Ne","Gt","Ge","Lt","Le","AnnotationPath","Apply","Cast","Collection","If","IsOf","LabeledElement","LabeledElementReference","Null","NavigationPropertyPath","Path","PropertyPath","Record","UrlRef","Annotation*"]),Binary:d(null,null,!0),Bool:d(null,null,!0),Cast:d(["Type"],["Binary","Bool","Date","DateTimeOffset","Decimal","Duration","EnumMember","Float","Guid","Int","String","TimeOfDay","And","Or","Not","Eq","Ne","Gt","Ge","Lt","Le","AnnotationPath","Apply","Cast","Collection","If","IsOf","LabeledElement","LabeledElementReference","Null","NavigationPropertyPath","Path","PropertyPath","Record","UrlRef","Annotation*"]),Collection:d(null,["Binary*","Bool*","Date*","DateTimeOffset*","Decimal*","Duration*","EnumMember*","Float*","Guid*","Int*","String*","TimeOfDay*","And*","Or*","Not*","Eq*","Ne*","Gt*","Ge*","Lt*","Le*","AnnotationPath*","Apply*","Cast*","Collection*","If*","IsOf*","LabeledElement*","LabeledElementReference*","Null*","NavigationPropertyPath*","Path*","PropertyPath*","Record*","UrlRef*"]),ComplexType:d(["Name","BaseType","Abstract","OpenType"],["Property*","NavigationProperty*","Annotation*"]),Date:d(null,null,!0),DateTimeOffset:d(null,null,!0),Decimal:d(null,null,!0),Duration:d(null,null,!0),EntityContainer:d(["Name","Extends"],["EntitySet*","Singleton*","ActionImport*","FunctionImport*","Annotation*"]),EntitySet:d(["Name","EntityType","IncludeInServiceDocument"],["NavigationPropertyBinding*","Annotation*"]),EntityType:d(["Name","BaseType","Abstract","OpenType","HasStream"],["Key","Property*","NavigationProperty*","Annotation*"]),EnumMember:d(null,null,!0),EnumType:d(["Name","UnderlyingType","IsFlags"],["Member*"]),Float:d(null,null,!0),Function:d(["Name","IsBound","IsComposable","EntitySetPath"],["ReturnType","Parameter*","Annotation*"]),FunctionImport:d(["Name","Function","EntitySet","IncludeInServiceDocument","Annotation*"]),Guid:d(null,null,!0),If:d(null,["Binary*","Bool*","Date*","DateTimeOffset*","Decimal*","Duration*","EnumMember*","Float*","Guid*","Int*","String*","TimeOfDay*","And*","Or*","Not*","Eq*","Ne*","Gt*","Ge*","Lt*","Le*","AnnotationPath*","Apply*","Cast*","Collection*","If*","IsOf*","LabeledElement*","LabeledElementReference*","Null*","NavigationPropertyPath*","Path*","PropertyPath*","Record*","UrlRef*","Annotation*"]),Int:d(null,null,!0),IsOf:d(["Type","MaxLength","Precision","Scale","SRID","Annotation*"],["Binary","Bool","Date","DateTimeOffset","Decimal","Duration","EnumMember","Float","Guid","Int","String","TimeOfDay","And","Or","Not","Eq","Ne","Gt","Ge","Lt","Le","AnnotationPath","Apply","Cast","Collection","If","IsOf","LabeledElement","LabeledElementReference","Null","NavigationPropertyPath","Path","PropertyPath","Record","UrlRef","Annotation*"]),Key:d(null,["PropertyRef*"]),LabeledElement:d(["Name"],["Binary","Bool","Date","DateTimeOffset","Decimal","Duration","EnumMember","Float","Guid","Int","String","TimeOfDay","And","Or","Not","Eq","Ne","Gt","Ge","Lt","Le","AnnotationPath","Apply","Cast","Collection","If","IsOf","LabeledElement","LabeledElementReference","Null","NavigationPropertyPath","Path","PropertyPath","Record","UrlRef","Annotation*"]),LabeledElementReference:d(null,null,!0),Member:d(["Name","Value"],["Annotation*"]),NavigationProperty:d(["Name","Type","Nullable","Partner","ContainsTarget"],["ReferentialConstraint*","OnDelete","Annotation*"]),NavigationPropertyBinding:d(["Path","Target"]),NavigationPropertyPath:d(null,null,!0),Null:d(null,["Annotation*"]),OnDelete:d(["Action"],["Annotation*"]),Path:d(null,null,!0),Parameter:d(["Name","Type","Nullable","MaxLength","Precision","Scale","SRID"],["Annotation*"]),Property:d(["Name","Type","Nullable","MaxLength","Precision","Scale","Unicode","SRID","DefaultValue"],["Annotation*"]),PropertyPath:d(null,null,!0),PropertyRef:d(["Name","Alias"]),PropertyValue:d(["Property","Binary","Bool","Date","DateTimeOffset","Decimal","Duration","EnumMember","Float","Guid","Int","String","TimeOfDay","AnnotationPath","NavigationPropertyPath","Path","PropertyPath","UrlRef"],["Binary","Bool","Date","DateTimeOffset","Decimal","Duration","EnumMember","Float","Guid","Int","String","TimeOfDay","And","Or","Not","Eq","Ne","Gt","Ge","Lt","Le","AnnotationPath","Apply","Cast","Collection","If","IsOf","LabeledElement","LabeledElementReference","Null","NavigationPropertyPath","Path","PropertyPath","Record","UrlRef","Annotation*"]),Record:d(null,["PropertyValue*","Annotation*"]),ReferentialConstraint:d(["Property","ReferencedProperty","Annotation*"]),ReturnType:d(["Type","Nullable","MaxLength","Precision","Scale","SRID"]),String:d(null,null,!0),Schema:d(["Namespace","Alias"],["Action*","Annotations*","Annotation*","ComplexType*","EntityContainer","EntityType*","EnumType*","Function*","Term*","TypeDefinition*","Annotation*"]),Singleton:d(["Name","Type"],["NavigationPropertyBinding*","Annotation*"]),Term:d(["Name","Type","BaseTerm","DefaultValue ","AppliesTo","Nullable","MaxLength","Precision","Scale","SRID"],["Annotation*"]),TimeOfDay:d(null,null,!0),TypeDefinition:d(["Name","UnderlyingType","MaxLength","Unicode","Precision","Scale","SRID"],["Annotation*"]),UrlRef:d(null,["Binary","Bool","Date","DateTimeOffset","Decimal","Duration","EnumMember","Float","Guid","Int","String","TimeOfDay","And","Or","Not","Eq","Ne","Gt","Ge","Lt","Le","AnnotationPath","Apply","Cast","Collection","If","IsOf","LabeledElement","LabeledElementReference","Null","NavigationPropertyPath","Path","PropertyPath","Record","UrlRef","Annotation*"]),Edmx:d(["Version"],["DataServices","Reference*"],!1,x),DataServices:d(["m:MaxDataServiceVersion","m:DataServiceVersion"],["Schema*"],!1,x),Reference:d(["Uri"],["Include*","IncludeAnnotations*","Annotation*"],!1,x),Include:d(["Namespace","Alias"],null,!1,x),IncludeAnnotations:d(["TermNamespace","Qualifier","TargetNamespace"],null,!1,x)}};a.metadataHandler=l.handler(i,null,"application/xml",A),a.schema=B,a.scriptCase=e,a.getChildSchema=f,a.parseConceptualModelElement=h,a.metadataParser=i},net:function(a,b,c){function d(a){return!(a.method&&"GET"!==a.method)}function e(a){var b=window.document.createElement("IFRAME");b.style.display="none";var c=a.replace(/&/g,"&amp;").replace(/"/g,"&quot;").replace(/</g,"&lt;"),d='<html><head><script type="text/javascript" src="'+c+'"><\/script></head><body></body></html>';return window.document.getElementsByTagName("BODY")[0].appendChild(b),l(b,d),b}function f(){if(window.XMLHttpRequest)return new window.XMLHttpRequest;var a;if(window.ActiveXObject)try{return new window.ActiveXObject("Msxml2.XMLHTTP.6.0")}catch(b){try{return new window.ActiveXObject("Msxml2.XMLHTTP.3.0")}catch(b){a=b}}else a={message:"XMLHttpRequest not supported"};throw a}function g(a){return 0===a.indexOf("http://")||0===a.indexOf("https://")||0===a.indexOf("file://")}function h(a){if(!g(a))return!0;var b=window.location,c=b.protocol+"//"+b.host+"/";return 0===a.indexOf(c)}function i(a,b){try{delete window[a]}catch(c){window[a]=void 0,b===p-1&&(p-=1)}}function j(a){return a&&(l(a,""),a.parentNode.removeChild(a)),null}function k(a,b){var c,d,e=a.getAllResponseHeaders().split(/\r?\n/);for(c=0,d=e.length;c<d;c++)if(e[c]){var f=e[c].split(": ");b[f[0]]=f[1]}}function l(a,b){var c=a.contentWindow?a.contentWindow.document:a.contentDocument.document;c.open(),c.write(b),c.close()}var m=c("./../utils.js"),n=m.defined,o=m.delay,p=0;a.defaultHttpClient={callbackParameterName:"$callback",formatQueryString:"$format=json",enableJsonpCallback:!1,request:function(){var a=this;return function(b,c,g){var l,m={},q=null,r=!1;m.abort=function(){l=j(l),r||(r=!0,q&&(q.abort(),q=null),g({message:"Request aborted"}))};var s,t=function(){l=j(l),r||(r=!0,q=null,g({message:"Request timed out"}))},u=b.requestUri,v=n(b.enableJsonpCallback,a.enableJsonpCallback),w=n(b.callbackParameterName,a.callbackParameterName),x=n(b.formatQueryString,a.formatQueryString);if(!v||h(u)){if(q=f(),q.onreadystatechange=function(){if(!r&&null!==q&&4===q.readyState){var a=q.statusText,d=q.status;1223===d&&(d=204,a="No Content");var e=[];k(q,e);var f={requestUri:u,statusCode:d,statusText:a,headers:e,body:q.responseText};r=!0,q=null,d>=200&&d<=299?c(f):g({message:"HTTP request failed",request:b,response:f})}},q.open(b.method||"GET",u,!0,b.user,b.password),b.headers)for(s in b.headers)q.setRequestHeader(s,b.headers[s]);b.withCredentials&&(q.withCredentials=!0),b.timeoutMS&&(q.timeout=b.timeoutMS,q.ontimeout=t),q.send(b.body)}else{if(!d(b))throw{message:"Request is not local and cannot be done through JSONP."};var y=p;p+=1;var z,A=y.toString(),B=!1;s="handleJSONP_"+A,window[s]=function(a){if(l=j(l),!r){B=!0,window.clearTimeout(z),i(s,y),window.ActiveXObject&&(a=window.JSON.parse(window.JSON.stringify(a)));var b;b=x&&"$format=json"!=x?{"Content-Type":x.substring(8),"OData-Version":"4.0"}:{"Content-Type":"application/json;odata.metadata=minimal","OData-Version":"4.0"},o(function(){j(l),c({body:a,statusCode:200,headers:b})})}};var C=b.timeoutMS?b.timeoutMS:12e4;z=window.setTimeout(t,C);var D=w+"=parent."+s;x&&(D+="&"+x);var E=u.indexOf("?");-1===E?u=u+"?"+D:E===u.length-1?u+=D:u=u+"&"+D,l=e(u)}return m}}()},a.canUseJSONP=d,a.isAbsoluteUrl=g,a.isLocalUrl=h},odatautils:function(a,b,c){"use strict";function d(a,b){if(!a)return null;if(ca(a)){var c,e,f;for(c=0,e=a.length;c<e;c++)if(f=d(a[c],b))return f;return null}return a.dataServices?d(a.dataServices.schema,b):b(a)}function e(a,b){return a=0===a?"":"."+i(a.toString(),3),b>0&&(""===a&&(a=".000"),a+=i(b.toString(),4)),a}function f(a){return"/Date("+a.getTime()+")/"}function g(a){if("string"==typeof a)return a;var b=q(a),c=j(a.__offset);if(b&&"Z"!==c){a=new Date(a.valueOf());var d=W(c),f=a.getUTCHours()+d.d*d.h,g=a.getUTCMinutes()+d.d*d.m;a.setUTCHours(f,g)}else b||(c="");var h=a.getUTCFullYear(),k=a.getUTCMonth()+1,l="";h<=0&&(h=-(h-1),l="-");var m=e(a.getUTCMilliseconds(),a.__ns);return l+i(h,4)+"-"+i(k,2)+"-"+i(a.getUTCDate(),2)+"T"+i(a.getUTCHours(),2)+":"+i(a.getUTCMinutes(),2)+":"+i(a.getUTCSeconds(),2)+m+c}function h(a){var b=a.ms,c="";b<0&&(c="-",b=-b);var d=Math.floor(b/864e5);b-=864e5*d;var f=Math.floor(b/36e5);b-=36e5*f;var g=Math.floor(b/6e4);b-=6e4*g;var h=Math.floor(b/1e3);return b-=1e3*h,c+"P"+i(d,2)+"DT"+i(f,2)+"H"+i(g,2)+"M"+i(h,2)+e(b,a.ns)+"S"}function i(a,b,c){for(var d=a.toString(10);d.length<b;)c?d+="0":d="0"+d;return d}function j(a){return a&&"Z"!==a&&"+00:00"!==a&&"-00:00"!==a?a:"Z"}function k(a){if("string"==typeof a){var b=a.indexOf(")",10);if(0===a.indexOf("Collection(")&&b>0)return a.substring(11,b)}return null}function l(a,b,c,d,e,f){return e.request(a,function(e){try{e.headers&&P(e.headers),void 0===e.data&&204!==e.statusCode&&d.read(e,f)}catch(b){return void 0===b.request&&(b.request=a),void 0===b.response&&(b.response=e),void c(b)}try{b(e.data,e)}catch(a){throw a.bIsSuccessHandlerError=!0,a}},c)}function m(a){return p(a)&&ca(a.__batchRequests)}function n(a,b){var c=a&&a.results||a;return!!c&&o(b)||!b&&ca(c)&&!p(c[0])}function o(a){return hb.test(a)}function p(a){return!!a&&ea(a)&&!ca(a)&&!da(a)}function q(a){return"Edm.DateTimeOffset"===a.__edmType||!a.__edmType&&a.__offset}function r(a){if(!a&&!p(a))return!1;var b=a.__metadata||{},c=a.__deferred||{};return!b.type&&!!c.uri}function s(a){return p(a)&&a.__metadata&&"uri"in a.__metadata}function t(a,b){var c=a&&a.results||a;return ca(c)&&!o(b)&&p(c[0])}function u(a){return aa(fb,a)||-1===a.indexOf(".")&&aa(gb,a)}function v(a){return aa(db,a)||-1===a.indexOf(".")&&aa(eb,a)}function w(a){if(!a&&!p(a))return!1;var b=a.__metadata,c=a.__mediaresource;return!b&&!!c&&!!c.media_src}function x(a){return da(a)||"string"==typeof a||"number"==typeof a||"boolean"==typeof a}function y(a){return aa(cb,a)}function z(a,b){return r(a)?"deferred":s(a)?"entry":t(a)?"feed":b&&b.relationship?null!==a&&void 0!==a&&t(a)?"feed":"entry":null}function A(a,b){return ba(a,function(a){return a.name===b})}function B(a,b,c){return a?d(b,function(b){return N(a,b,c)}):null}function C(a,b){return ba(a,function(a){return a.name===b})}function D(a,b){return ba(a,function(a){return a.name===b})}function E(a,b){return B(a,b,"complexType")}function F(a,b){return B(a,b,"entityType")}function G(a){return d(a,function(a){if(ea(a.entityContainer))return a.entityContainer})}function H(a,b){return B(a,b,"entityContainer")}function I(a,b){return ba(a,function(a){return a.name===b})}function J(a,b){var c=null;if(a){var e=a.relationship,f=d(b,function(a){var b=M(a.namespace,e),c=a.association;if(b&&c){var d,f;for(d=0,f=c.length;d<f;d++)if(c[d].name===b)return c[d]}return null});if(f){var g=f.end[0];g.role!==a.toRole&&(g=f.end[1]),c=g.type}}return c}function K(a,b,c){if(a){var e=a.relationship,f=d(c,function(a){for(var b=a.entityContainer,c=0;c<b.length;c++){var d=b[c].associationSet;if(d)for(var f=0;f<d.length;f++)if(d[f].association==e)return d[f]}return null});if(f&&f.end[0]&&f.end[1])return f.end[0].entitySet==b?f.end[1].entitySet:f.end[0].entitySet}return null}function L(a,b){return d(b,function(b){var c=b.entityContainer,d=c.entitySet;if(d)for(var e=0;e<d.length;e++)if(d[e].name==a)return{entitySet:d[e],containerName:c.name,functionImport:c.functionImport};return null})}function M(a,b){return 0===b.indexOf(a)&&"."===b.charAt(a.length)?b.substr(a.length+1):null}function N(a,b,c){if(a&&b){var d=M(b.namespace,a);if(d)return ba(b[c],function(a){return a.name===d})}return null}function O(a,b){if(a===b)return a;for(var c=a.split("."),d=b.split("."),e=c.length>=d.length?c.length:d.length,f=0;f<e;f++){var g=c[f]&&fa(c[f]),h=d[f]&&fa(d[f]);if(g>h)return a;if(g<h)return b}}function P(a){for(var b in a){var c=b.toLowerCase(),d=ib[c];if(d&&b!==d){var e=a[b];delete a[b],a[d]=e}}}function Q(a){return"boolean"==typeof a?a:"string"==typeof a&&"true"===a.toLowerCase()}function R(a,b,c){var d=jb.exec(a),e=d?j(d[8]):null;if(!d||!b&&"Z"!==e){if(c)return null;throw{message:"Invalid date/time value"}}var f=fa(d[1]);f<=0&&f++;var g=d[7],h=0;if(g){if(g.length>7){if(c)return null;throw{message:"Cannot parse date/time value to given precision."}}h=i(g.substring(3),4,!0),g=i(g.substring(0,3),3,!0),g=fa(g),h=fa(h)}else g=0;var k=fa(d[4]),l=fa(d[5]),m=fa(d[6])||0;if("Z"!==e){var n=W(e),o=-n.d;k+=n.h*o,l+=n.m*o}var p=new Date;if(p.setUTCFullYear(f,fa(d[2])-1,fa(d[3])),p.setUTCHours(k,l,m,g),isNaN(p.valueOf())){if(c)return null;throw{message:"Invalid date/time value"}}return b&&(p.__edmType="Edm.DateTimeOffset",p.__offset=e),h&&(p.__ns=h),p}function S(a,b){var c=a.split("-");return 3!=c.length&&b?null:new Date(fa(c[0]),fa(c[1])-1,fa(c[2],0,0,0,0))}function T(a,b){var c=kb.exec(a);return{h:fa(c[1]),m:fa(c[2]),s:fa(c[4]),ms:fa(c[6])}}function U(a,b){return R(a,!0,b)}function V(a){var b=lb.exec(a);if(null===b)throw{message:"Invalid duration value."};var c=b[2]||"0",d=b[3]||"0",e=fa(b[4]||0),f=fa(b[5]||0),g=fa(b[6]||0),h=parseFloat(b[7]||0);if("0"!==c||"0"!==d)throw{message:"Unsupported duration value."};var j=b[8],k=0;if(j){if(j.length>7)throw{message:"Cannot parse duration value to given precision."};k=i(j.substring(3),4,!0),j=i(j.substring(0,3),3,!0),j=fa(j),k=fa(k)}else j=0;j+=1e3*h+6e4*g+36e5*f+864e5*e,"-"===b[1]&&(j=-j);var l={ms:j,__edmType:"Edm.Time"};return k&&(l.ns=k),l}function W(a){var b=a.substring(0,1);return b="+"===b?1:-1,{d:b,h:fa(a.substring(1)),m:fa(a.substring(a.indexOf(":")+1))}}function X(a,b,c){a.method||(a.method="GET"),a.headers?P(a.headers):a.headers={},void 0===a.headers.Accept&&(a.headers.Accept=b.accept),_(a.data)&&void 0===a.body&&b.write(a,c),_(a.headers["OData-MaxVersion"])||(a.headers["OData-MaxVersion"]=b.maxDataServiceVersion||"4.0"),void 0===a.async&&(a.async=!0)}function Y(a,b,c){if(a&&"object"==typeof a)for(var d in a){var e=a[d],f=Y(e,d,c);f=c(d,f,b),f!==e&&(void 0===e?delete a[d]:a[d]=f)}return a}function Z(a,b){return b("",Y(a,"",b))}var $=c("./../utils.js"),_=$.assigned,aa=$.contains,ba=$.find,ca=$.isArray,da=$.isDate,ea=$.isObject,fa=$.parseInt10,ga=function(a,b){return(a&&a.__metadata||{}).type||(b?b.type:null)},ha="Edm.",ia=ha+"Boolean",ja=ha+"Byte",ka=ha+"SByte",la=ha+"Int16",ma=ha+"Int32",na=ha+"Int64",oa=ha+"Single",pa=ha+"Double",qa=ha+"Decimal",ra=ha+"String",sa=ha+"Binary",ta=ha+"Date",ua=ha+"DateTimeOffset",va=ha+"Duration",wa=ha+"Guid",xa=ha+"Time",ya="Geography",za=ha+ya,Aa=za+"Point",Ba=za+"LineString",Ca=za+"Polygon",Da=za+"Collection",Ea=za+"MultiPolygon",Fa=za+"MultiLineString",Ga=za+"MultiPoint",Ha=ya+"Point",Ia=ya+"LineString",Ja=ya+"Polygon",Ka=ya+"Collection",La=ya+"MultiPolygon",Ma=ya+"MultiLineString",Na=ya+"MultiPoint",Oa="Geometry",Pa=ha+Oa,Qa=Pa+"Point",Ra=Pa+"LineString",Sa=Pa+"Polygon",Ta=Pa+"Collection",Ua=Pa+"MultiPolygon",Va=Pa+"MultiLineString",Wa=Pa+"MultiPoint",Xa=Oa+"Point",Ya=Oa+"LineString",Za=Oa+"Polygon",$a=Oa+"Collection",_a=Oa+"MultiPolygon",ab=Oa+"MultiLineString",bb=Oa+"MultiPoint",cb=[ra,ma,na,ia,pa,oa,ta,ua,va,xa,qa,wa,ja,la,ka,sa],db=[Pa,Qa,Ra,Sa,Ta,Ua,Va,Wa],eb=[Oa,Xa,Ya,Za,$a,_a,ab,bb],fb=[za,Aa,Ba,Ca,Da,Ea,Fa,Ga],gb=[ya,Ha,Ia,Ja,Ka,La,Ma,Na],hb=/Collection\((.*)\)/,ib={"content-type":"Content-Type","content-encoding":"Content-Encoding","content-length":"Content-Length","odata-version":"OData-Version",accept:"Accept","accept-charset":"Accept-Charset","if-match":"If-Match","if-none-match":"If-None-Match","odata-isolation":"OData-Isolation","odata-maxversion":"OData-MaxVersion",prefer:"Prefer","content-id":"Content-ID","content-transfer-encoding":"Content-Transfer-Encoding",etag:"ETag",location:"Location","odata-entityid":"OData-EntityId","preference-applied":"Preference-Applied","retry-after":"Retry-After"},jb=/^(-?\d{4,})-(\d{2})-(\d{2})T(\d{2}):(\d{2})(?::(\d{2}))?(?:\.(\d+))?(.*)$/,kb=/^(\d+):(\d+)(:(\d+)(.(\d+))?)?$/,lb=/^([+-])?P(?:(\d+)Y)?(?:(\d+)M)?(?:(\d+)D)?(?:T(?:(\d+)H)?(?:(\d+)M)?(?:(\d+)(?:\.(\d+))?S)?)?/;a.dataItemTypeName=ga,a.EDM_BINARY=sa,a.EDM_BOOLEAN=ia,a.EDM_BYTE=ja,a.EDM_DATE=ta,a.EDM_DATETIMEOFFSET=ua,a.EDM_DURATION=va,a.EDM_DECIMAL=qa,a.EDM_DOUBLE=pa,a.EDM_GEOGRAPHY=za,a.EDM_GEOGRAPHY_POINT=Aa,a.EDM_GEOGRAPHY_LINESTRING=Ba,a.EDM_GEOGRAPHY_POLYGON=Ca,a.EDM_GEOGRAPHY_COLLECTION=Da,a.EDM_GEOGRAPHY_MULTIPOLYGON=Ea,a.EDM_GEOGRAPHY_MULTILINESTRING=Fa,a.EDM_GEOGRAPHY_MULTIPOINT=Ga,a.EDM_GEOMETRY=Pa,a.EDM_GEOMETRY_POINT=Qa,a.EDM_GEOMETRY_LINESTRING=Ra,a.EDM_GEOMETRY_POLYGON=Sa,a.EDM_GEOMETRY_COLLECTION=Ta,a.EDM_GEOMETRY_MULTIPOLYGON=Ua,a.EDM_GEOMETRY_MULTILINESTRING=Va,a.EDM_GEOMETRY_MULTIPOINT=Wa,a.EDM_GUID=wa,a.EDM_INT16=la,a.EDM_INT32=ma,a.EDM_INT64=na,a.EDM_SBYTE=ka,a.EDM_SINGLE=oa,a.EDM_STRING=ra,a.EDM_TIMEOFDAY=xa,a.GEOJSON_POINT="Point",a.GEOJSON_LINESTRING="LineString",a.GEOJSON_POLYGON="Polygon",a.GEOJSON_MULTIPOINT="MultiPoint",a.GEOJSON_MULTILINESTRING="MultiLineString",a.GEOJSON_MULTIPOLYGON="MultiPolygon",a.GEOJSON_GEOMETRYCOLLECTION="GeometryCollection",a.forEachSchema=d,a.formatDateTimeOffset=g,a.formatDateTimeOffsetJSON=f,a.formatDuration=h,a.formatNumberWidth=i,a.getCanonicalTimezone=j,a.getCollectionType=k,a.invokeRequest=l,a.isBatch=m,a.isCollection=n,a.isCollectionType=o,a.isComplex=p,a.isDateTimeOffset=q,a.isDeferred=r,a.isEntry=s,a.isFeed=t,a.isGeographyEdmType=u,a.isGeometryEdmType=v,a.isNamedStream=w,a.isPrimitive=x,a.isPrimitiveEdmType=y,a.lookupComplexType=E,a.lookupDefaultEntityContainer=G,a.lookupEntityContainer=H,a.lookupEntitySet=C,a.lookupSingleton=D,a.lookupEntityType=F,a.lookupFunctionImport=I,a.lookupNavigationPropertyType=J,a.lookupNavigationPropertyEntitySet=K,a.lookupInSchema=N,a.lookupProperty=A,a.lookupInMetadata=B,a.getEntitySetInfo=L,a.maxVersion=O,a.navigationPropertyKind=z,a.normalizeHeaders=P,a.parseBool=Q,a.parseDate=S,a.parseDateTimeOffset=U,a.parseDuration=V,a.parseTimeOfDay=T,a.parseInt10=fa,a.prepareRequest=X,a.removeNamespace=M,a.traverse=Z},store:function(a,b,c){a.defaultStoreMechanism="best",a.createStore=function(b,c){c||(c=a.defaultStoreMechanism),"best"===c&&(c=DomStore.isSupported()?"dom":"memory");var e=d[c];if(e)return e.create(b);throw{message:"Failed to create store",name:b,mechanism:c}},a.DomStore=DomStore=c("./store/dom.js"),a.IndexedDBStore=IndexedDBStore=c("./store/indexeddb.js"),a.MemoryStore=MemoryStore=c("./store/memory.js");var d={indexeddb:IndexedDBStore,dom:DomStore,memory:MemoryStore};a.mechanisms=d},dom:function(a,b,c){"use strict";function d(){var a={v:this.valueOf(),t:"[object Date]"};for(var b in this)a[b]=this[b];return a}function e(a,b){if(b&&"[object Date]"===b.t){var c=new Date(b.v);for(var d in b)"t"!==d&&"v"!==d&&(c[d]=b[d]);b=c}return b}function f(a,b){return a.name+"#!#"+b}function g(a,b){return b.replace(a.name+"#!#","")}function h(a){this.name=a}var i=c("./../utils.js"),j=i.throwErrorCallback,k=i.delay,l=null;h.create=function(a){if(h.isSupported())return l=l||window.localStorage,new h(a);throw{message:"Web Storage not supported by the browser"}},h.isSupported=function(){return!!window.localStorage},h.prototype.add=function(a,b,c,d){d=d||this.defaultError;var e=this;this.contains(a,function(f){f?k(d,{message:"key already exists",key:a}):e.addOrUpdate(a,b,c,d)},d)},h.prototype.addOrUpdate=function(a,b,c,e){if(e=e||this.defaultError,a instanceof Array)e({message:"Array of keys not supported"});else{var g=f(this,a),h=Date.prototype.toJSON;try{var i=b;void 0!==i&&(Date.prototype.toJSON=d,i=window.JSON.stringify(b)),l.setItem(g,i),k(c,a,b)}catch(a){22===a.code||2147942414===a.number?k(e,{name:"QUOTA_EXCEEDED_ERR",error:a}):k(e,a)}finally{Date.prototype.toJSON=h}}},h.prototype.clear=function(a,b){b=b||this.defaultError;try{for(var c=0,d=l.length;d>0&&c<d;){var e=l.key(c);e!==g(this,e)?(l.removeItem(e),d=l.length):c++}k(a)}catch(a){k(b,a)}},h.prototype.close=function(){},h.prototype.contains=function(a,b,c){c=c||this.defaultError;try{var d=f(this,a),e=l.getItem(d);k(b,null!==e)}catch(a){k(c,a)}},h.prototype.defaultError=j,h.prototype.getAllKeys=function(a,b){b=b||this.defaultError;var c,d,e=[];try{for(c=0,d=l.length;c<d;c++){var f=l.key(c),h=g(this,f);f!==h&&e.push(h)}k(a,e)}catch(a){k(b,a)}},h.prototype.mechanism="dom",h.prototype.read=function(a,b,c){if(c=c||this.defaultError,a instanceof Array)c({message:"Array of keys not supported"});else try{var d=f(this,a),g=l.getItem(d);g=null!==g&&"undefined"!==g?window.JSON.parse(g,e):void 0,k(b,a,g)}catch(a){k(c,a)}},h.prototype.remove=function(a,b,c){if(c=c||this.defaultError,a instanceof Array)c({message:"Batches not supported"});else try{var d=f(this,a);l.removeItem(d),k(b)}catch(a){k(c,a)}},h.prototype.update=function(a,b,c,d){d=d||this.defaultError;var e=this;this.contains(a,function(f){f?e.addOrUpdate(a,b,c,d):k(d,{message:"key not found",key:a})},d)},b.exports=h},indexeddb:function(a,b,c){"use strict";function d(a,b){return function(c){var d=a||b;if(d){if("[object IDBDatabaseException]"===Object.prototype.toString.call(c))return 11===c.code?void d({name:"QuotaExceededError",error:c}):void d(c);var e;try{var f=c.target.error||c;e=f.name}catch(a){e="blocked"===c.type?"IndexedDBBlocked":"UnknownError"}d({name:e,error:c})}}}function e(a,b,c){var d=a.name,e="_odatajs_"+d,f=j.open(e);f.onblocked=c,f.onerror=c,f.onupgradeneeded=function(){var a=f.result;a.objectStoreNames.contains(d)||a.createObjectStore(d)},f.onsuccess=function(a){var e=f.result;if(!e.objectStoreNames.contains(d)){if("setVersion"in e){var g=e.setVersion("1.0");return g.onsuccess=function(){g.transaction.oncomplete=function(){b(e)},e.createObjectStore(d,null,!1)},g.onerror=c,void(g.onblocked=c)}return a.target.error={name:"DBSchemaMismatch"},void c(a)}e.onversionchange=function(a){a.target.close()},b(e)}}function f(a,b,c,f){var g=a.name,h=a.db,i=d(f,a.defaultError);if(h)return void c(h.transaction(g,b));e(a,function(d){a.db=d,c(d.transaction(g,b))},i)}function g(a){this.name=a}var h=c("./../utils.js"),i=h.throwErrorCallback,j=(h.delay,h.inBrowser()?window.mozIndexedDB||window.webkitIndexedDB||window.msIndexedDB||window.indexedDB:void 0),k=h.inBrowser()?window.IDBKeyRange||window.webkitIDBKeyRange:void 0,l=h.inBrowser()?window.IDBTransaction||window.webkitIDBTransaction||{}:{},m=l.READ_ONLY||"readonly",n=l.READ_WRITE||"readwrite";g.create=function(a){if(g.isSupported())return new g(a);throw{message:"IndexedDB is not supported on this browser"}},g.isSupported=function(){return!!j},g.prototype.add=function(a,b,c,e){var g=this.name,h=this.defaultError,i=[],j=[];a instanceof Array?(i=a,j=b):(i=[a],j=[b]),f(this,n,function(f){f.onabort=d(e,h,a,"add"),f.oncomplete=function(){a instanceof Array?c(i,j):c(a,b)};for(var k=0;k<i.length&&k<j.length;k++)f.objectStore(g).add({v:j[k]},i[k])},e)},g.prototype.addOrUpdate=function(a,b,c,e){var g=this.name,h=this.defaultError,i=[],j=[];a instanceof Array?(i=a,j=b):(i=[a],j=[b]),f(this,n,function(f){f.onabort=d(e,h),f.oncomplete=function(){a instanceof Array?c(i,j):c(a,b)};for(var k=0;k<i.length&&k<j.length;k++){var l={v:j[k]};f.objectStore(g).put(l,i[k])}},e)},g.prototype.clear=function(a,b){var c=this.name,e=this.defaultError;f(this,n,function(f){f.onerror=d(b,e),f.oncomplete=function(){a()},f.objectStore(c).clear()},b)},g.prototype.close=function(){this.db&&(this.db.close(),this.db=null)},g.prototype.contains=function(a,b,c){var e=this.name,g=this.defaultError;f(this,m,function(f){var h=f.objectStore(e),i=h.get(a);f.oncomplete=function(){b(!!i.result)},f.onerror=d(c,g)},c)},g.prototype.defaultError=i,g.prototype.getAllKeys=function(a,b){var c=this.name,e=this.defaultError;f(this,n,function(f){var g=[];f.oncomplete=function(){a(g)};var h=f.objectStore(c).openCursor();h.onerror=d(b,e),h.onsuccess=function(a){var b=a.target.result;b&&(g.push(b.key),b.continue.call(b))}},b)},g.prototype.mechanism="indexeddb",g.prototype.read=function(a,b,c){var e=this.name,g=this.defaultError,h=a instanceof Array?a:[a];f(this,m,function(f){var i=[];f.onerror=d(c,g,a,"read"),f.oncomplete=function(){a instanceof Array?b(h,i):b(h[0],i[0])};for(var j=0;j<h.length;j++){var k=f.objectStore(e);k.get.call(k,h[j]).onsuccess=function(a){var b=a.target.result;i.push(b?b.v:void 0)}}},c)},g.prototype.remove=function(a,b,c){var e=this.name,g=this.defaultError,h=a instanceof Array?a:[a];f(this,n,function(a){a.onerror=d(c,g),a.oncomplete=function(){b()};for(var f=0;f<h.length;f++){var i=a.objectStore(e);i.delete.call(i,h[f])}},c)},g.prototype.update=function(a,b,c,e){var g=this.name,h=this.defaultError,i=[],j=[];a instanceof Array?(i=a,j=b):(i=[a],j=[b]),f(this,n,function(f){f.onabort=d(e,h),f.oncomplete=function(){a instanceof Array?c(i,j):c(a,b)};for(var l=0;l<i.length&&l<j.length;l++){var m=f.objectStore(g).openCursor(k.only(i[l])),n={v:j[l]};m.pair={key:i[l],value:n},m.onsuccess=function(a){var b=a.target.result;b?b.update(a.target.pair.value):f.abort()}}},e)},b.exports=g},memory:function(a,b,c){"use strict";function d(a){function b(a,b){var c;return a instanceof Array&&(c="Array of keys not supported"),void 0!==a&&null!==a||(c="Invalid key"),!c||(g(b,{message:c}),!1)}var c=[],d=[],e={};this.name=a;var f=function(a){return a||this.defaultError};this.add=function(a,c,d,g){g=f(g),b(a,g)&&(e.hasOwnProperty(a)?g({message:"key already exists",key:a}):this.addOrUpdate(a,c,d,g))},this.addOrUpdate=function(a,h,i,j){if(j=f(j),b(a,j)){var k=e[a];void 0===k&&(k=c.length>0?c.splice(0,1):d.length),d[k]=h,e[a]=k,g(i,a,h)}},this.clear=function(a){d=[],e={},c=[],g(a)},this.contains=function(a,b){var c=e.hasOwnProperty(a);g(b,c)},this.getAllKeys=function(a){var b=[];for(var c in e)b.push(c);g(a,b)},this.read=function(a,c,h){if(h=f(h),b(a,h)){var i=e[a];g(c,a,d[i])}},this.remove=function(a,h,i){if(i=f(i),b(a,i)){var j=e[a];void 0!==j&&(j===d.length-1?d.pop():(d[j]=void 0,c.push(j)),delete e[a],0===d.length&&(c=[])),g(h)}},this.update=function(a,c,d,g){g=f(g),b(a,g)&&(e.hasOwnProperty(a)?this.addOrUpdate(a,c,d,g):g({message:"key not found",key:a}))}}var e=c("./../utils.js"),f=e.throwErrorCallback,g=e.delay;d.create=function(a){return new d(a)},d.isSupported=function(){return!0},d.prototype.close=function(){},d.prototype.defaultError=f,d.prototype.mechanism="memory",b.exports=d},utils:function(a,b,c){"use strict";function d(){return"undefined"!=typeof window}function e(a){return null!==a&&void 0!==a}function f(a,b){var c,d;for(c=0,d=a.length;c<d;c++)if(a[c]===b)return!0;return!1}function g(a,b){return void 0!==a?a:b}function h(a){if(1===arguments.length)return void window.setTimeout(a,0);var b=Array.prototype.slice.call(arguments,1);window.setTimeout(function(){a.apply(this,b)},0)}function i(a,b,c){if(!a)throw{message:"Assert fired: "+b,data:c}}function j(a,b){for(var c in b)a[c]=b[c];return a}function k(a,b){if(a){var c,d;for(c=0,d=a.length;c<d;c++)if(b(a[c]))return a[c]}return null}function l(a){return"[object Array]"===Object.prototype.toString.call(a)}function m(a){return"[object Date]"===Object.prototype.toString.call(a)}function n(a){return"object"==typeof a}function o(a){return parseInt(a,10)}function p(a,b,c){a.hasOwnProperty(b)&&(a[c]=a[b],delete a[b])}function q(a){throw a}function r(a){return a.trim?a.trim():a.replace(/^\s+|\s+$/g,"")}function s(a,b){return void 0!==a?a:b}function t(a){var b={isAbsolute:!1};if(a){var c=K.exec(a);if(c){var d,e;for(d=0,e=L.length;d<e;d++)c[d+1]&&(b[L[d]]=c[d+1])}b.scheme&&(b.isAbsolute=!0)}return b}function u(a){return"".concat(a.scheme||"",a.authority||"",a.path||"",a.query||"",a.fragment||"")}function v(a){var b=t(a),c=b.scheme,d=b.authority;if(c&&(b.scheme=c.toLowerCase(),d)){var e=M.exec(d);e&&(b.authority="//"+(e[1]?e[1]+"@":"")+e[2].toLowerCase()+(e[3]?":"+e[3]:""))}return a=u(b),a.replace(N,function(a){return a.toLowerCase()})}function w(a,b){if(!b)return a;var c=t(a);if(c.isAbsolute)return a;var d,e=t(b),f={};return c.authority?(f.authority=c.authority,d=c.path,f.query=c.query):(c.path?(d="/"===c.path.charAt(0)?c.path:x(c.path,e.path),f.query=c.query):(d=e.path,f.query=c.query||e.query),f.authority=e.authority),f.path=y(d),f.scheme=e.scheme,f.fragment=c.fragment,u(f)}function x(a,b){var c,d="/";return b&&(c=b.lastIndexOf("/"),d=b.substring(0,c),"/"!==d.charAt(d.length-1)&&(d+="/")),d+a}function y(a){for(var b,c="",d="";a;)0===a.indexOf("..")||0===a.indexOf(".")?a=a.replace(/^\.\.?\/?/g,""):0===a.indexOf("/..")?(a=a.replace(/^\/\..\/?/g,"/"),b=c.lastIndexOf("/"),c=-1===b?"":c.substring(0,b)):0===a.indexOf("/.")?a=a.replace(/^\/\.\/?/g,"/"):(d=a,b=a.indexOf("/",1),-1!==b&&(d=a.substring(0,b)),c+=d,a=a.replace(d,""));return c}function z(a){var b=[];if(void 0===window.atob)b=A(a);else for(var c=window.atob(a),d=0;d<c.length;d++)b.push(c.charCodeAt(d));for(var e="",f="0123456789ABCDEF",g=0;g<b.length;g++){var h=b[g];e+=f[h>>4],e+=f[15&h]}return e}function A(a){for(var b="",c=0;c<a.length;c++){var d=B(a[c]),e="";null!==d&&(e=d.toString(2),b+=C(e))}var f=[],g=parseInt(b.length/8,10);for(c=0;c<g;c++){var h=parseInt(b.substring(8*c,8*(c+1)),2);f.push(h)}return f}function B(a){var b=a.charCodeAt(0),c=65;return b>=65&&b<=90?b-c:b>=97&&b<=122?b-c-6:b>=48&&b<=57?b+4:"+"==a?62:"/"==a?63:null}function C(a){for(;a.length<6;)a="0"+a;return a}function D(a){return a&&a.value?a.value.length:0}function E(a,b,c){if(void 0===a||void 0===a.value)return a;b<0&&(b=0);var d=D(a);d<c&&(c=d);var e={};for(var f in a)e[f]="value"==f?a[f].slice(b,c):a[f];return e}function F(a,b){return void 0===b||void 0===b.value?a:void 0===a||0===Object.keys(a).length?b:void 0===a.value?(a.value=b.value,a):(a.value=a.value.concat(b.value),a)}function G(a,b){return-1!==a.indexOf(b,a.length-b.length)}function H(a,b){return 0===a.indexOf(b)}function I(a,b){var c=b;if(!e(a))return c;switch(a.toLowerCase()){case"none":c=0;break;case"minimal":c=1;break;case"full":c=2}return c}var J=function(a){return window.ActiveXObject?new window.ActiveXObject(a):null},K=/^([^:\/?#]+:)?(\/\/[^\/?#]*)?([^?#:]+)?(\?[^#]*)?(#.*)?/,L=["scheme","authority","path","query","fragment"],M=/^\/{0,2}(?:([^@]*)@)?([^:]+)(?::{1}(\d+))?/,N=/%[0-9A-F]{2}/gi;a.inBrowser=d,a.activeXObject=J,a.assigned=e,a.contains=f,a.defined=g,a.delay=h,a.djsassert=i,a.extend=j,a.find=k,a.getURIInfo=t,a.isArray=l,a.isDate=m,a.isObject=n,a.normalizeURI=w,a.normalizeURICase=v,a.parseInt10=o,a.renameProperty=p,a.throwErrorCallback=q,a.trimString=r,a.undefinedDefault=s,a.decodeBase64=A,a.convertByteArrayToHexString=z,a.getJsonValueArraryLength=D,a.sliceJsonValueArray=E,a.concatJsonValueArray=F,a.startsWith=H,a.endsWith=G,a.getFormatKind=I},xml:function(a,b,c){"use strict";function d(a){return/(^\s)|(\s$)/.test(a)}function e(a){var b=/^\s*$/;return null===a||b.test(a)}function f(a){for(;null!==a&&1===a.nodeType;){var b=q(a,"space",$);if("preserve"===b)return!0;if("default"===b)break;a=a.parentNode}return!1}function g(a){var b=a.nodeName;return"xmlns"==b||0===b.indexOf("xmlns:")}function h(a,b,c){try{a.setProperty(b,c)}catch(a){}}function i(){var a=R("Msxml2.DOMDocument.3.0");return a&&(h(a,"ProhibitDTD",!0),h(a,"MaxElementDepth",256),h(a,"AllowDocumentFunction",!1),h(a,"AllowXsltScript",!1)),a}function j(){try{var a=R("Msxml2.DOMDocument.6.0");return a&&(a.async=!0),a}catch(a){return i()}}function k(a){var b=j();if(!b)return null;b.loadXML(a);var c=b.parseError;return 0!==c.errorCode&&l(c.reason,c.srcText,a),b}function l(a,b,c){throw"string"==typeof a&&(a={message:a}),T(a,{srcText:b||"",errorXmlText:c||""})}function m(a){var b=void 0;b=Q.inBrowser()?window.DOMParser&&new window.DOMParser:new(c("xmldom").DOMParser);var d;if(!b)return d=k(a),d||l("XML DOM parser not supported"),d;try{d=b.parseFromString(a,"text/xml")}catch(b){l(b,"",a)}var e=d.documentElement,f=e.namespaceURI,g=A(e);if("parsererror"===g&&f===_){var h=w(e,_,"sourcetext"),i=h?C(h):"";l(z(e)||"",i,a)}if("h3"===g&&f===Y||x(e,Y,"h3")){for(var j="",m=[],n=e.firstChild;n;)1===n.nodeType&&(j+=z(n)||""),m.push(n.nextSibling),n=n.firstChild||m.shift();j+=z(e)||"",l(j,"",a)}return d}function n(a,b){return a?a+":"+b:b}function o(a,b){if(d(b.data)){var c=r(a,$,"space");c||(c=I(a.ownerDocument,$,n("xml","space")),H(a,c)),c.value="preserve"}return a.appendChild(b),a}function p(a,b){var c,d,e=a.attributes;for(c=0,d=e.length;c<d;c++)b(e.item(c))}function q(a,b,c){var d=r(a,b,c);return d?C(d):null}function r(a,b,c){var d=a.attributes;return d.getNamedItemNS?d.getNamedItemNS(c||null,b):d.getQualifiedItem(b,c)||null}function s(a,b){var c=r(a,"base",$);return(c?V(c.value,b):b)||null}function t(a,b){D(a,!1,function(a){return 1===a.nodeType&&b(a),!0})}function u(a,b,c){var d,e,f=c.split("/");for(d=0,e=f.length;d<e;d++)a=a&&w(a,b,f[d]);return a||null}function v(a,b,c){var d=c.lastIndexOf("/"),e=c.substring(d+1),f=c.substring(0,d),g=f?u(a,b,f):a;return g?"@"===e.charAt(0)?r(g,e.substring(1),b):w(g,b,e):null}function w(a,b,c){return y(a,b,c,!1)}function x(a,b,c){if(a.getElementsByTagNameNS){var d=a.getElementsByTagNameNS(b,c);return d.length>0?d[0]:null}return y(a,b,c,!0)}function y(a,b,c,d){var e=null;return D(a,d,function(a){if(1===a.nodeType){var d=!b||B(a)===b,f=!c||A(a)===c;d&&f&&(e=a)}return null===e}),e}function z(a){var b,c=null,d=9===a.nodeType&&a.documentElement?a.documentElement:a,g=!1===d.ownerDocument.preserveWhiteSpace;return D(d,!1,function(a){if(3===a.nodeType||4===a.nodeType){var h=C(a),i=g||!e(h);i||(void 0===b&&(b=f(d)),i=b),i&&(c?c+=h:c=h)}return!0}),c}function A(a){return a.localName||a.baseName}function B(a){return a.namespaceURI||null}function C(a){return 1===a.nodeType?z(a):a.nodeValue}function D(a,b,c){for(var d=[],e=a.firstChild,f=!0;e&&f;)(f=c(e))&&(b&&e.firstChild&&d.push(e.firstChild),e=e.nextSibling||d.shift())}function E(a,b,c){for(var d=a.nextSibling;d;){if(1===d.nodeType){var e=!b||B(d)===b,f=!c||A(d)===c;if(e&&f)return d}d=d.nextSibling}return null}function F(){var a=window.document.implementation;return a&&a.createDocument?a.createDocument(null,null,null):j()}function G(a,b){if(!U(b))return H(a,b);var c,d;for(c=0,d=b.length;c<d;c++)b[c]&&H(a,b[c]);return a}function H(a,b){if(S(a!==b,"xmlAppendChild() - parent and child are one and the same!"),b){if("string"==typeof b)return o(a,M(a.ownerDocument,b));2===b.nodeType?a.setAttributeNodeNS?a.setAttributeNodeNS(b):a.setAttributeNode(b):a.appendChild(b)}return a}function I(a,b,c,d){var e=a.createAttributeNS&&a.createAttributeNS(b,c)||a.createNode(2,c,b||void 0);return e.value=d||"",e}function J(a,b,c,d){return G(a.createElementNS&&a.createElementNS(nampespaceURI,c)||a.createNode(1,c,nampespaceURI||void 0),d||[])}function K(a,b,c){return I(a,Z,n("xmlns",c),b)}function L(a,b){for(var c="<c>"+b+"</c>",d=m(c),e=d.documentElement,f=("importNode"in a?a.importNode(e,!0):e),g=a.createDocumentFragment(),h=f.firstChild;h;)g.appendChild(h),h=h.nextSibling;return g}function M(a,b){return a.createTextNode(b)}function N(a,b,c,d,e){var f,g,h="",i=e.split("/"),j=w,k=J,l=b;for(f=0,g=i.length;f<g;f++){h=i[f],"@"===h.charAt(0)&&(h=h.substring(1),j=r,k=I);var m=j(l,c,h);m||(m=k(a,c,n(d,h)),H(l,m)),l=m}return l}function O(a){var b=window.XMLSerializer;if(b){return(new b).serializeToString(a)}if(a.xml)return a.xml;throw{message:"XML serialization unsupported"}}function P(a){var b,c=a.childNodes,d=c.length;if(0===d)return"";var e=a.ownerDocument,f=e.createDocumentFragment(),g=e.createElement("c");for(f.appendChild(g),b=0;b<d;b++)g.appendChild(c[b]);var h=O(f);for(h=h.substr(3,h.length-7),b=0;b<d;b++)a.appendChild(g.childNodes[b]);return h}var Q=c("./utils.js"),R=Q.activeXObject,S=Q.djsassert,T=Q.extend,U=Q.isArray,V=Q.normalizeURI,W="http://",X=W+"www.w3.org/",Y=X+"1999/xhtml",Z=X+"2000/xmlns/",$=X+"XML/1998/namespace",_=W+"www.mozilla.org/newlayout/xml/parsererror.xml";a.http=W,a.w3org=X,a.xmlNS=$,a.xmlnsNS=Z,a.hasLeadingOrTrailingWhitespace=d,a.isXmlNSDeclaration=g,a.xmlAppendChild=H,a.xmlAppendChildren=G,a.xmlAttributeNode=r,a.xmlAttributes=p,a.xmlAttributeValue=q,a.xmlBaseURI=s,a.xmlChildElements=t,a.xmlFindElementByPath=u,a.xmlFindNodeByPath=v,a.xmlFirstChildElement=w,a.xmlFirstDescendantElement=x,a.xmlInnerText=z,a.xmlLocalName=A,a.xmlNamespaceURI=B,a.xmlNodeValue=C,a.xmlDom=F,a.xmlNewAttribute=I,a.xmlNewElement=J,a.xmlNewFragment=L,a.xmlNewNodeByPath=N,a.xmlNewNSDeclaration=K,a.xmlNewText=M,a.xmlParse=m,a.xmlQualifiedName=n,a.xmlSerialize=O,a.xmlSerializeDescendants=P,a.xmlSiblingElement=E}},c={},d=function(a){var e=a.substring(a.lastIndexOf("/")+1,a.length-3);return c[e]?c[e].exports:(c[e]={exports:{}},b[e].call(this,c[e].exports,c[e],d),c[e].exports)};window.odatajs={},a.call(this,window.odatajs,window.odatajs,d)}();
//# sourceMappingURL=odatajs-4.0.4.map;


==> icde2022-reviews_files/site <==
.clearfix{*zoom:1}.clearfix:before,.clearfix:after{display:table;content:"";line-height:0}.clearfix:after{clear:both}.hide-text{font:0/0 a;color:transparent;text-shadow:none;background-color:transparent;border:0}.input-block-level{display:block;width:100%;min-height:30px;-webkit-box-sizing:border-box;-moz-box-sizing:border-box;box-sizing:border-box}article,aside,details,figcaption,figure,footer,header,hgroup,nav,section{display:block}audio,canvas,video{display:inline-block;*display:inline;*zoom:1}audio:not([controls]){display:none}html{font-size:100%;-webkit-text-size-adjust:100%;-ms-text-size-adjust:100%}a:focus{outline:thin dotted #333;outline:5px auto -webkit-focus-ring-color;outline-offset:-2px}a:hover,a:active{outline:0}sub,sup{position:relative;font-size:75%;line-height:0;vertical-align:baseline}sup{top:-.5em}sub{bottom:-.25em}img{max-width:100%;width:auto \9;height:auto;vertical-align:middle;border:0;-ms-interpolation-mode:bicubic}#map_canvas img,.google-maps img{max-width:none}button,input,select,textarea{margin:0;font-size:100%;vertical-align:middle}button,input{*overflow:visible;line-height:normal}button::-moz-focus-inner,input::-moz-focus-inner{padding:0;border:0}button,html input[type="button"],input[type="reset"],input[type="submit"]{-webkit-appearance:button;cursor:pointer}label,select,button,input[type="button"],input[type="reset"],input[type="submit"],input[type="radio"],input[type="checkbox"]{cursor:pointer}input[type="search"]{-webkit-box-sizing:content-box;-moz-box-sizing:content-box;box-sizing:content-box;-webkit-appearance:textfield}input[type="search"]::-webkit-search-decoration,input[type="search"]::-webkit-search-cancel-button{-webkit-appearance:none}textarea{overflow:auto;vertical-align:top}@media print{*{text-shadow:none!important;color:#000!important;background:transparent!important;box-shadow:none!important}a,a:visited{text-decoration:underline}a[href]:after{content:" (" attr(href) ")"}abbr[title]:after{content:" (" attr(title) ")"}.ir a:after,a[href^="javascript:"]:after,a[href^="#"]:after{content:""}pre,blockquote{border:1px solid #999;page-break-inside:avoid}thead{display:table-header-group}tr,img{page-break-inside:avoid}img{max-width:100%!important}@page{margin:.5cm}p,h2,h3{orphans:3;widows:3}h2,h3{page-break-after:avoid}}body{margin:0;font-family:"Helvetica Neue",Helvetica,Arial,sans-serif;font-size:14px;line-height:20px;color:#333;background-color:#fff}a{color:#007294;text-decoration:none}a:hover,a:focus{color:#007ea3;text-decoration:underline}.img-rounded{-webkit-border-radius:6px;-moz-border-radius:6px;border-radius:6px}.img-polaroid{padding:4px;background-color:#fff;border:1px solid #ccc;border:1px solid rgba(0,0,0,.2);-webkit-box-shadow:0 1px 3px rgba(0,0,0,.1);-moz-box-shadow:0 1px 3px rgba(0,0,0,.1);box-shadow:0 1px 3px rgba(0,0,0,.1)}.img-circle{-webkit-border-radius:500px;-moz-border-radius:500px;border-radius:500px}.row{margin-left:-20px;*zoom:1}.row:before,.row:after{display:table;content:"";line-height:0}.row:after{clear:both}[class*="span"]{float:left;min-height:1px;margin-left:20px}.container,.navbar-static-top .container,.navbar-fixed-top .container,.navbar-fixed-bottom .container{width:97%}.span12{width:940px}.span11{width:860px}.span10{width:780px}.span9{width:700px}.span8{width:620px}.span7{width:540px}.span6{width:460px}.span5{width:380px}.span4{width:300px}.span3{width:220px}.span2{width:140px}.span1{width:60px}.offset12{margin-left:980px}.offset11{margin-left:900px}.offset10{margin-left:820px}.offset9{margin-left:740px}.offset8{margin-left:660px}.offset7{margin-left:580px}.offset6{margin-left:500px}.offset5{margin-left:420px}.offset4{margin-left:340px}.offset3{margin-left:260px}.offset2{margin-left:180px}.offset1{margin-left:100px}.row-fluid{width:100%;*zoom:1}.row-fluid:before,.row-fluid:after{display:table;content:"";line-height:0}.row-fluid:after{clear:both}.row-fluid [class*="span"]{display:block;width:100%;min-height:30px;-webkit-box-sizing:border-box;-moz-box-sizing:border-box;box-sizing:border-box;float:left;margin-left:2.127659574%;*margin-left:2.074468085%}.row-fluid [class*="span"]:first-child{margin-left:0}.row-fluid .controls-row [class*="span"]+[class*="span"]{margin-left:2.127659574%}.row-fluid .span12{width:100%;*width:99.946808511%}.row-fluid .span11{width:91.489361702%;*width:91.436170213%}.row-fluid .span10{width:82.978723404%;*width:82.925531915%}.row-fluid .span9{width:74.468085106%;*width:74.414893617%}.row-fluid .span8{width:65.957446809%;*width:65.904255319%}.row-fluid .span7{width:57.446808511%;*width:57.393617021%}.row-fluid .span6{width:48.936170213%;*width:48.882978723%}.row-fluid .span5{width:40.425531915%;*width:40.372340426%}.row-fluid .span4{width:31.914893617%;*width:31.861702128%}.row-fluid .span3{width:23.404255319%;*width:23.35106383%}.row-fluid .span2{width:14.893617021%;*width:14.840425532%}.row-fluid .span1{width:6.382978723%;*width:6.329787234%}.row-fluid .offset12{margin-left:104.255319149%;*margin-left:104.14893617%}.row-fluid .offset12:first-child{margin-left:102.127659574%;*margin-left:102.021276596%}.row-fluid .offset11{margin-left:95.744680851%;*margin-left:95.638297872%}.row-fluid .offset11:first-child{margin-left:93.617021277%;*margin-left:93.510638298%}.row-fluid .offset10{margin-left:87.234042553%;*margin-left:87.127659574%}.row-fluid .offset10:first-child{margin-left:85.106382979%;*margin-left:85%}.row-fluid .offset9{margin-left:78.723404255%;*margin-left:78.617021277%}.row-fluid .offset9:first-child{margin-left:76.595744681%;*margin-left:76.489361702%}.row-fluid .offset8{margin-left:70.212765957%;*margin-left:70.106382979%}.row-fluid .offset8:first-child{margin-left:68.085106383%;*margin-left:67.978723404%}.row-fluid .offset7{margin-left:61.70212766%;*margin-left:61.595744681%}.row-fluid .offset7:first-child{margin-left:59.574468085%;*margin-left:59.468085106%}.row-fluid .offset6{margin-left:53.191489362%;*margin-left:53.085106383%}.row-fluid .offset6:first-child{margin-left:51.063829787%;*margin-left:50.957446809%}.row-fluid .offset5{margin-left:44.680851064%;*margin-left:44.574468085%}.row-fluid .offset5:first-child{margin-left:42.553191489%;*margin-left:42.446808511%}.row-fluid .offset4{margin-left:36.170212766%;*margin-left:36.063829787%}.row-fluid .offset4:first-child{margin-left:34.042553191%;*margin-left:33.936170213%}.row-fluid .offset3{margin-left:27.659574468%;*margin-left:27.553191489%}.row-fluid .offset3:first-child{margin-left:25.531914894%;*margin-left:25.425531915%}.row-fluid .offset2{margin-left:19.14893617%;*margin-left:19.042553191%}.row-fluid .offset2:first-child{margin-left:17.021276596%;*margin-left:16.914893617%}.row-fluid .offset1{margin-left:10.638297872%;*margin-left:10.531914894%}.row-fluid .offset1:first-child{margin-left:8.510638298%;*margin-left:8.404255319%}[class*="span"].hide,.row-fluid [class*="span"].hide{display:none}[class*="span"].pull-right,.row-fluid [class*="span"].pull-right{float:right}.container{margin-right:auto;margin-left:auto;*zoom:1}.container:before,.container:after{display:table;content:"";line-height:0}.container:after{clear:both}.container-fluid{padding-right:20px;padding-left:20px;*zoom:1}.container-fluid:before,.container-fluid:after{display:table;content:"";line-height:0}.container-fluid:after{clear:both}p{margin:0 0 10px}.lead{margin-bottom:20px;font-size:21px;font-weight:200;line-height:30px}small{font-size:85%}strong{font-weight:bold}em{font-style:italic}cite{font-style:normal}.muted{color:#6c757d}a.muted:hover,a.muted:focus{color:#545b62}.text-warning{color:#c09853}a.text-warning:hover,a.text-warning:focus{color:#a47e3c}.text-error{color:#b94a48}a.text-error:hover,a.text-error:focus{color:#953b39}.text-info{color:#2d6987}a.text-info:hover,a.text-info:focus{color:#204b61}.text-success{color:#417e42}a.text-success:hover,a.text-success:focus{color:#2f5c30}.text-left{text-align:left}.text-right{text-align:right}.text-center{text-align:center}h1,h2,h3,h4,h5,h6{margin:10px 0;font-family:inherit;font-weight:bold;line-height:20px;color:inherit;text-rendering:optimizelegibility}h1 small,h2 small,h3 small,h4 small,h5 small,h6 small{font-weight:normal;line-height:1;color:#6c757d}h1,h2,h3{line-height:40px}h1{font-size:38.5px}h2{font-size:31.5px}h3{font-size:24.5px}h4{font-size:17.5px}h5{font-size:14px}h6{font-size:11.9px}h1 small{font-size:24.5px}h2 small{font-size:17.5px}h3 small{font-size:14px}h4 small{font-size:14px}.page-header{padding-bottom:9px;margin:20px 0 30px;border-bottom:1px solid #eee}ul,ol{padding:0;margin:0 0 10px 25px}ul ul,ul ol,ol ol,ol ul{margin-bottom:0}li{line-height:20px}ul.unstyled,ol.unstyled{margin-left:0;list-style:none}ul.inline,ol.inline{margin-left:0;list-style:none}ul.inline>li,ol.inline>li{display:inline-block;*display:inline;*zoom:1;padding-left:5px;padding-right:5px}dl{margin-bottom:20px}dt,dd{line-height:20px}dt{font-weight:bold}dd{margin-left:10px}.dl-horizontal{*zoom:1}.dl-horizontal:before,.dl-horizontal:after{display:table;content:"";line-height:0}.dl-horizontal:after{clear:both}.dl-horizontal dt{float:left;width:160px;clear:left;text-align:right;overflow:hidden;text-overflow:ellipsis;white-space:nowrap}.dl-horizontal dd{margin-left:180px}hr{margin:20px 0;border:0;border-top:1px solid #eee;border-bottom:1px solid #fff}abbr[title],abbr[data-original-title]{cursor:help;border-bottom:1px dotted #6c757d}abbr.initialism{font-size:90%;text-transform:uppercase}blockquote{padding:0 0 0 15px;margin:0 0 20px;border-left:5px solid #eee}blockquote p{margin-bottom:0;font-size:17.5px;font-weight:300;line-height:1.25}blockquote small{display:block;line-height:20px;color:#6c757d}blockquote small:before{content:'— '}blockquote.pull-right{float:right;padding-right:15px;padding-left:0;border-right:5px solid #eee;border-left:0}blockquote.pull-right p,blockquote.pull-right small{text-align:right}blockquote.pull-right small:before{content:''}blockquote.pull-right small:after{content:' —'}q:before,q:after,blockquote:before,blockquote:after{content:""}address{display:block;margin-bottom:20px;font-style:normal;line-height:20px}code,pre{padding:0 3px 2px;font-family:Monaco,Menlo,Consolas,"Courier New",monospace;font-size:12px;color:#333;-webkit-border-radius:3px;-moz-border-radius:3px;border-radius:3px}code{padding:2px 4px;color:#d14;background-color:#f7f7f9;border:1px solid #e1e1e8;white-space:nowrap}pre{display:block;padding:9.5px;margin:0 0 10px;font-size:13px;line-height:20px;word-break:break-all;word-wrap:break-word;white-space:pre;white-space:pre-wrap;background-color:#f5f5f5;border:1px solid #ccc;border:1px solid rgba(0,0,0,.15);-webkit-border-radius:4px;-moz-border-radius:4px;border-radius:4px}pre.prettyprint{margin-bottom:20px}pre code{padding:0;color:inherit;white-space:pre;white-space:pre-wrap;background-color:transparent;border:0}.pre-scrollable{max-height:340px;overflow-y:scroll}form{margin:0 0 20px}fieldset{padding:0;margin:0;border:0}legend{display:block;width:100%;padding:0;margin-bottom:20px;font-size:21px;line-height:40px;color:#333;border:0;border-bottom:1px solid #e5e5e5}legend small{font-size:15px;color:#6c757d}label,input,button,select,textarea{font-size:14px;font-weight:normal;line-height:20px}input,button,select,textarea{font-family:"Helvetica Neue",Helvetica,Arial,sans-serif}label{display:block;margin-bottom:5px}select,textarea,input[type="text"],input[type="password"],input[type="datetime"],input[type="datetime-local"],input[type="date"],input[type="month"],input[type="time"],input[type="week"],input[type="number"],input[type="email"],input[type="url"],input[type="search"],input[type="tel"],input[type="color"],.uneditable-input{display:inline-block;height:20px;padding:4px 6px;margin-bottom:10px;font-size:14px;line-height:20px;color:#555;-webkit-border-radius:4px;-moz-border-radius:4px;border-radius:4px;vertical-align:middle}input,textarea,.uneditable-input{width:206px}textarea{height:auto}textarea,input[type="text"],input[type="password"],input[type="datetime"],input[type="datetime-local"],input[type="date"],input[type="month"],input[type="time"],input[type="week"],input[type="number"],input[type="email"],input[type="url"],input[type="search"],input[type="tel"],input[type="color"],.uneditable-input{background-color:#fff;border:1px solid #ccc;-webkit-box-shadow:inset 0 1px 1px rgba(0,0,0,.075);-moz-box-shadow:inset 0 1px 1px rgba(0,0,0,.075);box-shadow:inset 0 1px 1px rgba(0,0,0,.075);-webkit-transition:border linear .2s,box-shadow linear .2s;-moz-transition:border linear .2s,box-shadow linear .2s;-o-transition:border linear .2s,box-shadow linear .2s;transition:border linear .2s,box-shadow linear .2s}textarea:focus,input[type="text"]:focus,input[type="password"]:focus,input[type="datetime"]:focus,input[type="datetime-local"]:focus,input[type="date"]:focus,input[type="month"]:focus,input[type="time"]:focus,input[type="week"]:focus,input[type="number"]:focus,input[type="email"]:focus,input[type="url"]:focus,input[type="search"]:focus,input[type="tel"]:focus,input[type="color"]:focus,.uneditable-input:focus{border-color:rgba(82,168,236,.8);outline:0;outline:thin dotted \9;-webkit-box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 8px rgba(82,168,236,.6);-moz-box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 8px rgba(82,168,236,.6);box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 8px rgba(82,168,236,.6)}input[type="radio"],input[type="checkbox"]{margin:4px 0 0;*margin-top:0;margin-top:1px \9;line-height:normal}input[type="file"],input[type="image"],input[type="submit"],input[type="reset"],input[type="button"],input[type="radio"],input[type="checkbox"]{width:auto}select,input[type="file"]{height:30px;*margin-top:4px;line-height:30px}select{width:220px;border:1px solid #ccc;background-color:#fff}select[multiple],select[size]{height:auto}select:focus,input[type="file"]:focus,input[type="radio"]:focus,input[type="checkbox"]:focus{outline:thin dotted #333;outline:5px auto -webkit-focus-ring-color;outline-offset:-2px}.uneditable-input,.uneditable-textarea{color:#6c757d;background-color:#fcfcfc;border-color:#ccc;-webkit-box-shadow:inset 0 1px 2px rgba(0,0,0,.025);-moz-box-shadow:inset 0 1px 2px rgba(0,0,0,.025);box-shadow:inset 0 1px 2px rgba(0,0,0,.025);cursor:not-allowed}.uneditable-input{overflow:hidden;white-space:nowrap}.uneditable-textarea{width:auto;height:auto}input:-moz-placeholder,textarea:-moz-placeholder{color:#707070}input:-ms-input-placeholder,textarea:-ms-input-placeholder{color:#707070}input::-webkit-input-placeholder,textarea::-webkit-input-placeholder{color:#707070}.radio,.checkbox{min-height:20px;padding-left:20px}.radio input[type="radio"],.checkbox input[type="checkbox"]{float:left;margin-left:-20px}.controls>.radio:first-child,.controls>.checkbox:first-child{padding-top:5px}.radio.inline,.checkbox.inline{display:inline-block;padding-top:5px;margin-bottom:0;vertical-align:middle}.radio.inline+.radio.inline,.checkbox.inline+.checkbox.inline{margin-left:10px}.input-mini{width:60px}.input-small{width:90px}.input-medium{width:150px}.input-large{width:210px}.input-xlarge{width:270px}.input-xxlarge{width:530px}input[class*="span"],select[class*="span"],textarea[class*="span"],.uneditable-input[class*="span"],.row-fluid input[class*="span"],.row-fluid select[class*="span"],.row-fluid textarea[class*="span"],.row-fluid .uneditable-input[class*="span"]{float:none;margin-left:0}.input-append input[class*="span"],.input-append .uneditable-input[class*="span"],.input-prepend input[class*="span"],.input-prepend .uneditable-input[class*="span"],.row-fluid input[class*="span"],.row-fluid select[class*="span"],.row-fluid textarea[class*="span"],.row-fluid .uneditable-input[class*="span"],.row-fluid .input-prepend [class*="span"],.row-fluid .input-append [class*="span"]{display:inline-block}input,textarea,.uneditable-input{margin-left:0}.controls-row [class*="span"]+[class*="span"]{margin-left:20px}input.span12,textarea.span12,.uneditable-input.span12{width:926px}input.span11,textarea.span11,.uneditable-input.span11{width:846px}input.span10,textarea.span10,.uneditable-input.span10{width:766px}input.span9,textarea.span9,.uneditable-input.span9{width:686px}input.span8,textarea.span8,.uneditable-input.span8{width:606px}input.span7,textarea.span7,.uneditable-input.span7{width:526px}input.span6,textarea.span6,.uneditable-input.span6{width:446px}input.span5,textarea.span5,.uneditable-input.span5{width:366px}input.span4,textarea.span4,.uneditable-input.span4{width:286px}input.span3,textarea.span3,.uneditable-input.span3{width:206px}input.span2,textarea.span2,.uneditable-input.span2{width:126px}input.span1,textarea.span1,.uneditable-input.span1{width:46px}.controls-row{*zoom:1}.controls-row:before,.controls-row:after{display:table;content:"";line-height:0}.controls-row:after{clear:both}.controls-row [class*="span"],.row-fluid .controls-row [class*="span"]{float:left}.controls-row .checkbox[class*="span"],.controls-row .radio[class*="span"]{padding-top:5px}input[disabled],select[disabled],textarea[disabled],input[readonly],select[readonly],textarea[readonly]{cursor:not-allowed;background-color:#eee}input[type="radio"][disabled],input[type="checkbox"][disabled],input[type="radio"][readonly],input[type="checkbox"][readonly]{background-color:transparent}.control-group.warning .control-label,.control-group.warning .help-block,.control-group.warning .help-inline{color:#c09853}.control-group.warning .checkbox,.control-group.warning .radio,.control-group.warning input,.control-group.warning select,.control-group.warning textarea{color:#c09853}.control-group.warning input,.control-group.warning select,.control-group.warning textarea{border-color:#c09853;-webkit-box-shadow:inset 0 1px 1px rgba(0,0,0,.075);-moz-box-shadow:inset 0 1px 1px rgba(0,0,0,.075);box-shadow:inset 0 1px 1px rgba(0,0,0,.075)}.control-group.warning input:focus,.control-group.warning select:focus,.control-group.warning textarea:focus{border-color:#a47e3c;-webkit-box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #dbc59e;-moz-box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #dbc59e;box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #dbc59e}.control-group.warning .input-prepend .add-on,.control-group.warning .input-append .add-on{color:#c09853;background-color:#fcf8e3;border-color:#c09853}.control-group.error .control-label,.control-group.error .help-block,.control-group.error .help-inline{color:#b94a48}.control-group.error .checkbox,.control-group.error .radio,.control-group.error input,.control-group.error select,.control-group.error textarea{color:#b94a48}.control-group.error input,.control-group.error select,.control-group.error textarea{border-color:#b94a48;-webkit-box-shadow:inset 0 1px 1px rgba(0,0,0,.075);-moz-box-shadow:inset 0 1px 1px rgba(0,0,0,.075);box-shadow:inset 0 1px 1px rgba(0,0,0,.075)}.control-group.error input:focus,.control-group.error select:focus,.control-group.error textarea:focus{border-color:#953b39;-webkit-box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #d59392;-moz-box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #d59392;box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #d59392}.control-group.error .input-prepend .add-on,.control-group.error .input-append .add-on{color:#b94a48;background-color:#f2dede;border-color:#b94a48}.control-group.success .control-label,.control-group.success .help-block,.control-group.success .help-inline{color:#417e42}.control-group.success .checkbox,.control-group.success .radio,.control-group.success input,.control-group.success select,.control-group.success textarea{color:#417e42}.control-group.success input,.control-group.success select,.control-group.success textarea{border-color:#417e42;-webkit-box-shadow:inset 0 1px 1px rgba(0,0,0,.075);-moz-box-shadow:inset 0 1px 1px rgba(0,0,0,.075);box-shadow:inset 0 1px 1px rgba(0,0,0,.075)}.control-group.success input:focus,.control-group.success select:focus,.control-group.success textarea:focus{border-color:#2f5c30;-webkit-box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #70b571;-moz-box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #70b571;box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #70b571}.control-group.success .input-prepend .add-on,.control-group.success .input-append .add-on{color:#417e42;background-color:#dff0d8;border-color:#417e42}.control-group.info .control-label,.control-group.info .help-block,.control-group.info .help-inline{color:#2d6987}.control-group.info .checkbox,.control-group.info .radio,.control-group.info input,.control-group.info select,.control-group.info textarea{color:#2d6987}.control-group.info input,.control-group.info select,.control-group.info textarea{border-color:#2d6987;-webkit-box-shadow:inset 0 1px 1px rgba(0,0,0,.075);-moz-box-shadow:inset 0 1px 1px rgba(0,0,0,.075);box-shadow:inset 0 1px 1px rgba(0,0,0,.075)}.control-group.info input:focus,.control-group.info select:focus,.control-group.info textarea:focus{border-color:#204b61;-webkit-box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #54a0c6;-moz-box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #54a0c6;box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #54a0c6}.control-group.info .input-prepend .add-on,.control-group.info .input-append .add-on{color:#2d6987;background-color:#eef7fb;border-color:#2d6987}input:focus:invalid,textarea:focus:invalid,select:focus:invalid{color:#b94a48;border-color:#ee5f5b}input:focus:invalid:focus,textarea:focus:invalid:focus,select:focus:invalid:focus{border-color:#e9322d;-webkit-box-shadow:0 0 6px #f8b9b7;-moz-box-shadow:0 0 6px #f8b9b7;box-shadow:0 0 6px #f8b9b7}.form-actions{padding:19px 20px 20px;margin-top:20px;margin-bottom:20px;background-color:#f5f5f5;border-top:1px solid #e5e5e5;*zoom:1}.form-actions:before,.form-actions:after{display:table;content:"";line-height:0}.form-actions:after{clear:both}.form-actions-left-align{padding:19px 10px 20px;margin-top:20px;margin-bottom:20px;background-color:#f5f5f5;border-top:1px solid #e5e5e5}.help-block,.help-inline{color:#595959}.help-block{display:block;margin-bottom:10px}.help-inline{display:inline-block;*display:inline;*zoom:1;vertical-align:middle;padding-left:5px}.input-append,.input-prepend{display:inline-block;margin-bottom:10px;vertical-align:middle;font-size:0;white-space:nowrap}.input-append input,.input-prepend input,.input-append select,.input-prepend select,.input-append .uneditable-input,.input-prepend .uneditable-input,.input-append .dropdown-menu,.input-prepend .dropdown-menu,.input-append .popover,.input-prepend .popover{font-size:14px}.input-append input,.input-prepend input,.input-append select,.input-prepend select,.input-append .uneditable-input,.input-prepend .uneditable-input{position:relative;margin-bottom:0;*margin-left:0;vertical-align:top;-webkit-border-radius:0 4px 4px 0;-moz-border-radius:0 4px 4px 0;border-radius:0 4px 4px 0}.input-append input:focus,.input-prepend input:focus,.input-append select:focus,.input-prepend select:focus,.input-append .uneditable-input:focus,.input-prepend .uneditable-input:focus{z-index:2}.input-append .add-on,.input-prepend .add-on{display:inline-block;width:auto;height:20px;min-width:16px;padding:4px 5px;font-size:14px;font-weight:normal;line-height:20px;text-align:center;text-shadow:0 1px 0 white;background-color:#eee;border:1px solid #ccc}.input-append .add-on,.input-prepend .add-on,.input-append .btn,.input-prepend .btn,.input-append .btn-group>.dropdown-toggle,.input-prepend .btn-group>.dropdown-toggle{vertical-align:top;-webkit-border-radius:0;-moz-border-radius:0;border-radius:0}.input-append .active,.input-prepend .active{background-color:#a9dba9;border-color:#46a546}.input-prepend .add-on,.input-prepend .btn{margin-right:-1px}.input-prepend .add-on:first-child,.input-prepend .btn:first-child{-webkit-border-radius:4px 0 0 4px;-moz-border-radius:4px 0 0 4px;border-radius:4px 0 0 4px}.input-append input,.input-append select,.input-append .uneditable-input{-webkit-border-radius:4px 0 0 4px;-moz-border-radius:4px 0 0 4px;border-radius:4px 0 0 4px}.input-append input+.btn-group .btn:last-child,.input-append select+.btn-group .btn:last-child,.input-append .uneditable-input+.btn-group .btn:last-child{-webkit-border-radius:0 4px 4px 0;-moz-border-radius:0 4px 4px 0;border-radius:0 4px 4px 0}.input-append .add-on,.input-append .btn,.input-append .btn-group{margin-left:-1px}.input-append .add-on:last-child,.input-append .btn:last-child,.input-append .btn-group:last-child>.dropdown-toggle{-webkit-border-radius:0 4px 4px 0;-moz-border-radius:0 4px 4px 0;border-radius:0 4px 4px 0}.input-prepend.input-append input,.input-prepend.input-append select,.input-prepend.input-append .uneditable-input{-webkit-border-radius:0;-moz-border-radius:0;border-radius:0}.input-prepend.input-append input+.btn-group .btn,.input-prepend.input-append select+.btn-group .btn,.input-prepend.input-append .uneditable-input+.btn-group .btn{-webkit-border-radius:0 4px 4px 0;-moz-border-radius:0 4px 4px 0;border-radius:0 4px 4px 0}.input-prepend.input-append .add-on:first-child,.input-prepend.input-append .btn:first-child{margin-right:-1px;-webkit-border-radius:4px 0 0 4px;-moz-border-radius:4px 0 0 4px;border-radius:4px 0 0 4px}.input-prepend.input-append .add-on:last-child,.input-prepend.input-append .btn:last-child{margin-left:-1px;-webkit-border-radius:0 4px 4px 0;-moz-border-radius:0 4px 4px 0;border-radius:0 4px 4px 0}.input-prepend.input-append .btn-group:first-child{margin-left:0}input.search-query{padding-right:14px;padding-right:4px \9;padding-left:14px;padding-left:4px \9;margin-bottom:0;-webkit-border-radius:15px;-moz-border-radius:15px;border-radius:15px}.form-search .input-append .search-query,.form-search .input-prepend .search-query{-webkit-border-radius:0;-moz-border-radius:0;border-radius:0}.form-search .input-append .search-query{-webkit-border-radius:14px 0 0 14px;-moz-border-radius:14px 0 0 14px;border-radius:14px 0 0 14px}.form-search .input-append .btn{-webkit-border-radius:0 14px 14px 0;-moz-border-radius:0 14px 14px 0;border-radius:0 14px 14px 0}.form-search .input-prepend .search-query{-webkit-border-radius:0 14px 14px 0;-moz-border-radius:0 14px 14px 0;border-radius:0 14px 14px 0}.form-search .input-prepend .btn{-webkit-border-radius:14px 0 0 14px;-moz-border-radius:14px 0 0 14px;border-radius:14px 0 0 14px}.form-search input,.form-inline input,.form-horizontal input,.form-search textarea,.form-inline textarea,.form-horizontal textarea,.form-search select,.form-inline select,.form-horizontal select,.form-search .help-inline,.form-inline .help-inline,.form-horizontal .help-inline,.form-search .uneditable-input,.form-inline .uneditable-input,.form-horizontal .uneditable-input,.form-search .input-prepend,.form-inline .input-prepend,.form-horizontal .input-prepend,.form-search .input-append,.form-inline .input-append,.form-horizontal .input-append{display:inline-block;*display:inline;*zoom:1;margin-bottom:0;vertical-align:middle}.form-search .hide,.form-inline .hide,.form-horizontal .hide{display:none}.form-search label,.form-inline label,.form-search .btn-group,.form-inline .btn-group{display:inline-block}.form-search .input-append,.form-inline .input-append,.form-search .input-prepend,.form-inline .input-prepend{margin-bottom:0}.form-search .radio,.form-search .checkbox,.form-inline .radio,.form-inline .checkbox{padding-left:0;margin-bottom:0;vertical-align:middle}.form-search .radio input[type="radio"],.form-search .checkbox input[type="checkbox"],.form-inline .radio input[type="radio"],.form-inline .checkbox input[type="checkbox"]{float:left;margin-right:3px;margin-left:0}.control-group{margin-bottom:10px}legend+.control-group{margin-top:20px;-webkit-margin-top-collapse:separate}.form-horizontal .control-group{margin-bottom:20px;*zoom:1}.form-horizontal .control-group:before,.form-horizontal .control-group:after{display:table;content:"";line-height:0}.form-horizontal .control-group:after{clear:both}.form-horizontal .control-label{float:left;width:160px;padding-top:5px;text-align:right}.form-horizontal .controls{*display:inline-block;*padding-left:20px;margin-left:180px;*margin-left:0}.form-horizontal .controls:first-child{*padding-left:180px}.form-horizontal .help-block{margin-bottom:0}.form-horizontal input+.help-block,.form-horizontal select+.help-block,.form-horizontal textarea+.help-block,.form-horizontal .uneditable-input+.help-block,.form-horizontal .input-prepend+.help-block,.form-horizontal .input-append+.help-block{margin-top:10px}.form-horizontal .form-actions{padding-left:180px}.form-horizontal .post-message{width:300px}.form-horizontal .post-message-submission-count{margin-top:6px}textarea.repro-textarea{width:400px}ul.repro-questions{list-style-type:circle}ul.repro-questions>li{margin:10px 0}.tiny-input{width:60px}table{max-width:100%;background-color:transparent;border-collapse:collapse;border-spacing:0}.table{width:100%;margin-bottom:20px}.table th,.table td{padding:8px;line-height:20px;text-align:left;vertical-align:top;border-top:1px solid #ddd}.table th{font-weight:bold}.table thead th{vertical-align:bottom}.table caption+thead tr:first-child th,.table caption+thead tr:first-child td,.table colgroup+thead tr:first-child th,.table colgroup+thead tr:first-child td,.table thead:first-child tr:first-child th,.table thead:first-child tr:first-child td{border-top:0}.table tbody+tbody{border-top:2px solid #ddd}.table .table{background-color:#fff}.table-condensed th,.table-condensed td{padding:4px 5px}.table-bordered{border:1px solid #ddd;border-collapse:separate;*border-collapse:collapse;border-left:0;-webkit-border-radius:4px;-moz-border-radius:4px;border-radius:4px}.table-bordered th,.table-bordered td{border-left:1px solid #ddd}.table-bordered caption+thead tr:first-child th,.table-bordered caption+tbody tr:first-child th,.table-bordered caption+tbody tr:first-child td,.table-bordered colgroup+thead tr:first-child th,.table-bordered colgroup+tbody tr:first-child th,.table-bordered colgroup+tbody tr:first-child td,.table-bordered thead:first-child tr:first-child th,.table-bordered tbody:first-child tr:first-child th,.table-bordered tbody:first-child tr:first-child td{border-top:0}.table-bordered thead:first-child tr:first-child>th:first-child,.table-bordered tbody:first-child tr:first-child>td:first-child,.table-bordered tbody:first-child tr:first-child>th:first-child{-webkit-border-top-left-radius:4px;-moz-border-radius-topleft:4px;border-top-left-radius:4px}.table-bordered thead:first-child tr:first-child>th:last-child,.table-bordered tbody:first-child tr:first-child>td:last-child,.table-bordered tbody:first-child tr:first-child>th:last-child{-webkit-border-top-right-radius:4px;-moz-border-radius-topright:4px;border-top-right-radius:4px}.table-bordered thead:last-child tr:last-child>th:first-child,.table-bordered tbody:last-child tr:last-child>td:first-child,.table-bordered tbody:last-child tr:last-child>th:first-child,.table-bordered tfoot:last-child tr:last-child>td:first-child,.table-bordered tfoot:last-child tr:last-child>th:first-child{-webkit-border-bottom-left-radius:4px;-moz-border-radius-bottomleft:4px;border-bottom-left-radius:4px}.table-bordered thead:last-child tr:last-child>th:last-child,.table-bordered tbody:last-child tr:last-child>td:last-child,.table-bordered tbody:last-child tr:last-child>th:last-child,.table-bordered tfoot:last-child tr:last-child>td:last-child,.table-bordered tfoot:last-child tr:last-child>th:last-child{-webkit-border-bottom-right-radius:4px;-moz-border-radius-bottomright:4px;border-bottom-right-radius:4px}.table-bordered tfoot+tbody:last-child tr:last-child td:first-child{-webkit-border-bottom-left-radius:0;-moz-border-radius-bottomleft:0;border-bottom-left-radius:0}.table-bordered tfoot+tbody:last-child tr:last-child td:last-child{-webkit-border-bottom-right-radius:0;-moz-border-radius-bottomright:0;border-bottom-right-radius:0}.table-bordered caption+thead tr:first-child th:first-child,.table-bordered caption+tbody tr:first-child td:first-child,.table-bordered colgroup+thead tr:first-child th:first-child,.table-bordered colgroup+tbody tr:first-child td:first-child{-webkit-border-top-left-radius:4px;-moz-border-radius-topleft:4px;border-top-left-radius:4px}.table-bordered caption+thead tr:first-child th:last-child,.table-bordered caption+tbody tr:first-child td:last-child,.table-bordered colgroup+thead tr:first-child th:last-child,.table-bordered colgroup+tbody tr:first-child td:last-child{-webkit-border-top-right-radius:4px;-moz-border-radius-topright:4px;border-top-right-radius:4px}.table-striped tbody>tr:nth-child(odd)>td,.table-striped tbody>tr:nth-child(odd)>th{background-color:#f9f9f9}.table-hover tbody tr:hover>td,.table-hover tbody tr:hover>th{background-color:#f5f5f5}table td[class*="span"],table th[class*="span"],.row-fluid table td[class*="span"],.row-fluid table th[class*="span"]{display:table-cell;float:none;margin-left:0}.table td.span1,.table th.span1{float:none;width:44px;margin-left:0}.table td.span2,.table th.span2{float:none;width:124px;margin-left:0}.table td.span3,.table th.span3{float:none;width:204px;margin-left:0}.table td.span4,.table th.span4{float:none;width:284px;margin-left:0}.table td.span5,.table th.span5{float:none;width:364px;margin-left:0}.table td.span6,.table th.span6{float:none;width:444px;margin-left:0}.table td.span7,.table th.span7{float:none;width:524px;margin-left:0}.table td.span8,.table th.span8{float:none;width:604px;margin-left:0}.table td.span9,.table th.span9{float:none;width:684px;margin-left:0}.table td.span10,.table th.span10{float:none;width:764px;margin-left:0}.table td.span11,.table th.span11{float:none;width:844px;margin-left:0}.table td.span12,.table th.span12{float:none;width:924px;margin-left:0}.table tbody tr.success>td{background-color:#dff0d8}.table tbody tr.error>td{background-color:#f2dede}.table tbody tr.warning>td{background-color:#fcf8e3}.table tbody tr.info>td{background-color:#eef7fb}.table-hover tbody tr.success:hover>td{background-color:#d0e9c6}.table-hover tbody tr.error:hover>td{background-color:#ebcccc}.table-hover tbody tr.warning:hover>td{background-color:#faf2cc}.table-hover tbody tr.info:hover>td{background-color:#d9edf7}[class^="icon-"],[class*=" icon-"]{display:inline-block;width:14px;height:14px;*margin-right:.3em;line-height:14px;vertical-align:text-top;background-image:url("../images/glyphicons-halflings.png");background-position:14px 14px;background-repeat:no-repeat;margin-top:1px}.icon-white,.nav-pills>.active>a>[class^="icon-"],.nav-pills>.active>a>[class*=" icon-"],.nav-list>.active>a>[class^="icon-"],.nav-list>.active>a>[class*=" icon-"],.navbar-inverse .nav>.active>a>[class^="icon-"],.navbar-inverse .nav>.active>a>[class*=" icon-"],.dropdown-menu>li>a:hover>[class^="icon-"],.dropdown-menu>li>a:focus>[class^="icon-"],.dropdown-menu>li>a:hover>[class*=" icon-"],.dropdown-menu>li>a:focus>[class*=" icon-"],.dropdown-menu>.active>a>[class^="icon-"],.dropdown-menu>.active>a>[class*=" icon-"],.dropdown-submenu:hover>a>[class^="icon-"],.dropdown-submenu:focus>a>[class^="icon-"],.dropdown-submenu:hover>a>[class*=" icon-"],.dropdown-submenu:focus>a>[class*=" icon-"]{background-image:url("../images/glyphicons-halflings-white.png")}.icon-glass{background-position:0 0}.icon-music{background-position:-24px 0}.icon-search{background-position:-48px 0}.icon-envelope{background-position:-72px 0}.icon-heart{background-position:-96px 0}.icon-star{background-position:-120px 0}.icon-star-empty{background-position:-144px 0}.icon-user{background-position:-168px 0}.icon-film{background-position:-192px 0}.icon-th-large{background-position:-216px 0}.icon-th{background-position:-240px 0}.icon-th-list{background-position:-264px 0}.icon-ok{background-position:-288px 0}.icon-remove{background-position:-312px 0}.icon-zoom-in{background-position:-336px 0}.icon-zoom-out{background-position:-360px 0}.icon-off{background-position:-384px 0}.icon-signal{background-position:-408px 0}.icon-cog{background-position:-432px 0}.icon-trash{background-position:-456px 0}.icon-home{background-position:0 -24px}.icon-file{background-position:-24px -24px}.icon-time{background-position:-48px -24px}.icon-road{background-position:-72px -24px}.icon-download-alt{background-position:-96px -24px}.icon-download{background-position:-120px -24px}.icon-upload{background-position:-144px -24px}.icon-inbox{background-position:-168px -24px}.icon-play-circle{background-position:-192px -24px}.icon-repeat{background-position:-216px -24px}.icon-refresh{background-position:-240px -24px}.icon-list-alt{background-position:-264px -24px}.icon-lock{background-position:-287px -24px}.icon-flag{background-position:-312px -24px}.icon-headphones{background-position:-336px -24px}.icon-volume-off{background-position:-360px -24px}.icon-volume-down{background-position:-384px -24px}.icon-volume-up{background-position:-408px -24px}.icon-qrcode{background-position:-432px -24px}.icon-barcode{background-position:-456px -24px}.icon-tag{background-position:0 -48px}.icon-tags{background-position:-25px -48px}.icon-book{background-position:-48px -48px}.icon-bookmark{background-position:-72px -48px}.icon-print{background-position:-96px -48px}.icon-camera{background-position:-120px -48px}.icon-font{background-position:-144px -48px}.icon-bold{background-position:-167px -48px}.icon-italic{background-position:-192px -48px}.icon-text-height{background-position:-216px -48px}.icon-text-width{background-position:-240px -48px}.icon-align-left{background-position:-264px -48px}.icon-align-center{background-position:-288px -48px}.icon-align-right{background-position:-312px -48px}.icon-align-justify{background-position:-336px -48px}.icon-list{background-position:-360px -48px}.icon-indent-left{background-position:-384px -48px}.icon-indent-right{background-position:-408px -48px}.icon-facetime-video{background-position:-432px -48px}.icon-picture{background-position:-456px -48px}.icon-pencil{background-position:0 -72px}.icon-map-marker{background-position:-24px -72px}.icon-adjust{background-position:-48px -72px}.icon-tint{background-position:-72px -72px}.icon-edit{background-position:-96px -72px}.icon-share{background-position:-120px -72px}.icon-check{background-position:-144px -72px}.icon-move{background-position:-168px -72px}.icon-step-backward{background-position:-192px -72px}.icon-fast-backward{background-position:-216px -72px}.icon-backward{background-position:-240px -72px}.icon-play{background-position:-264px -72px}.icon-pause{background-position:-288px -72px}.icon-stop{background-position:-312px -72px}.icon-forward{background-position:-336px -72px}.icon-fast-forward{background-position:-360px -72px}.icon-step-forward{background-position:-384px -72px}.icon-eject{background-position:-408px -72px}.icon-chevron-left{background-position:-432px -72px}.icon-chevron-right{background-position:-456px -72px}.icon-plus-sign{background-position:0 -96px}.icon-minus-sign{background-position:-24px -96px}.icon-remove-sign{background-position:-48px -96px}.icon-ok-sign{background-position:-72px -96px}.icon-question-sign{background-position:-96px -96px}.icon-info-sign{background-position:-120px -96px}.icon-screenshot{background-position:-144px -96px}.icon-remove-circle{background-position:-168px -96px}.icon-ok-circle{background-position:-192px -96px}.icon-ban-circle{background-position:-216px -96px}.icon-arrow-left{background-position:-240px -96px}.icon-arrow-right{background-position:-264px -96px}.icon-arrow-up{background-position:-289px -96px}.icon-arrow-down{background-position:-312px -96px}.icon-share-alt{background-position:-336px -96px}.icon-resize-full{background-position:-360px -96px}.icon-resize-small{background-position:-384px -96px}.icon-plus{background-position:-408px -96px}.icon-minus{background-position:-433px -96px}.icon-asterisk{background-position:-456px -96px}.icon-exclamation-sign{background-position:0 -120px}.icon-gift{background-position:-24px -120px}.icon-leaf{background-position:-48px -120px}.icon-fire{background-position:-72px -120px}.icon-eye-open{background-position:-96px -120px}.icon-eye-close{background-position:-120px -120px}.icon-warning-sign{background-position:-144px -120px}.icon-plane{background-position:-168px -120px}.icon-calendar{background-position:-192px -120px}.icon-random{background-position:-216px -120px;width:16px}.icon-comment{background-position:-240px -120px}.icon-magnet{background-position:-264px -120px}.icon-chevron-up{background-position:-288px -120px}.icon-chevron-down{background-position:-313px -119px}.icon-retweet{background-position:-336px -120px}.icon-shopping-cart{background-position:-360px -120px}.icon-folder-close{background-position:-384px -120px;width:16px}.icon-folder-open{background-position:-408px -120px;width:16px}.icon-resize-vertical{background-position:-432px -119px}.icon-resize-horizontal{background-position:-456px -118px}.icon-hdd{background-position:0 -144px}.icon-bullhorn{background-position:-24px -144px}.icon-bell{background-position:-48px -144px}.icon-certificate{background-position:-72px -144px}.icon-thumbs-up{background-position:-96px -144px}.icon-thumbs-down{background-position:-120px -144px}.icon-hand-right{background-position:-144px -144px}.icon-hand-left{background-position:-168px -144px}.icon-hand-up{background-position:-192px -144px}.icon-hand-down{background-position:-216px -144px}.icon-circle-arrow-right{background-position:-240px -144px}.icon-circle-arrow-left{background-position:-264px -144px}.icon-circle-arrow-up{background-position:-288px -144px}.icon-circle-arrow-down{background-position:-312px -144px}.icon-globe{background-position:-336px -144px}.icon-wrench{background-position:-360px -144px}.icon-tasks{background-position:-384px -144px}.icon-filter{background-position:-408px -144px}.icon-briefcase{background-position:-432px -144px}.icon-fullscreen{background-position:-456px -144px}.dropup,.dropdown{position:relative}.dropdown-toggle{*margin-bottom:-3px}.dropdown-toggle:active,.open .dropdown-toggle{outline:0}.caret{display:inline-block;width:0;height:0;vertical-align:top;border-top:4px solid #000;border-right:4px solid transparent;border-left:4px solid transparent;content:""}.dropdown .caret{margin-top:8px;margin-left:2px}.dropdown-menu{position:absolute;top:100%;left:0;z-index:1000;display:none;float:left;min-width:160px;padding:5px 0;margin:2px 0 0;list-style:none;background-color:#fff;border:1px solid #ccc;border:1px solid rgba(0,0,0,.2);*border-right-width:2px;*border-bottom-width:2px;-webkit-border-radius:6px;-moz-border-radius:6px;border-radius:6px;-webkit-box-shadow:0 5px 10px rgba(0,0,0,.2);-moz-box-shadow:0 5px 10px rgba(0,0,0,.2);box-shadow:0 5px 10px rgba(0,0,0,.2);-webkit-background-clip:padding-box;-moz-background-clip:padding;background-clip:padding-box}.dropdown-menu.pull-right{right:0;left:auto}.dropdown-menu .divider{*width:100%;height:1px;margin:9px 1px;*margin:-5px 0 5px;overflow:hidden;background-color:#e5e5e5;border-bottom:1px solid #fff}.dropdown-menu>li>a{display:block;padding:3px 20px;clear:both;font-weight:normal;line-height:20px;color:#333;white-space:nowrap}.dropdown-menu>li>a:hover,.dropdown-menu>li>a:focus,.dropdown-submenu:hover>a,.dropdown-submenu:focus>a{text-decoration:none;color:#fff;background-color:#007699;background-image:-moz-linear-gradient(top,#007ea3,#006a8a);background-image:-webkit-gradient(linear,0 0,0 100%,from(#007ea3),to(#006a8a));background-image:-webkit-linear-gradient(top,#007ea3,#006a8a);background-image:-o-linear-gradient(top,#007ea3,#006a8a);background-image:linear-gradient(to bottom,#007ea3,#006a8a);background-repeat:repeat-x;filter:progid:DXImageTransform.Microsoft.gradient(startColorstr='#ff007ea3',endColorstr='#ff006a8a',GradientType=0)}.dropdown-menu>.active>a,.dropdown-menu>.active>a:hover,.dropdown-menu>.active>a:focus{color:#fff;text-decoration:none;outline:0;background-color:#007699;background-image:-moz-linear-gradient(top,#007ea3,#006a8a);background-image:-webkit-gradient(linear,0 0,0 100%,from(#007ea3),to(#006a8a));background-image:-webkit-linear-gradient(top,#007ea3,#006a8a);background-image:-o-linear-gradient(top,#007ea3,#006a8a);background-image:linear-gradient(to bottom,#007ea3,#006a8a);background-repeat:repeat-x;filter:progid:DXImageTransform.Microsoft.gradient(startColorstr='#ff007ea3',endColorstr='#ff006a8a',GradientType=0)}.dropdown-menu>.disabled>a,.dropdown-menu>.disabled>a:hover,.dropdown-menu>.disabled>a:focus{color:#6c757d}.dropdown-menu>.disabled>a:hover,.dropdown-menu>.disabled>a:focus{text-decoration:none;background-color:transparent;background-image:none;filter:progid:DXImageTransform.Microsoft.gradient(enabled=false);cursor:default}.open{*z-index:1000}.open>.dropdown-menu{display:block}.dropdown-backdrop{position:fixed;left:0;right:0;bottom:0;top:0;z-index:990}.pull-right>.dropdown-menu{right:0;left:auto}.dropup .caret,.navbar-fixed-bottom .dropdown .caret{border-top:0;border-bottom:4px solid #000;content:""}.dropup .dropdown-menu,.navbar-fixed-bottom .dropdown .dropdown-menu{top:auto;bottom:100%;margin-bottom:1px}.dropdown-submenu{position:relative}.dropdown-submenu>.dropdown-menu{top:0;left:100%;margin-top:-6px;margin-left:-1px;-webkit-border-radius:0 6px 6px 6px;-moz-border-radius:0 6px 6px 6px;border-radius:0 6px 6px 6px}.dropdown-submenu:hover>.dropdown-menu{display:block}.dropup .dropdown-submenu>.dropdown-menu{top:auto;bottom:0;margin-top:0;margin-bottom:-2px;-webkit-border-radius:5px 5px 5px 0;-moz-border-radius:5px 5px 5px 0;border-radius:5px 5px 5px 0}.dropdown-submenu>a:after{display:block;content:" ";float:right;width:0;height:0;border-color:transparent;border-style:solid;border-width:5px 0 5px 5px;border-left-color:#ccc;margin-top:5px;margin-right:-10px}.dropdown-submenu:hover>a:after{border-left-color:#fff}.dropdown-submenu.pull-left{float:none}.dropdown-submenu.pull-left>.dropdown-menu{right:100%;left:auto;margin-right:-10px;-webkit-border-radius:6px 0 6px 6px;-moz-border-radius:6px 0 6px 6px;border-radius:6px 0 6px 6px}.dropdown .dropdown-menu .nav-header{padding-left:20px;padding-right:20px}.typeahead{z-index:1051;margin-top:2px;-webkit-border-radius:4px;-moz-border-radius:4px;border-radius:4px}.well{min-height:20px;padding:19px;margin-bottom:20px;background-color:#f5f5f5;border:1px solid #e3e3e3;-webkit-border-radius:4px;-moz-border-radius:4px;border-radius:4px;-webkit-box-shadow:inset 0 1px 1px rgba(0,0,0,.05);-moz-box-shadow:inset 0 1px 1px rgba(0,0,0,.05);box-shadow:inset 0 1px 1px rgba(0,0,0,.05)}.well blockquote{border-color:#ddd;border-color:rgba(0,0,0,.15)}.well-large{padding:24px;-webkit-border-radius:6px;-moz-border-radius:6px;border-radius:6px}.well-small{padding:9px;-webkit-border-radius:3px;-moz-border-radius:3px;border-radius:3px}.fade{opacity:0;-webkit-transition:opacity .15s linear;-moz-transition:opacity .15s linear;-o-transition:opacity .15s linear;transition:opacity .15s linear}.fade.in{opacity:1}.collapse{position:relative;height:0;overflow:hidden;-webkit-transition:height .35s ease;-moz-transition:height .35s ease;-o-transition:height .35s ease;transition:height .35s ease}.collapse.in{height:auto}.close{float:right;font-size:20px;font-weight:bold;line-height:20px;color:#000;text-shadow:0 1px 0 white;opacity:.2;filter:alpha(opacity=20)}.close:hover,.close:focus{color:#000;text-decoration:none;cursor:pointer;opacity:.4;filter:alpha(opacity=40)}button.close{padding:0;cursor:pointer;background:transparent;border:0;-webkit-appearance:none}.btn{display:inline-block;*display:inline;*zoom:1;padding:4px 12px;margin-bottom:0;font-size:14px;line-height:20px;text-align:center;vertical-align:middle;cursor:pointer;color:#333;text-shadow:0 1px 1px rgba(255,255,255,.75);background-color:#f5f5f5;background-image:-moz-linear-gradient(top,white,#e6e6e6);background-image:-webkit-gradient(linear,0 0,0 100%,from(white),to(#e6e6e6));background-image:-webkit-linear-gradient(top,white,#e6e6e6);background-image:-o-linear-gradient(top,white,#e6e6e6);background-image:linear-gradient(to bottom,white,#e6e6e6);background-repeat:repeat-x;filter:progid:DXImageTransform.Microsoft.gradient(startColorstr='#ffffffff',endColorstr='#ffe6e6e6',GradientType=0);border-color:#e6e6e6 #e6e6e6 silver;border-color:rgba(0,0,0,.1) rgba(0,0,0,.1) rgba(0,0,0,.25);*background-color:#e6e6e6;filter:progid:DXImageTransform.Microsoft.gradient(enabled=false);border:1px solid #ccc;*border:0;border-bottom-color:#b3b3b3;-webkit-border-radius:4px;-moz-border-radius:4px;border-radius:4px;*margin-left:.3em;-webkit-box-shadow:inset 0 1px 0 rgba(255,255,255,.2),0 1px 2px rgba(0,0,0,.05);-moz-box-shadow:inset 0 1px 0 rgba(255,255,255,.2),0 1px 2px rgba(0,0,0,.05);box-shadow:inset 0 1px 0 rgba(255,255,255,.2),0 1px 2px rgba(0,0,0,.05)}.btn:hover,.btn:focus,.btn:active,.btn.active,.btn.disabled,.btn[disabled]{color:#333;background-color:#e6e6e6;*background-color:#d9d9d9}.btn:active,.btn.active{background-color:#ccc \9}.btn:first-child{*margin-left:0}.btn:hover,.btn:focus{color:#333;text-decoration:none;background-position:0 -15px;-webkit-transition:background-position .1s linear;-moz-transition:background-position .1s linear;-o-transition:background-position .1s linear;transition:background-position .1s linear}.btn:focus{outline:thin dotted #333;outline:5px auto -webkit-focus-ring-color;outline-offset:-2px}.btn.active,.btn:active{background-image:none;outline:0;-webkit-box-shadow:inset 0 2px 4px rgba(0,0,0,.15),0 1px 2px rgba(0,0,0,.05);-moz-box-shadow:inset 0 2px 4px rgba(0,0,0,.15),0 1px 2px rgba(0,0,0,.05);box-shadow:inset 0 2px 4px rgba(0,0,0,.15),0 1px 2px rgba(0,0,0,.05)}.btn.disabled,.btn[disabled]{cursor:default;background-image:none;opacity:.65;filter:alpha(opacity=65);-webkit-box-shadow:none;-moz-box-shadow:none;box-shadow:none}.btn-large{padding:11px 19px;font-size:17.5px;-webkit-border-radius:6px;-moz-border-radius:6px;border-radius:6px}.btn-large [class^="icon-"],.btn-large [class*=" icon-"]{margin-top:4px}.btn-small{padding:2px 10px;font-size:11.9px;-webkit-border-radius:3px;-moz-border-radius:3px;border-radius:3px}.btn-small [class^="icon-"],.btn-small [class*=" icon-"]{margin-top:0}.btn-mini [class^="icon-"],.btn-mini [class*=" icon-"]{margin-top:-1px}.btn-mini{padding:0 6px;font-size:10.5px;-webkit-border-radius:3px;-moz-border-radius:3px;border-radius:3px}.btn-block{display:block;width:100%;padding-left:0;padding-right:0;-webkit-box-sizing:border-box;-moz-box-sizing:border-box;box-sizing:border-box}.btn-block+.btn-block{margin-top:5px}input[type="submit"].btn-block,input[type="reset"].btn-block,input[type="button"].btn-block{width:100%}.btn-primary.active,.btn-warning.active,.btn-danger.active,.btn-success.active,.btn-info.active,.btn-inverse.active{color:rgba(255,255,255,.75)}.btn-primary{color:#fff;text-shadow:0 -1px 0 rgba(0,0,0,.25);background-color:#0068a3;background-image:-moz-linear-gradient(top,#007ea3,#0048a3);background-image:-webkit-gradient(linear,0 0,0 100%,from(#007ea3),to(#0048a3));background-image:-webkit-linear-gradient(top,#007ea3,#0048a3);background-image:-o-linear-gradient(top,#007ea3,#0048a3);background-image:linear-gradient(to bottom,#007ea3,#0048a3);background-repeat:repeat-x;filter:progid:DXImageTransform.Microsoft.gradient(startColorstr='#ff007ea3',endColorstr='#ff0048a3',GradientType=0);border-color:#0048a3 #0048a3 #002656;border-color:rgba(0,0,0,.1) rgba(0,0,0,.1) rgba(0,0,0,.25);*background-color:#0048a3;filter:progid:DXImageTransform.Microsoft.gradient(enabled=false)}.btn-primary:hover,.btn-primary:focus,.btn-primary:active,.btn-primary.active,.btn-primary.disabled,.btn-primary[disabled]{color:#fff;background-color:#0048a3;*background-color:#003c8a}.btn-primary:active,.btn-primary.active{background-color:#003170 \9}.btn-warning{color:#fff;text-shadow:0 -1px 0 rgba(0,0,0,.25);background-color:#faa732;background-image:-moz-linear-gradient(top,#fbb450,#f89406);background-image:-webkit-gradient(linear,0 0,0 100%,from(#fbb450),to(#f89406));background-image:-webkit-linear-gradient(top,#fbb450,#f89406);background-image:-o-linear-gradient(top,#fbb450,#f89406);background-image:linear-gradient(to bottom,#fbb450,#f89406);background-repeat:repeat-x;filter:progid:DXImageTransform.Microsoft.gradient(startColorstr='#fffbb450',endColorstr='#fff89406',GradientType=0);border-color:#f89406 #f89406 #ad6704;border-color:rgba(0,0,0,.1) rgba(0,0,0,.1) rgba(0,0,0,.25);*background-color:#f89406;filter:progid:DXImageTransform.Microsoft.gradient(enabled=false)}.btn-warning:hover,.btn-warning:focus,.btn-warning:active,.btn-warning.active,.btn-warning.disabled,.btn-warning[disabled]{color:#fff;background-color:#f89406;*background-color:#df8505}.btn-warning:active,.btn-warning.active{background-color:#c67605 \9}.btn-danger{color:#fff;text-shadow:0 -1px 0 rgba(0,0,0,.25);background-color:#da4f49;background-image:-moz-linear-gradient(top,#ee5f5b,#bd362f);background-image:-webkit-gradient(linear,0 0,0 100%,from(#ee5f5b),to(#bd362f));background-image:-webkit-linear-gradient(top,#ee5f5b,#bd362f);background-image:-o-linear-gradient(top,#ee5f5b,#bd362f);background-image:linear-gradient(to bottom,#ee5f5b,#bd362f);background-repeat:repeat-x;filter:progid:DXImageTransform.Microsoft.gradient(startColorstr='#ffee5f5b',endColorstr='#ffbd362f',GradientType=0);border-color:#bd362f #bd362f #802420;border-color:rgba(0,0,0,.1) rgba(0,0,0,.1) rgba(0,0,0,.25);*background-color:#bd362f;filter:progid:DXImageTransform.Microsoft.gradient(enabled=false)}.btn-danger:hover,.btn-danger:focus,.btn-danger:active,.btn-danger.active,.btn-danger.disabled,.btn-danger[disabled]{color:#fff;background-color:#bd362f;*background-color:#a9302a}.btn-danger:active,.btn-danger.active{background-color:#942a25 \9}.btn-success{color:#fff;text-shadow:0 -1px 0 rgba(0,0,0,.25);background-color:#368336;background-image:-moz-linear-gradient(top,#389538,#336733);background-image:-webkit-gradient(linear,0 0,0 100%,from(#389538),to(#336733));background-image:-webkit-linear-gradient(top,#389538,#336733);background-image:-o-linear-gradient(top,#389538,#336733);background-image:linear-gradient(to bottom,#389538,#336733);background-repeat:repeat-x;filter:progid:DXImageTransform.Microsoft.gradient(startColorstr='#ff389538',endColorstr='#ff336733',GradientType=0);border-color:#336733 #336733 #1a341a;border-color:rgba(0,0,0,.1) rgba(0,0,0,.1) rgba(0,0,0,.25);*background-color:#336733;filter:progid:DXImageTransform.Microsoft.gradient(enabled=false)}.btn-success:hover,.btn-success:focus,.btn-success:active,.btn-success.active,.btn-success.disabled,.btn-success[disabled]{color:#fff;background-color:#336733;*background-color:#2b562b}.btn-success:active,.btn-success.active{background-color:#224522 \9}.btn-info{color:#fff;text-shadow:0 -1px 0 rgba(0,0,0,.25);background-color:#49afcd;background-image:-moz-linear-gradient(top,#5bc0de,#2f96b4);background-image:-webkit-gradient(linear,0 0,0 100%,from(#5bc0de),to(#2f96b4));background-image:-webkit-linear-gradient(top,#5bc0de,#2f96b4);background-image:-o-linear-gradient(top,#5bc0de,#2f96b4);background-image:linear-gradient(to bottom,#5bc0de,#2f96b4);background-repeat:repeat-x;filter:progid:DXImageTransform.Microsoft.gradient(startColorstr='#ff5bc0de',endColorstr='#ff2f96b4',GradientType=0);border-color:#2f96b4 #2f96b4 #1f6377;border-color:rgba(0,0,0,.1) rgba(0,0,0,.1) rgba(0,0,0,.25);*background-color:#2f96b4;filter:progid:DXImageTransform.Microsoft.gradient(enabled=false)}.btn-info:hover,.btn-info:focus,.btn-info:active,.btn-info.active,.btn-info.disabled,.btn-info[disabled]{color:#fff;background-color:#2f96b4;*background-color:#2a85a0}.btn-info:active,.btn-info.active{background-color:#24748c \9}.btn-inverse{color:#fff;text-shadow:0 -1px 0 rgba(0,0,0,.25);background-color:#363636;background-image:-moz-linear-gradient(top,#444,#222);background-image:-webkit-gradient(linear,0 0,0 100%,from(#444),to(#222));background-image:-webkit-linear-gradient(top,#444,#222);background-image:-o-linear-gradient(top,#444,#222);background-image:linear-gradient(to bottom,#444,#222);background-repeat:repeat-x;filter:progid:DXImageTransform.Microsoft.gradient(startColorstr='#ff444444',endColorstr='#ff222222',GradientType=0);border-color:#222 #222 #000;border-color:rgba(0,0,0,.1) rgba(0,0,0,.1) rgba(0,0,0,.25);*background-color:#222;filter:progid:DXImageTransform.Microsoft.gradient(enabled=false)}.btn-inverse:hover,.btn-inverse:focus,.btn-inverse:active,.btn-inverse.active,.btn-inverse.disabled,.btn-inverse[disabled]{color:#fff;background-color:#222;*background-color:#151515}.btn-inverse:active,.btn-inverse.active{background-color:#080808 \9}button.btn,input[type="submit"].btn{*padding-top:3px;*padding-bottom:3px}button.btn::-moz-focus-inner,input[type="submit"].btn::-moz-focus-inner{padding:0;border:0}button.btn.btn-large,input[type="submit"].btn.btn-large{*padding-top:7px;*padding-bottom:7px}button.btn.btn-small,input[type="submit"].btn.btn-small{*padding-top:3px;*padding-bottom:3px}button.btn.btn-mini,input[type="submit"].btn.btn-mini{*padding-top:1px;*padding-bottom:1px}.btn-link,.btn-link:active,.btn-link[disabled]{background-color:transparent;background-image:none;-webkit-box-shadow:none;-moz-box-shadow:none;box-shadow:none}.btn-link{border-color:transparent;cursor:pointer;color:#007294;-webkit-border-radius:0;-moz-border-radius:0;border-radius:0}.btn-link:hover,.btn-link:focus{color:#007ea3;text-decoration:underline;background-color:transparent}.btn-link[disabled]:hover,.btn-link[disabled]:focus{color:#333;text-decoration:none}.btn-group{position:relative;display:inline-block;*display:inline;*zoom:1;font-size:0;vertical-align:middle;white-space:nowrap;*margin-left:.3em}.btn-group:first-child{*margin-left:0}.btn-group+.btn-group{margin-left:5px}.btn-toolbar{font-size:0;margin-top:10px;margin-bottom:10px}.btn-toolbar>.btn+.btn,.btn-toolbar>.btn-group+.btn,.btn-toolbar>.btn+.btn-group{margin-left:5px}.btn-group>.btn{position:relative;-webkit-border-radius:0;-moz-border-radius:0;border-radius:0}.btn-group>.btn+.btn{margin-left:-1px}.btn-group>.btn,.btn-group>.dropdown-menu,.btn-group>.popover{font-size:14px}.btn-group>.btn-mini{font-size:10.5px}.btn-group>.btn-small{font-size:11.9px}.btn-group>.btn-large{font-size:17.5px}.btn-group>.btn:first-child{margin-left:0;-webkit-border-top-left-radius:4px;-moz-border-radius-topleft:4px;border-top-left-radius:4px;-webkit-border-bottom-left-radius:4px;-moz-border-radius-bottomleft:4px;border-bottom-left-radius:4px}.btn-group>.btn:last-child,.btn-group>.dropdown-toggle{-webkit-border-top-right-radius:4px;-moz-border-radius-topright:4px;border-top-right-radius:4px;-webkit-border-bottom-right-radius:4px;-moz-border-radius-bottomright:4px;border-bottom-right-radius:4px}.btn-group>.btn.large:first-child{margin-left:0;-webkit-border-top-left-radius:6px;-moz-border-radius-topleft:6px;border-top-left-radius:6px;-webkit-border-bottom-left-radius:6px;-moz-border-radius-bottomleft:6px;border-bottom-left-radius:6px}.btn-group>.btn.large:last-child,.btn-group>.large.dropdown-toggle{-webkit-border-top-right-radius:6px;-moz-border-radius-topright:6px;border-top-right-radius:6px;-webkit-border-bottom-right-radius:6px;-moz-border-radius-bottomright:6px;border-bottom-right-radius:6px}.btn-group>.btn:hover,.btn-group>.btn:focus,.btn-group>.btn:active,.btn-group>.btn.active{z-index:2}.btn-group .dropdown-toggle:active,.btn-group.open .dropdown-toggle{outline:0}.btn-group>.btn+.dropdown-toggle{padding-left:8px;padding-right:8px;-webkit-box-shadow:inset 1px 0 0 rgba(255,255,255,.125),inset 0 1px 0 rgba(255,255,255,.2),0 1px 2px rgba(0,0,0,.05);-moz-box-shadow:inset 1px 0 0 rgba(255,255,255,.125),inset 0 1px 0 rgba(255,255,255,.2),0 1px 2px rgba(0,0,0,.05);box-shadow:inset 1px 0 0 rgba(255,255,255,.125),inset 0 1px 0 rgba(255,255,255,.2),0 1px 2px rgba(0,0,0,.05);*padding-top:5px;*padding-bottom:5px}.btn-group>.btn-mini+.dropdown-toggle{padding-left:5px;padding-right:5px;*padding-top:2px;*padding-bottom:2px}.btn-group>.btn-small+.dropdown-toggle{*padding-top:5px;*padding-bottom:4px}.btn-group>.btn-large+.dropdown-toggle{padding-left:12px;padding-right:12px;*padding-top:7px;*padding-bottom:7px}.btn-group.open .dropdown-toggle{background-image:none;-webkit-box-shadow:inset 0 2px 4px rgba(0,0,0,.15),0 1px 2px rgba(0,0,0,.05);-moz-box-shadow:inset 0 2px 4px rgba(0,0,0,.15),0 1px 2px rgba(0,0,0,.05);box-shadow:inset 0 2px 4px rgba(0,0,0,.15),0 1px 2px rgba(0,0,0,.05)}.btn-group.open .btn.dropdown-toggle{background-color:#e6e6e6}.btn-group.open .btn-primary.dropdown-toggle{background-color:#0048a3}.btn-group.open .btn-warning.dropdown-toggle{background-color:#f89406}.btn-group.open .btn-danger.dropdown-toggle{background-color:#bd362f}.btn-group.open .btn-success.dropdown-toggle{background-color:#336733}.btn-group.open .btn-info.dropdown-toggle{background-color:#2f96b4}.btn-group.open .btn-inverse.dropdown-toggle{background-color:#222}.btn .caret{margin-top:8px;margin-left:0}.btn-large .caret{margin-top:6px}.btn-large .caret{border-left-width:5px;border-right-width:5px;border-top-width:5px}.btn-mini .caret,.btn-small .caret{margin-top:8px}.dropup .btn-large .caret{border-bottom-width:5px}.btn-primary .caret,.btn-warning .caret,.btn-danger .caret,.btn-info .caret,.btn-success .caret,.btn-inverse .caret{border-top-color:#fff;border-bottom-color:#fff}.btn-group-vertical{display:inline-block;*display:inline;*zoom:1}.btn-group-vertical>.btn{display:block;float:none;max-width:100%;-webkit-border-radius:0;-moz-border-radius:0;border-radius:0}.btn-group-vertical>.btn+.btn{margin-left:0;margin-top:-1px}.btn-group-vertical>.btn:first-child{-webkit-border-radius:4px 4px 0 0;-moz-border-radius:4px 4px 0 0;border-radius:4px 4px 0 0}.btn-group-vertical>.btn:last-child{-webkit-border-radius:0 0 4px 4px;-moz-border-radius:0 0 4px 4px;border-radius:0 0 4px 4px}.btn-group-vertical>.btn-large:first-child{-webkit-border-radius:6px 6px 0 0;-moz-border-radius:6px 6px 0 0;border-radius:6px 6px 0 0}.btn-group-vertical>.btn-large:last-child{-webkit-border-radius:0 0 6px 6px;-moz-border-radius:0 0 6px 6px;border-radius:0 0 6px 6px}.alert{padding:8px 35px 8px 14px;margin-bottom:20px;text-shadow:0 1px 0 rgba(255,255,255,.5);background-color:#fcf8e3;border:1px solid #fbeed5;-webkit-border-radius:4px;-moz-border-radius:4px;border-radius:4px}.alert,.alert h4{color:#c09853}.alert h4{margin:0}.alert .close{position:relative;top:-2px;right:-21px;line-height:20px}.alert-success{background-color:#dff0d8;border-color:#d6e9c6;color:#417e42}.alert-success h4{color:#417e42}.alert-danger,.alert-error{background-color:#f2dede;border-color:#eed3d7;color:#b94a48}.alert-danger h4,.alert-error h4{color:#b94a48}.alert-info{background-color:#eef7fb;border-color:#d1eff5;color:#2d6987}.alert-info h4{color:#2d6987}.alert-block{padding-top:14px;padding-bottom:14px}.alert-block>p,.alert-block>ul{margin-bottom:0}.alert-block p+p{margin-top:5px}.nav{margin-left:0;margin-bottom:20px;list-style:none}.nav>li>a{display:block}.nav>li>a:hover,.nav>li>a:focus{text-decoration:none;background-color:#eee}.nav>li>a>img{max-width:none}.nav>.pull-right{float:right}.nav-header{display:block;padding:3px 15px;font-size:11px;font-weight:bold;line-height:20px;color:#6c757d;text-shadow:0 1px 0 rgba(255,255,255,.5);text-transform:uppercase}.nav li+.nav-header{margin-top:9px}.nav-list{padding-left:15px;padding-right:15px;margin-bottom:0}.nav-list>li>a,.nav-list .nav-header{margin-left:-15px;margin-right:-15px;text-shadow:0 1px 0 rgba(255,255,255,.5)}.nav-list>li>a{padding:3px 15px}.nav-list>.active>a,.nav-list>.active>a:hover,.nav-list>.active>a:focus{color:#fff;text-shadow:0 -1px 0 rgba(0,0,0,.2);background-color:#007ea3}.nav-list [class^="icon-"],.nav-list [class*=" icon-"]{margin-right:2px}.nav-list .divider{*width:100%;height:1px;margin:9px 1px;*margin:-5px 0 5px;overflow:hidden;background-color:#e5e5e5;border-bottom:1px solid #fff}.nav-tabs,.nav-pills{*zoom:1}.nav-tabs:before,.nav-pills:before,.nav-tabs:after,.nav-pills:after{display:table;content:"";line-height:0}.nav-tabs:after,.nav-pills:after{clear:both}.nav-tabs>li,.nav-pills>li{float:left}.nav-tabs>li>a,.nav-pills>li>a{padding-right:12px;padding-left:12px;margin-right:2px;line-height:14px}.nav-tabs{border-bottom:1px solid #ddd}.nav-tabs>li{margin-bottom:-1px}.nav-tabs>li>a{padding-top:8px;padding-bottom:8px;line-height:20px;border:1px solid transparent;-webkit-border-radius:4px 4px 0 0;-moz-border-radius:4px 4px 0 0;border-radius:4px 4px 0 0}.nav-tabs>li>a:hover,.nav-tabs>li>a:focus{border-color:#eee #eee #ddd}.nav-tabs>.active>a,.nav-tabs>.active>a:hover,.nav-tabs>.active>a:focus{color:#555;background-color:#fff;border:1px solid #ddd;border-bottom-color:transparent;cursor:default}.nav-pills>li>a{padding-top:8px;padding-bottom:8px;margin-top:2px;margin-bottom:2px;-webkit-border-radius:5px;-moz-border-radius:5px;border-radius:5px}.nav-pills>.active>a,.nav-pills>.active>a:hover,.nav-pills>.active>a:focus{color:#fff;background-color:#007ea3}.nav-stacked>li{float:none}.nav-stacked>li>a{margin-right:0}.nav-tabs.nav-stacked{border-bottom:0}.nav-tabs.nav-stacked>li>a{border:1px solid #ddd;-webkit-border-radius:0;-moz-border-radius:0;border-radius:0}.nav-tabs.nav-stacked>li:first-child>a{-webkit-border-top-right-radius:4px;-moz-border-radius-topright:4px;border-top-right-radius:4px;-webkit-border-top-left-radius:4px;-moz-border-radius-topleft:4px;border-top-left-radius:4px}.nav-tabs.nav-stacked>li:last-child>a{-webkit-border-bottom-right-radius:4px;-moz-border-radius-bottomright:4px;border-bottom-right-radius:4px;-webkit-border-bottom-left-radius:4px;-moz-border-radius-bottomleft:4px;border-bottom-left-radius:4px}.nav-tabs.nav-stacked>li>a:hover,.nav-tabs.nav-stacked>li>a:focus{border-color:#ddd;z-index:2}.nav-pills.nav-stacked>li>a{margin-bottom:3px}.nav-pills.nav-stacked>li:last-child>a{margin-bottom:1px}.nav-tabs .dropdown-menu{-webkit-border-radius:0 0 6px 6px;-moz-border-radius:0 0 6px 6px;border-radius:0 0 6px 6px}.nav-pills .dropdown-menu{-webkit-border-radius:6px;-moz-border-radius:6px;border-radius:6px}.nav .dropdown-toggle .caret{border-top-color:#007ea3;border-bottom-color:#007ea3;margin-top:6px}.nav .dropdown-toggle:hover .caret,.nav .dropdown-toggle:focus .caret{border-top-color:#007ea3;border-bottom-color:#007ea3}.nav-tabs .dropdown-toggle .caret{margin-top:8px}.nav .active .dropdown-toggle .caret{border-top-color:#fff;border-bottom-color:#fff}.nav-tabs .active .dropdown-toggle .caret{border-top-color:#555;border-bottom-color:#555}.nav>.dropdown.active>a:hover,.nav>.dropdown.active>a:focus{cursor:pointer}.nav-tabs .open .dropdown-toggle,.nav-pills .open .dropdown-toggle,.nav>li.dropdown.open.active>a:hover,.nav>li.dropdown.open.active>a:focus{color:#fff;background-color:#6c757d;border-color:#6c757d}.nav li.dropdown.open .caret,.nav li.dropdown.open.active .caret,.nav li.dropdown.open a:hover .caret,.nav li.dropdown.open a:focus .caret{border-top-color:#fff;border-bottom-color:#fff;opacity:1;filter:alpha(opacity=100)}.tabs-stacked .open>a:hover,.tabs-stacked .open>a:focus{border-color:#6c757d}.tabbable{*zoom:1}.tabbable:before,.tabbable:after{display:table;content:"";line-height:0}.tabbable:after{clear:both}.tab-content{overflow:auto}.tabs-below>.nav-tabs,.tabs-right>.nav-tabs,.tabs-left>.nav-tabs{border-bottom:0}.tab-content>.tab-pane,.pill-content>.pill-pane{display:none}.tab-content>.active,.pill-content>.active{display:block}.tabs-below>.nav-tabs{border-top:1px solid #ddd}.tabs-below>.nav-tabs>li{margin-top:-1px;margin-bottom:0}.tabs-below>.nav-tabs>li>a{-webkit-border-radius:0 0 4px 4px;-moz-border-radius:0 0 4px 4px;border-radius:0 0 4px 4px}.tabs-below>.nav-tabs>li>a:hover,.tabs-below>.nav-tabs>li>a:focus{border-bottom-color:transparent;border-top-color:#ddd}.tabs-below>.nav-tabs>.active>a,.tabs-below>.nav-tabs>.active>a:hover,.tabs-below>.nav-tabs>.active>a:focus{border-color:transparent #ddd #ddd #ddd}.tabs-left>.nav-tabs>li,.tabs-right>.nav-tabs>li{float:none}.tabs-left>.nav-tabs>li>a,.tabs-right>.nav-tabs>li>a{min-width:74px;margin-right:0;margin-bottom:3px}.tabs-left>.nav-tabs{float:left;margin-right:19px;border-right:1px solid #ddd}.tabs-left>.nav-tabs>li>a{margin-right:-1px;-webkit-border-radius:4px 0 0 4px;-moz-border-radius:4px 0 0 4px;border-radius:4px 0 0 4px}.tabs-left>.nav-tabs>li>a:hover,.tabs-left>.nav-tabs>li>a:focus{border-color:#eee #ddd #eee #eee}.tabs-left>.nav-tabs .active>a,.tabs-left>.nav-tabs .active>a:hover,.tabs-left>.nav-tabs .active>a:focus{border-color:#ddd transparent #ddd #ddd;*border-right-color:#fff}.tabs-right>.nav-tabs{float:right;margin-left:19px;border-left:1px solid #ddd}.tabs-right>.nav-tabs>li>a{margin-left:-1px;-webkit-border-radius:0 4px 4px 0;-moz-border-radius:0 4px 4px 0;border-radius:0 4px 4px 0}.tabs-right>.nav-tabs>li>a:hover,.tabs-right>.nav-tabs>li>a:focus{border-color:#eee #eee #eee #ddd}.tabs-right>.nav-tabs .active>a,.tabs-right>.nav-tabs .active>a:hover,.tabs-right>.nav-tabs .active>a:focus{border-color:#ddd #ddd #ddd transparent;*border-left-color:#fff}.nav>.disabled>a{color:#6c757d}.nav>.disabled>a:hover,.nav>.disabled>a:focus{text-decoration:none;background-color:transparent;cursor:default}.nav.inline,.nav.inline:before,.nav.inline:after{display:inline-block}.nav.inline{margin-top:0;margin-bottom:0}.nav.inline>li{margin-bottom:inherit}.nav.small-padding>li{font-weight:normal;padding-left:1px;padding-right:1px}.nav.small-padding>li.active{font-weight:bold}.nav.small-padding>li>a{padding-left:5px;padding-right:5px}.nav.smaller{font-size:70%}.navbar{overflow:visible;margin-bottom:20px;*position:relative;*z-index:2}.navbar-inner{min-height:40px;padding-left:20px;padding-right:20px;background-color:#007ea3;background-image:-moz-linear-gradient(top,#007ea3,#007ea3);background-image:-webkit-gradient(linear,0 0,0 100%,from(#007ea3),to(#007ea3));background-image:-webkit-linear-gradient(top,#007ea3,#007ea3);background-image:-o-linear-gradient(top,#007ea3,#007ea3);background-image:linear-gradient(to bottom,#007ea3,#007ea3);background-repeat:repeat-x;filter:progid:DXImageTransform.Microsoft.gradient(startColorstr='#ff007ea3',endColorstr='#ff007ea3',GradientType=0);border:1px solid #007ea3;-webkit-border-radius:4px;-moz-border-radius:4px;border-radius:4px;-webkit-box-shadow:0 1px 4px rgba(0,0,0,.065);-moz-box-shadow:0 1px 4px rgba(0,0,0,.065);box-shadow:0 1px 4px rgba(0,0,0,.065);*zoom:1}.navbar-inner:before,.navbar-inner:after{display:table;content:"";line-height:0}.navbar-inner:after{clear:both}.navbar .container{width:auto}.nav-collapse.collapse{height:auto;overflow:visible}.navbar .brand{float:left;display:block;padding:10px 20px 10px;margin-left:-20px;font-size:20px;font-weight:200;color:#eee;text-shadow:0 1px 0 #007ea3}.navbar .brand:hover,.navbar .brand:focus{text-decoration:none}.navbar-text{margin-bottom:0;line-height:40px;color:#fff}.navbar-link{color:#eee}.navbar-link:hover,.navbar-link:focus{color:#fff}.navbar .divider-vertical{height:40px;margin:0 9px;border-left:1px solid #007ea3;border-right:1px solid #007ea3}.navbar .btn,.navbar .btn-group{margin-top:5px}.navbar .btn-group .btn,.navbar .input-prepend .btn,.navbar .input-append .btn,.navbar .input-prepend .btn-group,.navbar .input-append .btn-group{margin-top:0}.navbar-form{margin-bottom:0;*zoom:1}.navbar-form:before,.navbar-form:after{display:table;content:"";line-height:0}.navbar-form:after{clear:both}.navbar-form input,.navbar-form select,.navbar-form .radio,.navbar-form .checkbox{margin-top:5px}.navbar-form input,.navbar-form select,.navbar-form .btn{display:inline-block;margin-bottom:0}.navbar-form input[type="image"],.navbar-form input[type="checkbox"],.navbar-form input[type="radio"]{margin-top:3px}.navbar-form .input-append,.navbar-form .input-prepend{margin-top:5px;white-space:nowrap}.navbar-form .input-append input,.navbar-form .input-prepend input{margin-top:0}.navbar-search{position:relative;float:left;margin-top:5px;margin-bottom:0}.navbar-search .search-query{margin-bottom:0;padding:4px 14px;font-family:"Helvetica Neue",Helvetica,Arial,sans-serif;font-size:13px;font-weight:normal;line-height:1;-webkit-border-radius:15px;-moz-border-radius:15px;border-radius:15px}.navbar-static-top{position:static;margin-bottom:0}.navbar-static-top .navbar-inner{-webkit-border-radius:0;-moz-border-radius:0;border-radius:0}.navbar-fixed-top,.navbar-fixed-bottom{position:fixed;right:0;left:0;z-index:1030;margin-bottom:0}.navbar-fixed-top .navbar-inner,.navbar-static-top .navbar-inner{border-width:0 0 1px}.navbar-fixed-bottom .navbar-inner{border-width:1px 0 0}.navbar-fixed-top .navbar-inner,.navbar-fixed-bottom .navbar-inner{padding-left:0;padding-right:0;-webkit-border-radius:0;-moz-border-radius:0;border-radius:0}.navbar-static-top .container,.navbar-fixed-top .container,.navbar-fixed-bottom .container{width:940px}.navbar-fixed-top{top:0}.navbar-fixed-top .navbar-inner,.navbar-static-top .navbar-inner{-webkit-box-shadow:0 1px 10px rgba(0,0,0,.1);-moz-box-shadow:0 1px 10px rgba(0,0,0,.1);box-shadow:0 1px 10px rgba(0,0,0,.1)}.navbar-fixed-bottom{bottom:0}.navbar-fixed-bottom .navbar-inner{-webkit-box-shadow:0 -1px 10px rgba(0,0,0,.1);-moz-box-shadow:0 -1px 10px rgba(0,0,0,.1);box-shadow:0 -1px 10px rgba(0,0,0,.1)}.navbar .nav{position:relative;left:0;display:block;float:left;margin:0 10px 0 0}.navbar .nav.pull-right{float:right;margin-right:0}.navbar .nav>li{float:left}.navbar .nav>li>a{float:none;padding:10px 15px 10px;color:#eee;text-decoration:none;text-shadow:0 1px 0 #007ea3}.navbar .nav .dropdown-toggle .caret{margin-top:8px}.navbar .nav>li>a:focus,.navbar .nav>li>a:hover{background-color:transparent;color:#fff;text-decoration:none}.navbar .nav>.active>a,.navbar .nav>.active>a:hover,.navbar .nav>.active>a:focus{color:#333;text-decoration:none;background-color:#fff;-webkit-box-shadow:inset 0 3px 8px rgba(0,0,0,.125);-moz-box-shadow:inset 0 3px 8px rgba(0,0,0,.125);box-shadow:inset 0 3px 8px rgba(0,0,0,.125)}.navbar .btn-navbar{display:none;float:right;padding:7px 10px;margin-left:5px;margin-right:5px;color:#fff;text-shadow:0 -1px 0 rgba(0,0,0,.25);background-color:#006a8a;background-image:-moz-linear-gradient(top,#006a8a,#006a8a);background-image:-webkit-gradient(linear,0 0,0 100%,from(#006a8a),to(#006a8a));background-image:-webkit-linear-gradient(top,#006a8a,#006a8a);background-image:-o-linear-gradient(top,#006a8a,#006a8a);background-image:linear-gradient(to bottom,#006a8a,#006a8a);background-repeat:repeat-x;filter:progid:DXImageTransform.Microsoft.gradient(startColorstr='#ff006a8a',endColorstr='#ff006a8a',GradientType=0);border-color:#006a8a #006a8a #002f3d;border-color:rgba(0,0,0,.1) rgba(0,0,0,.1) rgba(0,0,0,.25);*background-color:#006a8a;filter:progid:DXImageTransform.Microsoft.gradient(enabled=false);-webkit-box-shadow:inset 0 1px 0 rgba(255,255,255,.1),0 1px 0 rgba(255,255,255,.075);-moz-box-shadow:inset 0 1px 0 rgba(255,255,255,.1),0 1px 0 rgba(255,255,255,.075);box-shadow:inset 0 1px 0 rgba(255,255,255,.1),0 1px 0 rgba(255,255,255,.075)}.navbar .btn-navbar:hover,.navbar .btn-navbar:focus,.navbar .btn-navbar:active,.navbar .btn-navbar.active,.navbar .btn-navbar.disabled,.navbar .btn-navbar[disabled]{color:#fff;background-color:#006a8a;*background-color:#005770}.navbar .btn-navbar:active,.navbar .btn-navbar.active{background-color:#004356 \9}.navbar .btn-navbar .icon-bar{display:block;width:18px;height:2px;background-color:#f5f5f5;-webkit-border-radius:1px;-moz-border-radius:1px;border-radius:1px;-webkit-box-shadow:0 1px 0 rgba(0,0,0,.25);-moz-box-shadow:0 1px 0 rgba(0,0,0,.25);box-shadow:0 1px 0 rgba(0,0,0,.25)}.btn-navbar .icon-bar+.icon-bar{margin-top:3px}.navbar .nav>li>.dropdown-menu:before{content:'';display:inline-block;border-left:7px solid transparent;border-right:7px solid transparent;border-bottom:7px solid #ccc;border-bottom-color:rgba(0,0,0,.2);position:absolute;top:-7px;left:9px}.navbar .nav>li>.dropdown-menu:after{content:'';display:inline-block;border-left:6px solid transparent;border-right:6px solid transparent;border-bottom:6px solid #fff;position:absolute;top:-6px;left:10px}.navbar-fixed-bottom .nav>li>.dropdown-menu:before{border-top:7px solid #ccc;border-top-color:rgba(0,0,0,.2);border-bottom:0;bottom:-7px;top:auto}.navbar-fixed-bottom .nav>li>.dropdown-menu:after{border-top:6px solid #fff;border-bottom:0;bottom:-6px;top:auto}.navbar .nav li.dropdown>a:hover .caret,.navbar .nav li.dropdown>a:focus .caret{border-top-color:#fff;border-bottom-color:#fff}.navbar .nav li.dropdown.open>.dropdown-toggle,.navbar .nav li.dropdown.active>.dropdown-toggle,.navbar .nav li.dropdown.open.active>.dropdown-toggle{background-color:#fff;color:#333}.navbar .nav li.dropdown>.dropdown-toggle .caret{border-top-color:#eee;border-bottom-color:#eee}.navbar .nav li.dropdown.open>.dropdown-toggle .caret,.navbar .nav li.dropdown.active>.dropdown-toggle .caret,.navbar .nav li.dropdown.open.active>.dropdown-toggle .caret{border-top-color:#333;border-bottom-color:#333}.navbar .pull-right>li>.dropdown-menu,.navbar .nav>li>.dropdown-menu.pull-right{left:auto;right:0}.navbar .pull-right>li>.dropdown-menu:before,.navbar .nav>li>.dropdown-menu.pull-right:before{left:auto;right:12px}.navbar .pull-right>li>.dropdown-menu:after,.navbar .nav>li>.dropdown-menu.pull-right:after{left:auto;right:13px}.navbar .pull-right>li>.dropdown-menu .dropdown-menu,.navbar .nav>li>.dropdown-menu.pull-right .dropdown-menu{left:auto;right:100%;margin-left:0;margin-right:-1px;-webkit-border-radius:6px 0 6px 6px;-moz-border-radius:6px 0 6px 6px;border-radius:6px 0 6px 6px}.navbar-inverse .navbar-inner{background-color:#1b1b1b;background-image:-moz-linear-gradient(top,#222,#111);background-image:-webkit-gradient(linear,0 0,0 100%,from(#222),to(#111));background-image:-webkit-linear-gradient(top,#222,#111);background-image:-o-linear-gradient(top,#222,#111);background-image:linear-gradient(to bottom,#222,#111);background-repeat:repeat-x;filter:progid:DXImageTransform.Microsoft.gradient(startColorstr='#ff222222',endColorstr='#ff111111',GradientType=0);border-color:#252525}.navbar-inverse .brand,.navbar-inverse .nav>li>a{color:#6c757d;text-shadow:0 -1px 0 rgba(0,0,0,.25)}.navbar-inverse .brand:hover,.navbar-inverse .nav>li>a:hover,.navbar-inverse .brand:focus,.navbar-inverse .nav>li>a:focus{color:#fff}.navbar-inverse .brand{color:#6c757d}.navbar-inverse .navbar-text{color:#6c757d}.navbar-inverse .nav>li>a:focus,.navbar-inverse .nav>li>a:hover{background-color:transparent;color:#fff}.navbar-inverse .nav .active>a,.navbar-inverse .nav .active>a:hover,.navbar-inverse .nav .active>a:focus{color:#fff;background-color:#111}.navbar-inverse .navbar-link{color:#6c757d}.navbar-inverse .navbar-link:hover,.navbar-inverse .navbar-link:focus{color:#fff}.navbar-inverse .divider-vertical{border-left-color:#111;border-right-color:#222}.navbar-inverse .nav li.dropdown.open>.dropdown-toggle,.navbar-inverse .nav li.dropdown.active>.dropdown-toggle,.navbar-inverse .nav li.dropdown.open.active>.dropdown-toggle{background-color:#111;color:#fff}.navbar-inverse .nav li.dropdown>a:hover .caret,.navbar-inverse .nav li.dropdown>a:focus .caret{border-top-color:#fff;border-bottom-color:#fff}.navbar-inverse .nav li.dropdown>.dropdown-toggle .caret{border-top-color:#6c757d;border-bottom-color:#6c757d}.navbar-inverse .nav li.dropdown.open>.dropdown-toggle .caret,.navbar-inverse .nav li.dropdown.active>.dropdown-toggle .caret,.navbar-inverse .nav li.dropdown.open.active>.dropdown-toggle .caret{border-top-color:#fff;border-bottom-color:#fff}.navbar-inverse .navbar-search .search-query{color:#fff;background-color:#515151;border-color:#111;-webkit-box-shadow:inset 0 1px 2px rgba(0,0,0,.1),0 1px 0 rgba(255,255,255,.15);-moz-box-shadow:inset 0 1px 2px rgba(0,0,0,.1),0 1px 0 rgba(255,255,255,.15);box-shadow:inset 0 1px 2px rgba(0,0,0,.1),0 1px 0 rgba(255,255,255,.15);-webkit-transition:none;-moz-transition:none;-o-transition:none;transition:none}.navbar-inverse .navbar-search .search-query:-moz-placeholder{color:#ccc}.navbar-inverse .navbar-search .search-query:-ms-input-placeholder{color:#ccc}.navbar-inverse .navbar-search .search-query::-webkit-input-placeholder{color:#ccc}.navbar-inverse .navbar-search .search-query:focus,.navbar-inverse .navbar-search .search-query.focused{padding:5px 15px;color:#333;text-shadow:0 1px 0 white;background-color:#fff;border:0;-webkit-box-shadow:0 0 3px rgba(0,0,0,.15);-moz-box-shadow:0 0 3px rgba(0,0,0,.15);box-shadow:0 0 3px rgba(0,0,0,.15);outline:0}.navbar-inverse .btn-navbar{color:#fff;text-shadow:0 -1px 0 rgba(0,0,0,.25);background-color:#0e0e0e;background-image:-moz-linear-gradient(top,#151515,#040404);background-image:-webkit-gradient(linear,0 0,0 100%,from(#151515),to(#040404));background-image:-webkit-linear-gradient(top,#151515,#040404);background-image:-o-linear-gradient(top,#151515,#040404);background-image:linear-gradient(to bottom,#151515,#040404);background-repeat:repeat-x;filter:progid:DXImageTransform.Microsoft.gradient(startColorstr='#ff151515',endColorstr='#ff040404',GradientType=0);border-color:#040404 #040404 #000;border-color:rgba(0,0,0,.1) rgba(0,0,0,.1) rgba(0,0,0,.25);*background-color:#040404;filter:progid:DXImageTransform.Microsoft.gradient(enabled=false)}.navbar-inverse .btn-navbar:hover,.navbar-inverse .btn-navbar:focus,.navbar-inverse .btn-navbar:active,.navbar-inverse .btn-navbar.active,.navbar-inverse .btn-navbar.disabled,.navbar-inverse .btn-navbar[disabled]{color:#fff;background-color:#040404;*background-color:#000}.navbar-inverse .btn-navbar:active,.navbar-inverse .btn-navbar.active{background-color:#000 \9}.breadcrumb{padding:8px 15px;margin:0 0 20px;list-style:none;background-color:#f5f5f5;-webkit-border-radius:4px;-moz-border-radius:4px;border-radius:4px}.breadcrumb>li{display:inline-block;*display:inline;*zoom:1;text-shadow:0 1px 0 white}.breadcrumb>li>.divider{padding:0 5px;color:#ccc}.breadcrumb>.active{color:#6c757d}.pagination{margin:20px 0}.pagination ul{display:inline-block;*display:inline;*zoom:1;margin-left:0;margin-bottom:0;-webkit-border-radius:4px;-moz-border-radius:4px;border-radius:4px;-webkit-box-shadow:0 1px 2px rgba(0,0,0,.05);-moz-box-shadow:0 1px 2px rgba(0,0,0,.05);box-shadow:0 1px 2px rgba(0,0,0,.05)}.pagination ul>li{display:inline}.pagination ul>li>a,.pagination ul>li>span{float:left;padding:4px 12px;line-height:20px;text-decoration:none;background-color:#fff;border:1px solid #ddd;border-left-width:0}.pagination ul>li>a:hover,.pagination ul>li>a:focus,.pagination ul>.active>a,.pagination ul>.active>span{background-color:#f5f5f5}.pagination ul>.active>a,.pagination ul>.active>span{color:#6c757d;cursor:default}.pagination ul>.disabled>span,.pagination ul>.disabled>a,.pagination ul>.disabled>a:hover,.pagination ul>.disabled>a:focus{color:#6c757d;background-color:transparent;cursor:default}.pagination ul>li:first-child>a,.pagination ul>li:first-child>span{border-left-width:1px;-webkit-border-top-left-radius:4px;-moz-border-radius-topleft:4px;border-top-left-radius:4px;-webkit-border-bottom-left-radius:4px;-moz-border-radius-bottomleft:4px;border-bottom-left-radius:4px}.pagination ul>li:last-child>a,.pagination ul>li:last-child>span{-webkit-border-top-right-radius:4px;-moz-border-radius-topright:4px;border-top-right-radius:4px;-webkit-border-bottom-right-radius:4px;-moz-border-radius-bottomright:4px;border-bottom-right-radius:4px}.pagination-centered{text-align:center}.pagination-right{text-align:right}.pagination-large ul>li>a,.pagination-large ul>li>span{padding:11px 19px;font-size:17.5px}.pagination-large ul>li:first-child>a,.pagination-large ul>li:first-child>span{-webkit-border-top-left-radius:6px;-moz-border-radius-topleft:6px;border-top-left-radius:6px;-webkit-border-bottom-left-radius:6px;-moz-border-radius-bottomleft:6px;border-bottom-left-radius:6px}.pagination-large ul>li:last-child>a,.pagination-large ul>li:last-child>span{-webkit-border-top-right-radius:6px;-moz-border-radius-topright:6px;border-top-right-radius:6px;-webkit-border-bottom-right-radius:6px;-moz-border-radius-bottomright:6px;border-bottom-right-radius:6px}.pagination-mini ul>li:first-child>a,.pagination-small ul>li:first-child>a,.pagination-mini ul>li:first-child>span,.pagination-small ul>li:first-child>span{-webkit-border-top-left-radius:3px;-moz-border-radius-topleft:3px;border-top-left-radius:3px;-webkit-border-bottom-left-radius:3px;-moz-border-radius-bottomleft:3px;border-bottom-left-radius:3px}.pagination-mini ul>li:last-child>a,.pagination-small ul>li:last-child>a,.pagination-mini ul>li:last-child>span,.pagination-small ul>li:last-child>span{-webkit-border-top-right-radius:3px;-moz-border-radius-topright:3px;border-top-right-radius:3px;-webkit-border-bottom-right-radius:3px;-moz-border-radius-bottomright:3px;border-bottom-right-radius:3px}.pagination-small ul>li>a,.pagination-small ul>li>span{padding:2px 10px;font-size:11.9px}.pagination-mini ul>li>a,.pagination-mini ul>li>span{padding:0 6px;font-size:10.5px}.pager{margin:20px 0;list-style:none;text-align:center;*zoom:1}.pager:before,.pager:after{display:table;content:"";line-height:0}.pager:after{clear:both}.pager li{display:inline}.pager li>a,.pager li>span{display:inline-block;padding:5px 14px;background-color:#fff;border:1px solid #ddd;-webkit-border-radius:15px;-moz-border-radius:15px;border-radius:15px}.pager li>a:hover,.pager li>a:focus{text-decoration:none;background-color:#f5f5f5}.pager .next>a,.pager .next>span{float:right}.pager .previous>a,.pager .previous>span{float:left}.pager .disabled>a,.pager .disabled>a:hover,.pager .disabled>a:focus,.pager .disabled>span{color:#6c757d;background-color:#fff;cursor:default}.modal-backdrop{position:fixed;top:0;right:0;bottom:0;left:0;z-index:1040;background-color:#000}.modal-backdrop.fade{opacity:0}.modal-backdrop,.modal-backdrop.fade.in{opacity:.8;filter:alpha(opacity=80)}.modalBase{position:fixed;top:10%;left:50%;z-index:1050;width:560px;margin-left:-280px;background-color:#fff;border:1px solid #999;border:1px solid rgba(0,0,0,.3);*border:1px solid #999;-webkit-border-radius:6px;-moz-border-radius:6px;border-radius:6px;-webkit-box-shadow:0 3px 7px rgba(0,0,0,.3);-moz-box-shadow:0 3px 7px rgba(0,0,0,.3);box-shadow:0 3px 7px rgba(0,0,0,.3);-webkit-background-clip:padding-box;-moz-background-clip:padding-box;background-clip:padding-box;outline:none}.modalBase.fade{-webkit-transition:opacity .3s linear,top .3s ease-out;-moz-transition:opacity .3s linear,top .3s ease-out;-o-transition:opacity .3s linear,top .3s ease-out;transition:opacity .3s linear,top .3s ease-out;top:-25%}.modalBase.fade.in{top:10%}.modal{position:fixed;top:10%;left:50%;z-index:1050;width:560px;margin-left:-280px;background-color:#fff;border:1px solid #999;border:1px solid rgba(0,0,0,.3);*border:1px solid #999;-webkit-border-radius:6px;-moz-border-radius:6px;border-radius:6px;-webkit-box-shadow:0 3px 7px rgba(0,0,0,.3);-moz-box-shadow:0 3px 7px rgba(0,0,0,.3);box-shadow:0 3px 7px rgba(0,0,0,.3);-webkit-background-clip:padding-box;-moz-background-clip:padding-box;background-clip:padding-box;outline:none}.modal.fade{-webkit-transition:opacity .3s linear,top .3s ease-out;-moz-transition:opacity .3s linear,top .3s ease-out;-o-transition:opacity .3s linear,top .3s ease-out;transition:opacity .3s linear,top .3s ease-out;top:-25%}.modal.fade.in{top:10%}.modal-header{padding:9px 15px;border-bottom:1px solid #eee}.modal-header .close{margin-top:2px}.modal-header h1,.modal-header h2,.modal-header h3{margin:0;line-height:30px}.modal-body{position:relative;overflow-y:auto;max-height:60vh;padding:15px}.modal-form{margin-bottom:0}.modal-footer{padding:14px 15px 15px;margin-bottom:0;text-align:right;background-color:#f5f5f5;border-top:1px solid #ddd;-webkit-border-radius:0 0 6px 6px;-moz-border-radius:0 0 6px 6px;border-radius:0 0 6px 6px;-webkit-box-shadow:inset 0 1px 0 white;-moz-box-shadow:inset 0 1px 0 white;box-shadow:inset 0 1px 0 white;*zoom:1}.modal-footer:before,.modal-footer:after{display:table;content:"";line-height:0}.modal-footer:after{clear:both}.modal-footer .btn+.btn{margin-left:5px;margin-bottom:0}.modal-footer .btn-group .btn+.btn{margin-left:-1px}.modal-footer .btn-block+.btn-block{margin-left:0}.tooltip{position:absolute;z-index:1030;display:block;visibility:visible;font-size:11px;line-height:1.4;opacity:0;filter:alpha(opacity=0)}.tooltip.in{opacity:.8;filter:alpha(opacity=80)}.tooltip.top{margin-top:-3px;padding:5px 0}.tooltip.right{margin-left:3px;padding:0 5px}.tooltip.bottom{margin-top:3px;padding:5px 0}.tooltip.left{margin-left:-3px;padding:0 5px}.tooltip-inner{max-width:200px;padding:8px;color:#fff;text-align:center;text-decoration:none;background-color:#000;-webkit-border-radius:4px;-moz-border-radius:4px;border-radius:4px}.tooltip-arrow{position:absolute;width:0;height:0;border-color:transparent;border-style:solid}.tooltip.top .tooltip-arrow{bottom:0;left:50%;margin-left:-5px;border-width:5px 5px 0;border-top-color:#000}.tooltip.right .tooltip-arrow{top:50%;left:0;margin-top:-5px;border-width:5px 5px 5px 0;border-right-color:#000}.tooltip.left .tooltip-arrow{top:50%;right:0;margin-top:-5px;border-width:5px 0 5px 5px;border-left-color:#000}.tooltip.bottom .tooltip-arrow{top:0;left:50%;margin-left:-5px;border-width:0 5px 5px;border-bottom-color:#000}.popover{position:absolute;top:0;left:0;z-index:1010;display:none;max-width:276px;padding:1px;text-align:left;background-color:#fff;-webkit-background-clip:padding-box;-moz-background-clip:padding;background-clip:padding-box;border:1px solid #ccc;border:1px solid rgba(0,0,0,.2);-webkit-border-radius:6px;-moz-border-radius:6px;border-radius:6px;-webkit-box-shadow:0 5px 10px rgba(0,0,0,.2);-moz-box-shadow:0 5px 10px rgba(0,0,0,.2);box-shadow:0 5px 10px rgba(0,0,0,.2);white-space:normal}.popover.top{margin-top:-10px}.popover.right{margin-left:10px}.popover.bottom{margin-top:10px}.popover.left{margin-left:-10px}.popover-title{margin:0;padding:8px 14px;font-size:14px;font-weight:normal;line-height:18px;background-color:#f7f7f7;border-bottom:1px solid #eaeaea;-webkit-border-radius:5px 5px 0 0;-moz-border-radius:5px 5px 0 0;border-radius:5px 5px 0 0}.popover-title:empty{display:none}.popover-content{padding:9px 14px}.popover .arrow,.popover .arrow:after{position:absolute;display:block;width:0;height:0;border-color:transparent;border-style:solid}.popover .arrow{border-width:11px}.popover .arrow:after{border-width:10px;content:""}.popover.top .arrow{left:50%;margin-left:-11px;border-bottom-width:0;border-top-color:#999;border-top-color:rgba(0,0,0,.25);bottom:-11px}.popover.top .arrow:after{bottom:1px;margin-left:-10px;border-bottom-width:0;border-top-color:#fff}.popover.right .arrow{top:50%;left:-11px;margin-top:-11px;border-left-width:0;border-right-color:#999;border-right-color:rgba(0,0,0,.25)}.popover.right .arrow:after{left:1px;bottom:-10px;border-left-width:0;border-right-color:#fff}.popover.bottom .arrow{left:50%;margin-left:-11px;border-top-width:0;border-bottom-color:#999;border-bottom-color:rgba(0,0,0,.25);top:-11px}.popover.bottom .arrow:after{top:1px;margin-left:-10px;border-top-width:0;border-bottom-color:#fff}.popover.left .arrow{top:50%;right:-11px;margin-top:-11px;border-right-width:0;border-left-color:#999;border-left-color:rgba(0,0,0,.25)}.popover.left .arrow:after{right:1px;border-right-width:0;border-left-color:#fff;bottom:-10px}.thumbnails{margin-left:-20px;list-style:none;*zoom:1}.thumbnails:before,.thumbnails:after{display:table;content:"";line-height:0}.thumbnails:after{clear:both}.row-fluid .thumbnails{margin-left:0}.thumbnails>li{float:left;margin-bottom:20px;margin-left:20px}.thumbnail{display:block;padding:4px;line-height:20px;border:1px solid #ddd;-webkit-border-radius:4px;-moz-border-radius:4px;border-radius:4px;-webkit-box-shadow:0 1px 3px rgba(0,0,0,.055);-moz-box-shadow:0 1px 3px rgba(0,0,0,.055);box-shadow:0 1px 3px rgba(0,0,0,.055);-webkit-transition:all .2s ease-in-out;-moz-transition:all .2s ease-in-out;-o-transition:all .2s ease-in-out;transition:all .2s ease-in-out}a.thumbnail:hover,a.thumbnail:focus{border-color:#007294;-webkit-box-shadow:0 1px 4px rgba(0,105,214,.25);-moz-box-shadow:0 1px 4px rgba(0,105,214,.25);box-shadow:0 1px 4px rgba(0,105,214,.25)}.thumbnail>img{display:block;max-width:100%;margin-left:auto;margin-right:auto}.thumbnail .caption{padding:9px;color:#555}.media,.media-body{overflow:hidden;*overflow:visible;zoom:1}.media,.media .media{margin-top:15px}.media:first-child{margin-top:0}.media-object{display:block}.media-heading{margin:0 0 5px}.media>.pull-left{margin-right:10px}.media>.pull-right{margin-left:10px}.media-list{margin-left:0;list-style:none}.label,.badge{display:inline-block;padding:2px 4px;font-size:11.844px;font-weight:bold;line-height:14px;color:#fff;vertical-align:baseline;white-space:nowrap;text-shadow:0 -1px 0 rgba(0,0,0,.25);background-color:#6c757d}.label{-webkit-border-radius:3px;-moz-border-radius:3px;border-radius:3px}.badge{padding-left:9px;padding-right:9px;-webkit-border-radius:9px;-moz-border-radius:9px;border-radius:9px}.label:empty,.badge:empty{display:none}a.label:hover,a.label:focus,a.badge:hover,a.badge:focus{color:#fff;text-decoration:none;cursor:pointer}.label-important,.badge-important{background-color:#b94a48}.label-important[href],.badge-important[href]{background-color:#953b39}.label-warning,.badge-warning{background-color:#f89406}.label-warning[href],.badge-warning[href]{background-color:#c67605}.label-success,.badge-success{background-color:#417e42}.label-success[href],.badge-success[href]{background-color:#2f5c30}.label-info,.badge-info{background-color:#2d6987}.label-info[href],.badge-info[href]{background-color:#204b61}.label-inverse,.badge-inverse{background-color:#333}.label-inverse[href],.badge-inverse[href]{background-color:#1a1a1a}.btn .label,.btn .badge{position:relative;top:-1px}.btn-mini .label,.btn-mini .badge{top:0}@-webkit-keyframes progress-bar-stripes{from{background-position:40px 0}to{background-position:0 0}}@-moz-keyframes progress-bar-stripes{from{background-position:40px 0}to{background-position:0 0}}@-ms-keyframes progress-bar-stripes{from{background-position:40px 0}to{background-position:0 0}}@-o-keyframes progress-bar-stripes{from{background-position:0 0;}to{background-position:40px 0;}}@keyframes progress-bar-stripes{from{background-position:40px 0}to{background-position:0 0}}.progress{overflow:hidden;height:20px;margin-bottom:20px;background-color:#f7f7f7;background-image:-moz-linear-gradient(top,whitesmoke,#f9f9f9);background-image:-webkit-gradient(linear,0 0,0 100%,from(whitesmoke),to(#f9f9f9));background-image:-webkit-linear-gradient(top,whitesmoke,#f9f9f9);background-image:-o-linear-gradient(top,whitesmoke,#f9f9f9);background-image:linear-gradient(to bottom,whitesmoke,#f9f9f9);background-repeat:repeat-x;filter:progid:DXImageTransform.Microsoft.gradient(startColorstr='#fff5f5f5',endColorstr='#fff9f9f9',GradientType=0);-webkit-box-shadow:inset 0 1px 2px rgba(0,0,0,.1);-moz-box-shadow:inset 0 1px 2px rgba(0,0,0,.1);box-shadow:inset 0 1px 2px rgba(0,0,0,.1);-webkit-border-radius:4px;-moz-border-radius:4px;border-radius:4px}.progress .bar{width:0%;height:100%;color:#fff;float:left;font-size:12px;text-align:center;text-shadow:0 -1px 0 rgba(0,0,0,.25);background-color:#0e90d2;background-image:-moz-linear-gradient(top,#149bdf,#0480be);background-image:-webkit-gradient(linear,0 0,0 100%,from(#149bdf),to(#0480be));background-image:-webkit-linear-gradient(top,#149bdf,#0480be);background-image:-o-linear-gradient(top,#149bdf,#0480be);background-image:linear-gradient(to bottom,#149bdf,#0480be);background-repeat:repeat-x;filter:progid:DXImageTransform.Microsoft.gradient(startColorstr='#ff149bdf',endColorstr='#ff0480be',GradientType=0);-webkit-box-shadow:inset 0 -1px 0 rgba(0,0,0,.15);-moz-box-shadow:inset 0 -1px 0 rgba(0,0,0,.15);box-shadow:inset 0 -1px 0 rgba(0,0,0,.15);-webkit-box-sizing:border-box;-moz-box-sizing:border-box;box-sizing:border-box;-webkit-transition:width .6s ease;-moz-transition:width .6s ease;-o-transition:width .6s ease;transition:width .6s ease}.progress .bar+.bar{-webkit-box-shadow:inset 1px 0 0 rgba(0,0,0,.15),inset 0 -1px 0 rgba(0,0,0,.15);-moz-box-shadow:inset 1px 0 0 rgba(0,0,0,.15),inset 0 -1px 0 rgba(0,0,0,.15);box-shadow:inset 1px 0 0 rgba(0,0,0,.15),inset 0 -1px 0 rgba(0,0,0,.15)}.progress-striped .bar{background-color:#149bdf;background-image:-webkit-gradient(linear,0 100%,100% 0,color-stop(.25,rgba(255,255,255,.15)),color-stop(.25,transparent),color-stop(.5,transparent),color-stop(.5,rgba(255,255,255,.15)),color-stop(.75,rgba(255,255,255,.15)),color-stop(.75,transparent),to(transparent));background-image:-webkit-linear-gradient(45deg,rgba(255,255,255,.15) 25%,transparent 25%,transparent 50%,rgba(255,255,255,.15) 50%,rgba(255,255,255,.15) 75%,transparent 75%,transparent);background-image:-moz-linear-gradient(45deg,rgba(255,255,255,.15) 25%,transparent 25%,transparent 50%,rgba(255,255,255,.15) 50%,rgba(255,255,255,.15) 75%,transparent 75%,transparent);background-image:-o-linear-gradient(45deg,rgba(255,255,255,.15) 25%,transparent 25%,transparent 50%,rgba(255,255,255,.15) 50%,rgba(255,255,255,.15) 75%,transparent 75%,transparent);background-image:linear-gradient(45deg,rgba(255,255,255,.15) 25%,transparent 25%,transparent 50%,rgba(255,255,255,.15) 50%,rgba(255,255,255,.15) 75%,transparent 75%,transparent);-webkit-background-size:40px 40px;-moz-background-size:40px 40px;-o-background-size:40px 40px;background-size:40px 40px}.progress.active .bar{-webkit-animation:progress-bar-stripes 2s linear infinite;-moz-animation:progress-bar-stripes 2s linear infinite;-ms-animation:progress-bar-stripes 2s linear infinite;-o-animation:progress-bar-stripes 2s linear infinite;animation:progress-bar-stripes 2s linear infinite}.progress-danger .bar,.progress .bar-danger{background-color:#dd514c;background-image:-moz-linear-gradient(top,#ee5f5b,#c43c35);background-image:-webkit-gradient(linear,0 0,0 100%,from(#ee5f5b),to(#c43c35));background-image:-webkit-linear-gradient(top,#ee5f5b,#c43c35);background-image:-o-linear-gradient(top,#ee5f5b,#c43c35);background-image:linear-gradient(to bottom,#ee5f5b,#c43c35);background-repeat:repeat-x;filter:progid:DXImageTransform.Microsoft.gradient(startColorstr='#ffee5f5b',endColorstr='#ffc43c35',GradientType=0)}.progress-danger.progress-striped .bar,.progress-striped .bar-danger{background-color:#ee5f5b;background-image:-webkit-gradient(linear,0 100%,100% 0,color-stop(.25,rgba(255,255,255,.15)),color-stop(.25,transparent),color-stop(.5,transparent),color-stop(.5,rgba(255,255,255,.15)),color-stop(.75,rgba(255,255,255,.15)),color-stop(.75,transparent),to(transparent));background-image:-webkit-linear-gradient(45deg,rgba(255,255,255,.15) 25%,transparent 25%,transparent 50%,rgba(255,255,255,.15) 50%,rgba(255,255,255,.15) 75%,transparent 75%,transparent);background-image:-moz-linear-gradient(45deg,rgba(255,255,255,.15) 25%,transparent 25%,transparent 50%,rgba(255,255,255,.15) 50%,rgba(255,255,255,.15) 75%,transparent 75%,transparent);background-image:-o-linear-gradient(45deg,rgba(255,255,255,.15) 25%,transparent 25%,transparent 50%,rgba(255,255,255,.15) 50%,rgba(255,255,255,.15) 75%,transparent 75%,transparent);background-image:linear-gradient(45deg,rgba(255,255,255,.15) 25%,transparent 25%,transparent 50%,rgba(255,255,255,.15) 50%,rgba(255,255,255,.15) 75%,transparent 75%,transparent)}.progress-success .bar,.progress .bar-success{background-color:#5eb95e;background-image:-moz-linear-gradient(top,#62c462,#57a957);background-image:-webkit-gradient(linear,0 0,0 100%,from(#62c462),to(#57a957));background-image:-webkit-linear-gradient(top,#62c462,#57a957);background-image:-o-linear-gradient(top,#62c462,#57a957);background-image:linear-gradient(to bottom,#62c462,#57a957);background-repeat:repeat-x;filter:progid:DXImageTransform.Microsoft.gradient(startColorstr='#ff62c462',endColorstr='#ff57a957',GradientType=0)}.progress-success.progress-striped .bar,.progress-striped .bar-success{background-color:#62c462;background-image:-webkit-gradient(linear,0 100%,100% 0,color-stop(.25,rgba(255,255,255,.15)),color-stop(.25,transparent),color-stop(.5,transparent),color-stop(.5,rgba(255,255,255,.15)),color-stop(.75,rgba(255,255,255,.15)),color-stop(.75,transparent),to(transparent));background-image:-webkit-linear-gradient(45deg,rgba(255,255,255,.15) 25%,transparent 25%,transparent 50%,rgba(255,255,255,.15) 50%,rgba(255,255,255,.15) 75%,transparent 75%,transparent);background-image:-moz-linear-gradient(45deg,rgba(255,255,255,.15) 25%,transparent 25%,transparent 50%,rgba(255,255,255,.15) 50%,rgba(255,255,255,.15) 75%,transparent 75%,transparent);background-image:-o-linear-gradient(45deg,rgba(255,255,255,.15) 25%,transparent 25%,transparent 50%,rgba(255,255,255,.15) 50%,rgba(255,255,255,.15) 75%,transparent 75%,transparent);background-image:linear-gradient(45deg,rgba(255,255,255,.15) 25%,transparent 25%,transparent 50%,rgba(255,255,255,.15) 50%,rgba(255,255,255,.15) 75%,transparent 75%,transparent)}.progress-info .bar,.progress .bar-info{background-color:#4bb1cf;background-image:-moz-linear-gradient(top,#5bc0de,#339bb9);background-image:-webkit-gradient(linear,0 0,0 100%,from(#5bc0de),to(#339bb9));background-image:-webkit-linear-gradient(top,#5bc0de,#339bb9);background-image:-o-linear-gradient(top,#5bc0de,#339bb9);background-image:linear-gradient(to bottom,#5bc0de,#339bb9);background-repeat:repeat-x;filter:progid:DXImageTransform.Microsoft.gradient(startColorstr='#ff5bc0de',endColorstr='#ff339bb9',GradientType=0)}.progress-info.progress-striped .bar,.progress-striped .bar-info{background-color:#5bc0de;background-image:-webkit-gradient(linear,0 100%,100% 0,color-stop(.25,rgba(255,255,255,.15)),color-stop(.25,transparent),color-stop(.5,transparent),color-stop(.5,rgba(255,255,255,.15)),color-stop(.75,rgba(255,255,255,.15)),color-stop(.75,transparent),to(transparent));background-image:-webkit-linear-gradient(45deg,rgba(255,255,255,.15) 25%,transparent 25%,transparent 50%,rgba(255,255,255,.15) 50%,rgba(255,255,255,.15) 75%,transparent 75%,transparent);background-image:-moz-linear-gradient(45deg,rgba(255,255,255,.15) 25%,transparent 25%,transparent 50%,rgba(255,255,255,.15) 50%,rgba(255,255,255,.15) 75%,transparent 75%,transparent);background-image:-o-linear-gradient(45deg,rgba(255,255,255,.15) 25%,transparent 25%,transparent 50%,rgba(255,255,255,.15) 50%,rgba(255,255,255,.15) 75%,transparent 75%,transparent);background-image:linear-gradient(45deg,rgba(255,255,255,.15) 25%,transparent 25%,transparent 50%,rgba(255,255,255,.15) 50%,rgba(255,255,255,.15) 75%,transparent 75%,transparent)}.progress-warning .bar,.progress .bar-warning{background-color:#faa732;background-image:-moz-linear-gradient(top,#fbb450,#f89406);background-image:-webkit-gradient(linear,0 0,0 100%,from(#fbb450),to(#f89406));background-image:-webkit-linear-gradient(top,#fbb450,#f89406);background-image:-o-linear-gradient(top,#fbb450,#f89406);background-image:linear-gradient(to bottom,#fbb450,#f89406);background-repeat:repeat-x;filter:progid:DXImageTransform.Microsoft.gradient(startColorstr='#fffbb450',endColorstr='#fff89406',GradientType=0)}.progress-warning.progress-striped .bar,.progress-striped .bar-warning{background-color:#fbb450;background-image:-webkit-gradient(linear,0 100%,100% 0,color-stop(.25,rgba(255,255,255,.15)),color-stop(.25,transparent),color-stop(.5,transparent),color-stop(.5,rgba(255,255,255,.15)),color-stop(.75,rgba(255,255,255,.15)),color-stop(.75,transparent),to(transparent));background-image:-webkit-linear-gradient(45deg,rgba(255,255,255,.15) 25%,transparent 25%,transparent 50%,rgba(255,255,255,.15) 50%,rgba(255,255,255,.15) 75%,transparent 75%,transparent);background-image:-moz-linear-gradient(45deg,rgba(255,255,255,.15) 25%,transparent 25%,transparent 50%,rgba(255,255,255,.15) 50%,rgba(255,255,255,.15) 75%,transparent 75%,transparent);background-image:-o-linear-gradient(45deg,rgba(255,255,255,.15) 25%,transparent 25%,transparent 50%,rgba(255,255,255,.15) 50%,rgba(255,255,255,.15) 75%,transparent 75%,transparent);background-image:linear-gradient(45deg,rgba(255,255,255,.15) 25%,transparent 25%,transparent 50%,rgba(255,255,255,.15) 50%,rgba(255,255,255,.15) 75%,transparent 75%,transparent)}.accordion{margin-bottom:20px}.accordion-group{margin-bottom:2px;border:1px solid #e5e5e5;-webkit-border-radius:4px;-moz-border-radius:4px;border-radius:4px}.accordion-heading{border-bottom:0}.accordion-heading .accordion-toggle{display:block;padding:8px 15px}.accordion-toggle{cursor:pointer}.accordion-inner{padding:9px 15px;border-top:1px solid #e5e5e5}.carousel{position:relative;margin-bottom:20px;line-height:1}.carousel-inner{overflow:hidden;width:100%;position:relative}.carousel-inner>.item{display:none;position:relative;-webkit-transition:.6s ease-in-out left;-moz-transition:.6s ease-in-out left;-o-transition:.6s ease-in-out left;transition:.6s ease-in-out left}.carousel-inner>.item>img,.carousel-inner>.item>a>img{display:block;line-height:1}.carousel-inner>.active,.carousel-inner>.next,.carousel-inner>.prev{display:block}.carousel-inner>.active{left:0}.carousel-inner>.next,.carousel-inner>.prev{position:absolute;top:0;width:100%}.carousel-inner>.next{left:100%}.carousel-inner>.prev{left:-100%}.carousel-inner>.next.left,.carousel-inner>.prev.right{left:0}.carousel-inner>.active.left{left:-100%}.carousel-inner>.active.right{left:100%}.carousel-control{position:absolute;top:40%;left:15px;width:40px;height:40px;margin-top:-20px;font-size:60px;font-weight:100;line-height:30px;color:#fff;text-align:center;background:#222;border:3px solid #fff;-webkit-border-radius:23px;-moz-border-radius:23px;border-radius:23px;opacity:.5;filter:alpha(opacity=50)}.carousel-control.right{left:auto;right:15px}.carousel-control:hover,.carousel-control:focus{color:#fff;text-decoration:none;opacity:.9;filter:alpha(opacity=90)}.carousel-indicators{position:absolute;top:15px;right:15px;z-index:5;margin:0;list-style:none}.carousel-indicators li{display:block;float:left;width:10px;height:10px;margin-left:5px;text-indent:-999px;background-color:#ccc;background-color:rgba(255,255,255,.25);border-radius:5px}.carousel-indicators .active{background-color:#fff}.carousel-caption{position:absolute;left:0;right:0;bottom:0;padding:15px;background:#333;background:rgba(0,0,0,.75)}.carousel-caption h4,.carousel-caption p{color:#fff;line-height:20px}.carousel-caption h4{margin:0 0 5px}.carousel-caption p{margin-bottom:0}.hero-unit{padding:60px;margin-bottom:30px;font-size:18px;font-weight:200;line-height:30px;color:inherit;background-color:#eee;-webkit-border-radius:6px;-moz-border-radius:6px;border-radius:6px}.hero-unit h1{margin-bottom:0;font-size:60px;line-height:1;color:inherit;letter-spacing:-1px}.hero-unit li{line-height:30px}.pull-right{float:right}.pull-left{float:left}.hide{display:none}.show{display:block}.invisible{visibility:hidden}.affix{position:fixed}@-ms-viewport{width:device-width;}.hidden{display:none;visibility:hidden}.visible-phone{display:none!important}.visible-tablet{display:none!important}.hidden-desktop{display:none!important}.visible-desktop{display:inherit!important}@media(min-width:768px) and (max-width:979px){.hidden-desktop{display:inherit!important}.visible-desktop{display:none!important}.visible-tablet{display:inherit!important}.hidden-tablet{display:none!important}}@media(max-width:767px){.hidden-desktop{display:inherit!important}.visible-desktop{display:none!important}.visible-phone{display:inherit!important}.hidden-phone{display:none!important}}.visible-print{display:none!important}@media print{.visible-print{display:inherit!important}.hidden-print{display:none!important}}@media(min-width:1200px){.row{margin-left:-30px;*zoom:1}.row:before,.row:after{display:table;content:"";line-height:0}.row:after{clear:both}[class*="span"]{float:left;min-height:1px;margin-left:30px}.container,.navbar-static-top .container,.navbar-fixed-top .container,.navbar-fixed-bottom .container{width:97%}.span12{width:1170px}.span11{width:1070px}.span10{width:970px}.span9{width:870px}.span8{width:770px}.span7{width:670px}.span6{width:570px}.span5{width:470px}.span4{width:370px}.span3{width:270px}.span2{width:170px}.span1{width:70px}.offset12{margin-left:1230px}.offset11{margin-left:1130px}.offset10{margin-left:1030px}.offset9{margin-left:930px}.offset8{margin-left:830px}.offset7{margin-left:730px}.offset6{margin-left:630px}.offset5{margin-left:530px}.offset4{margin-left:430px}.offset3{margin-left:330px}.offset2{margin-left:230px}.offset1{margin-left:130px}.row-fluid{width:100%;*zoom:1}.row-fluid:before,.row-fluid:after{display:table;content:"";line-height:0}.row-fluid:after{clear:both}.row-fluid [class*="span"]{display:block;width:100%;min-height:30px;-webkit-box-sizing:border-box;-moz-box-sizing:border-box;box-sizing:border-box;float:left;margin-left:2.564102564%;*margin-left:2.510911075%}.row-fluid [class*="span"]:first-child{margin-left:0}.row-fluid .controls-row [class*="span"]+[class*="span"]{margin-left:2.564102564%}.row-fluid .span12{width:100%;*width:99.946808511%}.row-fluid .span11{width:91.452991453%;*width:91.399799964%}.row-fluid .span10{width:82.905982906%;*width:82.852791417%}.row-fluid .span9{width:74.358974359%;*width:74.30578287%}.row-fluid .span8{width:65.811965812%;*width:65.758774323%}.row-fluid .span7{width:57.264957265%;*width:57.211765776%}.row-fluid .span6{width:48.717948718%;*width:48.664757229%}.row-fluid .span5{width:40.170940171%;*width:40.117748682%}.row-fluid .span4{width:31.623931624%;*width:31.570740135%}.row-fluid .span3{width:23.076923077%;*width:23.023731588%}.row-fluid .span2{width:14.52991453%;*width:14.476723041%}.row-fluid .span1{width:5.982905983%;*width:5.929714494%}.row-fluid .offset12{margin-left:105.128205128%;*margin-left:105.021822149%}.row-fluid .offset12:first-child{margin-left:102.564102564%;*margin-left:102.457719585%}.row-fluid .offset11{margin-left:96.581196581%;*margin-left:96.474813602%}.row-fluid .offset11:first-child{margin-left:94.017094017%;*margin-left:93.910711038%}.row-fluid .offset10{margin-left:88.034188034%;*margin-left:87.927805055%}.row-fluid .offset10:first-child{margin-left:85.47008547%;*margin-left:85.363702491%}.row-fluid .offset9{margin-left:79.487179487%;*margin-left:79.380796508%}.row-fluid .offset9:first-child{margin-left:76.923076923%;*margin-left:76.816693944%}.row-fluid .offset8{margin-left:70.94017094%;*margin-left:70.833787961%}.row-fluid .offset8:first-child{margin-left:68.376068376%;*margin-left:68.269685397%}.row-fluid .offset7{margin-left:62.393162393%;*margin-left:62.286779414%}.row-fluid .offset7:first-child{margin-left:59.829059829%;*margin-left:59.72267685%}.row-fluid .offset6{margin-left:53.846153846%;*margin-left:53.739770867%}.row-fluid .offset6:first-child{margin-left:51.282051282%;*margin-left:51.175668303%}.row-fluid .offset5{margin-left:45.299145299%;*margin-left:45.19276232%}.row-fluid .offset5:first-child{margin-left:42.735042735%;*margin-left:42.628659756%}.row-fluid .offset4{margin-left:36.752136752%;*margin-left:36.645753773%}.row-fluid .offset4:first-child{margin-left:34.188034188%;*margin-left:34.081651209%}.row-fluid .offset3{margin-left:28.205128205%;*margin-left:28.098745226%}.row-fluid .offset3:first-child{margin-left:25.641025641%;*margin-left:25.534642662%}.row-fluid .offset2{margin-left:19.658119658%;*margin-left:19.551736679%}.row-fluid .offset2:first-child{margin-left:17.094017094%;*margin-left:16.987634115%}.row-fluid .offset1{margin-left:11.111111111%;*margin-left:11.004728132%}.row-fluid .offset1:first-child{margin-left:8.547008547%;*margin-left:8.440625568%}input,textarea,.uneditable-input{margin-left:0}.controls-row [class*="span"]+[class*="span"]{margin-left:30px}input.span12,textarea.span12,.uneditable-input.span12{width:1156px}input.span11,textarea.span11,.uneditable-input.span11{width:1056px}input.span10,textarea.span10,.uneditable-input.span10{width:956px}input.span9,textarea.span9,.uneditable-input.span9{width:856px}input.span8,textarea.span8,.uneditable-input.span8{width:756px}input.span7,textarea.span7,.uneditable-input.span7{width:656px}input.span6,textarea.span6,.uneditable-input.span6{width:556px}input.span5,textarea.span5,.uneditable-input.span5{width:456px}input.span4,textarea.span4,.uneditable-input.span4{width:356px}input.span3,textarea.span3,.uneditable-input.span3{width:256px}input.span2,textarea.span2,.uneditable-input.span2{width:156px}input.span1,textarea.span1,.uneditable-input.span1{width:56px}.thumbnails{margin-left:-30px}.thumbnails>li{margin-left:30px}.row-fluid .thumbnails{margin-left:0}}@media(min-width:768px) and (max-width:979px){.row{margin-left:-20px;*zoom:1}.row:before,.row:after{display:table;content:"";line-height:0}.row:after{clear:both}[class*="span"]{float:left;min-height:1px;margin-left:20px}.container,.navbar-static-top .container,.navbar-fixed-top .container,.navbar-fixed-bottom .container{width:97%}.span12{width:724px}.span11{width:662px}.span10{width:600px}.span9{width:538px}.span8{width:476px}.span7{width:414px}.span6{width:352px}.span5{width:290px}.span4{width:228px}.span3{width:166px}.span2{width:104px}.span1{width:42px}.offset12{margin-left:764px}.offset11{margin-left:702px}.offset10{margin-left:640px}.offset9{margin-left:578px}.offset8{margin-left:516px}.offset7{margin-left:454px}.offset6{margin-left:392px}.offset5{margin-left:330px}.offset4{margin-left:268px}.offset3{margin-left:206px}.offset2{margin-left:144px}.offset1{margin-left:82px}.row-fluid{width:100%;*zoom:1}.row-fluid:before,.row-fluid:after{display:table;content:"";line-height:0}.row-fluid:after{clear:both}.row-fluid [class*="span"]{display:block;width:100%;min-height:30px;-webkit-box-sizing:border-box;-moz-box-sizing:border-box;box-sizing:border-box;float:left;margin-left:2.762430939%;*margin-left:2.70923945%}.row-fluid [class*="span"]:first-child{margin-left:0}.row-fluid .controls-row [class*="span"]+[class*="span"]{margin-left:2.762430939%}.row-fluid .span12{width:100%;*width:99.946808511%}.row-fluid .span11{width:91.436464088%;*width:91.383272599%}.row-fluid .span10{width:82.872928177%;*width:82.819736687%}.row-fluid .span9{width:74.309392265%;*width:74.256200776%}.row-fluid .span8{width:65.745856354%;*width:65.692664864%}.row-fluid .span7{width:57.182320442%;*width:57.129128953%}.row-fluid .span6{width:48.61878453%;*width:48.565593041%}.row-fluid .span5{width:40.055248619%;*width:40.002057129%}.row-fluid .span4{width:31.491712707%;*width:31.438521218%}.row-fluid .span3{width:22.928176796%;*width:22.874985306%}.row-fluid .span2{width:14.364640884%;*width:14.311449395%}.row-fluid .span1{width:5.801104972%;*width:5.747913483%}.row-fluid .offset12{margin-left:105.524861878%;*margin-left:105.4184789%}.row-fluid .offset12:first-child{margin-left:102.762430939%;*margin-left:102.656047961%}.row-fluid .offset11{margin-left:96.961325967%;*margin-left:96.854942988%}.row-fluid .offset11:first-child{margin-left:94.198895028%;*margin-left:94.092512049%}.row-fluid .offset10{margin-left:88.397790055%;*margin-left:88.291407077%}.row-fluid .offset10:first-child{margin-left:85.635359116%;*margin-left:85.528976137%}.row-fluid .offset9{margin-left:79.834254144%;*margin-left:79.727871165%}.row-fluid .offset9:first-child{margin-left:77.071823204%;*margin-left:76.965440226%}.row-fluid .offset8{margin-left:71.270718232%;*margin-left:71.164335253%}.row-fluid .offset8:first-child{margin-left:68.508287293%;*margin-left:68.401904314%}.row-fluid .offset7{margin-left:62.70718232%;*margin-left:62.600799342%}.row-fluid .offset7:first-child{margin-left:59.944751381%;*margin-left:59.838368402%}.row-fluid .offset6{margin-left:54.143646409%;*margin-left:54.03726343%}.row-fluid .offset6:first-child{margin-left:51.38121547%;*margin-left:51.274832491%}.row-fluid .offset5{margin-left:45.580110497%;*margin-left:45.473727519%}.row-fluid .offset5:first-child{margin-left:42.817679558%;*margin-left:42.711296579%}.row-fluid .offset4{margin-left:37.016574586%;*margin-left:36.910191607%}.row-fluid .offset4:first-child{margin-left:34.254143646%;*margin-left:34.147760668%}.row-fluid .offset3{margin-left:28.453038674%;*margin-left:28.346655695%}.row-fluid .offset3:first-child{margin-left:25.690607735%;*margin-left:25.584224756%}.row-fluid .offset2{margin-left:19.889502762%;*margin-left:19.783119784%}.row-fluid .offset2:first-child{margin-left:17.127071823%;*margin-left:17.020688844%}.row-fluid .offset1{margin-left:11.325966851%;*margin-left:11.219583872%}.row-fluid .offset1:first-child{margin-left:8.563535912%;*margin-left:8.457152933%}input,textarea,.uneditable-input{margin-left:0}.controls-row [class*="span"]+[class*="span"]{margin-left:20px}input.span12,textarea.span12,.uneditable-input.span12{width:710px}input.span11,textarea.span11,.uneditable-input.span11{width:648px}input.span10,textarea.span10,.uneditable-input.span10{width:586px}input.span9,textarea.span9,.uneditable-input.span9{width:524px}input.span8,textarea.span8,.uneditable-input.span8{width:462px}input.span7,textarea.span7,.uneditable-input.span7{width:400px}input.span6,textarea.span6,.uneditable-input.span6{width:338px}input.span5,textarea.span5,.uneditable-input.span5{width:276px}input.span4,textarea.span4,.uneditable-input.span4{width:214px}input.span3,textarea.span3,.uneditable-input.span3{width:152px}input.span2,textarea.span2,.uneditable-input.span2{width:90px}input.span1,textarea.span1,.uneditable-input.span1{width:28px}}@media(max-width:767px){body{padding-left:20px;padding-right:20px}.navbar-fixed-top,.navbar-fixed-bottom,.navbar-static-top{margin-left:-20px;margin-right:-20px}.container-fluid{padding:0}.dl-horizontal dt{float:none;clear:none;width:auto;text-align:left}.dl-horizontal dd{margin-left:0}.container{width:auto}.row-fluid{width:100%}.row,.thumbnails{margin-left:0}.thumbnails>li{float:none;margin-left:0}[class*="span"],.uneditable-input[class*="span"],.row-fluid [class*="span"]{float:none;display:block;width:100%;margin-left:0;-webkit-box-sizing:border-box;-moz-box-sizing:border-box;box-sizing:border-box}.span12,.row-fluid .span12{width:100%;-webkit-box-sizing:border-box;-moz-box-sizing:border-box;box-sizing:border-box}.row-fluid [class*="offset"]:first-child{margin-left:0}.input-large,.input-xlarge,.input-xxlarge,input[class*="span"],select[class*="span"],textarea[class*="span"],.uneditable-input{display:block;width:100%;min-height:30px;-webkit-box-sizing:border-box;-moz-box-sizing:border-box;box-sizing:border-box}.input-prepend input,.input-append input,.input-prepend input[class*="span"],.input-append input[class*="span"]{display:inline-block;width:auto}.controls-row [class*="span"]+[class*="span"]{margin-left:0}.modal{position:fixed;top:20px;left:20px;right:20px;width:auto;margin:0}.modal.fade{top:-100px}.modal.fade.in{top:20px}}@media(max-width:480px){.nav-collapse{-webkit-transform:translate3d(0,0,0)}.page-header h1 small{display:block;line-height:20px}input[type="checkbox"],input[type="radio"]{border:1px solid #ccc}.form-horizontal .control-label{float:none;width:auto;padding-top:0;text-align:left}.form-horizontal .controls{margin-left:0}.form-horizontal .control-list{padding-top:0}.form-horizontal .form-actions{padding-left:10px;padding-right:10px}.media .pull-left,.media .pull-right{float:none;display:block;margin-bottom:10px}.media-object{margin-right:0;margin-left:0}.modal{top:10px;left:10px;right:10px}.modal-header .close{padding:10px;margin:-10px}.carousel-caption{position:static}}@media(max-width:979px){body{padding-top:0}.navbar-fixed-top,.navbar-fixed-bottom{position:static}.navbar-fixed-top{margin-bottom:20px}.navbar-fixed-bottom{margin-top:20px}.navbar-fixed-top .navbar-inner,.navbar-fixed-bottom .navbar-inner{padding:5px}.navbar .container{width:auto;padding:0}.navbar .brand{padding-left:10px;padding-right:10px;margin:0 0 0 -5px}.nav-collapse{clear:both}.nav-collapse .nav{float:none;margin:0 0 10px}.nav-collapse .nav>li{float:none}.nav-collapse .nav>li>a{margin-bottom:2px}.nav-collapse .nav>.divider-vertical{display:none}.nav-collapse .nav .nav-header{color:#fff;text-shadow:none}.nav-collapse .nav>li>a,.nav-collapse .dropdown-menu a{padding:9px 15px;font-weight:bold;color:#eee;-webkit-border-radius:3px;-moz-border-radius:3px;border-radius:3px}.nav-collapse .btn{padding:4px 10px 4px;font-weight:normal;-webkit-border-radius:4px;-moz-border-radius:4px;border-radius:4px}.nav-collapse .dropdown-menu li+li a{margin-bottom:2px}.nav-collapse .nav>li>a:hover,.nav-collapse .nav>li>a:focus,.nav-collapse .dropdown-menu a:hover,.nav-collapse .dropdown-menu a:focus{background-color:#007ea3}.navbar-inverse .nav-collapse .nav>li>a,.navbar-inverse .nav-collapse .dropdown-menu a{color:#6c757d}.navbar-inverse .nav-collapse .nav>li>a:hover,.navbar-inverse .nav-collapse .nav>li>a:focus,.navbar-inverse .nav-collapse .dropdown-menu a:hover,.navbar-inverse .nav-collapse .dropdown-menu a:focus{background-color:#111}.nav-collapse.in .btn-group{margin-top:5px;padding:0}.nav-collapse .dropdown-menu{position:static;top:auto;left:auto;float:none;display:none;max-width:none;margin:0 15px;padding:0;background-color:transparent;border:none;-webkit-border-radius:0;-moz-border-radius:0;border-radius:0;-webkit-box-shadow:none;-moz-box-shadow:none;box-shadow:none}.nav-collapse .open>.dropdown-menu{display:block}.nav-collapse .dropdown-menu:before,.nav-collapse .dropdown-menu:after{display:none}.nav-collapse .dropdown-menu .divider{display:none}.nav-collapse .nav>li>.dropdown-menu:before,.nav-collapse .nav>li>.dropdown-menu:after{display:none}.nav-collapse .navbar-form,.nav-collapse .navbar-search{float:none;padding:10px 15px;margin:10px 0;border-top:1px solid #007ea3;border-bottom:1px solid #007ea3;-webkit-box-shadow:inset 0 1px 0 rgba(255,255,255,.1),0 1px 0 rgba(255,255,255,.1);-moz-box-shadow:inset 0 1px 0 rgba(255,255,255,.1),0 1px 0 rgba(255,255,255,.1);box-shadow:inset 0 1px 0 rgba(255,255,255,.1),0 1px 0 rgba(255,255,255,.1)}.navbar-inverse .nav-collapse .navbar-form,.navbar-inverse .nav-collapse .navbar-search{border-top-color:#111;border-bottom-color:#111}.navbar .nav-collapse .nav.pull-right{float:none;margin-left:0}.nav-collapse,.nav-collapse.collapse{overflow:hidden;height:0}.navbar .btn-navbar{display:block}.navbar-static .navbar-inner{padding-left:10px;padding-right:10px}}@media(min-width:980px){.nav-collapse.collapse{height:auto!important;overflow:visible!important}}.fa,.fas,.far,.fal,.fad,.fab{-moz-osx-font-smoothing:grayscale;-webkit-font-smoothing:antialiased;display:inline-block;font-style:normal;font-variant:normal;text-rendering:auto;line-height:1}.fa-lg{font-size:1.333333333em;line-height:.75em;vertical-align:-.0667em}.fa-xs{font-size:.75em}.fa-sm{font-size:.875em}.fa-1x{font-size:1em}.fa-2x{font-size:2em}.fa-3x{font-size:3em}.fa-4x{font-size:4em}.fa-5x{font-size:5em}.fa-6x{font-size:6em}.fa-7x{font-size:7em}.fa-8x{font-size:8em}.fa-9x{font-size:9em}.fa-10x{font-size:10em}.fa-fw{text-align:center;width:1.25em}.fa-ul{list-style-type:none;margin-left:2.5em;padding-left:0}.fa-ul>li{position:relative}.fa-li{left:-2em;position:absolute;text-align:center;width:2em;line-height:inherit}.fa-border{border-radius:.1em;border:solid .08em #eee;padding:.2em .25em .15em}.fa-pull-left{float:left}.fa-pull-right{float:right}.fa.fa-pull-left,.fas.fa-pull-left,.far.fa-pull-left,.fal.fa-pull-left,.fab.fa-pull-left{margin-right:.3em}.fa.fa-pull-right,.fas.fa-pull-right,.far.fa-pull-right,.fal.fa-pull-right,.fab.fa-pull-right{margin-left:.3em}.fa-spin{animation:fa-spin 2s infinite linear}.fa-pulse{animation:fa-spin 1s infinite steps(8)}@keyframes fa-spin{0%{transform:rotate(0deg)}100%{transform:rotate(360deg)}}.fa-rotate-90{-ms-filter:"progid:DXImageTransform.Microsoft.BasicImage(rotation=1)";transform:rotate(90deg)}.fa-rotate-180{-ms-filter:"progid:DXImageTransform.Microsoft.BasicImage(rotation=2)";transform:rotate(180deg)}.fa-rotate-270{-ms-filter:"progid:DXImageTransform.Microsoft.BasicImage(rotation=3)";transform:rotate(270deg)}.fa-flip-horizontal{-ms-filter:"progid:DXImageTransform.Microsoft.BasicImage(rotation=0, mirror=1)";transform:scale(-1,1)}.fa-flip-vertical{-ms-filter:"progid:DXImageTransform.Microsoft.BasicImage(rotation=2, mirror=1)";transform:scale(1,-1)}.fa-flip-both,.fa-flip-horizontal.fa-flip-vertical{-ms-filter:"progid:DXImageTransform.Microsoft.BasicImage(rotation=2, mirror=1)";transform:scale(-1,-1)}:root .fa-rotate-90,:root .fa-rotate-180,:root .fa-rotate-270,:root .fa-flip-horizontal,:root .fa-flip-vertical,:root .fa-flip-both{filter:none}.fa-stack{display:inline-block;height:2em;line-height:2em;position:relative;vertical-align:middle;width:2em}.fa-stack-1x,.fa-stack-2x{left:0;position:absolute;text-align:center;width:100%}.fa-stack-1x{line-height:inherit}.fa-stack-2x{font-size:2em}.fa-inverse{color:#fff}.fa-500px:before{content:""}.fa-accessible-icon:before{content:""}.fa-accusoft:before{content:""}.fa-acquisitions-incorporated:before{content:""}.fa-ad:before{content:""}.fa-address-book:before{content:""}.fa-address-card:before{content:""}.fa-adjust:before{content:""}.fa-adn:before{content:""}.fa-adversal:before{content:""}.fa-affiliatetheme:before{content:""}.fa-air-freshener:before{content:""}.fa-airbnb:before{content:""}.fa-algolia:before{content:""}.fa-align-center:before{content:""}.fa-align-justify:before{content:""}.fa-align-left:before{content:""}.fa-align-right:before{content:""}.fa-alipay:before{content:""}.fa-allergies:before{content:""}.fa-amazon:before{content:""}.fa-amazon-pay:before{content:""}.fa-ambulance:before{content:""}.fa-american-sign-language-interpreting:before{content:""}.fa-amilia:before{content:""}.fa-anchor:before{content:""}.fa-android:before{content:""}.fa-angellist:before{content:""}.fa-angle-double-down:before{content:""}.fa-angle-double-left:before{content:""}.fa-angle-double-right:before{content:""}.fa-angle-double-up:before{content:""}.fa-angle-down:before{content:""}.fa-angle-left:before{content:""}.fa-angle-right:before{content:""}.fa-angle-up:before{content:""}.fa-angry:before{content:""}.fa-angrycreative:before{content:""}.fa-angular:before{content:""}.fa-ankh:before{content:""}.fa-app-store:before{content:""}.fa-app-store-ios:before{content:""}.fa-apper:before{content:""}.fa-apple:before{content:""}.fa-apple-alt:before{content:""}.fa-apple-pay:before{content:""}.fa-archive:before{content:""}.fa-archway:before{content:""}.fa-arrow-alt-circle-down:before{content:""}.fa-arrow-alt-circle-left:before{content:""}.fa-arrow-alt-circle-right:before{content:""}.fa-arrow-alt-circle-up:before{content:""}.fa-arrow-circle-down:before{content:""}.fa-arrow-circle-left:before{content:""}.fa-arrow-circle-right:before{content:""}.fa-arrow-circle-up:before{content:""}.fa-arrow-down:before{content:""}.fa-arrow-left:before{content:""}.fa-arrow-right:before{content:""}.fa-arrow-up:before{content:""}.fa-arrows-alt:before{content:""}.fa-arrows-alt-h:before{content:""}.fa-arrows-alt-v:before{content:""}.fa-artstation:before{content:""}.fa-assistive-listening-systems:before{content:""}.fa-asterisk:before{content:""}.fa-asymmetrik:before{content:""}.fa-at:before{content:""}.fa-atlas:before{content:""}.fa-atlassian:before{content:""}.fa-atom:before{content:""}.fa-audible:before{content:""}.fa-audio-description:before{content:""}.fa-autoprefixer:before{content:""}.fa-avianex:before{content:""}.fa-aviato:before{content:""}.fa-award:before{content:""}.fa-aws:before{content:""}.fa-baby:before{content:""}.fa-baby-carriage:before{content:""}.fa-backspace:before{content:""}.fa-backward:before{content:""}.fa-bacon:before{content:""}.fa-bacteria:before{content:""}.fa-bacterium:before{content:""}.fa-bahai:before{content:""}.fa-balance-scale:before{content:""}.fa-balance-scale-left:before{content:""}.fa-balance-scale-right:before{content:""}.fa-ban:before{content:""}.fa-band-aid:before{content:""}.fa-bandcamp:before{content:""}.fa-barcode:before{content:""}.fa-bars:before{content:""}.fa-baseball-ball:before{content:""}.fa-basketball-ball:before{content:""}.fa-bath:before{content:""}.fa-battery-empty:before{content:""}.fa-battery-full:before{content:""}.fa-battery-half:before{content:""}.fa-battery-quarter:before{content:""}.fa-battery-three-quarters:before{content:""}.fa-battle-net:before{content:""}.fa-bed:before{content:""}.fa-beer:before{content:""}.fa-behance:before{content:""}.fa-behance-square:before{content:""}.fa-bell:before{content:""}.fa-bell-slash:before{content:""}.fa-bezier-curve:before{content:""}.fa-bible:before{content:""}.fa-bicycle:before{content:""}.fa-biking:before{content:""}.fa-bimobject:before{content:""}.fa-binoculars:before{content:""}.fa-biohazard:before{content:""}.fa-birthday-cake:before{content:""}.fa-bitbucket:before{content:""}.fa-bitcoin:before{content:""}.fa-bity:before{content:""}.fa-black-tie:before{content:""}.fa-blackberry:before{content:""}.fa-blender:before{content:""}.fa-blender-phone:before{content:""}.fa-blind:before{content:""}.fa-blog:before{content:""}.fa-blogger:before{content:""}.fa-blogger-b:before{content:""}.fa-bluetooth:before{content:""}.fa-bluetooth-b:before{content:""}.fa-bold:before{content:""}.fa-bolt:before{content:""}.fa-bomb:before{content:""}.fa-bone:before{content:""}.fa-bong:before{content:""}.fa-book:before{content:""}.fa-book-dead:before{content:""}.fa-book-medical:before{content:""}.fa-book-open:before{content:""}.fa-book-reader:before{content:""}.fa-bookmark:before{content:""}.fa-bootstrap:before{content:""}.fa-border-all:before{content:""}.fa-border-none:before{content:""}.fa-border-style:before{content:""}.fa-bowling-ball:before{content:""}.fa-box:before{content:""}.fa-box-open:before{content:""}.fa-box-tissue:before{content:""}.fa-boxes:before{content:""}.fa-braille:before{content:""}.fa-brain:before{content:""}.fa-bread-slice:before{content:""}.fa-briefcase:before{content:""}.fa-briefcase-medical:before{content:""}.fa-broadcast-tower:before{content:""}.fa-broom:before{content:""}.fa-brush:before{content:""}.fa-btc:before{content:""}.fa-buffer:before{content:""}.fa-bug:before{content:""}.fa-building:before{content:""}.fa-bullhorn:before{content:""}.fa-bullseye:before{content:""}.fa-burn:before{content:""}.fa-buromobelexperte:before{content:""}.fa-bus:before{content:""}.fa-bus-alt:before{content:""}.fa-business-time:before{content:""}.fa-buy-n-large:before{content:""}.fa-buysellads:before{content:""}.fa-calculator:before{content:""}.fa-calendar:before{content:""}.fa-calendar-alt:before{content:""}.fa-calendar-check:before{content:""}.fa-calendar-day:before{content:""}.fa-calendar-minus:before{content:""}.fa-calendar-plus:before{content:""}.fa-calendar-times:before{content:""}.fa-calendar-week:before{content:""}.fa-camera:before{content:""}.fa-camera-retro:before{content:""}.fa-campground:before{content:""}.fa-canadian-maple-leaf:before{content:""}.fa-candy-cane:before{content:""}.fa-cannabis:before{content:""}.fa-capsules:before{content:""}.fa-car:before{content:""}.fa-car-alt:before{content:""}.fa-car-battery:before{content:""}.fa-car-crash:before{content:""}.fa-car-side:before{content:""}.fa-caravan:before{content:""}.fa-caret-down:before{content:""}.fa-caret-left:before{content:""}.fa-caret-right:before{content:""}.fa-caret-square-down:before{content:""}.fa-caret-square-left:before{content:""}.fa-caret-square-right:before{content:""}.fa-caret-square-up:before{content:""}.fa-caret-up:before{content:""}.fa-carrot:before{content:""}.fa-cart-arrow-down:before{content:""}.fa-cart-plus:before{content:""}.fa-cash-register:before{content:""}.fa-cat:before{content:""}.fa-cc-amazon-pay:before{content:""}.fa-cc-amex:before{content:""}.fa-cc-apple-pay:before{content:""}.fa-cc-diners-club:before{content:""}.fa-cc-discover:before{content:""}.fa-cc-jcb:before{content:""}.fa-cc-mastercard:before{content:""}.fa-cc-paypal:before{content:""}.fa-cc-stripe:before{content:""}.fa-cc-visa:before{content:""}.fa-centercode:before{content:""}.fa-centos:before{content:""}.fa-certificate:before{content:""}.fa-chair:before{content:""}.fa-chalkboard:before{content:""}.fa-chalkboard-teacher:before{content:""}.fa-charging-station:before{content:""}.fa-chart-area:before{content:""}.fa-chart-bar:before{content:""}.fa-chart-line:before{content:""}.fa-chart-pie:before{content:""}.fa-check:before{content:""}.fa-check-circle:before{content:""}.fa-check-double:before{content:""}.fa-check-square:before{content:""}.fa-cheese:before{content:""}.fa-chess:before{content:""}.fa-chess-bishop:before{content:""}.fa-chess-board:before{content:""}.fa-chess-king:before{content:""}.fa-chess-knight:before{content:""}.fa-chess-pawn:before{content:""}.fa-chess-queen:before{content:""}.fa-chess-rook:before{content:""}.fa-chevron-circle-down:before{content:""}.fa-chevron-circle-left:before{content:""}.fa-chevron-circle-right:before{content:""}.fa-chevron-circle-up:before{content:""}.fa-chevron-down:before{content:""}.fa-chevron-left:before{content:""}.fa-chevron-right:before{content:""}.fa-chevron-up:before{content:""}.fa-child:before{content:""}.fa-chrome:before{content:""}.fa-chromecast:before{content:""}.fa-church:before{content:""}.fa-circle:before{content:""}.fa-circle-notch:before{content:""}.fa-city:before{content:""}.fa-clinic-medical:before{content:""}.fa-clipboard:before{content:""}.fa-clipboard-check:before{content:""}.fa-clipboard-list:before{content:""}.fa-clock:before{content:""}.fa-clone:before{content:""}.fa-closed-captioning:before{content:""}.fa-cloud:before{content:""}.fa-cloud-download-alt:before{content:""}.fa-cloud-meatball:before{content:""}.fa-cloud-moon:before{content:""}.fa-cloud-moon-rain:before{content:""}.fa-cloud-rain:before{content:""}.fa-cloud-showers-heavy:before{content:""}.fa-cloud-sun:before{content:""}.fa-cloud-sun-rain:before{content:""}.fa-cloud-upload-alt:before{content:""}.fa-cloudflare:before{content:""}.fa-cloudscale:before{content:""}.fa-cloudsmith:before{content:""}.fa-cloudversify:before{content:""}.fa-cocktail:before{content:""}.fa-code:before{content:""}.fa-code-branch:before{content:""}.fa-codepen:before{content:""}.fa-codiepie:before{content:""}.fa-coffee:before{content:""}.fa-cog:before{content:""}.fa-cogs:before{content:""}.fa-coins:before{content:""}.fa-columns:before{content:""}.fa-comment:before{content:""}.fa-comment-alt:before{content:""}.fa-comment-dollar:before{content:""}.fa-comment-dots:before{content:""}.fa-comment-medical:before{content:""}.fa-comment-slash:before{content:""}.fa-comments:before{content:""}.fa-comments-dollar:before{content:""}.fa-compact-disc:before{content:""}.fa-compass:before{content:""}.fa-compress:before{content:""}.fa-compress-alt:before{content:""}.fa-compress-arrows-alt:before{content:""}.fa-concierge-bell:before{content:""}.fa-confluence:before{content:""}.fa-connectdevelop:before{content:""}.fa-contao:before{content:""}.fa-cookie:before{content:""}.fa-cookie-bite:before{content:""}.fa-copy:before{content:""}.fa-copyright:before{content:""}.fa-cotton-bureau:before{content:""}.fa-couch:before{content:""}.fa-cpanel:before{content:""}.fa-creative-commons:before{content:""}.fa-creative-commons-by:before{content:""}.fa-creative-commons-nc:before{content:""}.fa-creative-commons-nc-eu:before{content:""}.fa-creative-commons-nc-jp:before{content:""}.fa-creative-commons-nd:before{content:""}.fa-creative-commons-pd:before{content:""}.fa-creative-commons-pd-alt:before{content:""}.fa-creative-commons-remix:before{content:""}.fa-creative-commons-sa:before{content:""}.fa-creative-commons-sampling:before{content:""}.fa-creative-commons-sampling-plus:before{content:""}.fa-creative-commons-share:before{content:""}.fa-creative-commons-zero:before{content:""}.fa-credit-card:before{content:""}.fa-critical-role:before{content:""}.fa-crop:before{content:""}.fa-crop-alt:before{content:""}.fa-cross:before{content:""}.fa-crosshairs:before{content:""}.fa-crow:before{content:""}.fa-crown:before{content:""}.fa-crutch:before{content:""}.fa-css3:before{content:""}.fa-css3-alt:before{content:""}.fa-cube:before{content:""}.fa-cubes:before{content:""}.fa-cut:before{content:""}.fa-cuttlefish:before{content:""}.fa-d-and-d:before{content:""}.fa-d-and-d-beyond:before{content:""}.fa-dailymotion:before{content:""}.fa-dashcube:before{content:""}.fa-database:before{content:""}.fa-deaf:before{content:""}.fa-deezer:before{content:""}.fa-delicious:before{content:""}.fa-democrat:before{content:""}.fa-deploydog:before{content:""}.fa-deskpro:before{content:""}.fa-desktop:before{content:""}.fa-dev:before{content:""}.fa-deviantart:before{content:""}.fa-dharmachakra:before{content:""}.fa-dhl:before{content:""}.fa-diagnoses:before{content:""}.fa-diaspora:before{content:""}.fa-dice:before{content:""}.fa-dice-d20:before{content:""}.fa-dice-d6:before{content:""}.fa-dice-five:before{content:""}.fa-dice-four:before{content:""}.fa-dice-one:before{content:""}.fa-dice-six:before{content:""}.fa-dice-three:before{content:""}.fa-dice-two:before{content:""}.fa-digg:before{content:""}.fa-digital-ocean:before{content:""}.fa-digital-tachograph:before{content:""}.fa-directions:before{content:""}.fa-discord:before{content:""}.fa-discourse:before{content:""}.fa-disease:before{content:""}.fa-divide:before{content:""}.fa-dizzy:before{content:""}.fa-dna:before{content:""}.fa-dochub:before{content:""}.fa-docker:before{content:""}.fa-dog:before{content:""}.fa-dollar-sign:before{content:""}.fa-dolly:before{content:""}.fa-dolly-flatbed:before{content:""}.fa-donate:before{content:""}.fa-door-closed:before{content:""}.fa-door-open:before{content:""}.fa-dot-circle:before{content:""}.fa-dove:before{content:""}.fa-download:before{content:""}.fa-draft2digital:before{content:""}.fa-drafting-compass:before{content:""}.fa-dragon:before{content:""}.fa-draw-polygon:before{content:""}.fa-dribbble:before{content:""}.fa-dribbble-square:before{content:""}.fa-dropbox:before{content:""}.fa-drum:before{content:""}.fa-drum-steelpan:before{content:""}.fa-drumstick-bite:before{content:""}.fa-drupal:before{content:""}.fa-dumbbell:before{content:""}.fa-dumpster:before{content:""}.fa-dumpster-fire:before{content:""}.fa-dungeon:before{content:""}.fa-dyalog:before{content:""}.fa-earlybirds:before{content:""}.fa-ebay:before{content:""}.fa-edge:before{content:""}.fa-edge-legacy:before{content:""}.fa-edit:before{content:""}.fa-egg:before{content:""}.fa-eject:before{content:""}.fa-elementor:before{content:""}.fa-ellipsis-h:before{content:""}.fa-ellipsis-v:before{content:""}.fa-ello:before{content:""}.fa-ember:before{content:""}.fa-empire:before{content:""}.fa-envelope:before{content:""}.fa-envelope-open:before{content:""}.fa-envelope-open-text:before{content:""}.fa-envelope-square:before{content:""}.fa-envira:before{content:""}.fa-equals:before{content:""}.fa-eraser:before{content:""}.fa-erlang:before{content:""}.fa-ethereum:before{content:""}.fa-ethernet:before{content:""}.fa-etsy:before{content:""}.fa-euro-sign:before{content:""}.fa-evernote:before{content:""}.fa-exchange-alt:before{content:""}.fa-exclamation:before{content:""}.fa-exclamation-circle:before{content:""}.fa-exclamation-triangle:before{content:""}.fa-expand:before{content:""}.fa-expand-alt:before{content:""}.fa-expand-arrows-alt:before{content:""}.fa-expeditedssl:before{content:""}.fa-external-link-alt:before{content:""}.fa-external-link-square-alt:before{content:""}.fa-eye:before{content:""}.fa-eye-dropper:before{content:""}.fa-eye-slash:before{content:""}.fa-facebook:before{content:""}.fa-facebook-f:before{content:""}.fa-facebook-messenger:before{content:""}.fa-facebook-square:before{content:""}.fa-fan:before{content:""}.fa-fantasy-flight-games:before{content:""}.fa-fast-backward:before{content:""}.fa-fast-forward:before{content:""}.fa-faucet:before{content:""}.fa-fax:before{content:""}.fa-feather:before{content:""}.fa-feather-alt:before{content:""}.fa-fedex:before{content:""}.fa-fedora:before{content:""}.fa-female:before{content:""}.fa-fighter-jet:before{content:""}.fa-figma:before{content:""}.fa-file:before{content:""}.fa-file-alt:before{content:""}.fa-file-archive:before{content:""}.fa-file-audio:before{content:""}.fa-file-code:before{content:""}.fa-file-contract:before{content:""}.fa-file-csv:before{content:""}.fa-file-download:before{content:""}.fa-file-excel:before{content:""}.fa-file-export:before{content:""}.fa-file-image:before{content:""}.fa-file-import:before{content:""}.fa-file-invoice:before{content:""}.fa-file-invoice-dollar:before{content:""}.fa-file-medical:before{content:""}.fa-file-medical-alt:before{content:""}.fa-file-pdf:before{content:""}.fa-file-powerpoint:before{content:""}.fa-file-prescription:before{content:""}.fa-file-signature:before{content:""}.fa-file-upload:before{content:""}.fa-file-video:before{content:""}.fa-file-word:before{content:""}.fa-fill:before{content:""}.fa-fill-drip:before{content:""}.fa-film:before{content:""}.fa-filter:before{content:""}.fa-fingerprint:before{content:""}.fa-fire:before{content:""}.fa-fire-alt:before{content:""}.fa-fire-extinguisher:before{content:""}.fa-firefox:before{content:""}.fa-firefox-browser:before{content:""}.fa-first-aid:before{content:""}.fa-first-order:before{content:""}.fa-first-order-alt:before{content:""}.fa-firstdraft:before{content:""}.fa-fish:before{content:""}.fa-fist-raised:before{content:""}.fa-flag:before{content:""}.fa-flag-checkered:before{content:""}.fa-flag-usa:before{content:""}.fa-flask:before{content:""}.fa-flickr:before{content:""}.fa-flipboard:before{content:""}.fa-flushed:before{content:""}.fa-fly:before{content:""}.fa-folder:before{content:""}.fa-folder-minus:before{content:""}.fa-folder-open:before{content:""}.fa-folder-plus:before{content:""}.fa-font:before{content:""}.fa-font-awesome:before{content:""}.fa-font-awesome-alt:before{content:""}.fa-font-awesome-flag:before{content:""}.fa-font-awesome-logo-full:before{content:""}.fa-fonticons:before{content:""}.fa-fonticons-fi:before{content:""}.fa-football-ball:before{content:""}.fa-fort-awesome:before{content:""}.fa-fort-awesome-alt:before{content:""}.fa-forumbee:before{content:""}.fa-forward:before{content:""}.fa-foursquare:before{content:""}.fa-free-code-camp:before{content:""}.fa-freebsd:before{content:""}.fa-frog:before{content:""}.fa-frown:before{content:""}.fa-frown-open:before{content:""}.fa-fulcrum:before{content:""}.fa-funnel-dollar:before{content:""}.fa-futbol:before{content:""}.fa-galactic-republic:before{content:""}.fa-galactic-senate:before{content:""}.fa-gamepad:before{content:""}.fa-gas-pump:before{content:""}.fa-gavel:before{content:""}.fa-gem:before{content:""}.fa-genderless:before{content:""}.fa-get-pocket:before{content:""}.fa-gg:before{content:""}.fa-gg-circle:before{content:""}.fa-ghost:before{content:""}.fa-gift:before{content:""}.fa-gifts:before{content:""}.fa-git:before{content:""}.fa-git-alt:before{content:""}.fa-git-square:before{content:""}.fa-github:before{content:""}.fa-github-alt:before{content:""}.fa-github-square:before{content:""}.fa-gitkraken:before{content:""}.fa-gitlab:before{content:""}.fa-gitter:before{content:""}.fa-glass-cheers:before{content:""}.fa-glass-martini:before{content:""}.fa-glass-martini-alt:before{content:""}.fa-glass-whiskey:before{content:""}.fa-glasses:before{content:""}.fa-glide:before{content:""}.fa-glide-g:before{content:""}.fa-globe:before{content:""}.fa-globe-africa:before{content:""}.fa-globe-americas:before{content:""}.fa-globe-asia:before{content:""}.fa-globe-europe:before{content:""}.fa-gofore:before{content:""}.fa-golf-ball:before{content:""}.fa-goodreads:before{content:""}.fa-goodreads-g:before{content:""}.fa-google:before{content:""}.fa-google-drive:before{content:""}.fa-google-pay:before{content:""}.fa-google-play:before{content:""}.fa-google-plus:before{content:""}.fa-google-plus-g:before{content:""}.fa-google-plus-square:before{content:""}.fa-google-wallet:before{content:""}.fa-gopuram:before{content:""}.fa-graduation-cap:before{content:""}.fa-gratipay:before{content:""}.fa-grav:before{content:""}.fa-greater-than:before{content:""}.fa-greater-than-equal:before{content:""}.fa-grimace:before{content:""}.fa-grin:before{content:""}.fa-grin-alt:before{content:""}.fa-grin-beam:before{content:""}.fa-grin-beam-sweat:before{content:""}.fa-grin-hearts:before{content:""}.fa-grin-squint:before{content:""}.fa-grin-squint-tears:before{content:""}.fa-grin-stars:before{content:""}.fa-grin-tears:before{content:""}.fa-grin-tongue:before{content:""}.fa-grin-tongue-squint:before{content:""}.fa-grin-tongue-wink:before{content:""}.fa-grin-wink:before{content:""}.fa-grip-horizontal:before{content:""}.fa-grip-lines:before{content:""}.fa-grip-lines-vertical:before{content:""}.fa-grip-vertical:before{content:""}.fa-gripfire:before{content:""}.fa-grunt:before{content:""}.fa-guilded:before{content:""}.fa-guitar:before{content:""}.fa-gulp:before{content:""}.fa-h-square:before{content:""}.fa-hacker-news:before{content:""}.fa-hacker-news-square:before{content:""}.fa-hackerrank:before{content:""}.fa-hamburger:before{content:""}.fa-hammer:before{content:""}.fa-hamsa:before{content:""}.fa-hand-holding:before{content:""}.fa-hand-holding-heart:before{content:""}.fa-hand-holding-medical:before{content:""}.fa-hand-holding-usd:before{content:""}.fa-hand-holding-water:before{content:""}.fa-hand-lizard:before{content:""}.fa-hand-middle-finger:before{content:""}.fa-hand-paper:before{content:""}.fa-hand-peace:before{content:""}.fa-hand-point-down:before{content:""}.fa-hand-point-left:before{content:""}.fa-hand-point-right:before{content:""}.fa-hand-point-up:before{content:""}.fa-hand-pointer:before{content:""}.fa-hand-rock:before{content:""}.fa-hand-scissors:before{content:""}.fa-hand-sparkles:before{content:""}.fa-hand-spock:before{content:""}.fa-hands:before{content:""}.fa-hands-helping:before{content:""}.fa-hands-wash:before{content:""}.fa-handshake:before{content:""}.fa-handshake-alt-slash:before{content:""}.fa-handshake-slash:before{content:""}.fa-hanukiah:before{content:""}.fa-hard-hat:before{content:""}.fa-hashtag:before{content:""}.fa-hat-cowboy:before{content:""}.fa-hat-cowboy-side:before{content:""}.fa-hat-wizard:before{content:""}.fa-hdd:before{content:""}.fa-head-side-cough:before{content:""}.fa-head-side-cough-slash:before{content:""}.fa-head-side-mask:before{content:""}.fa-head-side-virus:before{content:""}.fa-heading:before{content:""}.fa-headphones:before{content:""}.fa-headphones-alt:before{content:""}.fa-headset:before{content:""}.fa-heart:before{content:""}.fa-heart-broken:before{content:""}.fa-heartbeat:before{content:""}.fa-helicopter:before{content:""}.fa-highlighter:before{content:""}.fa-hiking:before{content:""}.fa-hippo:before{content:""}.fa-hips:before{content:""}.fa-hire-a-helper:before{content:""}.fa-history:before{content:""}.fa-hive:before{content:""}.fa-hockey-puck:before{content:""}.fa-holly-berry:before{content:""}.fa-home:before{content:""}.fa-hooli:before{content:""}.fa-hornbill:before{content:""}.fa-horse:before{content:""}.fa-horse-head:before{content:""}.fa-hospital:before{content:""}.fa-hospital-alt:before{content:""}.fa-hospital-symbol:before{content:""}.fa-hospital-user:before{content:""}.fa-hot-tub:before{content:""}.fa-hotdog:before{content:""}.fa-hotel:before{content:""}.fa-hotjar:before{content:""}.fa-hourglass:before{content:""}.fa-hourglass-end:before{content:""}.fa-hourglass-half:before{content:""}.fa-hourglass-start:before{content:""}.fa-house-damage:before{content:""}.fa-house-user:before{content:""}.fa-houzz:before{content:""}.fa-hryvnia:before{content:""}.fa-html5:before{content:""}.fa-hubspot:before{content:""}.fa-i-cursor:before{content:""}.fa-ice-cream:before{content:""}.fa-icicles:before{content:""}.fa-icons:before{content:""}.fa-id-badge:before{content:""}.fa-id-card:before{content:""}.fa-id-card-alt:before{content:""}.fa-ideal:before{content:""}.fa-igloo:before{content:""}.fa-image:before{content:""}.fa-images:before{content:""}.fa-imdb:before{content:""}.fa-inbox:before{content:""}.fa-indent:before{content:""}.fa-industry:before{content:""}.fa-infinity:before{content:""}.fa-info:before{content:""}.fa-info-circle:before{content:""}.fa-innosoft:before{content:""}.fa-instagram:before{content:""}.fa-instagram-square:before{content:""}.fa-instalod:before{content:""}.fa-intercom:before{content:""}.fa-internet-explorer:before{content:""}.fa-invision:before{content:""}.fa-ioxhost:before{content:""}.fa-italic:before{content:""}.fa-itch-io:before{content:""}.fa-itunes:before{content:""}.fa-itunes-note:before{content:""}.fa-java:before{content:""}.fa-jedi:before{content:""}.fa-jedi-order:before{content:""}.fa-jenkins:before{content:""}.fa-jira:before{content:""}.fa-joget:before{content:""}.fa-joint:before{content:""}.fa-joomla:before{content:""}.fa-journal-whills:before{content:""}.fa-js:before{content:""}.fa-js-square:before{content:""}.fa-jsfiddle:before{content:""}.fa-kaaba:before{content:""}.fa-kaggle:before{content:""}.fa-key:before{content:""}.fa-keybase:before{content:""}.fa-keyboard:before{content:""}.fa-keycdn:before{content:""}.fa-khanda:before{content:""}.fa-kickstarter:before{content:""}.fa-kickstarter-k:before{content:""}.fa-kiss:before{content:""}.fa-kiss-beam:before{content:""}.fa-kiss-wink-heart:before{content:""}.fa-kiwi-bird:before{content:""}.fa-korvue:before{content:""}.fa-landmark:before{content:""}.fa-language:before{content:""}.fa-laptop:before{content:""}.fa-laptop-code:before{content:""}.fa-laptop-house:before{content:""}.fa-laptop-medical:before{content:""}.fa-laravel:before{content:""}.fa-lastfm:before{content:""}.fa-lastfm-square:before{content:""}.fa-laugh:before{content:""}.fa-laugh-beam:before{content:""}.fa-laugh-squint:before{content:""}.fa-laugh-wink:before{content:""}.fa-layer-group:before{content:""}.fa-leaf:before{content:""}.fa-leanpub:before{content:""}.fa-lemon:before{content:""}.fa-less:before{content:""}.fa-less-than:before{content:""}.fa-less-than-equal:before{content:""}.fa-level-down-alt:before{content:""}.fa-level-up-alt:before{content:""}.fa-life-ring:before{content:""}.fa-lightbulb:before{content:""}.fa-line:before{content:""}.fa-link:before{content:""}.fa-linkedin:before{content:""}.fa-linkedin-in:before{content:""}.fa-linode:before{content:""}.fa-linux:before{content:""}.fa-lira-sign:before{content:""}.fa-list:before{content:""}.fa-list-alt:before{content:""}.fa-list-ol:before{content:""}.fa-list-ul:before{content:""}.fa-location-arrow:before{content:""}.fa-lock:before{content:""}.fa-lock-open:before{content:""}.fa-long-arrow-alt-down:before{content:""}.fa-long-arrow-alt-left:before{content:""}.fa-long-arrow-alt-right:before{content:""}.fa-long-arrow-alt-up:before{content:""}.fa-low-vision:before{content:""}.fa-luggage-cart:before{content:""}.fa-lungs:before{content:""}.fa-lungs-virus:before{content:""}.fa-lyft:before{content:""}.fa-magento:before{content:""}.fa-magic:before{content:""}.fa-magnet:before{content:""}.fa-mail-bulk:before{content:""}.fa-mailchimp:before{content:""}.fa-male:before{content:""}.fa-mandalorian:before{content:""}.fa-map:before{content:""}.fa-map-marked:before{content:""}.fa-map-marked-alt:before{content:""}.fa-map-marker:before{content:""}.fa-map-marker-alt:before{content:""}.fa-map-pin:before{content:""}.fa-map-signs:before{content:""}.fa-markdown:before{content:""}.fa-marker:before{content:""}.fa-mars:before{content:""}.fa-mars-double:before{content:""}.fa-mars-stroke:before{content:""}.fa-mars-stroke-h:before{content:""}.fa-mars-stroke-v:before{content:""}.fa-mask:before{content:""}.fa-mastodon:before{content:""}.fa-maxcdn:before{content:""}.fa-mdb:before{content:""}.fa-medal:before{content:""}.fa-medapps:before{content:""}.fa-medium:before{content:""}.fa-medium-m:before{content:""}.fa-medkit:before{content:""}.fa-medrt:before{content:""}.fa-meetup:before{content:""}.fa-megaport:before{content:""}.fa-meh:before{content:""}.fa-meh-blank:before{content:""}.fa-meh-rolling-eyes:before{content:""}.fa-memory:before{content:""}.fa-mendeley:before{content:""}.fa-menorah:before{content:""}.fa-mercury:before{content:""}.fa-meteor:before{content:""}.fa-microblog:before{content:""}.fa-microchip:before{content:""}.fa-microphone:before{content:""}.fa-microphone-alt:before{content:""}.fa-microphone-alt-slash:before{content:""}.fa-microphone-slash:before{content:""}.fa-microscope:before{content:""}.fa-microsoft:before{content:""}.fa-minus:before{content:""}.fa-minus-circle:before{content:""}.fa-minus-square:before{content:""}.fa-mitten:before{content:""}.fa-mix:before{content:""}.fa-mixcloud:before{content:""}.fa-mixer:before{content:""}.fa-mizuni:before{content:""}.fa-mobile:before{content:""}.fa-mobile-alt:before{content:""}.fa-modx:before{content:""}.fa-monero:before{content:""}.fa-money-bill:before{content:""}.fa-money-bill-alt:before{content:""}.fa-money-bill-wave:before{content:""}.fa-money-bill-wave-alt:before{content:""}.fa-money-check:before{content:""}.fa-money-check-alt:before{content:""}.fa-monument:before{content:""}.fa-moon:before{content:""}.fa-mortar-pestle:before{content:""}.fa-mosque:before{content:""}.fa-motorcycle:before{content:""}.fa-mountain:before{content:""}.fa-mouse:before{content:""}.fa-mouse-pointer:before{content:""}.fa-mug-hot:before{content:""}.fa-music:before{content:""}.fa-napster:before{content:""}.fa-neos:before{content:""}.fa-network-wired:before{content:""}.fa-neuter:before{content:""}.fa-newspaper:before{content:""}.fa-nimblr:before{content:""}.fa-node:before{content:""}.fa-node-js:before{content:""}.fa-not-equal:before{content:""}.fa-notes-medical:before{content:""}.fa-npm:before{content:""}.fa-ns8:before{content:""}.fa-nutritionix:before{content:""}.fa-object-group:before{content:""}.fa-object-ungroup:before{content:""}.fa-octopus-deploy:before{content:""}.fa-odnoklassniki:before{content:""}.fa-odnoklassniki-square:before{content:""}.fa-oil-can:before{content:""}.fa-old-republic:before{content:""}.fa-om:before{content:""}.fa-opencart:before{content:""}.fa-openid:before{content:""}.fa-opera:before{content:""}.fa-optin-monster:before{content:""}.fa-orcid:before{content:""}.fa-osi:before{content:""}.fa-otter:before{content:""}.fa-outdent:before{content:""}.fa-page4:before{content:""}.fa-pagelines:before{content:""}.fa-pager:before{content:""}.fa-paint-brush:before{content:""}.fa-paint-roller:before{content:""}.fa-palette:before{content:""}.fa-palfed:before{content:""}.fa-pallet:before{content:""}.fa-paper-plane:before{content:""}.fa-paperclip:before{content:""}.fa-parachute-box:before{content:""}.fa-paragraph:before{content:""}.fa-parking:before{content:""}.fa-passport:before{content:""}.fa-pastafarianism:before{content:""}.fa-paste:before{content:""}.fa-patreon:before{content:""}.fa-pause:before{content:""}.fa-pause-circle:before{content:""}.fa-paw:before{content:""}.fa-paypal:before{content:""}.fa-peace:before{content:""}.fa-pen:before{content:""}.fa-pen-alt:before{content:""}.fa-pen-fancy:before{content:""}.fa-pen-nib:before{content:""}.fa-pen-square:before{content:""}.fa-pencil-alt:before{content:""}.fa-pencil-ruler:before{content:""}.fa-penny-arcade:before{content:""}.fa-people-arrows:before{content:""}.fa-people-carry:before{content:""}.fa-pepper-hot:before{content:""}.fa-perbyte:before{content:""}.fa-percent:before{content:""}.fa-percentage:before{content:""}.fa-periscope:before{content:""}.fa-person-booth:before{content:""}.fa-phabricator:before{content:""}.fa-phoenix-framework:before{content:""}.fa-phoenix-squadron:before{content:""}.fa-phone:before{content:""}.fa-phone-alt:before{content:""}.fa-phone-slash:before{content:""}.fa-phone-square:before{content:""}.fa-phone-square-alt:before{content:""}.fa-phone-volume:before{content:""}.fa-photo-video:before{content:""}.fa-php:before{content:""}.fa-pied-piper:before{content:""}.fa-pied-piper-alt:before{content:""}.fa-pied-piper-hat:before{content:""}.fa-pied-piper-pp:before{content:""}.fa-pied-piper-square:before{content:""}.fa-piggy-bank:before{content:""}.fa-pills:before{content:""}.fa-pinterest:before{content:""}.fa-pinterest-p:before{content:""}.fa-pinterest-square:before{content:""}.fa-pizza-slice:before{content:""}.fa-place-of-worship:before{content:""}.fa-plane:before{content:""}.fa-plane-arrival:before{content:""}.fa-plane-departure:before{content:""}.fa-plane-slash:before{content:""}.fa-play:before{content:""}.fa-play-circle:before{content:""}.fa-playstation:before{content:""}.fa-plug:before{content:""}.fa-plus:before{content:""}.fa-plus-circle:before{content:""}.fa-plus-square:before{content:""}.fa-podcast:before{content:""}.fa-poll:before{content:""}.fa-poll-h:before{content:""}.fa-poo:before{content:""}.fa-poo-storm:before{content:""}.fa-poop:before{content:""}.fa-portrait:before{content:""}.fa-pound-sign:before{content:""}.fa-power-off:before{content:""}.fa-pray:before{content:""}.fa-praying-hands:before{content:""}.fa-prescription:before{content:""}.fa-prescription-bottle:before{content:""}.fa-prescription-bottle-alt:before{content:""}.fa-print:before{content:""}.fa-procedures:before{content:""}.fa-product-hunt:before{content:""}.fa-project-diagram:before{content:""}.fa-pump-medical:before{content:""}.fa-pump-soap:before{content:""}.fa-pushed:before{content:""}.fa-puzzle-piece:before{content:""}.fa-python:before{content:""}.fa-qq:before{content:""}.fa-qrcode:before{content:""}.fa-question:before{content:""}.fa-question-circle:before{content:""}.fa-quidditch:before{content:""}.fa-quinscape:before{content:""}.fa-quora:before{content:""}.fa-quote-left:before{content:""}.fa-quote-right:before{content:""}.fa-quran:before{content:""}.fa-r-project:before{content:""}.fa-radiation:before{content:""}.fa-radiation-alt:before{content:""}.fa-rainbow:before{content:""}.fa-random:before{content:""}.fa-raspberry-pi:before{content:""}.fa-ravelry:before{content:""}.fa-react:before{content:""}.fa-reacteurope:before{content:""}.fa-readme:before{content:""}.fa-rebel:before{content:""}.fa-receipt:before{content:""}.fa-record-vinyl:before{content:""}.fa-recycle:before{content:""}.fa-red-river:before{content:""}.fa-reddit:before{content:""}.fa-reddit-alien:before{content:""}.fa-reddit-square:before{content:""}.fa-redhat:before{content:""}.fa-redo:before{content:""}.fa-redo-alt:before{content:""}.fa-registered:before{content:""}.fa-remove-format:before{content:""}.fa-renren:before{content:""}.fa-reply:before{content:""}.fa-reply-all:before{content:""}.fa-replyd:before{content:""}.fa-republican:before{content:""}.fa-researchgate:before{content:""}.fa-resolving:before{content:""}.fa-restroom:before{content:""}.fa-retweet:before{content:""}.fa-rev:before{content:""}.fa-ribbon:before{content:""}.fa-ring:before{content:""}.fa-road:before{content:""}.fa-robot:before{content:""}.fa-rocket:before{content:""}.fa-rocketchat:before{content:""}.fa-rockrms:before{content:""}.fa-route:before{content:""}.fa-rss:before{content:""}.fa-rss-square:before{content:""}.fa-ruble-sign:before{content:""}.fa-ruler:before{content:""}.fa-ruler-combined:before{content:""}.fa-ruler-horizontal:before{content:""}.fa-ruler-vertical:before{content:""}.fa-running:before{content:""}.fa-rupee-sign:before{content:""}.fa-rust:before{content:""}.fa-sad-cry:before{content:""}.fa-sad-tear:before{content:""}.fa-safari:before{content:""}.fa-salesforce:before{content:""}.fa-sass:before{content:""}.fa-satellite:before{content:""}.fa-satellite-dish:before{content:""}.fa-save:before{content:""}.fa-schlix:before{content:""}.fa-school:before{content:""}.fa-screwdriver:before{content:""}.fa-scribd:before{content:""}.fa-scroll:before{content:""}.fa-sd-card:before{content:""}.fa-search:before{content:""}.fa-search-dollar:before{content:""}.fa-search-location:before{content:""}.fa-search-minus:before{content:""}.fa-search-plus:before{content:""}.fa-searchengin:before{content:""}.fa-seedling:before{content:""}.fa-sellcast:before{content:""}.fa-sellsy:before{content:""}.fa-server:before{content:""}.fa-servicestack:before{content:""}.fa-shapes:before{content:""}.fa-share:before{content:""}.fa-share-alt:before{content:""}.fa-share-alt-square:before{content:""}.fa-share-square:before{content:""}.fa-shekel-sign:before{content:""}.fa-shield-alt:before{content:""}.fa-shield-virus:before{content:""}.fa-ship:before{content:""}.fa-shipping-fast:before{content:""}.fa-shirtsinbulk:before{content:""}.fa-shoe-prints:before{content:""}.fa-shopify:before{content:""}.fa-shopping-bag:before{content:""}.fa-shopping-basket:before{content:""}.fa-shopping-cart:before{content:""}.fa-shopware:before{content:""}.fa-shower:before{content:""}.fa-shuttle-van:before{content:""}.fa-sign:before{content:""}.fa-sign-in-alt:before{content:""}.fa-sign-language:before{content:""}.fa-sign-out-alt:before{content:""}.fa-signal:before{content:""}.fa-signature:before{content:""}.fa-sim-card:before{content:""}.fa-simplybuilt:before{content:""}.fa-sink:before{content:""}.fa-sistrix:before{content:""}.fa-sitemap:before{content:""}.fa-sith:before{content:""}.fa-skating:before{content:""}.fa-sketch:before{content:""}.fa-skiing:before{content:""}.fa-skiing-nordic:before{content:""}.fa-skull:before{content:""}.fa-skull-crossbones:before{content:""}.fa-skyatlas:before{content:""}.fa-skype:before{content:""}.fa-slack:before{content:""}.fa-slack-hash:before{content:""}.fa-slash:before{content:""}.fa-sleigh:before{content:""}.fa-sliders-h:before{content:""}.fa-slideshare:before{content:""}.fa-smile:before{content:""}.fa-smile-beam:before{content:""}.fa-smile-wink:before{content:""}.fa-smog:before{content:""}.fa-smoking:before{content:""}.fa-smoking-ban:before{content:""}.fa-sms:before{content:""}.fa-snapchat:before{content:""}.fa-snapchat-ghost:before{content:""}.fa-snapchat-square:before{content:""}.fa-snowboarding:before{content:""}.fa-snowflake:before{content:""}.fa-snowman:before{content:""}.fa-snowplow:before{content:""}.fa-soap:before{content:""}.fa-socks:before{content:""}.fa-solar-panel:before{content:""}.fa-sort:before{content:""}.fa-sort-alpha-down:before{content:""}.fa-sort-alpha-down-alt:before{content:""}.fa-sort-alpha-up:before{content:""}.fa-sort-alpha-up-alt:before{content:""}.fa-sort-amount-down:before{content:""}.fa-sort-amount-down-alt:before{content:""}.fa-sort-amount-up:before{content:""}.fa-sort-amount-up-alt:before{content:""}.fa-sort-down:before{content:""}.fa-sort-numeric-down:before{content:""}.fa-sort-numeric-down-alt:before{content:""}.fa-sort-numeric-up:before{content:""}.fa-sort-numeric-up-alt:before{content:""}.fa-sort-up:before{content:""}.fa-soundcloud:before{content:""}.fa-sourcetree:before{content:""}.fa-spa:before{content:""}.fa-space-shuttle:before{content:""}.fa-speakap:before{content:""}.fa-speaker-deck:before{content:""}.fa-spell-check:before{content:""}.fa-spider:before{content:""}.fa-spinner:before{content:""}.fa-splotch:before{content:""}.fa-spotify:before{content:""}.fa-spray-can:before{content:""}.fa-square:before{content:""}.fa-square-full:before{content:""}.fa-square-root-alt:before{content:""}.fa-squarespace:before{content:""}.fa-stack-exchange:before{content:""}.fa-stack-overflow:before{content:""}.fa-stackpath:before{content:""}.fa-stamp:before{content:""}.fa-star:before{content:""}.fa-star-and-crescent:before{content:""}.fa-star-half:before{content:""}.fa-star-half-alt:before{content:""}.fa-star-of-david:before{content:""}.fa-star-of-life:before{content:""}.fa-staylinked:before{content:""}.fa-steam:before{content:""}.fa-steam-square:before{content:""}.fa-steam-symbol:before{content:""}.fa-step-backward:before{content:""}.fa-step-forward:before{content:""}.fa-stethoscope:before{content:""}.fa-sticker-mule:before{content:""}.fa-sticky-note:before{content:""}.fa-stop:before{content:""}.fa-stop-circle:before{content:""}.fa-stopwatch:before{content:""}.fa-stopwatch-20:before{content:""}.fa-store:before{content:""}.fa-store-alt:before{content:""}.fa-store-alt-slash:before{content:""}.fa-store-slash:before{content:""}.fa-strava:before{content:""}.fa-stream:before{content:""}.fa-street-view:before{content:""}.fa-strikethrough:before{content:""}.fa-stripe:before{content:""}.fa-stripe-s:before{content:""}.fa-stroopwafel:before{content:""}.fa-studiovinari:before{content:""}.fa-stumbleupon:before{content:""}.fa-stumbleupon-circle:before{content:""}.fa-subscript:before{content:""}.fa-subway:before{content:""}.fa-suitcase:before{content:""}.fa-suitcase-rolling:before{content:""}.fa-sun:before{content:""}.fa-superpowers:before{content:""}.fa-superscript:before{content:""}.fa-supple:before{content:""}.fa-surprise:before{content:""}.fa-suse:before{content:""}.fa-swatchbook:before{content:""}.fa-swift:before{content:""}.fa-swimmer:before{content:""}.fa-swimming-pool:before{content:""}.fa-symfony:before{content:""}.fa-synagogue:before{content:""}.fa-sync:before{content:""}.fa-sync-alt:before{content:""}.fa-syringe:before{content:""}.fa-table:before{content:""}.fa-table-tennis:before{content:""}.fa-tablet:before{content:""}.fa-tablet-alt:before{content:""}.fa-tablets:before{content:""}.fa-tachometer-alt:before{content:""}.fa-tag:before{content:""}.fa-tags:before{content:""}.fa-tape:before{content:""}.fa-tasks:before{content:""}.fa-taxi:before{content:""}.fa-teamspeak:before{content:""}.fa-teeth:before{content:""}.fa-teeth-open:before{content:""}.fa-telegram:before{content:""}.fa-telegram-plane:before{content:""}.fa-temperature-high:before{content:""}.fa-temperature-low:before{content:""}.fa-tencent-weibo:before{content:""}.fa-tenge:before{content:""}.fa-terminal:before{content:""}.fa-text-height:before{content:""}.fa-text-width:before{content:""}.fa-th:before{content:""}.fa-th-large:before{content:""}.fa-th-list:before{content:""}.fa-the-red-yeti:before{content:""}.fa-theater-masks:before{content:""}.fa-themeco:before{content:""}.fa-themeisle:before{content:""}.fa-thermometer:before{content:""}.fa-thermometer-empty:before{content:""}.fa-thermometer-full:before{content:""}.fa-thermometer-half:before{content:""}.fa-thermometer-quarter:before{content:""}.fa-thermometer-three-quarters:before{content:""}.fa-think-peaks:before{content:""}.fa-thumbs-down:before{content:""}.fa-thumbs-up:before{content:""}.fa-thumbtack:before{content:""}.fa-ticket-alt:before{content:""}.fa-tiktok:before{content:""}.fa-times:before{content:""}.fa-times-circle:before{content:""}.fa-tint:before{content:""}.fa-tint-slash:before{content:""}.fa-tired:before{content:""}.fa-toggle-off:before{content:""}.fa-toggle-on:before{content:""}.fa-toilet:before{content:""}.fa-toilet-paper:before{content:""}.fa-toilet-paper-slash:before{content:""}.fa-toolbox:before{content:""}.fa-tools:before{content:""}.fa-tooth:before{content:""}.fa-torah:before{content:""}.fa-torii-gate:before{content:""}.fa-tractor:before{content:""}.fa-trade-federation:before{content:""}.fa-trademark:before{content:""}.fa-traffic-light:before{content:""}.fa-trailer:before{content:""}.fa-train:before{content:""}.fa-tram:before{content:""}.fa-transgender:before{content:""}.fa-transgender-alt:before{content:""}.fa-trash:before{content:""}.fa-trash-alt:before{content:""}.fa-trash-restore:before{content:""}.fa-trash-restore-alt:before{content:""}.fa-tree:before{content:""}.fa-trello:before{content:""}.fa-tripadvisor:before{content:""}.fa-trophy:before{content:""}.fa-truck:before{content:""}.fa-truck-loading:before{content:""}.fa-truck-monster:before{content:""}.fa-truck-moving:before{content:""}.fa-truck-pickup:before{content:""}.fa-tshirt:before{content:""}.fa-tty:before{content:""}.fa-tumblr:before{content:""}.fa-tumblr-square:before{content:""}.fa-tv:before{content:""}.fa-twitch:before{content:""}.fa-twitter:before{content:""}.fa-twitter-square:before{content:""}.fa-typo3:before{content:""}.fa-uber:before{content:""}.fa-ubuntu:before{content:""}.fa-uikit:before{content:""}.fa-umbraco:before{content:""}.fa-umbrella:before{content:""}.fa-umbrella-beach:before{content:""}.fa-uncharted:before{content:""}.fa-underline:before{content:""}.fa-undo:before{content:""}.fa-undo-alt:before{content:""}.fa-uniregistry:before{content:""}.fa-unity:before{content:""}.fa-universal-access:before{content:""}.fa-university:before{content:""}.fa-unlink:before{content:""}.fa-unlock:before{content:""}.fa-unlock-alt:before{content:""}.fa-unsplash:before{content:""}.fa-untappd:before{content:""}.fa-upload:before{content:""}.fa-ups:before{content:""}.fa-usb:before{content:""}.fa-user:before{content:""}.fa-user-alt:before{content:""}.fa-user-alt-slash:before{content:""}.fa-user-astronaut:before{content:""}.fa-user-check:before{content:""}.fa-user-circle:before{content:""}.fa-user-clock:before{content:""}.fa-user-cog:before{content:""}.fa-user-edit:before{content:""}.fa-user-friends:before{content:""}.fa-user-graduate:before{content:""}.fa-user-injured:before{content:""}.fa-user-lock:before{content:""}.fa-user-md:before{content:""}.fa-user-minus:before{content:""}.fa-user-ninja:before{content:""}.fa-user-nurse:before{content:""}.fa-user-plus:before{content:""}.fa-user-secret:before{content:""}.fa-user-shield:before{content:""}.fa-user-slash:before{content:""}.fa-user-tag:before{content:""}.fa-user-tie:before{content:""}.fa-user-times:before{content:""}.fa-users:before{content:""}.fa-users-cog:before{content:""}.fa-users-slash:before{content:""}.fa-usps:before{content:""}.fa-ussunnah:before{content:""}.fa-utensil-spoon:before{content:""}.fa-utensils:before{content:""}.fa-vaadin:before{content:""}.fa-vector-square:before{content:""}.fa-venus:before{content:""}.fa-venus-double:before{content:""}.fa-venus-mars:before{content:""}.fa-vest:before{content:""}.fa-vest-patches:before{content:""}.fa-viacoin:before{content:""}.fa-viadeo:before{content:""}.fa-viadeo-square:before{content:""}.fa-vial:before{content:""}.fa-vials:before{content:""}.fa-viber:before{content:""}.fa-video:before{content:""}.fa-video-slash:before{content:""}.fa-vihara:before{content:""}.fa-vimeo:before{content:""}.fa-vimeo-square:before{content:""}.fa-vimeo-v:before{content:""}.fa-vine:before{content:""}.fa-virus:before{content:""}.fa-virus-slash:before{content:""}.fa-viruses:before{content:""}.fa-vk:before{content:""}.fa-vnv:before{content:""}.fa-voicemail:before{content:""}.fa-volleyball-ball:before{content:""}.fa-volume-down:before{content:""}.fa-volume-mute:before{content:""}.fa-volume-off:before{content:""}.fa-volume-up:before{content:""}.fa-vote-yea:before{content:""}.fa-vr-cardboard:before{content:""}.fa-vuejs:before{content:""}.fa-walking:before{content:""}.fa-wallet:before{content:""}.fa-warehouse:before{content:""}.fa-watchman-monitoring:before{content:""}.fa-water:before{content:""}.fa-wave-square:before{content:""}.fa-waze:before{content:""}.fa-weebly:before{content:""}.fa-weibo:before{content:""}.fa-weight:before{content:""}.fa-weight-hanging:before{content:""}.fa-weixin:before{content:""}.fa-whatsapp:before{content:""}.fa-whatsapp-square:before{content:""}.fa-wheelchair:before{content:""}.fa-whmcs:before{content:""}.fa-wifi:before{content:""}.fa-wikipedia-w:before{content:""}.fa-wind:before{content:""}.fa-window-close:before{content:""}.fa-window-maximize:before{content:""}.fa-window-minimize:before{content:""}.fa-window-restore:before{content:""}.fa-windows:before{content:""}.fa-wine-bottle:before{content:""}.fa-wine-glass:before{content:""}.fa-wine-glass-alt:before{content:""}.fa-wix:before{content:""}.fa-wizards-of-the-coast:before{content:""}.fa-wodu:before{content:""}.fa-wolf-pack-battalion:before{content:""}.fa-won-sign:before{content:""}.fa-wordpress:before{content:""}.fa-wordpress-simple:before{content:""}.fa-wpbeginner:before{content:""}.fa-wpexplorer:before{content:""}.fa-wpforms:before{content:""}.fa-wpressr:before{content:""}.fa-wrench:before{content:""}.fa-x-ray:before{content:""}.fa-xbox:before{content:""}.fa-xing:before{content:""}.fa-xing-square:before{content:""}.fa-y-combinator:before{content:""}.fa-yahoo:before{content:""}.fa-yammer:before{content:""}.fa-yandex:before{content:""}.fa-yandex-international:before{content:""}.fa-yarn:before{content:""}.fa-yelp:before{content:""}.fa-yen-sign:before{content:""}.fa-yin-yang:before{content:""}.fa-yoast:before{content:""}.fa-youtube:before{content:""}.fa-youtube-square:before{content:""}.fa-zhihu:before{content:""}.sr-only{border:0;clip:rect(0,0,0,0);height:1px;margin:-1px;overflow:hidden;padding:0;position:absolute;width:1px}.sr-only-focusable:active,.sr-only-focusable:focus{clip:auto;height:auto;margin:0;overflow:visible;position:static;width:auto}@font-face{font-family:'Font Awesome 5 Free';font-style:normal;font-weight:400;font-display:block;src:url('../fontawesome/webfonts/fa-regular-400.eot');src:url('../fontawesome/webfonts/fa-regular-400.eot?#iefix') format('embedded-opentype'),url('../fontawesome/webfonts/fa-regular-400.woff2') format('woff2'),url('../fontawesome/webfonts/fa-regular-400.woff') format('woff'),url('../fontawesome/webfonts/fa-regular-400.ttf') format('truetype'),url('../fontawesome/webfonts/fa-regular-400.svg#fontawesome') format('svg')}.far{font-family:'Font Awesome 5 Free';font-weight:400}@font-face{font-family:'Font Awesome 5 Free';font-style:normal;font-weight:900;font-display:block;src:url('../fontawesome/webfonts/fa-solid-900.eot');src:url('../fontawesome/webfonts/fa-solid-900.eot?#iefix') format('embedded-opentype'),url('../fontawesome/webfonts/fa-solid-900.woff2') format('woff2'),url('../fontawesome/webfonts/fa-solid-900.woff') format('woff'),url('../fontawesome/webfonts/fa-solid-900.ttf') format('truetype'),url('../fontawesome/webfonts/fa-solid-900.svg#fontawesome') format('svg')}.fa,.fas{font-family:'Font Awesome 5 Free';font-weight:900}.navbar .btn-navbar{color:#fff;text-shadow:0 -1px 0 rgba(0,0,0,.25);background-color:#002f3d;background-image:-moz-linear-gradient(top,#002f3d,#002f3d);background-image:-webkit-gradient(linear,0 0,0 100%,from(#002f3d),to(#002f3d));background-image:-webkit-linear-gradient(top,#002f3d,#002f3d);background-image:-o-linear-gradient(top,#002f3d,#002f3d);background-image:linear-gradient(to bottom,#002f3d,#002f3d);background-repeat:repeat-x;filter:progid:DXImageTransform.Microsoft.gradient(startColorstr='#ff002f3d',endColorstr='#ff002f3d',GradientType=0);border-color:#002f3d #002f3d #000;border-color:rgba(0,0,0,.1) rgba(0,0,0,.1) rgba(0,0,0,.25);*background-color:#002f3d;filter:progid:DXImageTransform.Microsoft.gradient(enabled=false)}.navbar .btn-navbar:hover,.navbar .btn-navbar:focus,.navbar .btn-navbar:active,.navbar .btn-navbar.active,.navbar .btn-navbar.disabled,.navbar .btn-navbar[disabled]{color:#fff;background-color:#002f3d;*background-color:#001b23}.navbar .btn-navbar:active,.navbar .btn-navbar.active{background-color:#00080a \9}@media(max-width:979px){.nav-collapse.collapse:not(.in)>*{display:none}.nav-collapse .open>.dropdown-menu{position:relative}}footer a{text-decoration:underline}html,body{height:100%}body{overflow-y:scroll}::placeholder{color:green;opacity:1}div.header{height:10px;background-color:#253d57;color:#fff;font-size:18px;font-weight:bold}div.header a,div.header a:hover{color:#fff;text-decoration:none}div.header a img,div.header a:hover img{padding-right:20px}div.navbar-inner{border:none;font-size:15px}div.navbar-inner .active{margin-top:-4px;border-top:4px solid #46a546}div.navbar-inner .nav>.active>a:focus{background-color:#98d4ee}div.navbar-inner .nav>li>a{text-shadow:none}div.navbar-inner .nav>li>a:focus{background-color:#98d4ee}div.filter-panel{color:#fff;padding-top:5px}.ajax-progress{background-image:url('../images/ajax32.gif');background-position:center;background-repeat:no-repeat;z-index:1060}.ajax-progress-container{background-image:url('../images/ajax16-3.gif');background-position:center;background-repeat:no-repeat}.ajax-progress-container.conflict{margin-left:-20px;min-width:20px;min-height:20px;display:inline-block;vertical-align:middle}.ajax-progress-container>*{display:none}.left-menu .well{padding:0;margin-top:20px}.left-menu .menu-group{padding:3px 5px;font-weight:bold;background-color:#d4d4d4}.left-menu .menu-group[data-toggle="collapse"]{cursor:pointer}.left-menu .controls{padding:10px;padding-bottom:0}.left-menu .controls select,.left-menu .controls input,.left-menu .controls textarea{width:100%}div.messages{bottom:10px;position:fixed;z-index:1070;width:940px}div.messages iframe{display:block;width:880px;height:300px;background:#fff}@media(min-width:1200px){div.messages{width:1170px}div.messages iframe{width:1100px}}@media(min-width:768px) and (max-width:979px){div.messages{width:724px}div.messages iframe{width:682px}}@media(max-width:767px){div.messages{width:auto;margin-right:20px}div.messages iframe{width:auto}}@media print{a[href]:after{content:none}}.form-settings .controls{margin-left:410px}.form-settings .control-label{width:400px}.form-horizontal h1,.view-horizontal h1{border-bottom:1px solid #6c757d;font-size:17.5px;line-height:20px;font-weight:normal;padding-top:10px;padding-bottom:5px}.form-horizontal h2,.view-horizontal h2{font-size:11.9px;line-height:20px;color:#555;background:#f5f5f5;padding-left:10px;padding-top:7px;padding-bottom:7px;text-transform:uppercase;border-bottom:1px solid #e5e5e5}.form-horizontal .controls.control-text,.view-horizontal .controls.control-text{padding-top:5px}.error .control-label,.error .help-block,.error .help-inline{color:#b94a48}.error .checkbox,.error .radio,.error input,.error select,.error textarea{color:#b94a48}.error input,.error select,.error textarea{border-color:#b94a48;-webkit-box-shadow:inset 0 1px 1px rgba(0,0,0,.075);-moz-box-shadow:inset 0 1px 1px rgba(0,0,0,.075);box-shadow:inset 0 1px 1px rgba(0,0,0,.075)}.error input:focus,.error select:focus,.error textarea:focus{border-color:#953b39;-webkit-box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #d59392;-moz-box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #d59392;box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #d59392}.error .input-prepend .add-on,.error .input-append .add-on{color:#b94a48;background-color:#f2dede;border-color:#b94a48}.warning .control-label,.warning .help-block,.warning .help-inline{color:#c09853}.warning .checkbox,.warning .radio,.warning input,.warning select,.warning textarea{color:#c09853}.warning input,.warning select,.warning textarea{border-color:#c09853;-webkit-box-shadow:inset 0 1px 1px rgba(0,0,0,.075);-moz-box-shadow:inset 0 1px 1px rgba(0,0,0,.075);box-shadow:inset 0 1px 1px rgba(0,0,0,.075)}.warning input:focus,.warning select:focus,.warning textarea:focus{border-color:#a47e3c;-webkit-box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #dbc59e;-moz-box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #dbc59e;box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #dbc59e}.warning .input-prepend .add-on,.warning .input-append .add-on{color:#c09853;background-color:#fcf8e3;border-color:#c09853}.success .control-label,.success .help-block,.success .help-inline{color:#417e42}.success .checkbox,.success .radio,.success input,.success select,.success textarea{color:#417e42}.success input,.success select,.success textarea{border-color:#417e42;-webkit-box-shadow:inset 0 1px 1px rgba(0,0,0,.075);-moz-box-shadow:inset 0 1px 1px rgba(0,0,0,.075);box-shadow:inset 0 1px 1px rgba(0,0,0,.075)}.success input:focus,.success select:focus,.success textarea:focus{border-color:#2f5c30;-webkit-box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #70b571;-moz-box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #70b571;box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #70b571}.success .input-prepend .add-on,.success .input-append .add-on{color:#417e42;background-color:#dff0d8;border-color:#417e42}.info .control-label,.info .help-block,.info .help-inline{color:#2d6987}.info .checkbox,.info .radio,.info input,.info select,.info textarea{color:#2d6987}.info input,.info select,.info textarea{border-color:#2d6987;-webkit-box-shadow:inset 0 1px 1px rgba(0,0,0,.075);-moz-box-shadow:inset 0 1px 1px rgba(0,0,0,.075);box-shadow:inset 0 1px 1px rgba(0,0,0,.075)}.info input:focus,.info select:focus,.info textarea:focus{border-color:#204b61;-webkit-box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #54a0c6;-moz-box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #54a0c6;box-shadow:inset 0 1px 1px rgba(0,0,0,.075),0 0 6px #54a0c6}.info .input-prepend .add-on,.info .input-append .add-on{color:#2d6987;background-color:#eef7fb;border-color:#2d6987}@media(max-width:480px){.form-settings .controls{margin-left:0}.controls.control-text{padding-top:0}}.form-actions a,.form-actions button{margin-left:40px}.form-actions .alert{margin-bottom:0}.modal-with-dropdown-menu{position:fixed;top:10%;left:50%;z-index:1050;width:560px;margin-left:-280px;background-color:#fff;border:1px solid #999;border:1px solid rgba(0,0,0,.3);*border:1px solid #999;-webkit-border-radius:6px;-moz-border-radius:6px;border-radius:6px;-webkit-box-shadow:0 3px 7px rgba(0,0,0,.3);-moz-box-shadow:0 3px 7px rgba(0,0,0,.3);box-shadow:0 3px 7px rgba(0,0,0,.3);-webkit-background-clip:padding-box;-moz-background-clip:padding-box;background-clip:padding-box;outline:none;position:absolute}.modal-with-dropdown-menu.fade{-webkit-transition:opacity .3s linear,top .3s ease-out;-moz-transition:opacity .3s linear,top .3s ease-out;-o-transition:opacity .3s linear,top .3s ease-out;transition:opacity .3s linear,top .3s ease-out;top:-25%}.modal-with-dropdown-menu.fade.in{top:10%}.modal-with-dropdown-menu>form{margin:0}.modal-with-dropdown-menu .modal-body{overflow:visible;max-height:none}.modal{overflow:auto;max-height:80vh}.modal>form{margin:0}.modal .modal-header{background-color:#f5f5f5;-webkit-border-top-left-radius:6px;-moz-border-radius-topleft:6px;border-top-left-radius:6px;-webkit-border-top-right-radius:6px;-moz-border-radius-topright:6px;border-top-right-radius:6px}@media(max-width:767px){.modal{position:absolute}}.modal-backdrop,.modal-backdrop.fade.in{opacity:.5;filter:alpha(opacity=50)}.table thead th{vertical-align:middle}tr.highlight>td{background-color:#f9f9f9}span.tree-symbol{font-size:22px;margin-top:-4px;display:inline-table}.child-item{font-size:10.5px;padding-left:15px}td.button-column{text-align:center}.button-column{width:1px;white-space:nowrap}.first-button-column th:first-child,.first-button-column td:first-child{width:1px;white-space:nowrap}.last-button-column th:last-child,.last-button-column td:last-child{width:1px;white-space:nowrap}td.label-column{text-align:right;font-weight:bold}td.custom-column,th.custom-column{background-color:#f5f5f5}td>input[type="radio"],td>input[type="checkbox"]{margin:0}td>label{display:inline;margin:0}div.showMore{text-align:right;margin-top:0;padding-bottom:20px}.view-horizontal>div.row{padding-top:2px;padding-bottom:4px}.view-horizontal>div.row>div:first-child:not(.no-bold){font-weight:bold}.view-striped>div.row{border-bottom:1px solid #ddd;margin-left:0}.view-striped>div.row>div{margin-left:0}@media(min-width:768px){.view-striped>div.row>div:first-child{padding-left:20px}}.view-striped>div.row:nth-of-type(odd){background-color:#f9f9f9}ul.dropdown-menu.dropdown-form{padding:10px}ul.dropdown-menu a{cursor:pointer}.icon-disabled{opacity:.25}.small{color:#6c757d;font-size:10.5px}h1.small{color:inherit;font-size:24.5px}.actions .pagination{margin:0}.nowrap-small-link{font-size:11.9px;white-space:nowrap}ul.inline-list{margin:0;list-style-type:none}ul.inline>li{display:inline-block}ul.inline>li:first-child{margin-left:0;padding-left:0}ul.inline>li>label{display:inline-block}ul,ul ul{list-style-type:disc;margin-bottom:0}.questionheading{color:#555;background-color:#f5f5f5;margin-top:15px;margin-bottom:5px;font-size:1.1em}.small-subjectarea-section{height:150px;overflow-y:auto}.large-subjectarea-section{height:350px;overflow-y:auto}.dropTarget{min-height:20px;padding:19px;margin-bottom:20px;background-color:#f5f5f5;border:1px solid #e3e3e3;-webkit-border-radius:4px;-moz-border-radius:4px;border-radius:4px;-webkit-box-shadow:inset 0 1px 1px rgba(0,0,0,.05);-moz-box-shadow:inset 0 1px 1px rgba(0,0,0,.05);box-shadow:inset 0 1px 1px rgba(0,0,0,.05);text-align:center;border-style:dashed;border-width:4px}.dropTarget blockquote{border-color:#ddd;border-color:rgba(0,0,0,.15)}.dragOver{border-color:#000}div#but-footer{min-height:100%;height:auto!important;height:100%;margin:0 auto -68px}div#push-footer{height:102px}div.footer{border-top:3px solid #007ea3;height:45px;padding-top:20px;background-color:#eee}@media(max-width:767px){.footer{margin-left:-20px;margin-right:-20px;padding-left:20px;padding-right:20px}.footer .footer-copyright,.footer .footer-links-container,.footer .social-media-icon{clear:both;float:left}.footer .footer-links-container{margin:10px 0}}@media(min-width:768px){.footer .footer-links-container{margin-left:20px;display:unset}.footer .social-media-icon{float:right}.footer .social-media-icon img{margin-left:16px}}legend{color:#007ea3!important}.validation-summary-errors,.field-validation-valid{color:#b94a48}*{padding:0;margin:0}div#SubmissionListForm table{padding-right:25px;border-right:0;border-top:0;border-bottom:0}div#ExternalReviewForm tbody .id,div#ReferenceForm tbody .id,div#MetaBiddingForm tbody .id,div#BiddingForm tbody .id,div#submissionListForm tbody .id,div#emailMessagesForm tbody .id,div#auditForm tbody .id,div#DeletedSubmissionListForm tbody .id,#SuggestionForm tbody .id{width:35px}div#ExternalReviewForm tbody .abstract,div#ReferenceForm tbody .abstract,div#MetaBiddingForm tbody .abstract,div#BiddingForm tbody .abstract,div#submissionListForm tbody .abstract,div#emailMessagesForm tbody .abstract,div#auditForm tbody .abstract,div#DeletedSubmissionListForm tbody .abstract,#SuggestionForm tbody .abstract{bottom:5px;right:5px;font-size:12px;cursor:pointer}.table-common-container header,div#ProceedingEditorSubmissions header,div#divUserDisputeConflicts header,div#metaReviewerListForm header,div#reviewerListForm header,div#DeletedSubmissionListForm header,div#SuggestionForm header,div#MetaBiddingForm header,div#ExternalReviewForm header,div#ReferenceForm header,div#BiddingForm header,div#SubmissionListForm header,div#EmailMessagesForm header,div#AuditForm header,div#ReviewerInvitationListForm header,div#ReviewerInvitationForSubmissionListForm header,div#userListForm header,div#AutoAssignmentPapers header,div#AutoAssignmentReviewers header,div#AutoAssignmentSettings header,div#AutoAssignmentConfirmation header{font-size:25px;font-weight:bold;height:40px;line-height:40px;position:relative;margin:10px 0;min-height:40px;padding:0;background-color:#fff;background-image:none;border:none;box-shadow:none;-webkit-box-shadow:none}.table-common-container header.no-margin-top,div#ProceedingEditorSubmissions header.no-margin-top,div#divUserDisputeConflicts header.no-margin-top,div#metaReviewerListForm header.no-margin-top,div#reviewerListForm header.no-margin-top,div#DeletedSubmissionListForm header.no-margin-top,div#SuggestionForm header.no-margin-top,div#MetaBiddingForm header.no-margin-top,div#ExternalReviewForm header.no-margin-top,div#ReferenceForm header.no-margin-top,div#BiddingForm header.no-margin-top,div#SubmissionListForm header.no-margin-top,div#EmailMessagesForm header.no-margin-top,div#AuditForm header.no-margin-top,div#ReviewerInvitationListForm header.no-margin-top,div#ReviewerInvitationForSubmissionListForm header.no-margin-top,div#userListForm header.no-margin-top,div#AutoAssignmentPapers header.no-margin-top,div#AutoAssignmentReviewers header.no-margin-top,div#AutoAssignmentSettings header.no-margin-top,div#AutoAssignmentConfirmation header.no-margin-top{margin-top:0}.table-common-container header .title,div#ProceedingEditorSubmissions header .title,div#divUserDisputeConflicts header .title,div#metaReviewerListForm header .title,div#reviewerListForm header .title,div#DeletedSubmissionListForm header .title,div#SuggestionForm header .title,div#MetaBiddingForm header .title,div#ExternalReviewForm header .title,div#ReferenceForm header .title,div#BiddingForm header .title,div#SubmissionListForm header .title,div#EmailMessagesForm header .title,div#AuditForm header .title,div#ReviewerInvitationListForm header .title,div#ReviewerInvitationForSubmissionListForm header .title,div#userListForm header .title,div#AutoAssignmentPapers header .title,div#AutoAssignmentReviewers header .title,div#AutoAssignmentSettings header .title,div#AutoAssignmentConfirmation header .title{color:#0088ac;font-size:17px;font-weight:bold}.table-common-container header .actions,div#ProceedingEditorSubmissions header .actions,div#divUserDisputeConflicts header .actions,div#metaReviewerListForm header .actions,div#reviewerListForm header .actions,div#DeletedSubmissionListForm header .actions,div#SuggestionForm header .actions,div#MetaBiddingForm header .actions,div#ExternalReviewForm header .actions,div#ReferenceForm header .actions,div#BiddingForm header .actions,div#SubmissionListForm header .actions,div#EmailMessagesForm header .actions,div#AuditForm header .actions,div#ReviewerInvitationListForm header .actions,div#ReviewerInvitationForSubmissionListForm header .actions,div#userListForm header .actions,div#AutoAssignmentPapers header .actions,div#AutoAssignmentReviewers header .actions,div#AutoAssignmentSettings header .actions,div#AutoAssignmentConfirmation header .actions{float:right;margin:10px 0;font-size:12px}.table-common-container header .actions .box,div#ProceedingEditorSubmissions header .actions .box,div#divUserDisputeConflicts header .actions .box,div#metaReviewerListForm header .actions .box,div#reviewerListForm header .actions .box,div#DeletedSubmissionListForm header .actions .box,div#SuggestionForm header .actions .box,div#MetaBiddingForm header .actions .box,div#ExternalReviewForm header .actions .box,div#ReferenceForm header .actions .box,div#BiddingForm header .actions .box,div#SubmissionListForm header .actions .box,div#EmailMessagesForm header .actions .box,div#AuditForm header .actions .box,div#ReviewerInvitationListForm header .actions .box,div#ReviewerInvitationForSubmissionListForm header .actions .box,div#userListForm header .actions .box,div#AutoAssignmentPapers header .actions .box,div#AutoAssignmentReviewers header .actions .box,div#AutoAssignmentSettings header .actions .box,div#AutoAssignmentConfirmation header .actions .box{line-height:40px;vertical-align:middle;float:right;margin-right:20px}.table-common-container header .actions .box span,div#ProceedingEditorSubmissions header .actions .box span,div#divUserDisputeConflicts header .actions .box span,div#metaReviewerListForm header .actions .box span,div#reviewerListForm header .actions .box span,div#DeletedSubmissionListForm header .actions .box span,div#SuggestionForm header .actions .box span,div#MetaBiddingForm header .actions .box span,div#ExternalReviewForm header .actions .box span,div#ReferenceForm header .actions .box span,div#BiddingForm header .actions .box span,div#SubmissionListForm header .actions .box span,div#EmailMessagesForm header .actions .box span,div#AuditForm header .actions .box span,div#ReviewerInvitationListForm header .actions .box span,div#ReviewerInvitationForSubmissionListForm header .actions .box span,div#userListForm header .actions .box span,div#AutoAssignmentPapers header .actions .box span,div#AutoAssignmentReviewers header .actions .box span,div#AutoAssignmentSettings header .actions .box span,div#AutoAssignmentConfirmation header .actions .box span{color:#0088ac;font-size:15px;display:inline-block;line-height:40px;vertical-align:middle}.table-common-container header .actions .box small,div#ProceedingEditorSubmissions header .actions .box small,div#divUserDisputeConflicts header .actions .box small,div#metaReviewerListForm header .actions .box small,div#reviewerListForm header .actions .box small,div#DeletedSubmissionListForm header .actions .box small,div#SuggestionForm header .actions .box small,div#MetaBiddingForm header .actions .box small,div#ExternalReviewForm header .actions .box small,div#ReferenceForm header .actions .box small,div#BiddingForm header .actions .box small,div#SubmissionListForm header .actions .box small,div#EmailMessagesForm header .actions .box small,div#AuditForm header .actions .box small,div#ReviewerInvitationListForm header .actions .box small,div#ReviewerInvitationForSubmissionListForm header .actions .box small,div#userListForm header .actions .box small,div#AutoAssignmentPapers header .actions .box small,div#AutoAssignmentReviewers header .actions .box small,div#AutoAssignmentSettings header .actions .box small,div#AutoAssignmentConfirmation header .actions .box small{width:30px}.table-common-container header .actions .box a,div#ProceedingEditorSubmissions header .actions .box a,div#divUserDisputeConflicts header .actions .box a,div#metaReviewerListForm header .actions .box a,div#reviewerListForm header .actions .box a,div#DeletedSubmissionListForm header .actions .box a,div#SuggestionForm header .actions .box a,div#MetaBiddingForm header .actions .box a,div#ExternalReviewForm header .actions .box a,div#ReferenceForm header .actions .box a,div#BiddingForm header .actions .box a,div#SubmissionListForm header .actions .box a,div#EmailMessagesForm header .actions .box a,div#AuditForm header .actions .box a,div#ReviewerInvitationListForm header .actions .box a,div#ReviewerInvitationForSubmissionListForm header .actions .box a,div#userListForm header .actions .box a,div#AutoAssignmentPapers header .actions .box a,div#AutoAssignmentReviewers header .actions .box a,div#AutoAssignmentSettings header .actions .box a,div#AutoAssignmentConfirmation header .actions .box a{width:30px;margin:0 2px}.table-common-container header .actions .box.show .btn-success,div#ProceedingEditorSubmissions header .actions .box.show .btn-success,div#divUserDisputeConflicts header .actions .box.show .btn-success,div#metaReviewerListForm header .actions .box.show .btn-success,div#reviewerListForm header .actions .box.show .btn-success,div#DeletedSubmissionListForm header .actions .box.show .btn-success,div#SuggestionForm header .actions .box.show .btn-success,div#MetaBiddingForm header .actions .box.show .btn-success,div#ExternalReviewForm header .actions .box.show .btn-success,div#ReferenceForm header .actions .box.show .btn-success,div#BiddingForm header .actions .box.show .btn-success,div#SubmissionListForm header .actions .box.show .btn-success,div#EmailMessagesForm header .actions .box.show .btn-success,div#AuditForm header .actions .box.show .btn-success,div#ReviewerInvitationListForm header .actions .box.show .btn-success,div#ReviewerInvitationForSubmissionListForm header .actions .box.show .btn-success,div#userListForm header .actions .box.show .btn-success,div#AutoAssignmentPapers header .actions .box.show .btn-success,div#AutoAssignmentReviewers header .actions .box.show .btn-success,div#AutoAssignmentSettings header .actions .box.show .btn-success,div#AutoAssignmentConfirmation header .actions .box.show .btn-success{color:#fff}.table-common-container header .actions .box.other,div#ProceedingEditorSubmissions header .actions .box.other,div#divUserDisputeConflicts header .actions .box.other,div#metaReviewerListForm header .actions .box.other,div#reviewerListForm header .actions .box.other,div#DeletedSubmissionListForm header .actions .box.other,div#SuggestionForm header .actions .box.other,div#MetaBiddingForm header .actions .box.other,div#ExternalReviewForm header .actions .box.other,div#ReferenceForm header .actions .box.other,div#BiddingForm header .actions .box.other,div#SubmissionListForm header .actions .box.other,div#EmailMessagesForm header .actions .box.other,div#AuditForm header .actions .box.other,div#ReviewerInvitationListForm header .actions .box.other,div#ReviewerInvitationForSubmissionListForm header .actions .box.other,div#userListForm header .actions .box.other,div#AutoAssignmentPapers header .actions .box.other,div#AutoAssignmentReviewers header .actions .box.other,div#AutoAssignmentSettings header .actions .box.other,div#AutoAssignmentConfirmation header .actions .box.other{margin-right:0}.table-common-container header .actions .box.other .act-title,div#ProceedingEditorSubmissions header .actions .box.other .act-title,div#divUserDisputeConflicts header .actions .box.other .act-title,div#metaReviewerListForm header .actions .box.other .act-title,div#reviewerListForm header .actions .box.other .act-title,div#DeletedSubmissionListForm header .actions .box.other .act-title,div#SuggestionForm header .actions .box.other .act-title,div#MetaBiddingForm header .actions .box.other .act-title,div#ExternalReviewForm header .actions .box.other .act-title,div#ReferenceForm header .actions .box.other .act-title,div#BiddingForm header .actions .box.other .act-title,div#SubmissionListForm header .actions .box.other .act-title,div#EmailMessagesForm header .actions .box.other .act-title,div#AuditForm header .actions .box.other .act-title,div#ReviewerInvitationListForm header .actions .box.other .act-title,div#ReviewerInvitationForSubmissionListForm header .actions .box.other .act-title,div#userListForm header .actions .box.other .act-title,div#AutoAssignmentPapers header .actions .box.other .act-title,div#AutoAssignmentReviewers header .actions .box.other .act-title,div#AutoAssignmentSettings header .actions .box.other .act-title,div#AutoAssignmentConfirmation header .actions .box.other .act-title{width:60px}.table-common-container header .actions .box.other .dropdown-menu a,div#ProceedingEditorSubmissions header .actions .box.other .dropdown-menu a,div#divUserDisputeConflicts header .actions .box.other .dropdown-menu a,div#metaReviewerListForm header .actions .box.other .dropdown-menu a,div#reviewerListForm header .actions .box.other .dropdown-menu a,div#DeletedSubmissionListForm header .actions .box.other .dropdown-menu a,div#SuggestionForm header .actions .box.other .dropdown-menu a,div#MetaBiddingForm header .actions .box.other .dropdown-menu a,div#ExternalReviewForm header .actions .box.other .dropdown-menu a,div#ReferenceForm header .actions .box.other .dropdown-menu a,div#BiddingForm header .actions .box.other .dropdown-menu a,div#SubmissionListForm header .actions .box.other .dropdown-menu a,div#EmailMessagesForm header .actions .box.other .dropdown-menu a,div#AuditForm header .actions .box.other .dropdown-menu a,div#ReviewerInvitationListForm header .actions .box.other .dropdown-menu a,div#ReviewerInvitationForSubmissionListForm header .actions .box.other .dropdown-menu a,div#userListForm header .actions .box.other .dropdown-menu a,div#AutoAssignmentPapers header .actions .box.other .dropdown-menu a,div#AutoAssignmentReviewers header .actions .box.other .dropdown-menu a,div#AutoAssignmentSettings header .actions .box.other .dropdown-menu a,div#AutoAssignmentConfirmation header .actions .box.other .dropdown-menu a{width:inherit}.table-common-container header .actions .box.reset a,div#ProceedingEditorSubmissions header .actions .box.reset a,div#divUserDisputeConflicts header .actions .box.reset a,div#metaReviewerListForm header .actions .box.reset a,div#reviewerListForm header .actions .box.reset a,div#DeletedSubmissionListForm header .actions .box.reset a,div#SuggestionForm header .actions .box.reset a,div#MetaBiddingForm header .actions .box.reset a,div#ExternalReviewForm header .actions .box.reset a,div#ReferenceForm header .actions .box.reset a,div#BiddingForm header .actions .box.reset a,div#SubmissionListForm header .actions .box.reset a,div#EmailMessagesForm header .actions .box.reset a,div#AuditForm header .actions .box.reset a,div#ReviewerInvitationListForm header .actions .box.reset a,div#ReviewerInvitationForSubmissionListForm header .actions .box.reset a,div#userListForm header .actions .box.reset a,div#AutoAssignmentPapers header .actions .box.reset a,div#AutoAssignmentReviewers header .actions .box.reset a,div#AutoAssignmentSettings header .actions .box.reset a,div#AutoAssignmentConfirmation header .actions .box.reset a{width:90px}.table-common-container header .actions .dropdown-menu a,div#ProceedingEditorSubmissions header .actions .dropdown-menu a,div#divUserDisputeConflicts header .actions .dropdown-menu a,div#metaReviewerListForm header .actions .dropdown-menu a,div#reviewerListForm header .actions .dropdown-menu a,div#DeletedSubmissionListForm header .actions .dropdown-menu a,div#SuggestionForm header .actions .dropdown-menu a,div#MetaBiddingForm header .actions .dropdown-menu a,div#ExternalReviewForm header .actions .dropdown-menu a,div#ReferenceForm header .actions .dropdown-menu a,div#BiddingForm header .actions .dropdown-menu a,div#SubmissionListForm header .actions .dropdown-menu a,div#EmailMessagesForm header .actions .dropdown-menu a,div#AuditForm header .actions .dropdown-menu a,div#ReviewerInvitationListForm header .actions .dropdown-menu a,div#ReviewerInvitationForSubmissionListForm header .actions .dropdown-menu a,div#userListForm header .actions .dropdown-menu a,div#AutoAssignmentPapers header .actions .dropdown-menu a,div#AutoAssignmentReviewers header .actions .dropdown-menu a,div#AutoAssignmentSettings header .actions .dropdown-menu a,div#AutoAssignmentConfirmation header .actions .dropdown-menu a{font-size:15px;color:#000}.table-common-container header .actions .dropdown-menu a:hover,div#ProceedingEditorSubmissions header .actions .dropdown-menu a:hover,div#divUserDisputeConflicts header .actions .dropdown-menu a:hover,div#metaReviewerListForm header .actions .dropdown-menu a:hover,div#reviewerListForm header .actions .dropdown-menu a:hover,div#DeletedSubmissionListForm header .actions .dropdown-menu a:hover,div#SuggestionForm header .actions .dropdown-menu a:hover,div#MetaBiddingForm header .actions .dropdown-menu a:hover,div#ExternalReviewForm header .actions .dropdown-menu a:hover,div#ReferenceForm header .actions .dropdown-menu a:hover,div#BiddingForm header .actions .dropdown-menu a:hover,div#SubmissionListForm header .actions .dropdown-menu a:hover,div#EmailMessagesForm header .actions .dropdown-menu a:hover,div#AuditForm header .actions .dropdown-menu a:hover,div#ReviewerInvitationListForm header .actions .dropdown-menu a:hover,div#ReviewerInvitationForSubmissionListForm header .actions .dropdown-menu a:hover,div#userListForm header .actions .dropdown-menu a:hover,div#AutoAssignmentPapers header .actions .dropdown-menu a:hover,div#AutoAssignmentReviewers header .actions .dropdown-menu a:hover,div#AutoAssignmentSettings header .actions .dropdown-menu a:hover,div#AutoAssignmentConfirmation header .actions .dropdown-menu a:hover{color:#f5f5f5;text-decoration:none}.table-common-container header .actions .dropdown-menu li.disabled a,div#ProceedingEditorSubmissions header .actions .dropdown-menu li.disabled a,div#divUserDisputeConflicts header .actions .dropdown-menu li.disabled a,div#metaReviewerListForm header .actions .dropdown-menu li.disabled a,div#reviewerListForm header .actions .dropdown-menu li.disabled a,div#DeletedSubmissionListForm header .actions .dropdown-menu li.disabled a,div#SuggestionForm header .actions .dropdown-menu li.disabled a,div#MetaBiddingForm header .actions .dropdown-menu li.disabled a,div#ExternalReviewForm header .actions .dropdown-menu li.disabled a,div#ReferenceForm header .actions .dropdown-menu li.disabled a,div#BiddingForm header .actions .dropdown-menu li.disabled a,div#SubmissionListForm header .actions .dropdown-menu li.disabled a,div#EmailMessagesForm header .actions .dropdown-menu li.disabled a,div#AuditForm header .actions .dropdown-menu li.disabled a,div#ReviewerInvitationListForm header .actions .dropdown-menu li.disabled a,div#ReviewerInvitationForSubmissionListForm header .actions .dropdown-menu li.disabled a,div#userListForm header .actions .dropdown-menu li.disabled a,div#AutoAssignmentPapers header .actions .dropdown-menu li.disabled a,div#AutoAssignmentReviewers header .actions .dropdown-menu li.disabled a,div#AutoAssignmentSettings header .actions .dropdown-menu li.disabled a,div#AutoAssignmentConfirmation header .actions .dropdown-menu li.disabled a{color:#999}.table-common-container header .actions .paging a.number,div#ProceedingEditorSubmissions header .actions .paging a.number,div#divUserDisputeConflicts header .actions .paging a.number,div#metaReviewerListForm header .actions .paging a.number,div#reviewerListForm header .actions .paging a.number,div#DeletedSubmissionListForm header .actions .paging a.number,div#SuggestionForm header .actions .paging a.number,div#MetaBiddingForm header .actions .paging a.number,div#ExternalReviewForm header .actions .paging a.number,div#ReferenceForm header .actions .paging a.number,div#BiddingForm header .actions .paging a.number,div#SubmissionListForm header .actions .paging a.number,div#EmailMessagesForm header .actions .paging a.number,div#AuditForm header .actions .paging a.number,div#ReviewerInvitationListForm header .actions .paging a.number,div#ReviewerInvitationForSubmissionListForm header .actions .paging a.number,div#userListForm header .actions .paging a.number,div#AutoAssignmentPapers header .actions .paging a.number,div#AutoAssignmentReviewers header .actions .paging a.number,div#AutoAssignmentSettings header .actions .paging a.number,div#AutoAssignmentConfirmation header .actions .paging a.number{color:#fff;border-radius:3px;padding:2px 10px 5px 10px}.table-common-container header .actions .paging a.number:hover,div#ProceedingEditorSubmissions header .actions .paging a.number:hover,div#divUserDisputeConflicts header .actions .paging a.number:hover,div#metaReviewerListForm header .actions .paging a.number:hover,div#reviewerListForm header .actions .paging a.number:hover,div#DeletedSubmissionListForm header .actions .paging a.number:hover,div#SuggestionForm header .actions .paging a.number:hover,div#MetaBiddingForm header .actions .paging a.number:hover,div#ExternalReviewForm header .actions .paging a.number:hover,div#ReferenceForm header .actions .paging a.number:hover,div#BiddingForm header .actions .paging a.number:hover,div#SubmissionListForm header .actions .paging a.number:hover,div#EmailMessagesForm header .actions .paging a.number:hover,div#AuditForm header .actions .paging a.number:hover,div#ReviewerInvitationListForm header .actions .paging a.number:hover,div#ReviewerInvitationForSubmissionListForm header .actions .paging a.number:hover,div#userListForm header .actions .paging a.number:hover,div#AutoAssignmentPapers header .actions .paging a.number:hover,div#AutoAssignmentReviewers header .actions .paging a.number:hover,div#AutoAssignmentSettings header .actions .paging a.number:hover,div#AutoAssignmentConfirmation header .actions .paging a.number:hover{border-radius:4px;background-color:#f5f5f5;color:#0088ac}.table-common-container header .actions .paging .prev,div#ProceedingEditorSubmissions header .actions .paging .prev,div#divUserDisputeConflicts header .actions .paging .prev,div#metaReviewerListForm header .actions .paging .prev,div#reviewerListForm header .actions .paging .prev,div#DeletedSubmissionListForm header .actions .paging .prev,div#SuggestionForm header .actions .paging .prev,div#MetaBiddingForm header .actions .paging .prev,div#ExternalReviewForm header .actions .paging .prev,div#ReferenceForm header .actions .paging .prev,div#BiddingForm header .actions .paging .prev,div#SubmissionListForm header .actions .paging .prev,div#EmailMessagesForm header .actions .paging .prev,div#AuditForm header .actions .paging .prev,div#ReviewerInvitationListForm header .actions .paging .prev,div#ReviewerInvitationForSubmissionListForm header .actions .paging .prev,div#userListForm header .actions .paging .prev,div#AutoAssignmentPapers header .actions .paging .prev,div#AutoAssignmentReviewers header .actions .paging .prev,div#AutoAssignmentSettings header .actions .paging .prev,div#AutoAssignmentConfirmation header .actions .paging .prev,.table-common-container header .actions .paging .next,div#ProceedingEditorSubmissions header .actions .paging .next,div#divUserDisputeConflicts header .actions .paging .next,div#metaReviewerListForm header .actions .paging .next,div#reviewerListForm header .actions .paging .next,div#DeletedSubmissionListForm header .actions .paging .next,div#SuggestionForm header .actions .paging .next,div#MetaBiddingForm header .actions .paging .next,div#ExternalReviewForm header .actions .paging .next,div#ReferenceForm header .actions .paging .next,div#BiddingForm header .actions .paging .next,div#SubmissionListForm header .actions .paging .next,div#EmailMessagesForm header .actions .paging .next,div#AuditForm header .actions .paging .next,div#ReviewerInvitationListForm header .actions .paging .next,div#ReviewerInvitationForSubmissionListForm header .actions .paging .next,div#userListForm header .actions .paging .next,div#AutoAssignmentPapers header .actions .paging .next,div#AutoAssignmentReviewers header .actions .paging .next,div#AutoAssignmentSettings header .actions .paging .next,div#AutoAssignmentConfirmation header .actions .paging .next{width:10px}.table-common-container header .actions .paging .cur,div#ProceedingEditorSubmissions header .actions .paging .cur,div#divUserDisputeConflicts header .actions .paging .cur,div#metaReviewerListForm header .actions .paging .cur,div#reviewerListForm header .actions .paging .cur,div#DeletedSubmissionListForm header .actions .paging .cur,div#SuggestionForm header .actions .paging .cur,div#MetaBiddingForm header .actions .paging .cur,div#ExternalReviewForm header .actions .paging .cur,div#ReferenceForm header .actions .paging .cur,div#BiddingForm header .actions .paging .cur,div#SubmissionListForm header .actions .paging .cur,div#EmailMessagesForm header .actions .paging .cur,div#AuditForm header .actions .paging .cur,div#ReviewerInvitationListForm header .actions .paging .cur,div#ReviewerInvitationForSubmissionListForm header .actions .paging .cur,div#userListForm header .actions .paging .cur,div#AutoAssignmentPapers header .actions .paging .cur,div#AutoAssignmentReviewers header .actions .paging .cur,div#AutoAssignmentSettings header .actions .paging .cur,div#AutoAssignmentConfirmation header .actions .paging .cur{font-weight:bold;font-size:large}.table-common-container header .actions .act-title,div#ProceedingEditorSubmissions header .actions .act-title,div#divUserDisputeConflicts header .actions .act-title,div#metaReviewerListForm header .actions .act-title,div#reviewerListForm header .actions .act-title,div#DeletedSubmissionListForm header .actions .act-title,div#SuggestionForm header .actions .act-title,div#MetaBiddingForm header .actions .act-title,div#ExternalReviewForm header .actions .act-title,div#ReferenceForm header .actions .act-title,div#BiddingForm header .actions .act-title,div#SubmissionListForm header .actions .act-title,div#EmailMessagesForm header .actions .act-title,div#AuditForm header .actions .act-title,div#ReviewerInvitationListForm header .actions .act-title,div#ReviewerInvitationForSubmissionListForm header .actions .act-title,div#userListForm header .actions .act-title,div#AutoAssignmentPapers header .actions .act-title,div#AutoAssignmentReviewers header .actions .act-title,div#AutoAssignmentSettings header .actions .act-title,div#AutoAssignmentConfirmation header .actions .act-title{font-weight:normal}.table-common-container header .actions .act-title span,div#ProceedingEditorSubmissions header .actions .act-title span,div#divUserDisputeConflicts header .actions .act-title span,div#metaReviewerListForm header .actions .act-title span,div#reviewerListForm header .actions .act-title span,div#DeletedSubmissionListForm header .actions .act-title span,div#SuggestionForm header .actions .act-title span,div#MetaBiddingForm header .actions .act-title span,div#ExternalReviewForm header .actions .act-title span,div#ReferenceForm header .actions .act-title span,div#BiddingForm header .actions .act-title span,div#SubmissionListForm header .actions .act-title span,div#EmailMessagesForm header .actions .act-title span,div#AuditForm header .actions .act-title span,div#ReviewerInvitationListForm header .actions .act-title span,div#ReviewerInvitationForSubmissionListForm header .actions .act-title span,div#userListForm header .actions .act-title span,div#AutoAssignmentPapers header .actions .act-title span,div#AutoAssignmentReviewers header .actions .act-title span,div#AutoAssignmentSettings header .actions .act-title span,div#AutoAssignmentConfirmation header .actions .act-title span{height:9px}.table-common-container table th,div#ProceedingEditorSubmissions table th,div#divUserDisputeConflicts table th,div#metaReviewerListForm table th,div#reviewerListForm table th,div#DeletedSubmissionListForm table th,div#SuggestionForm table th,div#MetaBiddingForm table th,div#ExternalReviewForm table th,div#ReferenceForm table th,div#BiddingForm table th,div#SubmissionListForm table th,div#EmailMessagesForm table th,div#AuditForm table th,div#ReviewerInvitationListForm table th,div#ReviewerInvitationForSubmissionListForm table th,div#userListForm table th,div#AutoAssignmentPapers table th,div#AutoAssignmentReviewers table th,div#AutoAssignmentSettings table th,div#AutoAssignmentConfirmation table th{text-align:center;font-weight:normal}.table-common-container table td.narrower,div#ProceedingEditorSubmissions table td.narrower,div#divUserDisputeConflicts table td.narrower,div#metaReviewerListForm table td.narrower,div#reviewerListForm table td.narrower,div#DeletedSubmissionListForm table td.narrower,div#SuggestionForm table td.narrower,div#MetaBiddingForm table td.narrower,div#ExternalReviewForm table td.narrower,div#ReferenceForm table td.narrower,div#BiddingForm table td.narrower,div#SubmissionListForm table td.narrower,div#EmailMessagesForm table td.narrower,div#AuditForm table td.narrower,div#ReviewerInvitationListForm table td.narrower,div#ReviewerInvitationForSubmissionListForm table td.narrower,div#userListForm table td.narrower,div#AutoAssignmentPapers table td.narrower,div#AutoAssignmentReviewers table td.narrower,div#AutoAssignmentSettings table td.narrower,div#AutoAssignmentConfirmation table td.narrower,.table-common-container table th.narrower,div#ProceedingEditorSubmissions table th.narrower,div#divUserDisputeConflicts table th.narrower,div#metaReviewerListForm table th.narrower,div#reviewerListForm table th.narrower,div#DeletedSubmissionListForm table th.narrower,div#SuggestionForm table th.narrower,div#MetaBiddingForm table th.narrower,div#ExternalReviewForm table th.narrower,div#ReferenceForm table th.narrower,div#BiddingForm table th.narrower,div#SubmissionListForm table th.narrower,div#EmailMessagesForm table th.narrower,div#AuditForm table th.narrower,div#ReviewerInvitationListForm table th.narrower,div#ReviewerInvitationForSubmissionListForm table th.narrower,div#userListForm table th.narrower,div#AutoAssignmentPapers table th.narrower,div#AutoAssignmentReviewers table th.narrower,div#AutoAssignmentSettings table th.narrower,div#AutoAssignmentConfirmation table th.narrower{width:75px}.table-common-container table td.narrow,div#ProceedingEditorSubmissions table td.narrow,div#divUserDisputeConflicts table td.narrow,div#metaReviewerListForm table td.narrow,div#reviewerListForm table td.narrow,div#DeletedSubmissionListForm table td.narrow,div#SuggestionForm table td.narrow,div#MetaBiddingForm table td.narrow,div#ExternalReviewForm table td.narrow,div#ReferenceForm table td.narrow,div#BiddingForm table td.narrow,div#SubmissionListForm table td.narrow,div#EmailMessagesForm table td.narrow,div#AuditForm table td.narrow,div#ReviewerInvitationListForm table td.narrow,div#ReviewerInvitationForSubmissionListForm table td.narrow,div#userListForm table td.narrow,div#AutoAssignmentPapers table td.narrow,div#AutoAssignmentReviewers table td.narrow,div#AutoAssignmentSettings table td.narrow,div#AutoAssignmentConfirmation table td.narrow,.table-common-container table th.narrow,div#ProceedingEditorSubmissions table th.narrow,div#divUserDisputeConflicts table th.narrow,div#metaReviewerListForm table th.narrow,div#reviewerListForm table th.narrow,div#DeletedSubmissionListForm table th.narrow,div#SuggestionForm table th.narrow,div#MetaBiddingForm table th.narrow,div#ExternalReviewForm table th.narrow,div#ReferenceForm table th.narrow,div#BiddingForm table th.narrow,div#SubmissionListForm table th.narrow,div#EmailMessagesForm table th.narrow,div#AuditForm table th.narrow,div#ReviewerInvitationListForm table th.narrow,div#ReviewerInvitationForSubmissionListForm table th.narrow,div#userListForm table th.narrow,div#AutoAssignmentPapers table th.narrow,div#AutoAssignmentReviewers table th.narrow,div#AutoAssignmentSettings table th.narrow,div#AutoAssignmentConfirmation table th.narrow{width:100px}.table-common-container table thead tr:first-child th,div#ProceedingEditorSubmissions table thead tr:first-child th,div#divUserDisputeConflicts table thead tr:first-child th,div#metaReviewerListForm table thead tr:first-child th,div#reviewerListForm table thead tr:first-child th,div#DeletedSubmissionListForm table thead tr:first-child th,div#SuggestionForm table thead tr:first-child th,div#MetaBiddingForm table thead tr:first-child th,div#ExternalReviewForm table thead tr:first-child th,div#ReferenceForm table thead tr:first-child th,div#BiddingForm table thead tr:first-child th,div#SubmissionListForm table thead tr:first-child th,div#EmailMessagesForm table thead tr:first-child th,div#AuditForm table thead tr:first-child th,div#ReviewerInvitationListForm table thead tr:first-child th,div#ReviewerInvitationForSubmissionListForm table thead tr:first-child th,div#userListForm table thead tr:first-child th,div#AutoAssignmentPapers table thead tr:first-child th,div#AutoAssignmentReviewers table thead tr:first-child th,div#AutoAssignmentSettings table thead tr:first-child th,div#AutoAssignmentConfirmation table thead tr:first-child th{border-top:2px solid #ededed}.table-common-container table thead tr:last-child th,div#ProceedingEditorSubmissions table thead tr:last-child th,div#divUserDisputeConflicts table thead tr:last-child th,div#metaReviewerListForm table thead tr:last-child th,div#reviewerListForm table thead tr:last-child th,div#DeletedSubmissionListForm table thead tr:last-child th,div#SuggestionForm table thead tr:last-child th,div#MetaBiddingForm table thead tr:last-child th,div#ExternalReviewForm table thead tr:last-child th,div#ReferenceForm table thead tr:last-child th,div#BiddingForm table thead tr:last-child th,div#SubmissionListForm table thead tr:last-child th,div#EmailMessagesForm table thead tr:last-child th,div#AuditForm table thead tr:last-child th,div#ReviewerInvitationListForm table thead tr:last-child th,div#ReviewerInvitationForSubmissionListForm table thead tr:last-child th,div#userListForm table thead tr:last-child th,div#AutoAssignmentPapers table thead tr:last-child th,div#AutoAssignmentReviewers table thead tr:last-child th,div#AutoAssignmentSettings table thead tr:last-child th,div#AutoAssignmentConfirmation table thead tr:last-child th{border-bottom:2px solid #ededed}.table-common-container table thead th,div#ProceedingEditorSubmissions table thead th,div#divUserDisputeConflicts table thead th,div#metaReviewerListForm table thead th,div#reviewerListForm table thead th,div#DeletedSubmissionListForm table thead th,div#SuggestionForm table thead th,div#MetaBiddingForm table thead th,div#ExternalReviewForm table thead th,div#ReferenceForm table thead th,div#BiddingForm table thead th,div#SubmissionListForm table thead th,div#EmailMessagesForm table thead th,div#AuditForm table thead th,div#ReviewerInvitationListForm table thead th,div#ReviewerInvitationForSubmissionListForm table thead th,div#userListForm table thead th,div#AutoAssignmentPapers table thead th,div#AutoAssignmentReviewers table thead th,div#AutoAssignmentSettings table thead th,div#AutoAssignmentConfirmation table thead th{background-color:#efefef;color:#666}.table-common-container table thead th.txt>a.sortlink,div#ProceedingEditorSubmissions table thead th.txt>a.sortlink,div#divUserDisputeConflicts table thead th.txt>a.sortlink,div#metaReviewerListForm table thead th.txt>a.sortlink,div#reviewerListForm table thead th.txt>a.sortlink,div#DeletedSubmissionListForm table thead th.txt>a.sortlink,div#SuggestionForm table thead th.txt>a.sortlink,div#MetaBiddingForm table thead th.txt>a.sortlink,div#ExternalReviewForm table thead th.txt>a.sortlink,div#ReferenceForm table thead th.txt>a.sortlink,div#BiddingForm table thead th.txt>a.sortlink,div#SubmissionListForm table thead th.txt>a.sortlink,div#EmailMessagesForm table thead th.txt>a.sortlink,div#AuditForm table thead th.txt>a.sortlink,div#ReviewerInvitationListForm table thead th.txt>a.sortlink,div#ReviewerInvitationForSubmissionListForm table thead th.txt>a.sortlink,div#userListForm table thead th.txt>a.sortlink,div#AutoAssignmentPapers table thead th.txt>a.sortlink,div#AutoAssignmentReviewers table thead th.txt>a.sortlink,div#AutoAssignmentSettings table thead th.txt>a.sortlink,div#AutoAssignmentConfirmation table thead th.txt>a.sortlink{text-decoration:none;color:inherit}.table-common-container table thead th.txt:hover,div#ProceedingEditorSubmissions table thead th.txt:hover,div#divUserDisputeConflicts table thead th.txt:hover,div#metaReviewerListForm table thead th.txt:hover,div#reviewerListForm table thead th.txt:hover,div#DeletedSubmissionListForm table thead th.txt:hover,div#SuggestionForm table thead th.txt:hover,div#MetaBiddingForm table thead th.txt:hover,div#ExternalReviewForm table thead th.txt:hover,div#ReferenceForm table thead th.txt:hover,div#BiddingForm table thead th.txt:hover,div#SubmissionListForm table thead th.txt:hover,div#EmailMessagesForm table thead th.txt:hover,div#AuditForm table thead th.txt:hover,div#ReviewerInvitationListForm table thead th.txt:hover,div#ReviewerInvitationForSubmissionListForm table thead th.txt:hover,div#userListForm table thead th.txt:hover,div#AutoAssignmentPapers table thead th.txt:hover,div#AutoAssignmentReviewers table thead th.txt:hover,div#AutoAssignmentSettings table thead th.txt:hover,div#AutoAssignmentConfirmation table thead th.txt:hover{cursor:pointer;text-decoration:underline}.table-common-container table #filters .query,div#ProceedingEditorSubmissions table #filters .query,div#divUserDisputeConflicts table #filters .query,div#metaReviewerListForm table #filters .query,div#reviewerListForm table #filters .query,div#DeletedSubmissionListForm table #filters .query,div#SuggestionForm table #filters .query,div#MetaBiddingForm table #filters .query,div#ExternalReviewForm table #filters .query,div#ReferenceForm table #filters .query,div#BiddingForm table #filters .query,div#SubmissionListForm table #filters .query,div#EmailMessagesForm table #filters .query,div#AuditForm table #filters .query,div#ReviewerInvitationListForm table #filters .query,div#ReviewerInvitationForSubmissionListForm table #filters .query,div#userListForm table #filters .query,div#AutoAssignmentPapers table #filters .query,div#AutoAssignmentReviewers table #filters .query,div#AutoAssignmentSettings table #filters .query,div#AutoAssignmentConfirmation table #filters .query{width:100%;height:40px;position:relative}.table-common-container table #filters .query input,div#ProceedingEditorSubmissions table #filters .query input,div#divUserDisputeConflicts table #filters .query input,div#metaReviewerListForm table #filters .query input,div#reviewerListForm table #filters .query input,div#DeletedSubmissionListForm table #filters .query input,div#SuggestionForm table #filters .query input,div#MetaBiddingForm table #filters .query input,div#ExternalReviewForm table #filters .query input,div#ReferenceForm table #filters .query input,div#BiddingForm table #filters .query input,div#SubmissionListForm table #filters .query input,div#EmailMessagesForm table #filters .query input,div#AuditForm table #filters .query input,div#ReviewerInvitationListForm table #filters .query input,div#ReviewerInvitationForSubmissionListForm table #filters .query input,div#userListForm table #filters .query input,div#AutoAssignmentPapers table #filters .query input,div#AutoAssignmentReviewers table #filters .query input,div#AutoAssignmentSettings table #filters .query input,div#AutoAssignmentConfirmation table #filters .query input{width:calc(100% - 12px);border-radius:10px}.table-common-container table #filters .query input.error,div#ProceedingEditorSubmissions table #filters .query input.error,div#divUserDisputeConflicts table #filters .query input.error,div#metaReviewerListForm table #filters .query input.error,div#reviewerListForm table #filters .query input.error,div#DeletedSubmissionListForm table #filters .query input.error,div#SuggestionForm table #filters .query input.error,div#MetaBiddingForm table #filters .query input.error,div#ExternalReviewForm table #filters .query input.error,div#ReferenceForm table #filters .query input.error,div#BiddingForm table #filters .query input.error,div#SubmissionListForm table #filters .query input.error,div#EmailMessagesForm table #filters .query input.error,div#AuditForm table #filters .query input.error,div#ReviewerInvitationListForm table #filters .query input.error,div#ReviewerInvitationForSubmissionListForm table #filters .query input.error,div#userListForm table #filters .query input.error,div#AutoAssignmentPapers table #filters .query input.error,div#AutoAssignmentReviewers table #filters .query input.error,div#AutoAssignmentSettings table #filters .query input.error,div#AutoAssignmentConfirmation table #filters .query input.error{background-color:#f5b7b7}.table-common-container table #filters .query input:not(:focus),div#ProceedingEditorSubmissions table #filters .query input:not(:focus),div#divUserDisputeConflicts table #filters .query input:not(:focus),div#metaReviewerListForm table #filters .query input:not(:focus),div#reviewerListForm table #filters .query input:not(:focus),div#DeletedSubmissionListForm table #filters .query input:not(:focus),div#SuggestionForm table #filters .query input:not(:focus),div#MetaBiddingForm table #filters .query input:not(:focus),div#ExternalReviewForm table #filters .query input:not(:focus),div#ReferenceForm table #filters .query input:not(:focus),div#BiddingForm table #filters .query input:not(:focus),div#SubmissionListForm table #filters .query input:not(:focus),div#EmailMessagesForm table #filters .query input:not(:focus),div#AuditForm table #filters .query input:not(:focus),div#ReviewerInvitationListForm table #filters .query input:not(:focus),div#ReviewerInvitationForSubmissionListForm table #filters .query input:not(:focus),div#userListForm table #filters .query input:not(:focus),div#AutoAssignmentPapers table #filters .query input:not(:focus),div#AutoAssignmentReviewers table #filters .query input:not(:focus),div#AutoAssignmentSettings table #filters .query input:not(:focus),div#AutoAssignmentConfirmation table #filters .query input:not(:focus){color:#707070}.table-common-container table #filters .query i,div#ProceedingEditorSubmissions table #filters .query i,div#divUserDisputeConflicts table #filters .query i,div#metaReviewerListForm table #filters .query i,div#reviewerListForm table #filters .query i,div#DeletedSubmissionListForm table #filters .query i,div#SuggestionForm table #filters .query i,div#MetaBiddingForm table #filters .query i,div#ExternalReviewForm table #filters .query i,div#ReferenceForm table #filters .query i,div#BiddingForm table #filters .query i,div#SubmissionListForm table #filters .query i,div#EmailMessagesForm table #filters .query i,div#AuditForm table #filters .query i,div#ReviewerInvitationListForm table #filters .query i,div#ReviewerInvitationForSubmissionListForm table #filters .query i,div#userListForm table #filters .query i,div#AutoAssignmentPapers table #filters .query i,div#AutoAssignmentReviewers table #filters .query i,div#AutoAssignmentSettings table #filters .query i,div#AutoAssignmentConfirmation table #filters .query i{position:absolute;top:7px;right:5px;cursor:pointer}.table-common-container table #filters .query .link-remove,div#ProceedingEditorSubmissions table #filters .query .link-remove,div#divUserDisputeConflicts table #filters .query .link-remove,div#metaReviewerListForm table #filters .query .link-remove,div#reviewerListForm table #filters .query .link-remove,div#DeletedSubmissionListForm table #filters .query .link-remove,div#SuggestionForm table #filters .query .link-remove,div#MetaBiddingForm table #filters .query .link-remove,div#ExternalReviewForm table #filters .query .link-remove,div#ReferenceForm table #filters .query .link-remove,div#BiddingForm table #filters .query .link-remove,div#SubmissionListForm table #filters .query .link-remove,div#EmailMessagesForm table #filters .query .link-remove,div#AuditForm table #filters .query .link-remove,div#ReviewerInvitationListForm table #filters .query .link-remove,div#ReviewerInvitationForSubmissionListForm table #filters .query .link-remove,div#userListForm table #filters .query .link-remove,div#AutoAssignmentPapers table #filters .query .link-remove,div#AutoAssignmentReviewers table #filters .query .link-remove,div#AutoAssignmentSettings table #filters .query .link-remove,div#AutoAssignmentConfirmation table #filters .query .link-remove{position:absolute;top:29px;right:5px;font-size:8px;font-family:Arial;font-style:italic;cursor:pointer}.table-common-container table #filters .selector,div#ProceedingEditorSubmissions table #filters .selector,div#divUserDisputeConflicts table #filters .selector,div#metaReviewerListForm table #filters .selector,div#reviewerListForm table #filters .selector,div#DeletedSubmissionListForm table #filters .selector,div#SuggestionForm table #filters .selector,div#MetaBiddingForm table #filters .selector,div#ExternalReviewForm table #filters .selector,div#ReferenceForm table #filters .selector,div#BiddingForm table #filters .selector,div#SubmissionListForm table #filters .selector,div#EmailMessagesForm table #filters .selector,div#AuditForm table #filters .selector,div#ReviewerInvitationListForm table #filters .selector,div#ReviewerInvitationForSubmissionListForm table #filters .selector,div#userListForm table #filters .selector,div#AutoAssignmentPapers table #filters .selector,div#AutoAssignmentReviewers table #filters .selector,div#AutoAssignmentSettings table #filters .selector,div#AutoAssignmentConfirmation table #filters .selector{background-color:#fff;border:1px solid #ddd;-webkit-box-shadow:0 5px 10px rgba(0,0,0,.2);-moz-box-shadow:0 5px 10px rgba(0,0,0,.2);box-shadow:0 5px 10px rgba(0,0,0,.2);padding:5px;border-radius:10px;position:relative;z-index:5;width:150%}.table-common-container table #filters .selector .selected .all,div#ProceedingEditorSubmissions table #filters .selector .selected .all,div#divUserDisputeConflicts table #filters .selector .selected .all,div#metaReviewerListForm table #filters .selector .selected .all,div#reviewerListForm table #filters .selector .selected .all,div#DeletedSubmissionListForm table #filters .selector .selected .all,div#SuggestionForm table #filters .selector .selected .all,div#MetaBiddingForm table #filters .selector .selected .all,div#ExternalReviewForm table #filters .selector .selected .all,div#ReferenceForm table #filters .selector .selected .all,div#BiddingForm table #filters .selector .selected .all,div#SubmissionListForm table #filters .selector .selected .all,div#EmailMessagesForm table #filters .selector .selected .all,div#AuditForm table #filters .selector .selected .all,div#ReviewerInvitationListForm table #filters .selector .selected .all,div#ReviewerInvitationForSubmissionListForm table #filters .selector .selected .all,div#userListForm table #filters .selector .selected .all,div#AutoAssignmentPapers table #filters .selector .selected .all,div#AutoAssignmentReviewers table #filters .selector .selected .all,div#AutoAssignmentSettings table #filters .selector .selected .all,div#AutoAssignmentConfirmation table #filters .selector .selected .all,.table-common-container table #filters .selector .found .all,div#ProceedingEditorSubmissions table #filters .selector .found .all,div#divUserDisputeConflicts table #filters .selector .found .all,div#metaReviewerListForm table #filters .selector .found .all,div#reviewerListForm table #filters .selector .found .all,div#DeletedSubmissionListForm table #filters .selector .found .all,div#SuggestionForm table #filters .selector .found .all,div#MetaBiddingForm table #filters .selector .found .all,div#ExternalReviewForm table #filters .selector .found .all,div#ReferenceForm table #filters .selector .found .all,div#BiddingForm table #filters .selector .found .all,div#SubmissionListForm table #filters .selector .found .all,div#EmailMessagesForm table #filters .selector .found .all,div#AuditForm table #filters .selector .found .all,div#ReviewerInvitationListForm table #filters .selector .found .all,div#ReviewerInvitationForSubmissionListForm table #filters .selector .found .all,div#userListForm table #filters .selector .found .all,div#AutoAssignmentPapers table #filters .selector .found .all,div#AutoAssignmentReviewers table #filters .selector .found .all,div#AutoAssignmentSettings table #filters .selector .found .all,div#AutoAssignmentConfirmation table #filters .selector .found .all{border-bottom:1px solid #ddd;background-color:#ddd;border-radius:5px 5px 0 0;padding-top:3px}.table-common-container table #filters .selector .selected .all input,div#ProceedingEditorSubmissions table #filters .selector .selected .all input,div#divUserDisputeConflicts table #filters .selector .selected .all input,div#metaReviewerListForm table #filters .selector .selected .all input,div#reviewerListForm table #filters .selector .selected .all input,div#DeletedSubmissionListForm table #filters .selector .selected .all input,div#SuggestionForm table #filters .selector .selected .all input,div#MetaBiddingForm table #filters .selector .selected .all input,div#ExternalReviewForm table #filters .selector .selected .all input,div#ReferenceForm table #filters .selector .selected .all input,div#BiddingForm table #filters .selector .selected .all input,div#SubmissionListForm table #filters .selector .selected .all input,div#EmailMessagesForm table #filters .selector .selected .all input,div#AuditForm table #filters .selector .selected .all input,div#ReviewerInvitationListForm table #filters .selector .selected .all input,div#ReviewerInvitationForSubmissionListForm table #filters .selector .selected .all input,div#userListForm table #filters .selector .selected .all input,div#AutoAssignmentPapers table #filters .selector .selected .all input,div#AutoAssignmentReviewers table #filters .selector .selected .all input,div#AutoAssignmentSettings table #filters .selector .selected .all input,div#AutoAssignmentConfirmation table #filters .selector .selected .all input,.table-common-container table #filters .selector .found .all input,div#ProceedingEditorSubmissions table #filters .selector .found .all input,div#divUserDisputeConflicts table #filters .selector .found .all input,div#metaReviewerListForm table #filters .selector .found .all input,div#reviewerListForm table #filters .selector .found .all input,div#DeletedSubmissionListForm table #filters .selector .found .all input,div#SuggestionForm table #filters .selector .found .all input,div#MetaBiddingForm table #filters .selector .found .all input,div#ExternalReviewForm table #filters .selector .found .all input,div#ReferenceForm table #filters .selector .found .all input,div#BiddingForm table #filters .selector .found .all input,div#SubmissionListForm table #filters .selector .found .all input,div#EmailMessagesForm table #filters .selector .found .all input,div#AuditForm table #filters .selector .found .all input,div#ReviewerInvitationListForm table #filters .selector .found .all input,div#ReviewerInvitationForSubmissionListForm table #filters .selector .found .all input,div#userListForm table #filters .selector .found .all input,div#AutoAssignmentPapers table #filters .selector .found .all input,div#AutoAssignmentReviewers table #filters .selector .found .all input,div#AutoAssignmentSettings table #filters .selector .found .all input,div#AutoAssignmentConfirmation table #filters .selector .found .all input{width:20px;margin:0}.table-common-container table #filters .selector .selected .all label,div#ProceedingEditorSubmissions table #filters .selector .selected .all label,div#divUserDisputeConflicts table #filters .selector .selected .all label,div#metaReviewerListForm table #filters .selector .selected .all label,div#reviewerListForm table #filters .selector .selected .all label,div#DeletedSubmissionListForm table #filters .selector .selected .all label,div#SuggestionForm table #filters .selector .selected .all label,div#MetaBiddingForm table #filters .selector .selected .all label,div#ExternalReviewForm table #filters .selector .selected .all label,div#ReferenceForm table #filters .selector .selected .all label,div#BiddingForm table #filters .selector .selected .all label,div#SubmissionListForm table #filters .selector .selected .all label,div#EmailMessagesForm table #filters .selector .selected .all label,div#AuditForm table #filters .selector .selected .all label,div#ReviewerInvitationListForm table #filters .selector .selected .all label,div#ReviewerInvitationForSubmissionListForm table #filters .selector .selected .all label,div#userListForm table #filters .selector .selected .all label,div#AutoAssignmentPapers table #filters .selector .selected .all label,div#AutoAssignmentReviewers table #filters .selector .selected .all label,div#AutoAssignmentSettings table #filters .selector .selected .all label,div#AutoAssignmentConfirmation table #filters .selector .selected .all label,.table-common-container table #filters .selector .found .all label,div#ProceedingEditorSubmissions table #filters .selector .found .all label,div#divUserDisputeConflicts table #filters .selector .found .all label,div#metaReviewerListForm table #filters .selector .found .all label,div#reviewerListForm table #filters .selector .found .all label,div#DeletedSubmissionListForm table #filters .selector .found .all label,div#SuggestionForm table #filters .selector .found .all label,div#MetaBiddingForm table #filters .selector .found .all label,div#ExternalReviewForm table #filters .selector .found .all label,div#ReferenceForm table #filters .selector .found .all label,div#BiddingForm table #filters .selector .found .all label,div#SubmissionListForm table #filters .selector .found .all label,div#EmailMessagesForm table #filters .selector .found .all label,div#AuditForm table #filters .selector .found .all label,div#ReviewerInvitationListForm table #filters .selector .found .all label,div#ReviewerInvitationForSubmissionListForm table #filters .selector .found .all label,div#userListForm table #filters .selector .found .all label,div#AutoAssignmentPapers table #filters .selector .found .all label,div#AutoAssignmentReviewers table #filters .selector .found .all label,div#AutoAssignmentSettings table #filters .selector .found .all label,div#AutoAssignmentConfirmation table #filters .selector .found .all label{background-color:#ddd;color:#000;font-size:12px;border-radius:3px 3px 0 0}.table-common-container table #filters .selector .selected .list,div#ProceedingEditorSubmissions table #filters .selector .selected .list,div#divUserDisputeConflicts table #filters .selector .selected .list,div#metaReviewerListForm table #filters .selector .selected .list,div#reviewerListForm table #filters .selector .selected .list,div#DeletedSubmissionListForm table #filters .selector .selected .list,div#SuggestionForm table #filters .selector .selected .list,div#MetaBiddingForm table #filters .selector .selected .list,div#ExternalReviewForm table #filters .selector .selected .list,div#ReferenceForm table #filters .selector .selected .list,div#BiddingForm table #filters .selector .selected .list,div#SubmissionListForm table #filters .selector .selected .list,div#EmailMessagesForm table #filters .selector .selected .list,div#AuditForm table #filters .selector .selected .list,div#ReviewerInvitationListForm table #filters .selector .selected .list,div#ReviewerInvitationForSubmissionListForm table #filters .selector .selected .list,div#userListForm table #filters .selector .selected .list,div#AutoAssignmentPapers table #filters .selector .selected .list,div#AutoAssignmentReviewers table #filters .selector .selected .list,div#AutoAssignmentSettings table #filters .selector .selected .list,div#AutoAssignmentConfirmation table #filters .selector .selected .list,.table-common-container table #filters .selector .found .list,div#ProceedingEditorSubmissions table #filters .selector .found .list,div#divUserDisputeConflicts table #filters .selector .found .list,div#metaReviewerListForm table #filters .selector .found .list,div#reviewerListForm table #filters .selector .found .list,div#DeletedSubmissionListForm table #filters .selector .found .list,div#SuggestionForm table #filters .selector .found .list,div#MetaBiddingForm table #filters .selector .found .list,div#ExternalReviewForm table #filters .selector .found .list,div#ReferenceForm table #filters .selector .found .list,div#BiddingForm table #filters .selector .found .list,div#SubmissionListForm table #filters .selector .found .list,div#EmailMessagesForm table #filters .selector .found .list,div#AuditForm table #filters .selector .found .list,div#ReviewerInvitationListForm table #filters .selector .found .list,div#ReviewerInvitationForSubmissionListForm table #filters .selector .found .list,div#userListForm table #filters .selector .found .list,div#AutoAssignmentPapers table #filters .selector .found .list,div#AutoAssignmentReviewers table #filters .selector .found .list,div#AutoAssignmentSettings table #filters .selector .found .list,div#AutoAssignmentConfirmation table #filters .selector .found .list{list-style-type:none;padding:0;margin:0;max-height:30vh;overflow-y:auto}.table-common-container table #filters .selector .selected .list li,div#ProceedingEditorSubmissions table #filters .selector .selected .list li,div#divUserDisputeConflicts table #filters .selector .selected .list li,div#metaReviewerListForm table #filters .selector .selected .list li,div#reviewerListForm table #filters .selector .selected .list li,div#DeletedSubmissionListForm table #filters .selector .selected .list li,div#SuggestionForm table #filters .selector .selected .list li,div#MetaBiddingForm table #filters .selector .selected .list li,div#ExternalReviewForm table #filters .selector .selected .list li,div#ReferenceForm table #filters .selector .selected .list li,div#BiddingForm table #filters .selector .selected .list li,div#SubmissionListForm table #filters .selector .selected .list li,div#EmailMessagesForm table #filters .selector .selected .list li,div#AuditForm table #filters .selector .selected .list li,div#ReviewerInvitationListForm table #filters .selector .selected .list li,div#ReviewerInvitationForSubmissionListForm table #filters .selector .selected .list li,div#userListForm table #filters .selector .selected .list li,div#AutoAssignmentPapers table #filters .selector .selected .list li,div#AutoAssignmentReviewers table #filters .selector .selected .list li,div#AutoAssignmentSettings table #filters .selector .selected .list li,div#AutoAssignmentConfirmation table #filters .selector .selected .list li,.table-common-container table #filters .selector .found .list li,div#ProceedingEditorSubmissions table #filters .selector .found .list li,div#divUserDisputeConflicts table #filters .selector .found .list li,div#metaReviewerListForm table #filters .selector .found .list li,div#reviewerListForm table #filters .selector .found .list li,div#DeletedSubmissionListForm table #filters .selector .found .list li,div#SuggestionForm table #filters .selector .found .list li,div#MetaBiddingForm table #filters .selector .found .list li,div#ExternalReviewForm table #filters .selector .found .list li,div#ReferenceForm table #filters .selector .found .list li,div#BiddingForm table #filters .selector .found .list li,div#SubmissionListForm table #filters .selector .found .list li,div#EmailMessagesForm table #filters .selector .found .list li,div#AuditForm table #filters .selector .found .list li,div#ReviewerInvitationListForm table #filters .selector .found .list li,div#ReviewerInvitationForSubmissionListForm table #filters .selector .found .list li,div#userListForm table #filters .selector .found .list li,div#AutoAssignmentPapers table #filters .selector .found .list li,div#AutoAssignmentReviewers table #filters .selector .found .list li,div#AutoAssignmentSettings table #filters .selector .found .list li,div#AutoAssignmentConfirmation table #filters .selector .found .list li{padding:5px 0;margin:0;border-bottom:1px solid #ddd;text-align:left;font-family:'Helvetica Neue',Helvetica,Arial,sans-serif;text-transform:capitalize}.table-common-container table #filters .selector .selected .list li:hover,div#ProceedingEditorSubmissions table #filters .selector .selected .list li:hover,div#divUserDisputeConflicts table #filters .selector .selected .list li:hover,div#metaReviewerListForm table #filters .selector .selected .list li:hover,div#reviewerListForm table #filters .selector .selected .list li:hover,div#DeletedSubmissionListForm table #filters .selector .selected .list li:hover,div#SuggestionForm table #filters .selector .selected .list li:hover,div#MetaBiddingForm table #filters .selector .selected .list li:hover,div#ExternalReviewForm table #filters .selector .selected .list li:hover,div#ReferenceForm table #filters .selector .selected .list li:hover,div#BiddingForm table #filters .selector .selected .list li:hover,div#SubmissionListForm table #filters .selector .selected .list li:hover,div#EmailMessagesForm table #filters .selector .selected .list li:hover,div#AuditForm table #filters .selector .selected .list li:hover,div#ReviewerInvitationListForm table #filters .selector .selected .list li:hover,div#ReviewerInvitationForSubmissionListForm table #filters .selector .selected .list li:hover,div#userListForm table #filters .selector .selected .list li:hover,div#AutoAssignmentPapers table #filters .selector .selected .list li:hover,div#AutoAssignmentReviewers table #filters .selector .selected .list li:hover,div#AutoAssignmentSettings table #filters .selector .selected .list li:hover,div#AutoAssignmentConfirmation table #filters .selector .selected .list li:hover,.table-common-container table #filters .selector .found .list li:hover,div#ProceedingEditorSubmissions table #filters .selector .found .list li:hover,div#divUserDisputeConflicts table #filters .selector .found .list li:hover,div#metaReviewerListForm table #filters .selector .found .list li:hover,div#reviewerListForm table #filters .selector .found .list li:hover,div#DeletedSubmissionListForm table #filters .selector .found .list li:hover,div#SuggestionForm table #filters .selector .found .list li:hover,div#MetaBiddingForm table #filters .selector .found .list li:hover,div#ExternalReviewForm table #filters .selector .found .list li:hover,div#ReferenceForm table #filters .selector .found .list li:hover,div#BiddingForm table #filters .selector .found .list li:hover,div#SubmissionListForm table #filters .selector .found .list li:hover,div#EmailMessagesForm table #filters .selector .found .list li:hover,div#AuditForm table #filters .selector .found .list li:hover,div#ReviewerInvitationListForm table #filters .selector .found .list li:hover,div#ReviewerInvitationForSubmissionListForm table #filters .selector .found .list li:hover,div#userListForm table #filters .selector .found .list li:hover,div#AutoAssignmentPapers table #filters .selector .found .list li:hover,div#AutoAssignmentReviewers table #filters .selector .found .list li:hover,div#AutoAssignmentSettings table #filters .selector .found .list li:hover,div#AutoAssignmentConfirmation table #filters .selector .found .list li:hover{text-decoration:none;color:#fff;background-color:#007699;background-image:-moz-linear-gradient(top,#007ea3,#006a8a);background-image:-webkit-gradient(linear,0 0,0 100%,from(#007ea3),to(#006a8a));background-image:-webkit-linear-gradient(top,#007ea3,#006a8a);background-image:-o-linear-gradient(top,#007ea3,#006a8a);background-image:linear-gradient(to bottom,#007ea3,#006a8a);background-repeat:repeat-x;filter:progid:DXImageTransform.Microsoft.gradient(startColorstr='#ff007ea3',endColorstr='#ff006a8a',GradientType=0);cursor:pointer}.table-common-container table #filters .selector .selected .list .item input,div#ProceedingEditorSubmissions table #filters .selector .selected .list .item input,div#divUserDisputeConflicts table #filters .selector .selected .list .item input,div#metaReviewerListForm table #filters .selector .selected .list .item input,div#reviewerListForm table #filters .selector .selected .list .item input,div#DeletedSubmissionListForm table #filters .selector .selected .list .item input,div#SuggestionForm table #filters .selector .selected .list .item input,div#MetaBiddingForm table #filters .selector .selected .list .item input,div#ExternalReviewForm table #filters .selector .selected .list .item input,div#ReferenceForm table #filters .selector .selected .list .item input,div#BiddingForm table #filters .selector .selected .list .item input,div#SubmissionListForm table #filters .selector .selected .list .item input,div#EmailMessagesForm table #filters .selector .selected .list .item input,div#AuditForm table #filters .selector .selected .list .item input,div#ReviewerInvitationListForm table #filters .selector .selected .list .item input,div#ReviewerInvitationForSubmissionListForm table #filters .selector .selected .list .item input,div#userListForm table #filters .selector .selected .list .item input,div#AutoAssignmentPapers table #filters .selector .selected .list .item input,div#AutoAssignmentReviewers table #filters .selector .selected .list .item input,div#AutoAssignmentSettings table #filters .selector .selected .list .item input,div#AutoAssignmentConfirmation table #filters .selector .selected .list .item input,.table-common-container table #filters .selector .found .list .item input,div#ProceedingEditorSubmissions table #filters .selector .found .list .item input,div#divUserDisputeConflicts table #filters .selector .found .list .item input,div#metaReviewerListForm table #filters .selector .found .list .item input,div#reviewerListForm table #filters .selector .found .list .item input,div#DeletedSubmissionListForm table #filters .selector .found .list .item input,div#SuggestionForm table #filters .selector .found .list .item input,div#MetaBiddingForm table #filters .selector .found .list .item input,div#ExternalReviewForm table #filters .selector .found .list .item input,div#ReferenceForm table #filters .selector .found .list .item input,div#BiddingForm table #filters .selector .found .list .item input,div#SubmissionListForm table #filters .selector .found .list .item input,div#EmailMessagesForm table #filters .selector .found .list .item input,div#AuditForm table #filters .selector .found .list .item input,div#ReviewerInvitationListForm table #filters .selector .found .list .item input,div#ReviewerInvitationForSubmissionListForm table #filters .selector .found .list .item input,div#userListForm table #filters .selector .found .list .item input,div#AutoAssignmentPapers table #filters .selector .found .list .item input,div#AutoAssignmentReviewers table #filters .selector .found .list .item input,div#AutoAssignmentSettings table #filters .selector .found .list .item input,div#AutoAssignmentConfirmation table #filters .selector .found .list .item input{width:20px;margin:0}.table-common-container table #filters .selector .selected .list .item span,div#ProceedingEditorSubmissions table #filters .selector .selected .list .item span,div#divUserDisputeConflicts table #filters .selector .selected .list .item span,div#metaReviewerListForm table #filters .selector .selected .list .item span,div#reviewerListForm table #filters .selector .selected .list .item span,div#DeletedSubmissionListForm table #filters .selector .selected .list .item span,div#SuggestionForm table #filters .selector .selected .list .item span,div#MetaBiddingForm table #filters .selector .selected .list .item span,div#ExternalReviewForm table #filters .selector .selected .list .item span,div#ReferenceForm table #filters .selector .selected .list .item span,div#BiddingForm table #filters .selector .selected .list .item span,div#SubmissionListForm table #filters .selector .selected .list .item span,div#EmailMessagesForm table #filters .selector .selected .list .item span,div#AuditForm table #filters .selector .selected .list .item span,div#ReviewerInvitationListForm table #filters .selector .selected .list .item span,div#ReviewerInvitationForSubmissionListForm table #filters .selector .selected .list .item span,div#userListForm table #filters .selector .selected .list .item span,div#AutoAssignmentPapers table #filters .selector .selected .list .item span,div#AutoAssignmentReviewers table #filters .selector .selected .list .item span,div#AutoAssignmentSettings table #filters .selector .selected .list .item span,div#AutoAssignmentConfirmation table #filters .selector .selected .list .item span,.table-common-container table #filters .selector .found .list .item span,div#ProceedingEditorSubmissions table #filters .selector .found .list .item span,div#divUserDisputeConflicts table #filters .selector .found .list .item span,div#metaReviewerListForm table #filters .selector .found .list .item span,div#reviewerListForm table #filters .selector .found .list .item span,div#DeletedSubmissionListForm table #filters .selector .found .list .item span,div#SuggestionForm table #filters .selector .found .list .item span,div#MetaBiddingForm table #filters .selector .found .list .item span,div#ExternalReviewForm table #filters .selector .found .list .item span,div#ReferenceForm table #filters .selector .found .list .item span,div#BiddingForm table #filters .selector .found .list .item span,div#SubmissionListForm table #filters .selector .found .list .item span,div#EmailMessagesForm table #filters .selector .found .list .item span,div#AuditForm table #filters .selector .found .list .item span,div#ReviewerInvitationListForm table #filters .selector .found .list .item span,div#ReviewerInvitationForSubmissionListForm table #filters .selector .found .list .item span,div#userListForm table #filters .selector .found .list .item span,div#AutoAssignmentPapers table #filters .selector .found .list .item span,div#AutoAssignmentReviewers table #filters .selector .found .list .item span,div#AutoAssignmentSettings table #filters .selector .found .list .item span,div#AutoAssignmentConfirmation table #filters .selector .found .list .item span{position:initial;font-size:13px;font-weight:normal;font-style:normal}.table-common-container table #filters .selector .found .all,div#ProceedingEditorSubmissions table #filters .selector .found .all,div#divUserDisputeConflicts table #filters .selector .found .all,div#metaReviewerListForm table #filters .selector .found .all,div#reviewerListForm table #filters .selector .found .all,div#DeletedSubmissionListForm table #filters .selector .found .all,div#SuggestionForm table #filters .selector .found .all,div#MetaBiddingForm table #filters .selector .found .all,div#ExternalReviewForm table #filters .selector .found .all,div#ReferenceForm table #filters .selector .found .all,div#BiddingForm table #filters .selector .found .all,div#SubmissionListForm table #filters .selector .found .all,div#EmailMessagesForm table #filters .selector .found .all,div#AuditForm table #filters .selector .found .all,div#ReviewerInvitationListForm table #filters .selector .found .all,div#ReviewerInvitationForSubmissionListForm table #filters .selector .found .all,div#userListForm table #filters .selector .found .all,div#AutoAssignmentPapers table #filters .selector .found .all,div#AutoAssignmentReviewers table #filters .selector .found .all,div#AutoAssignmentSettings table #filters .selector .found .all,div#AutoAssignmentConfirmation table #filters .selector .found .all{border-radius:0}.table-common-container table #filters .selector .actions,div#ProceedingEditorSubmissions table #filters .selector .actions,div#divUserDisputeConflicts table #filters .selector .actions,div#metaReviewerListForm table #filters .selector .actions,div#reviewerListForm table #filters .selector .actions,div#DeletedSubmissionListForm table #filters .selector .actions,div#SuggestionForm table #filters .selector .actions,div#MetaBiddingForm table #filters .selector .actions,div#ExternalReviewForm table #filters .selector .actions,div#ReferenceForm table #filters .selector .actions,div#BiddingForm table #filters .selector .actions,div#SubmissionListForm table #filters .selector .actions,div#EmailMessagesForm table #filters .selector .actions,div#AuditForm table #filters .selector .actions,div#ReviewerInvitationListForm table #filters .selector .actions,div#ReviewerInvitationForSubmissionListForm table #filters .selector .actions,div#userListForm table #filters .selector .actions,div#AutoAssignmentPapers table #filters .selector .actions,div#AutoAssignmentReviewers table #filters .selector .actions,div#AutoAssignmentSettings table #filters .selector .actions,div#AutoAssignmentConfirmation table #filters .selector .actions{padding:3px 0;position:relative;text-align:center;background-color:#0088ac;border-radius:0 0 5px 5px}.table-common-container table #filters .selector .actions a,div#ProceedingEditorSubmissions table #filters .selector .actions a,div#divUserDisputeConflicts table #filters .selector .actions a,div#metaReviewerListForm table #filters .selector .actions a,div#reviewerListForm table #filters .selector .actions a,div#DeletedSubmissionListForm table #filters .selector .actions a,div#SuggestionForm table #filters .selector .actions a,div#MetaBiddingForm table #filters .selector .actions a,div#ExternalReviewForm table #filters .selector .actions a,div#ReferenceForm table #filters .selector .actions a,div#BiddingForm table #filters .selector .actions a,div#SubmissionListForm table #filters .selector .actions a,div#EmailMessagesForm table #filters .selector .actions a,div#AuditForm table #filters .selector .actions a,div#ReviewerInvitationListForm table #filters .selector .actions a,div#ReviewerInvitationForSubmissionListForm table #filters .selector .actions a,div#userListForm table #filters .selector .actions a,div#AutoAssignmentPapers table #filters .selector .actions a,div#AutoAssignmentReviewers table #filters .selector .actions a,div#AutoAssignmentSettings table #filters .selector .actions a,div#AutoAssignmentConfirmation table #filters .selector .actions a{margin:0 5px;font-size:12px}.table-common-container table .marked,div#ProceedingEditorSubmissions table .marked,div#divUserDisputeConflicts table .marked,div#metaReviewerListForm table .marked,div#reviewerListForm table .marked,div#DeletedSubmissionListForm table .marked,div#SuggestionForm table .marked,div#MetaBiddingForm table .marked,div#ExternalReviewForm table .marked,div#ReferenceForm table .marked,div#BiddingForm table .marked,div#SubmissionListForm table .marked,div#EmailMessagesForm table .marked,div#AuditForm table .marked,div#ReviewerInvitationListForm table .marked,div#ReviewerInvitationForSubmissionListForm table .marked,div#userListForm table .marked,div#AutoAssignmentPapers table .marked,div#AutoAssignmentReviewers table .marked,div#AutoAssignmentSettings table .marked,div#AutoAssignmentConfirmation table .marked{color:#0088ac}.table-common-container table thead,div#ProceedingEditorSubmissions table thead,div#divUserDisputeConflicts table thead,div#metaReviewerListForm table thead,div#reviewerListForm table thead,div#DeletedSubmissionListForm table thead,div#SuggestionForm table thead,div#MetaBiddingForm table thead,div#ExternalReviewForm table thead,div#ReferenceForm table thead,div#BiddingForm table thead,div#SubmissionListForm table thead,div#EmailMessagesForm table thead,div#AuditForm table thead,div#ReviewerInvitationListForm table thead,div#ReviewerInvitationForSubmissionListForm table thead,div#userListForm table thead,div#AutoAssignmentPapers table thead,div#AutoAssignmentReviewers table thead,div#AutoAssignmentSettings table thead,div#AutoAssignmentConfirmation table thead{text-transform:capitalize;font-size:15px;font-style:normal;font-weight:normal!important;background-color:#e6e6e6}.table-common-container table th.id,div#ProceedingEditorSubmissions table th.id,div#divUserDisputeConflicts table th.id,div#metaReviewerListForm table th.id,div#reviewerListForm table th.id,div#DeletedSubmissionListForm table th.id,div#SuggestionForm table th.id,div#MetaBiddingForm table th.id,div#ExternalReviewForm table th.id,div#ReferenceForm table th.id,div#BiddingForm table th.id,div#SubmissionListForm table th.id,div#EmailMessagesForm table th.id,div#AuditForm table th.id,div#ReviewerInvitationListForm table th.id,div#ReviewerInvitationForSubmissionListForm table th.id,div#userListForm table th.id,div#AutoAssignmentPapers table th.id,div#AutoAssignmentReviewers table th.id,div#AutoAssignmentSettings table th.id,div#AutoAssignmentConfirmation table th.id,.table-common-container table th.status,div#ProceedingEditorSubmissions table th.status,div#divUserDisputeConflicts table th.status,div#metaReviewerListForm table th.status,div#reviewerListForm table th.status,div#DeletedSubmissionListForm table th.status,div#SuggestionForm table th.status,div#MetaBiddingForm table th.status,div#ExternalReviewForm table th.status,div#ReferenceForm table th.status,div#BiddingForm table th.status,div#SubmissionListForm table th.status,div#EmailMessagesForm table th.status,div#AuditForm table th.status,div#ReviewerInvitationListForm table th.status,div#ReviewerInvitationForSubmissionListForm table th.status,div#userListForm table th.status,div#AutoAssignmentPapers table th.status,div#AutoAssignmentReviewers table th.status,div#AutoAssignmentSettings table th.status,div#AutoAssignmentConfirmation table th.status,.table-common-container table th.completed,div#ProceedingEditorSubmissions table th.completed,div#divUserDisputeConflicts table th.completed,div#metaReviewerListForm table th.completed,div#reviewerListForm table th.completed,div#DeletedSubmissionListForm table th.completed,div#SuggestionForm table th.completed,div#MetaBiddingForm table th.completed,div#ExternalReviewForm table th.completed,div#ReferenceForm table th.completed,div#BiddingForm table th.completed,div#SubmissionListForm table th.completed,div#EmailMessagesForm table th.completed,div#AuditForm table th.completed,div#ReviewerInvitationListForm table th.completed,div#ReviewerInvitationForSubmissionListForm table th.completed,div#userListForm table th.completed,div#AutoAssignmentPapers table th.completed,div#AutoAssignmentReviewers table th.completed,div#AutoAssignmentSettings table th.completed,div#AutoAssignmentConfirmation table th.completed,.table-common-container table th.assigned,div#ProceedingEditorSubmissions table th.assigned,div#divUserDisputeConflicts table th.assigned,div#metaReviewerListForm table th.assigned,div#reviewerListForm table th.assigned,div#DeletedSubmissionListForm table th.assigned,div#SuggestionForm table th.assigned,div#MetaBiddingForm table th.assigned,div#ExternalReviewForm table th.assigned,div#ReferenceForm table th.assigned,div#BiddingForm table th.assigned,div#SubmissionListForm table th.assigned,div#EmailMessagesForm table th.assigned,div#AuditForm table th.assigned,div#ReviewerInvitationListForm table th.assigned,div#ReviewerInvitationForSubmissionListForm table th.assigned,div#userListForm table th.assigned,div#AutoAssignmentPapers table th.assigned,div#AutoAssignmentReviewers table th.assigned,div#AutoAssignmentSettings table th.assigned,div#AutoAssignmentConfirmation table th.assigned,.table-common-container table th.discussion,div#ProceedingEditorSubmissions table th.discussion,div#divUserDisputeConflicts table th.discussion,div#metaReviewerListForm table th.discussion,div#reviewerListForm table th.discussion,div#DeletedSubmissionListForm table th.discussion,div#SuggestionForm table th.discussion,div#MetaBiddingForm table th.discussion,div#ExternalReviewForm table th.discussion,div#ReferenceForm table th.discussion,div#BiddingForm table th.discussion,div#SubmissionListForm table th.discussion,div#EmailMessagesForm table th.discussion,div#AuditForm table th.discussion,div#ReviewerInvitationListForm table th.discussion,div#ReviewerInvitationForSubmissionListForm table th.discussion,div#userListForm table th.discussion,div#AutoAssignmentPapers table th.discussion,div#AutoAssignmentReviewers table th.discussion,div#AutoAssignmentSettings table th.discussion,div#AutoAssignmentConfirmation table th.discussion,.table-common-container table th.percentage,div#ProceedingEditorSubmissions table th.percentage,div#divUserDisputeConflicts table th.percentage,div#metaReviewerListForm table th.percentage,div#reviewerListForm table th.percentage,div#DeletedSubmissionListForm table th.percentage,div#SuggestionForm table th.percentage,div#MetaBiddingForm table th.percentage,div#ExternalReviewForm table th.percentage,div#ReferenceForm table th.percentage,div#BiddingForm table th.percentage,div#SubmissionListForm table th.percentage,div#EmailMessagesForm table th.percentage,div#AuditForm table th.percentage,div#ReviewerInvitationListForm table th.percentage,div#ReviewerInvitationForSubmissionListForm table th.percentage,div#userListForm table th.percentage,div#AutoAssignmentPapers table th.percentage,div#AutoAssignmentReviewers table th.percentage,div#AutoAssignmentSettings table th.percentage,div#AutoAssignmentConfirmation table th.percentage,.table-common-container table th.conflicts,div#ProceedingEditorSubmissions table th.conflicts,div#divUserDisputeConflicts table th.conflicts,div#metaReviewerListForm table th.conflicts,div#reviewerListForm table th.conflicts,div#DeletedSubmissionListForm table th.conflicts,div#SuggestionForm table th.conflicts,div#MetaBiddingForm table th.conflicts,div#ExternalReviewForm table th.conflicts,div#ReferenceForm table th.conflicts,div#BiddingForm table th.conflicts,div#SubmissionListForm table th.conflicts,div#EmailMessagesForm table th.conflicts,div#AuditForm table th.conflicts,div#ReviewerInvitationListForm table th.conflicts,div#ReviewerInvitationForSubmissionListForm table th.conflicts,div#userListForm table th.conflicts,div#AutoAssignmentPapers table th.conflicts,div#AutoAssignmentReviewers table th.conflicts,div#AutoAssignmentSettings table th.conflicts,div#AutoAssignmentConfirmation table th.conflicts{width:80px}.table-common-container table th.conflictReasons,div#ProceedingEditorSubmissions table th.conflictReasons,div#divUserDisputeConflicts table th.conflictReasons,div#metaReviewerListForm table th.conflictReasons,div#reviewerListForm table th.conflictReasons,div#DeletedSubmissionListForm table th.conflictReasons,div#SuggestionForm table th.conflictReasons,div#MetaBiddingForm table th.conflictReasons,div#ExternalReviewForm table th.conflictReasons,div#ReferenceForm table th.conflictReasons,div#BiddingForm table th.conflictReasons,div#SubmissionListForm table th.conflictReasons,div#EmailMessagesForm table th.conflictReasons,div#AuditForm table th.conflictReasons,div#ReviewerInvitationListForm table th.conflictReasons,div#ReviewerInvitationForSubmissionListForm table th.conflictReasons,div#userListForm table th.conflictReasons,div#AutoAssignmentPapers table th.conflictReasons,div#AutoAssignmentReviewers table th.conflictReasons,div#AutoAssignmentSettings table th.conflictReasons,div#AutoAssignmentConfirmation table th.conflictReasons{width:300px}.table-common-container table th.conflictDisputeReason,div#ProceedingEditorSubmissions table th.conflictDisputeReason,div#divUserDisputeConflicts table th.conflictDisputeReason,div#metaReviewerListForm table th.conflictDisputeReason,div#reviewerListForm table th.conflictDisputeReason,div#DeletedSubmissionListForm table th.conflictDisputeReason,div#SuggestionForm table th.conflictDisputeReason,div#MetaBiddingForm table th.conflictDisputeReason,div#ExternalReviewForm table th.conflictDisputeReason,div#ReferenceForm table th.conflictDisputeReason,div#BiddingForm table th.conflictDisputeReason,div#SubmissionListForm table th.conflictDisputeReason,div#EmailMessagesForm table th.conflictDisputeReason,div#AuditForm table th.conflictDisputeReason,div#ReviewerInvitationListForm table th.conflictDisputeReason,div#ReviewerInvitationForSubmissionListForm table th.conflictDisputeReason,div#userListForm table th.conflictDisputeReason,div#AutoAssignmentPapers table th.conflictDisputeReason,div#AutoAssignmentReviewers table th.conflictDisputeReason,div#AutoAssignmentSettings table th.conflictDisputeReason,div#AutoAssignmentConfirmation table th.conflictDisputeReason,.table-common-container table td.conflictDisputeReason,div#ProceedingEditorSubmissions table td.conflictDisputeReason,div#divUserDisputeConflicts table td.conflictDisputeReason,div#metaReviewerListForm table td.conflictDisputeReason,div#reviewerListForm table td.conflictDisputeReason,div#DeletedSubmissionListForm table td.conflictDisputeReason,div#SuggestionForm table td.conflictDisputeReason,div#MetaBiddingForm table td.conflictDisputeReason,div#ExternalReviewForm table td.conflictDisputeReason,div#ReferenceForm table td.conflictDisputeReason,div#BiddingForm table td.conflictDisputeReason,div#SubmissionListForm table td.conflictDisputeReason,div#EmailMessagesForm table td.conflictDisputeReason,div#AuditForm table td.conflictDisputeReason,div#ReviewerInvitationListForm table td.conflictDisputeReason,div#ReviewerInvitationForSubmissionListForm table td.conflictDisputeReason,div#userListForm table td.conflictDisputeReason,div#AutoAssignmentPapers table td.conflictDisputeReason,div#AutoAssignmentReviewers table td.conflictDisputeReason,div#AutoAssignmentSettings table td.conflictDisputeReason,div#AutoAssignmentConfirmation table td.conflictDisputeReason{width:300px}.table-common-container table th.conflictDisputeStatus,div#ProceedingEditorSubmissions table th.conflictDisputeStatus,div#divUserDisputeConflicts table th.conflictDisputeStatus,div#metaReviewerListForm table th.conflictDisputeStatus,div#reviewerListForm table th.conflictDisputeStatus,div#DeletedSubmissionListForm table th.conflictDisputeStatus,div#SuggestionForm table th.conflictDisputeStatus,div#MetaBiddingForm table th.conflictDisputeStatus,div#ExternalReviewForm table th.conflictDisputeStatus,div#ReferenceForm table th.conflictDisputeStatus,div#BiddingForm table th.conflictDisputeStatus,div#SubmissionListForm table th.conflictDisputeStatus,div#EmailMessagesForm table th.conflictDisputeStatus,div#AuditForm table th.conflictDisputeStatus,div#ReviewerInvitationListForm table th.conflictDisputeStatus,div#ReviewerInvitationForSubmissionListForm table th.conflictDisputeStatus,div#userListForm table th.conflictDisputeStatus,div#AutoAssignmentPapers table th.conflictDisputeStatus,div#AutoAssignmentReviewers table th.conflictDisputeStatus,div#AutoAssignmentSettings table th.conflictDisputeStatus,div#AutoAssignmentConfirmation table th.conflictDisputeStatus,.table-common-container table td.conflictDisputeStatus,div#ProceedingEditorSubmissions table td.conflictDisputeStatus,div#divUserDisputeConflicts table td.conflictDisputeStatus,div#metaReviewerListForm table td.conflictDisputeStatus,div#reviewerListForm table td.conflictDisputeStatus,div#DeletedSubmissionListForm table td.conflictDisputeStatus,div#SuggestionForm table td.conflictDisputeStatus,div#MetaBiddingForm table td.conflictDisputeStatus,div#ExternalReviewForm table td.conflictDisputeStatus,div#ReferenceForm table td.conflictDisputeStatus,div#BiddingForm table td.conflictDisputeStatus,div#SubmissionListForm table td.conflictDisputeStatus,div#EmailMessagesForm table td.conflictDisputeStatus,div#AuditForm table td.conflictDisputeStatus,div#ReviewerInvitationListForm table td.conflictDisputeStatus,div#ReviewerInvitationForSubmissionListForm table td.conflictDisputeStatus,div#userListForm table td.conflictDisputeStatus,div#AutoAssignmentPapers table td.conflictDisputeStatus,div#AutoAssignmentReviewers table td.conflictDisputeStatus,div#AutoAssignmentSettings table td.conflictDisputeStatus,div#AutoAssignmentConfirmation table td.conflictDisputeStatus{width:110px}.table-common-container table th[sortby]:hover,div#ProceedingEditorSubmissions table th[sortby]:hover,div#divUserDisputeConflicts table th[sortby]:hover,div#metaReviewerListForm table th[sortby]:hover,div#reviewerListForm table th[sortby]:hover,div#DeletedSubmissionListForm table th[sortby]:hover,div#SuggestionForm table th[sortby]:hover,div#MetaBiddingForm table th[sortby]:hover,div#ExternalReviewForm table th[sortby]:hover,div#ReferenceForm table th[sortby]:hover,div#BiddingForm table th[sortby]:hover,div#SubmissionListForm table th[sortby]:hover,div#EmailMessagesForm table th[sortby]:hover,div#AuditForm table th[sortby]:hover,div#ReviewerInvitationListForm table th[sortby]:hover,div#ReviewerInvitationForSubmissionListForm table th[sortby]:hover,div#userListForm table th[sortby]:hover,div#AutoAssignmentPapers table th[sortby]:hover,div#AutoAssignmentReviewers table th[sortby]:hover,div#AutoAssignmentSettings table th[sortby]:hover,div#AutoAssignmentConfirmation table th[sortby]:hover,.table-common-container table th[sortby].selected,div#ProceedingEditorSubmissions table th[sortby].selected,div#divUserDisputeConflicts table th[sortby].selected,div#metaReviewerListForm table th[sortby].selected,div#reviewerListForm table th[sortby].selected,div#DeletedSubmissionListForm table th[sortby].selected,div#SuggestionForm table th[sortby].selected,div#MetaBiddingForm table th[sortby].selected,div#ExternalReviewForm table th[sortby].selected,div#ReferenceForm table th[sortby].selected,div#BiddingForm table th[sortby].selected,div#SubmissionListForm table th[sortby].selected,div#EmailMessagesForm table th[sortby].selected,div#AuditForm table th[sortby].selected,div#ReviewerInvitationListForm table th[sortby].selected,div#ReviewerInvitationForSubmissionListForm table th[sortby].selected,div#userListForm table th[sortby].selected,div#AutoAssignmentPapers table th[sortby].selected,div#AutoAssignmentReviewers table th[sortby].selected,div#AutoAssignmentSettings table th[sortby].selected,div#AutoAssignmentConfirmation table th[sortby].selected{background-color:rgba(0,0,0,.2);cursor:pointer;border-top:1px solid #eceac2}.table-common-container table tbody tr:nth-child(2n+1),div#ProceedingEditorSubmissions table tbody tr:nth-child(2n+1),div#divUserDisputeConflicts table tbody tr:nth-child(2n+1),div#metaReviewerListForm table tbody tr:nth-child(2n+1),div#reviewerListForm table tbody tr:nth-child(2n+1),div#DeletedSubmissionListForm table tbody tr:nth-child(2n+1),div#SuggestionForm table tbody tr:nth-child(2n+1),div#MetaBiddingForm table tbody tr:nth-child(2n+1),div#ExternalReviewForm table tbody tr:nth-child(2n+1),div#ReferenceForm table tbody tr:nth-child(2n+1),div#BiddingForm table tbody tr:nth-child(2n+1),div#SubmissionListForm table tbody tr:nth-child(2n+1),div#EmailMessagesForm table tbody tr:nth-child(2n+1),div#AuditForm table tbody tr:nth-child(2n+1),div#ReviewerInvitationListForm table tbody tr:nth-child(2n+1),div#ReviewerInvitationForSubmissionListForm table tbody tr:nth-child(2n+1),div#userListForm table tbody tr:nth-child(2n+1),div#AutoAssignmentPapers table tbody tr:nth-child(2n+1),div#AutoAssignmentReviewers table tbody tr:nth-child(2n+1),div#AutoAssignmentSettings table tbody tr:nth-child(2n+1),div#AutoAssignmentConfirmation table tbody tr:nth-child(2n+1){background-color:#f7fcff}.table-common-container table tbody tr:hover,div#ProceedingEditorSubmissions table tbody tr:hover,div#divUserDisputeConflicts table tbody tr:hover,div#metaReviewerListForm table tbody tr:hover,div#reviewerListForm table tbody tr:hover,div#DeletedSubmissionListForm table tbody tr:hover,div#SuggestionForm table tbody tr:hover,div#MetaBiddingForm table tbody tr:hover,div#ExternalReviewForm table tbody tr:hover,div#ReferenceForm table tbody tr:hover,div#BiddingForm table tbody tr:hover,div#SubmissionListForm table tbody tr:hover,div#EmailMessagesForm table tbody tr:hover,div#AuditForm table tbody tr:hover,div#ReviewerInvitationListForm table tbody tr:hover,div#ReviewerInvitationForSubmissionListForm table tbody tr:hover,div#userListForm table tbody tr:hover,div#AutoAssignmentPapers table tbody tr:hover,div#AutoAssignmentReviewers table tbody tr:hover,div#AutoAssignmentSettings table tbody tr:hover,div#AutoAssignmentConfirmation table tbody tr:hover{background-color:#98d4ee}.table-common-container table td,div#ProceedingEditorSubmissions table td,div#divUserDisputeConflicts table td,div#metaReviewerListForm table td,div#reviewerListForm table td,div#DeletedSubmissionListForm table td,div#SuggestionForm table td,div#MetaBiddingForm table td,div#ExternalReviewForm table td,div#ReferenceForm table td,div#BiddingForm table td,div#SubmissionListForm table td,div#EmailMessagesForm table td,div#AuditForm table td,div#ReviewerInvitationListForm table td,div#ReviewerInvitationForSubmissionListForm table td,div#userListForm table td,div#AutoAssignmentPapers table td,div#AutoAssignmentReviewers table td,div#AutoAssignmentSettings table td,div#AutoAssignmentConfirmation table td{vertical-align:middle;text-align:center}.table-common-container table tbody .submission,div#ProceedingEditorSubmissions table tbody .submission,div#divUserDisputeConflicts table tbody .submission,div#metaReviewerListForm table tbody .submission,div#reviewerListForm table tbody .submission,div#DeletedSubmissionListForm table tbody .submission,div#SuggestionForm table tbody .submission,div#MetaBiddingForm table tbody .submission,div#ExternalReviewForm table tbody .submission,div#ReferenceForm table tbody .submission,div#BiddingForm table tbody .submission,div#SubmissionListForm table tbody .submission,div#EmailMessagesForm table tbody .submission,div#AuditForm table tbody .submission,div#ReviewerInvitationListForm table tbody .submission,div#ReviewerInvitationForSubmissionListForm table tbody .submission,div#userListForm table tbody .submission,div#AutoAssignmentPapers table tbody .submission,div#AutoAssignmentReviewers table tbody .submission,div#AutoAssignmentSettings table tbody .submission,div#AutoAssignmentConfirmation table tbody .submission{position:relative;text-align:left;vertical-align:top}.table-common-container table tbody .submission .abstract,div#ProceedingEditorSubmissions table tbody .submission .abstract,div#divUserDisputeConflicts table tbody .submission .abstract,div#metaReviewerListForm table tbody .submission .abstract,div#reviewerListForm table tbody .submission .abstract,div#DeletedSubmissionListForm table tbody .submission .abstract,div#SuggestionForm table tbody .submission .abstract,div#MetaBiddingForm table tbody .submission .abstract,div#ExternalReviewForm table tbody .submission .abstract,div#ReferenceForm table tbody .submission .abstract,div#BiddingForm table tbody .submission .abstract,div#SubmissionListForm table tbody .submission .abstract,div#EmailMessagesForm table tbody .submission .abstract,div#AuditForm table tbody .submission .abstract,div#ReviewerInvitationListForm table tbody .submission .abstract,div#ReviewerInvitationForSubmissionListForm table tbody .submission .abstract,div#userListForm table tbody .submission .abstract,div#AutoAssignmentPapers table tbody .submission .abstract,div#AutoAssignmentReviewers table tbody .submission .abstract,div#AutoAssignmentSettings table tbody .submission .abstract,div#AutoAssignmentConfirmation table tbody .submission .abstract{bottom:5px;right:5px;font-size:12px;cursor:pointer}.table-common-container table .status a,div#ProceedingEditorSubmissions table .status a,div#divUserDisputeConflicts table .status a,div#metaReviewerListForm table .status a,div#reviewerListForm table .status a,div#DeletedSubmissionListForm table .status a,div#SuggestionForm table .status a,div#MetaBiddingForm table .status a,div#ExternalReviewForm table .status a,div#ReferenceForm table .status a,div#BiddingForm table .status a,div#SubmissionListForm table .status a,div#EmailMessagesForm table .status a,div#AuditForm table .status a,div#ReviewerInvitationListForm table .status a,div#ReviewerInvitationForSubmissionListForm table .status a,div#userListForm table .status a,div#AutoAssignmentPapers table .status a,div#AutoAssignmentReviewers table .status a,div#AutoAssignmentSettings table .status a,div#AutoAssignmentConfirmation table .status a{cursor:pointer}.table-common-container table tbody .btn-group .dropdown-menu li,div#ProceedingEditorSubmissions table tbody .btn-group .dropdown-menu li,div#divUserDisputeConflicts table tbody .btn-group .dropdown-menu li,div#metaReviewerListForm table tbody .btn-group .dropdown-menu li,div#reviewerListForm table tbody .btn-group .dropdown-menu li,div#DeletedSubmissionListForm table tbody .btn-group .dropdown-menu li,div#SuggestionForm table tbody .btn-group .dropdown-menu li,div#MetaBiddingForm table tbody .btn-group .dropdown-menu li,div#ExternalReviewForm table tbody .btn-group .dropdown-menu li,div#ReferenceForm table tbody .btn-group .dropdown-menu li,div#BiddingForm table tbody .btn-group .dropdown-menu li,div#SubmissionListForm table tbody .btn-group .dropdown-menu li,div#EmailMessagesForm table tbody .btn-group .dropdown-menu li,div#AuditForm table tbody .btn-group .dropdown-menu li,div#ReviewerInvitationListForm table tbody .btn-group .dropdown-menu li,div#ReviewerInvitationForSubmissionListForm table tbody .btn-group .dropdown-menu li,div#userListForm table tbody .btn-group .dropdown-menu li,div#AutoAssignmentPapers table tbody .btn-group .dropdown-menu li,div#AutoAssignmentReviewers table tbody .btn-group .dropdown-menu li,div#AutoAssignmentSettings table tbody .btn-group .dropdown-menu li,div#AutoAssignmentConfirmation table tbody .btn-group .dropdown-menu li{text-align:left}.table-common-container table table.inline-review,div#ProceedingEditorSubmissions table table.inline-review,div#divUserDisputeConflicts table table.inline-review,div#metaReviewerListForm table table.inline-review,div#reviewerListForm table table.inline-review,div#DeletedSubmissionListForm table table.inline-review,div#SuggestionForm table table.inline-review,div#MetaBiddingForm table table.inline-review,div#ExternalReviewForm table table.inline-review,div#ReferenceForm table table.inline-review,div#BiddingForm table table.inline-review,div#SubmissionListForm table table.inline-review,div#EmailMessagesForm table table.inline-review,div#AuditForm table table.inline-review,div#ReviewerInvitationListForm table table.inline-review,div#ReviewerInvitationForSubmissionListForm table table.inline-review,div#userListForm table table.inline-review,div#AutoAssignmentPapers table table.inline-review,div#AutoAssignmentReviewers table table.inline-review,div#AutoAssignmentSettings table table.inline-review,div#AutoAssignmentConfirmation table table.inline-review{border:none}.table-common-container table table.inline-review thead,div#ProceedingEditorSubmissions table table.inline-review thead,div#divUserDisputeConflicts table table.inline-review thead,div#metaReviewerListForm table table.inline-review thead,div#reviewerListForm table table.inline-review thead,div#DeletedSubmissionListForm table table.inline-review thead,div#SuggestionForm table table.inline-review thead,div#MetaBiddingForm table table.inline-review thead,div#ExternalReviewForm table table.inline-review thead,div#ReferenceForm table table.inline-review thead,div#BiddingForm table table.inline-review thead,div#SubmissionListForm table table.inline-review thead,div#EmailMessagesForm table table.inline-review thead,div#AuditForm table table.inline-review thead,div#ReviewerInvitationListForm table table.inline-review thead,div#ReviewerInvitationForSubmissionListForm table table.inline-review thead,div#userListForm table table.inline-review thead,div#AutoAssignmentPapers table table.inline-review thead,div#AutoAssignmentReviewers table table.inline-review thead,div#AutoAssignmentSettings table table.inline-review thead,div#AutoAssignmentConfirmation table table.inline-review thead,.table-common-container table table.inline-review tbody,div#ProceedingEditorSubmissions table table.inline-review tbody,div#divUserDisputeConflicts table table.inline-review tbody,div#metaReviewerListForm table table.inline-review tbody,div#reviewerListForm table table.inline-review tbody,div#DeletedSubmissionListForm table table.inline-review tbody,div#SuggestionForm table table.inline-review tbody,div#MetaBiddingForm table table.inline-review tbody,div#ExternalReviewForm table table.inline-review tbody,div#ReferenceForm table table.inline-review tbody,div#BiddingForm table table.inline-review tbody,div#SubmissionListForm table table.inline-review tbody,div#EmailMessagesForm table table.inline-review tbody,div#AuditForm table table.inline-review tbody,div#ReviewerInvitationListForm table table.inline-review tbody,div#ReviewerInvitationForSubmissionListForm table table.inline-review tbody,div#userListForm table table.inline-review tbody,div#AutoAssignmentPapers table table.inline-review tbody,div#AutoAssignmentReviewers table table.inline-review tbody,div#AutoAssignmentSettings table table.inline-review tbody,div#AutoAssignmentConfirmation table table.inline-review tbody,.table-common-container table table.inline-review tr,div#ProceedingEditorSubmissions table table.inline-review tr,div#divUserDisputeConflicts table table.inline-review tr,div#metaReviewerListForm table table.inline-review tr,div#reviewerListForm table table.inline-review tr,div#DeletedSubmissionListForm table table.inline-review tr,div#SuggestionForm table table.inline-review tr,div#MetaBiddingForm table table.inline-review tr,div#ExternalReviewForm table table.inline-review tr,div#ReferenceForm table table.inline-review tr,div#BiddingForm table table.inline-review tr,div#SubmissionListForm table table.inline-review tr,div#EmailMessagesForm table table.inline-review tr,div#AuditForm table table.inline-review tr,div#ReviewerInvitationListForm table table.inline-review tr,div#ReviewerInvitationForSubmissionListForm table table.inline-review tr,div#userListForm table table.inline-review tr,div#AutoAssignmentPapers table table.inline-review tr,div#AutoAssignmentReviewers table table.inline-review tr,div#AutoAssignmentSettings table table.inline-review tr,div#AutoAssignmentConfirmation table table.inline-review tr,.table-common-container table table.inline-review td,div#ProceedingEditorSubmissions table table.inline-review td,div#divUserDisputeConflicts table table.inline-review td,div#metaReviewerListForm table table.inline-review td,div#reviewerListForm table table.inline-review td,div#DeletedSubmissionListForm table table.inline-review td,div#SuggestionForm table table.inline-review td,div#MetaBiddingForm table table.inline-review td,div#ExternalReviewForm table table.inline-review td,div#ReferenceForm table table.inline-review td,div#BiddingForm table table.inline-review td,div#SubmissionListForm table table.inline-review td,div#EmailMessagesForm table table.inline-review td,div#AuditForm table table.inline-review td,div#ReviewerInvitationListForm table table.inline-review td,div#ReviewerInvitationForSubmissionListForm table table.inline-review td,div#userListForm table table.inline-review td,div#AutoAssignmentPapers table table.inline-review td,div#AutoAssignmentReviewers table table.inline-review td,div#AutoAssignmentSettings table table.inline-review td,div#AutoAssignmentConfirmation table table.inline-review td,.table-common-container table table.inline-review th,div#ProceedingEditorSubmissions table table.inline-review th,div#divUserDisputeConflicts table table.inline-review th,div#metaReviewerListForm table table.inline-review th,div#reviewerListForm table table.inline-review th,div#DeletedSubmissionListForm table table.inline-review th,div#SuggestionForm table table.inline-review th,div#MetaBiddingForm table table.inline-review th,div#ExternalReviewForm table table.inline-review th,div#ReferenceForm table table.inline-review th,div#BiddingForm table table.inline-review th,div#SubmissionListForm table table.inline-review th,div#EmailMessagesForm table table.inline-review th,div#AuditForm table table.inline-review th,div#ReviewerInvitationListForm table table.inline-review th,div#ReviewerInvitationForSubmissionListForm table table.inline-review th,div#userListForm table table.inline-review th,div#AutoAssignmentPapers table table.inline-review th,div#AutoAssignmentReviewers table table.inline-review th,div#AutoAssignmentSettings table table.inline-review th,div#AutoAssignmentConfirmation table table.inline-review th{background-color:transparent;border:none}.table-common-container table table.inline-review thead>tr:first-child>th,div#ProceedingEditorSubmissions table table.inline-review thead>tr:first-child>th,div#divUserDisputeConflicts table table.inline-review thead>tr:first-child>th,div#metaReviewerListForm table table.inline-review thead>tr:first-child>th,div#reviewerListForm table table.inline-review thead>tr:first-child>th,div#DeletedSubmissionListForm table table.inline-review thead>tr:first-child>th,div#SuggestionForm table table.inline-review thead>tr:first-child>th,div#MetaBiddingForm table table.inline-review thead>tr:first-child>th,div#ExternalReviewForm table table.inline-review thead>tr:first-child>th,div#ReferenceForm table table.inline-review thead>tr:first-child>th,div#BiddingForm table table.inline-review thead>tr:first-child>th,div#SubmissionListForm table table.inline-review thead>tr:first-child>th,div#EmailMessagesForm table table.inline-review thead>tr:first-child>th,div#AuditForm table table.inline-review thead>tr:first-child>th,div#ReviewerInvitationListForm table table.inline-review thead>tr:first-child>th,div#ReviewerInvitationForSubmissionListForm table table.inline-review thead>tr:first-child>th,div#userListForm table table.inline-review thead>tr:first-child>th,div#AutoAssignmentPapers table table.inline-review thead>tr:first-child>th,div#AutoAssignmentReviewers table table.inline-review thead>tr:first-child>th,div#AutoAssignmentSettings table table.inline-review thead>tr:first-child>th,div#AutoAssignmentConfirmation table table.inline-review thead>tr:first-child>th{border-top:none}.table-common-container table table.inline-review thead>tr:last-child>th,div#ProceedingEditorSubmissions table table.inline-review thead>tr:last-child>th,div#divUserDisputeConflicts table table.inline-review thead>tr:last-child>th,div#metaReviewerListForm table table.inline-review thead>tr:last-child>th,div#reviewerListForm table table.inline-review thead>tr:last-child>th,div#DeletedSubmissionListForm table table.inline-review thead>tr:last-child>th,div#SuggestionForm table table.inline-review thead>tr:last-child>th,div#MetaBiddingForm table table.inline-review thead>tr:last-child>th,div#ExternalReviewForm table table.inline-review thead>tr:last-child>th,div#ReferenceForm table table.inline-review thead>tr:last-child>th,div#BiddingForm table table.inline-review thead>tr:last-child>th,div#SubmissionListForm table table.inline-review thead>tr:last-child>th,div#EmailMessagesForm table table.inline-review thead>tr:last-child>th,div#AuditForm table table.inline-review thead>tr:last-child>th,div#ReviewerInvitationListForm table table.inline-review thead>tr:last-child>th,div#ReviewerInvitationForSubmissionListForm table table.inline-review thead>tr:last-child>th,div#userListForm table table.inline-review thead>tr:last-child>th,div#AutoAssignmentPapers table table.inline-review thead>tr:last-child>th,div#AutoAssignmentReviewers table table.inline-review thead>tr:last-child>th,div#AutoAssignmentSettings table table.inline-review thead>tr:last-child>th,div#AutoAssignmentConfirmation table table.inline-review thead>tr:last-child>th{border-bottom:none}.table-common-container table table.inline-review thead>tr:last-child,div#ProceedingEditorSubmissions table table.inline-review thead>tr:last-child,div#divUserDisputeConflicts table table.inline-review thead>tr:last-child,div#metaReviewerListForm table table.inline-review thead>tr:last-child,div#reviewerListForm table table.inline-review thead>tr:last-child,div#DeletedSubmissionListForm table table.inline-review thead>tr:last-child,div#SuggestionForm table table.inline-review thead>tr:last-child,div#MetaBiddingForm table table.inline-review thead>tr:last-child,div#ExternalReviewForm table table.inline-review thead>tr:last-child,div#ReferenceForm table table.inline-review thead>tr:last-child,div#BiddingForm table table.inline-review thead>tr:last-child,div#SubmissionListForm table table.inline-review thead>tr:last-child,div#EmailMessagesForm table table.inline-review thead>tr:last-child,div#AuditForm table table.inline-review thead>tr:last-child,div#ReviewerInvitationListForm table table.inline-review thead>tr:last-child,div#ReviewerInvitationForSubmissionListForm table table.inline-review thead>tr:last-child,div#userListForm table table.inline-review thead>tr:last-child,div#AutoAssignmentPapers table table.inline-review thead>tr:last-child,div#AutoAssignmentReviewers table table.inline-review thead>tr:last-child,div#AutoAssignmentSettings table table.inline-review thead>tr:last-child,div#AutoAssignmentConfirmation table table.inline-review thead>tr:last-child{border-bottom:1px solid #ddd}.table-common-container table table.inline-review thead>tr>th,div#ProceedingEditorSubmissions table table.inline-review thead>tr>th,div#divUserDisputeConflicts table table.inline-review thead>tr>th,div#metaReviewerListForm table table.inline-review thead>tr>th,div#reviewerListForm table table.inline-review thead>tr>th,div#DeletedSubmissionListForm table table.inline-review thead>tr>th,div#SuggestionForm table table.inline-review thead>tr>th,div#MetaBiddingForm table table.inline-review thead>tr>th,div#ExternalReviewForm table table.inline-review thead>tr>th,div#ReferenceForm table table.inline-review thead>tr>th,div#BiddingForm table table.inline-review thead>tr>th,div#SubmissionListForm table table.inline-review thead>tr>th,div#EmailMessagesForm table table.inline-review thead>tr>th,div#AuditForm table table.inline-review thead>tr>th,div#ReviewerInvitationListForm table table.inline-review thead>tr>th,div#ReviewerInvitationForSubmissionListForm table table.inline-review thead>tr>th,div#userListForm table table.inline-review thead>tr>th,div#AutoAssignmentPapers table table.inline-review thead>tr>th,div#AutoAssignmentReviewers table table.inline-review thead>tr>th,div#AutoAssignmentSettings table table.inline-review thead>tr>th,div#AutoAssignmentConfirmation table table.inline-review thead>tr>th{font-weight:bold}.table-common-container table table.inline-review td.inline-review-answers,div#ProceedingEditorSubmissions table table.inline-review td.inline-review-answers,div#divUserDisputeConflicts table table.inline-review td.inline-review-answers,div#metaReviewerListForm table table.inline-review td.inline-review-answers,div#reviewerListForm table table.inline-review td.inline-review-answers,div#DeletedSubmissionListForm table table.inline-review td.inline-review-answers,div#SuggestionForm table table.inline-review td.inline-review-answers,div#MetaBiddingForm table table.inline-review td.inline-review-answers,div#ExternalReviewForm table table.inline-review td.inline-review-answers,div#ReferenceForm table table.inline-review td.inline-review-answers,div#BiddingForm table table.inline-review td.inline-review-answers,div#SubmissionListForm table table.inline-review td.inline-review-answers,div#EmailMessagesForm table table.inline-review td.inline-review-answers,div#AuditForm table table.inline-review td.inline-review-answers,div#ReviewerInvitationListForm table table.inline-review td.inline-review-answers,div#ReviewerInvitationForSubmissionListForm table table.inline-review td.inline-review-answers,div#userListForm table table.inline-review td.inline-review-answers,div#AutoAssignmentPapers table table.inline-review td.inline-review-answers,div#AutoAssignmentReviewers table table.inline-review td.inline-review-answers,div#AutoAssignmentSettings table table.inline-review td.inline-review-answers,div#AutoAssignmentConfirmation table table.inline-review td.inline-review-answers{white-space:nowrap}.table-common-container table table.inline-review td.inline-review-answers span:not(:last-child)::after,div#ProceedingEditorSubmissions table table.inline-review td.inline-review-answers span:not(:last-child)::after,div#divUserDisputeConflicts table table.inline-review td.inline-review-answers span:not(:last-child)::after,div#metaReviewerListForm table table.inline-review td.inline-review-answers span:not(:last-child)::after,div#reviewerListForm table table.inline-review td.inline-review-answers span:not(:last-child)::after,div#DeletedSubmissionListForm table table.inline-review td.inline-review-answers span:not(:last-child)::after,div#SuggestionForm table table.inline-review td.inline-review-answers span:not(:last-child)::after,div#MetaBiddingForm table table.inline-review td.inline-review-answers span:not(:last-child)::after,div#ExternalReviewForm table table.inline-review td.inline-review-answers span:not(:last-child)::after,div#ReferenceForm table table.inline-review td.inline-review-answers span:not(:last-child)::after,div#BiddingForm table table.inline-review td.inline-review-answers span:not(:last-child)::after,div#SubmissionListForm table table.inline-review td.inline-review-answers span:not(:last-child)::after,div#EmailMessagesForm table table.inline-review td.inline-review-answers span:not(:last-child)::after,div#AuditForm table table.inline-review td.inline-review-answers span:not(:last-child)::after,div#ReviewerInvitationListForm table table.inline-review td.inline-review-answers span:not(:last-child)::after,div#ReviewerInvitationForSubmissionListForm table table.inline-review td.inline-review-answers span:not(:last-child)::after,div#userListForm table table.inline-review td.inline-review-answers span:not(:last-child)::after,div#AutoAssignmentPapers table table.inline-review td.inline-review-answers span:not(:last-child)::after,div#AutoAssignmentReviewers table table.inline-review td.inline-review-answers span:not(:last-child)::after,div#AutoAssignmentSettings table table.inline-review td.inline-review-answers span:not(:last-child)::after,div#AutoAssignmentConfirmation table table.inline-review td.inline-review-answers span:not(:last-child)::after{content:","}.table-common-container table table.inline-recommendation,div#ProceedingEditorSubmissions table table.inline-recommendation,div#divUserDisputeConflicts table table.inline-recommendation,div#metaReviewerListForm table table.inline-recommendation,div#reviewerListForm table table.inline-recommendation,div#DeletedSubmissionListForm table table.inline-recommendation,div#SuggestionForm table table.inline-recommendation,div#MetaBiddingForm table table.inline-recommendation,div#ExternalReviewForm table table.inline-recommendation,div#ReferenceForm table table.inline-recommendation,div#BiddingForm table table.inline-recommendation,div#SubmissionListForm table table.inline-recommendation,div#EmailMessagesForm table table.inline-recommendation,div#AuditForm table table.inline-recommendation,div#ReviewerInvitationListForm table table.inline-recommendation,div#ReviewerInvitationForSubmissionListForm table table.inline-recommendation,div#userListForm table table.inline-recommendation,div#AutoAssignmentPapers table table.inline-recommendation,div#AutoAssignmentReviewers table table.inline-recommendation,div#AutoAssignmentSettings table table.inline-recommendation,div#AutoAssignmentConfirmation table table.inline-recommendation{border:none}.table-common-container table table.inline-recommendation thead,div#ProceedingEditorSubmissions table table.inline-recommendation thead,div#divUserDisputeConflicts table table.inline-recommendation thead,div#metaReviewerListForm table table.inline-recommendation thead,div#reviewerListForm table table.inline-recommendation thead,div#DeletedSubmissionListForm table table.inline-recommendation thead,div#SuggestionForm table table.inline-recommendation thead,div#MetaBiddingForm table table.inline-recommendation thead,div#ExternalReviewForm table table.inline-recommendation thead,div#ReferenceForm table table.inline-recommendation thead,div#BiddingForm table table.inline-recommendation thead,div#SubmissionListForm table table.inline-recommendation thead,div#EmailMessagesForm table table.inline-recommendation thead,div#AuditForm table table.inline-recommendation thead,div#ReviewerInvitationListForm table table.inline-recommendation thead,div#ReviewerInvitationForSubmissionListForm table table.inline-recommendation thead,div#userListForm table table.inline-recommendation thead,div#AutoAssignmentPapers table table.inline-recommendation thead,div#AutoAssignmentReviewers table table.inline-recommendation thead,div#AutoAssignmentSettings table table.inline-recommendation thead,div#AutoAssignmentConfirmation table table.inline-recommendation thead,.table-common-container table table.inline-recommendation tbody,div#ProceedingEditorSubmissions table table.inline-recommendation tbody,div#divUserDisputeConflicts table table.inline-recommendation tbody,div#metaReviewerListForm table table.inline-recommendation tbody,div#reviewerListForm table table.inline-recommendation tbody,div#DeletedSubmissionListForm table table.inline-recommendation tbody,div#SuggestionForm table table.inline-recommendation tbody,div#MetaBiddingForm table table.inline-recommendation tbody,div#ExternalReviewForm table table.inline-recommendation tbody,div#ReferenceForm table table.inline-recommendation tbody,div#BiddingForm table table.inline-recommendation tbody,div#SubmissionListForm table table.inline-recommendation tbody,div#EmailMessagesForm table table.inline-recommendation tbody,div#AuditForm table table.inline-recommendation tbody,div#ReviewerInvitationListForm table table.inline-recommendation tbody,div#ReviewerInvitationForSubmissionListForm table table.inline-recommendation tbody,div#userListForm table table.inline-recommendation tbody,div#AutoAssignmentPapers table table.inline-recommendation tbody,div#AutoAssignmentReviewers table table.inline-recommendation tbody,div#AutoAssignmentSettings table table.inline-recommendation tbody,div#AutoAssignmentConfirmation table table.inline-recommendation tbody,.table-common-container table table.inline-recommendation tr,div#ProceedingEditorSubmissions table table.inline-recommendation tr,div#divUserDisputeConflicts table table.inline-recommendation tr,div#metaReviewerListForm table table.inline-recommendation tr,div#reviewerListForm table table.inline-recommendation tr,div#DeletedSubmissionListForm table table.inline-recommendation tr,div#SuggestionForm table table.inline-recommendation tr,div#MetaBiddingForm table table.inline-recommendation tr,div#ExternalReviewForm table table.inline-recommendation tr,div#ReferenceForm table table.inline-recommendation tr,div#BiddingForm table table.inline-recommendation tr,div#SubmissionListForm table table.inline-recommendation tr,div#EmailMessagesForm table table.inline-recommendation tr,div#AuditForm table table.inline-recommendation tr,div#ReviewerInvitationListForm table table.inline-recommendation tr,div#ReviewerInvitationForSubmissionListForm table table.inline-recommendation tr,div#userListForm table table.inline-recommendation tr,div#AutoAssignmentPapers table table.inline-recommendation tr,div#AutoAssignmentReviewers table table.inline-recommendation tr,div#AutoAssignmentSettings table table.inline-recommendation tr,div#AutoAssignmentConfirmation table table.inline-recommendation tr,.table-common-container table table.inline-recommendation td,div#ProceedingEditorSubmissions table table.inline-recommendation td,div#divUserDisputeConflicts table table.inline-recommendation td,div#metaReviewerListForm table table.inline-recommendation td,div#reviewerListForm table table.inline-recommendation td,div#DeletedSubmissionListForm table table.inline-recommendation td,div#SuggestionForm table table.inline-recommendation td,div#MetaBiddingForm table table.inline-recommendation td,div#ExternalReviewForm table table.inline-recommendation td,div#ReferenceForm table table.inline-recommendation td,div#BiddingForm table table.inline-recommendation td,div#SubmissionListForm table table.inline-recommendation td,div#EmailMessagesForm table table.inline-recommendation td,div#AuditForm table table.inline-recommendation td,div#ReviewerInvitationListForm table table.inline-recommendation td,div#ReviewerInvitationForSubmissionListForm table table.inline-recommendation td,div#userListForm table table.inline-recommendation td,div#AutoAssignmentPapers table table.inline-recommendation td,div#AutoAssignmentReviewers table table.inline-recommendation td,div#AutoAssignmentSettings table table.inline-recommendation td,div#AutoAssignmentConfirmation table table.inline-recommendation td,.table-common-container table table.inline-recommendation th,div#ProceedingEditorSubmissions table table.inline-recommendation th,div#divUserDisputeConflicts table table.inline-recommendation th,div#metaReviewerListForm table table.inline-recommendation th,div#reviewerListForm table table.inline-recommendation th,div#DeletedSubmissionListForm table table.inline-recommendation th,div#SuggestionForm table table.inline-recommendation th,div#MetaBiddingForm table table.inline-recommendation th,div#ExternalReviewForm table table.inline-recommendation th,div#ReferenceForm table table.inline-recommendation th,div#BiddingForm table table.inline-recommendation th,div#SubmissionListForm table table.inline-recommendation th,div#EmailMessagesForm table table.inline-recommendation th,div#AuditForm table table.inline-recommendation th,div#ReviewerInvitationListForm table table.inline-recommendation th,div#ReviewerInvitationForSubmissionListForm table table.inline-recommendation th,div#userListForm table table.inline-recommendation th,div#AutoAssignmentPapers table table.inline-recommendation th,div#AutoAssignmentReviewers table table.inline-recommendation th,div#AutoAssignmentSettings table table.inline-recommendation th,div#AutoAssignmentConfirmation table table.inline-recommendation th{background-color:transparent;border:none}.table-common-container table table.inline-recommendation thead>tr:first-child>th,div#ProceedingEditorSubmissions table table.inline-recommendation thead>tr:first-child>th,div#divUserDisputeConflicts table table.inline-recommendation thead>tr:first-child>th,div#metaReviewerListForm table table.inline-recommendation thead>tr:first-child>th,div#reviewerListForm table table.inline-recommendation thead>tr:first-child>th,div#DeletedSubmissionListForm table table.inline-recommendation thead>tr:first-child>th,div#SuggestionForm table table.inline-recommendation thead>tr:first-child>th,div#MetaBiddingForm table table.inline-recommendation thead>tr:first-child>th,div#ExternalReviewForm table table.inline-recommendation thead>tr:first-child>th,div#ReferenceForm table table.inline-recommendation thead>tr:first-child>th,div#BiddingForm table table.inline-recommendation thead>tr:first-child>th,div#SubmissionListForm table table.inline-recommendation thead>tr:first-child>th,div#EmailMessagesForm table table.inline-recommendation thead>tr:first-child>th,div#AuditForm table table.inline-recommendation thead>tr:first-child>th,div#ReviewerInvitationListForm table table.inline-recommendation thead>tr:first-child>th,div#ReviewerInvitationForSubmissionListForm table table.inline-recommendation thead>tr:first-child>th,div#userListForm table table.inline-recommendation thead>tr:first-child>th,div#AutoAssignmentPapers table table.inline-recommendation thead>tr:first-child>th,div#AutoAssignmentReviewers table table.inline-recommendation thead>tr:first-child>th,div#AutoAssignmentSettings table table.inline-recommendation thead>tr:first-child>th,div#AutoAssignmentConfirmation table table.inline-recommendation thead>tr:first-child>th{border-top:none}.table-common-container table table.inline-recommendation thead>tr:last-child>th,div#ProceedingEditorSubmissions table table.inline-recommendation thead>tr:last-child>th,div#divUserDisputeConflicts table table.inline-recommendation thead>tr:last-child>th,div#metaReviewerListForm table table.inline-recommendation thead>tr:last-child>th,div#reviewerListForm table table.inline-recommendation thead>tr:last-child>th,div#DeletedSubmissionListForm table table.inline-recommendation thead>tr:last-child>th,div#SuggestionForm table table.inline-recommendation thead>tr:last-child>th,div#MetaBiddingForm table table.inline-recommendation thead>tr:last-child>th,div#ExternalReviewForm table table.inline-recommendation thead>tr:last-child>th,div#ReferenceForm table table.inline-recommendation thead>tr:last-child>th,div#BiddingForm table table.inline-recommendation thead>tr:last-child>th,div#SubmissionListForm table table.inline-recommendation thead>tr:last-child>th,div#EmailMessagesForm table table.inline-recommendation thead>tr:last-child>th,div#AuditForm table table.inline-recommendation thead>tr:last-child>th,div#ReviewerInvitationListForm table table.inline-recommendation thead>tr:last-child>th,div#ReviewerInvitationForSubmissionListForm table table.inline-recommendation thead>tr:last-child>th,div#userListForm table table.inline-recommendation thead>tr:last-child>th,div#AutoAssignmentPapers table table.inline-recommendation thead>tr:last-child>th,div#AutoAssignmentReviewers table table.inline-recommendation thead>tr:last-child>th,div#AutoAssignmentSettings table table.inline-recommendation thead>tr:last-child>th,div#AutoAssignmentConfirmation table table.inline-recommendation thead>tr:last-child>th{border-bottom:none}.table-common-container table table.inline-recommendation thead>tr:last-child,div#ProceedingEditorSubmissions table table.inline-recommendation thead>tr:last-child,div#divUserDisputeConflicts table table.inline-recommendation thead>tr:last-child,div#metaReviewerListForm table table.inline-recommendation thead>tr:last-child,div#reviewerListForm table table.inline-recommendation thead>tr:last-child,div#DeletedSubmissionListForm table table.inline-recommendation thead>tr:last-child,div#SuggestionForm table table.inline-recommendation thead>tr:last-child,div#MetaBiddingForm table table.inline-recommendation thead>tr:last-child,div#ExternalReviewForm table table.inline-recommendation thead>tr:last-child,div#ReferenceForm table table.inline-recommendation thead>tr:last-child,div#BiddingForm table table.inline-recommendation thead>tr:last-child,div#SubmissionListForm table table.inline-recommendation thead>tr:last-child,div#EmailMessagesForm table table.inline-recommendation thead>tr:last-child,div#AuditForm table table.inline-recommendation thead>tr:last-child,div#ReviewerInvitationListForm table table.inline-recommendation thead>tr:last-child,div#ReviewerInvitationForSubmissionListForm table table.inline-recommendation thead>tr:last-child,div#userListForm table table.inline-recommendation thead>tr:last-child,div#AutoAssignmentPapers table table.inline-recommendation thead>tr:last-child,div#AutoAssignmentReviewers table table.inline-recommendation thead>tr:last-child,div#AutoAssignmentSettings table table.inline-recommendation thead>tr:last-child,div#AutoAssignmentConfirmation table table.inline-recommendation thead>tr:last-child{border-bottom:1px solid #ddd}.table-common-container table table.inline-recommendation thead>tr>th,div#ProceedingEditorSubmissions table table.inline-recommendation thead>tr>th,div#divUserDisputeConflicts table table.inline-recommendation thead>tr>th,div#metaReviewerListForm table table.inline-recommendation thead>tr>th,div#reviewerListForm table table.inline-recommendation thead>tr>th,div#DeletedSubmissionListForm table table.inline-recommendation thead>tr>th,div#SuggestionForm table table.inline-recommendation thead>tr>th,div#MetaBiddingForm table table.inline-recommendation thead>tr>th,div#ExternalReviewForm table table.inline-recommendation thead>tr>th,div#ReferenceForm table table.inline-recommendation thead>tr>th,div#BiddingForm table table.inline-recommendation thead>tr>th,div#SubmissionListForm table table.inline-recommendation thead>tr>th,div#EmailMessagesForm table table.inline-recommendation thead>tr>th,div#AuditForm table table.inline-recommendation thead>tr>th,div#ReviewerInvitationListForm table table.inline-recommendation thead>tr>th,div#ReviewerInvitationForSubmissionListForm table table.inline-recommendation thead>tr>th,div#userListForm table table.inline-recommendation thead>tr>th,div#AutoAssignmentPapers table table.inline-recommendation thead>tr>th,div#AutoAssignmentReviewers table table.inline-recommendation thead>tr>th,div#AutoAssignmentSettings table table.inline-recommendation thead>tr>th,div#AutoAssignmentConfirmation table table.inline-recommendation thead>tr>th{font-size:small;font-weight:bold}.table-common-container table table.shared-from,div#ProceedingEditorSubmissions table table.shared-from,div#divUserDisputeConflicts table table.shared-from,div#metaReviewerListForm table table.shared-from,div#reviewerListForm table table.shared-from,div#DeletedSubmissionListForm table table.shared-from,div#SuggestionForm table table.shared-from,div#MetaBiddingForm table table.shared-from,div#ExternalReviewForm table table.shared-from,div#ReferenceForm table table.shared-from,div#BiddingForm table table.shared-from,div#SubmissionListForm table table.shared-from,div#EmailMessagesForm table table.shared-from,div#AuditForm table table.shared-from,div#ReviewerInvitationListForm table table.shared-from,div#ReviewerInvitationForSubmissionListForm table table.shared-from,div#userListForm table table.shared-from,div#AutoAssignmentPapers table table.shared-from,div#AutoAssignmentReviewers table table.shared-from,div#AutoAssignmentSettings table table.shared-from,div#AutoAssignmentConfirmation table table.shared-from{border:none}.table-common-container table table.shared-from tbody,div#ProceedingEditorSubmissions table table.shared-from tbody,div#divUserDisputeConflicts table table.shared-from tbody,div#metaReviewerListForm table table.shared-from tbody,div#reviewerListForm table table.shared-from tbody,div#DeletedSubmissionListForm table table.shared-from tbody,div#SuggestionForm table table.shared-from tbody,div#MetaBiddingForm table table.shared-from tbody,div#ExternalReviewForm table table.shared-from tbody,div#ReferenceForm table table.shared-from tbody,div#BiddingForm table table.shared-from tbody,div#SubmissionListForm table table.shared-from tbody,div#EmailMessagesForm table table.shared-from tbody,div#AuditForm table table.shared-from tbody,div#ReviewerInvitationListForm table table.shared-from tbody,div#ReviewerInvitationForSubmissionListForm table table.shared-from tbody,div#userListForm table table.shared-from tbody,div#AutoAssignmentPapers table table.shared-from tbody,div#AutoAssignmentReviewers table table.shared-from tbody,div#AutoAssignmentSettings table table.shared-from tbody,div#AutoAssignmentConfirmation table table.shared-from tbody,.table-common-container table table.shared-from tr,div#ProceedingEditorSubmissions table table.shared-from tr,div#divUserDisputeConflicts table table.shared-from tr,div#metaReviewerListForm table table.shared-from tr,div#reviewerListForm table table.shared-from tr,div#DeletedSubmissionListForm table table.shared-from tr,div#SuggestionForm table table.shared-from tr,div#MetaBiddingForm table table.shared-from tr,div#ExternalReviewForm table table.shared-from tr,div#ReferenceForm table table.shared-from tr,div#BiddingForm table table.shared-from tr,div#SubmissionListForm table table.shared-from tr,div#EmailMessagesForm table table.shared-from tr,div#AuditForm table table.shared-from tr,div#ReviewerInvitationListForm table table.shared-from tr,div#ReviewerInvitationForSubmissionListForm table table.shared-from tr,div#userListForm table table.shared-from tr,div#AutoAssignmentPapers table table.shared-from tr,div#AutoAssignmentReviewers table table.shared-from tr,div#AutoAssignmentSettings table table.shared-from tr,div#AutoAssignmentConfirmation table table.shared-from tr,.table-common-container table table.shared-from td,div#ProceedingEditorSubmissions table table.shared-from td,div#divUserDisputeConflicts table table.shared-from td,div#metaReviewerListForm table table.shared-from td,div#reviewerListForm table table.shared-from td,div#DeletedSubmissionListForm table table.shared-from td,div#SuggestionForm table table.shared-from td,div#MetaBiddingForm table table.shared-from td,div#ExternalReviewForm table table.shared-from td,div#ReferenceForm table table.shared-from td,div#BiddingForm table table.shared-from td,div#SubmissionListForm table table.shared-from td,div#EmailMessagesForm table table.shared-from td,div#AuditForm table table.shared-from td,div#ReviewerInvitationListForm table table.shared-from td,div#ReviewerInvitationForSubmissionListForm table table.shared-from td,div#userListForm table table.shared-from td,div#AutoAssignmentPapers table table.shared-from td,div#AutoAssignmentReviewers table table.shared-from td,div#AutoAssignmentSettings table table.shared-from td,div#AutoAssignmentConfirmation table table.shared-from td{background-color:transparent;border:none}.table-common-container table table.shared-from td,div#ProceedingEditorSubmissions table table.shared-from td,div#divUserDisputeConflicts table table.shared-from td,div#metaReviewerListForm table table.shared-from td,div#reviewerListForm table table.shared-from td,div#DeletedSubmissionListForm table table.shared-from td,div#SuggestionForm table table.shared-from td,div#MetaBiddingForm table table.shared-from td,div#ExternalReviewForm table table.shared-from td,div#ReferenceForm table table.shared-from td,div#BiddingForm table table.shared-from td,div#SubmissionListForm table table.shared-from td,div#EmailMessagesForm table table.shared-from td,div#AuditForm table table.shared-from td,div#ReviewerInvitationListForm table table.shared-from td,div#ReviewerInvitationForSubmissionListForm table table.shared-from td,div#userListForm table table.shared-from td,div#AutoAssignmentPapers table table.shared-from td,div#AutoAssignmentReviewers table table.shared-from td,div#AutoAssignmentSettings table table.shared-from td,div#AutoAssignmentConfirmation table table.shared-from td{white-space:nowrap;text-align:left}.table-common-container table table.smr-name-rating,div#ProceedingEditorSubmissions table table.smr-name-rating,div#divUserDisputeConflicts table table.smr-name-rating,div#metaReviewerListForm table table.smr-name-rating,div#reviewerListForm table table.smr-name-rating,div#DeletedSubmissionListForm table table.smr-name-rating,div#SuggestionForm table table.smr-name-rating,div#MetaBiddingForm table table.smr-name-rating,div#ExternalReviewForm table table.smr-name-rating,div#ReferenceForm table table.smr-name-rating,div#BiddingForm table table.smr-name-rating,div#SubmissionListForm table table.smr-name-rating,div#EmailMessagesForm table table.smr-name-rating,div#AuditForm table table.smr-name-rating,div#ReviewerInvitationListForm table table.smr-name-rating,div#ReviewerInvitationForSubmissionListForm table table.smr-name-rating,div#userListForm table table.smr-name-rating,div#AutoAssignmentPapers table table.smr-name-rating,div#AutoAssignmentReviewers table table.smr-name-rating,div#AutoAssignmentSettings table table.smr-name-rating,div#AutoAssignmentConfirmation table table.smr-name-rating{border:none}.table-common-container table table.smr-name-rating tbody,div#ProceedingEditorSubmissions table table.smr-name-rating tbody,div#divUserDisputeConflicts table table.smr-name-rating tbody,div#metaReviewerListForm table table.smr-name-rating tbody,div#reviewerListForm table table.smr-name-rating tbody,div#DeletedSubmissionListForm table table.smr-name-rating tbody,div#SuggestionForm table table.smr-name-rating tbody,div#MetaBiddingForm table table.smr-name-rating tbody,div#ExternalReviewForm table table.smr-name-rating tbody,div#ReferenceForm table table.smr-name-rating tbody,div#BiddingForm table table.smr-name-rating tbody,div#SubmissionListForm table table.smr-name-rating tbody,div#EmailMessagesForm table table.smr-name-rating tbody,div#AuditForm table table.smr-name-rating tbody,div#ReviewerInvitationListForm table table.smr-name-rating tbody,div#ReviewerInvitationForSubmissionListForm table table.smr-name-rating tbody,div#userListForm table table.smr-name-rating tbody,div#AutoAssignmentPapers table table.smr-name-rating tbody,div#AutoAssignmentReviewers table table.smr-name-rating tbody,div#AutoAssignmentSettings table table.smr-name-rating tbody,div#AutoAssignmentConfirmation table table.smr-name-rating tbody,.table-common-container table table.smr-name-rating tr,div#ProceedingEditorSubmissions table table.smr-name-rating tr,div#divUserDisputeConflicts table table.smr-name-rating tr,div#metaReviewerListForm table table.smr-name-rating tr,div#reviewerListForm table table.smr-name-rating tr,div#DeletedSubmissionListForm table table.smr-name-rating tr,div#SuggestionForm table table.smr-name-rating tr,div#MetaBiddingForm table table.smr-name-rating tr,div#ExternalReviewForm table table.smr-name-rating tr,div#ReferenceForm table table.smr-name-rating tr,div#BiddingForm table table.smr-name-rating tr,div#SubmissionListForm table table.smr-name-rating tr,div#EmailMessagesForm table table.smr-name-rating tr,div#AuditForm table table.smr-name-rating tr,div#ReviewerInvitationListForm table table.smr-name-rating tr,div#ReviewerInvitationForSubmissionListForm table table.smr-name-rating tr,div#userListForm table table.smr-name-rating tr,div#AutoAssignmentPapers table table.smr-name-rating tr,div#AutoAssignmentReviewers table table.smr-name-rating tr,div#AutoAssignmentSettings table table.smr-name-rating tr,div#AutoAssignmentConfirmation table table.smr-name-rating tr,.table-common-container table table.smr-name-rating td,div#ProceedingEditorSubmissions table table.smr-name-rating td,div#divUserDisputeConflicts table table.smr-name-rating td,div#metaReviewerListForm table table.smr-name-rating td,div#reviewerListForm table table.smr-name-rating td,div#DeletedSubmissionListForm table table.smr-name-rating td,div#SuggestionForm table table.smr-name-rating td,div#MetaBiddingForm table table.smr-name-rating td,div#ExternalReviewForm table table.smr-name-rating td,div#ReferenceForm table table.smr-name-rating td,div#BiddingForm table table.smr-name-rating td,div#SubmissionListForm table table.smr-name-rating td,div#EmailMessagesForm table table.smr-name-rating td,div#AuditForm table table.smr-name-rating td,div#ReviewerInvitationListForm table table.smr-name-rating td,div#ReviewerInvitationForSubmissionListForm table table.smr-name-rating td,div#userListForm table table.smr-name-rating td,div#AutoAssignmentPapers table table.smr-name-rating td,div#AutoAssignmentReviewers table table.smr-name-rating td,div#AutoAssignmentSettings table table.smr-name-rating td,div#AutoAssignmentConfirmation table table.smr-name-rating td{background-color:transparent;border:none}.table-common-container table table.smr-name-rating td,div#ProceedingEditorSubmissions table table.smr-name-rating td,div#divUserDisputeConflicts table table.smr-name-rating td,div#metaReviewerListForm table table.smr-name-rating td,div#reviewerListForm table table.smr-name-rating td,div#DeletedSubmissionListForm table table.smr-name-rating td,div#SuggestionForm table table.smr-name-rating td,div#MetaBiddingForm table table.smr-name-rating td,div#ExternalReviewForm table table.smr-name-rating td,div#ReferenceForm table table.smr-name-rating td,div#BiddingForm table table.smr-name-rating td,div#SubmissionListForm table table.smr-name-rating td,div#EmailMessagesForm table table.smr-name-rating td,div#AuditForm table table.smr-name-rating td,div#ReviewerInvitationListForm table table.smr-name-rating td,div#ReviewerInvitationForSubmissionListForm table table.smr-name-rating td,div#userListForm table table.smr-name-rating td,div#AutoAssignmentPapers table table.smr-name-rating td,div#AutoAssignmentReviewers table table.smr-name-rating td,div#AutoAssignmentSettings table table.smr-name-rating td,div#AutoAssignmentConfirmation table table.smr-name-rating td{text-align:left}div.truncate{width:60px;white-space:nowrap;overflow:hidden;text-overflow:ellipsis}div#AutoAssignmentPapers td.id,div#AutoAssignmentPapers th.id{width:60px}div#AutoAssignmentPapers td.id{font-weight:bold}div#AutoAssignmentPapers td.title{text-align:left}div#AutoAssignmentPapers td.track{width:80px}div#AutoAssignmentPapers td.assigned,div#AutoAssignmentPapers th.assigned{width:100px}div#AutoAssignmentPapers td.completed,div#AutoAssignmentPapers th.completed{width:100px}div#AutoAssignmentPapers td.reviewers,div#AutoAssignmentPapers th.reviewers{width:240px}div#AutoAssignmentPapers .reviewers input{width:calc(30%);text-align:center;margin:3px;border-radius:10px}div#AutoAssignmentPapers td{padding:0 10px}div#AutoAssignmentPapers .min-title{font-size:13px;text-transform:capitalize;text-decoration:underline;font-weight:bold}div#AutoAssignmentPapers .min-row-title{display:inline-block;width:80px;text-align:left;font-size:13px;text-transform:none}div#AutoAssignmentPapers .mon-row-field{width:20px;margin:0;border-radius:10px}div#AutoAssignmentPapers input.error{background-color:#f5b7b7;border:dashed 1px red;border-radius:10px}div#AutoAssignmentPapers .assigned.error{font-weight:bold;color:green}div#AutoAssignmentReviewers td.id,div#AutoAssignmentReviewers th.id{width:60px}div#AutoAssignmentReviewers td.id{font-weight:bold}div#AutoAssignmentReviewers td.papers,div#AutoAssignmentReviewers th.papers{width:240px}div#AutoAssignmentReviewers td.comleted,div#AutoAssignmentReviewers th.completed,div#AutoAssignmentReviewers td.assigned,div#AutoAssignmentReviewers th.assigned,div#AutoAssignmentReviewers td.percentage,div#AutoAssignmentReviewers th.percentage{width:80px}div#AutoAssignmentReviewers td.name,div#AutoAssignmentReviewers th.name,div#AutoAssignmentReviewers td.surname,div#AutoAssignmentReviewers th.surname{width:100px}div#AutoAssignmentReviewers .papers input{width:calc(30%);text-align:center;margin:3px;border-radius:10px}div#AutoAssignmentReviewers td{padding:0 10px}div#AutoAssignmentReviewers .max-title{font-size:13px;text-transform:capitalize;text-decoration:underline;font-weight:bold}div#AutoAssignmentReviewers .min-row-title{display:inline-block;width:80px;text-align:left;font-size:13px;text-transform:none}div#AutoAssignmentReviewers .mon-row-field{width:20px;margin:0;border-radius:10px}div#AutoAssignmentReviewers input.error{background-color:#f5b7b7;border:dashed 1px red}.infoHeader tr>td:first-child{font-weight:bold;width:90px;vertical-align:top}.infoHeader td{padding-bottom:5px}.dropdown-menu-extra-size{min-width:300px}.dropdown-menu-extra-size a{width:260px!important}.dropdown-menu-small-size{min-width:180px}.dropdown-menu-small-size a{width:130px!important}#divDisputeDialog .control-group{margin-bottom:5px}#divDisputeDialog .control-group>.control-label{font-weight:bold;padding-top:0}#divDisputeDialog .control-group>.controls.value{padding-top:0}#divDisputeDialog .control-group>.controls.value ul{list-style:none;margin:0}.reviews-container .review-card{margin:10px 0}.reviews-container .review-card .heading{background-color:#f5f5f5;border-bottom:1px #d3d3d3 solid;overflow:auto;padding:10px;page-break-inside:avoid}.reviews-container .review-card .heading .title{margin:0;line-height:30px}.reviews-container .review-card .heading .rating-select{margin:0;width:auto}.reviews-container .review-card .body{padding:10px}.reviews-container .review-card .body ul.files,.reviews-container .review-card .body ul.ratings,.reviews-container .review-card .body ul.questions{list-style-type:none;margin:0}.reviews-container .review-card .body ul.questions>li{margin:5px 0}fieldset .return-button,fieldset .submission-info,fieldset .download-link,fieldset .command-box,fieldset .new-topic-button{margin-bottom:10px}fieldset .submission-info div{padding:2px 0}fieldset .submission-info label{font-weight:bold}fieldset .submission-info .title,fieldset .submission-info label{display:inline-block;width:150px}fieldset .topic-content label{display:inline-block;width:150px}fieldset .topic-content input,fieldset .topic-content textarea{display:inline-block;width:100%}fieldset .command-box{height:40px;border-radius:5px;background-color:#d3d3d3}fieldset .command-box table{height:40px}fieldset .command-box td{vertical-align:middle}fieldset .command-box .search{margin:0;margin-left:20px;font-style:italic;color:gray;font-size:12px}fieldset .command-box .view-change a{cursor:pointer}fieldset #discussion-feed table{height:40px;border-radius:5px;background-color:#eee;margin-bottom:20px}fieldset #discussion-feed table a{color:#006887}fieldset #discussion-feed .search-box{padding-top:10px;padding-left:5px}fieldset #discussion-feed .search{width:438px}fieldset #discussion-feed .sorting{text-align:right;padding-right:20px}fieldset #discussion-feed .sorting span,fieldset #discussion-feed .sorting ul,fieldset #discussion-feed .sorting li{display:inline-block;height:25px;line-height:25px;vertical-align:middle}fieldset #discussion-feed .sorting span{padding-left:20px}fieldset #discussion-feed .sorting ul{list-style-type:none}fieldset #discussion-feed .sorting li{float:left;padding:0 7px;cursor:pointer}fieldset #discussion-feed .sizer select{width:70px;margin:0}fieldset #discussion-feed #messages{list-style-type:none}fieldset #discussion-feed #messages li{border-bottom:1px solid #e5e5e5;margin-bottom:10px}fieldset #discussion-feed #messages .item-reviewer .reviewer-name{display:inline-block;margin-right:10px;font-weight:bold}fieldset #discussion-feed #messages .item-reviewer .date-title,fieldset #discussion-feed #messages .item-reviewer .date-value{font-style:italic;color:#555}fieldset #discussion-feed #messages .item-topic,fieldset #discussion-feed #messages .item-message{margin:5px}fieldset #discussion-feed #messages .item-commands a{cursor:pointer}fieldset #discussion-feed #messages .reply-form textarea{width:100%}.datepiker{width:calc(80%);margin-right:10px;cursor:pointer}table a i+span{padding-left:3px}.like-h2{color:#555;background:#f5f5f5;padding:7px 0 7px 10px;font-size:11.9px;border-bottom:1px solid #e5e5e5;margin:10px 0}.text-uppercase{text-transform:uppercase}.disabled{pointer-events:none}.strike{text-decoration:line-through}.no-margin-bottom{margin-bottom:0}.padding-top-2{padding-top:2px}.padding-top-5{padding-top:5px}.padding-vertical-5{padding-top:5px;padding-bottom:5px}.padding-top-7{padding-top:7px}.padding-bottom-5{padding-bottom:5px;width:150px}.strong{font-weight:bold}.sortable{cursor:pointer}.sortable i.icon-arrow-down,.sortable i.icon-arrow-up{margin-left:5px}.sortable .sortlink{text-decoration:none;color:inherit}.sortable:hover{text-decoration:underline}.large{font-size:17.5px}.larger{font-size:16.1px}.font-size-normal{font-size:14px}.orange{color:#ffa500}.green{color:green}.alert_no_backgroud{color:#2d6987;font-style:italic}.header_10px_margin{font-size:small;margin:10px 0}.error_text{color:#b94a48}.inline-block{display:inline-block}.messages-top{position:relative}.messages-above-overlay{z-index:1050;position:relative}.just-small{font-size:10.5px}.just-tiny{font-size:9.1px}.left{text-align:left}.hour{height:60px;border-bottom:solid #000 1px}ul.session-planning-sessions{list-style-type:none;margin-left:0}ul.session-planning-sessions>li{margin-bottom:30px}ul.session-planning-sessions>li .session-planning-session-details{margin-bottom:10px}ul.session-planning-sessions>li ul.session-planning-presentations>li{margin-bottom:10px}ul.session-planning-sessions>li ul.session-planning-presentations>li ul.session-planning-presenters{margin-left:0;list-style-type:none}ul.session-planning-sessions>li ul.session-planning-presentations>li ul.session-planning-presenters>li{display:inline-block}ul.session-planning-sessions>li ul.session-planning-presentations>li ul.session-planning-presenters>li:after{content:"; "}ul.session-planning-sessions>li ul.session-planning-presentations>li ul.session-planning-presenters>li:last-child:after{content:""}.session-planning-conflict-candidates>ul{list-style:none;display:inline;margin-left:0;margin-right:10px}.session-planning-conflict-candidates>ul>li{display:inline-block;margin-right:inherit}.session-planning-conflict-candidates>ul>li>.close{margin-left:5px}ul.session-planning-conflict-results{list-style:none}ul.session-planning-conflict-results>li{margin-bottom:30px}.menusection{margin-top:5px;padding:5px;background-color:#add8e6;color:#fff}.italic{font-style:italic}.nowrap_inline_block{display:inline-block;white-space:nowrap}.toggleable-column{position:relative}.toggleable-column .column-visibility-button{position:absolute;top:0;right:0;padding:2px 2px;display:none;border-radius:0 0 0 2px;background-color:#007ea3;color:#fff}.toggleable-column:hover .column-visibility-button{display:block}.app-download-icon img{margin-left:16px;height:36px;width:120px}.question+.tooltip>.tooltip-inner{max-width:350px;border:1px solid green;padding:10px;font-size:1.2em;text-align:left}.login-box{background-color:#fff;margin:2em auto;border:solid 1px #999;border-radius:3px}.login-box .login-box-content{padding:1em}.login-box header{padding:.5em;font-size:21px;line-height:40px;background-color:#007ea3;color:#fff;text-align:center}.login-box input,.login-box button[type="submit"],.login-box a.btn{height:3em;line-height:2.25em;width:100%!important;-webkit-box-sizing:border-box;-moz-box-sizing:border-box;box-sizing:border-box}.login-box .login-providers{margin-top:.75em}.login-box form{padding:0;margin:0}@media(max-width:767px){.login-box{width:calc(90%);max-width:calc(90%)}}@media(min-width:768px){.login-box{width:400px;max-width:400px}}.text-preline{white-space:pre-line}.disabled-question{opacity:.7}.margin-bottom-10{margin-bottom:10px}.edit-domains{display:inline-block;width:100%;max-width:600px;margin:0}.previewEmail{width:620px}.af-comment-form input,.af-comment-form textarea{width:100%}.af-comment{padding-top:10px}.af-comment+.af-comment{padding-left:10px}.af-comment+.af-comment>div{border-left:4px solid gray;padding-left:5px}.inline-editable>i.icon-edit{display:none;margin-left:5px}.inline-editable:hover>i.icon-edit{display:inline-block}button.ui-datepicker-trigger{border:none;background-color:transparent}.activity-row td.activty-name{width:200px}.activity-row span.label-warning{display:none}.activity-row:hover span.label-warning{display:inline-block}a>i.fa,a>i.fas,a>i.far,a>i.fal,a>i.fad,a>i.fab{color:#333;min-width:14px;min-height:14px;text-align:center;font-size:16px}

==> icde2022-reviews_files/underscore <==
//     Underscore.js 1.6.0
//     http://underscorejs.org
//     (c) 2009-2014 Jeremy Ashkenas, DocumentCloud and Investigative Reporters & Editors
//     Underscore may be freely distributed under the MIT license.

(function() {

    // Baseline setup
    // --------------

    // Establish the root object, `window` in the browser, or `exports` on the server.
    var root = this;

    // Save the previous value of the `_` variable.
    var previousUnderscore = root._;

    // Establish the object that gets returned to break out of a loop iteration.
    var breaker = {};

    // Save bytes in the minified (but not gzipped) version:
    var ArrayProto = Array.prototype, ObjProto = Object.prototype, FuncProto = Function.prototype;

    // Create quick reference variables for speed access to core prototypes.
    var
        push = ArrayProto.push,
        slice = ArrayProto.slice,
        concat = ArrayProto.concat,
        toString = ObjProto.toString,
        hasOwnProperty = ObjProto.hasOwnProperty;

    // All **ECMAScript 5** native function implementations that we hope to use
    // are declared here.
    var
        nativeIsArray = Array.isArray,
        nativeKeys = Object.keys,
        nativeBind = FuncProto.bind;

    // Create a safe reference to the Underscore object for use below.
    var _ = function(obj) {
        if (obj instanceof _) return obj;
        if (!(this instanceof _)) return new _(obj);
        this._wrapped = obj;
    };

    // Export the Underscore object for **Node.js**, with
    // backwards-compatibility for the old `require()` API. If we're in
    // the browser, add `_` as a global object via a string identifier,
    // for Closure Compiler "advanced" mode.
    if (typeof exports !== 'undefined') {
        if (typeof module !== 'undefined' && module.exports) {
            exports = module.exports = _;
        }
        exports._ = _;
    } else {
        root._ = _;
    }

    // Current version.
    _.VERSION = '1.6.0';

    // Collection Functions
    // --------------------

    // The cornerstone, an `each` implementation, aka `forEach`.
    // Handles raw objects in addition to array-likes. Treats all
    // sparse array-likes as if they were dense.
    _.each = _.forEach = function(obj, iterator, context) {
        if (obj == null) return obj;
        if (obj.length === +obj.length) {
            for (var i = 0, length = obj.length; i < length; i++) {
                if (iterator.call(context, obj[i], i, obj) === breaker) return;
            }
        } else {
            var keys = _.keys(obj);
            for (var i = 0, length = keys.length; i < length; i++) {
                if (iterator.call(context, obj[keys[i]], keys[i], obj) === breaker) return;
            }
        }
        return obj;
    };

    // Return the results of applying the iterator to each element.
    _.map = _.collect = function(obj, iterator, context) {
        var results = [];
        if (obj == null) return results;
        _.each(obj, function(value, index, list) {
            results.push(iterator.call(context, value, index, list));
        });
        return results;
    };

    var reduceError = 'Reduce of empty array with no initial value';

    // **Reduce** builds up a single result from a list of values, aka `inject`,
    // or `foldl`.
    _.reduce = _.foldl = _.inject = function(obj, iterator, memo, context) {
        var initial = arguments.length > 2;
        if (obj == null) obj = [];
        _.each(obj, function(value, index, list) {
            if (!initial) {
                memo = value;
                initial = true;
            } else {
                memo = iterator.call(context, memo, value, index, list);
            }
        });
        if (!initial) throw new TypeError(reduceError);
        return memo;
    };

    // The right-associative version of reduce, also known as `foldr`.
    _.reduceRight = _.foldr = function(obj, iterator, memo, context) {
        var initial = arguments.length > 2;
        if (obj == null) obj = [];
        var length = obj.length;
        if (length !== +length) {
            var keys = _.keys(obj);
            length = keys.length;
        }
        _.each(obj, function(value, index, list) {
            index = keys ? keys[--length] : --length;
            if (!initial) {
                memo = obj[index];
                initial = true;
            } else {
                memo = iterator.call(context, memo, obj[index], index, list);
            }
        });
        if (!initial) throw new TypeError(reduceError);
        return memo;
    };

    // Return the first value which passes a truth test. Aliased as `detect`.
    _.find = _.detect = function(obj, predicate, context) {
        var result;
        _.some(obj, function(value, index, list) {
            if (predicate.call(context, value, index, list)) {
                result = value;
                return true;
            }
        });
        return result;
    };

    // Return all the elements that pass a truth test.
    // Aliased as `select`.
    _.filter = _.select = function(obj, predicate, context) {
        var results = [];
        if (obj == null) return results;
        _.each(obj, function(value, index, list) {
            if (predicate.call(context, value, index, list)) results.push(value);
        });
        return results;
    };

    // Return all the elements for which a truth test fails.
    _.reject = function(obj, predicate, context) {
        return _.filter(obj, _.negate(predicate), context);
    };

    // Determine whether all of the elements match a truth test.
    // Aliased as `all`.
    _.every = _.all = function(obj, predicate, context) {
        predicate || (predicate = _.identity);
        var result = true;
        if (obj == null) return result;
        _.each(obj, function(value, index, list) {
            if (!(result = result && predicate.call(context, value, index, list))) return breaker;
        });
        return !!result;
    };

    // Determine if at least one element in the object matches a truth test.
    // Aliased as `any`.
    _.some = _.any = function(obj, predicate, context) {
        predicate || (predicate = _.identity);
        var result = false;
        if (obj == null) return result;
        _.each(obj, function(value, index, list) {
            if (result || (result = predicate.call(context, value, index, list))) return breaker;
        });
        return !!result;
    };

    // Determine if the array or object contains a given value (using `===`).
    // Aliased as `include`.
    _.contains = _.include = function(obj, target) {
        if (obj == null) return false;
        if (obj.length === +obj.length) return _.indexOf(obj, target) >= 0;
        return _.some(obj, function(value) {
            return value === target;
        });
    };

    // Invoke a method (with arguments) on every item in a collection.
    _.invoke = function(obj, method) {
        var args = slice.call(arguments, 2);
        var isFunc = _.isFunction(method);
        return _.map(obj, function(value) {
            return (isFunc ? method : value[method]).apply(value, args);
        });
    };

    // Convenience version of a common use case of `map`: fetching a property.
    _.pluck = function(obj, key) {
        return _.map(obj, _.property(key));
    };

    // Convenience version of a common use case of `filter`: selecting only objects
    // containing specific `key:value` pairs.
    _.where = function(obj, attrs) {
        return _.filter(obj, _.matches(attrs));
    };

    // Convenience version of a common use case of `find`: getting the first object
    // containing specific `key:value` pairs.
    _.findWhere = function(obj, attrs) {
        return _.find(obj, _.matches(attrs));
    };

    // Return the maximum element or (element-based computation).
    _.max = function(obj, iterator, context) {
        var result = -Infinity,
            lastComputed = -Infinity,
            value,
            computed;
        if (!iterator && _.isArray(obj)) {
            for (var i = 0, length = obj.length; i < length; i++) {
                value = obj[i];
                if (value > result) {
                    result = value;
                }
            }
        } else {
            _.each(obj, function(value, index, list) {
                computed = iterator ? iterator.call(context, value, index, list) : value;
                if (computed > lastComputed) {
                    result = value;
                    lastComputed = computed;
                }
            });
        }
        return result;
    };

    // Return the minimum element (or element-based computation).
    _.min = function(obj, iterator, context) {
        var result = Infinity,
            lastComputed = Infinity,
            value,
            computed;
        if (!iterator && _.isArray(obj)) {
            for (var i = 0, length = obj.length; i < length; i++) {
                value = obj[i];
                if (value < result) {
                    result = value;
                }
            }
        } else {
            _.each(obj, function(value, index, list) {
                computed = iterator ? iterator.call(context, value, index, list) : value;
                if (computed < lastComputed) {
                    result = value;
                    lastComputed = computed;
                }
            });
        }
        return result;
    };

    // Shuffle an array, using the modern version of the
    // [Fisher-Yates shuffle](http://en.wikipedia.org/wiki/Fisher–Yates_shuffle).
    _.shuffle = function(obj) {
        var rand;
        var index = 0;
        var shuffled = [];
        _.each(obj, function(value) {
            rand = _.random(index++);
            shuffled[index - 1] = shuffled[rand];
            shuffled[rand] = value;
        });
        return shuffled;
    };

    // Sample **n** random values from a collection.
    // If **n** is not specified, returns a single random element.
    // The internal `guard` argument allows it to work with `map`.
    _.sample = function(obj, n, guard) {
        if (n == null || guard) {
            if (obj.length !== +obj.length) obj = _.values(obj);
            return obj[_.random(obj.length - 1)];
        }
        return _.shuffle(obj).slice(0, Math.max(0, n));
    };

    // An internal function to generate lookup iterators.
    var lookupIterator = function(value, context) {
        if (value == null) return _.identity;
        if (!_.isFunction(value)) return _.property(value);
        if (!context) return value;
        return function() {
            return value.apply(context, arguments);
        };
    };

    // Sort the object's values by a criterion produced by an iterator.
    _.sortBy = function(obj, iterator, context) {
        iterator = lookupIterator(iterator, context);
        return _.pluck(_.map(obj, function(value, index, list) {
            return {
                value: value,
                index: index,
                criteria: iterator(value, index, list)
            };
        }).sort(function(left, right) {
            var a = left.criteria;
            var b = right.criteria;
            if (a !== b) {
                if (a > b || a === void 0) return 1;
                if (a < b || b === void 0) return -1;
            }
            return left.index - right.index;
        }), 'value');
    };

    // An internal function used for aggregate "group by" operations.
    var group = function(behavior) {
        return function(obj, iterator, context) {
            var result = {};
            iterator = lookupIterator(iterator, context);
            _.each(obj, function(value, index) {
                var key = iterator(value, index, obj);
                behavior(result, value, key);
            });
            return result;
        };
    };

    // Groups the object's values by a criterion. Pass either a string attribute
    // to group by, or a function that returns the criterion.
    _.groupBy = group(function(result, value, key) {
        _.has(result, key) ? result[key].push(value) : result[key] = [value];
    });

    // Indexes the object's values by a criterion, similar to `groupBy`, but for
    // when you know that your index values will be unique.
    _.indexBy = group(function(result, value, key) {
        result[key] = value;
    });

    // Counts instances of an object that group by a certain criterion. Pass
    // either a string attribute to count by, or a function that returns the
    // criterion.
    _.countBy = group(function(result, value, key) {
        _.has(result, key) ? result[key]++ : result[key] = 1;
    });

    // Use a comparator function to figure out the smallest index at which
    // an object should be inserted so as to maintain order. Uses binary search.
    _.sortedIndex = function(array, obj, iterator, context) {
        iterator = lookupIterator(iterator, context);
        var value = iterator(obj);
        var low = 0, high = array.length;
        while (low < high) {
            var mid = (low + high) >>> 1;
            iterator(array[mid]) < value ? low = mid + 1 : high = mid;
        }
        return low;
    };

    // Safely create a real, live array from anything iterable.
    _.toArray = function(obj) {
        if (!obj) return [];
        if (_.isArray(obj)) return slice.call(obj);
        if (obj.length === +obj.length) return _.map(obj, _.identity);
        return _.values(obj);
    };

    // Return the number of elements in an object.
    _.size = function(obj) {
        if (obj == null) return 0;
        return (obj.length === +obj.length) ? obj.length : _.keys(obj).length;
    };

    // Array Functions
    // ---------------

    // Get the first element of an array. Passing **n** will return the first N
    // values in the array. Aliased as `head` and `take`. The **guard** check
    // allows it to work with `_.map`.
    _.first = _.head = _.take = function(array, n, guard) {
        if (array == null) return void 0;
        if ((n == null) || guard) return array[0];
        if (n < 0) return [];
        return slice.call(array, 0, n);
    };

    // Returns everything but the last entry of the array. Especially useful on
    // the arguments object. Passing **n** will return all the values in
    // the array, excluding the last N. The **guard** check allows it to work with
    // `_.map`.
    _.initial = function(array, n, guard) {
        return slice.call(array, 0, Math.max(0, array.length - (n == null || guard ? 1 : n)));
    };

    // Get the last element of an array. Passing **n** will return the last N
    // values in the array. The **guard** check allows it to work with `_.map`.
    _.last = function(array, n, guard) {
        if (array == null) return void 0;
        if ((n == null) || guard) return array[array.length - 1];
        return slice.call(array, Math.max(array.length - n, 0));
    };

    // Returns everything but the first entry of the array. Aliased as `tail` and `drop`.
    // Especially useful on the arguments object. Passing an **n** will return
    // the rest N values in the array. The **guard**
    // check allows it to work with `_.map`.
    _.rest = _.tail = _.drop = function(array, n, guard) {
        return slice.call(array, (n == null) || guard ? 1 : n);
    };

    // Trim out all falsy values from an array.
    _.compact = function(array) {
        return _.filter(array, _.identity);
    };

    // Internal implementation of a recursive `flatten` function.
    var flatten = function(input, shallow, strict, output) {
        if (shallow && _.every(input, _.isArray)) {
            return concat.apply(output, input);
        }
        for (var i = 0, length = input.length; i < length; i++) {
            var value = input[i];
            if (!_.isArray(value) && !_.isArguments(value)) {
                if (!strict) output.push(value);
            } else if (shallow) {
                push.apply(output, value);
            } else {
                flatten(value, shallow, strict, output);
            }
        }
        return output;
    };

    // Flatten out an array, either recursively (by default), or just one level.
    _.flatten = function(array, shallow) {
        return flatten(array, shallow, false, []);
    };

    // Return a version of the array that does not contain the specified value(s).
    _.without = function(array) {
        return _.difference(array, slice.call(arguments, 1));
    };

    // Split an array into two arrays: one whose elements all satisfy the given
    // predicate, and one whose elements all do not satisfy the predicate.
    _.partition = function(obj, predicate, context) {
        predicate = lookupIterator(predicate, context);
        var pass = [], fail = [];
        _.each(obj, function(value, key, obj) {
            (predicate(value, key, obj) ? pass : fail).push(value);
        });
        return [pass, fail];
    };

    // Produce a duplicate-free version of the array. If the array has already
    // been sorted, you have the option of using a faster algorithm.
    // Aliased as `unique`.
    _.uniq = _.unique = function(array, isSorted, iterator, context) {
        if (array == null) return [];
        if (_.isFunction(isSorted)) {
            context = iterator;
            iterator = isSorted;
            isSorted = false;
        }
        var result = [];
        var seen = [];
        for (var i = 0, length = array.length; i < length; i++) {
            var value = array[i];
            if (iterator) value = iterator.call(context, value, i, array);
            if (isSorted ? (!i || seen !== value) : !_.contains(seen, value)) {
                if (isSorted) seen = value;
                else seen.push(value);
                result.push(array[i]);
            }
        }
        return result;
    };

    // Produce an array that contains the union: each distinct element from all of
    // the passed-in arrays.
    _.union = function() {
        return _.uniq(flatten(arguments, true, true, []));
    };

    // Produce an array that contains every item shared between all the
    // passed-in arrays.
    _.intersection = function(array) {
        if (array == null) return [];
        var result = [];
        var argsLength = arguments.length;
        for (var i = 0, length = array.length; i < length; i++) {
            var item = array[i];
            if (_.contains(result, item)) continue;
            for (var j = 1; j < argsLength; j++) {
                if (!_.contains(arguments[j], item)) break;
            }
            if (j === argsLength) result.push(item);
        }
        return result;
    };

    // Take the difference between one array and a number of other arrays.
    // Only the elements present in just the first array will remain.
    _.difference = function(array) {
        var rest = flatten(slice.call(arguments, 1), true, true, []);
        return _.filter(array, function(value) { return !_.contains(rest, value); });
    };

    // Zip together multiple lists into a single array -- elements that share
    // an index go together.
    _.zip = function() {
        var length = _.max(_.pluck(arguments, 'length').concat(0));
        var results = new Array(length);
        for (var i = 0; i < length; i++) {
            results[i] = _.pluck(arguments, '' + i);
        }
        return results;
    };

    // Converts lists into objects. Pass either a single array of `[key, value]`
    // pairs, or two parallel arrays of the same length -- one of keys, and one of
    // the corresponding values.
    _.object = function(list, values) {
        if (list == null) return {};
        var result = {};
        for (var i = 0, length = list.length; i < length; i++) {
            if (values) {
                result[list[i]] = values[i];
            } else {
                result[list[i][0]] = list[i][1];
            }
        }
        return result;
    };

    // Return the position of the first occurrence of an item in an array,
    // or -1 if the item is not included in the array.
    // If the array is large and already in sort order, pass `true`
    // for **isSorted** to use binary search.
    _.indexOf = function(array, item, isSorted) {
        if (array == null) return -1;
        var i = 0, length = array.length;
        if (isSorted) {
            if (typeof isSorted == 'number') {
                i = (isSorted < 0 ? Math.max(0, length + isSorted) : isSorted);
            } else {
                i = _.sortedIndex(array, item);
                return array[i] === item ? i : -1;
            }
        }
        for (; i < length; i++) if (array[i] === item) return i;
        return -1;
    };

    _.lastIndexOf = function(array, item, from) {
        if (array == null) return -1;
        var i = from == null ? array.length : from;
        while (i--) if (array[i] === item) return i;
        return -1;
    };

    // Generate an integer Array containing an arithmetic progression. A port of
    // the native Python `range()` function. See
    // [the Python documentation](http://docs.python.org/library/functions.html#range).
    _.range = function(start, stop, step) {
        if (arguments.length <= 1) {
            stop = start || 0;
            start = 0;
        }
        step = arguments[2] || 1;

        var length = Math.max(Math.ceil((stop - start) / step), 0);
        var idx = 0;
        var range = new Array(length);

        while (idx < length) {
            range[idx++] = start;
            start += step;
        }

        return range;
    };

    // Function (ahem) Functions
    // ------------------

    // Reusable constructor function for prototype setting.
    var ctor = function() {};

    // Create a function bound to a given object (assigning `this`, and arguments,
    // optionally). Delegates to **ECMAScript 5**'s native `Function.bind` if
    // available.
    _.bind = function(func, context) {
        var args, bound;
        if (nativeBind && func.bind === nativeBind) return nativeBind.apply(func, slice.call(arguments, 1));
        if (!_.isFunction(func)) throw new TypeError('Bind must be called on a function');
        args = slice.call(arguments, 2);
        return bound = function() {
            if (!(this instanceof bound)) return func.apply(context, args.concat(slice.call(arguments)));
            ctor.prototype = func.prototype;
            var self = new ctor;
            ctor.prototype = null;
            var result = func.apply(self, args.concat(slice.call(arguments)));
            if (Object(result) === result) return result;
            return self;
        };
    };

    // Partially apply a function by creating a version that has had some of its
    // arguments pre-filled, without changing its dynamic `this` context. _ acts
    // as a placeholder, allowing any combination of arguments to be pre-filled.
    _.partial = function(func) {
        var boundArgs = slice.call(arguments, 1);
        return function() {
            var position = 0;
            var args = boundArgs.slice();
            for (var i = 0, length = args.length; i < length; i++) {
                if (args[i] === _) args[i] = arguments[position++];
            }
            while (position < arguments.length) args.push(arguments[position++]);
            return func.apply(this, args);
        };
    };

    // Bind a number of an object's methods to that object. Remaining arguments
    // are the method names to be bound. Useful for ensuring that all callbacks
    // defined on an object belong to it.
    _.bindAll = function(obj) {
        var funcs = slice.call(arguments, 1);
        if (funcs.length === 0) throw new Error('bindAll must be passed function names');
        _.each(funcs, function(f) { obj[f] = _.bind(obj[f], obj); });
        return obj;
    };

    // Memoize an expensive function by storing its results.
    _.memoize = function(func, hasher) {
        var memo = {};
        hasher || (hasher = _.identity);
        return function() {
            var key = hasher.apply(this, arguments);
            return _.has(memo, key) ? memo[key] : (memo[key] = func.apply(this, arguments));
        };
    };

    // Delays a function for the given number of milliseconds, and then calls
    // it with the arguments supplied.
    _.delay = function(func, wait) {
        var args = slice.call(arguments, 2);
        return setTimeout(function() { return func.apply(null, args); }, wait);
    };

    // Defers a function, scheduling it to run after the current call stack has
    // cleared.
    _.defer = function(func) {
        return _.delay.apply(_, [func, 1].concat(slice.call(arguments, 1)));
    };

    // Returns a function, that, when invoked, will only be triggered at most once
    // during a given window of time. Normally, the throttled function will run
    // as much as it can, without ever going more than once per `wait` duration;
    // but if you'd like to disable the execution on the leading edge, pass
    // `{leading: false}`. To disable execution on the trailing edge, ditto.
    _.throttle = function(func, wait, options) {
        var context, args, result;
        var timeout = null;
        var previous = 0;
        options || (options = {});
        var later = function() {
            previous = options.leading === false ? 0 : _.now();
            timeout = null;
            result = func.apply(context, args);
            context = args = null;
        };
        return function() {
            var now = _.now();
            if (!previous && options.leading === false) previous = now;
            var remaining = wait - (now - previous);
            context = this;
            args = arguments;
            if (remaining <= 0 || remaining > wait) {
                clearTimeout(timeout);
                timeout = null;
                previous = now;
                result = func.apply(context, args);
                context = args = null;
            } else if (!timeout && options.trailing !== false) {
                timeout = setTimeout(later, remaining);
            }
            return result;
        };
    };

    // Returns a function, that, as long as it continues to be invoked, will not
    // be triggered. The function will be called after it stops being called for
    // N milliseconds. If `immediate` is passed, trigger the function on the
    // leading edge, instead of the trailing.
    _.debounce = function(func, wait, immediate) {
        var timeout, args, context, timestamp, result;

        var later = function() {
            var last = _.now() - timestamp;

            if (last < wait && last > 0) {
                timeout = setTimeout(later, wait - last);
            } else {
                timeout = null;
                if (!immediate) {
                    result = func.apply(context, args);
                    context = args = null;
                }
            }
        };

        return function() {
            context = this;
            args = arguments;
            timestamp = _.now();
            var callNow = immediate && !timeout;
            if (!timeout) {
                timeout = setTimeout(later, wait);
            }
            if (callNow) {
                result = func.apply(context, args);
                context = args = null;
            }

            return result;
        };
    };

    // Returns a function that will be executed at most one time, no matter how
    // often you call it. Useful for lazy initialization.
    _.once = function(func) {
        var ran = false, memo;
        return function() {
            if (ran) return memo;
            ran = true;
            memo = func.apply(this, arguments);
            func = null;
            return memo;
        };
    };

    // Returns the first function passed as an argument to the second,
    // allowing you to adjust arguments, run code before and after, and
    // conditionally execute the original function.
    _.wrap = function(func, wrapper) {
        return _.partial(wrapper, func);
    };

    // Returns a negated version of the passed-in predicate.
    _.negate = function(predicate) {
        return function() {
            return !predicate.apply(this, arguments);
        };
    };

    // Returns a function that is the composition of a list of functions, each
    // consuming the return value of the function that follows.
    _.compose = function() {
        var funcs = arguments;
        return function() {
            var args = arguments;
            for (var i = funcs.length - 1; i >= 0; i--) {
                args = [funcs[i].apply(this, args)];
            }
            return args[0];
        };
    };

    // Returns a function that will only be executed after being called N times.
    _.after = function(times, func) {
        return function() {
            if (--times < 1) {
                return func.apply(this, arguments);
            }
        };
    };

    // Object Functions
    // ----------------

    // Retrieve the names of an object's properties.
    // Delegates to **ECMAScript 5**'s native `Object.keys`
    _.keys = function(obj) {
        if (!_.isObject(obj)) return [];
        if (nativeKeys) return nativeKeys(obj);
        var keys = [];
        for (var key in obj) if (_.has(obj, key)) keys.push(key);
        return keys;
    };

    // Retrieve the values of an object's properties.
    _.values = function(obj) {
        var keys = _.keys(obj);
        var length = keys.length;
        var values = new Array(length);
        for (var i = 0; i < length; i++) {
            values[i] = obj[keys[i]];
        }
        return values;
    };

    // Convert an object into a list of `[key, value]` pairs.
    _.pairs = function(obj) {
        var keys = _.keys(obj);
        var length = keys.length;
        var pairs = new Array(length);
        for (var i = 0; i < length; i++) {
            pairs[i] = [keys[i], obj[keys[i]]];
        }
        return pairs;
    };

    // Invert the keys and values of an object. The values must be serializable.
    _.invert = function(obj) {
        var result = {};
        var keys = _.keys(obj);
        for (var i = 0, length = keys.length; i < length; i++) {
            result[obj[keys[i]]] = keys[i];
        }
        return result;
    };

    // Return a sorted list of the function names available on the object.
    // Aliased as `methods`
    _.functions = _.methods = function(obj) {
        var names = [];
        for (var key in obj) {
            if (_.isFunction(obj[key])) names.push(key);
        }
        return names.sort();
    };

    // Extend a given object with all the properties in passed-in object(s).
    _.extend = function(obj) {
        _.each(slice.call(arguments, 1), function(source) {
            if (source) {
                for (var prop in source) {
                    obj[prop] = source[prop];
                }
            }
        });
        return obj;
    };

    // Return a copy of the object only containing the whitelisted properties.
    _.pick = function(obj, iterator, context) {
        var result = {};
        if (_.isFunction(iterator)) {
            for (var key in obj) {
                var value = obj[key];
                if (iterator.call(context, value, key, obj)) result[key] = value;
            }
        } else {
            var keys = concat.apply([], slice.call(arguments, 1));
            for (var i = 0, length = keys.length; i < length; i++) {
                var key = keys[i];
                if (key in obj) result[key] = obj[key];
            }
        }
        return result;
    };

    // Return a copy of the object without the blacklisted properties.
    _.omit = function(obj, iterator, context) {
        var keys;
        if (_.isFunction(iterator)) {
            iterator = _.negate(iterator);
        } else {
            keys = _.map(concat.apply([], slice.call(arguments, 1)), String);
            iterator = function(value, key) { return !_.contains(keys, key); };
        }
        return _.pick(obj, iterator, context);
    };

    // Fill in a given object with default properties.
    _.defaults = function(obj) {
        _.each(slice.call(arguments, 1), function(source) {
            if (source) {
                for (var prop in source) {
                    if (obj[prop] === void 0) obj[prop] = source[prop];
                }
            }
        });
        return obj;
    };

    // Create a (shallow-cloned) duplicate of an object.
    _.clone = function(obj) {
        if (!_.isObject(obj)) return obj;
        return _.isArray(obj) ? obj.slice() : _.extend({}, obj);
    };

    // Invokes interceptor with the obj, and then returns obj.
    // The primary purpose of this method is to "tap into" a method chain, in
    // order to perform operations on intermediate results within the chain.
    _.tap = function(obj, interceptor) {
        interceptor(obj);
        return obj;
    };

    // Internal recursive comparison function for `isEqual`.
    var eq = function(a, b, aStack, bStack) {
        // Identical objects are equal. `0 === -0`, but they aren't identical.
        // See the [Harmony `egal` proposal](http://wiki.ecmascript.org/doku.php?id=harmony:egal).
        if (a === b) return a !== 0 || 1 / a == 1 / b;
        // A strict comparison is necessary because `null == undefined`.
        if (a == null || b == null) return a === b;
        // Unwrap any wrapped objects.
        if (a instanceof _) a = a._wrapped;
        if (b instanceof _) b = b._wrapped;
        // Compare `[[Class]]` names.
        var className = toString.call(a);
        if (className != toString.call(b)) return false;
        switch (className) {
            // Strings, numbers, dates, and booleans are compared by value.
        case '[object String]':
            // Primitives and their corresponding object wrappers are equivalent; thus, `"5"` is
            // equivalent to `new String("5")`.
            return a == String(b);
        case '[object Number]':
            // `NaN`s are equivalent, but non-reflexive. An `egal` comparison is performed for
            // other numeric values.
            return a != +a ? b != +b : (a == 0 ? 1 / a == 1 / b : a == +b);
        case '[object Date]':
        case '[object Boolean]':
            // Coerce dates and booleans to numeric primitive values. Dates are compared by their
            // millisecond representations. Note that invalid dates with millisecond representations
            // of `NaN` are not equivalent.
            return +a == +b;
        // RegExps are compared by their source patterns and flags.
        case '[object RegExp]':
            return a.source == b.source &&
                a.global == b.global &&
                a.multiline == b.multiline &&
                a.ignoreCase == b.ignoreCase;
        }
        if (typeof a != 'object' || typeof b != 'object') return false;
        // Assume equality for cyclic structures. The algorithm for detecting cyclic
        // structures is adapted from ES 5.1 section 15.12.3, abstract operation `JO`.
        var length = aStack.length;
        while (length--) {
            // Linear search. Performance is inversely proportional to the number of
            // unique nested structures.
            if (aStack[length] == a) return bStack[length] == b;
        }
        // Objects with different constructors are not equivalent, but `Object`s
        // from different frames are.
        var aCtor = a.constructor, bCtor = b.constructor;
        if (aCtor !== bCtor && !(_.isFunction(aCtor) && (aCtor instanceof aCtor) &&
                _.isFunction(bCtor) && (bCtor instanceof bCtor))
            && ('constructor' in a && 'constructor' in b)) {
            return false;
        }
        // Add the first object to the stack of traversed objects.
        aStack.push(a);
        bStack.push(b);
        var size = 0, result = true;
        // Recursively compare objects and arrays.
        if (className == '[object Array]') {
            // Compare array lengths to determine if a deep comparison is necessary.
            size = a.length;
            result = size == b.length;
            if (result) {
                // Deep compare the contents, ignoring non-numeric properties.
                while (size--) {
                    if (!(result = eq(a[size], b[size], aStack, bStack))) break;
                }
            }
        } else {
            // Deep compare objects.
            for (var key in a) {
                if (_.has(a, key)) {
                    // Count the expected number of properties.
                    size++;
                    // Deep compare each member.
                    if (!(result = _.has(b, key) && eq(a[key], b[key], aStack, bStack))) break;
                }
            }
            // Ensure that both objects contain the same number of properties.
            if (result) {
                for (key in b) {
                    if (_.has(b, key) && !(size--)) break;
                }
                result = !size;
            }
        }
        // Remove the first object from the stack of traversed objects.
        aStack.pop();
        bStack.pop();
        return result;
    };

    // Perform a deep comparison to check if two objects are equal.
    _.isEqual = function(a, b) {
        return eq(a, b, [], []);
    };

    // Is a given array, string, or object empty?
    // An "empty" object has no enumerable own-properties.
    _.isEmpty = function(obj) {
        if (obj == null) return true;
        if (_.isArray(obj) || _.isString(obj) || _.isArguments(obj)) return obj.length === 0;
        for (var key in obj) if (_.has(obj, key)) return false;
        return true;
    };

    // Is a given value a DOM element?
    _.isElement = function(obj) {
        return !!(obj && obj.nodeType === 1);
    };

    // Is a given value an array?
    // Delegates to ECMA5's native Array.isArray
    _.isArray = nativeIsArray || function(obj) {
        return toString.call(obj) == '[object Array]';
    };

    // Is a given variable an object?
    _.isObject = function(obj) {
        return obj === Object(obj);
    };

    // Add some isType methods: isArguments, isFunction, isString, isNumber, isDate, isRegExp.
    _.each(['Arguments', 'Function', 'String', 'Number', 'Date', 'RegExp'], function(name) {
        _['is' + name] = function(obj) {
            return toString.call(obj) == '[object ' + name + ']';
        };
    });

    // Define a fallback version of the method in browsers (ahem, IE), where
    // there isn't any inspectable "Arguments" type.
    if (!_.isArguments(arguments)) {
        _.isArguments = function(obj) {
            return !!(obj && _.has(obj, 'callee'));
        };
    }

    // Optimize `isFunction` if appropriate.
    if (typeof (/./) !== 'function') {
        _.isFunction = function(obj) {
            return typeof obj === 'function';
        };
    }

    // Is a given object a finite number?
    _.isFinite = function(obj) {
        return isFinite(obj) && !isNaN(parseFloat(obj));
    };

    // Is the given value `NaN`? (NaN is the only number which does not equal itself).
    _.isNaN = function(obj) {
        return _.isNumber(obj) && obj != +obj;
    };

    // Is a given value a boolean?
    _.isBoolean = function(obj) {
        return obj === true || obj === false || toString.call(obj) == '[object Boolean]';
    };

    // Is a given value equal to null?
    _.isNull = function(obj) {
        return obj === null;
    };

    // Is a given variable undefined?
    _.isUndefined = function(obj) {
        return obj === void 0;
    };

    // Shortcut function for checking if an object has a given property directly
    // on itself (in other words, not on a prototype).
    _.has = function(obj, key) {
        return hasOwnProperty.call(obj, key);
    };

    // Utility Functions
    // -----------------

    // Run Underscore.js in *noConflict* mode, returning the `_` variable to its
    // previous owner. Returns a reference to the Underscore object.
    _.noConflict = function() {
        root._ = previousUnderscore;
        return this;
    };

    // Keep the identity function around for default iterators.
    _.identity = function(value) {
        return value;
    };

    _.constant = function(value) {
        return function() {
            return value;
        };
    };

    _.noop = function() {};

    _.property = function(key) {
        return function(obj) {
            return obj[key];
        };
    };

    // Returns a predicate for checking whether an object has a given set of `key:value` pairs.
    _.matches = function(attrs) {
        return function(obj) {
            if (obj == null) return _.isEmpty(attrs);
            if (obj === attrs) return true;
            for (var key in attrs) if (attrs[key] !== obj[key]) return false;
            return true;
        };
    };

    // Run a function **n** times.
    _.times = function(n, iterator, context) {
        var accum = Array(Math.max(0, n));
        for (var i = 0; i < n; i++) accum[i] = iterator.call(context, i);
        return accum;
    };

    // Return a random integer between min and max (inclusive).
    _.random = function(min, max) {
        if (max == null) {
            max = min;
            min = 0;
        }
        return min + Math.floor(Math.random() * (max - min + 1));
    };

    // A (possibly faster) way to get the current timestamp as an integer.
    _.now = Date.now || function() { return new Date().getTime(); };

    // List of HTML entities for escaping.
    var entityMap = {
        escape: {
            '&': '&amp;',
            '<': '&lt;',
            '>': '&gt;',
            '"': '&quot;',
            "'": '&#x27;'
        }
    };
    entityMap.unescape = _.invert(entityMap.escape);

    // Regexes containing the keys and values listed immediately above.
    var entityRegexes = {
        escape: new RegExp('[' + _.keys(entityMap.escape).join('') + ']', 'g'),
        unescape: new RegExp('(' + _.keys(entityMap.unescape).join('|') + ')', 'g')
    };

    // Functions for escaping and unescaping strings to/from HTML interpolation.
    _.each(['escape', 'unescape'], function(method) {
        _[method] = function(string) {
            if (string == null) return '';
            return ('' + string).replace(entityRegexes[method], function(match) {
                return entityMap[method][match];
            });
        };
    });

    // If the value of the named `property` is a function then invoke it with the
    // `object` as context; otherwise, return it.
    _.result = function(object, property) {
        if (object == null) return void 0;
        var value = object[property];
        return _.isFunction(value) ? object[property]() : value;
    };

    // Add your own custom functions to the Underscore object.
    _.mixin = function(obj) {
        _.each(_.functions(obj), function(name) {
            var func = _[name] = obj[name];
            _.prototype[name] = function() {
                var args = [this._wrapped];
                push.apply(args, arguments);
                return result.call(this, func.apply(_, args));
            };
        });
    };

    // Generate a unique integer id (unique within the entire client session).
    // Useful for temporary DOM ids.
    var idCounter = 0;
    _.uniqueId = function(prefix) {
        var id = ++idCounter + '';
        return prefix ? prefix + id : id;
    };

    // By default, Underscore uses ERB-style template delimiters, change the
    // following template settings to use alternative delimiters.
    _.templateSettings = {
        evaluate: /<%([\s\S]+?)%>/g,
        interpolate: /<%=([\s\S]+?)%>/g,
        escape: /<%-([\s\S]+?)%>/g
    };

    // When customizing `templateSettings`, if you don't want to define an
    // interpolation, evaluation or escaping regex, we need one that is
    // guaranteed not to match.
    var noMatch = /(.)^/;

    // Certain characters need to be escaped so that they can be put into a
    // string literal.
    var escapes = {
        "'": "'",
        '\\': '\\',
        '\r': 'r',
        '\n': 'n',
        '\u2028': 'u2028',
        '\u2029': 'u2029'
    };

    var escaper = /\\|'|\r|\n|\u2028|\u2029/g;

    var escapeChar = function(match) {
        return '\\' + escapes[match];
    };

    // JavaScript micro-templating, similar to John Resig's implementation.
    // Underscore templating handles arbitrary delimiters, preserves whitespace,
    // and correctly escapes quotes within interpolated code.
    _.template = function(text, data, settings) {
        settings = _.defaults({}, settings, _.templateSettings);

        // Combine delimiters into one regular expression via alternation.
        var matcher = new RegExp([
            (settings.escape || noMatch).source,
            (settings.interpolate || noMatch).source,
            (settings.evaluate || noMatch).source
        ].join('|') + '|$', 'g');

        // Compile the template source, escaping string literals appropriately.
        var index = 0;
        var source = "__p+='";
        text.replace(matcher, function(match, escape, interpolate, evaluate, offset) {
            source += text.slice(index, offset).replace(escaper, escapeChar);
            index = offset + match.length;

            if (escape) {
                source += "'+\n((__t=(" + escape + "))==null?'':_.escape(__t))+\n'";
            } else if (interpolate) {
                source += "'+\n((__t=(" + interpolate + "))==null?'':__t)+\n'";
            } else if (evaluate) {
                source += "';\n" + evaluate + "\n__p+='";
            }

            // Adobe VMs need the match returned to produce the correct offest.
            return match;
        });
        source += "';\n";

        // If a variable is not specified, place data values in local scope.
        if (!settings.variable) source = 'with(obj||{}){\n' + source + '}\n';

        source = "var __t,__p='',__j=Array.prototype.join," +
            "print=function(){__p+=__j.call(arguments,'');};\n" +
            source + "return __p;\n";

        try {
            var render = new Function(settings.variable || 'obj', '_', source);
        } catch (e) {
            e.source = source;
            throw e;
        }

        if (data) return render(data, _);
        var template = function(data) {
            return render.call(this, data, _);
        };

        // Provide the compiled source as a convenience for precompilation.
        var argument = settings.variable || 'obj';
        template.source = 'function(' + argument + '){\n' + source + '}';

        return template;
    };

    // Add a "chain" function, which will delegate to the wrapper.
    _.chain = function(obj) {
        return _(obj).chain();
    };

    // OOP
    // ---------------
    // If Underscore is called as a function, it returns a wrapped object that
    // can be used OO-style. This wrapper holds altered versions of all the
    // underscore functions. Wrapped objects may be chained.

    // Helper function to continue chaining intermediate results.
    var result = function(obj) {
        return this._chain ? _(obj).chain() : obj;
    };

    // Add all of the Underscore functions to the wrapper object.
    _.mixin(_);

    // Add all mutator Array functions to the wrapper.
    _.each(['pop', 'push', 'reverse', 'shift', 'sort', 'splice', 'unshift'], function(name) {
        var method = ArrayProto[name];
        _.prototype[name] = function() {
            var obj = this._wrapped;
            method.apply(obj, arguments);
            if ((name == 'shift' || name == 'splice') && obj.length === 0) delete obj[0];
            return result.call(this, obj);
        };
    });

    // Add all accessor Array functions to the wrapper.
    _.each(['concat', 'join', 'slice'], function(name) {
        var method = ArrayProto[name];
        _.prototype[name] = function() {
            return result.call(this, method.apply(this._wrapped, arguments));
        };
    });

    _.extend(_.prototype, {

        // Start chaining a wrapped Underscore object.
        chain: function() {
            this._chain = true;
            return this;
        },

        // Extracts the result from a wrapped and chained object.
        value: function() {
            return this._wrapped;
        }

    });

    // AMD registration happens at the end for compatibility with AMD loaders
    // that may not enforce next-turn semantics on modules. Even though general
    // practice for AMD registration is to be anonymous, underscore registers
    // as a named module because, like jQuery, it is a base library that is
    // popular enough to be bundled in a third party lib, but not be part of
    // an AMD load request. Those cases could generate an error when an
    // anonymous define() is called outside of a loader request.
    if (typeof define === 'function' && define.amd) {
        define('underscore', [], function() {
            return _;
        });
    }
}).call(this);;

